Provable Multi-Task Representation Learning by Two-Layer ReLU Neural Networks

An increasingly popular machine learning paradigm is to pretrain a neural network (NN) on many tasks offline, then adapt it to downstream tasks, often by re-training only the last linear layer of the network. This approach yields strong downstream performance in a variety of contexts, demonstrating that multitask pretraining leads to effective feature learning. Although several recent theoretical studies have shown that shallow NNs learn meaningful features when either (i) they are trained on a {\em single} task or (ii) they are {\em linear}, very little is known about the closer-to-practice case of {\em nonlinear} NNs trained on {\em multiple} tasks. In this work, we present the first results proving that feature learning occurs during training with a nonlinear model on multiple tasks. Our key insight is that multi-task pretraining induces a pseudo-contrastive loss that favors representations that align points that typically have the same label across tasks. Using this observation, we show that when the tasks are binary classification tasks with labels depending on the projection of the data onto an $r$-dimensional subspace within the $d\gg r$-dimensional input space, a simple gradient-based multitask learning algorithm on a two-layer ReLU NN recovers this projection, allowing for generalization to downstream tasks with sample and neuron complexity independent of $d$. In contrast, we show that with high probability over the draw of a single task, training on this single task cannot guarantee to learn all $r$ ground-truth features.

==> Experiments.tex <==
% \section{Experiments}


% % future experiments: test that federated learning alg that warm-starts the head

% In this section we empirically validate our theoretical findings on synthetic data. Here we relax some of the assumptions 

% (1) necessity of adapting head: two easy tasks, adapting works, gd fails, shown by both training trajectory and downstream performance

% (2) necessity of task balancedness assumption

% (3) FedAvg/Local GD is a noisy approximation of MTRL.

% We set $r=2$ and $d=10$. 
% choices: how to update ai

% \textbf{Relaxation of assumptions.} Behavior of MTRL is similar for finite tasks, finite samples per task, and multiple steps of updating the model weights.

% \textbf{The manner in which MTRL learns extends to other simple MTL algorithms.}  FedAvg/Local GD is a noisy approximation of MTRL. Adapting the heads is critical.

% \textbf{SMGD indeed fails.}

% show plot of features moving outwards

% \begin{figure}
%   \centering
%   % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%    \includegraphics[width=0.4\linewidth]{mtpara.pdf}
%   % \fbox{\rule[-.5cm]{0cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%    \includegraphics[width=0.4\linewidth]{mtperp.pdf}
%   \caption{$r=2$, $d=10$, $m=4$}
% \end{figure}

==> Formulation-ICML.tex <==
\section{Formulation} \label{sec:formulation}

% Instead of the previous Gaussian input data model, let us 


In this section, we formally define the multi-task learning problem and the algorithms analyzed in Section \ref{sec:results}. Our motivation is drawn from classification problems where the input data for all tasks share a common representation, i.e. a small set of features that determine their labels. However, the mapping from these features to labels varies across tasks. Ultimately, the goal of the multi-task learner is to leverage the large set of pretraining tasks to learn a representation that captures the small set of label-relevant features, thereby enabling strong performance on downstream tasks.



\subsection{Pretraining tasks and data generating model} 

We consider pretraining on a set of $T$ binary classification tasks, each drawn independently from a distribution $\mathcal{T}$ over tasks. All these tasks share a common characteristic: their labeling function depends solely on a projection of the input features onto a low-dimensional subspace. Specifically, each task $i$ consists of a distribution $\mathcal{D}_i$ on $\mathcal{X}\times \mathcal{Y}$, where the input space is $\mathcal{X}=\mathbb{R}^d$ and the label space is $\mathcal{Y}= \{-1,1\}$.
% Following \citep{damian2022neural,shi2022theoretical,} we consider that the labelling function for each task $i$ is a function of a linear projection of the input data onto a low-dimensional subspace. % In particular, 
% the sign of the first {$r$} coordinates of $\mathbf{x}$, denoted by $\mathbf{x}_{:r}$. 
% More precisely, 
Samples are drawn from $\mathcal{D}_i$ by first selecting a Gaussian feature vector $\mathbf{x} \in \mathcal{X}$, then computing its label $f_i(\mathbf{x}) \in \mathcal{Y}$ as follows:
% The labelling function for task $i$, denoted by $f_i:\mathcal{X} \to\mathcal{Y}  $, is a composition of a low-dimensional linear projection then for any sample $\mathbf{x} \in \mathcal{X}$, where here we assume $\mathbf{x}$ is drawn from the standard Gaussian distribution, we have 
\begin{equation} \label{eq1}
    \mathbf{x}\sim \mathcal{N}(\mathbf{0}_d,\mathbf{I}_d);  \;\;  f_i(\mathbf{x}) = {g}_i(\sign(\mathbf{M}\mathbf{x})) \in \{-1,1\}. 
\end{equation}
Here, $\mathbf{M} \coloneqq [\mathbf{m}_1,\dots, \mathbf{m}_r]^\top \in \mathbb{R}^{r \times d}$ is a matrix with orthonormal rows that captures the $r$ label-relevant features $(\sign(\mathbf{m}_1^\top\mathbf{x}),\dots, \sign(\mathbf{m}_r^\top\mathbf{x}))$ in $\mathbf{x}$, and  ${g}_i: \mathcal{H}^{r} \rightarrow \{-1,1\}$ is the ground-truth link function for task $i$ that maps vertices on the $r$-dimensional Rademacher hypercube to binary labels.  To model shared information across the tasks, we assume that $r\ll d$. Thus, the complexity of solving a new task can be drastically reduced by learning an appropriate low-dimensional projection onto the row space of $\mathbf{M}$. 
% This paradigm of learning a low-dimensional set of data features is common in learning theory, and the matrix $\mathbf{M}$ is  
The question we ask here is whether gradient-based multi-task pretraining can  efficiently recover the $r$ label-relevant features expressed by $\mathbf{M}$.
% We let $\mathcal{D}_i$ denote the joint distribution over pairs $(\mathbf{x}, f_{i}^\ast(\mathbf{x}))$ generated as above for task $i$.
% A finite number of samples drawn from $\mathcal{D}_i$ are available for training on each task.

This setting is similar to the sparse coding model studied by \citet{shi2022theoretical}, except  we assume the input data is continuous in $\mathbb{R}^d$, while  \citet{shi2022theoretical} assume the input data is on the hypercube $\mathcal{H}^d$. By assuming that the labelling function is a function of ``sign'' of the $r$ ground-truth features, we make our model more similar to the one in \cite{shi2022theoretical}, as they assume the label for each task is a function of the first $r$ coordinates of the integer input data. 

% \textcolor{blue}{not sure I understand this: $\mathbf{z}_{:r}$ is independently generated from $\mathbf{M}$, so it seems that the previous sentence should be revised. I.e. the label only depends on $\mathbf{z}_{:r}$ and not the columns of $\mathbf{M}$. }
%Our setting is similar to the sparse coding model studied by \cite{shi2022theoretical}, except that our latent vectors are Gaussian, rather than being vertices on the hypercube $\{-1,1\}^d$.   Formally, in our setting labeled points 
 %for any task $ \in \mathcal{T}$ are sampled from $\mathcal{D}_i$ as follows


%Thus, the first $r$ coordinates of $\mathbf{z} = \mathbf{M}^\top\mathbf{x}$ determine the labels for the $i$-th task according to the ground-truth labelling function $\bar{f}_{i}^\ast: \{-1, 1\}^{r}\rightarrow \{-1,1\}$, while the remaining $k-r$ coordinates of $\mathbf{z}$ are spurious. So, the data can be projected onto the low-dimensional space $\text{col}(\mathbf{M}_{:r})$ and preserve all information relevant to its label, for all tasks in $\mathcal{T}$. We let $\bar{\mathcal{T}} \coloneqq \{\bar{f}_{i}^\ast : \mathcal{D}_i \in \mathcal{T}\}$  denote the collection of ground-truth labelling functions corresponding to tasks in $\mathcal{T}$.
% \textcolor{blue}{this good (i.e. explaining what's the signal and what's the spurious features; I would add more of these high-level sentences in te paragraph above)}

% \textcolor{blue}{can you (briefly) mention the advantages of your model compared to the previous sparse coding ones?}
% Our setting allows the latent variables to 

Critically, the set of label-relevant coordinates of the input data are shared among all tasks, while the link functions $g_i$ mapping from these coordinates to labels are specific to each task. Thus, the goal of the multi-task learner is to recover the shared label-relevant features, so that it may solve a downstream task with complexity scaling only with the number $r$ of label-relevant features, rather than the much larger ambient dimension of the data $d$.
This model draws inspiration from classification tasks in which labels are functions of the presence (or lack thereof) of a small number of features in the data. For example, whether or not a brain MRI reveals cancerous tissue depends on the presence of tumor-shaped structures in the image, indicated by a small number of features relative to the MRI dimension. 

% While prior work has used such settings to motivate studying the dynamics of neural network training with a similar data model with discrete input vectors in the single-task setting \citep{shi2022theoretical,wen2021toward},
% % However, in the sparse coding model the latent variables are either on the Rademacher hypercube $\{-1,1\}^d$ or in the set $\{-1,0,1\}^d$, rather than being Gaussian samples in $\mathbb{R}^d$. 
% our model captures more general scenarios in which features appear in the data on a continuous spectrum, while the label is a quantization of these continuous features.

% is common among all tasks, meaning the input data across all tasks shares both spurious and label-relevant features, however the mapping from label-relevant features to labels differs across tasks. 

% . However, it is not clear how this is possible  since  the spurious features dominate the ground-truth features in $\mathbf{x}$ (that is, ${\|\mathbf{M}_{r:}^\top\mathbf{x}\|_2^2} = \hat{\Omega}\left(\frac{k-r}{r}\right){\|\mathbf{M}_{:r}^\top\mathbf{x}\|_2^2}$ with high probability).
% \textcolor{blue}{it might be good to write explicitly somewhere that $k >> r$; Right now you just use the word ``outweigh'' at some point. }


More formally, the generative model in \eqref{eq1} implies that, for any task, the sample labels are a function of the projection of the data onto the $r$ ground-truth features in $\mathbf{M}$. We use $\mathcal{T}$ to denote the distribution over link functions $g_i:\mathcal{H}^r\rightarrow \{-1,1\}$, and $\mathcal{T}(\mathbf{M})$ to denote the distribution over functions mapping from $\mathbb{R}^d\rightarrow \{-1,1\}$, i.e. the distribution over $f_i$, where $f_i(\mathbf{x})= g_i(\sign(\mathbf{Mx}))$ and $g_i \sim \mathcal{T}$. 

However, in order to recover {\em all} the $r$ ground-truth features,  it is not sufficient that the labels simply depend on the $r$ ground-truth features -- they must depend on {\em all} of them in aggregate across tasks. For example, if the labels for all tasks can be written as functions of only the projection of the inputs onto the first $r-1$ rows of $\mathbf{M}$, there is no hope to recover the $r$-th row of $\mathbf{M}$. Thus, the tasks must be ``diverse'' in the sense that in aggregate they depend on {\em all} ground-truth features. 
% but rather they depend on {\em all} of the features in aggregate across tasks. To this aim we impose a condition that can be interpreted as task diversity.
%% ...  it must be the case that the other $d-r$ coordinates are spurious. 
% For this to be the case we must make a further assumption on the collection of tasks $\mathcal{T}$. 
% Next we give two examples of collections of labelling functions that satisfy Assumption 3.1.
% An example  of a collection of tasks that satisfies Assumption 3.1 is the collection of all possible labellings of $2^r$ inputs.
%% This can be captured by considering that 

To formalize this idea, we 
make the following assumption on the distribution of task link functions $\mathcal{T}$. 
Our condition entails 
that for any pair of points with different sign patterns on their $r$ label-relevant features, it is equally likely for them to have the same label as it is for them to have different labels on a task link function drawn from $\mathcal{T}$. 
% Next we formalize this assumption. 
\begin{assumption}\label{assump:diversity}
For any two points $\mathbf{z},\mathbf{z}'\in \mathcal{H}^r$ such that $\mathbf{z}\neq \mathbf{z}'$,
% $\sign(\mathbf{Mx})\neq \sign( \mathbf{Mx}')$, % and $\mathbf{v}\neq -\mathbf{v}'$,
% $\sign(\mathbf{M}_{:r}^\top\mathbf{x}) \neq \sign(\mathbf{M}_{:r}^\top\mathbf{x}')$ and $\sign(\mathbf{M}_{:r}^\top\mathbf{x}) \neq -\sign(\mathbf{M}_{:r}^\top\mathbf{x}')$, 
the probability that the labels of $\mathbf{z}$ and $\mathbf{z}'$ are the same for a task link function drawn from ${\mathcal{T}}$  satisfies: %, for some $\delta \in [0,\tfrac{1}{2})$:
\begin{align}
       % \tfrac{1}{2} - \delta \leq 
       \Pr_{i \sim {\mathcal{T}}} \left[ {g}_i(\mathbf{z}) = {g}_i( \mathbf{z}')  \right]& 
    % \begin{cases} =  1  & \text{if} \; \sign(\mathbf{M}_{:r}^\top\mathbf{x}) = \sign(\mathbf{M}_{:r}^\top\mathbf{x}') \\
    = \tfrac{1}{2}. \label{onehalff}
    % + \delta \nonumber
    % & \text{otherwise} \\
    % \end{cases}
\end{align}
\end{assumption}
\vspace{-2mm}
Assumption \ref{assump:diversity} is necessary to  ensure the task link functions depend equally on all inputs. To see this, suppose that all pairs of inputs $\mathbf{z},\mathbf{z}'$ with identical first $r-1$ coordinates but differing $r$-th coordinates had the same labels, i.e. $\Pr_{i \sim {\mathcal{T}}} \left[ {g}_i(\mathbf{z}) = {g}_i( \mathbf{z}')  \right]
    = 1. $ Then, all link functions in the support of $\mathcal{T}$ would in fact only depend on the first $r-1$ input coordinates, rather than all $r$ inputs. So, we need $\Pr_{i } \left[ {g}_i(\mathbf{z}) = {g}_i( \mathbf{z}')  \right] <1$ for some dependence on all inputs. We make a stronger  assumption of $\frac{1}{2}$ in the RHS of \eqref{onehalff} that  ensures perfectly  balanced  dependence  across all inputs. We note that our results do not strictly require perfect balance, rather it is useful for ease of exposition\footnote{Our results hold for {\em finitely-many} tasks drawn for training, so the empirical distribution of tasks does not assign equal importance to each of the $r$ input features, in the sense that Assumption \ref{assump:diversity} does not hold exactly on the empirical task distribution. This implies that our results can extend to cases in which the population distribution of tasks $\mathcal{T}$ does not satisfy Assumption \ref{assump:diversity} exactly, i.e. we can tolerate $\Pr_{i \sim {\mathcal{T}}} \left[ {g}_i(\sign(\mathbf{Mx})) = {g}_i( \sign(\mathbf{Mx}'))  \right] \leq \frac{1}{2} + \epsilon$ for some small $\epsilon>0$.}.
    
    Another interpretation of Assumption \ref{assump:diversity} is that it enforces that the correlation of the labels of $\mathbf{z}$ and $\mathbf{z}'$ across tasks, i.e. $\E_{i \sim {\mathcal{T}}} \left[ {g}_i(\mathbf{z}) {g}_i( \mathbf{z}')  \right]$, is 1 if $\mathbf{z}=\mathbf{z}'$, and 0 otherwise. In other words, the label correlation of $\mathbf{x}$ and $\mathbf{x}'$ across tasks is 1 if the ground-truth features of $\mathbf{x}$ and $\mathbf{x}'$ are the same, and 0 otherwise. 
    % This is a special case of the more general, informal, and very natural condition that 
    We will show in  Section \ref{sec:sketch} intuitively why the correlation of the labels  of $\mathbf{x}$ and $\mathbf{x}'$  need only be ``roughly''
 increasing with the similarity of the ground-truth features in   $\mathbf{x}$ and $\mathbf{x}'$, a very natural condition,  for gradient-based multi-task training to recover $\text{row}(\mathbf{M})$.
% requires that the task distribution is sufficiently well-balanced to 
% to not convey any label bias towards any pair of inputs that differ on the ground-truth features -- all pairs of inputs with differing sign patterns on the ground-truth features are equally likely to have the same label as they are to have different labels.
For now, we describe two examples of task distributions that satisfy Assumption \ref{assump:diversity}.

% \textcolor{blue}{HH: I feel that these examples should appear earlier, e.g. before the paragraph starting with "However, .." Or maybe you'll need a running example to better illustrate the distributions and the shared features. }
% Since in all cases all tasks differ only by their link functions ${g}_{i}$, we formally define the task distribution $\mathcal{T}$ as a distribution over link functions $g_i: \mathcal{H}^r\rightarrow\{-1,1\}$, whereas $\mathcal{T}(\mathbf{M})$ is implicitly defined as the distribution over functions $f_i(\mathbf{x}) = g_i(\sign(\mathbf{Mx})), g_i \sim \mathcal{T}$.
% \begin{itemize}[leftmargin=3mm]
    % \item \textbf{Uniform distribution over separating hyperplanes through the origin.} Here we consider tasks with labels determined by whether the projected input lies in a particular halfspace. That is, $\mathcal{T}_{\text{half}} \coloneqq \text{Unif}(\{ g_i: g_i(\mathbf{v}) = \sign(\boldsymbol{\theta}_i^\top \mathbf{v}  ) \text{ for all }\mathbf{v}\in \mathcal{H}^r, \; \text{for some } \boldsymbol{\theta}_i\in \mathbb{S}^{r-1} \})$.
    % \item 
    
    \textbf{Example 1: Uniform distribution over all tasks.} Here we have $\mathcal{T}=\mathcal{T}_{\text{all}}$, where 
    \begin{align}
     \vspace{-2mm}
        \mathcal{T}_{\text{all}} \coloneqq \text{Unif}(\{ g_i: \mathcal{H}^r \rightarrow \{-1,1\} \}),
    \end{align}
     % \vspace{-2mm}
    % \vspace{-2mm}
    i.e.  $\mathcal{T}_{\text{all}}$ is the uniform distribution over all possible mappings from the $r$-dimensional $\pm 1$ hypercube to $\{-1,1\}.$
    % \item 



    \textbf{Example 2: Uniform distribution over all sparse parity tasks.} {\em Sparse parity} tasks are a well-studied class of tasks in which the label is the parity of a subset of the number of $-1$'s among a particular subset of input bits \cite{kearns1998efficient}. In this case we have $\mathcal{T}= \mathcal{T}_{\text{s.p.}}$, where $ \mathcal{T}_{\text{s.p.}}$ is the uniform distribution over parity functions on $r$ input bits, formally defined as follows:
    \begin{align}
    \vspace{-2mm}
        \mathcal{T}_{\text{s.p.}} \coloneqq &\;\text{Unif}(\{ g_i: g_i(\mathbf{z}) = (-1)^{\sum_{j \in \mathcal{S}_i} \chi\{{z}_j = -1\}},\nonumber \\
        &\quad\quad \quad \quad \;\; \mathcal{S}_i \subseteq [r],\; \forall \; \mathbf{z}\in \mathcal{H}^r  \}).\label{sparsepar}
        \vspace{-2mm}
    \end{align}
    Both $\mathcal{T}_{\text{all}}$ and $\mathcal{T}_{\text{s.p.}}$ effectively assign equal importance to all $r$ inputs, so they naturally satisfy Assumption \ref{assump:diversity} (please see Appendix \ref{app:sec:dists} for proofs). 
    %With that being said, 
    % Our results show that the more tasks we observe during training
% \end{itemize}
% Note: we can also include the case of linear tasks. but this requires new proofs. note perp matrices will be zero.


%and assuming that the pair is equally-likely to share a label on a task drawn from $\mathcal{T}$ as it is to have different labels (the values of the $d-r$ spurious coordinates provide no information about whether the pair is likely to share a label).
% The interpretation of the above assumption as task diversity follows from the observation that
%% For example, 
% Note that \ref{assump:diversity}  rules out the possibility of most tasks labelling most inputs the same, which would cloud the importance of the $r$ ground-truth features. For example, 
% if all tasks labelled all inputs as `1', then it would be impossible to recover the $r$ ground-truth features, since they are irrelevant to the label for all tasks. 

%%%%%%%%%
% Assumption \ref{assump:diversity} enforces task diversity by ensuring that all pairs of distinct sign inputs are equally likely to have distinct labels as not -- i.e. there is no subset of the $r$ coordinates that is more indicative of the inputs sharing a label than the other coordinates. Such an assumption is necessary because, in the extreme case, if all tasks could be written as functions of only the first coordinate, it would be impossible to recover the remaining $r-1$ coordinates. Thus, we need the collection of possible training tasks to be sufficiently diverse such that all $r$ coordinates are equally relevant to the label, on average across tasks (i.e. one coordinate may be irrelevant to the label for some task, but it must be relevant for others). We note that, strict equality in the assumption is not necessary, but made for convenience. Indeed, we only sample $T <\infty$ tasks from $\mathcal{T}$ for training, so our empirical task distribution is not guaranteed to satisfy Assumption \ref{assump:diversity} with strict equality. To satisfy the assumption, we can set $\mathcal{T}$ to be the set of all possible labellings of the $2^r$ inputs on the $r$-dimensional hypercube, noting that our results do not require $T$ to scale with $\mathcal{T}$.
%%%%%%%%

% Assumption \ref{assump:diversity} enforces both of 
% Observe that if all tasks label all inputs as '1', then no coordinate is relevant to the label and $\Pr_{i \sim \Unif({\mathcal{T}})} \left[ \bar{f}_i^*(\sign(\mathbf{x}_{:r})) = \bar{f}_i^*( \sign(\mathbf{x}_{:r}'))  \right]=1$ for all $\mathbf{x}\neq \mathbf{x}'$, while if the tasks only depend on the first coordinate, $\Pr_{i \sim \Unif({\mathcal{T}})} \left[ \bar{f}_i^*(\sign(\mathbf{x}_{:r})) = \bar{f}_i^*( \sign(\mathbf{x}_{:r}'))  \right]=1$ for all $\mathbf{x}, \mathbf{x}'$ with the same sign on the first coordinate. 


% Assumption \ref{assump:diversity} states that if two data points do not share signs of ground-truth features, then they are just as likely to share a label on a random task as they are to have differing labels. 
% % almost as likely to share a label on a random task as they are to have differing labels, up to $\delta$ error. 
% On the other hand, the data generative model implies that if two points do share the same sign pattern for the ground-truth features, then they share the same label  on a random task with probability one.
% This means that the only information that predicts whether two points will have the same label on a random task is the sign pattern of their ground-truth features -- the spurious features do not convey any such information.



% For pretraining, the multi-task learner draws $T$ tasks  uniformly at random from $\mathcal{T}$, where possibly $T \ll |\mathcal{T}|$. We make only one assumption on the 
% % collection of ground-truth labelling functions $\bar{\mathcal{T}}$ corresponding to the 
% collection of tasks $\mathcal{T}$. 
% \textcolor{blue}{is there a difference between $\bar{\mathcal{T}}$ and $\mathcal{T}$? Can we use $\mathcal{T}$ for both with some slight abuse of notation? Also, we have $f$ and $\bar{f}$; can we simplify this notation somehow (not sure if the two are very different)?} 
% Nevertheless, we show that head-adaptive algorithms can learn the ground-truth features as long as a simple assumption on the tasks $\mathcal{T}$ is satisfied. For ease of notation we use $i\sim \Unif(\mathcal{T})$ to denote drawing a task $\mathcal{D}_i$ uniformly at random from $\mathcal{T}$. 


% , i.e. $\bar{\mathcal{T}} \coloneqq \{ \bar{f}_i^*:\{-1,1\}^r \rightarrow \{-1,1\} \} $. 
% The strict $1/2$ requirement can be removed to include additional task collections, but we 

% \textbf{Example 1: All possible labellings of $2^r$ inputs.} Here $\bar{\mathcal{T}} \coloneqq \{ \bar{f}_i^*:\{-1,1\}^r \rightarrow \{-1,1\} \} $ is analogous to the power set on $r$ elements. Although in this case $|\bar{\mathcal{T}}|= 2^{2^r}$, we show in Theorem \ref{thm:1} that multi-task learning can still learn meaningful features when $n$ scales only exponentially with $r$. 

% {\color{gray}
% \textbf{Example 2: Parities on subsets of $[r]$.} Here $\bar{\mathcal{T}} \coloneqq \{ \bar{f}_i^*:\{-1,1\}^r \rightarrow \{-1,1\} | \bar{f}_i^*(\mathbf{v}) = \prod_{j \in A} v_j, \; A \subseteq [r] \} $. In this case, each $\bar{f}_i^*\in \bar{\mathcal{T}}$ outputs the parity of the input bits on a subset $A$ of the first $r$ bits. In other words, each task is a sparse parity problem, which has received much attention in studies of single task feature learning \cite{daniely2020learning,shi2022theoretical,frei2022random}. Unlike prior work, we show in the subsequent section that pretraining on many sparse parity tasks allows the network to learn features that generalize beyond sparse parity tasks.}

% Assumption 3.1 is satisfied if $\mathcal{T}$  consists of all binary labellings of $2^r$ inputs.
% We call this a ``task diversity'' assumption because it entails that the tasks must be diverse enough to rule out correlations between spurious features and labels.

% For pretraining,  we make no further assumptions on the ground-truth labelling functions $f_{i}^\ast$, meaning they can be arbitrarily complex. For downstream guarantees, we need to ensure that any downstream $f_{i'}^\ast$ must be implementable by the learning model, which we discuss later.
% \textcolor{blue}{this paragraph is a bit vague at this moment (and it might be unnecessary), so maybe you want to move it down}

\subsection{Learning model and loss}  We consider multi-task pretraining of a two-layer neural network $\hat{y}(\cdot) = \hat{y}(\cdot; \mathbf{W},\mathbf{b},\mathbf{a}):\mathbb{R}^d\rightarrow \mathbb{R}$ with $m$ ReLU  neurons in the hidden layer, namely
\begin{align}
\vspace{-1mm}
  \hat{y}(\mathbf{x}) = \hat{y}(\mathbf{x}; \mathbf{W},\mathbf{b},\mathbf{a}) := \sum_{j=1}^m a_j \sigma (\mathbf{w}_j^\top \mathbf{x} + b_j)
  \vspace{-1mm}
\end{align}
where $\sigma(\mathbf{x})=\max(\mathbf{x},\mathbf{0})$ element-wise, $\mathbf{w}_j \in \mathbb{R}^d$ and $b_j \in \mathbb{R}$ are the weight vector and bias for the $j$-th neuron, respectively, and $a_j\in \mathbb{R}$ is the last-layer weight for the $j$-th neuron. We let $\mathbf{W} = [\w_1,\dots,\w_m]\in \mathbb{R}^{d \times m}$ denote the matrix of concatenated weight vectors, $\mathbf{b}=[b_1,\dots,b_m]\in \mathbb{R}^m$ denote the vector of biases, and $\mathbf{a}= [a_1,\dots,a_m] \in \mathbb{R}^m$ denote the vector of last-layer weights, which we call the head. 
% Solving a task $i$ entails that predictions $f(\mathbf{x}; \mathbf{W},\mathbf{b},\mathbf{a}) $ align well with the corresponding label $f_i(\mathbf{x})$ of $\mathbf{x}$, which 
We use the hinge loss to measure the accuracy of the predictions of this model:
\begin{align} %\label{eq:hingeloss}
    \ell(\hat{y}(\mathbf{x}), f_i(\mathbf{x})):= \max\big(1 - f_i(\mathbf{x}) \hat{y}(\mathbf{x}), 0\big), \nonumber 
\end{align}
% \textcolor{blue}{why does the regularization appear in the individual loss for each data point? It might be better o add the regularization terms at the end to the some of the losses over all the data points (like structural ERM). I know what you're doing is equivalent. }  
% Let $\mathcal{D}_i$ denote the distribution over labelled pairs $(\mathbf{x},f_i(\mathbf{x}))$ for task $i$. 
and for each task $i$, we define %the empirical loss on a finite dataset $\hat{\mathcal{D}}_i$ drawn from $\mathcal{D}_i$
% for task $i$ as functions of the model parameters $(\mathbf{W},\mathbf{b},\mathbf{a})$ 
% as follows:
% the average point-wise loss over labelled points $(\mathbf{x},f_i(\mathbf{x}))$ drawn from $\mathcal{D}_i$:
% , plus $\ell_2$ regularization:
\begin{align}
     \mathcal{L}_i(\mathbf{W},\mathbf{b},\mathbf{a}) &:=  \mathbb{E}_{(\mathbf{x},f_i(\mathbf{x}))\sim \mathcal{D}_i}\left[ \ell(
     \hat{y}(\mathbf{x}), 
     % f(\mathbf{x};\mathbf{W},\mathbf{b},\mathbf{a}), 
     f_i(\mathbf{x})) \right]  \nonumber \\
     \hat{\mathcal{L}}_i(\mathbf{W},\mathbf{b},\mathbf{a}; \hat{\mathcal{D}}_i) &:= \frac{1}{|\hat{\mathcal{D}}_i|}\sum_{(\mathbf{x},f_i(\mathbf{x}))\in \hat{\mathcal{D}}_i}  \ell(
     \hat{y}(\mathbf{x}), 
     % f(\mathbf{x};\mathbf{W},\mathbf{b},\mathbf{a}), 
     f_i(\mathbf{x})) \nonumber 
     \vspace{-1mm}
     % + \frac{\lambda_{\mathbf{a}}}{2} \|\mathbf{a}\|_2^2 +  \frac{\lambda_{\mathbf{w}}}{2} \|\mathbf{W}\|_F^2, 
\end{align}
%{\color{red}{well I am not sure if you ever use the loss $\hat{\mathcal{L}}_i$ in the paper.}}
as the population loss on $\mathcal{D}_i$ and empirical loss on a finite dataset $\hat{\mathcal{D}}_i$ drawn from $\mathcal{D}_i$, respectively.
Ultimately, the goal of multi-task pretraining is to learn a first-layer representation that generalizes to downstream tasks, in the sense that we can easily train a new classifier
% , task-specific head $\mathbf{a}_{n+1}$ 
on top of the first layer in order to achieve small task-specific loss.
% $\mathcal{L}_{n+1}(\mathbf{W},\mathbf{b},\mathbf{a})$. 
To this end, we consider optimizing the following multi-task objective:
% The global loss is the average loss on each task: , plus $\ell_2$ regularization of the weights and head
\begin{align}&\min_{\mathbf{W},\mathbf{b}, \{\mathbf{a}_1, \dots, \mathbf{a}_T\}}
 {\mathcal{L}}(\mathbf{W},\mathbf{b},\{\mathbf{a}_i\}_{i=1}^T ) \nonumber \\
 &:= \frac{1}{T}\sum_{i=1}^T  {\mathcal{L}}_i(\mathbf{W},\mathbf{b},\mathbf{a}_i)  +   \frac{\lambda_{\mathbf{a}}}{2} \|\mathbf{a}_i\|_2^2 +  \frac{\lambda_{\mathbf{w}}}{2} \|\mathbf{W}\|_F^2  \label{obj_glob_i},
 \vspace{-1mm}
\end{align}
where $\lambda_{\mathbf{a}}$ and $\lambda_{\w}$ are regularization parameters. 
% Optimizing $ \mathcal{L}_{\text{SM}}$ entails learning a single model that minimizes the average loss across tasks, arguably the simplest approach to multi-task learning.
% and is common in multi-task settings such as federated learning \citep{mcmahan2017communication,karimireddy2020scaffold}.
Optimizing $\mathcal{L}$ entails learning task-specific heads on top of a shared representation, a widely used and empirically successful approach to multi-task learning \citep{zhang2021survey,crawshaw2020multi,ruder2017overview}. By optimizing the above problem, we hope to find a $\mathbf{W}$ that projects input data onto the row space of $\mathbf{M}$ and thus captures all $r$ label-relevant features, while disregarding all other spurious features.
% a set of $(\mathbf{W},\mathbf{b})$ that learn the label-relevant features and we can argue that the output of first layer 
% denoted by $[\sigma (\mathbf{w}_1^\top \mathbf{x} + b_1),\dots, \sigma (\mathbf{w}_m^\top \mathbf{x} + b_m)]\in \mathbb{R}^m$ 
% only contains information about the first $r$ coordinates of $\mathbf{x}$. 
However, we cannot access $\mathcal{L}$ directly, and instead must approximate it via stochastic queries of finite samples from each $\mathcal{D}_i$.
So,  we will use the gradient of $\hat{\mathcal{L}}_i$ instead of $\mathcal{L}$ to update the variables, 
as we discuss next. 
%\textcolor{blue}{maybe discuss very briefly here what the actual optimization problem is? I.e. you'd like to minimize the above loss over the choice of the representation $W$ and the task-specific heads $a_i$'s. How is $b$ chosen?}

% {\color{red} finite sample loss}
% \cite{shi2022theoretical} showed that running GD on the one-task population loss causes all neurons to go to $\propto  \sum_{l=1}^r \mathbf{M}_{l}$. This allows it to learn the task iff $g$ depends on $\boldsymbol{\phi}^{(:r)}$ only through $\sum_{l=1}^r \phi^{(l)}$. We would like to learn the features themselves in order to enable learning a larger class of functions.

% Our key assumption on the tasks that enables  
% concern: people will say that lower bound depends fundamentally on GD, SGD might work
% \cite{wen2021toward}

% We are motivated by \cite{shi2022theoretical}, who considered this model and showed that GD learns the average of the important features. Feature learning requires that we learn the important features themselves, not their average. Learning the average of the features seems to be a flaw inherent to GD in this setting, not their analysis. 
% so there is hope that multi-tasking/head diversity can allow for learning individual features and proving that GD cannot learn them.

% Specifically, the model is:

% Fix some column-orthonormal dictionary matrix $\mathbf{M}\in \mathbb{R}^{d \times k}$. The $j$-th sample for task $i$ is generated as:
% \begin{align}
%     \boldsymbol{\phi}_{i,j} \sim \{0,1\}^k, \quad \mathbf{x}_{i,j} = \mathbf{M}\boldsymbol{\phi}_{i,j}, \quad y_{i,j} = g_i(\boldsymbol{\phi}_{i,j}^{(:r)})
% \end{align}
% where $\boldsymbol{\phi}_{i,j}^{(:r)}$ denotes the first $r\leq k$ elements of $\boldsymbol{\phi}_{i,j}$. 

\subsection{Algorithm} \label{sec:alg}

\begin{comment}
We consider two pretraining algorithms that aim to learn a generalizable representation $\mathbf{W}$, described as follows.


\textbf{Pretraining Option 1: Single-Model Gradient Descent (SMGD).} SMGD runs gradient descent with step size $\eta$ on the global loss \eqref{obj_glob}. First it initializes $\mathbf{W}_0$ and $\mathbf{a}_0$ according to any initialization procedure. Then, for all rounds $t = 1,\dots,T$, it computes
\begin{align}
    \mathbf{a}_{t+1}^{\text{SMGD}} &= \mathbf{a}_{t}^{\text{SMGD}} - \eta \nabla_{\mathbf{a}} \mathcal{L}(\mathbf{W}_t^{\text{SMGD}},\mathbf{a}_t^{\text{SMGD}}); \quad \mathbf{W}_{t+1}^{\text{SMGD}} = \mathbf{W}_{t}^{\text{SMGD}} - \eta \nabla_{\mathbf{W}} \mathcal{L}(\mathbf{W}_t^{\text{SMGD}},\mathbf{a}_t^{\text{SMGD}})
\end{align}
This is the simplest multi-task learning algorithm we consider. It is also referred to Distributed Gradient Descent or simply Gradient Descent in distributed and federated settings.
\end{comment}


We consider a two-stage learning process: (1) Representation learning, in which we aim to learn effective features using $T$ available tasks, and (2) Downstream evaluation, in which we encounter a new task and aim to efficiently learn an accurate classifier on the pre-trained features. 
% We consider two different algorithms for pretraining.

% The gradient-based multi-task learning algorithm we study executes two phases: (1) a pretraining phase in which the ground-truth features are learned by training on all $n$ sampled tasks, and (2) a fine-tuning phase in which the first-layer biases are re-initialized and the head is re-trained on a single downstream task.

% \textbf{Pretraining Algorithm 1: Single-Model Gradient Descent (SMGD).} SMGD runs gradient descent with step size $\eta$ on the global loss \eqref{obj_glob}. First it initializes $\mathbf{W}_0$ and $\mathbf{a}_0$ according to any initialization procedure. Then, for all rounds $t = 1,\dots,T$, it computes
% \begin{align}
%     \mathbf{a}_{t+1}^{\text{SMGD}} &= \mathbf{a}_{t}^{\text{SMGD}} - \eta \nabla_{\mathbf{a}} \mathcal{L}(\mathbf{W}_t^{\text{SMGD}},\mathbf{a}_t^{\text{SMGD}}); \quad \mathbf{W}_{t+1}^{\text{SMGD}} = \mathbf{W}_{t}^{\text{SMGD}} - \eta \nabla_{\mathbf{W}} \mathcal{L}(\mathbf{W}_t^{\text{SMGD}},\mathbf{a}_t^{\text{SMGD}})
% \end{align}
% This is the simplest multi-task learning algorithm we consider. It is also referred to Distributed Gradient Descent or simply Gradient Descent in distributed and federated settings.







\textbf{Representation learning phase.} %Unlike SMGD, 
% \textbf{Phase 1: pretraining.}
% MTRL is the main focus of our study.
% Unlike SMGD, MTRL 
The multi-task  learning algorithm we consider aims to solve the global objective \eqref{obj_glob_i} with task-specific heads. 
% To do so, it first 
% executes a symmetric initialization, as in previous studies of feature learning \cite{damian2022neural,shi2022theoretical}. 
% For simplicity we assume $m$ is even. 
% Note that the initialization for all task heads is the same for simplicity.
We denote  the $j$-th neuron weights at initialization as $ \mathbf{w}_{j}^0  \in \mathbb{R}^d$,  and  
% $a_{i,j}^0$ as the $j$-th element of the 
 the global bias and 
head corresponding to task $i$ at time $0$ as $\mathbf{b}^0\in \mathbb{R}^m$ and $\mathbf{a}_i^0\in \mathbb{R}^m$, respectively. We initialize these parameters as: 
% We initialize the parameters corresponding to $j \leq \frac{m}{2}$ as:
\begin{align}
    \mathbf{w}_{j}^{0} \sim \mathcal{N}(\mathbf{0}_d,\nu_{\mathbf{w}}^2\mathbf{I}_d),  \quad 
    % a_{i,j}^0\sim \mathcal{N}({0},\nu_{\mathbf{a}}^2),
    \mathbf{a}_i^0 =\mathbf{0}_m,
    \quad \mathbf{b}^0=\mathbf{0}_m
    % b_{j}^{0}=0
\end{align}
where $\nu_{\mathbf{w}} \in \mathbb{R}_{\geq 0}$.
% We initialize the remaining weights (corresponding to $j>\frac{m}{2}$) as $\mathbf{w}_{j}^0 = \mathbf{w}_{j-m/2}^0,$ $b_{j}^0=0$, and $a_{i,j}^0 = -a_{i,j-m/2}^0$ for all tasks $i\in [T]$. For simplicity we assume $m$ is even. 
% randomly initializes the representation $\mathbf{W}_0^{\text{MTRL}}$. 
After initialization, we execute an alternating gradient descent-based algorithm.
We first optimize the heads, i.e., $\mathbf{a}_{1},\dots, \mathbf{a}_{T}$, with one step of stochastic gradient descent (SGD) on the corresponding task-specific empirical loss on a batch of samples $\hat{\mathcal{D}}_{i,\mathbf{a}}$ for each task $i$:
% Note that since each $\mathcal{L}_i$ is a strongly convex function with respect to $\mathbf{a}$, this optimization problem can be solved efficiently and the condition number is $1$ so that a constant number of iterations can yield a small loss. In fact,  we only run one step of gradient descent for each head on the regularized task-specific loss:
% alternates between minimization steps for the task-specific heads and gradient descent steps for the representation. 
% In particular, on round $t$, the parameters are updated as follows:
\begin{equation}
    \mathbf{a}_{i}^1 =  (1 - \eta \lambda_{\mathbf{a}})\mathbf{a}_{i}^0 -  \eta  \nabla_{\mathbf{a}} \hat{\mathcal{L}}_i(\mathbf{W}^0,\mathbf{b}^0,\mathbf{a}_i^{0}; \hat{\mathcal{D}}_{i,\mathbf{a}})
    \quad \forall \; i \in [T]. \nonumber
\end{equation}
The same number of samples is used for each task, denoted by $n_1\coloneqq |\hat{\mathcal{D}}_{i,\mathbf{a}}|$.
Next, we update the model weights $\mathbf{W}$ with one step of SGD  on the global empirical loss induced by the updated heads, with a fresh batch of samples $\hat{\mathcal{D}}_{i, \mathbf{W}}$ for each task $i$: 
\begin{align}
    % \mathbf{a}_{1,i} &\in \arg \min_{\mathbf{a}\in \mathbb{R}^m} \mathcal{L}_i(\mathbf{W}_t,\mathbf{a}) \quad \forall \; \i \in \mathcal{T}  ^{\text{MTRL}}
    \vspace{-1mm}
    \mathbf{W}^1 &= \mathbf{W}^{0} -   \frac{\eta}{T} \sum_{i=1}^T \nabla_{\mathbf{W}}   \hat{\mathcal{L}}_i(\mathbf{W}^0, \mathbf{b}^0,\mathbf{a}_{i}^1; \hat{\mathcal{D}}_{i,\mathbf{W}})  \nonumber
    \vspace{-1mm}
\end{align}
% The representation-learning abilities of AltMinGD have been previously analyzed in the federated setting \citet{collins2021exploiting}, but this analysis was limited to linear models.
% We show that only one gradient descent step for the representation is sufficient to learn the ground-truth dictionary features. 
Again all tasks use the same number of samples, denoted by $n_2\coloneqq |\hat{\mathcal{D}}_{i,\mathbf{W}}|$.
In Theorem \ref{thm:1}, we show that this single iteration of alternating stochastic gradient descent with respect to $\{\mathbf{a}_1,\dots,\mathbf{a}_T\}$ and $\mathbf{W}$ is sufficient to learn meaningful features. Notably, it is standard practice in the feature learning theory literature to consider only one gradient descent  step for the first layer weights
\citep{daniely2020learning,abbe2022merged,barak2022hidden,damian2022neural,ba2022high}. 
{We later show empirically that in our multi-task setting, it is necessary to first optimize the heads before updating the first-layer weights in order to recover the ground-truth features.} 
In any case, following \citet{damian2022neural}, we do not update the biases during pretraining. 
%Hence, the output of the representation learning phase are the weights and bias $ \mathbf{W}^+$, $ \mathbf{b}^0$, and task-specific heads that are $ \mathbf{a}_{1}^+, \dots, \mathbf{a}_{T}^+$. 
% Note that we only use $ \mathbf{W}^1$ for the downstream task, as we specify next. 
Next we describe how we leverage the pre-trained weights $\mathbf{W}^1$ for learning a downstream task.




\textbf{Downstream evaluation phase.}  After the representation learning phase, we consider learning a prediction function to fit a downstream task that may have {\em any} link function  on the $r$ ground-truth features, i.e. any function in the support of $\mathcal{T}_{\text{all}}$. Since we consider such a wide range of possible downstream tasks, we need to increase the model complexity to allow for solving such tasks.
% Nevertheless, these functions can still be learned efficiently 
% Thus, we append a random
% Thus, we consider pr insert a random ReLU layer following the first layer whose weights 
Thus, we use prediction functions  with two hidden layers with first layer weights determined by the output of the representation learning phase, and second hidden layer parameters set randomly.
% Intuitively, we add a random  second layer on top of the trained first layer so that the model has enough expressivity to solve {\em any} downstream task on the $r$ ground-truth features. 
This random second layer is necessary  to linearly separate the classes induced by {\em any} binary function on the $r$ coordinates with high probability, without having to use a very wide first layer;
please see Remark \ref{rem:2} for more details.


% {\color{gray}
In other words, the first hidden layer has $m$ neurons and the weights are a scaled version of $ \mathbf{W}^1$ denoted by $\alpha \mathbf{W}^1$, and the bias term is $ \mathbf{b}$. Note that here $\alpha>0$ is a re-scaling factor (see  Appendix \ref{app:down} for more details). The second hidden layer of the classifier has $\hat{m}$ neurons with weights denoted by $\hat{\mathbf{W}} \coloneqq [\hat{\mathbf{w}}_1,\dots,\hat{\mathbf{w}}_{\hat{m}}]^\top\in \mathbb
{R}^{\hat{m}\times m}$ and bias by $\hat{\mathbf{b}}\in  \mathbb{R}^{\hat{m}}$. Hence, the embedding of these two layers for input $\mathbf{x}$, which we denote by $ \phi(\mathbf{x})\in \mathbb{R}^{\hat{m}}$, is given by 
\begin{align}
\vspace{-1mm}
    \phi(\mathbf{x}) =  \sigma\left( \hat{\mathbf{W}} \  \sigma\left(\alpha{}\mathbf{W}^1\mathbf{x} + \mathbf{b}\right) + \hat{\mathbf{b}}\right) \label{F}
    \vspace{-1mm}
\end{align}
Again note that $\mathbf{W}^1$ is fixed from the previous phase; it remains to set  ${\mathbf{b}}$, $ \hat{\mathbf{W}}$, and $\hat{\mathbf{b}}$ to create an effective embedding for the downstream task. We do this by sampling $\hat{\mathbf{W}}$ and $(\mathbf{b},\hat{\mathbf{b}})$ from mean-zero Gaussian and uniform distributions, respectively, with variances that depend only on $m$; 
% please 
see Appendix \ref{app:down} for more details.
% {\color{red}{you need to be more specific here}}

% To do so, we randomly set these parameters
% % . More precisely, we first randomly initialize $ \hat{\mathbf{W}}$, ${\mathbf{b}}$, and  $\hat{\mathbf{b}}$ 
% according to 
% $$
% \mathbf{b}\sim \text{Unif}\left(\left[-\frac{\sqrt{2}{\gamma}}{\sqrt{m}},\frac{\sqrt{2}{\gamma}}{\sqrt{m}}\right]^m\right), 
% \quad \hat{\mathbf{b}} \ {\sim}\  \text{Unif} \left(\left[-\frac{\sqrt{2}\hat{\gamma}}{\sqrt{\hat{m}}},\frac{\sqrt{2}\hat{\gamma}}{\sqrt{\hat{m}}}\right]^{\hat{m}}\right)
% \quad 
% \hat{\mathbf{w}}_j {\sim} \mathcal{N}\left(\mathbf{0}_m,\frac{2}{\hat{m}}\mathbf{I}_m\right),
% $$
% for all $j \in [\hat{m}]$,  where  $\text{Unif}([a,b]^m)$ denotes the uniform distribution on the box $[a,b]^m \subset \mathbb{R}^m$.
% }

Next, given a dataset $\hat{\mathcal{D}}_{T+1} \coloneqq \{(\mathbf{x}_l,f_{T+1}(\mathbf{x}_l))\}_{\ell=1}^N$ of $N$ i.i.d. samples from a distribution $\mathcal{D}_{T+1}$ corresponding to a downstream task, we learn a task-specific head $\mathbf{a}$ and a bias term $\tau$ by solving the following problem:
\begin{align}
    % ( \mathbf{a}_{T+1}, \tau_{T+1}) \in\  
    \min_{ \mathbf{a}\in \mathbb{R}^{\hat{m}}, \tau \in \mathbb{R}} \ \frac{1}{N}\sum_{l=1}^N \ell(\mathbf{a}^\top \phi(\mathbf{x}_l )\!+\!\tau\! , f_{T+1}(\mathbf{x}_l)  ) + \frac{\hat{\lambda}_{\mathbf{a}}}{2}\|\mathbf{a}\|_2^2.  \nonumber
    % \label{ada}
    \vspace{-1mm}
\end{align}
We use the resulting head, i.e.,  $\mathbf{a}_{T+1}$, and bias term, i.e. $\tau_{T+1}$, to define the  prediction function for task $T+1$ as
% . In particular, using the fact that $g(\mathbf{x})= \sigma\left( \hat{\mathbf{W}} \  \sigma\left(\alpha{}\mathbf{W}^+\mathbf{x} + \mathbf{b}\right) + \hat{\mathbf{b}}\right)$, our final prediction function is 
% $F(\mathbf{x} \ ;\ \mathbf{a}_{T+1}, \tau_{T+1}, \mathbf{W}^+,\mathbf{b},\hat{\mathbf{W}},\hat{\mathbf{b}} )$ is given by
\begin{align}
\vspace{-1mm}
&F(\mathbf{x}; \mathbf{a}_{T+1}, \tau_{T+1}, \mathbf{W}^1,\mathbf{b},\hat{\mathbf{W}},\hat{\mathbf{b}} )
\ \nonumber\\
&:=\ \mathbf{a}_{T+1}^\top \sigma\left( \hat{\mathbf{W}} \  \sigma\left(\alpha{}\mathbf{W}^1\mathbf{x} + \mathbf{b}\right) + \hat{\mathbf{b}}\right) +\tau_{T+1}. \nonumber
\vspace{-1mm}
\end{align}
For ease of notation, we denote the above function by $F(\mathbf{x})$. We evaluate the performance of the prediction function on the task population loss:
\begin{align}
\vspace{-1mm}
    \mathcal{L}_{T+1}^{\text{eval}}(F) \coloneqq \mathbb{E}_{(\mathbf{x},f_{T+1}(\mathbf{x})) \sim \mathcal{D}_{T+1}  } [ \ell(F(\mathbf{x} ), f_{T+1}(\mathbf{x})  ) ]. \nonumber
    \vspace{-1mm}
\end{align}
Note that $\mathcal{L}_{T+1}^{\text{eval}}$ is a random function of $\mathbf{b},\hat{\mathbf{W}},\hat{\mathbf{b}}$, and $\hat{\mathcal{D}}_{T+1}$ in addition to the randomness from pretraining. We  upper bound $\mathcal{L}_{T+1}^{\text{eval}}$ with high probability %for particular types of downstream tasks 
in Theorem \ref{thm:downstream}.


% Given a downstream task with labelling function $\bar{f}_{n+1}^\ast$. 

% loss function $\mathcal{L}_{n+1}(\cdot,\cdot)$ and a pre-trained representation $\mathbf{W}_1$, we 

% {\color{gray}
% compute the linear probe
% \begin{align}
%     \mathbf{a}_{n+1}(\mathbf{W}_1) \in \arg\min _{\mathbf{a}\in \mathbb{R}^m} \mathcal{L}_{n+1}(\mathbf{W}_1,\mathbf{a})
% \end{align}
% and the resulting task loss $\mathcal{L}_{n+1}(\mathbf{W},\mathbf{a}_{n+1}(\mathbf{W}))$. Linear probing can be thought of as fine-tuning only the last layer of the network (note that $ \mathbf{a}_{i+1}(\mathbf{W})$ can be computed with only a few fine-tuning gradient descent steps as $\mathcal{L}_i$ is strongly convex in $\mathbf{a}_i$). The ultimate goal is to learn a $\mathbf{W}$ that achieves minimax loss on some set of downstream tasks $\mathcal{T}^{\text{eval}}$, namely to achieve small $\rho(\mathbf{W},\mathcal{T}^{\text{eval}})$:
% \begin{align}
%     \rho(\mathbf{W},\mathcal{T}^{\text{eval}}) \coloneqq \sup_{(i+1)\sim \mathcal{T}^{\text{eval}}}  \mathcal{L}_{n+1}(\mathbf{W},\mathbf{a}_{n+1}(\mathbf{W})).
% \end{align}
% }

% Today write negative result in main body. do literature review.
% tomorrow: Finish proof sketch. CHange to infinite samples. Think about whether we can improve the result (large r). . Finish downstream guarantees.


% for downstream tasks, need to  assume $\mathbf{z} \sim \Unif(\mathcal{H}^k)$.

% \textcolor{blue}{HH: Read until here}




==> Formulation.tex <==
\section{Formulation} \label{sec:formulation}

% Instead of the previous Gaussian input data model, let us 

In section we formally define the multi-task learning  problem and the algorithms we analyze in Section \ref{sec:results}. We are motivated by classification problems in which the input data for all tasks share a common, small set of features that determine their label,  but the mapping from these features to labels differs across tasks. Ultimately, the multi-task learner aims to leverage the large set of available pre-training tasks to learn a representation that recovers the small set of label-relevant features to allow for strong performance on downstream tasks.

\subsection{Pre-training tasks and data generating model} To model such settings, we consider pre-training on a set of $T$ 
binary classification tasks
drawn uniformly from a collection of  tasks denoted by $\mathcal{T}$. These tasks consist of a distribution on $\mathcal{X}\times \mathcal{Y}$, where the input space is $\mathcal{X}=\mathbb{R}^d$ and the label space  is $\mathcal{Y}= \{-1,1\}$.
We assume that the labelling function for each task $i$ is a function of the sign of the first {$r$} coordinates of $\mathbf{x}$, denoted by $\mathbf{x}_{:r}$. More precisely, if we define $f_i^*:\mathcal{X} \to\mathcal{Y}  $ as the labelling function of task $i$, then for any sample $\mathbf{x} \in \mathcal{X}$, where here we assume $\mathbf{x}$ is drawn from the standard Gaussian distribution, we have 
\begin{align} \label{eq1}
    \mathbf{x}\sim \mathcal{N}(\mathbf{0}_d,\mathbf{I}_d);  \quad  f_i^\ast(\mathbf{x}) = \bar{f}_i^\ast(\sign(\mathbf{x}_{:r})) \in \{-1,1\}.
\end{align}
Here,  $\bar{f}_{i}^\ast: \{-1, 1\}^{r}\rightarrow \{-1,1\}$ is the
ground-truth labelling function for task $i$ that only depends on the sign of the first $r$ coordinates of $\mathbf{x}$. As a learner, for each task $i$ among the given tasks, we have access to samples pair of the form $(\mathbf{x},f_i^\ast(\mathbf{x})) $. This setting is similar to the sparse coding model studied in \cite{shi2022theoretical}, except the fact that we assume the input data is defined on $\mathbb{R}^d$, while in \cite{shi2022theoretical} the authors assume the input data is defined over the hypercube in $\mathbb{R}^d$. By assuming that the labelling function is a function of ``sign'' of the first $r$ coordinates, we make our model more similar to the one in \cite{shi2022theoretical}, as they assume the label for each task is a function of the first $r$ coordinates of the integer input data. 

% \textcolor{blue}{not sure I understand this: $\mathbf{z}_{:r}$ is independently generated from $\mathbf{M}$, so it seems that the previous sentence should be revised. I.e. the label only depends on $\mathbf{z}_{:r}$ and not the columns of $\mathbf{M}$. }
%Our setting is similar to the sparse coding model studied by \cite{shi2022theoretical}, except that our latent vectors are Gaussian, rather than being vertices on the hypercube $\{-1,1\}^d$.   Formally, in our setting labeled points 
 %for any task $ \in \mathcal{T}$ are sampled from $\mathcal{D}_i$ as follows


%Thus, the first $r$ coordinates of $\mathbf{z} = \mathbf{M}^\top\mathbf{x}$ determine the labels for the $i$-th task according to the ground-truth labelling function $\bar{f}_{i}^\ast: \{-1, 1\}^{r}\rightarrow \{-1,1\}$, while the remaining $k-r$ coordinates of $\mathbf{z}$ are spurious. So, the data can be projected onto the low-dimensional space $\text{col}(\mathbf{M}_{:r})$ and preserve all information relevant to its label, for all tasks in $\mathcal{T}$. We let $\bar{\mathcal{T}} \coloneqq \{\bar{f}_{i}^\ast : \mathcal{D}_i \in \mathcal{T}\}$  denote the collection of ground-truth labelling functions corresponding to tasks in $\mathcal{T}$.
% \textcolor{blue}{this good (i.e. explaining what's the signal and what's the spurious features; I would add more of these high-level sentences in te paragraph above)}

% \textcolor{blue}{can you (briefly) mention the advantages of your model compared to the previous sparse coding ones?}
% Our setting allows the latent variables to 

Critically, the set of label-relevant coordinates of the input data are shared among all tasks, while the functions $\bar{f}_i^*$ mapping from these coordinates to labels are specific to each task. Thus, the goal of the multi-task learner is to recover the shared label-relevant coordinates, so that it may solve a downstream task with complexity scaling only with the number $r$ of label-relevant coordinates, rather than the much larger ambient dimension of the data $d$.

This model draws inspiration from realistic classification tasks in which labels are functions of the presence (or lack thereof) of a small number of features in the data. For example, whether or not a brain MRI reveals cancerous tissue depends on the presence of tumor-shaped structures in the image, indicated by a small number of features relative to the dimension of the MRI. While prior work has used such settings to motivate studying the dynamics of neural network training with a similar data model with discrete input vectors in the single-task setting \citep{shi2022theoretical,wen2021toward},
% However, in the sparse coding model the latent variables are either on the Rademacher hypercube $\{-1,1\}^d$ or in the set $\{-1,0,1\}^d$, rather than being Gaussian samples in $\mathbb{R}^d$. 
our model captures more general scenarios in which features appear in the data on a continuous spectrum, while the label is a quantization of these continuous features.

% is common among all tasks, meaning the input data across all tasks shares both spurious and label-relevant features, however the mapping from label-relevant features to labels differs across tasks. 

% . However, it is not clear how this is possible  since  the spurious features dominate the ground-truth features in $\mathbf{x}$ (that is, ${\|\mathbf{M}_{r:}^\top\mathbf{x}\|_2^2} = \hat{\Omega}\left(\frac{k-r}{r}\right){\|\mathbf{M}_{:r}^\top\mathbf{x}\|_2^2}$ with high probability).
% \textcolor{blue}{it might be good to write explicitly somewhere that $k >> r$; Right now you just use the word ``outweigh'' at some point. }


The generative model in \eqref{eq1} implies that, for any task in $\mathcal{T}$, the label of samples are a function of the first $r$ coordinates. 
However, in order to recover all the $r$ label-relevant coordinates, we must ensure there is sufficient diversity in the labels. To this aim we impose a condition that can be interpreted as task diversity.
%% ...  it must be the case that the other $d-r$ coordinates are spurious. 
% For this to be the case we must make a further assumption on the collection of tasks $\mathcal{T}$. 
% Next we give two examples of collections of labelling functions that satisfy Assumption 3.1.
% An example  of a collection of tasks that satisfies Assumption 3.1 is the collection of all possible labellings of $2^r$ inputs.
%% This can be captured by considering that 
Specifically, our condition ensures that for any pair of points with different sign patterns on their $r$ label-relevant features, it is equally likely for them to have the same label as it is for them to have different labels on a task drawn from $\mathcal{T}$. Next, we formalize this assumption. 

\begin{assumption}\label{assump:diversity}
For any two points $\mathbf{x},\mathbf{x}'\in \mathcal{X}$ such that $\sign(\mathbf{x}_{:r})\neq \sign( \mathbf{x}_{:r}')$, % and $\mathbf{v}\neq -\mathbf{v}'$,
% $\sign(\mathbf{M}_{:r}^\top\mathbf{x}) \neq \sign(\mathbf{M}_{:r}^\top\mathbf{x}')$ and $\sign(\mathbf{M}_{:r}^\top\mathbf{x}) \neq -\sign(\mathbf{M}_{:r}^\top\mathbf{x}')$, 
the probability that the labels of $\mathbf{x}$ and $\mathbf{x}'$ are the same for a task drawn uniformly from ${\mathcal{T}}$  satisfies: %, for some $\delta \in [0,\tfrac{1}{2})$:
\begin{align}
       % \tfrac{1}{2} - \delta \leq 
       \Pr_{i \sim \Unif({\mathcal{T}})} \left[ \bar{f}_i^*(\sign(\mathbf{x}_{:r})) = \bar{f}_i^*( \sign(\mathbf{x}_{:r}'))  \right]& 
    % \begin{cases} =  1  & \text{if} \; \sign(\mathbf{M}_{:r}^\top\mathbf{x}) = \sign(\mathbf{M}_{:r}^\top\mathbf{x}') \\
    = \tfrac{1}{2} \nonumber
    % + \delta \nonumber
    % & \text{otherwise} \\
    % \end{cases}
\end{align}
\end{assumption}
%and assuming that the pair is equally-likely to share a label on a task drawn from $\mathcal{T}$ as it is to have different labels (the values of the $d-r$ spurious coordinates provide no information about whether the pair is likely to share a label).
% The interpretation of the above assumption as task diversity follows from the observation that
%% For example, 
% Note that \ref{assump:diversity}  rules out the possibility of most tasks labelling most inputs the same, which would cloud the importance of the $r$ ground-truth features. For example, 
% if all tasks labelled all inputs as `1', then it would be impossible to recover the $r$ ground-truth features, since they are irrelevant to the label for all tasks. 
Assumption \ref{assump:diversity} enforces task diversity by ensuring that all pairs of distinct sign inputs are equally likely to have distinct labels as not -- i.e. there is no subset of the $r$ coordinates that is more indicative of the inputs sharing a label than the other coordinates. Such an assumption is necessary because, in the extreme case, if all tasks could be written as functions of only the first coordinate, it would be impossible to recover the remaining $r-1$ coordinates. Thus, we need the collection of possible training tasks to be sufficiently diverse such that all $r$ coordinates are equally relevant to the label, on average across tasks (i.e. one coordinate may be irrelevant to the label for some task, but it must be relevant for others). We note that, strict equality in the assumption is not necessary, but made for convenience. Indeed, we only sample $T <\infty$ tasks from $\mathcal{T}$ for training, so our empirical task distribution is not guaranteed to satisfy Assumption \ref{assump:diversity} with strict equality. To satisfy the assumption, we can set $\mathcal{T}$ to be the set of all possible labellings of the $2^r$ inputs on the $r$-dimensional hypercube, noting that our results do not require $T$ to scale with $\mathcal{T}$.

% Assumption \ref{assump:diversity} enforces both of 
% Observe that if all tasks label all inputs as '1', then no coordinate is relevant to the label and $\Pr_{i \sim \Unif({\mathcal{T}})} \left[ \bar{f}_i^*(\sign(\mathbf{x}_{:r})) = \bar{f}_i^*( \sign(\mathbf{x}_{:r}'))  \right]=1$ for all $\mathbf{x}\neq \mathbf{x}'$, while if the tasks only depend on the first coordinate, $\Pr_{i \sim \Unif({\mathcal{T}})} \left[ \bar{f}_i^*(\sign(\mathbf{x}_{:r})) = \bar{f}_i^*( \sign(\mathbf{x}_{:r}'))  \right]=1$ for all $\mathbf{x}, \mathbf{x}'$ with the same sign on the first coordinate. 


% Assumption \ref{assump:diversity} states that if two data points do not share signs of ground-truth features, then they are just as likely to share a label on a random task as they are to have differing labels. 
% % almost as likely to share a label on a random task as they are to have differing labels, up to $\delta$ error. 
% On the other hand, the data generative model implies that if two points do share the same sign pattern for the ground-truth features, then they share the same label  on a random task with probability one.
% This means that the only information that predicts whether two points will have the same label on a random task is the sign pattern of their ground-truth features -- the spurious features do not convey any such information.



% For pre-training, the multi-task learner draws $T$ tasks  uniformly at random from $\mathcal{T}$, where possibly $T \ll |\mathcal{T}|$. We make only one assumption on the 
% % collection of ground-truth labelling functions $\bar{\mathcal{T}}$ corresponding to the 
% collection of tasks $\mathcal{T}$. 
% \textcolor{blue}{is there a difference between $\bar{\mathcal{T}}$ and $\mathcal{T}$? Can we use $\mathcal{T}$ for both with some slight abuse of notation? Also, we have $f$ and $\bar{f}$; can we simplify this notation somehow (not sure if the two are very different)?} 
% Nevertheless, we show that head-adaptive algorithms can learn the ground-truth features as long as a simple assumption on the tasks $\mathcal{T}$ is satisfied. For ease of notation we use $i\sim \Unif(\mathcal{T})$ to denote drawing a task $\mathcal{D}_i$ uniformly at random from $\mathcal{T}$. 


% , i.e. $\bar{\mathcal{T}} \coloneqq \{ \bar{f}_i^*:\{-1,1\}^r \rightarrow \{-1,1\} \} $. 
% The strict $1/2$ requirement can be removed to include additional task collections, but we 

% \textbf{Example 1: All possible labellings of $2^r$ inputs.} Here $\bar{\mathcal{T}} \coloneqq \{ \bar{f}_i^*:\{-1,1\}^r \rightarrow \{-1,1\} \} $ is analogous to the power set on $r$ elements. Although in this case $|\bar{\mathcal{T}}|= 2^{2^r}$, we show in Theorem \ref{thm:1} that multi-task learning can still learn meaningful features when $n$ scales only exponentially with $r$. 

% {\color{gray}
% \textbf{Example 2: Parities on subsets of $[r]$.} Here $\bar{\mathcal{T}} \coloneqq \{ \bar{f}_i^*:\{-1,1\}^r \rightarrow \{-1,1\} | \bar{f}_i^*(\mathbf{v}) = \prod_{j \in A} v_j, \; A \subseteq [r] \} $. In this case, each $\bar{f}_i^*\in \bar{\mathcal{T}}$ outputs the parity of the input bits on a subset $A$ of the first $r$ bits. In other words, each task is a sparse parity problem, which has received much attention in studies of single task feature learning \cite{daniely2020learning,shi2022theoretical,frei2022random}. Unlike prior work, we show in the subsequent section that pre-training on many sparse parity tasks allows the network to learn features that generalize beyond sparse parity tasks.}

% Assumption 3.1 is satisfied if $\mathcal{T}$  consists of all binary labellings of $2^r$ inputs.
% We call this a ``task diversity'' assumption because it entails that the tasks must be diverse enough to rule out correlations between spurious features and labels.

% For pre-training,  we make no further assumptions on the ground-truth labelling functions $f_{i}^\ast$, meaning they can be arbitrarily complex. For downstream guarantees, we need to ensure that any downstream $f_{i'}^\ast$ must be implementable by the learning model, which we discuss later.
% \textcolor{blue}{this paragraph is a bit vague at this moment (and it might be unnecessary), so maybe you want to move it down}

\subsection{Learning model and loss}  We consider pre-training a two-layer neural network $f(\cdot; \mathbf{W},\mathbf{b},\mathbf{a}):\mathbb{R}^d\rightarrow \mathbb{R}$ with $m$ ReLU-activated neurons in the hidden layer, namely
\begin{align}
    f(\mathbf{x}; \mathbf{W},\mathbf{b},\mathbf{a}) := \sum_{j=1}^m a_j \sigma (\mathbf{w}_j^\top \mathbf{x} + b_j)
\end{align}
where $\sigma(\mathbf{x})=\max(\mathbf{x},\mathbf{0})$ element-wise, $\mathbf{w}_j \in \mathbb{R}^d$ and $b_j \in \mathbb{R}$ are the weight vector and bias for the $j$-th neuron, respectively, and $a_j\in \mathbb{R}$ is the last-layer weight for the $j$-th neuron. We let $\mathbf{W} = [\w_1,\dots,\w_m]\in \mathbb{R}^{d \times m}$ denote the matrix of concatenated weight vectors, $\mathbf{b}=[b_1,\dots,b_m]\in \mathbb{R}^m$ denote the vector of biases, and $\mathbf{a}= [a_1,\dots,a_m] \in \mathbb{R}^m$ denote the vector of last-layer weights, which we call the head. Solving a task $i$ entails that predictions $f(\mathbf{x}; \mathbf{W},\mathbf{b},\mathbf{a}) $ align well with the corresponding label $f_i^\ast(\mathbf{x})$ of $\mathbf{x}$, which we measure using the hinge loss:
\begin{align}\label{eq:hingeloss}
    \ell(f(\mathbf{x};\mathbf{W},\mathbf{b},\mathbf{a}), f_i^\ast(\mathbf{x})):= \max\big(1 - f_i^\ast(\mathbf{x}) f(\mathbf{x};\mathbf{W},\mathbf{b},\mathbf{a}), 0\big)
\end{align}
% \textcolor{blue}{why does the regularization appear in the individual loss for each data point? It might be better o add the regularization terms at the end to the some of the losses over all the data points (like structural ERM). I know what you're doing is equivalent. }  
% Let $\mathcal{D}_i$ denote the distribution over labelled pairs $(\mathbf{x},f_i^\ast(\mathbf{x}))$ for task $i$. 
The loss for task $i$ as a function of the model parameters $(\mathbf{W},\mathbf{b},\mathbf{a})$ is the average point-wise loss over labelled points $(\mathbf{x},f_i^\ast(\mathbf{x}))$ drawn from $\mathcal{D}_i$:
% , plus $\ell_2$ regularization:
\begin{align}
     \mathcal{L}_i(\mathbf{W},\mathbf{b},\mathbf{a}) &:=  \mathbb{E}_{(\mathbf{x},f_i^\ast(\mathbf{x}))\sim \mathcal{D}_i}\left[ \ell(f(\mathbf{x};\mathbf{W},\mathbf{b},\mathbf{a}), f_i^*(\mathbf{x})) \right]  
     % + \frac{\lambda_{\mathbf{a}}}{2} \|\mathbf{a}\|_2^2 +  \frac{\lambda_{\mathbf{w}}}{2} \|\mathbf{W}\|_F^2, 
\end{align}
Ultimately, the goal of multi-task pre-training is to learn a first-layer representation that generalizes to downstream tasks, in the sense that we can easily train a new classifier
% , task-specific head $\mathbf{a}_{n+1}$ 
on top of the first layer in order to achieve small task-specific loss.
% $\mathcal{L}_{n+1}(\mathbf{W},\mathbf{b},\mathbf{a})$. 
To this end, our goal is minimize the following multi-task loss function
% The global loss is the average loss on each task: , plus $\ell_2$ regularization of the weights and head
\begin{align}\min_{\mathbf{W},\mathbf{b}, \{\mathbf{a}_1, \dots, \mathbf{a}_T\}}
 {\mathcal{L}}(\mathbf{W},\mathbf{b},\{\mathbf{a}_i\}_{i=1}^T ) := \frac{1}{T}\sum_{i=1}^T  \mathcal{L}_i(\mathbf{W},\mathbf{b},\mathbf{a}_i)  +   \frac{\lambda_{\mathbf{a}}}{2} \|\mathbf{a}_i\|_2^2 +  \frac{\lambda_{\mathbf{w}}}{2} \|\mathbf{W}\|_F^2  \label{obj_glob_i},
\end{align}
where $\lambda_{\mathbf{a}}$ and $\lambda_{\w}$ are regularization parameters. 
% Optimizing $ \mathcal{L}_{\text{SM}}$ entails learning a single model that minimizes the average loss across tasks, arguably the simplest approach to multi-task learning.
% and is common in multi-task settings such as federated learning \citep{mcmahan2017communication,karimireddy2020scaffold}.
Optimizing $\mathcal{L}$ entails learning task-specific heads on top of a shared representation, a widely used and empirically successful approach to multi-task learning \citep{zhang2021survey,crawshaw2020multi,ruder2017overview}. Basically, by solving the above problem, we hope to find a set of $(\mathbf{W},\mathbf{b})$ such that they learn the important features and we can argue that the output of first layer denoted by $[\sigma (\mathbf{w}_1^\top \mathbf{x} + b_1),\dots, \sigma (\mathbf{w}_m^\top \mathbf{x} + b_m)]\in \mathbb{R}^m$ only contains information about the first $r$ coordinates of $\mathbf{x}$. 
Next we discuss the optimization algorithms we study. 
%\textcolor{blue}{maybe discuss very briefly here what the actual optimization problem is? I.e. you'd like to minimize the above loss over the choice of the representation $W$ and the task-specific heads $a_i$'s. How is $b$ chosen?}


% {\color{red} finite sample loss}
% \cite{shi2022theoretical} showed that running GD on the one-task population loss causes all neurons to go to $\propto  \sum_{l=1}^r \mathbf{M}_{l}$. This allows it to learn the task iff $g$ depends on $\boldsymbol{\phi}^{(:r)}$ only through $\sum_{l=1}^r \phi^{(l)}$. We would like to learn the features themselves in order to enable learning a larger class of functions.

% Our key assumption on the tasks that enables  
% concern: people will say that lower bound depends fundamentally on GD, SGD might work
% \cite{wen2021toward}

% We are motivated by \cite{shi2022theoretical}, who considered this model and showed that GD learns the average of the important features. Feature learning requires that we learn the important features themselves, not their average. Learning the average of the features seems to be a flaw inherent to GD in this setting, not their analysis. 
% so there is hope that multi-tasking/head diversity can allow for learning individual features and proving that GD cannot learn them.


% Specifically, the model is:

% Fix some column-orthonormal dictionary matrix $\mathbf{M}\in \mathbb{R}^{d \times k}$. The $j$-th sample for task $i$ is generated as:
% \begin{align}
%     \boldsymbol{\phi}_{i,j} \sim \{0,1\}^k, \quad \mathbf{x}_{i,j} = \mathbf{M}\boldsymbol{\phi}_{i,j}, \quad y_{i,j} = g_i(\boldsymbol{\phi}_{i,j}^{(:r)})
% \end{align}
% where $\boldsymbol{\phi}_{i,j}^{(:r)}$ denotes the first $r\leq k$ elements of $\boldsymbol{\phi}_{i,j}$. 

\section{Algorithm} \label{sec:alg}

\begin{comment}
We consider two pre-training algorithms that aim to learn a generalizable representation $\mathbf{W}$, described as follows.


\textbf{Pretraining Option 1: Single-Model Gradient Descent (SMGD).} SMGD runs gradient descent with step size $\eta$ on the global loss \eqref{obj_glob}. First it initializes $\mathbf{W}_0$ and $\mathbf{a}_0$ according to any initialization procedure. Then, for all rounds $t = 1,\dots,T$, it computes
\begin{align}
    \mathbf{a}_{t+1}^{\text{SMGD}} &= \mathbf{a}_{t}^{\text{SMGD}} - \eta \nabla_{\mathbf{a}} \mathcal{L}(\mathbf{W}_t^{\text{SMGD}},\mathbf{a}_t^{\text{SMGD}}); \quad \mathbf{W}_{t+1}^{\text{SMGD}} = \mathbf{W}_{t}^{\text{SMGD}} - \eta \nabla_{\mathbf{W}} \mathcal{L}(\mathbf{W}_t^{\text{SMGD}},\mathbf{a}_t^{\text{SMGD}})
\end{align}
This is the simplest multi-task learning algorithm we consider. It is also referred to Distributed Gradient Descent or simply Gradient Descent in distributed and federated settings.
\end{comment}

We consider a two-stage learning process: (1) Representation learning, in which we aim to learn effective features using $n$ available tasks, and (2) Downstream evaluation, in which we encounter a new task and aim to efficiently learn an accurate linear classifier on top of the pre-trained features. 
% We consider two different algorithms for pre-training.

% The gradient-based multi-task learning algorithm we study executes two phases: (1) a pre-training phase in which the ground-truth features are learned by training on all $n$ sampled tasks, and (2) a fine-tuning phase in which the first-layer biases are re-initialized and the head is re-trained on a single downstream task.

% \textbf{Pretraining Algorithm 1: Single-Model Gradient Descent (SMGD).} SMGD runs gradient descent with step size $\eta$ on the global loss \eqref{obj_glob}. First it initializes $\mathbf{W}_0$ and $\mathbf{a}_0$ according to any initialization procedure. Then, for all rounds $t = 1,\dots,T$, it computes
% \begin{align}
%     \mathbf{a}_{t+1}^{\text{SMGD}} &= \mathbf{a}_{t}^{\text{SMGD}} - \eta \nabla_{\mathbf{a}} \mathcal{L}(\mathbf{W}_t^{\text{SMGD}},\mathbf{a}_t^{\text{SMGD}}); \quad \mathbf{W}_{t+1}^{\text{SMGD}} = \mathbf{W}_{t}^{\text{SMGD}} - \eta \nabla_{\mathbf{W}} \mathcal{L}(\mathbf{W}_t^{\text{SMGD}},\mathbf{a}_t^{\text{SMGD}})
% \end{align}
% This is the simplest multi-task learning algorithm we consider. It is also referred to Distributed Gradient Descent or simply Gradient Descent in distributed and federated settings.









\textbf{Representation learning phase.} %Unlike SMGD, 
% \textbf{Phase 1: Pre-training.}
% MTRL is the main focus of our study.
% Unlike SMGD, MTRL 
The multi-task  learning algorithm we consider aims to solve the global objective \eqref{obj_glob_i} with task-specific heads. To do so, it first 
executes a symmetric initialization, as in previous studies of feature learning \cite{damian2022neural,shi2022theoretical}. 
% Note that the initialization for all task heads is the same for simplicity.
Consider $ \mathbf{w}_{j}^0 $ and $b_{j}^0$ as the weights and bias of first layer corresponding to the $j$-th neuron at time $0$, respectively, and  $a_{i,j}^0$ as the $j$-th element of the head corresponding to task $i$ at time $0$. Further for simplicity assume $m$ is even. 
Then, for all the weights corresponding to $j \leq \frac{m}{2}$, we set the weights as
\begin{align}
    \mathbf{w}_{j}^{0} \sim \mathcal{N}(\mathbf{0}_d,\nu_{\mathbf{w}}^2\mathbf{I}_d),  \quad a_{i,j}^0\sim \mathcal{N}({0},\nu_{\mathbf{a}}^2), \quad b_{j}^{0}=0
\end{align}
where $\nu_{\mathbf{w}},\nu_{\mathbf{a}} \in \mathbb{R}_{\geq 0}$. Moreover, for the remaining weights that correspond to $j>\frac{m}{2}$, we set the initial weights as $\mathbf{w}_{j}^0 = \mathbf{w}_{j-m/2}^0,$ $b_{j}^0=0$, and $a_{i,j}^0 = -a_{i,j-m/2}^0$ for all tasks $i\in [T]$. 
% randomly initializes the representation $\mathbf{W}_0^{\text{MTRL}}$. 
Once the random initialization procedure is done, we first optimize the heads, i.e., $\mathbf{a}_{1},\dots, \mathbf{a}_{T}$. 
Note that since each $\mathcal{L}_i$ is a strongly convex function with respect to $\mathbf{a}$, this optimization problem can be solved efficiently and the condition number is $1$ so that a constant number of iterations can yield a small loss. In fact,  we only run one step of gradient descent for each head on the regularized task-specific loss:
% alternates between minimization steps for the task-specific heads and gradient descent steps for the representation. 
% In particular, on round $t$, the parameters are updated as follows:
\begin{equation}
    \mathbf{a}_{i}^+ =  (1 - \eta \lambda_{\mathbf{a}})\mathbf{a}_{i}^0 -  \eta  \nabla_{\mathbf{a}} \mathcal{L}_i(\mathbf{W}^0,\mathbf{b}^0,\mathbf{a}_i^{0})
    \quad \forall \; i \in [T]  
\end{equation}
Next, the algorithm updates the model weights with one step of gradient descent  on the global loss induced by the task-optimal heads:
\begin{align}
    % \mathbf{a}_{1,i} &\in \arg \min_{\mathbf{a}\in \mathbb{R}^m} \mathcal{L}_i(\mathbf{W}_t,\mathbf{a}) \quad \forall \; \i \in \mathcal{T}  ^{\text{MTRL}}
    \mathbf{W}^+ &= \mathbf{W}^{0} -   \frac{\eta}{T} \sum_{i=1}^T \nabla_{\mathbf{W}}   \mathcal{L}_i(\mathbf{W}^0, \mathbf{b}^0,\mathbf{a}_{i}^+) 
\end{align}
% The representation-learning abilities of AltMinGD have been previously analyzed in the federated setting \citet{collins2021exploiting}, but this analysis was limited to linear models.
% We show that only one gradient descent step for the representation is sufficient to learn the ground-truth dictionary features. 
Later in Theorem \ref{thm:1}, we show that one gradient step is sufficient to learn meaningful features. We note that it is standard practice in the theory of feature learning literature to consider only one gradient descent  step for the first layer weights
\citep{daniely2020learning,abbe2022merged,barak2022hidden,damian2022neural,ba2022high}. 
We do not update the biases during pre-training, as in \citep{damian2022neural}. 
%Hence, the output of the representation learning phase are the weights and bias $ \mathbf{W}^+$, $ \mathbf{b}^0$, and task-specific heads that are $ \mathbf{a}_{1}^+, \dots, \mathbf{a}_{T}^+$. 
Note that we only use $ \mathbf{W}^+$ for the downstream task as we specify next. 




\textbf{Downstream evaluation phase.}  After the first phase, we consider learning a prediction function to fit a downstream task. This function is a neural network with two hidden layers where the weights of the first layer are fixed and determined by the output of the first phase, and the parameters of the second hidden layer are set randomly. Intuitively, we add a random  second layer on top of the trained first layer so that we can solve a wide range of downstream tasks on the $r$ important coordinates with high probability. Indeed this is necessary for the network $g$ to be able to linearly separate the classes induced any binary function on the $r$ coordinates with high probability, without having to use a very wide first layer. See Section \ref{sec:results} for more details.

In other words, the first hidden layer has $m$ neurons and the weights are a scaled version of $ \mathbf{W}^+$ denoted by $\alpha \mathbf{W}^+$ and the bias term is $ \mathbf{b}$. Note that here $\alpha>0$ is a re-scaling factor (see  Appendix \ref{app:down} for more details on $\alpha$). The second hidden layer of the classifier has $\hat{m}$ neurons and we denote its weights by $\hat{\mathbf{W}} \coloneqq [\hat{\mathbf{w}}_1,\dots,\hat{\mathbf{w}}_{\hat{m}}]^\top\in \mathbb
{R}^{\hat{m}\times m}$ and its bias by $\hat{\mathbf{b}}\in  \mathbb{R}^{\hat{m}}$. Hence, the embedding of these two layers for input $\mathbf{x}$, which we denote by $ g(\mathbf{x})\in \mathbb{R}^{\hat{m}}$ is given by 
\begin{align}
    g(\mathbf{x}) =  \sigma\left( \hat{\mathbf{W}} \  \sigma\left(\alpha{}\mathbf{W}^+\mathbf{x} + \mathbf{b}\right) + \hat{\mathbf{b}}\right) \label{F}
\end{align}
Again note that $\mathbf{W}^+$ are fixed and selected in the previous phase; it remains to set  ${\mathbf{b}}$, $ \hat{\mathbf{W}}$, and $\hat{\mathbf{b}}$ to create a good embedding for the downstream task. 
To do so, we randomly set these parameters
% . More precisely, we first randomly initialize $ \hat{\mathbf{W}}$, ${\mathbf{b}}$, and  $\hat{\mathbf{b}}$ 
according to 
$$
\mathbf{b}\sim \text{Unif}\left(\left[-\frac{\sqrt{2}{\gamma}}{\sqrt{m}},\frac{\sqrt{2}{\gamma}}{\sqrt{m}}\right]^m\right), 
\quad \hat{\mathbf{b}} \ {\sim}\  \text{Unif} \left(\left[-\frac{\sqrt{2}\hat{\gamma}}{\sqrt{\hat{m}}},\frac{\sqrt{2}\hat{\gamma}}{\sqrt{\hat{m}}}\right]^{\hat{m}}\right)
\quad 
\hat{\mathbf{w}}_j {\sim} \mathcal{N}\left(\mathbf{0}_m,\frac{2}{\hat{m}}\mathbf{I}_m\right),
$$
for all $j \in [\hat{m}]$,  where  $\text{Unif}([a,b]^m)$ denotes the uniform distribution on the box $[a,b]^m \subset \mathbb{R}^m$.








Next, given a set $S_{T+1} \coloneqq \{(\mathbf{x}_l,f_{T+1}^*(\mathbf{x}_l))\}_{\ell=1}^n$ of $n$ i.i.d. samples from a downstream task denoted by $T+1$, we learn a task-specific head $\mathbf{a}$ and a bias term $\tau$ by solving the following problem
\begin{align}
    ( \mathbf{a}_{T+1}, \tau_{T+1}) \in\  \argmin_{ \mathbf{a}\in \mathbb{R}^{\hat{m}}, \tau \in \mathbb{R}} \ \frac{1}{n}\sum_{l=1}^n \ell(\mathbf{a}^\top g(\mathbf{x}_l )+\tau , f_{T+1}^*(\mathbf{x}_l)  ) + \frac{\hat{\lambda}_{\mathbf{a}}}{2}\|\mathbf{a}\|_2^2 \label{ada}
\end{align}
Once this step is done, we use the learned head, i.e.,  $\mathbf{a}_{T+1}$, and bias term $\tau_{T+1}$ to define the  prediction function for task $T+1$. In particular, using the fact that $g(\mathbf{x})= \sigma\left( \hat{\mathbf{W}} \  \sigma\left(\alpha{}\mathbf{W}^+\mathbf{x} + \mathbf{b}\right) + \hat{\mathbf{b}}\right)$, our final prediction function is $F(\mathbf{x} \ ;\ \mathbf{a}_{T+1}, \tau_{T+1}, \mathbf{W}^+,\mathbf{b},\hat{\mathbf{W}},\hat{\mathbf{b}} )$ is given by
$$
F(\mathbf{x} \ ;\ \mathbf{a}_{T+1}, \tau, \mathbf{W}^+,\mathbf{b},\hat{\mathbf{W}},\hat{\mathbf{b}} )
\ :=\ \mathbf{a}_{T+1}^\top \sigma\left( \hat{\mathbf{W}} \  \sigma\left(\alpha{}\mathbf{W}^+\mathbf{x} + \mathbf{b}\right) + \hat{\mathbf{b}}\right) +\tau_{T+1}
$$
For ease of notation, we denote the above function by $F(\mathbf{x})$. Hence, the performance of our prediction function can be evaluated by 
\begin{align}
    \mathcal{L}_{T+1}^{(\text{eval})} \coloneqq \mathbb{E}_{(\mathbf{x},f_{T+1}^*(\mathbf{x})) \sim \mathcal{D}_{T+1}  } [ \ell(F(\mathbf{x}_l ), f_{T+1}^*(\mathbf{x}_l)  ) ].
\end{align}
Note that $\mathcal{L}_{T+1}^{(\text{eval})}$ is a random function of $\mathbf{b},\hat{\mathbf{W}},\hat{\mathbf{b}}$, and ${S}_{T+1}$ in addition to the randomness in the representation learning process. As a result, we provide a high probability upper bound on $\mathcal{L}_{T+1}^{(\text{eval})}$ for particular types of downstream tasks in Theorem \ref{thm:downstream}.


% Given a downstream task with labelling function $\bar{f}_{n+1}^\ast$. 

% loss function $\mathcal{L}_{n+1}(\cdot,\cdot)$ and a pre-trained representation $\mathbf{W}_1$, we 

% {\color{gray}
% compute the linear probe
% \begin{align}
%     \mathbf{a}_{n+1}(\mathbf{W}_1) \in \arg\min _{\mathbf{a}\in \mathbb{R}^m} \mathcal{L}_{n+1}(\mathbf{W}_1,\mathbf{a})
% \end{align}
% and the resulting task loss $\mathcal{L}_{n+1}(\mathbf{W},\mathbf{a}_{n+1}(\mathbf{W}))$. Linear probing can be thought of as fine-tuning only the last layer of the network (note that $ \mathbf{a}_{i+1}(\mathbf{W})$ can be computed with only a few fine-tuning gradient descent steps as $\mathcal{L}_i$ is strongly convex in $\mathbf{a}_i$). The ultimate goal is to learn a $\mathbf{W}$ that achieves minimax loss on some set of downstream tasks $\mathcal{T}^{\text{eval}}$, namely to achieve small $\rho(\mathbf{W},\mathcal{T}^{\text{eval}})$:
% \begin{align}
%     \rho(\mathbf{W},\mathcal{T}^{\text{eval}}) \coloneqq \sup_{(i+1)\sim \mathcal{T}^{\text{eval}}}  \mathcal{L}_{n+1}(\mathbf{W},\mathbf{a}_{n+1}(\mathbf{W})).
% \end{align}
% }

% Today write negative result in main body. do literature review.
% tomorrow: Finish proof sketch. CHange to infinite samples. Think about whether we can improve the result (large r). . Finish downstream guarantees.


% for downstream tasks, need to  assume $\mathbf{z} \sim \Unif(\mathcal{H}^k)$.

% \textcolor{blue}{HH: Read until here}






==> Introduction-ICML.tex <==
\section{Introduction} 
\label{sec:intro}

% Although much progress has been made in understanding the dynamics of neural networks trained with gradient-based methods in recent years, empirical innovation in deep learning continues to outpace theoretical development. A particularly stark example of this concerns multi-task learning.
% In practice, there has been a movement towards pretraining massive models that can solve  many tasks with a small  amount of fine-tuning, at the expense of huge computational resources required for pretraining \citep{chowdhery2022palm,smith2022using}. 
% A a result, it is imperative for modern models to be able to solve many tasks simultaneously, or after some  small amount of fine-tuning, rather than re-training the model from scratch for each task. 
% To ensure these models can indeed generalize to many tasks, they are typically pre-trained via multi-task learning, which aims to jointly optimize a set of loss functions, each corresponding to a different task. 
% , with the goal of finding a model that performs well on each task as well as downstream tasks, perhaps after fine-tuning some or all of the model layers.
% \textcolor{blue}{It's not clear what the point of the last few sentences is. Maybe you wanna say that empirically there has been a huge success in pretraining large models and then fine-tuning them, but theoretically there is not that much understanding on the dynamics?}

Recent empirical results have demonstrated huge successes in pretraining large neural networks (NNs) on many tasks with gradient-based algorithms \citep{%aghajanyan2021muppet,zhong2021adapting,sanh2021multi-task,wang2022benchmarking,
crawshaw2020multi,zhang2021survey,
wang2023multitask}.
% ,daras2022multi-tasking,wei2021finetuned
% ,bubeck2023sparks
These works suggest that the quality of the pretrained representation improves with the number of pretraining tasks, yet this phenomenon remains not well understood from a theoretical standpoint. 
% Multiple studies have further demonstrated that pretraining on a variety of tasks is not only sufficient but also necessary for effective downstream model performance \citep{}. 
%lu202012,liu2016recurrent,
% Multi-task learning has achieved a variety of success in practice . 
% For example, it has been observed that pretraining large language models (LLMs) on multiple diverse tasks can lead to learning more robust features for  downstream task performance \citep{daras2022multi-tasking,bubeck2023sparks}. 
% This penomenon 
Specifically, the natural questions of {\em why} nonlinear NNs learn effective feature representations when pretrained on multiple tasks with gradient-based methods and {\em how} the number of pretraining tasks affect the downstream performance of these representations remain largely unanswered.

% \textcolor{blue}{HH: From here onwards looks like a literature review. It'd be better to identify the problem that we study before hand. I.e. in the previous sentence we say that the quality of the rep improves with multiple tasks. So an important problem, or a natural problem is to understand fundamentally why this is the case and how is the scaling (quality vs tasks), or other problems that we study. We mention this first, and then say what people have done previously, and then conclude that new ideas are needed to answer our questions.}

Significant progress has been made in theoretically understanding the dynamics of NNs trained with gradient-based methods in recent years, especially in regards to proving that shallow NNs can learn meaningful features when trained with gradient descent and its variants \cite{damian2022neural,shi2022theoretical,abbe2020poly,abbe2022merged,allen2019learning,bai2019beyond,li2020learning,daniely2020learning,barak2022hidden,telgarsky2022feature,akiyama2022excess,zhou2021local}. 
However, these results are  limited to single-task settings, so they cannot explain the improvements in model performance seen by pretraining on many tasks. While a few studies show the representation learning benefits of multi-task pretraining with gradient-based algorithms \cite{argyriou2006multi,thekumparampil2021sample,collins2022maml,collins2022fedavg,saunshi2021representation,sun2021towards,chua2021fine,bullins2019generalize,chen2022active}, these analyses study only linear models; it is not clear whether they can generalize to even simple non-linear NNs. 

% As a result, new ideas are required to understand multi-task feature learning with nonlinear neural networks. To this end, in this work we
In this work, we aim to bridge this gap by 
analyzing the training dynamics of  a two-layer ReLU network pretrained with a generic gradient-based multi-task learning algorithm on  many binary classification tasks.  Following the aforementioned line of work, 
% analyzing feature learning dynamics in single-task 
% \cite{damian2022neural,shi2022theoretical,abbe2020poly,abbe2022merged,daniely2020learning,telgarsky2022feature,maurer2016benefit,du2020fewshot} 
% and linear 
% \citep{thekumparampil2021sample,collins2022maml,collins2021exploiting,saunshi2021representation,sun2021towards,chua2021fine,bullins2019generalize,chen2022active,tripuraneni2020provable} 
% settings 
% \textcolor{blue}{HH: Consider just saying "following the aforementioned line of work, we suppose ..."},
we suppose the existence of a ground-truth low-dimensional subspace that for all tasks preserves all information in the input data relevant to its label. %Furthermore, in the multi-task setting of this paper we assume this subspace is shared among all tasks.
We ask whether a variant of gradient descent applied to this  multi-task setting can learn a representation that projects the input data onto the ground-truth subspace. Learning such a representation entails successful pretraining, since it reduces the complexity of solving a downstream task to that of solving a classification problem in the low-dimensional space,  
% downstream tasks by solving a classification in the low-dimensional subspace
% % number of
% last layer 
% model parameters that 
% whose dimension scales only with the dimension of the low-dimensional subspace, 
rather than the potentially very high-dimensional input data  space.
% It is advantageous to learn such a representation because the model can drastically reduce the dimension of the data
% Still, much is unknown about which specific algorithms are most effective and, most importantly, why. On the empirical side, many works have focused on the issue of conflicting gradients, showing that  when running standard gradient descent to minimize the average task loss with a single model, diverse objective functions for each task can cause conflicting task-specific gradients that lead to information loss when aggregating these gradients globally. A variety of sophisticated  techniques have been proposed to address this issue \citep{chen2018gradnorm}, yet simple modifications of the standard gradient descent, such as learning a shared early model layers (representation) with task-specific last layers (heads), seem to work at least as well as their more sophisticated counterparts
% % , and even in the face of objective heterogeneity  
% \citep{xin2022current,kurin2022defense}. We refer to this general, widely popular multi-task learning method of learning a shared representation and task-specific heads as Multi-Task Representation Learning (MTRL).

% {\color{gray}

% Despite its relative simplicity, our theoretical understanding of MTRL is nascent. 
% There are a few examples of recent works theoretically studying the effectiveness of MTRL and closely related algorithms in both generic multi-task learning contexts as well as in more specific multi-task settings such as federated learning \citep{collins2021exploiting,} and meta- or few-shot learning \citep{collins2022maml,thekumparampil2021statistically}. However, these analyses are either limited to linear settings \citep{collins2021exploiting,collins2022maml,thekumparampil2021statistically,}
% % assume the dimension of the ground-truth representation is known by the learner, 
% or only consider the landscape induced by the MTRL objective, not the feature learning process of the algorithm \citep{du2020fewshot,tripuraneni2020provable}. On the other hand, many works have studied feature learning in (nonlinear) neural networks, yet the vast majority consider only single-task settings, which involve fundamentally different dynamics than in the multi-task case. 

% In this work, we bridge this gap by analyzing the dynamics of the MTRL and single-model gradient descent algorithms on a one-hidden-layer ReLU network. We employ a labelled data generating model in which the input data is a linear combination of dictionary features determined by a Gaussian latent variable, and the  labels for each binary classification  task are a distinct function of the latent Gaussian coordinates of a small of ground-truth features common across tasks. The goal for multi-task learner is therefore to recover the shared set of label-relevant features. }

% Learning models that can perform well on a variaety of tasks

% In recent years, the impressive performances of large language models on a variety of natural language processing tasks have highlighted the potential for 

% Multi-task pretraining 


% Here' we use task
% We use `task specific adaptation' as a generic term encompassing a variety of algorithmic techniques used to adapt a global model to particular tasks, including designating model parameters as task-specific and executing 
% so-called inner-loop updates in meta-learning and local updates in federated learning. 
Figure \ref{fig:multi} shows that gradient-based  multi-task learning with a two-layer ReLU NN with first-layer parameters (the representation) shared among all tasks and last-layer weights (the head) learned uniquely for each task indeed recovers the ground-truth subspace with error diminishing with the number of tasks. We theoretically justify this observation, providing the first known proofs of multi-task feature learning with a nonlinear model along with a new explanation for why multi-tasking aids feature learning.
% We prove that gradient-based  multi-task learning with a two-layer ReLU network with first-layer parameters (the representation) shared among all tasks and last-layer weights (the head) learned uniquely for each task is indeed able to recover the ground-truth subspace.
% after one gradient descent update of task-specific last model layer parameters followed by one gradient descent update  of the first-layer model parameters. % while single-model gradient descent cannot be guaranteed to  recover the ground-truth features.
% Our results therefore show for the first time that multi-task  representation learning is not an artifact of linearity.  
% -- suggesting that the feature learning demonstra in previous settings is not due to the linear nature of the model studied 
% but a fundamental property of the MTRL approach.
 Our theoretical contributions are summarized below, and verified numerically  in Appendix \ref{sec:sims}.
\begin{itemize}[leftmargin=3mm]
% \setlength{\itemindent}{-1em}
% \setlength{\parindent}{-2em}
 
% We allow for tasks of arbitrary complexity during pretraining, as long as they are functions of the signs of the coordinates of $r$ label-relevant features in the data, where $r$ is taken to be much less than the ambient dimension of the data, $d$, and the aggregated set of pretraining tasks satisfy a natural
% certain diversity assumption. 
% We show that the representation learned during multi-task pretraining with MTRL allows for learning the set of $p$-degree polynomials on the signs of the ground-truth latent coordinates by training a linear probe on top of the learned features with $O(r^p)$ neurons and $O()$ samples. In contrast, using random model weights without any pretraining, i.e. the NTK regime, would require $\Omega(d^p)$ neurons to learn a downstream task in this family.

% Features emerge after one update of the representation parameters from Gaussian initialization as long as the task-specific heads are properly trained. Result for both perfect training of the heads and partial training.%(error of feature learning will be exactly the error from partial training of heads. note partial training includes training with finite samples. will need to use concentration results on hypercube. but regardless will still need 2k samples...
% can also show concentration result for tasks. finite rep samples per task with finite tasks is difficult thugh...argue that in the age of foundation model pretraining we have infinte samples effectively
% We don't need to know the dimension of the representation. We provide downstream task performance guarantees.
\vspace{-2mm}

\item \textbf{Proof of multi-task representation learning with two-layer ReLU network.} We consider binary classification tasks whose labels depend on only $r$ features of the input, where $r$ is much smaller than the ambient dimension $d$, and a large class of task distributions that includes, e.g., a uniform distribution over sparse parity tasks.
% Under the assumption that  two points with differing $r$ important features are equally likely to have the same label  on a randomly drawn task as not, 
We prove that multi-task pretraining with a gradient-based learning algorithm on $T$ tasks drawn from such a distribution 
% one stochastic gradient descent (SGD) update of each of the task-specific heads followed by one SGD update of the representation 
% removes all spurious features and 
leads the first-layer ReLU weights to approximately project onto the ground-truth $r$-dimensional feature space, with error diminishing with $T$ and the number of samples per task $n$ as roughly $2^r\frac{\sqrt{d}}{\sqrt{T}}(1 + \frac{\sqrt{d}}{\sqrt{n}})$ (see Proposition \ref{prop:1} and Theorem \ref{thm:1}).  The key to this result is showing   that updating task-specific heads prior to the representation induces a {\em pseudo-contrastive loss function of the representation}, which encourages learning the ground-truth features  to align points likely to share a label on a randomly drawn task (see Section \ref{sec:sketch}).
% as long as the number of pretraining tasks $T$ satisfies $T > 2^{2r} d$ and the number of samples per task satisfies $n > 2^{2r}d^2/T$. 

% \item sample complexity
% \vspace{-1mm}

% In particular, this contrastive loss encourages representations of pairs of points that are likely to have the same label on a randomly drawn task to be similar, and representations of pairs of points that are unlikely. 
% is the label-weighted average of the features 
% We formally capture this idea and prove that it enables feature learning.

\item \textbf{Generalization guarantees.} We show that we can add a random ReLU layer on top of the pretrained representation, then train a linear layer on top of this random layer with finite samples, to solve {\em any} downstream task with binary labels that are a function of the $r$ important features. 
% Here, these $r$ features are discrete-valued, whereas during pretraining they are continuous. 
Crucially, we prove that  the sample and neuron complexity of solving the downstream task are independent of the ambient dimension $d$ (see Theorem \ref{thm:downstream}).
% \vspace{-1mm}

\item \textbf{Negative results.} We confirm the necessity of multi-task pretraining by proving that using a random features model (no pretraining) or pretraining on only a {\em single}, randomly-selected task with high probability require neuron or sample complexity scaling polynomially in $d$ for solving a downstream task (see Theorems \ref{thm:lower} and \ref{thm:single}).

% \item \textbf{Task-specific heads facilitate representation learning.}
% meaning pretraining effectively reduces the problem dimensiona dn achi
% the representation weights are dominated by their projections onto the ground-truth subspace, and are nearly isotropic within the ground-truth space. 
% This allows us to show that 

% \item \textbf{Experimental validation.} We verify our theoretical results on synthetic data in Section \ref{sec:sims}. {\color{red}{needs to be expanded}}
    % \item \textbf{Necessity of head adaptation.} We confirm that the task-specific adaptation of the head is critical to representation learning by proving  that gradient descent on a single model (with no task-specific adaptation) cannot learn the ground-truth features in a simple setting that is a special case of the general setting considered in our positive result. 
    % \textbf{Lower bound on the representation learning ability of single-model gradient descent.}
    % We confirm that the task-specific adaptation of the head is critical to representation learning by proving  that gradient descent on a single model (with no task-specific adaptation) cannot learn the ground-truth features in a simple setting that is a special case of the general setting considered in our positive result. The failure of single-model gradient descent is due to conflicting gradients, consistent with practice.
    % \item non-linearity is essential? yes for downstream but not for pretraining...
    % lower bound setting is not overparameterized
\end{itemize}


% \vspace{-2mm}
%\begin{comment}
\begin{figure}\label{fig:multi}
 \centering
 % \vspace{-3em}
  \includegraphics[width=0.96\linewidth]{Figures/num_tasks125mean.pdf}
 \caption{\textbf{Representation learning error vs  training iterations with varying numbers of tasks $T$.} 
 Here we sample tasks from the uniform distribution over sparse parity tasks on $r$ binary coordinates determined by $\sign(\mathbf{Mx})$ for some row-orthogonal matrix $\mathbf{M}$ and $d$-dimensional input $\mathbf{x}$. Here $d=32$, $r=3$,
 % $d\!=\!16$ and $r\!=\!4$, 
 and the learning model  is a two-layer, $m$-neuron ReLU network with first-layer weights $\mathbf{W}\!\in\! \mathbb{R}^{m\times d}$ (the representation). All cases use the same total number of training samples, i.e. the number of samples/task is inversely proportional to the number of training tasks $T$. Still, as $T$ increases, the row space of  $\mathbf{W}$ approaches that of $\mathbf{M}$ (smaller representation learning error).  Please see Appendix \ref{sec:sims} for  details.}
\end{figure}
%\end{comment}
% \vspace{-2mm}

\textbf{Notations.} We uppercase boldface to denote matrices, lowercase boldface to denote vectors, and standard typeface to denote scalars.
% , and calligraphy to denote sets. 
% We use $\mathbf{x}_{:r}$ to denote the first $r$ elements of the vector $\mathbf{x}$, and $\mathbf{x}_{r:}$  to denote the remaining elements.  
We employ $\text{Unif}(\mathcal{S})$ to denote the uniform distribution over the set $\mathcal{S}$.
We  denote the zero vector in $\mathbb{R}^d$ as $\mathbf{0}_d$, the  identity matrix in $\mathbb{R}^{d\times d}$ as $\mathbf{I}_d$, the standard multivariate normal distribution over $\mathbb{R}^d$ as $\mathcal{N}(\mathbf{0}_d,\mathbf{I}_d)$, and the Rademacher hypercube in $\mathbb{R}^d$ as $\mathcal{H}^d \coloneqq \{-1,1\}^d$. We denote the space of $r \times d$ matrices with orthonormal rows as $\mathbb{O}^{r\times d}$, and use $\chi\{A\}$ as the indicator function for the event $A$. We denote the set $\{1,\dots,r\}$ as $[r]$. We use ${\Omega}(\cdot),{\Theta}(\cdot)$ and ${O}(\cdot)$  in the standard fashion, and   $\tilde{\Omega}(\cdot),\tilde{\Theta}(\cdot)$ and $\tilde{O}(\cdot)$ to denote scalings up to logarithmic factors.


% "This return to “freezing” pre-trained
% models is appealing, especially as model size continues to increase. Rather than requiring a separate
% copy of the model for each downstream task, a
% single generalist model can simultaneously serve
% many different tasks." https://arxiv.org/pdf/2104.08691.pdf


==> Introduction.tex <==
\section{Introduction} 
\label{sec:intro}

% Although much progress has been made in understanding the dynamics of neural networks trained with gradient-based methods in recent years, empirical innovation in deep learning continues to outpace theoretical development. A particularly stark example of this concerns multi-task learning.
% In practice, there has been a movement towards pre-training massive models that can solve  many tasks with a small  amount of fine-tuning, at the expense of huge computational resources required for pre-training \citep{chowdhery2022palm,smith2022using}. 
% A a result, it is imperative for modern models to be able to solve many tasks simultaneously, or after some  small amount of fine-tuning, rather than re-training the model from scratch for each task. 
% To ensure these models can indeed generalize to many tasks, they are typically pre-trained via multi-task learning, which aims to jointly optimize a set of loss functions, each corresponding to a different task. 
% , with the goal of finding a model that performs well on each task as well as downstream tasks, perhaps after fine-tuning some or all of the model layers.
% \textcolor{blue}{It's not clear what the point of the last few sentences is. Maybe you wanna say that empirically there has been a huge success in pretraining large models and then fine-tuning them, but theoretically there is not that much understanding on the dynamics?}

Recent empirical results have demonstrated huge successes in pre-training large neural networks on many tasks with gradient-based algorithms \citep{%aghajanyan2021muppet,zhong2021adapting,sanh2021multitask,wang2022benchmarking,
crawshaw2020multi,zhang2021survey,
wang2023multitask,daras2022multitasking,wei2021finetuned,bubeck2023sparks}. These works suggest that the generalization capabilities of the pre-trained representation scales with the number of tasks used for pre-training.
% Multiple studies have further demonstrated that pre-training on a variety of tasks is not only sufficient but also necessary for effective downstream model performance \citep{}. 
%lu202012,liu2016recurrent,

% Multi-task learning has achieved a variety of success in practice . 
% For example, it has been observed that pre-training large language models (LLMs) on multiple diverse tasks can lead to learning more robust features for  downstream task performance \citep{daras2022multitasking,bubeck2023sparks}. 
% This penomenon 

At the same time, significant progress has been made in theoretically understanding the dynamics of neural networks trained with gradient-based methods in recent years, especially in regards to proving that shallow neural networks can learn meaningful features when trained with gradient descent and its variants \cite{damian2022neural,shi2022theoretical,abbe2022merged,allen2019learning,bai2019beyond,li2020learning,daniely2020learning,barak2022hidden,telgarsky2022feature,akiyama2022excess,zhou2021local}. 
However, these results are  limited to single-task settings, so they cannot explain the practical improvements in model performance seen by pre-training on many tasks. While a few studies exist showing the benefit of multi-task pre-training with gradient-based algorithms to representation learning \cite{thekumparampil2021sample,collins2022maml,collins2021exploiting,saunshi2021representation,sun2021towards,chua2021fine,bullins2019generalize,chen2022active}, these analyses are  limited to linear models and therefore it is not clear whether these results can generalize to even simple non-linear neural  networks.

In this work, we aim to bridge this gap by analyzing the dynamics of the parameters of a two-layer ReLU network pre-trained with a generic gradient-based multi-task learning algorithm on many binary classification tasks.  Following a long line of works analyzing feature learning dynamics in single-task \cite{damian2022neural,shi2022theoretical,abbe2020poly,abbe2022merged,daniely2020learning,telgarsky2022feature,maurer2016benefit,du2020fewshot} and linear \citep{thekumparampil2021sample,collins2022maml,collins2021exploiting,saunshi2021representation,sun2021towards,chua2021fine,bullins2019generalize,chen2022active,tripuraneni2020provable} settings, we suppose the existence of a ground-truth low-dimensional subspace that preserves all information in the data relevant to its label. Furthermore, in the multi-task setting of this paper we assume this subspace is shared among all tasks.
We ask whether a variant of gradient descent applied to this  multi-task setting can learn a representation that projects input data onto the ground-truth subspace. Learning such a representation is a proxy for successful pre-training, since it allows the model to easily be fine-tuned to solve downstream tasks by optimizing a number of last-layer model parameters that scales only with the dimension of this low-dimensional subspace, rather than the potentially very large ambient dimension of the data.
% It is advantageous to learn such a representation because the model can drastically reduce the dimension of the data
% Still, much is unknown about which specific algorithms are most effective and, most importantly, why. On the empirical side, many works have focused on the issue of conflicting gradients, showing that  when running standard gradient descent to minimize the average task loss with a single model, diverse objective functions for each task can cause conflicting task-specific gradients that lead to information loss when aggregating these gradients globally. A variety of sophisticated  techniques have been proposed to address this issue \citep{chen2018gradnorm}, yet simple modifications of the standard gradient descent, such as learning a shared early model layers (representation) with task-specific last layers (heads), seem to work at least as well as their more sophisticated counterparts
% % , and even in the face of objective heterogeneity  
% \citep{xin2022current,kurin2022defense}. We refer to this general, widely popular multi-task learning method of learning a shared representation and task-specific heads as Multi-Task Representation Learning (MTRL).

% {\color{gray}

% Despite its relative simplicity, our theoretical understanding of MTRL is nascent. 
% There are a few examples of recent works theoretically studying the effectiveness of MTRL and closely related algorithms in both generic multi-task learning contexts as well as in more specific multi-task settings such as federated learning \citep{collins2021exploiting,} and meta- or few-shot learning \citep{collins2022maml,thekumparampil2021statistically}. However, these analyses are either limited to linear settings \citep{collins2021exploiting,collins2022maml,thekumparampil2021statistically,}
% % assume the dimension of the ground-truth representation is known by the learner, 
% or only consider the landscape induced by the MTRL objective, not the feature learning process of the algorithm \citep{du2020fewshot,tripuraneni2020provable}. On the other hand, many works have studied feature learning in (nonlinear) neural networks, yet the vast majority consider only single-task settings, which involve fundamentally different dynamics than in the multi-task case. 

% In this work, we bridge this gap by analyzing the dynamics of the MTRL and single-model gradient descent algorithms on a one-hidden-layer ReLU network. We employ a labelled data generating model in which the input data is a linear combination of dictionary features determined by a Gaussian latent variable, and the  labels for each binary classification  task are a distinct function of the latent Gaussian coordinates of a small of ground-truth features common across tasks. The goal for multi-task learner is therefore to recover the shared set of label-relevant features. }

% Learning models that can perform well on a variaety of tasks

% In recent years, the impressive performances of large language models on a variety of natural language processing tasks have highlighted the potential for 

% Multi-task pre-training 

% Here' we use task
% We use `task specific adaptation' as a generic term encompassing a variety of algorithmic techniques used to adapt a global model to particular tasks, including designating model parameters as task-specific and executing 
% so-called inner-loop updates in meta-learning and local updates in federated learning. 
We prove that gradient-based  multi-task learning with a two-layer ReLU network with first-layer parameters (the representation) shared among all tasks and last-layer weights (the head) learned uniquely for each task is indeed able to recover the ground-truth subspace.
% after one gradient descent update of task-specific last model layer parameters followed by one gradient descent update  of the first-layer model parameters. % while single-model gradient descent cannot be guaranteed to  recover the ground-truth features.
% Our results therefore show for the first time that multi-task  representation learning is not an artifact of linearity.  
% -- suggesting that the feature learning demonstra in previous settings is not due to the linear nature of the model studied 
% but a fundamental property of the MTRL approach.
In summary, our main contributions are as follows:
\begin{itemize}[leftmargin=10mm]
% \setlength{\itemindent}{-1em}
% \setlength{\parindent}{-2em}
 
% We allow for tasks of arbitrary complexity during pre-training, as long as they are functions of the signs of the coordinates of $r$ label-relevant features in the data, where $r$ is taken to be much less than the ambient dimension of the data, $d$, and the aggregated set of pre-training tasks satisfy a natural
% certain diversity assumption. 
% We show that the representation learned during multi-task pre-training with MTRL allows for learning the set of $p$-degree polynomials on the signs of the ground-truth latent coordinates by training a linear probe on top of the learned features with $O(r^p)$ neurons and $O()$ samples. In contrast, using random model weights without any pre-training, i.e. the NTK regime, would require $\Omega(d^p)$ neurons to learn a downstream task in this family.

% Features emerge after one update of the representation parameters from Gaussian initialization as long as the task-specific heads are properly trained. Result for both perfect training of the heads and partial training.%(error of feature learning will be exactly the error from partial training of heads. note partial training includes training with finite samples. will need to use concentration results on hypercube. but regardless will still need 2k samples...
% can also show concentration result for tasks. finite rep samples per task with finite tasks is difficult thugh...argue that in the age of foundation model pretraining we have infinte samples effectively
% We don't need to know the dimension of the representation. We provide downstream task performance guarantees.

\item \textbf{Proof of multi-task representation learning with two-layer ReLU network.} We consider binary classification tasks whose labels are functions of only $r$ features of the input data, where $r$ is much smaller than the ambient dimension $d$. 
% Under the assumption that  two points with differing $r$ important features are equally likely to have the same label  on a randomly drawn task as not, 
We prove that one gradient descent update of each of the task-specific heads followed by one gradient descent update of the representation removes all spurious features and leads to a dense projection onto the ground-truth $r$-dimensional feature space as long as the number of pre-training tasks $T \gg r2^{2r} d^2$. 


\item \textbf{Insight that task specific heads induce a contrastive loss that facilitates representation learning.} Key to our proof is showing that updating task-specific heads prior to the representation induces a contrastive loss function of the representation, which encourages learning the ground-truth features in order to align points likely to share a label on a randomly drawn task. 
% In particular, this contrastive loss encourages representations of pairs of points that are likely to have the same label on a randomly drawn task to be similar, and representations of pairs of points that are unlikely. 
% is the label-weighted average of the features 
% We formally capture this idea and prove that it enables feature learning.

\item \textbf{Downstream guarantees.} We show that we can add a random ReLU layer on top of the pre-trained representation, then train a linear layer on top of this random layer with finite samples, to solve {\em any} downstream task with binary labels that are a function of the $r$ important features. 
% Here, these $r$ features are discrete-valued, whereas during pre-training they are continuous. 
Crucially, we prove that  the sample and neuron complexity required for solving the downstream task are independent of the ambient dimension $d$, making it exponentially smaller in $d$ than the complexity required for solving such tasks with a random feature representation (see Theorems \ref{thm:downstream} and \ref{thm:lower}).
% meaning pre-training effectively reduces the problem dimensiona dn achi
% the representation weights are dominated by their projections onto the ground-truth subspace, and are nearly isotropic within the ground-truth space. 
% This allows us to show that 

% \textbf{Experimental validation.} We verify on synthetic data that 
    % \item \textbf{Necessity of head adaptation.} We confirm that the task-specific adaptation of the head is critical to representation learning by proving  that gradient descent on a single model (with no task-specific adaptation) cannot learn the ground-truth features in a simple setting that is a special case of the general setting considered in our positive result. 
    % \textbf{Lower bound on the representation learning ability of single-model gradient descent.}
    % We confirm that the task-specific adaptation of the head is critical to representation learning by proving  that gradient descent on a single model (with no task-specific adaptation) cannot learn the ground-truth features in a simple setting that is a special case of the general setting considered in our positive result. The failure of single-model gradient descent is due to conflicting gradients, consistent with practice.
    % \item non-linearity is essential? yes for downstream but not for pretraining...
    % lower bound setting is not overparameterized
\end{itemize}




\textbf{Notations.} We uppercase boldface to denote matrices, lowercase boldface to denote vectors, standard typeface to denote scalars.
% , and calligraphy to denote sets. 
We use $\mathbf{x}_{:r}$ to denote the first $r$ elements of the vector $\mathbf{x}$, and $\mathbf{x}_{r:}$  to denote the remaining elements.   We use $\text{Unif}(\mathcal{T})$ to denote the uniform distribution over the set $\mathcal{T}$.
We use $\mathbf{0}_d$ to denote the $d$-dimensional vector of zeros, $\mathbf{I}_d$ to denote the $d$-by-$d$-dimensional identity matrix, and $\mathcal{N}(\mathbf{0}_d,\mathbf{I}_d)$ to denote the $d$-dimensional multivariate normal distribution.



% "This return to “freezing” pre-trained
% models is appealing, especially as model size continues to increase. Rather than requiring a separate
% copy of the model for each downstream task, a
% single generalist model can simultaneously serve
% many different tasks." https://arxiv.org/pdf/2104.08691.pdf


==> Notes_multi-step.tex <==





\begin{lemma} \label{lem:second}
    Second step
\end{lemma}


\begin{proof}
From Lemma \ref{lem:first}, we have that for each neuron $j$,
$\mathbf{w}_{j,1} = \tilde{\w}_{j,0} +\mathbf{n}_{j,0} $
where $\tilde{\w}_{j,0}:= \begin{bmatrix}
    (1+\eta 2^{-r-2} -\eta\lambda )\mathbf{w}_{||} \\
    (1+\eta 2^{-r-2} \frac{2}{\pi} -\eta\lambda )\mathbf{w}_{\perp } \\
\end{bmatrix}$ and $\|\mathbf{n}_{j,0} \|_2 \leq \frac{c}{\sqrt{k}} \|\w_{j,0}\|_2$.




% This means that 

% \begin{align}
%     \nabla_{\w_j}\mathcal{L}_i()
% \end{align}

% \begin{align}
%     \|\mathbf{A}(\tilde{\w}_{j,0}) - \mathbf{A}(\tilde{\w}_{j,0}+\mathbf{n}_{j,0})\|_2
% \end{align}

% P is 1/rt(k)
% meaning there are 1/rt(k) times 2**k
%  suffixes that might change

% worst case is when n is propto standard basis vector, w is propto ones vector
% in this case norm of epxectation is norm of n


% but parallel part is same norm as error... may get overriden ... screwed

% options:

% show these second moments are actually 1/k4

% show tighter bound on norm of off-diagonal sub-blocks (would be sufficient)

% ....need to figure out how many iterations we need before we no longer need isotropicity

% but we do always need Aparapara to be close to identity

% it would be sufficient for either all xi approx half or half xi approx full

% % as para part gets larger, xi's don't necessarily change

% at start, all xi approx half. then, for larger para, some xis become full and others become empty, but not all will polarize
%  % which should be fine

%  if we only care about norm and not direciton:

%  we can upper bound 

%  to do:

%  write up apara proof

%  figure out how many steps we need before we no longer need isotrop

 

%  come up with strategy for second step.



 \begin{align}
     &\E_{\w_{\perp}}\left[\sum_{i=1}^{k-r} w_{\perp,i}\left(\E_{\vv}[\sigma'(\vv^\top \w_{\perp} -b) v_i]- \E_{\z}[\sigma'(\z^\top \w_{\perp} -b) z_i]\right)\right] \nonumber \\
     &= \sum_{i=1}^{k-r} \E_{\vv}\left[\E_{\w_{\perp}}\left[w_{\perp,i}\sigma'(\vv^\top \w_{\perp} -b)\right] v_i\right]- \E_{\z}\left[\E_{\w_{\perp}}\left[w_{\perp,i}\sigma'(\z^\top \w_{\perp} -b) \right]z_i \right] \nonumber \\
     &= \sum_{i=1}^{k-r} \E_{\vv}\left[\E_{\w_{\perp}}\left[w_{\perp,i}\sigma'(\vv^\top \w_{\perp} -b)\right] v_i\right]- \E_{\z}\left[\E_{\w_{\perp}}\left[w_{\perp,i}\sigma'(\z^\top \w_{\perp} -b) \right]z_i \right] \nonumber \\
     &= \sum_{i=1}^{k-r} \E_{\vv}\left[\E_{\w_{\perp}}\left[w_{\perp,i}\sigma'(\vv^\top \w_{\perp} -b)\right] v_i\right]- \E_{\z}\left[\E_{\w_{\perp}}\left[w_{\perp,i}\sigma'(\z^\top \w_{\perp} -b) z_i\right] \right] \nonumber \\
     &= \sum_{i=1}^{k-r} \sqrt{\frac{2}{\pi}} \left( \frac{1}{\sqrt{k}} - \E_{\z}\left[\frac{z_i^2}{\|[\uu, \z]\|_2} \right]\right) \\
     &= \sqrt{\frac{2}{\pi}} \left( \frac{k-r}{\sqrt{k}} - \E_{\z}\left[\frac{\sum_{i=1}^{k-r} z_i^2}{\sqrt{r + \sum_{i=1}^{k-r}z_i^2}} \right]\right) 
     \end{align}
     this is not zero. but it is diminishing with k.
     
     \begin{align}
     &\sum_{i=1}^{k-r}\sum_{i'=1}^{k-r} w_{\perp,i}w_{\perp,i'}\left(\E_{\vv}[\sigma'(\vv^\top \w_{\perp} -b) v_i]- \E_{\z}[\sigma'(\z^\top \w_{\perp} -b) z_i]\right)\left(\E_{\vv}[\sigma'(\vv^\top \w_{\perp} -b) v_{i'}]- \E_{\z}[\sigma'(\z^\top \w_{\perp} -b) z_{i'}]\right)
 \end{align}



 
idea to sum over k coords rather than argue coordinate wise should help. 
in order to do this, we need ot multiply with w.

make sure that stein's lemma doesn't help.

again move expectation over w inside. write bias explicityl in terms of prefix.. divide into three exps: wi, wi', and the other wj's. Put i,i' on the outside, should be able to get a similar arccos thing with wi,wi' fixed. 



multiple issues:

1. off diag may dominate parallel: use that off diag is also aligned

2. norms of para, perp are coupled with their direcitons: new analysis should give imprved bounds when norm of para is larger

3. exit strategy?

a. perp becomes zero.

Induction should be something like: 

1. for any bias b (corresponding to norm of wpara essentially), the expected value of the perp vector is a scalar (that depends on bias) times wperp0 plus some small discretization error.
- this means that perp stays aligned -- but how to deal with accumulating errors?
- note this does not use the r=0 approximation
- can tighten this by looking at projection onto wperp0
- const should shrink with bias, slowly at first then faster, until constant becomes zero.  this is the key thing, because this can be used to show shrinking discretization error and then easier alignment of wperp, and ultimately the exit condition. alginment of wpara will still be tough...

2. Apara is always close to scaled identity, with constant lower bound. does bound on this rely on gaussianity? yes, but 

3. off diags are aligned and small

4. note there are 2**r-1 positive prefixes and 2**k-r-1 posiitve suffixes. As wpara grows, more pos prefixes become larger than positive suffixes. for a given pos prefix, let yi...
- how to track decrease in norm of Aperp...

5. 

first need to show that para and perp are aligned.


\begin{align}
    a_{t+1} &\geq a_t\left(1 - \eta \lambda + \eta 2^{-r-2} + \eta 2^{-r-2} \tfrac{2}{\pi}\left(1 - \tfrac{a_t^2\|\mathbf{w}_{0,||}\|_2^2}{b_t^2 \|\mathbf{w}_{0,\perp}\|_2^2}\right) \right) - {\color{red} \eta c_4 \left(\left(\frac{1}{k}  +\|\mathbf{n}_t\|_2\right)a_t\|\mathbf{w}_0\|_2 + \|\mathbf{n}_t\|_2 \right) }   \end{align}

\begin{align}
    \w_{t+1,\perp} &= b_t(1-\eta \lambda)\w_{0,\perp} + (1-\eta \lambda)\mathbf{n}_{t,\perp} + \eta  2^{-r-2} \frac{2}{\pi} b_t\frac{ a_t^2\|\mathbf{w}_{0,||}\|_2^2}{ b_t^2\|\mathbf{w}_{0,\perp}\|_2^2} \left( 1 - \frac{  a_t^2 \|\mathbf{w}_{0,||}\|_2^2 }{ 2b_t^2 \|\mathbf{w}_{0,\perp}\|_2^2 } \right)  \mathbf{w}_{0,\perp} \nonumber \\
    &\quad + \eta 2^{-r-2}  \frac{2}{\pi} b_t \left( 1 - { \frac{a_t^2 \|\mathbf{w}_{0,||}\|_2^2 }{b_t^2 \|\mathbf{w}_{0,\perp}\|_2^2} } \right)  \mathbf{w}_{0,\perp} + {\color{red} \eta c_4 \left(\left(\frac{1}{k}  +\|\mathbf{n}_t\|_2\right)a_t\|\mathbf{w}_0\|_2 + \|\mathbf{n}_t\|_2 \right) } 
\end{align}

    
    \begin{align}
    b_{t+1} &\leq b_t\left(1 - \eta \lambda + \eta 2^{-r-2} \tfrac{2}{\pi} \tfrac{ a_t^2\|\mathbf{w}_{0,||}\|_2^2}{ b_t^2\|\mathbf{w}_{0,\perp}\|_2^2} \left(1 - \tfrac{a_t^2\|\mathbf{w}_{0,||}\|_2^2}{b_t^2 \|\mathbf{w}_{0,\perp}\|_2^2}\right) + \eta 2^{-r-2}  \tfrac{2}{\pi} \left( 1 - { \tfrac{a_t^2 \|\mathbf{w}_{0,||}\|_2^2 }{b_t^2 \|\mathbf{w}_{0,\perp}\|_2^2} } \right) \right) \nonumber \\
    &\quad + {\color{red} \eta c_4 \left(\left(\frac{1}{k}  +\|\mathbf{n}_t\|_2\right)a_t\|\mathbf{w}_0\|_2 + \|\mathbf{n}_t\|_2 \right) }  \\
    &= b_t\left(1 - \eta \lambda  + \eta 2^{-r-2}  \tfrac{2}{\pi} \left( 1 - { \tfrac{a_t^4 \|\mathbf{w}_{0,||}\|_2^4 }{b_t^4 \|\mathbf{w}_{0,\perp}\|_2^4} } \right) \right) + {\color{red} \eta c_4 \left(\left(\frac{1}{k}  +\|\mathbf{n}_t\|_2\right)a_t\|\mathbf{w}_0\|_2 + \|\mathbf{n}_t\|_2 \right) }  \\
    \|\mathbf{n}_{t+1}\|_2 &\leq  \left(1 - \eta \lambda  + \eta c_2  +  \eta c_3 ( a_t \|\mathbf{w}_0\|_2 + \|\mathbf{n}_t\|_2) \right) \|\mathbf{n}_t\|_2 + \eta \tfrac{c_1}{k} a_t \|\mathbf{w}_0\|_2  
\end{align}
{\color{blue} As long as $\|\mathbf{w}_0\|$ is sufficiently small, this system behaves as desired because $b_t$ goes to zero long before $a_t$, and while $\|\mathbf{n}_t\|_2$ is still small. This implies that we eventually have $\w_t \approx [\w_{0,||},0]$ as desired.}


% Need to balance growth of $a_t$ with decrease of others.

% check if the above recursion is viable. note it is self-contained.

% go until at/bt = rt(k)

% Need to control E3t


With high probability:
\begin{align}
    \|\E_{\mathbf{v}}[v_1 \sigma'( \mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )] - \E_{\mathbf{z}}[z_1 \sigma'( \mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )] \|_2 &= O\left(\frac{1}{k} \right) 
\end{align}
since
\begin{align}
   \E_{\w}\left[\left(\E_{\mathbf{v}}[v_1 \sigma'( \mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )] - \E_{\mathbf{z}}[z_1 \sigma'( \mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )]\right)^2 \right] &= O\left(\frac{1}{k^4} \right) 
\end{align}
and this should actually decrease as $a_t/b_t$ increases (good)

the question is do we need to union bound over all $a_t, b_t$ (and pay an extra $\log(T)$ penalty)? yes i think so. and if we need to pay this penalty, is it better to not pay it and simply upper bound the $a_t,b_t$ norm by the above $a_t,b_t=1,1$ case?

{\color{red}
All that remains to show is:
\begin{lemma}
   \begin{align}
    \left\|\mathbf{A}([a_t,b_t] \mathbf{w}_0+\mathbf{n}_t) - \mathbf{A}([a_t,b_t]\mathbf{w}_0 ) \right\|_2 &= O(\|\mathbf{n}_t\|_2) \nonumber 
\end{align} 
\end{lemma}

\begin{proof}

   \begin{align}
   &\left\|\mathbb{E}_{\mathbf{v}} \left[\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v} + \mathbf{w}^\top \mathbf{n})\mathbf{v}\right] - \mathbb{E}_{\mathbf{v}} \left[\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]\right\|_2 \nonumber\\
   &= \left\|\mathbb{E}_{\mathbf{v}} \left[\left(\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v} + \mathbf{w}^\top \mathbf{n}) - \sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v})\right)\mathbf{v}\right] \right\|_2  \nonumber \\
   &= \left\|\mathbb{E}_{\mathbf{v}} \left[\chi\left\{\mathbf{w}^\top \mathbf{n} > -a_t \mathbf{w}_{||}^\top \mathbf{u}- b_t \mathbf{w}_{\perp}^\top \mathbf{v} >  0  \right\}\mathbf{v}\right] - \mathbb{E}_{\mathbf{v}} \left[\chi\left\{ \mathbf{w}^\top \mathbf{n} < -a_t \mathbf{w}_{||}^\top \mathbf{u}- b_t \mathbf{w}_{\perp}^\top \mathbf{v} <  0  \right\}\mathbf{v}\right] \right\|_2  \nonumber 
\end{align} 

% Note that by symmetry of $\w$,
% \begin{align}
%    \mathbb{E}_{\mathbf{w}}  \mathbb{E}_{\mathbf{v}} \left[\chi\left\{\mathbf{w}^\top \mathbf{n} > -a_t \mathbf{w}_{||}^\top \mathbf{u}- b_t \mathbf{w}_{\perp}^\top \mathbf{v} >  0  \right\}\mathbf{v}\right] &= \mathbb{E}_{\mathbf{w}} \mathbb{E}_{\mathbf{v}} \left[\chi\left\{ \mathbf{w}^\top \mathbf{n} < -a_t \mathbf{w}_{||}^\top \mathbf{u}- b_t \mathbf{w}_{\perp}^\top \mathbf{v} <  0  \right\}\mathbf{v}\right] \nonumber
% \end{align}



\begin{align}
    a
\end{align}


Option 1: can add activation noise. Would address first problem.

Option 2: bias won't work because it will be coupled with weight. Label noise might work.

Option 3: show that w whp cannot be perturbed to change set of positive vertices significantly.

Option 4: The worst case perturbation of w is some simple projection onto an orthogonal subspace.

    - But it is not the same projection (e.g. project onto line resulting from rotating w 90 degrees left) every time. evidenced by 2 dimensional case.

    - But it is a projection onto an orthogonal space. F

\end{proof}

}


Induction:
\begin{enumerate}
    \item 
\end{enumerate}

\end{proof}







\newpage


% where $a_t > 1$ is a scalar, $b_t < 1$ is a scalar that  converges to zero, and $\|\mathbf{n}_t\|_2 = O\left(\tfrac{\|\w_0\|_2}{k}\right)$ and is orthogonal to $\w_0$.

We have

\begin{align}
    \mathbf{w}_{t+1} &= (1 - \eta \lambda) \w_t + \eta \mathbf{A}(\w_t)\w_t,
\end{align}
where $
    \mathbf{A}(\mathbf{w}_t) := \begin{bmatrix}
       \mathbf{A}_{\parallel,\parallel}(\mathbf{w}_t)
          & \mathbf{A}_{\parallel,\perp}(\mathbf{w}_t)  \\
          \mathbf{A}_{\perp,\parallel}(\mathbf{w}_t) &  \mathbf{A}_{\perp,\perp}(\mathbf{w}_t)   \\
    \end{bmatrix}
$ and
\begin{align}
    \mathbf{A}_{||,||}(\mathbf{w}) &:= 2^{-r} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[ \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}} \left[\sigma'( \mathbf{w}_{||}^\top \mathbf{u}+  \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2 \mathbf{uu}^\top  \right] \\
    \mathbf{A}_{||,\perp}(\mathbf{w}) &:= 2^{-r} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[ \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}} \left[\sigma'(  \mathbf{w}_{||}^\top \mathbf{u}+  \mathbf{w}_{\perp}^\top \mathbf{v} )\right] \mathbf{u} \; \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}}\left[\sigma'( \mathbf{w}_{||}^\top \mathbf{u}+  \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right] \\
    \mathbf{A}_{\perp,||}(\mathbf{w}) &:= 2^{-r} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[  \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}}\left[\sigma'( \mathbf{w}_{||}^\top \mathbf{u}+  \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right] \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}} \left[\sigma'(  \mathbf{w}_{||}^\top \mathbf{u}+  \mathbf{w}_{\perp}^\top \mathbf{v})\right] \mathbf{u}^\top  \right] \\
    \mathbf{A}_{\perp,\perp}(\mathbf{w}) &:= 2^{-r} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[  \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}}\left[\sigma'( \mathbf{w}_{||}^\top \mathbf{u}+  \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]  \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}}\left[\sigma'( \mathbf{w}_{||}^\top \mathbf{u}+  \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right] 
\end{align}
where $\mathbf{u}\sim \mathcal{H}^{r}$ denotes a uniform sample from the Rademacher hypercube in $r$ dimensions.

WLOG let $\w_t = [ a_t \w_{0,\parallel}; b_t \w_{0,\perp} ] + \mathbf{n}_t,$ where $\mathbf{n}_{t,\parallel}^\top \w_{0,\parallel}=0$ and $\mathbf{n}_{t,\perp}^\top \w_{0,\perp}=0$. Denote
\begin{align}
   & \mathbf{A}^{\star}([a_t\w_{0,\parallel},b_t\w_{0,\perp}]) \nonumber \\
   &:= \begin{bmatrix}
       { 2^{-r-2} } \mathbf{I}_r
          & 2^{-r-2} \frac{2 a_t}{\pi b_t}  \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[   \mathbf{u}\mathbf{u}^\top  \exp\left(-\frac{a_t^2 (\mathbf{w}_{0,\parallel}^\top \mathbf{u})^2 }{ 2b_t^2 \|\mathbf{w}_{0,\perp}\|_2^2 } \right)   \right]   \frac{\mathbf{w}_{0,\parallel} \mathbf{w}_{0,\perp}^\top}{\|\mathbf{w}_{0,\perp}\|_2^2}  \\
          2^{-r-2} \frac{2 a_t}{\pi b_t} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[   \mathbf{u}\mathbf{u}^\top \exp\left(-\frac{a_t^2 (\mathbf{w}_{0,\parallel}^\top \mathbf{u})^2 }{ 2b_t^2 \|\mathbf{w}_{0,\perp}\|_2^2 } \right)   \right]  \frac{\mathbf{w}_{0,\perp} \mathbf{w}_{0,\parallel}^\top}{\|\mathbf{w}_{0,\perp}\|_2^2}   & 2^{-r-2}  \frac{2}{\pi} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[  \exp\left(-\frac{a_t^2 (\mathbf{w}_{0,\parallel}^\top \mathbf{u})^2 }{ b_t^2 \|\mathbf{w}_{0,\perp}\|_2^2 } \right)   \right]   \frac{\mathbf{w}_{0,\perp}\mathbf{w}_{0,\perp}^\top}{\|\mathbf{w}_{0,\perp}\|_2^2}   \\
    \end{bmatrix}
\end{align}


We would like to show that $\mathbf{A}(\mathbf{w}_t) \approx \mathbf{A}([a_t\w_{0,\parallel},b_t\w_{0,\perp}] ) \approx  \mathbf{A}^{\star}([a_t\w_{0,\parallel},b_t\w_{0,\perp}])$, where $a_t$ is increasing and $b_t$ is decreasing to zero, for all iterations $t$ up to some iteration $T$ at which $b_T=0$ and $ \|[a_T\w_{0,\parallel},\mathbf{0}]\|_2 \gg \|\mathbf{n}_T\|_2 $.

% On the first gradient step, $a_0=b_0=1$, and $\mathbf{A}^{\star}([a_t\w_{0,\parallel},b_t\w_{0,\perp}]) = \mathbf{A}^{\star}(\mathbf{w}_0) $ is the matrix we shown 

To do this, I believe we need a two-phase analysis. In the first phase, $\frac{a_t}{b_t} \ll {\sqrt{k}}$, thus $ \exp\left(-\frac{a_t^2 (\mathbf{w}_{0,\parallel}^\top \mathbf{u})^2 }{ b_t^2 \|\mathbf{w}_{0,\perp}\|_2^2 } \right) \approx  1$. In this phase, $a_t$ increases linearly, $b_t$ decreases linearly, and $\|\mathbf{n}_t\|_2$ increases linearly (but it starts close to zero, so it remains dominated by $a_t$, as $a_0=1$).

We have shown that on the first iteration, $\|\mathbf{A}(\mathbf{w}_0)- \mathbf{A}^{\star}([a_0 \w_{0,\parallel},b_0 \w_{0,\perp}])\|_2 = O\left(\frac{1}{k}\right)$ with probability at least 0.99 over choice of $\mathbf{w}_0$ (trivially $a_0=b_0=1$ and $\mathbf{n}_0=\mathbf{0}$).

% To argue about subsequent steps, I believe we need a two-phase analysis. In the first phase, $\frac{a_t}{b_t} \ll {\sqrt{k}}$, thus $\exp\left( - { \frac{a_t^2 \|\mathbf{w}_{0,\parallel}\|_2^2 }{b_t^2 \|\mathbf{w}_{0,\perp}\|_2^2} } \right) \approx 1  - { \frac{a_t^2 \|\mathbf{w}_{0,\parallel}\|_2^2 }{b_t^2 \|\mathbf{w}_{0,\perp}\|_2^2} }\approx 1$. In this phase, $a_t$ increases linearly, $b_t$ decreases linearly, and $\|\mathbf{n}_t\|_2$ increases linearly (but sufficiently slowly). 

The inductive hypotheses for the rest of this phase are:

\begin{enumerate}
\item \begin{align}
     \left\|\mathbf{A}([a_t\w_{0,\parallel},b_t\w_{0,\perp}] ) - \mathbf{A}^\star([a_t\w_{0,\parallel},b_t\w_{0,\perp}] )\right\|_2 &\leq \tfrac{c_1}{k}
\end{align}

\item \begin{align}
     \left\|\mathbf{A}([a_t\w_{0,\parallel},b_t\w_{0,\perp}] + \mathbf{n}_t ) - \mathbf{A}([a_t\w_{0,\parallel},b_t\w_{0,\perp}])\right\|_2 &\leq {c_2}\frac{\|\mathbf{n}_t\|_2}{\| [a_t \mathbf{w}_{0,||};  b_t\mathbf{w}_{0,\perp}] \|_2}
\end{align}

    \item \begin{align}
    a_{t+1} &\geq \left(1 - \eta \lambda + \eta 2^{-r-2}(1+ \tfrac{2}{\pi} )\right)a_t - {\eta c_4 \left(\tfrac{a_t\|\mathbf{w}_0\|_2}{k}  + \|\mathbf{n}_t\|_2 \right) }   \end{align}
    \item     \begin{align}
    b_{t+1} &\leq 
   \left(1 - \eta \lambda  + \eta 2^{-r-2}  \tfrac{2}{\pi} \left( 1 + { \tfrac{a_t^2 \|\mathbf{w}_{0,\parallel}\|_2^2 }{b_t^2\|\mathbf{w}_{0,\perp}\|_2^2} } \right) \right)  b_t + {\eta c_4 \left(\tfrac{a_t\|\mathbf{w}_0\|_2}{k}  + \|\mathbf{n}_t\|_2 \right) }  \end{align}
    \item \begin{align}
    \|\mathbf{n}_{t+1}\|_2 &\leq   \left(1 - \eta \lambda  +  \eta c_3 ( 1+ \|\mathbf{n}_t\|_2) \right)\|\mathbf{n}_t\|_2 + \eta \tfrac{c_1}{k} a_t \|\mathbf{w}_0\|_2  
\end{align}
% \item $$\|\mathbf{n}_{t+1}\|_2 \leq  \tfrac{c_5}{k} \|\mathbf{w}_0\|_2 $$

\vspace{4mm}

where all $c_{\cdot}$'s are absolute constants. 






\end{enumerate}

\vspace{4mm}



% Empirically, as long as $\|\w_0\|_2$ is small, the dynamics described by inductive hypotheses 3,4,5 converge to $a_{T}> \Omega(\sqrt{k})$, $b_{T}=0$ and $\|\mathbf{n}_{T}\|_2 =  O(\tfrac{\|\mathbf{w}_0\|_2}{\sqrt{k}})$, thus the signal $[a_{T} \mathbf{w}_{0,\parallel}; \mathbf{0}]$ has Euclidean norm a factor  of $\sqrt{k}$ larger than that of the noise $\mathbf{n}_T$. $b_T$ converges linearly fast until some time at which the convergence becomes superlinear.



Inductive hypotheses 3,4,5 follow directly from the update rule for $\mathbf{w}_{t+1}$, inductive hypotheses $1,2$, and the definition of $\mathbf{A}^\star([a_t\mathbf{w}_{0,\parallel},b_t\mathbf{w}_{0,\perp}] )$. We need to make $\|\mathbf{w}_0\|_2\ll 1$  to ensure that $a_t$ dominates $\|\mathbf{n}_t\|_2$.




 
I am stuck on showing inductive hypotheses 1 and 2. 




% We need to show that $$\mathbf{A}_{\perp,\perp}(  [ a_t \w_{0,\parallel}; b_t \w_{0,\perp} ] ) \approx \left(1 -  \frac{a_t^2 ||\w_{0,\parallel}||^2}{ b_t^2 ||\w_{0,\perp}||^2}  \right)  \frac{2}{\pi ||\w_{0,\perp}||_2^2} \w_{0,\perp} \w_{0,\perp}^T,$$ where $\mathbf{A}_{\perp,\perp}(  \w )$ is the $\mathbf{A}_{\perp,\perp}$ matrix we've been discussing that results from the neuron weights $\w$. Note that this reduces to the $\mathbf{A}_{\perp,\perp}$ from the first step, since $a_0 = b_0 = 1$ and  $||\w_{0,\parallel}||^2/||\w_{0,\perp}||^2 = O(1/k)$, i.e. $\left(1 -  \frac{a_0^2 ||\w_{0,\parallel}||^2}{ b_0^2 ||\w_{0,\perp}||^2}  \right)  \approx 1.$
% The $\left(1 -  \frac{a_t^2 ||\w_{0,\parallel}||^2}{ b_t^2 ||\w_{0,\perp}||^2}  \right)$ factor results in a super-linear convergence rate, since the smaller that $b_t$ is, the larger contraction of $b_t$ in the update $b_{t+1}:$
% \begin{align}
%     b_{t+1} \lesssim b_t\left(1 - \eta \lambda +  \left(1 -  \frac{a_t^2 ||\w_{0,\parallel}||^2}{ b_t^2 ||\w_{0,\perp}||^2}  \right)  \frac{2}{\pi}   \right).
% \end{align}

% The induction holds as long as the following two missing steps hold:

% Each condition can be reduced to the following two conditions, respectively:


To show the first condition I want to show that $$\left\|\mathbf{A}([a_t\w_{0,\parallel},b_t\w_{0,\perp}] ) - \mathbf{A}^\star([a_t\w_{0,\parallel},b_t\w_{0,\perp}] )\right\|_2\leq c\left\|\mathbf{A}([\w_{0,\parallel},\w_{0,\perp}] ) - \mathbf{A}^\star([\w_{0,\parallel},\w_{0,\perp}] )\right\|_2$$ for a constant $c$. Intuitively this should be true because $a_t\geq 1$ and $b_t\leq 1$. To see this, note that upper bounding $\left\|\mathbf{A}([a_t\w_{0,\parallel},b_t\w_{0,\perp}] ) - \mathbf{A}^\star([a_t\w_{0,\parallel},b_t\w_{0,\perp}] )\right\|_2$ can be reduced to upper bounding
\begin{align}
  \left \| \mathbb{E}_{\mathbf{v}\sim \text{Unif}({\mathcal{H}^{k-r})}}\left[\sigma'( a_t \mathbf{w}_{0,||}^\top \mathbf{u}+  b_t\mathbf{w}_{0,\perp}^\top \mathbf{v})\mathbf{v} \right] - \mathbb{E}_{\mathbf{z}\sim \mathcal{N}(\mathbf{0},\mathbf{I})}\left[\sigma'( a_t\mathbf{w}_{0,||}^\top \mathbf{u}+  b_t \mathbf{w}_{0,\perp}^\top \mathbf{z})\mathbf{z} \right] \right\|_2
\end{align}
Since $a_t\geq 1$ and $b_t\leq 1$, these scalars place more weight on the term $\mathbf{w}_{0,||}^\top \mathbf{u}$ that is shared, and less weight on the term $\mathbf{w}_{0,\perp}^\top \mathbf{z}$ that differs. So we should have 
\begin{align}
 & \left \| \mathbb{E}_{\mathbf{v}\sim \text{Unif}({\mathcal{H}^{k-r})}}\left[\sigma'( a_t \mathbf{w}_{0,||}^\top \mathbf{u}+  b_t\mathbf{w}_{0,\perp}^\top \mathbf{v})\mathbf{v} \right] - \mathbb{E}_{\mathbf{z}\sim \mathcal{N}(\mathbf{0},\mathbf{I})}\left[\sigma'( a_t\mathbf{w}_{0,||}^\top \mathbf{u}+  b_t \mathbf{w}_{0,\perp}^\top \mathbf{z})\mathbf{z} \right] \right\|_2\nonumber \\
 &\leq c\left \| \mathbb{E}_{\mathbf{v}\sim \text{Unif}({\mathcal{H}^{k-r})}}\left[\sigma'(  \mathbf{w}_{0,||}^\top \mathbf{u}+  \mathbf{w}_{0,\perp}^\top \mathbf{v})\mathbf{v} \right] - \mathbb{E}_{\mathbf{z}\sim \mathcal{N}(\mathbf{0},\mathbf{I})}\left[\sigma'( \mathbf{w}_{0,||}^\top \mathbf{u}+  \mathbf{w}_{0,\perp}^\top \mathbf{z})\mathbf{z} \right] \right\|_2
\end{align}
where the constant $c$ allows for small discretization errors. In particular the above statement is not deterministically true for all $\mathbf{w}_{0}$ with $c=1$. However, empirically it seems to be true for a small constant $c>1$. Equivalently, we need to show $g(s) := \| \E_{\mathbf{v} \sim \text{Unif}(\mathcal{H})^{k-r} } [ \sigma'(  \w_{0,\perp}^T \mathbf{v} + s  ) \mathbf{v}] - \E_{\mathbf{z} \sim \mathcal{N}(\mathbf{0},\mathbf{I})} [ \sigma'(  \w_{0,\perp}^T \mathbf{z} + s  ) \mathbf{z}] ||_2 \leq c' g(0)$  for all scalars $s$, any $\w_{0,\perp} \in \mathbb{R}^{k-r}$, and an absolute constant $c'$. I don't think we can argue using the randomness of $\mathbf{w}_{0,\perp}$ because $a_t$ and $b_t$ are unknown functions of $\mathbf{w}_{0,\perp}$. 

Similarly, the second condition can be reduced to showing that 
\begin{align}
  &\bigg \| \mathbb{E}_{\mathbf{v}\sim \text{Unif}({\mathcal{H}^{k-r})}}\left[\sigma'( a_t \mathbf{w}_{0,||}^\top \mathbf{u}+  b_t\mathbf{w}_{0,\perp}^\top \mathbf{v} + \mathbf{n}_t^\top [\mathbf{u},\mathbf{v}])\mathbf{v} \right]- \mathbb{E}_{\mathbf{v}\sim \text{Unif}({\mathcal{H}^{k-r})}}\left[\sigma'( a_t \mathbf{w}_{0,||}^\top \mathbf{u}+  b_t\mathbf{w}_{0,\perp}^\top \mathbf{v} )\mathbf{v} \right] \bigg\|_2\nonumber \\
  &= O\left(\frac{\|\mathbf{n}_t\|_2}{\| [a_t \mathbf{w}_{0,||};  b_t\mathbf{w}_{0,\perp}] \|_2}\right)
\end{align}
Again I think we need to make a deterministic argument over all choices of $\mathbf{w}_0$, $a_t>1$, $b_t\in [0,1]$ and $\mathbf{n}_t$ since $a_t$, $b_t$ and $\mathbf{n}_t$  are unknown functions of $\mathbf{w}_{0,\perp}$. Intuitively, although $\sigma'$ is not smooth, $f(\mathbf{x})\coloneqq \mathbb{E}_{\mathbf{v}\sim \text{Unif}({\mathcal{H}^{k})}}\left[\sigma'( \mathbf{x}_{}^\top \mathbf{v})\mathbf{v} \right]$ should be smooth up to small discretization error, but I haven't been able to show this yet.

% \begin{enumerate}
%     \item $\| \mathbf{A}( [ a_t \w_{0,\parallel}; b_t \w_{0,\perp} ] + \mathbf{n}_t ) - \mathbf{A}( [ a_t \w_{0,\parallel}; b_t \w_{0,\perp} ] ) ||2 \leq c ||\mathbf{n}_t||_2$, where $\mathbf{A}(\w)$ is the full $\mathbf{A}$ matrix we've been discussing that results from the neuron weights $\w$ and $c$ is an absolute constant
%     \item $g(b) := \| \E_{\mathbf{v} \sim \text{Unif}(\mathcal{H})^{k-r} } [ \sigma'(  \w_{\perp}^T \mathbf{v} + s  ) \mathbf{v}] - \E_{\mathbf{z} \sim \mathcal{N}(\mathbf{0},\mathbf{I})} [ \sigma'(  \w_{\perp}^T \mathbf{z} + s  ) \mathbf{z}] ||_2 \leq c' g(0)$  for all scalars $s$, any $\w_{\perp} \in \mathbb{R}^{k-r}$, and an absolute constant $c'$
% \end{enumerate}


% These are smoothness conditions that I think are true but I don't know how to prove yet. The first condition is natural because we want to say the gradient we have at time t is approximately the gradient we would have if we had neuron weights that were aligned with $\w_{0,\parallel}$ and $\w_{0,\perp}$ (i.e. had an approximately** Gaussian selection of weights).

% **The second condition deals with the fact that $[ a_t \w_{0,\parallel}; b_t \w_{0,\perp} ]$  is not exactly Gaussian since $a_t$ and $b_t$ are coupled with $\w_0$. From the first step analysis we have that $\mathbf{A}(\w_0) \approx \mathbf{A}^\star(\w_0)$ where $\mathbf{A}^\star(\w_0)$ is some nice matrix. This is primarily due to the the approximation  $ \E_{\mathbf{v} \sim \text{Unif}(\mathcal{H})^{k-r} } [ \sigma'(  \w_{0,\perp}^T \mathbf{v} + \w_{0,\parallel}^T \mathbf{u}  ) \mathbf{v}] \approx \E_{\mathbf{z} \sim \mathcal{N}(\mathbf{0},\mathbf{I})} [ \sigma'(  \w_{0,\perp}^T \mathbf{z} + \w_{0,\parallel}^T \mathbf{u}  ) \mathbf{z}]$ . We used the Gaussianity of $\w_0$ to show this holds whp over $\w_0$.

% Now we want to say that
%  $$\E_{\mathbf{v} \sim \text{Unif}(\mathcal{H})^{k-r} }[ \sigma'(  \w_{0,\perp}^T \mathbf{v} + (a_t/b_t) \mathbf{w}_{0,\parallel}^T \mathbf{u}  ) \mathbf{v}] \approx \E_{\mathbf{z} \sim \mathcal{N}(\mathbf{0},\mathbf{I})} [ \sigma'(  \w_{\perp}^T \mathbf{z} + (a_t/b_t) \w_{0,\parallel}^T \mathbf{u}  ) \mathbf{z}].$$
% I don't think we can again argue using the randomness of $\w_0$ because $a_t/b_t$ is an unknown function of $\w_0$.  But for any fixed $\w_{0,\perp}$ (and thus $a_t/b_t$), I think it should be the case that condition 2 holds (intuitively, larger $a_t/b_t$ should only help the hypercube to Gaussian approximation, although empirically it does not monotonically help for all $\w_{0,\perp}$, so we allow for constant error $c'$). Once condition 2 holds, then we have $\E_{\mathbf{v} \sim \mathcal{H}^{k-r} } [ \sigma'(  \w_{0,\perp}^T \mathbf{v}  ) \mathbf{v}] \approx E_{\mathbf{z} \sim \mathcal{N}(\mathbf{0},\mathbf{I})} [ \sigma'(  \w_{0,\perp}^T \mathbf{z}) \mathbf{z}] $ from the first step analysis (as $\w_{0,\perp}$ is Gaussian and there are no other variables that depend on $\w_{0,\perp}$). This will allow us to bound the error $\| \mathbf{A}( [ a_t \w_{0,\parallel}; b_t \w_{0,\perp} ] )  - \mathbf{A}^\star ( [ a_t \w_{0,\parallel}; b_t \w_{0,\perp} ] ) ||_2 $. 

\vspace{6mm}

In the second phase of the induction, $\frac{a_t}{b_t}\approx \sqrt{k}$, so $\mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[  \exp\left(-\frac{a_t^2 (\mathbf{w}_{0,\parallel}^\top \mathbf{u})^2 }{ b_t^2 \|\mathbf{w}_{0,\perp}\|_2^2 } \right)   \right]$ is becoming very small. Thus $\|\mathbf{A}^\star([a_t\mathbf{w}_{0,\parallel},b_t\mathbf{w}_{0,\perp}] )\|_2$ is also becoming very small. This means that the contraction factor of $b_t$ is increasing (more extreme contraction) on every iteration. Eventually, there is an iteration $T$ at which $\mathbf{A}([a_T\mathbf{w}_{0,\parallel},b_T\mathbf{w}_{0,\perp}] ) = \mathbf{0}$ (note that it can be exactly zero since it is a discrete object). At this point, empirically we have 
 $a_{T}> \Omega(\sqrt{k})$, $b_t = O(\tfrac{\|\mathbf{w}_0\|_2}{\sqrt{k}})$ and $\|\mathbf{n}_{T}\|_2 =  O(\tfrac{\|\mathbf{w}_0\|_2}{\sqrt{k}})$, thus the signal $[a_{T} \mathbf{w}_{0,\parallel}; \mathbf{0}]$ has Euclidean norm a factor  of $\sqrt{k}$ larger than that of the noise $\mathbf{n}_T + [\mathbf{0}; b_{T} \mathbf{w}_{0,\perp}]$. I haven't thought through what the inductive hypotheses in this phase should be yet.
 % $b_T$ converges linearly fast until some time at which the convergence becomes superlinear. 
 % To account for this behavior we need to incorporate high order terms in the Taylor expansion of 



Gaussian case:

Assumption: For any two data points, probability of drawing task 

now it is easy. Just run for log k iterations, 
only complications: divide by norm of input to compute cosine similarity, maybe use arccos. the max/scaling of a.
lower bound no longer holds because task distribution does not satisfy assumption


ways to make it harder:

1. finite samples per task. not interesting?

2. weaker assumption on the task distribution. nah current one is fine

3. finite samples from the task distribution per round. maybe interesting but not very interesting

5. fedavg. or alternating muli


per-task case: you will learn whatever per-task important features subset

but averaging might cancel

A w1 + b w2 + c w3
a w1 + B w2 + c' w3

= yes this works

how does arbitrary dictionary affect it?

Need to estimate the matrix 

\begin{align}
    &\E_{\mathbf{z},\mathbf{z}'}\left[\left(\frac{1}{2} + \frac{1}{2}\Pr_{i}(f_i(\z) = f_i(\z')\right) \z' \z^\top \sigma'(\mathbf{W}\z) \sigma'(\mathbf{W}\z') \right]\nonumber \\
    &= \frac{1}{2}\E_{\mathbf{z},\mathbf{z}'}\left[\z' \z^\top \sigma'(\mathbf{W}\z) \sigma'(\mathbf{W}\z') \right]  + \frac{1}{2n}\sum_{i}\chi\{f_i(\z) = f_i(\z')\} \E_{\mathbf{z},\mathbf{z}'}\left[\z' \z^\top \sigma'(\mathbf{W}\z) \sigma'(\mathbf{W}\z') \right] \nonumber 
\end{align}
this is simply a $k$-dimensional covariance matrix

Finite samples:
\begin{align}
  % \frac{1}{|\mathcal{D}_{i,\text{rep}}||\mathcal{D}_{i,\text{head}|}}
 & \frac{1}{n_1 n_2}
  \sum_{j=1}^{n_1}\sum_{j'=1}^{n_2} \mathbf{z}_{i,j'}'\mathbf{z}_{i,j}^\top \sigma'(\mathbf{w}\z_{i,j}) \sigma'(\mathbf{w}\z'_{i,j'})\nonumber \\
  & \frac{1}{nn_1n_2} \sum_{i=1}^n \sum_{j=1}^{n_1}\sum_{j'=1}^{n_2} (\tfrac{1}{2} - \chi\{f_i(\z_{i,j}) = f_i(\z'_{i,j'})\} )\mathbf{z}_{i,j'}'\mathbf{z}_{i,j}^\top \sigma'(\mathbf{w}\z_{i,j}) \sigma'(\mathbf{w}\z'_{i,j'}) \nonumber 
\end{align}

\begin{align}
  & \frac{1}{nn_1n_2} \sum_{i=1}^n \sum_{j=1}^{n_1}\sum_{j'=1}^{n_2} (\tfrac{1}{2} - \chi\{f_i(\z_{i,j}) = f_i(\z'_{i,j'})\} )\mathbf{z}_{i,j'}'\mathbf{z}_{i,j}^\top \sigma'(\mathbf{w}^\top\z_{i,j}) \sigma'(\mathbf{w}^\top\z'_{i,j'}) \nonumber \\
  &\quad \quad -  \E_{\mathbf{z},\mathbf{z}'}\left[\left(\frac{1}{2} + \frac{1}{2}\Pr_{i}(f_i(\z) = f_i(\z')\right) \z' \z^\top \sigma'(\mathbf{w}^\top\z) \sigma'(\mathbf{w}^\top\z') \right] \nonumber \\
  &= \frac{1}{2}\left[\frac{1}{nn_1n_2} \sum_{i=1}^n \sum_{j=1}^{n_1}\sum_{j'=1}^{n_2} \mathbf{z}_{i,j'}'\mathbf{z}_{i,j}^\top \sigma'(\mathbf{w}^\top\z_{i,j}) \sigma'(\mathbf{w}^\top\z'_{i,j'}) - \E_{\mathbf{z},\mathbf{z}'}\left[\z' \z^\top \sigma'(\mathbf{w}^\top\z) \sigma'(\mathbf{w}^\top\z') \right] \right] \nonumber \\
  &\quad + \frac{1}{2}\Bigg[\frac{1}{nn_1n_2} \sum_{i=1}^n \sum_{j=1}^{n_1}\sum_{j'=1}^{n_2} \chi\{f_i(\z_{i,j}) = f_i(\z'_{i,j'}),\mathbf{w}^\top\z_{i,j}>0, \mathbf{w}^\top\z'_{i,j'}>0\} \mathbf{z}_{i,j'}'\mathbf{z}_{i,j}^\top\nonumber \\
  &\quad \quad - \E_{\mathbf{z},\mathbf{z}',i}\left[\chi\{f_i(\z) = f_i(\z'),\mathbf{w}^\top\z>0, \mathbf{w}^\top\z'>0\}\z' \z^\top \right] \Bigg]
\end{align}
the first difference is easy.  for the second:
\begin{align}
    &\frac{1}{2}\Bigg[\frac{1}{nn_1n_2} \sum_{i=1}^n \sum_{j=1}^{n_1}\sum_{j'=1}^{n_2} \chi\{f_i(\z_{i,j}) = f_i(\z'_{i,j'}),\mathbf{w}^\top\z_{i,j}>0, \mathbf{w}^\top\z'_{i,j'}>0\} \mathbf{z}_{i,j'}'\mathbf{z}_{i,j}^\top\nonumber \\
  &\quad \quad - \E_{\mathbf{z},\mathbf{z}',i}\left[\chi\{f_i(\z) = f_i(\z'),\mathbf{w}^\top\z>0, \mathbf{w}^\top\z'>0\}\z' \z^\top \right] \Bigg] \nonumber \\
  &= 
\end{align}





\newpage

==> Notes_sample_complexity.tex <==
\section{Finite samples}

Issues:

task complexity is effectively super-exponential in r

sample complexity per task is going to be $2^r$ poly$(d)/n$, n is number of tasks (gaussian helps, hypercube would be worse) (this is fine)

sample complexity of new task is O(r)? first need to answer which tasks can be implemented, and how

need to show that pre-training on one task cannot solve a new task without Omega(d) samples

consider a simple class of tasks: p-degree polynomials

training task distribution:

option 1: p-degree polynomials, there are many p-degree polynomials that do not generalize (e.g. those that do not satisfy hessian assumption), but training on many should generalize

option 2: functions of sum (including parities) - we know from shi paper that training on any single such task means the weights to go the average weight (when input data has structure), so they don't generalize to functions not of the sum

target task distribution:

plan: 

1. compute feature learning error induced by delta

2. come up with task distribution with quantifiable delta as a function of n. implies the larger n, the better feature learning

3. translate feature learning to downstream guarantees on this function class (what is sufficient for good transfer?)

4. show that whp, training on a single task from the distribution cannot transfer to a new task from this distribution (what is necessary for good transfer?)

3 and 4 are hard, replace with statement that we learn features such that there exists a good bias and head for each new task if necessary


----


each task corresponds to a vector on the 2**r-hypercube

each coord of matrix behaves like 1/rt(n)

then by gerschgorin, difference between this matrix and identity has norm at most 2**(3 r)/rt(n)  (3 because one to count all in row, theother to union bound over all 2**(2r) elmts

to make net error small enough: need rt(n) > 2**(3r) d**1.5 (with infinite samples per task)

for finite samples per task: much harder. need to show that distribution is basically uniform. i thin need 2**d samples

could consider other distributions of tasks (vectors on hypercube) e.g. clustered distribs. uniform is not capturing that differing points should have differing reps. also, a learning a single task sampled from uniofrm may generalize well

to capture this, need distrib induced by uniformly sampling halfspace. should be able to show this concentrates.
for sure, training on a single halfspace doesn't generalize

still need to figure out downstream. then do finite sample downstream

problem with saying ``there exists a good network'' is that there's no way to get negative result for one task?

negative result: if label only depends on sum of coordinates, then gd will learn average

tasks come from earlier relu networks.

right now, if new task comes from relu, what can we say?

if the new labels are generated by a relu 

if the new labels are clustered

there are a set of $c$ centroids on the hypersphere, if any 

input data is anything. function class is function determined by c centroids. label is label of closest centroid. still messy with border points.

for simplicity, new task data is normalized gaussian around one of c centroids on hypersphere 
centroids must be well-separated
 -  then we can learn this whp
 - and with O(r2r) samples (sparse regression)
  - how many centroids can we tolerate?
  - projection is gaussian with mean zero and variance r2
  - can normalize so it has var 1. 
  - so with constant neurons, will get one that is close to centroid whp
  
  - negative result: 
  1. random features would require Omega(d) samples... no random features could do it in c log(d) (but would require 2**d neurons?)
  2. single task pre-training would ...

two statements:

1. if new tasks are centroids, can solve
2. if hypercube, exists good netwokr

if pretrain data is hyperplanes

difficult to get finite-task guarantees

but suppose infinite tasks

data is gaussian, no sign. then with this data, can get very similar result as before

this means ... statements are same as above.

for a single task:

can be solved easily with lasso (r log (d))
but cannot generalize?

nonlinearity needed? no. would do better without it
even in our current case we don't need it....
need it for generalization but not feature learning

need linearity for parities. otherwise, loss would try to minimize similarity of opposite points, even though they have the same label

what is distrib on 2**r hypercube induced by this task distrib?

parity of subset of r points

2**r subsets

negative results would be (ideally):
can't learn single task efficiently (SQ bound, existing) including  random features and GD. but they don't include gaussian, so we can only make informal statement
another informal statement: previous work has shown that learning a parity task causes neurons to go to average, which prevents generalization to other tasks
linear thing is a remark (nte that in fact linear loss is zero)

positive result: 
distance 0 strings have the same label for 2**(r) tasks
distance 1 strings have the same label for 2**(r-1) tasks
distance 2 strings have the same label for 2**(r-2) x 2 tasks
distance 3 strings have the same label for 2**(r-3) (1 + (3 choose 2)) tasks
...
distance r-1 strings have same label for 2**(r-1) tasks
distance r strings have same label for for 2**(r) tasks

so it fits our model
so we learn the good features and can make the same generalization statements as above.
in-dist generalization: learning a single task generalizes well


things that are still missing: 
how many total samples for pretraining
fine-tuning provably solves any task
how many samples for fine-tuning
proof that you cannot learn single parity task efficiently with gaussian samples (SQ)
proof that single parity task cannot generalize to other tasks

problem... spare parities doesn't work


issues: 
1. need to show necessity of nonlinearity for training
2. necessity of multi-task
3. how to quanitfy success
4. necessity of head adaptation

need ot find setting where linear signal cancels but relu setting doesn't....


say that tasks generated by relus
single relu is just threshold. halfspace. same as hyperplanes
two relus is ....region cut out by two hyperplanes
need to quantize function.






\section{real finite samples}

note we ultimately want o average over tasks.

to get rid of max, condition on it being active/inactive for each task

active is zero.

for inactive, probability is the same for 

We have

\begin{align}
    &| \sum_i ( \E_{\mathbf{x}} \left[ \chi\{> 0\}  \left( 1- \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}'} [ f^*_{i}(\mathbf{x}') \sigma(\mathbf{W}^0 \mathbf{x}') ]^\top \sigma( \mathbf{W}^0\mathbf{x})  \right) )  \right]\nonumber \\
    &- \hat{\E}_{\mathbf{x}_j} \left[ \chi\{> 0\}  \left( 1- \eta f_{i}^*(\mathbf{x}_j) \hat{\mathbb{E}}_{\mathbf{x}_l'} [ f^*_{i}(\mathbf{x}_l') \sigma(\mathbf{W}^0 \mathbf{x}'_l) ]^\top \sigma( \mathbf{W}^0\mathbf{x}_j)  \right)  \right]|\nonumber \\
    &\leq \eta/T  |  \sum_i \E_{\mathbf{x}} \left[f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}'} [ f^*_{i}(\mathbf{x}') \sigma(\mathbf{W}^0 \mathbf{x}') ]^\top \sigma( \mathbf{W}^0\mathbf{x}) | >0  \right]\nonumber \\
    &- \sum_i \hat{\E}_{\mathbf{x}_{i,j}} \left[  f_{i}^*(\mathbf{x}_{i,j}) \hat{\mathbb{E}}_{\mathbf{x}_{i,l}'} [ f^*_{i}(\mathbf{x}_{i,l}') \sigma(\mathbf{W}^0 \mathbf{x}'_{i,l}) ]^\top \sigma( \mathbf{W}^0\mathbf{x}_{i,j}) |  |x|<.. \right]|
\end{align}

for max being active, worst case scenario is that $f_i^\ast(x) = sign(w^\top x)$

using this, we can upper bound inner prod as function of norm of x

we can condition on event that sampled x's are in ball at origin with sufficiently small radius

no this is not enough to get rid of the max

whatever ignore max for now...

show concen in each of $2^r$  quadrants...task have dif labels but labels for pop and finite are the same. easy. rademacher sum. use hoeffdings. gaussian in a quadrant is abs of gaussian multiplied with quadrant vect
abs of gaussian still subgaussian

hard part is getting rid of max


then


have something of the form
\begin{align}
    | E(f(x)) - \hat{E}(\hat{f}(x))| &\leq  | E(f(x)) - {E}(\hat{f}(x))| +  | \hat{E}(\hat{f}(x)) - {E}(\hat{f}(x))|\nonumber 
\end{align}

\begin{align}
    | E(f(x)) - {E}(\hat{f}(x))|  &= |E_v[  \chi(p^T v < 1)(1 - p^T v) -   \chi(e^T v < 1)(1 - e^T v)   ]|\nonumber \\
    &\leq 
\end{align}
note that by linearity of expectation sum over T of exps of dif gaussains is same as sum over T of the exp of the same gaussian

use dif gaussians. condition on each one separately

cross terms are uppper bounded by low probability that one of them is zero, and the boundedness of the other.

it remains to bound:
\begin{align}
    |\sum_i E_{v_i}[ (p_i - e_i)^T v_i | p_i^T v_i < 1, e_i^T v_i < 1]|
\end{align}

if tasks are drawn uniformly, we have sum of i.i.d. random variables (in i, ei), thus root T decay of variance so root T decay using chebyshev, now just need to bound variance 

\begin{align}
    E_{i,v_i}[ ((p_i - e_i)^T v_i)^2 | p_i^T v_i < 1, e_i^T v_i < 1]
\end{align}
[edit: this should be i, vi, vi'. but that is easier. also there is an expectation over ei on the outside]

now use cauchy-schwarz. but what is
\begin{align}
    E_{i,v_i}[ \|p_i - e_i\|_2^4 | p_i^T v_i < 1, e_i^T v_i < 1] &\leq E_i E_{v_i} [ \| p_i - e_i \|_2^4 \chi(p_i, e_i, v_i)  ] / P_{i,v_i}(p_i^T v_i < 1, e_i^T v_i < 1)\nonumber \\
    &\leq 2  E_i [ \| p_i - e_i \|_2^4 P_{v_i}(p_i, e_i, v_i < 1)  ]
\end{align} ?

need lower bound on  $P_{i,v_i}(p_i^T v_i < 1, e_i^T v_i < 1)$
 worst case $i$: all labels are positive
 even in this case, the event holds whp over x
 $p_i$ is deterministic. $e_i$ is random but independent of x
 can say that whp, $e_i$ is in a ball near origin
 so whp over $i,x_l'$, $ P_{i,v_i}(p_i^T v_i < 1, e_i^T v_i < 1) > 2$.

for every $i$, we know that $e_i - p_i$ is subgaussian

$  P_{v_i}(p_i, e_i, v_i < 1) $ is a random variable with randomness determined by task labels and ei

we can upper bound this in terms of worst case labelling
or we can simply upper bound by 1
everything is posistive
so now we have
\begin{align}
    E_{ei,i,v_i,vi'}[ \|p_i - e_i\|_2^4 | p_i^T v_i < 1, e_i^T v_i < 1]
    &\leq 2  E_{i,ei} [ \| p_i - e_i \|_2^4 ] \nonumber \\
\end{align} 

now, for any $i$, $ p_i - e_i$ is subgaussian with mean zero, so $\| p_i - e_i \|_2^4$ is proportional to subgaussian norm which decays with the number of inner samples. then union bound over all $2^r$ tasks, done. (bounding norm of  vi, vi' is easy)

for the other term:

\begin{align}
      | \hat{E}(\hat{f}(x)) - {E}(\hat{f}(x))|\nonumber 
\end{align}
for each $i$ seprately, condition expectation on x, xj being such that one max is active and the other is not (we know the probability of these events is small) and both max's being inactive

now we have
\begin{align}
    |\sum_i E_{v_i}[ e_i^T (v_i - ev_i|) | e_i^T v_i < 1, e_i^T v_i < 1]|
\end{align}

again sum of T iid mean zero r.v.s (in terms of (i, xij, xij'))

note ei is inner.

just need to bound variance. can do this using same approach as abve (cauchy schwarz)

bring Evi  inside... can't because conditioning

for bounding norm of ei it is easy.

fix fixed i:
\begin{align}
    &E_{evi, ei} [E_{v_i}[ e_i^T (v_i - ev_i|) | e_i^T v_i < 1, e_i^T v_i < 1]^2] \nonumber\\
    &=  E_{evi, ei} [E_{v_i,vi'}[ e_i^T (v_i - ev_i|)e_i^T (v_i' - ev_i|)  | e_i^T v_i < 1, e_i^T v_i < 1, ...]] \nonumber \\
    &= E_{evi, ei} [E_{v_i,vi'}[ e_i^T (v_i - ev_i|)e_i^T (v_i' - ev_i|) ] \nonumber \\
    & + [''] - [|] 
\end{align}
[ note: [''] = [|] P + c (1-P). just need to show P is close to 1. but this will not go to zero with more samples... but we don't need it to? the pop also has max error

so the proof should be like:

empirical with max converges to population without max plus some small perturbation.

this perturbation is equal to the current perturbation we have in going from population with max to population without max.

once we get rid of conditioning, it is easy. move exps inside, subgaussian.
]

before it was easier because we didnt need to cncentrate around Evi

note also there is implicit indicator on evi

naive cauchy-schwarz now : ei term would be easy

for the other term, add and subtract missing terms in evi, this is small, to remove indicator

% for other term, we have
\begin{align}
   E_{vi, vi', evi}[\|v_i - ev_i\|^2 \|vi' - evi\|^2]
\end{align}

x - avg(xi) where x, xi are iid subgaussian mean mu

\begin{align}
   E_{vi}[\|v_i - ev_i\|^2] - \|Ev_i - ev_i\|^2 = E ||vi||^2 - ||Evi||^2
\end{align}
is this small? no, it is a connstant. we used c-s too soon

but we need c-s to get rid of conditioning/indicator




\begin{lemma}
    \begin{align}
    &\Bigg| \frac{1}{T} \sum_i  \hat{\E}_{\mathbf{x}_j} \left[  \chi\{j > 0\} ( 1- \eta f_{i}^*(\mathbf{x}_j) \hat{\mathbb{E}}_{\mathbf{x}_j'} [ f^*_{i}(\mathbf{x}_l') \sigma(\mathbf{W}^0 \mathbf{x}_l') ]^\top \sigma( \mathbf{W}^0\mathbf{x}_j) ) \right]\nonumber \\
    &\quad \quad - \frac{1}{T} \sum_i {\E}_{\mathbf{x}} \left[ \chi{x >0} \left( 1- \eta f_{i}^*(\mathbf{x}) {\mathbb{E}}_{\mathbf{x}'} [ f^*_{i}(\mathbf{x}') \sigma(\mathbf{W}^0 \mathbf{x}') ]^\top \sigma( \mathbf{W}^0\mathbf{x})  \right)  \right]\bigg|\nonumber \\
    % &\frac{1}{nT}\left| \sum_{bad}\eta f_i^*(x) \right| 
    \end{align}
\end{lemma}

w.p. at least 

\begin{proof}
    \begin{align}
    &\Bigg| \frac{1}{T} \sum_i  \hat{\E}_{\mathbf{x}_j} \left[  \chi\{j > 0\} ( 1- \eta f_{i}^*(\mathbf{x}_j) \hat{\mathbb{E}}_{\mathbf{x}_j'} [ f^*_{i}(\mathbf{x}_l') \sigma(\mathbf{W}^0 \mathbf{x}_l') ]^\top \sigma( \mathbf{W}^0\mathbf{x}_j) ) \right]\nonumber \\
    &\quad \quad - \frac{1}{T} \sum_i {\E}_{\mathbf{x}} \left[ \chi\{x >0\} \left( 1- \eta f_{i}^*(\mathbf{x}) {\mathbb{E}}_{\mathbf{x}'} [ f^*_{i}(\mathbf{x}') \sigma(\mathbf{W}^0 \mathbf{x}') ]^\top \sigma( \mathbf{W}^0\mathbf{x})  \right)  \right]\bigg|\nonumber \\
    % &\frac{1}{nT}\left| \sum_{bad}\eta f_i^*(x) \right| 
    &\leq \eta  \Bigg| \frac{1}{T} \sum_i  \hat{\E}_{\mathbf{x}_j} \left[  \chi\{j > 0\} f_{i}^*(\mathbf{x}_j) \hat{\mathbb{E}}_{\mathbf{x}_j'} [ f^*_{i}(\mathbf{x}_l') \sigma(\mathbf{W}^0 \mathbf{x}_l') ]^\top \sigma( \mathbf{W}^0\mathbf{x}_j) ) \right]\nonumber \\
    &\quad \quad - {\E}_{\mathbf{x}} \left[ \chi\{x >0\} f^*(\mathbf{x}) {\mathbb{E}}_{\mathbf{x}'} [ f^*(\mathbf{x}') \sigma(\mathbf{W}^0 \mathbf{x}') ]^\top \sigma( \mathbf{W}^0\mathbf{x})  \right]\Bigg|\nonumber \\
    &\quad + \Bigg| \frac{1}{nT} \sum_i \sum_j \chi\{j > 0\} -  {\E}_{\mathbf{x}} \left[ \chi\{x >0\}  \right]\Bigg| \nonumber \\
    &= 
    \end{align}

Note each task is an iid random variable. By Hoeffding's,
\begin{align}
    \mathbb{P}_{f_1^\ast, \dots, f_T^\ast, x}\left(\Bigg| \frac{1}{nT} \sum_i \sum_j \chi\{j > 0\} -  {\E}_{\mathbf{x}} \left[ \chi\{x >0\}  \right]\Bigg| > \gamma \right) \leq 
\end{align}

with no truncation, and dif samples for head and rep, we can pull out inner exp and see that we have the sum of T iid subexp rvs with variance ... sum of n2 iid rvs? or n or 1?

intuitively, bound should be 1/T + 1/nx


could have realizable case, where dro is $2^r$, and then non-realizable case, where:
probability of same label, different clusters is epsilon
perp part is exactly the same
just need to characterize parallel assume it has lower-bounded minimum singular value

\end{proof}




\textbf{Comparison with bound on single task}


Steps:

Thorough lit review explaining single task results.

Positive results:

1. rep learning error for distribution of tasks satisfying assumption xx with sample complexity x. 

a. special case for training: tasks are parities. There are c 2r total tasks. May need to make c=2, consider flipped parities. yeah, it works.

1.1 downstream guarantee for all tasks with added layer

1.2 (maybe) downstream guarantee for ... polynomial tasks? with no added layer

a. reference comparison with single task, show simulations. 
- single parity task can generalize to parity and more generally sum tasks, but not other types of tasks.

cons with above: need 2r sample and neuron complexity

pros: better sample complexity than single task compared with shi et al. paper. more expressive rep compared to shi. (if polynomial) should not need extra layer for downstream. 







In the above, we have assumed that two points have the same label iff their gt reps have the same sign patterns, and otherwise they are equally likely to have the same label as not. This means that effectively only pairs of points with the same label carry signal, and the fraction of such pairs is 1/2r, so there is an inevitable req of 2r complexity. Next we consider another simple, natural setting that does not require such complexity, since the fraction of important pairs is 1/r. Moreover, this model has been used in prior work.



*******

or, start with this (yuanzhi without assump on z) model, then show: 1) we can learn rep with tasks satisfying sim. assump. special case 1: linear tasks with sparse codes (need noise to scale as 1/r). special case 2: linear tasks with dense codes (only point is to have case without 1/r noise dependence. maybe only this one though to avoid cut-and dry comp with yuanzhi). for both cases, clearly 1 task is insufficient. then: 2) with nonlinear tasks, we can still learn the rep (i.e. tasks satisfying diversity assump). special case 1: parities.
then generalization theorem(s) for both training data model cases. theorems should show gen with new layer to all tasks, and gen with no new layer to simple tasks. maybe use oco arg from shi/malach.
then comp with shi et al paper.

final:
story should probably be: first introduce data model (keep z as generic latent, eps with generic noise, generic task distrib), then loss, show it's like a CL. is that suff to get intuition? yes. generic tasks should label similar latents the same. then say we consider task distributions: 1) linear (with both sparse and dense), 2) parities, all (one theorem). 
generalization: 1 theorem for all cases, but two types of gen.
gains over single task:
1) linear -- get result (easy)
2) all -- comment that clearly one simple task is insufficient by same arg as linear. parities -- comp with shi and simulation
simulations:
1. one parity task goes to line, many feathers out
2. solving for optimal head is necessary

Either way, missing pieces are: 
1) parities satisfy assumpt (urgent) -- done
2) generalization to non-sum tasks without new layer
3) check that we can handle noise (yuanzhi) (urgent) -- done
4) check that we can make z on the hypercube (for analysis)
 - for non-linear tasks we can
 - for linear tasks we can


diffs from shi et al: 
we have noise in the data
we don't have activation noise (this makes their analysis easier)
we generalize to more things


*******


2. rep learning for second type of tasks (if time).

options:

% i. leaky relu. does it beat linear? flipping x para flips label, so we should be able to learn it with relu. but linear will also learn it. similarities do not change after leaky relu map.

ii. simple linear/yuanzhi model. 
pro: should no longer need 2r complexity. natural model. does not need weird task diversity assump (more natural one). studied by other relu paper. should not need extra layer for downstream. easy to show that one task is insufficient.
con: yuanzhi already showed CL can learn this with effectively one task (but requires d samples) -- this is fine.
     not clear yet if this works... 
     simple, kinda clear that linear can learn this too -- yuanzhi used it, so this is fine


todo:

1. check empirically that yuanzhi model works -- done

2. check empirically that parity works and the 1 task is insufficient -- done.

other possibilities considered:

1. using yuanzhi model for everything: didn't do because then we can't have parity tasks due to sparsity. we really can only have linear tasks.

2. for lower bound on single task:

a. stationary point of objective: hard because we need to account for max and regularization for fair comp with multi-task,
and in multi-task we don't characterize stationary points, we don't converge to one. Indeed, with max, one parity task may? be sufficient to learn all subspace directions.

b. global optimal is bad. again, hard to show, and we don't show the opposite of r multi

c. after one step, GD grows more in perp. This is most promising, but requires computing weird expectations (and probably considering types of ground-truth task functions one-by-one). Also, the goal theorem would be weird.





Data is generated as $\mathbf{x} = \mathbf{M}_{\parallel}\mathbf{z} + \mathbf{M}_{\perp}\mathbf{v} + \boldsymbol{\xi}$, where $\mathbf{z}\sim \mathcal{H}^r, \mathbf{v}\sim \mathcal{H}^{k-r}$, $\boldsymbol{\xi}\sim \mathcal{N}(\mathbf{0}_d, \sigma_{\chi}^2\mathbf{I}_d)$.


We need to control
\begin{align}
   & \mathbf{M}_{\perp}^\top \mathbb{E}_{\mathbf{z},z',\mathbf{{v}}, v', \boldsymbol{\xi}, \xi'}[ \chi\{ \mathbf{z} = z' \} (\mathbf{M}_{\parallel}\mathbf{z} + \mathbf{M}_{\perp}\mathbf{v} +  \boldsymbol{\xi})(\mathbf{M}_{\parallel}\mathbf{z}' + \mathbf{M}_{\perp}\mathbf{v}' +  \boldsymbol{\xi}')^\top \nonumber \\
   &\quad \quad\quad \quad\quad \quad \quad \sigma'(\mathbf{w}^\top (\mathbf{M}_{\parallel}\mathbf{z} + \mathbf{M}_{\perp}\mathbf{v} + \boldsymbol{\xi}))\sigma'(\mathbf{w}^\top (\mathbf{M}_{\parallel}\mathbf{z}' + \mathbf{M}_{\perp}\mathbf{v}' +  \boldsymbol{\xi}')) ]\mathbf{M}_{\perp} \nonumber \\
   &= \mathbb{E}_{\mathbf{z},z',\mathbf{{v}}, v', \boldsymbol{\xi}, \xi'}[ \chi\{ \mathbf{z} = z' \} (\mathbf{v} + \mathbf{M}_{\perp}^\top \boldsymbol{\xi})( \mathbf{v}' + \mathbf{M}_{\perp}^\top \boldsymbol{\xi}')^\top  \sigma'(\mathbf{w}^\top (\mathbf{M}_{\parallel}\mathbf{z} + \mathbf{M}_{\perp}\mathbf{v} + \boldsymbol{\xi}))\sigma'(\mathbf{w}^\top (\mathbf{M}_{\parallel}\mathbf{z}' + \mathbf{M}_{\perp}\mathbf{v}' + \boldsymbol{\xi}')) ] \nonumber \\
   &= \mathbb{E}_{\mathbf{z},z',\mathbf{{v}}, v', \boldsymbol{\xi}, \xi'}[ \chi\{ \mathbf{z} = z' \} \mathbf{v} (\mathbf{v}')^\top   \sigma'(\mathbf{w}^\top (\mathbf{M}_{\parallel}\mathbf{z} + \mathbf{M}_{\perp}\mathbf{v} + \boldsymbol{\xi}))\sigma'(\mathbf{w}^\top (\mathbf{M}_{\parallel}\mathbf{z}' + \mathbf{M}_{\perp}\mathbf{v}' +  \boldsymbol{\xi}')) ] \nonumber \\
   &\quad + \dots +\dots +\dots 
\end{align}
Note that in the first term, we can pull the expectations over $\xi,\xi'$ inside the expression to obtain
\begin{align}
   T_1 &= \mathbb{E}_{\mathbf{z},z',\mathbf{{v}}, v', \boldsymbol{\xi}, \xi'}[ \chi\{ \mathbf{z} = z' \} \mathbf{v} (\mathbf{v}')^\top   \sigma'(\mathbf{w}^\top (\mathbf{M}_{\parallel}\mathbf{z} + \mathbf{M}_{\perp}\mathbf{v} + \boldsymbol{\xi}))\sigma'(\mathbf{w}^\top (\mathbf{M}_{\parallel}\mathbf{z}' + \mathbf{M}_{\perp}\mathbf{v}' +  \boldsymbol{\xi}')) ] \nonumber \\
   &= \mathbb{E}_{\mathbf{z},z',\mathbf{{v}}, v'}[ \chi\{ \mathbf{z} = z' \} \mathbf{v} (\mathbf{v}')^\top   \mathbb{P}_{\xi}[\mathbf{w}^\top \boldsymbol{\xi} > - \mathbf{w}^\top (\mathbf{M}_{\parallel}\mathbf{z} + \mathbf{M}_{\perp}\mathbf{v} ) ]\mathbb{P
   }_{\xi'}[ \mathbf{w}^\top \boldsymbol{\xi}' > - \mathbf{w}^\top (\mathbf{M}_{\parallel}\mathbf{z}' + \mathbf{M}_{\perp}\mathbf{v}' ) ]]  \nonumber \\
   &=\mathbb{E}_{\mathbf{z},z',\mathbf{{v}}, v'}[ \chi\{ \mathbf{z} = z' \} \mathbf{v} (\mathbf{v}')^\top   \mathbb{P}_{\xi}[\mathbf{w}^\top \boldsymbol{\xi} <  \mathbf{w}^\top (\mathbf{M}_{\parallel}\mathbf{z} + \mathbf{M}_{\perp}\mathbf{v} ) ]\mathbb{P
   }_{\xi'}[ \mathbf{w}^\top \boldsymbol{\xi}' <  \mathbf{w}^\top (\mathbf{M}_{\parallel}\mathbf{z}' + \mathbf{M}_{\perp}\mathbf{v}' ) ]]  \nonumber \\
   &= \frac{1}{4}\mathbb{E}_{\mathbf{z},z',\mathbf{{v}}, v'}\left[ \chi\{ \mathbf{z} = z' \} \mathbf{v} (\mathbf{v}')^\top  \left(1 + \erf\left( \frac{\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z} + \mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v} }{\sqrt{2}\sigma_\xi \|\mathbf{w}\|_2}\right)\right) \left(1 + \erf\left( \frac{\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z}' + \mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v}' }{\sqrt{2}\sigma_\xi \|\mathbf{w}\|_2}\right) \right)\right] \nonumber \\
   &=  \frac{1}{4}\mathbb{E}_{\mathbf{z},z',\mathbf{{v}}, v'}\left[ \chi\{ \mathbf{z} = z' \} \mathbf{v} (\mathbf{v}')^\top \erf\left( \frac{\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z} + \mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v} }{\sqrt{2}\sigma_\xi \|\mathbf{w}\|_2}\right)\erf\left( \frac{\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z}' + \mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v}' }{\sqrt{2}\sigma_\xi \|\mathbf{w}\|_2}\right) \right] \nonumber \\
   &= \frac{1}{4}\mathbb{E}_{\mathbf{z},z',\mathbf{{v}}, v'}\left[ \chi\{ \mathbf{z} = z' \} \mathbb{E}_{\mathbf{{v}}}\left[ \mathbf{v} \erf\left( \frac{\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z} + \mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v} }{\sqrt{2}\sigma_\xi \|\mathbf{w}\|_2}\right)\right] \mathbb{E}_{\mathbf{{v}}'}\left[ (\mathbf{v}')^\top \erf\left( \frac{\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z}' + \mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v}' }{\sqrt{2}\sigma_\xi \|\mathbf{w}\|_2}\right) \right]\right] \nonumber \\
\end{align}
Note that the inner expectations over $v$, $v'$ are identical; we only need to compute one of them. 
Using the Taylor expansion of the error function, we obtain
\begin{align}
  &  \mathbb{E}_{\mathbf{{v}}}\left[ \mathbf{v} \erf\left( \frac{\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z} + \mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v} }{\sqrt{2}\sigma_\xi \|\mathbf{w}\|_2}\right)\right]  \nonumber \\
  &= \frac{2}{\sqrt{\pi}} \mathbb{E}_{\mathbf{{v}}}\left[ \mathbf{v} \left( \frac{\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z} + \mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v} }{\sqrt{2}\sigma_\xi \|\mathbf{w}\|_2}  - \frac{(\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z} + \mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v})^3 }{6\sqrt{2}\sigma_\xi^3 \|\mathbf{w}\|_2^3} +  \frac{(\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z} + \mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v})^5 }{40\sqrt{2}\sigma_\xi^5 \|\mathbf{w}\|_2^5} + \dots \right)\right]  \nonumber \\
  &= \sqrt{\frac{2}{\pi}} \Bigg(\frac{\mathbf{M}_{\perp}^\top\mathbf{w} }{\sigma_\xi \|\mathbf{w}\|_2}  - \frac{3(\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z})^2\mathbf{M}_{\perp}^\top\mathbf{w} + \mathbb{E}_{\mathbf{{v}}}\left[\mathbf{v}(\mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v})^3 \right]}{6\sigma_\xi^3 \|\mathbf{w}\|_2^3} \nonumber \\
  &\quad \quad +  \frac{ 5 (\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z})^4 \mathbf{M}_{\perp}^\top \mathbf{w} + 10(\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z} )^2 \mathbb{E}_{\mathbf{{v}}}\left[ \mathbf{v}(\mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v})^3 \right] + \mathbb{E}_{\mathbf{{v}}}\left[ \mathbf{v}(\mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v})^5 \right] }{40\sigma_\xi^5 \|\mathbf{w}\|_2^5} + \dots \Bigg)  \label{linn} \\
  &=  \sqrt{\frac{2}{\pi}} \Bigg(\frac{\mathbf{M}_{\perp}^\top\mathbf{w} }{\sigma_\xi \|\mathbf{w}\|_2}  - \frac{3(\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z})^2\mathbf{M}_{\perp}^\top\mathbf{w} +  3 \|\mathbf{M}_{\perp}^\top \mathbf{w}\|_2^2 \mathbf{M}_{\perp}^\top \mathbf{w} - 2 (\mathbf{W}_\perp \mathbf{w})^3 }{6\sigma_\xi^3 \|\mathbf{w}\|_2^3} \nonumber \\
  &\quad \quad +  \frac{ 5 (\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z})^4 \mathbf{M}_{\perp}^\top \mathbf{w} + 30(\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z} )^2  \|\mathbf{M}_{\perp}^\top \mathbf{w}\|_2^2 \mathbf{M}_{\perp}^\top \mathbf{w} - 20(\mathbf{w}^\top \mathbf{M}_{\parallel}\mathbf{z} )^2 (\mathbf{W}_\perp \mathbf{w})^3  + \mathbb{E}_{\mathbf{{v}}}\left[ \mathbf{v}(\mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v})^5 \right] }{40\sigma_\xi^5 \|\mathbf{w}\|_2^5} + \dots \Bigg)  \label{3rd} \\
  &=  \sqrt{\frac{2}{\pi}} \Bigg(\frac{\mathbf{M}_{\perp}^\top\mathbf{w} }{\sigma_\xi \|\mathbf{w}\|_2}  - \frac{O(\sigma_w^{3} rk^{0.5}) +  3 \|\mathbf{M}_{\perp}^\top \mathbf{w}\|_2^2 \mathbf{M}_{\perp}^\top \mathbf{w} - 2 (\mathbf{W}_\perp \mathbf{w})^3 }{6\sigma_\xi^3 \|\mathbf{w}\|_2^3} 
  \nonumber \\
  &\quad \quad 
  +  \frac{ O(\sigma_w^{5} rk^{1.5})+ \mathbb{E}_{\mathbf{{v}}}\left[ \mathbf{v}(\mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v})^5 \right] }{40\sigma_\xi^5 \|\mathbf{w}\|_2^5} + \dots \Bigg)  \nonumber \\
  &=  \sqrt{\frac{2}{\pi}} \Bigg(\frac{\mathbf{M}_{\perp}^\top\mathbf{w} }{\sigma_\xi \|\mathbf{w}\|_2}  - \frac{O(\sigma_w^{3} rk^{0.5}) +  3 \|\mathbf{M}_{\perp}^\top \mathbf{w}\|_2^2 \mathbf{M}_{\perp}^\top \mathbf{w} - 2 (\mathbf{W}_\perp \mathbf{w})^3 }{6\sigma_\xi^3 \|\mathbf{w}\|_2^3} \nonumber \\
  &\quad \quad +  \frac{ O(\sigma_w^{5} rk^{1.5}) + 6 \|\mathbf{M}_{\perp}^\top\mathbf{w}\|_2^4 \mathbf{M}_{\perp}^\top\mathbf{w}  - 4 \|\mathbf{M}_{\perp}^\top\mathbf{w}\|_4^4 \mathbf{M}_{\perp}^\top\mathbf{w}  + \|\mathbf{M}_{\perp}^\top\mathbf{w}\|_2^2 (\mathbf{M}_{\perp}^\top\mathbf{w})^3 - 2(\mathbf{M}_{\perp}^\top\mathbf{w})^5 }{40\sigma_\xi^5 \|\mathbf{w}\|_2^5} + \dots \Bigg)  \label{5th} \\
  &=  \sqrt{\frac{2}{\pi}} \Bigg(\frac{\mathbf{M}_{\perp}^\top\mathbf{w} }{\sigma_\xi \|\mathbf{w}\|_2}  - \frac{O(\sigma_w^{3} rk^{0.5}) +  3 \|\mathbf{M}_{\perp}^\top \mathbf{w}\|_2^2 \mathbf{M}_{\perp}^\top \mathbf{w} + O(\sigma_w^3 k^{0.5}) }{6\sigma_\xi^3 \|\mathbf{w}\|_2^3} \nonumber \\
  &\quad \quad +  \frac{ O(\sigma_w^{5} r k^{1.5}) + 6 \|\mathbf{M}_{\perp}^\top\mathbf{w}\|_2^4 \mathbf{M}_{\perp}^\top\mathbf{w}  + O(\sigma_w^5 k^{1.5})}{40\sigma_\xi^5 \|\mathbf{w}\|_2^5} + \dots \Bigg)  \label{o} \\
    &=  \frac{\sqrt{2}}{\sqrt{\pi} \|\mathbf{w}\|_2} {\mathbf{M}_{\perp}^\top\mathbf{w} } \Bigg(\frac{1}{\sigma_\xi}  - \frac{ \|\mathbf{M}_{\perp}^\top \mathbf{w}\|_2^2  }{2\sigma_\xi^3 \|\mathbf{w}\|_2^2} + \frac{3  \|\mathbf{M}_{\perp}^\top\mathbf{w}\|_2^4}{20 \sigma_\xi^5 \|\mathbf{w}\|_2^4 } \Bigg) \nonumber \\
   & \quad +  \sqrt{\frac{2}{\pi}}  \Bigg( \frac{O(\sigma_w^{3} rk^{0.5}) }{6\sigma_\xi^3 \|\mathbf{w}\|_2^3} + \frac{ O(\sigma_w^{5} r k^{1.5}) }{40\sigma_\xi^5 \|\mathbf{w}\|_2^5} + \dots \Bigg)  \label{oo} \\
   &=  \frac{\sqrt{2}}{\sqrt{\pi} \|\mathbf{w}\|_2} {\mathbf{M}_{\perp}^\top\mathbf{w} } \Bigg(\frac{1}{\sigma_\xi}  - \frac{ \|\mathbf{M}_{\perp}^\top \mathbf{w}\|_2^2  }{2\sigma_\xi^3 \|\mathbf{w}\|_2^2} + \frac{3  \|\mathbf{M}_{\perp}^\top\mathbf{w}\|_2^4}{20 \sigma_\xi^5 \|\mathbf{w}\|_2^4 } \Bigg) \nonumber \\
   & \quad + O\left( \frac{ rk^{0.5}}{\sigma_\xi^3 d^{1.5}} \right) + O\left( \frac{ r k^{1.5} }{\sigma_\xi^5 d^{2.5}}\right) + \dots   \label{oo} \\
  % &=  \frac{\sqrt{2}}{\sqrt{\pi} \|\mathbf{w}\|_2}  \mathbf{M}_{\perp}^\top\mathbf{w} \Bigg(\frac{1 }{\sigma_{\xi}}  - \frac{   \|\mathbf{M}_{\perp}^\top \mathbf{w}\|_2^2  }{2 \sigma_\xi^3 \|\mathbf{w}\|_2^2} + \Bigg) \nonumber \\
  % &\quad \quad +  \frac{ O(\sigma_w^{5} rk^{1.5})+ \mathbb{E}_{\mathbf{{v}}}\left[ \mathbf{v}(\mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v})^5 \right] }{40\sigma_\xi^5 \|\mathbf{w}\|_2^5} + \dots \Bigg)  \nonumber \\
\end{align}
where in \eqref{linn} we have used the linearity of the expectation and the fact that $\mathbb{E}_{\mathbf{v}}[\mathbf{vv}^\top] = \mathbf{I}_{k-r}$, in \eqref{3rd} we have used that $\mathbb{E}_{\mathbf{{v}}}\left[\mathbf{v}(\mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v})^3 \right] = 3 \|\mathbf{M}_{\perp}^\top \mathbf{w}\|_2^2 \mathbf{M}_{\perp}^\top \mathbf{w} - 2 (\mathbf{W}_\perp \mathbf{w})^3$, 
in \eqref{5th} we have used that 
$\mathbb{E}_{\mathbf{{v}}}\left[ \mathbf{v}(\mathbf{w}^\top \mathbf{M}_{\perp}\mathbf{v})^5 \right] = 6 \|\mathbf{M}_{\perp}^\top\mathbf{w}\|_2^4 \mathbf{M}_{\perp}^\top\mathbf{w}  - 4 \|\mathbf{M}_{\perp}^\top\mathbf{w}\|_4^4 \mathbf{M}_{\perp}^\top\mathbf{w}  + \|\mathbf{M}_{\perp}^\top\mathbf{w}\|_2^2 (\mathbf{M}_{\perp}^\top\mathbf{w})^3 - 2(\mathbf{M}_{\perp}^\top\mathbf{w})^5 $, and in \eqref{o} we have used that .


Next, 


note that scaling of sigma-eps matters relative to scaling of z, v. right now these are O(1), so sgima-eps should also be. can scale them down together.

use hermit epoly's? but again will have issue that higher order terms matter.

should that for every  hermite poly, the domininant term is the term we want... but need to show that the coefficients converge... 

larger noise will hurt you later (eps-eps term)

also current have issue that we need k approx d...

assume noise is large for now. come back to noiseless case later

bound it via bound on variance of norm




% generalization result:

% consider tasks of the form sign(polynomial)

% 1. show existence of good network 



what can we do:

any task with second relu layer.

sign of polynomial on binary inputs with  coeffs 1 and either an odd number of monomials or add 1/2 scalar
- step 1: by same argument as damian step 1, for each function in this class there exists a one-hidden-layer relu network including the learned features that can approximate this polynomial. might have mean squared error epsilon. This means we could have 2r*epsilon error on any one point. So we need epsilon < 2**(r+1)
- step 2: 

yuanzhi noise model doesn't work because we rely on constants. also we would need to add the second binary noise term anyway, otherwise we could learn rep with pca.

why we can't use mahdi paper: error bound isn't strong enough... but it might work

we can't use new undergrad paper because the margin is $1/r^{2^r}$ --> would require this many samples

the other papers either have too many/weird assumptions on initialization (hsu), not clear what the error is (bach), only apply to strange activations (yehudai and shamir), are only asymptotic (ghorbani)

stop just write........


we have 3 special cases of task distributions: 1) linear, 2) parities, 3) all binary, all on gaussian / sign of gaussian data

move downstream network construction to  appendix. focus instead on explaining the three special cases

formal negative results for 1 task: there exist global optima that cannot generalize to other parity tasks? true. include this (PROVE) but data must be on hypercube, which is weird...
- can you solve it with gaussian? or spherical? no, I think you need multiple layers, and need to learn all r feats.

whereas in our case, for linear loss all global optima... no can't say anything about global opt because tasks are not implementable.

missing: why optimizing heads locally is important. show that for the case of parities/all tasks/linear, the gradient become zero with a single head (PROVE)
- in practice, could be mitigated by multiple local steps


It is clear that learning a single linear task or, more generally,  a task that is a function a strict subset of the the 
\begin{theorem}
    
\end{theorem}

\begin{proof}
    
\end{proof}


\begin{theorem}
    consider any task which is a function of < r orthogonal directions within the subspace

    train with hypercube data
\end{theorem}


\begin{proof}
    Pick two points such that the sum of their first r coordinates is the same, so they have the same representation under the training task, but they have different sum of subset of coordinates. 
    
    obvious statement, just focus on parities. what does it mean to generalize? oven if task requires learning all r directions within subspace, does that get you generalization? depends on which task, maybe not

fails to generalize in the sense that there is no function that can map learned representation to new labels.

need to get hypercube to work in pos reults......
    
\end{proof}





Latest plan:

- change x to Mx

- sample complexity

- use this and empirics to show improvement over single task

- think more about generalization to smaller set of tasks 
-- maybe be able to make a corollary from current result, just change the set of tasks we care about generalization to

- move second layer construction to appendix

- maybe linear (angle) tasks
-- need concentration

- maybe lower bound on single head learning



ideas: 
look at mgf
approximate rademacher interval prob with sum of central binomial coeffs
 -- need to connet rademacher with binomial

 




==> Post-Neurips-notes.tex <==
How to improve the paper?

Issue 1: Assumption is not interpretable/too strong.

Issue 2: Non-linearity is not needed.

If we go with inner product/angle, then still non-linearity is not essential. But we can implement downstream tasks.  Issue is that we need infinite tasks? With finite tasks, 
for all u,v, need to show that empirical probability of same label is close to angle, can be done if we only need to consider u,v on hypercube, otherwise construct epsilon-net, again have exponentially-many in r points to consider, can union bound.
So what was the problem with this?
Issue: all tasks are linear. Can solve them without nonlinearity.
But, it is cool that by solving many easy tasks, you can generalize to hard tasks
But you don't need nonlinearity for training
Also, does it even work with arccos: yes. again use taylor expansion. tricky when u,v are close (inner prod not near zero) but it should work
Benefit: one task is not sufficient
Ah problem was that negative result for GD didn't work because 2-task distrib doesn't satisfy assumption
but the negative result should still hold with infinite tasks.
anyway it's not necessary
How can we make non-linearity essential?
xor of two halfspaces
$ P( ( (w^T u > 0 \cap z^T u < 0) \cup (w^T u < 0 \cap z^T u > 0) ) \cap ( (w^T v > 0 \cap z^T v < 0) \cup (w^T v < 0 \cap z^T v > 0) ) ) $ \\

4 disjoint events 
$(w^T u > 0 \cap z^T u < 0) \cap (w^T v > 0 \cap z^T v < 0)$ etc

$P( (w^T u > 0 \cap z^T u < 0) \cap (w^T v > 0 \cap z^T v < 0) ) = P( w^T u > 0 \cap w^T v > 0 ) P( z^T u < 0 \cap z^T v < 0) = (1 - angle)^2 \approx (inner prod)^2$

$ P( (w^T u > 0 \cap z^T u < 0) \cap (w^T v < 0 \cap z^T v > 0) )  = P( w^T u > 0 \cap w^T v < 0)^2$ something like angle $\approx (1 - inner prod)^2$ thus sum = $1 - 2 ip + ip^2$

So gradient is:
$- (1 - 2p(diff)) uv = - (2p(same) - 1) uv = - (2(1 - 2 ip + ip^2) - 1) uv ==  ip uv - ip^2 uv $ so update is $ w + (-ip uv + ip^2 uv) $. this is the opposite of what we want. in good case it is $ w +  ip uv $. so it doesn't work. unless you do a convoluted thing and make the step size really large so the sign flips.

how else can we make non-linearity essential while having a reasonable assumption on the probability of two points sharing a label?

Parities:
non-linearity needed to solve each one
but in population case you can't learn the rep.
maybe you can with noisy sgd

also, need setting where tasks are hard such that nonlinearity is required, but single task is insufficient. 

according to shi paper, parities are too easy because you can learn them by having all neurons go to sum of imp features

need setting where you learn full rank features via multitask parities and nonlinearity is necessary


-----

Need to learn nonlinear features

What info is multitasks giving?
Must be more than simply identifying important features because this can be done with multitask linear
And single task 


Intuitively multitasking should give you more diverse features
Which we are showing compared to shi paper
We need nonlinear features
We need a setting where
1. Nonlinearity allows contrastive loss to be meaningful

Tasks must be hard enough such that nonlinearity is required, but not too hard such that the features can be learned with one task
… but really, tasks being hard shouldn’t mean that a single task is sufficient…

Our grad is almost a kernel
In lee paper, note that sigma2 can be identity (linear)

Left off:
Parities are promising because single parity task does not entail learning all the features, and each task is nonlinear/requires nonlinearity
However learning the features does not require a nonlinear model
And if the set of tasks is all parities on subsets of the important features, our current algorithm can’t learn this.


-----



todo OCT 2023:

Finish sample complexity

-- need to lower bound single-task sample complexity/ learnability
-- for rep learning, we definitely need $2^r$ tasks, or do we?

get result that doesn't consider solving all downstream tasks -- only which tasks?

get regression result? no, that is new paper -- linear model can solve nonlinear tasks with multitask and optimized head

multiclass with jason








==> ProofSketch-ICML.tex <==
\vspace{-1mm}
\section{Proof Sketch} \label{sec:sketch}



In this section, we sketch the proof of Proposition \ref{prop:1}, which is the key feature learning result that enables downstream guarantees.
% We focus on the infinite sample case for ease of exposition.
% He we focus on AltMinGD since it is easier to analyze than FO-ANIL yet the analysis conveys all of the main ideas for the FO-ANIL analysis. 
The proof heavily leverages the fact that multi-task pretraining entails updating the first-layer weights {\em after} fitting a unique head to each task.
{{Surprisingly, we show that making one gradient-based update of the head for each task induces a pseudo-contrastive loss that encourages representations of two points to be similar if and only if they are likely to share a label on a randomly drawn task.}} Since two points are likely to share a label on a drawn task if and only if they share the same sign pattern on their $r$ ground-truth features (by Assumption \ref{assump:diversity}), the pseudo-contrastive loss inclines the representation to extract these $r$ latent features\footnote{We also show in Appendix \ref{app:regression} that these intuitions can be extended to the regression setting.}. For ease of exposition, in this setting we focus on the population setting with infinite tasks and samples per task, and defer the finite-task and samples proof to Appendix \ref{app:thrm1}.

\textbf{Step 1: Derive pseudo-contrastive loss after head updates.} We first update the task-specific head with one gradient step for each task $i$ given the initial parameters $(\mathbf{W}^0,\mathbf{b}^0,\mathbf{a}_{i}^0)$. 
% \textcolor{blue}{"optimal" head or one-step-gradient head?}
Due to the symmetric initialization, $f(\mathbf{x};\mathbf{W}^0,\mathbf{b}^0,\mathbf{a}^0_i)=0$ for all $\mathbf{x}\in \mathbb{R}^d$, so the hinge loss is affine in $\mathbf{a}_i^0$ for all tasks (the $\max(\cdot,0)$ threshold is inactive). Therefore, using the choice of $\lambda_{\mathbf{a}} = 1/\eta $ and $\mathbf{b}^0=\mathbf{0}_m$,
% we can set $ \nabla_{\mathbf{a}} \mathcal{L}_i(\mathbf{W}_0,\mathbf{b}_0,\mathbf{a}) = \mathbf{0}_m $ to find
% satisfying $ \|\mathbf{W}\|_2 \leq $ and $\|\mathbf{b}\|_2 \leq $.
% with dataset $\mathcal{D}_i$ given a representation $\mathbf{W}$ satisfying $\|\mathbf{W}\|_2 = O(k^{-1})$. 
\begin{align}
\vspace{-1mm}
   \mathbf{a}_{i}^1 &= (1 - \eta \lambda_{\mathbf{a}})\mathbf{a}_{i}^0 - \eta\nabla \mathcal{L}_i(\mathbf{W}^0,\mathbf{b}^0,\mathbf{a}_i^0) \nonumber \\
   &= \eta \mathbb{E}_{\mathbf{x}} [ f_{i}(\mathbf{x}) \sigma(\bar{\mathbf{W}}^0\mathbf{x}) ]  \label{head1}
   % \in \arg\min_{\mathbf{a}\in \mathbb{R}^m}\mathcal{L}_i(\mathbf{W}_0,\mathbf{b}_0,\mathbf{a}) %; \mathcal{D}_i)
   % \coloneqq \frac{1}{|\mathcal{D}_i|}\sum_{(y_{i,j},\mathbf{x}_{i,j})\in \mathcal{D}_i} \max\left( 1 - y_{i,j} \mathbf{a}^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}) , 0 \right) + \frac{\lambda_\mathbf{W}}{2} \|\mathbf{W}\|_F^2 + \frac{\lambda_\mathbf{a}}{2} \|\mathbf{a}\|_2^2 \nonumber \\
    % &\iff  \nabla_{\mathbf{a}} \mathcal{L}_i(\mathbf{W},\mathbf{b},\mathbf{a}_i) = \mathbf{0}_m  \nonumber \\ 
    %  \partial_{\mathbf{a}} 
    % \frac{1}{|\mathcal{D}_i|}\sum_{(y_{i,j},\mathbf{x}_{i,j})\in \mathcal{D}_i}y_{i,j} \sigma(\mathbf{W}\mathbf{x}_{i,j}) \chi\{\mathbf{a}^\top \sigma(\mathbf{W}\mathbf{x}_{i,j} )<1 \} \nonumber \\
    % \implies
    % \mathbf{a}_i = \frac{1}{\lambda_{1}|\mathcal{D}_i|}\sum_{(y_{i,j},\mathbf{x}_{i,j})\in \mathcal{D}_i}y_{i,j} \sigma(\mathbf{W}\mathbf{x}_{i,j}) 
    % &\iff \mathbf{a}_{0.i} = \frac{1}{\lambda_{1}}\mathbb{E}_{\mathbf{z}} [ f_{i}(\mathbf{M}\mathbf{z}) \sigma(\mathbf{W}_0\mathbf{Mz} + \mathbf{b}_0) ] 
\end{align} %\chi \{ f_{i}(\mathbf{Mz}) \sigma(\mathbf{W}\mathbf{Mz} + \mathbf{b}) < 1 \} 
% since $\mathcal{L}_i(\mathbf{W},\mathbf{a}; \mathcal{D}_{i,1})$ is a strongly convex function of $\mathbf{a}$, and the subgradient of $\mathcal{L}_i(\mathbf{W},\mathbf{a}; \mathcal{D}_i)$ with respect to $\mathbf{a}$ at $\mathbf{a}_i$ contains zero if each $\|\mathbf{x}_{i,j}\|_2 = \tilde{O}(\sqrt{k\log(k)})$\footnote{This ensures that the $\max()$ is inactive for all data points.}, which occurs with high probability. 
% \textcolor{blue}{the last equality feels like you've set ${a}_0$ to $0$ and hence might be confusing to the reader. Why don't you include ${a}_0$?}
where we use $\bar{\mathbf{W}}^0$ to denote a stop-gradient on ${\mathbf{W}}^0$.
As a result, the updated head for task $i$, $\mathbf{a}_{i}^1$, is proportional to the average label-weighted neuron output over the dataset for task $i$. Now we can insert this value of $\mathbf{a}_{i}^1$ back into the loss, to obtain $\mathcal{L}_i(\mathbf{W}^0, \mathbf{b}^0,\mathbf{a}_{i}^1)$. For ease of notation we define 
% $g(\mathbf{z};\mathbf{W},\mathbf{b})\coloneqq \sigma(\mathbf{W}\mathbf{Mz}+\mathbf{b})$ and 
$\beta({\mathbf{x},\mathbf{x}'})\coloneqq \mathbb{E}_{i}[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')]$ for all pairs of inputs $\mathbf{x},\mathbf{x}'$, and replace $\max(\cdot,0)$ with $\sigma(\cdot)$ in the hinge loss (recall $\sigma(\cdot)$ is the ReLU).
Taking the average over all tasks yields
% Doing this, taking the average over all tasks, and using $\|\mathbf{W}\|_2 = O(k^{-1})$ yields (ignoring regularization):
\begin{align}
\vspace{-1mm}
    &\mathcal{L}(\mathbf{W}^0,\mathbf{b}^0,\{\mathbf{a}^{1}_i\}_{i})\nonumber\\
    &= \E_{i,\mathbf{x} }  \left[ \sigma\left( 1- \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}'} [ f_{i}(\mathbf{x}') \sigma(\bar{\mathbf{W}}^0 \mathbf{x}') ]^\top \sigma( \mathbf{W}^0\mathbf{x})   \right) 
%     \frac{1}{n_2}\sum_{j=1}^{n_2}\max \left(1 - y_{i,j} \left(\frac{1}{\lambda_{1}n_1}\sum_{j'=1}^{n_1}\bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})  \right)^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}), 0\right) \right] \nonumber\\
% &= 1 -  \E_{i }  \left[ \frac{1}{\lambda_{1} n_1n_2}\sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})
\right] \nonumber \\
&\approx 1 -\eta \E_{\mathbf{x}, \mathbf{x}' }  \left[  \beta({\mathbf{x},\mathbf{x}'}) \sigma(\bar{\mathbf{W}}^0 \mathbf{x}')^\top \sigma( \mathbf{W}^0\mathbf{x}) \right] \label{tjjt}
\end{align}
% \begin{align}
% % F(\mathbf{W}) :=  
% \E_{i} \left[  \mathcal{L}_i(\mathbf{W},\mathbf{a}_i; \mathcal{D}_{i,2}) \right] &= \E_{i }  \left[ \frac{1}{n_2}\sum_{j=1}^{n_2}\max \left(1 - y_{i,j} \left(\frac{1}{\lambda_{1}n_1}\sum_{j'=1}^{n_1}\bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})  \right)^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}), 0\right) \right] \nonumber\\
% &= 1 -  \E_{i }  \left[ \frac{1}{\lambda_{1} n_1n_2}\sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})\right] \label{14}
% \end{align} 
% with high probability over the samples $\mathbf{x}_{i,j},\bar{\mathbf{x}}_{i,j'}$, 
% where we have used $\E_{i}$ as shorthand for $\E_{i \sim \text{Unif}(\mathcal{T})} $, and \eqref{14} follows using the fact that $\|\mathbf{W}\|_2 = O(k^{-1})$, so the $\max()$ is inactive for all data points. 
where %the notation $\bar{\sigma}$ denotes stop-gradient, and
the approximation holds as $|\eta \mathbb{E}_{\mathbf{x}'} [ f_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}') ]^\top \sigma(\mathbf{W}^0\mathbf{x}) | < 1$ w.h.p. over $\mathbf{x}$ and $\mathbf{W}^0$. The resulting loss in \eqref{tjjt} encourages the first-layer representation to align sample pairs $(\mathbf{x},{\mathbf{x}'})$ that  have the same label for most tasks ($ \beta({\mathbf{x},\mathbf{x}'}) \approx 1$) and penalizes the representation for aligning pairs of samples that do not have the same label on most tasks ($ \beta({\mathbf{x},\mathbf{x}'}) \ll 1$). In this way, \eqref{tjjt} is reminiscent of a constrastive loss\footnote{This analysis suggests that any $\beta(\mathbf{x},\mathbf{x}')$ that is ``roughly'' increasing with the similarity of $\mathbf{Mx}$ and $\mathbf{Mx}'$ results in a pseudo-contrastive loss, that, as we later show, results in representation learning. As such, our observations suggest that
 Assumption \ref{assump:diversity} can be relaxed to the very natural condition that the correlation of the labels of $\mathbf{x}$ and $\mathbf{x}'$ across tasks is roughly increasing with the similarity of their ground-truth features. We verify this conjecture empirically in Appendix \ref{sec:sims}.} \cite{chen2020simple} in which positive pairs are pairs with large $\beta$.
% behaves similarly to supervised contrastive losses \cite{khosla2020supervised}. 
% , which have been shown to encourage effective representations in practice 


% \vspace{-1mm}

% we expect that in typical multi-task settings, the correlation between the labels of two points across tasks should roughly increase with the similarity of their ground-truth features, which is exactly what this condition states (as long as the labels are mean zero). 

% However, these observations alone do not imply downstream performance guarantees: it remains to show how optimizing this loss recovers the ground-truth features in the data.
% Nevertheless, it remains to show that taking a gradient step with respect to \eqref{14} leads to a generalizable representation in our setting. 
To translate these intuitive connections with contrastive learning to feature learning, we must leverage Assumption \ref{assump:diversity}, which implies that
% , the larger number  of pretraining tasks  $T$,  the more  information that 
$\beta({\mathbf{x},\mathbf{x}'})$ encodes information about the ground-truth features  $\mathbf{Mx}$ and $\mathbf{Mx}'$.
In particular, pairs of points with the {\em same} sign patterns among the ground-truth features have the same label, so $\beta({\mathbf{x},\mathbf{x}'})=1$ almost surely, while pairs of points with {\em different} sign patterns on the ground-truth features have the same label for only half of the tasks in the universe of tasks $\mathcal{T}$, meaning $\beta({\mathbf{x},\mathbf{x}'})=0$.
% \rightarrow 0$.
% as the number of tasks drawn for training increases. 
% In other words, two points with differing sign patters in the ground-truth latent coordinates are almost equally as likely to share the same binary label as they are to have different labels. 
As a result, the loss can now be approximated as:
\begin{align}
    &\tfrac{1}{\eta}\mathcal{L}(\mathbf{W}^0,\mathbf{b}^0,\{\mathbf{a}_{i}^1\}_{i}) \approx \label{15}  \\
    &\!-\! \E_{\mathbf{x}, \mathbf{x}' } \! \left[ \chi\{\sign(\mathbf{Mx})\!= \!\sign(\mathbf{Mx}')\}\sigma(\bar{\mathbf{W}}^0\mathbf{x}') ^\top \sigma(\mathbf{W}^0\mathbf{x}) \right] \nonumber
\end{align}
% where $\chi \{A\}$ is the indicator function for the event $A$.
% \textcolor{blue}{$\chi\{\}$ or $\chi$? }
We next show that a gradient descent step on \eqref{15}
% \footnote{Technically speaking, the first ReLU operation $\sigma(\mathbf{W}^0\mathbf{x}')$ has a stop-gradient with respect to $\mathbf{W}$, since this term results from the update $\mathbf{a}_i^+$ and we do not differentiate with respect to $\mathbf{W}$ through this update.} 
results in $\mathbf{W}^1$ essentially projecting onto the row space of $\mathbf{M}$.

% \begin{remark}[Importance of nonlinearity] Without the nonlinearity due to the ReLU activation, the loss in \eqref{15} may become meaningless. For example, consider that $\bar{\mathcal{T}}$ is the set of parity-based labelings (Example 2 in Section \ref{sec:formulation}). Then, if we removed the ReLU activation the loss becomes zero for all features...
% \end{remark}

\textbf{Step 2: Update neuron weights.} The proof of this step requires computing the gradient of $\mathcal{L}(\mathbf{W}^0,\mathbf{b}^0,\{\mathbf{a}_{i}^1\}_{i})$  with respect to each vector of neuron weights. For ease of notation, we from here onwards denote $\mathbf{w}_{j}=\mathbf{w}_j^0$. Using \eqref{15}, this gradient can be approximated by $\mathbf{A}(\mathbf{w}_j)\mathbf{w}_{j}$, where  $\mathbf{A}(\mathbf{w}) \in \mathbb{R}^{d\times d}$ is defined as:
% $ \Pi_{\parallel}\left(\mathbf{A}(\mathbf{w}_{j}^0)\mathbf{w}_{j}^0\right) \approx \eta 2^{-r-2}(1+ 2/\pi) \mathbf{w}_{j,:r}^0 $, and $ \Pi_{\perp}\left(\mathbf{A}(\mathbf{w}_{j}^0)\mathbf{w}_{j}^0\right) \approx \eta 2^{-r-2}(1+ 2/\pi) \mathbf{w}_{j,:r}^0 $
% After some algebra, we find that this gradient is approximately equal to $\mathbf{A}(\mathbf{w}_{j}^0)\mathbf{w}_{j}^0)$, where  $\mathbf{A}(\mathbf{w}_{j}^0) \in \mathbb{R}^{d\times d}$ is a matrix satisfying 
% (recall that  $\mathbf{w}_{j,:r}^0$ denotes the first $r$ coordinates of $\mathbf{w}_{j}^0$ and $\mathbf{w}_{j,r:}^0$ denotes the last $d-r$ coordinates):
\begin{align}
    % &\\
    &\mathbf{A}(\mathbf{w}) := \!-\! \E_{\mathbf{x}, \mathbf{x}' }  \big[ \chi\{\sign(\mathbf{Mx}) = \sign(\mathbf{Mx}')\} \nonumber \\
    &\quad \quad \quad \quad  \quad \quad \quad \quad\times \sigma'(\mathbf{w}^\top \mathbf{x})\sigma'(\bar{\mathbf{w}}^\top \mathbf{x}')\mathbf{x}(\mathbf{x}')^\top \big]\label{16}  %\\
    % &\approx 2^{-r-2}\begin{bmatrix}
    %     \mathbf{I}_r & \tfrac{2}{\pi \|\mathbf{w}_{j,r:}^0\|_2^2} \mathbf{w}_{j,:r}^0(\mathbf{w}_{j,r:}^0)^\top \\
    %     \tfrac{2}{\pi \|\mathbf{w}_{j,r:}^0\|_2^2}\mathbf{w}_{j,r:}^0(\mathbf{w}_{j,:r}^0)^\top  & \tfrac{2}{\pi \|\mathbf{w}_{j,r:}^0\|_2^2}\mathbf{w}_{j,r:}^0(\mathbf{w}_{j,r:}^0)^\top 
    % \end{bmatrix} \label{a}
\end{align}
where $\sigma'(z) = 1$ if $z>0$ and $\sigma'(z) = 0$ otherwise.
The crucial reason why $\mathbf{A}(\mathbf{w}_{j})$ has favorable structure is due to the indicator $ \chi\{\sign(\mathbf{Mx})= \sign(\mathbf{Mx}')\}$ in the RHS of \eqref{15}.
% , which resulted from Assumption \ref{assump:diversity} and large $T$ as described above.
Intuitively, this indicator encourages the first-layer weights to align {\em only} the representations of points with the same sign pattern on the label-relevant coordinates, by ensuring that only these pairs of points appear in the gradient. 
With this indicator removed, we would have $\mathbf{A}(\mathbf{w}_{j}) = \frac{2}{\pi \|\mathbf{w}_{j}\|_2^2}\mathbf{w}_{j} \mathbf{w}_{j}^\top $, meaning the gradient would not put any emphasis on the ground-truth projection. However, 
the indicator means that $ \mathbf{A}(\mathbf{w}_{j})$ is an average outer product over vectors whose signs agree on the $r$ important features and may disagree on all other features. This disagreement results in cancellation during averaging, unlike the important $r$ features, leading to:
\begin{align}
\vspace{-1mm}
    % \mathbf{A}(\mathbf{w}_{j}) 
    % % &= -\E_{\mathbf{x}, \mathbf{x}' }  \left[ \chi\{\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}'_{:r})\} \sigma'((\mathbf{w}_{j}^0)^\top \mathbf{x})\sigma'((\mathbf{w}_{j}^0)^\top \mathbf{x}')\mathbf{x}(\mathbf{x}')^\top \right]. \label{16} %\\
    % &\approx -2^{-r-2}\begin{bmatrix}
    %     \mathbf{I}_r & \tfrac{2}{\pi \|\mathbf{Mw}_{j}\|_2^2} \mathbf{Mw}_{j}\mathbf{w}_{j}^\top\mathbf{M}^\top \\
    %     \tfrac{2}{\pi \|\mathbf{M}_{\perp}\mathbf{w}_{j}\|_2^2}\mathbf{M}_\perp\mathbf{w}_{j}\mathbf{w}_{j}^\top \mathbf{M}^\top & \tfrac{2}{\pi \|\mathbf{M}_{\perp}\mathbf{w}_{j}\|_2^2}\mathbf{M}_{\perp}\mathbf{w}_{j}\mathbf{w}_{j}^\top\mathbf{M}_{\perp}^\top 
    % \end{bmatrix} \label{a}
    \mathbf{M}\mathbf{A}(\mathbf{w}_{j}) \mathbf{w}_j 
    % &= -\E_{\mathbf{x}, \mathbf{x}' }  \left[ \chi\{\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}'_{:r})\} \sigma'((\mathbf{w}_{j}^0)^\top \mathbf{x})\sigma'((\mathbf{w}_{j}^0)^\top \mathbf{x}')\mathbf{x}(\mathbf{x}')^\top \right]. \label{16} %\\
    &\approx -\tfrac{1}{2^{r}\pi }\mathbf{Mw}_j \label{rowp} \\
   \mathbf{M}_\perp \mathbf{A}(\mathbf{w}_{j}) \mathbf{w}_j  &\approx -\tfrac{1}{2^{r+1}\pi }\mathbf{M}_\perp \mathbf{w}_j\label{rowp2}
    % \begin{bmatrix}
    %     \mathbf{I}_r & \tfrac{2}{\pi \|\mathbf{Mw}_{j}\|_2^2} \mathbf{Mw}_{j}\mathbf{w}_{j}^\top\mathbf{M}^\top \\
    %     \tfrac{2}{\pi \|\mathbf{M}_{\perp}\mathbf{w}_{j}\|_2^2}\mathbf{M}_\perp\mathbf{w}_{j}\mathbf{w}_{j}^\top \mathbf{M}^\top & \tfrac{2}{\pi \|\mathbf{M}_{\perp}\mathbf{w}_{j}\|_2^2}\mathbf{M}_{\perp}\mathbf{w}_{j}\mathbf{w}_{j}^\top\mathbf{M}_{\perp}^\top 
    % \end{bmatrix} 
    % \label{a}
\end{align}
meaning that the gradient up-weights the energy of $\mathbf{w}_j$ in the ground-truth subspace by a factor of roughly 2 compared to the the energy in the spurious subspace.
% where \eqref{16} follows immediately from \eqref{15}. 
% Observe that the minimum eigenvalue of the projection of the row and column spaces of $ \mathbf{A}(\mathbf{w}_{j})$ onto the row space of $\mathbf{M}$ (equation \eqref{rowp}) is $\frac{\pi}{2}$ times larger than the maximum eigenvalue of their projection onto the row space of $\mathbf{M}_{\perp}$  (equation \eqref{rowp2}).
% This shows $\mathbf{w}_{j}$ gains more energy in the ground-truth projection $\mathbf{Mw}_{j}$ than the spurious projection $\mathbf{M}_{\perp}\mathbf{w}_{j}$ by an $\Omega(1)$ factor. 
Moreover, applying $ \mathbf{A}(\mathbf{w}_{j})$ to $\mathbf{w}_{j}$ does not change the direction of $\mathbf{Mw}_{j}$, meaning $\mathbf{Mw}_{j}^1$ remains isotropic in $\mathbb{R}^r$. These observations are the crux of the proof; please see Appendix \ref{app:thrm1} for full details.



% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/multi-task_fig.pdf}
%     \caption{Caption}
%     \label{fig:enter-label}
% \end{figure}


% To complete the proof, we use \eqref{a} to approximate the updated projections after one gradient update:
% \begin{align}
% \mathbf{Mw}_{j}^1 &\approx   \left(1 - \eta \lambda_{\mathbf{w}} + {\eta^2 2^{-r-2}}\left(1 + \frac{2}{\pi}\right) \right) \mathbf{Mw}_{j}, \nonumber \\  \mathbf{M}_{\perp}\mathbf{w}_{j}^1 &\approx   \left(1 - \eta \lambda_{\mathbf{w}} + {\eta^2 2^{-r-2}}\frac{2}{\pi} \right) \mathbf{M}_{\perp}\mathbf{w}_{j} \nonumber
% \end{align}
% The coefficient of $ \mathbf{Mw}_{j}$ in the RHS of the first equation is strictly larger than the coefficient of  $ \mathbf{M}_{\perp}\mathbf{w}_{j} $ in the RHS of the second equation.  Thus, with proper regularization, we can approximately eliminate the spurious coordinates while maintaining $\eta \Omega(1)$ energy (and isotropicity) in the ground-truth coordinates with one gradient step. 
% This completes the proof.



% Applying these approximations completes the proof.










==> ProofSketch.tex <==
\section{Proof Sketch} \label{sec:sketch}

In this section we sketch the proof of Proposition \ref{prop:1}, which is the key feature learning result that enables downstream guarantees.
% We focus on the infinite sample case for ease of exposition.
% He we focus on AltMinGD since it is easier to analyze than FO-ANIL yet the analysis conveys all of the main ideas for the FO-ANIL analysis. 
The proof heavily leverages the fact that multi-task pre-training entails updating the first-layer weights {\em after} fitting a unique head to each task.
Surprisingly, we show that solving for the optimal head for each task induces a pseudo-contrastive loss that encourages representations of two points to be similar if and only if they are likely to share a label on a randomly drawn task. Since two points are likely to share a label on a drawn task if and only if they share the same sign pattern for their first $r$ ground-truth coordinates (by Assumption \ref{assump:diversity}), the pseudo-contrastive loss inclines the representation to extract the first $r$ latent coordinates.

\textbf{Step 1: Derive pseudo-contrastive loss after head updates.} We first update the task-specific head with one gradient step for each task $i$ given the initial parameters $(\mathbf{W}^0,\mathbf{b}^0,\mathbf{a}_{i}^0)$. 
% \textcolor{blue}{"optimal" head or one-step-gradient head?}
Due to the symmetric initialization, $f(\mathbf{x};\mathbf{W}^0,\mathbf{b}^0,\mathbf{a}^0_i)=0$ for all $\mathbf{x}\in \mathbb{R}^d$, so the hinge loss is affine in $\mathbf{a}_i^0$ for all tasks (the $\max(\cdot,0)$ threshold is inactive). Therefore, using the choice of $\lambda_{\mathbf{a}} = 1/\eta $ and $\mathbf{b}^0=\mathbf{0}_m$, we have
% we can set $ \nabla_{\mathbf{a}} \mathcal{L}_i(\mathbf{W}_0,\mathbf{b}_0,\mathbf{a}) = \mathbf{0}_m $ to find
% satisfying $ \|\mathbf{W}\|_2 \leq $ and $\|\mathbf{b}\|_2 \leq $.
% with dataset $\mathcal{D}_i$ given a representation $\mathbf{W}$ satisfying $\|\mathbf{W}\|_2 = O(k^{-1})$. 
\begin{align}
   \mathbf{a}_{i}^+ &= (1 - \eta \lambda_{\mathbf{a}})\mathbf{a}_{i}^0 - \eta\nabla \mathcal{L}_i(\mathbf{W}^0,\mathbf{b}^0,\mathbf{a}_i^0) = \eta \mathbb{E}_{\mathbf{x}} [ f^*_{i}(\mathbf{x}) \sigma(\mathbf{W}^0\mathbf{x}) ]  \nonumber
   % \in \arg\min_{\mathbf{a}\in \mathbb{R}^m}\mathcal{L}_i(\mathbf{W}_0,\mathbf{b}_0,\mathbf{a}) %; \mathcal{D}_i)
   % \coloneqq \frac{1}{|\mathcal{D}_i|}\sum_{(y_{i,j},\mathbf{x}_{i,j})\in \mathcal{D}_i} \max\left( 1 - y_{i,j} \mathbf{a}^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}) , 0 \right) + \frac{\lambda_\mathbf{W}}{2} \|\mathbf{W}\|_F^2 + \frac{\lambda_\mathbf{a}}{2} \|\mathbf{a}\|_2^2 \nonumber \\
    % &\iff  \nabla_{\mathbf{a}} \mathcal{L}_i(\mathbf{W},\mathbf{b},\mathbf{a}_i) = \mathbf{0}_m  \nonumber \\ 
    %  \partial_{\mathbf{a}} 
    % \frac{1}{|\mathcal{D}_i|}\sum_{(y_{i,j},\mathbf{x}_{i,j})\in \mathcal{D}_i}y_{i,j} \sigma(\mathbf{W}\mathbf{x}_{i,j}) \chi\{\mathbf{a}^\top \sigma(\mathbf{W}\mathbf{x}_{i,j} )<1 \} \nonumber \\
    % \implies
    % \mathbf{a}_i = \frac{1}{\lambda_{1}|\mathcal{D}_i|}\sum_{(y_{i,j},\mathbf{x}_{i,j})\in \mathcal{D}_i}y_{i,j} \sigma(\mathbf{W}\mathbf{x}_{i,j}) 
    % &\iff \mathbf{a}_{0.i} = \frac{1}{\lambda_{1}}\mathbb{E}_{\mathbf{z}} [ f^*_{i}(\mathbf{M}\mathbf{z}) \sigma(\mathbf{W}_0\mathbf{Mz} + \mathbf{b}_0) ] 
\end{align} %\chi \{ f^*_{i}(\mathbf{Mz}) \sigma(\mathbf{W}\mathbf{Mz} + \mathbf{b}) < 1 \} 
% since $\mathcal{L}_i(\mathbf{W},\mathbf{a}; \mathcal{D}_{i,1})$ is a strongly convex function of $\mathbf{a}$, and the subgradient of $\mathcal{L}_i(\mathbf{W},\mathbf{a}; \mathcal{D}_i)$ with respect to $\mathbf{a}$ at $\mathbf{a}_i$ contains zero if each $\|\mathbf{x}_{i,j}\|_2 = \tilde{O}(\sqrt{k\log(k)})$\footnote{This ensures that the $\max()$ is inactive for all data points.}, which occurs with high probability. 
% \textcolor{blue}{the last equality feels like you've set ${a}_0$ to $0$ and hence might be confusing to the reader. Why don't you include ${a}_0$?}
As a result, the updated head for task $i$, $\mathbf{a}_{i}^+$, is proportional to the average label-weighted neuron output over the dataset for task $i$. Now we can insert this value of $\mathbf{a}_{i}^+$ back into the loss, to obtain $\mathcal{L}_i(\mathbf{W}^0, \mathbf{b}^0,\mathbf{a}_{i}^+)$. For ease of notation we define 
% $g(\mathbf{z};\mathbf{W},\mathbf{b})\coloneqq \sigma(\mathbf{W}\mathbf{Mz}+\mathbf{b})$ and 
$\beta({\mathbf{x},\mathbf{x}'})\coloneqq \frac{1}{T}\sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}')$ for all pairs of inputs $\mathbf{x},\mathbf{x}'$.
Taking the average over all tasks yields
% Doing this, taking the average over all tasks, and using $\|\mathbf{W}\|_2 = O(k^{-1})$ yields (ignoring regularization):
\begin{align}
    \mathcal{L}(\mathbf{W}^0,\mathbf{b}^0,\{\mathbf{a}^{0}_i\}_{i}) &= \frac{1}{T}\sum_{i=1}^T\E_{\mathbf{x} }  \left[ \max\left( 1- \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}'} [ f^*_{i}(\mathbf{x}') \sigma(\mathbf{W}^0 \mathbf{x}') ]^\top \sigma( \mathbf{W}^0\mathbf{x})  , 0 \right) 
%     \frac{1}{n_2}\sum_{j=1}^{n_2}\max \left(1 - y_{i,j} \left(\frac{1}{\lambda_{1}n_1}\sum_{j'=1}^{n_1}\bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})  \right)^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}), 0\right) \right] \nonumber\\
% &= 1 -  \E_{i }  \left[ \frac{1}{\lambda_{1} n_1n_2}\sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})
\right] \label{14} \nonumber \\
&\approx 1 -\E_{\mathbf{x}, \mathbf{x}' }  \left[  \beta({\mathbf{x},\mathbf{x}'}) \sigma(\mathbf{W}^0 \mathbf{x}')^\top \sigma( \mathbf{W}^0\mathbf{x}) \right]
\end{align}
% \begin{align}
% % F(\mathbf{W}) :=  
% \E_{i} \left[  \mathcal{L}_i(\mathbf{W},\mathbf{a}_i; \mathcal{D}_{i,2}) \right] &= \E_{i }  \left[ \frac{1}{n_2}\sum_{j=1}^{n_2}\max \left(1 - y_{i,j} \left(\frac{1}{\lambda_{1}n_1}\sum_{j'=1}^{n_1}\bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})  \right)^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}), 0\right) \right] \nonumber\\
% &= 1 -  \E_{i }  \left[ \frac{1}{\lambda_{1} n_1n_2}\sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})\right] \label{14}
% \end{align} 
% with high probability over the samples $\mathbf{x}_{i,j},\bar{\mathbf{x}}_{i,j'}$, 
% where we have used $\E_{i}$ as shorthand for $\E_{i \sim \text{Unif}(\mathcal{T})} $, and \eqref{14} follows using the fact that $\|\mathbf{W}\|_2 = O(k^{-1})$, so the $\max()$ is inactive for all data points. 
where %the notation $\bar{\sigma}$ denotes stop-gradient, and
the approximation holds as $|\eta \mathbb{E}_{\mathbf{x}'} [ f^*_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}') ]^\top \sigma(\mathbf{W}^0\mathbf{x}) | < 1$ with high probability over $\mathbf{x}$ due to the initial scaling of $\mathbf{W}^0$. The resulting loss in \eqref{14} encourages the first-layer representation that aligns  pairs of samples $(\mathbf{x},{\mathbf{x}'})$ that typically have the same label among the sampled tasks ($ \beta({\mathbf{x},\mathbf{x}'}) \approx 1$) and penalizes the representation for aligning pairs of samples that typically do not have the same label ($ \beta({\mathbf{x},\mathbf{x}'}) \approx -1$). In this way, the loss in \eqref{14} behaves similarly to supervised contrastive losses, which have been shown to encourage effective representations in practice \cite{khosla2020supervised}. 



% However, these observations alone do not imply downstream performance guarantees: it remains to show how optimizing this loss recovers the ground-truth features in the data.
% Nevertheless, it remains to show that taking a gradient step with respect to \eqref{14} leads to a generalizable representation in our setting. 
To translate these intuitive connections with contrastive learning to feature learning in our setting, we must leverage Assumption \ref{assump:diversity}, which implies that, the larger number  of pre-training tasks  $T$,  the more  information that $\beta({\mathbf{x},\mathbf{x}'})$ encodes about the ground-truth features  $\mathbf{x}_{:r}$ and $\mathbf{x}_{:r}'$.
In particular, pairs of points with the {\em same} sign patterns among the ground-truth features have the same label, so $\beta({\mathbf{x},\mathbf{x}'})=1$ almost surely, while pairs of points with {\em different} sign patterns on the ground-truth features have the same label for only half of the tasks in the universe of tasks $\mathcal{T}$, meaning $\beta({\mathbf{z},\mathbf{z}'})\rightarrow 0$ as the number of tasks drawn for training increases. 
% In other words, two points with differing sign patters in the ground-truth latent coordinates are almost equally as likely to share the same binary label as they are to have different labels. 
As a result, the loss can now be approximated as:
\begin{align}
    \mathcal{L}(\mathbf{W}^0,\mathbf{b}^0,\{\mathbf{a}_{i}^0\}_{i}) &\approx -\E_{\mathbf{x}, \mathbf{x}' }  \left[ \chi\{\sign(\mathbf{x}_{:r})= \sign(\mathbf{x}'_{:r})\}\sigma(\mathbf{W}^0\mathbf{x}') ^\top \sigma(\mathbf{W}^0\mathbf{x}) \right] \label{15} 
\end{align}
where $\chi \{A\}$ is the indicator function for the event $A$.
% \textcolor{blue}{$\chi\{\}$ or $\chi$? }
We next show that taking a gradient descent step with respect to \eqref{15}
% \footnote{Technically speaking, the first ReLU operation $\sigma(\mathbf{W}^0\mathbf{x}')$ has a stop-gradient with respect to $\mathbf{W}$, since this term results from the update $\mathbf{a}_i^+$ and we do not differentiate with respect to $\mathbf{W}$ through this update.} 
results in $\mathbf{W}^1$ essentially becoming a projection onto the ground-truth first $r$ coordinates.

% \begin{remark}[Importance of nonlinearity] Without the nonlinearity due to the ReLU activation, the loss in \eqref{15} may become meaningless. For example, consider that $\bar{\mathcal{T}}$ is the set of parity-based labelings (Example 2 in Section \ref{sec:formulation}). Then, if we removed the ReLU activation the loss becomes zero for all features...
% \end{remark}

\textbf{Step 2: Update neuron weights.} The proof of this step requires computing the gradient of $\mathcal{L}(\mathbf{W}^0,\mathbf{b}^0,\{\mathbf{a}_{i}^0\}_{i})$  with respect to $\mathbf{w}_j$ for each neuron $j\in [m]$. Using \eqref{15}, this gradient can be approximated by $\mathbf{A}(\mathbf{w}_{j}^0)\mathbf{w}_{j}^0$, where  $\mathbf{A}(\mathbf{w}_{j}^0) \in \mathbb{R}^{d\times d}$ is defined as:
% $ \Pi_{\parallel}\left(\mathbf{A}(\mathbf{w}_{j}^0)\mathbf{w}_{j}^0\right) \approx \eta 2^{-r-2}(1+ 2/\pi) \mathbf{w}_{j,:r}^0 $, and $ \Pi_{\perp}\left(\mathbf{A}(\mathbf{w}_{j}^0)\mathbf{w}_{j}^0\right) \approx \eta 2^{-r-2}(1+ 2/\pi) \mathbf{w}_{j,:r}^0 $
% After some algebra, we find that this gradient is approximately equal to $\mathbf{A}(\mathbf{w}_{j}^0)\mathbf{w}_{j}^0)$, where  $\mathbf{A}(\mathbf{w}_{j}^0) \in \mathbb{R}^{d\times d}$ is a matrix satisfying 
% (recall that  $\mathbf{w}_{j,:r}^0$ denotes the first $r$ coordinates of $\mathbf{w}_{j}^0$ and $\mathbf{w}_{j,r:}^0$ denotes the last $d-r$ coordinates):
\begin{align}
    \mathbf{A}(\mathbf{w}_{j}^0) &= -\E_{\mathbf{x}, \mathbf{x}' }  \left[ \chi\{\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}'_{:r})\} \sigma'((\mathbf{w}_{j}^0)^\top \mathbf{x})\sigma'((\mathbf{w}_{j}^0)^\top \mathbf{x}')\mathbf{x}(\mathbf{x}')^\top \right]. \label{16} %\\
    % &\approx 2^{-r-2}\begin{bmatrix}
    %     \mathbf{I}_r & \tfrac{2}{\pi \|\mathbf{w}_{j,r:}^0\|_2^2} \mathbf{w}_{j,:r}^0(\mathbf{w}_{j,r:}^0)^\top \\
    %     \tfrac{2}{\pi \|\mathbf{w}_{j,r:}^0\|_2^2}\mathbf{w}_{j,r:}^0(\mathbf{w}_{j,:r}^0)^\top  & \tfrac{2}{\pi \|\mathbf{w}_{j,r:}^0\|_2^2}\mathbf{w}_{j,r:}^0(\mathbf{w}_{j,r:}^0)^\top 
    % \end{bmatrix} \label{a}
\end{align}
where $\sigma'(z) = 1$ if $z>0$ and $\sigma'(z) = 0$ otherwise.
The crucial reason why $\mathbf{A}(\mathbf{w}_{j}^0)$ has favorable structure is the indicator $ \chi\{\sign(\mathbf{x}_{:r})= \sign(\mathbf{x}'_{:r})\}$ in the RHS of \eqref{15}.
% , which resulted from Assumption \ref{assump:diversity} and large $T$ as described above.
Intuitively, this indicator is encouraging the first-layer weights to align {\em only} the representations of points with the same sign pattern on the label-relevant coordinates, by ensuring that only these pairs of points appear in the gradient. 
With this indicator removed, we would have $\mathbf{A}(\mathbf{w}_{j}^0) = \frac{2}{\pi \|\mathbf{w}_{j}^0\|_2^2}\mathbf{w}_{j}^0(\mathbf{w}_{j}^0)^\top $, meaning the gradient would not put any emphasis on the ground-truth projection. However, 
the indicator means that $ \mathbf{A}(\mathbf{w}_{j}^0)$ is an average outer product over vectors whose signs agree on the first $r$ coordinates and may disagree on all other $d-r$ coordinates. This disagreement results in cancellation in the average for these $d-r$ coordinates, unlike the first $r$ coordinates, leading to:
\begin{align}
    \mathbf{A}(\mathbf{w}_{j}^0) 
    % &= -\E_{\mathbf{x}, \mathbf{x}' }  \left[ \chi\{\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}'_{:r})\} \sigma'((\mathbf{w}_{j}^0)^\top \mathbf{x})\sigma'((\mathbf{w}_{j}^0)^\top \mathbf{x}')\mathbf{x}(\mathbf{x}')^\top \right]. \label{16} %\\
    &\approx -\eta 2^{-r-2}\begin{bmatrix}
        \mathbf{I}_r & \tfrac{2}{\pi \|\mathbf{w}_{j,r:}^0\|_2^2} \mathbf{w}_{j,:r}^0(\mathbf{w}_{j,r:}^0)^\top \\
        \tfrac{2}{\pi \|\mathbf{w}_{j,r:}^0\|_2^2}\mathbf{w}_{j,r:}^0(\mathbf{w}_{j,:r}^0)^\top  & \tfrac{2}{\pi \|\mathbf{w}_{j,r:}^0\|_2^2}\mathbf{w}_{j,r:}^0(\mathbf{w}_{j,r:}^0)^\top 
    \end{bmatrix} \label{a}
\end{align}

% where \eqref{16} follows immediately from \eqref{15}. 
Observe that the minimum eigenvalue of the top left submatrix of $ \mathbf{A}(\mathbf{w}_{j}^0)$ is strictly larger than the maximum eigenvalue of the bottom right submatrix.
This shows $\mathbf{w}_{j}^+$ gains more energy in the ground-truth projection $\mathbf{w}_{j,:r}^0$ than the spurious projection $\mathbf{w}_{j,r:}^0$ by an $\Omega(1)$ factor.  Moreover, applying $ \mathbf{A}(\mathbf{w}_{j}^0)$ to $\mathbf{w}_{j}^0$ does not change the direction of $\mathbf{w}_{j:r}^0$, meaning $\mathbf{w}_{j,:r}^+$ remains isotropic in $\mathbb{R}^r$.


To complete the proof, we use \eqref{a} to approximate the updated projections after one gradient update:
\begin{align}
\mathbf{w}_{j,:r}^+ &\approx   \left(1 - \eta \lambda_{\mathbf{w}} + {\eta^2 2^{-r-2}}\left(1 + \frac{2}{\pi}\right) \right) \mathbf{w}_{j,:r}^0, \quad   \mathbf{w}_{j,r:}^+ &\approx   \left(1 - \eta \lambda_{\mathbf{w}} + {\eta^2 2^{-r-2}}\frac{2}{\pi} \right) \mathbf{w}_{j,r:}^0 \nonumber
\end{align}
The coefficient of $ \mathbf{w}_{j,:r}^0$ in the RHS of the first equation is strictly larger than the coefficient of  $ \mathbf{w}_{j,r:}^0$ in the RHS of the second equation.  Thus, with proper regularization, we can approximately eliminate the spurious coordinates while maintaining $\eta \Omega(1)$ energy (and isotropicity) in the ground-truth coordinates with one gradient step. 
% This completes the proof.



% Applying these approximations completes the proof.



\textbf{Extension to other losses.} We have only considered the hinge loss for simplicity. However, our observation that multi-tasking with task-specific heads induces a contrastive loss that encourages feature learning extends to other loss functions as well. If we instead use the logistic loss function for binary classification, we find that the task-specific head for task $i$  updated after step of gradient descent starting from zero has the same form as \eqref{head1} up to an absolute constant, 
% $\mathbf{a}_{1,i} = \frac{1}{2}\mathbb{E}_{(\mathbf{x}_i,y_i)}[y_i \sigma(\mathbf{W}_0 \mathbf{x})]$
% the logistic loss $\ell(\hat{y}, y) \coloneqq \log(1 + e^{-y\hat{y}})$ satisfies that
and the global loss induced by the updated heads has the form
\begin{align}
    \mathcal{L} = \mathbb{E}_{i,\mathbf{x}_i,y_i}[\log(1 + \exp(- \mathbb{E}_{\mathbf{x}_i,y_i}))]
\end{align}
This loss again encourages 
We verify empirically in Section \ref{sec:sims} that multi-tasking with the logistic loss on sparse parity tasks indeed learns the correct representation, while running on only a single task fails to do so. 
For regression with the squared loss, we again have that starting from $\mathbf{a}_{i,0}$ and executing one GD update for task $i$'s  head results in $\mathbf{a}_{i,1} = \eta \mathbb{E}[y_i\sigma (\mathbf{W}\mathbf{x}_i)]$, which is the same form as the updates for the hinge and logistic loss. The resulting global loss is thus again a function of inner products between the representations of pairs of samples, but its connection with contrastive learning is less clear, as contrastive learning is motivated by data with class structure, not regression data.






==> Proof_Errors.tex <==
\begin{lemma}
    \begin{align}
   \E_{\mathbf{u}}\left[\mathbf{u}\left(\E_{\mathbf{v}}[ \sigma'( \mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )] - \E_{\mathbf{z}}[ \sigma'( \mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )]\right) \right] &= \mathbf{0}
\end{align}
\end{lemma}
\begin{proof}
    
\end{proof}

\begin{lemma}
    \begin{align}
   \P_{\mathbf{w}}\left[\left|\E_{\mathbf{v}}[ \sigma'( \mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )] - \frac{1}{2}\right| > \frac{c\sqrt{r}}{\sqrt{k}}\right] &\leq \mathbf{0}
\end{align}
\end{lemma}
\begin{proof}
    
\end{proof}

\begin{lemma}
    \begin{align}
   \E_{\w}\left[\left(\E_{\mathbf{v}}[ \sigma'( \mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )] - \E_{\mathbf{z}}[ \sigma'( \mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )]\right)^2 \right] &= O\left(\frac{1}{k^3} \right) 
\end{align}
\end{lemma}
\begin{proof}
    
\end{proof}


\begin{lemma}
    \begin{align}
   \Pr_{\w}\left[\left|\E_{\mathbf{v}}[ \sigma'( \mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )] - \E_{\mathbf{z}}[ \sigma'( \mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )]\right| \geq \frac{1}{\sqrt{k}}\right] &= O\left(\frac{1}{} \right) 
\end{align}
\end{lemma}

\begin{proof}
    
\end{proof}




\begin{lemma}
    \begin{align}
   \E_{\w}\left[\left(\E_{\mathbf{v}}[v_1 \sigma'( \mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )] - \E_{\mathbf{z}}[z_1 \sigma'( \mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )]\right)^2 \right] &= O\left(\frac{1}{k^3} \right) 
\end{align}
\end{lemma}

\begin{proof}


We have
\begin{align}
    &\E_{\w}\left[\left(\E_{\mathbf{v}}[v_1 \sigma'( \mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )] - \E_{\mathbf{z}}[z_1 \sigma'( \mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )]\right)^2 \right] \nonumber \\
    &= \E_{\mathbf{v},\mathbf{v}'}\left[v_1 v_1' \mathbb{P}_{\mathbf{w}}\left[\mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,\parallel} >0 \cap (\mathbf{v}')^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,\parallel} >0  \right]\right] \nonumber \\
    &\quad + \E_{\mathbf{z},\mathbf{z}'}\left[z_1 z_1' \mathbb{P}_{\mathbf{w}}\left[\mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,\parallel} >0 \cap (\mathbf{z}')^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,\parallel} >0  \right]\right] \nonumber \\
    &\quad - 2 \E_{\mathbf{v},\mathbf{z}}\left[v_1 z_1 \mathbb{P}_{\mathbf{w}}\left[ \mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} >0 \cap \mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} >0 \right] \right]
\end{align}
\textbf{The first term} is equal to:
\begin{align}
    & \E_{\mathbf{v},\mathbf{v}'}\left[v_1 v_1' \mathbb{P}_{\mathbf{w}}\left[\mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,\parallel} >0 \cap (\mathbf{v}')^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,\parallel} >0  \right]\right] \nonumber \\
    &=  -\frac{1}{2 \pi}\E_{\mathbf{v},\mathbf{v}'}\left[v_1 v_1' \cos^{-1}\left( \frac{\mathbf{v}^\top \mathbf{v}' + r}{k} \right)\right] \nonumber 
\end{align}
Next,
\begin{align}
   & \E_{\vv,\vv'} \left[v_1 v_1' \cos^{-1}\left(\frac{r + \vv^\top \vv'}{k}\right)\right] \nonumber \\
   &= \frac{1}{2}\E_{\vv, \vv'_{-1}} \left[ \cos^{-1}\left(\frac{r + 1 + \vv_{-1}^\top \vv'_{-1}}{k}\right)\right] -  \frac{1}{2}\E_{\vv, \vv'_{-1}} \left[ \cos^{-1}\left(\frac{r - 1 + \vv_{-1}^\top \vv'_{-1}}{k}\right)\right] \nonumber\\
   &= \frac{1}{2}\E_{\vv} \left[ 2^{-(k-r-1)}\sum_{q=0}^{k-r-1}{k-r-1 \choose q}\cos^{-1}\left(\frac{r - 1 + k-r-1-2q}{k}\right)\right] \nonumber\\
   &\quad -  \frac{1}{2}\E_{\vv} \left[ 2^{-(k-r-1)}\sum_{q=0}^{k-r-1}{k-r-1 \choose q}\cos^{-1}\left(\frac{r - 1 + k-r-1-2q}{k}\right)\right] \nonumber\\
   &=  2^{-(k-r)}\sum_{q=0}^{k-r-1}{k-r-1 \choose q}\left( \cos^{-1}\left(1 - \frac{2q}{k}\right) - \cos^{-1}\left(1 - \frac{2(q+1)}{k}\right) \right)
\end{align}
Note that the binomial coefficients place largest weight on the terms in the sum with $q\approx (k-r-1)/2$, and for these values of $q$, the inputs to the $\cos^{-1}$ functions are close to zero. We will use the Taylor series approximation of $\cos^{-1}$ around zero to simplify the sum. First assume that $k-r-1$ is even. We have
    \begin{align}
   & \E_{\vv,\vv'} \left[v_1 v_1' \cos^{-1}\left(\frac{r + \vv^\top \vv'}{k}\right)\right] \nonumber \\
   &=  2^{k-r} {k-r-1 \choose \frac{k-r-1}{2}}\left( \cos^{-1}\left(\frac{r +1 }{k}\right) - \cos^{-1}\left(\frac{r-1}{k}\right) \right)\nonumber \\
   &\quad + 2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'}\left( \cos^{-1}\left(\frac{r +1 - 2q'}{k}\right) - \cos^{-1}\left(\frac{r-1-2q'}{k}\right) \right) \nonumber\\
   &\quad + 2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left( \cos^{-1}\left(\frac{r +1 + 2q'}{k}\right) - \cos^{-1}\left(\frac{r-1+2q'}{k}\right) \right) \nonumber 
\end{align}
Taking the Taylor series expansion of the $\cos^{-1}$ functions in the first line, we obtain
\begin{align}
    &\cos^{-1}\left(\frac{r +1 }{k}\right) - \cos^{-1}\left(\frac{r-1}{k}\right) \nonumber \\
    &= \frac{\pi}{2} - \left(\frac{r +1 }{k} + \frac{(r +1)^3 }{6 k^3} + \frac{3   (r+1)^5}{40 k^5} + O\left(\frac{r^7}{k^7}\right) \right) \nonumber \\
    &\quad -  \frac{\pi}{2} + \left(\frac{r -1 }{k} + \frac{(r -1)^3 }{6 k^3} +  \frac{3   (r-1)^5}{40 k^5} + O\left(\frac{r^7}{k^7}\right)  \right) \nonumber \\
    &= -\frac{2}{k} - \frac{ 3r^2+1 }{3k^3}  -  \frac{ 3  \times (5 r^4 + 10 r^2 + 1) }{20 k^5} + O\left(\frac{r^6}{k^7}\right)\nonumber\\
    &= -\frac{2}{k} - \frac{ 3r^2+1 }{3k^3}  + O\left(\frac{r^4}{k^5}\right)
\end{align}
Similarly, for any $q' \in \left[\frac{k-r-1}{2}\right]$, 
\begin{align}
    &\cos^{-1}\left(\frac{r +1 - 2q'}{k}\right) - \cos^{-1}\left(\frac{r-1-2q'}{k}\right) \nonumber \\
    &= \frac{\pi}{2} - \left(\frac{r +1 -2q'}{k} + \frac{(r +1 -2q')^3 }{6 k^3} + \frac{(r-2q'+1)^5}{k^5} + O\left(\frac{(r-2q')^7}{k^7}\right)  \right) \nonumber \\
    &\quad -  \frac{\pi}{2} + \left(\frac{r -1 -2q' }{k} + \frac{(r -1 - 2q')^3 }{6 k^3} + \frac{(r-2q'-1)^5}{k^5} + O\left(\frac{(r-2q')^7}{k^7}\right) \right) \nonumber \\
    % &= \frac{\pi}{2} - \left(\frac{r +1 -2q'}{k} + \frac{(r +1 -2q')^3 }{6 k^3} + \frac{(r-2q'+1)^5}{k^5} + O\left(\frac{(r-2q')^7}{k^7}\right)  \right) \nonumber \\
    % &\quad -  \frac{\pi}{2} + \left(\frac{r -1 -2q' }{k} + \frac{(r -1 - 2q')^3 }{6 k^3} + \frac{(r-2q'-1)^5}{k^5} + O\left(\frac{(r-2q')^7}{k^7}\right) \right) \nonumber \\
    &= -\frac{2}{k} - \frac{ 3(r-2q')^2+1 }{3k^3} - \frac{ 3\times \left( 5( r-2q')^4 +  10( r-2q')^2+1 \right)}{20k^5}  + O\left(\frac{(r-2q')^6}{k^7}\right) \nonumber \\
    &= -\frac{2}{k} - \frac{ 3(r-2q')^2+1 }{3k^3} - \frac{ 12 (q')^4 }{ k^5} + O\left(\frac{ (q')^3}{k^5} \right) + O\left(\frac{(r-2q')^6}{k^7}\right) 
\end{align}
and 
\begin{align}
        &\cos^{-1}\left(\frac{r +1 + 2q'}{k}\right) - \cos^{-1}\left(\frac{r-1+2q'}{k}\right) \nonumber \\
    &= -\frac{2}{k} - \frac{ 3(r+2q')^2+1 }{3k^3}  - \frac{ 12 (q')^4 }{ k^5} + O\left(\frac{ (q')^3}{k^5} \right) + O\left(\frac{(r+2q')^6}{k^7}\right) 
\end{align}
Thus
\begin{align}
    & \E_{\vv,\vv'} \left[v_1 v_1' \cos^{-1}\left(\frac{r + \vv^\top \vv'}{k}\right)\right] \nonumber \\
   &=  2^{-(k-r)} {k-r-1 \choose \frac{k-r-1}{2}}\left(  -\frac{2}{k} - \frac{ 3r^2+1 }{3k^3}  + O\left(\frac{r^4}{k^5}\right)  \right)\nonumber \\
   &\quad + 2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'}\left(  -\frac{2}{k} - \frac{ 3(r-2q')^2+1 }{3k^3}   - \frac{ 12 (q')^4 }{ k^5} + O\left(\frac{ (q')^3}{k^5} \right) + O\left(\frac{(r+2q')^6}{k^7}\right)   \right) \nonumber\\
   &\quad + 2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(  -\frac{2}{k} - \frac{ 3(r+2q')^2+1 }{3k^3}   - \frac{ 12 (q')^4 }{ k^5} + O\left(\frac{ (q')^3}{k^5} \right) + O\left(\frac{(r+2q')^6}{k^7}\right)  \right) \nonumber \\
   &= -\frac{1}{k} -  2^{-(k-r)} {k-r-1 \choose \frac{k-r-1}{2}} \frac{ r^2 }{k^3} - 2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \frac{ (r-2q')^2 + (r+2q')^2}{k^3} \nonumber \\
   &\quad - \frac{1}{6 k^3} - 2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{24(q')^4}{k^{5}}    + O\left(\frac{ (q')^3}{k^5} \right) + O\left(\frac{(r+2q')^6}{k^7}\right)\right) \nonumber \\
   &= -\frac{1}{k} - \frac{1 + 3 r^2 }{6 k^3}  - 2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \frac{ 8(q')^2}{k^3}  - 2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \frac{24(q')^4}{k^{5}} \nonumber\\
   &\quad     +2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(O\left(\frac{ (q')^3}{k^5} \right) + O\left(\frac{(r+2q')^6}{k^7}\right)\right) % + O\left(\frac{r^2}{k^3}\right)  
   \label{show}
\end{align}

% note there is missing an O(r/k^3.5) term

For the sum of $(q')^2$ terms, we have
\begin{align}
     &\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} (q')^2  \nonumber \\
     % &= \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} + q'\right)^2\nonumber \\
    &= \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} + q'\right)^2  + \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2} - q'\right)^2  \nonumber \\
    &\quad - \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} \right)^2 - \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \frac{k-r-1}{2} q' \nonumber \\
    &\quad - \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2} \right)^2 + \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \frac{k-r-1}{2} q' \nonumber \\
    &= \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} + q'\right)^2  + \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2} - q'\right)^2  \nonumber \\
    &\quad - \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} \right)^2 - \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2} \right)^2 \nonumber \\
    &= \frac{1}{2}\sum_{q=0}^{{k-r-1}}{k-r-1 \choose q} q^2 - \frac{1}{2}{k-r-1 \choose \frac{k-r-1}{2}}\left(\frac{k-r-1}{2}\right)^2  \nonumber \\
    &\quad - \frac{1}{2}  \left(\frac{k-r-1}{2} \right)^2\sum_{q=0}^{k-r-1}{k-r-1 \choose q} +  \frac{1}{2}{k-r-1 \choose \frac{k-r-1}{2}} \left(\frac{k-r-1}{2} \right)^2 \nonumber \\
    &= (k-r-1 + (k-r-1)^2 )2^{k-r-4} - (k-r-1)^2 2^{k-r-4} \nonumber \\
    &= (k-r-1 )2^{k-r-4}\label{second}
    % \sum_{q=}^{{k-r-1}{k-r-1 \choose q} q^2 - {k-r-1 \choose \frac{k-r-1}{2}}(\frac{k-r-1}{2})^2 - 
\end{align}
% [which gives us the correct result]
Similarly,
\begin{align}
     &\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} (q')^4  \nonumber \\
     &= \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} + q'\right)^2\nonumber \\
    &= \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} + q'\right)^4  + \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2} - q'\right)^4  \nonumber \\
    &\quad - \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} \right)^4 -\frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2} \right)^4 
    % - \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \frac{k-r-1}{2} q'
    \nonumber \\
    &\quad - 3\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2}\right)^2 (q')^2 - 3\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2}\right)^2 (q')^2
    % \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2} \right)^2 + \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \frac{k-r-1}{2} q' 
    \nonumber \\
    &= \frac{1}{2} \sum_{q=0}^{k-r-1} {k-r-1 \choose  q} q^4  - \frac{1}{2} {k-r-1 \choose  \frac{k-r-1}{2}} \left(\frac{k-r-1}{2}\right)^4  \nonumber \\
    &\quad - \frac{1}{2}\left(\frac{k-r-1}{2} \right)^4\sum_{q=0}^{{k-r-1}}{k-r-1 \choose q}  + \frac{1}{2} {k-r-1 \choose  \frac{k-r-1}{2}} \left(\frac{k-r-1}{2}\right)^4
    % - \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \frac{k-r-1}{2} q'
    \nonumber \\
    &\quad - 3 \times (k-r-1 )2^{k-r-4}
    \nonumber \\
    &= 2^{k-r-5}( (k-r-1)^4 + 6 (k-r-1)^3 + 3(k-r-1)^2 - 2(k-r-1)) - 2^{k-r-5}( (k-r-1)^4 + 6 (k-r-1)^3) \nonumber \\
    &= 2^{k-r-5}(  3(k-r-1)^2 - 2(k-r-1)) 
\end{align}
where we have used the computation of $\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2}\right)^2 (q')^2 $ from \eqref{second} and the equality $ \sum_{q=0}^{n} {n \choose  q} q^4  = 2^{n-4}(n^4 + 6 n^3 + 3n^2 - 2n)$ (Boros and Moll 2004, pp. 14-15, and Wolfram page on binomial sums).

{\color{red} should be divided by 2 above}

Combining these two equalities with \eqref{show} yields
\begin{align}
     \E_{\vv,\vv'} \left[v_1 v_1' \cos^{-1}\left(\frac{r + \vv^\top \vv'}{k}\right)\right] &= -\frac{1}{ k} -\frac{1}{2 k^2} - \frac{1 + 3r^2}{6k^3} + \frac{r+1}{2k^3} - \frac{24\times \tfrac{3}{2} }{32 k^3} + O\left(\frac{r^3}{k^4}\right) \nonumber \\
    &= -\frac{1}{ k} -\frac{1}{2 k^2} - \frac{2+6r^2 - 6r -6 + \tfrac{27}{2}}{12k^3} + O\left(\frac{r^3}{k^4}\right) \nonumber \\
    &= -\frac{1}{ k} -\frac{1}{2 k^2} - \frac{6r^2 - 6r +9.5}{12k^3}  + O\left(\frac{r^3}{k^4}\right)
    % = -\frac{1}{2\pi k} -\frac{1}{4\pi k^2} + O\left(\frac{r^2}{k^3}\right)
\end{align}
therefore 
\begin{align}
     &\E_{\mathbf{v},\mathbf{v}'}\left[v_1 v_1' \mathbb{P}_{\mathbf{w}}\left[\mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,\parallel} >0 \cap (\mathbf{v}')^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,\parallel} >0  \right]\right] \nonumber\\
     &= \frac{1}{ 2 \pi k} + \frac{1}{4 \pi k^2} + \frac{12r^2 - 6r + 9.5}{24 \pi k^3} + O\left(\frac{r^3}{k^4}\right)
\end{align}


\textbf{For the second term,} 
\begin{align}
    &\E_{\mathbf{z},\mathbf{z}'}\left[z_1 z_1' \mathbb{P}_{\mathbf{w}}\left[\mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,\parallel} >0 \cap (\mathbf{z}')^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,\parallel} >0  \right]\right]  \nonumber \\
    &= \E_{\mathbf{w},z_1,z_1'}\left[z_1 z_1' \mathbb{P}_{\mathbf{z}_{-1}}\left[\mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,\parallel} >0 \right] \mathbb{P}_{\mathbf{z}_{-1}'} \left[(\mathbf{z}')^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,\parallel} >0  \right]\right]  \nonumber \\
    &= \frac{1}{4} \E_{\mathbf{w},z_1,z_1'}\left[z_1 z_1' \text{erf}\left(\frac{z_1 w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel}}{\sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2} \right) \text{erf}\left(\frac{z_1' w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel}}{\sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2} \right)\right]  \nonumber 
\end{align}
Using the Taylor expansion of the error function, we have
\begin{align}
    &\text{erf}\left(\frac{z_1 w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel}}{\sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2} \right) \nonumber \\
    &= \frac{2}{\sqrt{\pi}} \left(\frac{z_1 w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel}}{\sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2}  - \frac{(z_1 w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel})^3}{6\sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2^3} + 
    \frac{(z_1 w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel})^5}{40\sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2^5}   +  O\left(\frac{1}{k^{3.5}} \right)\right)
\end{align}
Thus, letting $\mu \coloneqq \mathbf{u}^\top\mathbf{w}_{0,\parallel} $, we have
\begin{align}
    &\E_{\mathbf{z},\mathbf{z}'}\left[z_1 z_1' \mathbb{P}_{\mathbf{w}}\left[\mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,\parallel} >0 \cap (\mathbf{z}')^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,\parallel} >0  \right]\right]  \nonumber \\
    &= \frac{1}{\pi} \E_{\mathbf{w},z_1,z_1'}\Bigg[z_1 z_1' \left(\frac{z_1 w_{0,\perp,1} + \mu}{\sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2}  - \frac{(z_1 w_{0,\perp,1} + \mu)^3}{6\sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2^3} + 
    \frac{(z_1 w_{0,\perp,1} + \mu)^5}{40\sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2^5}\right)\nonumber \\
    &\quad \quad \quad \quad \quad\quad \quad \quad \left( \frac{z_1' w_{0,\perp,1} + \mu}{\sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2}  - \frac{(z_1' w_{0,\perp,1} + \mu)^3}{6\sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2^3}+ 
    \frac{(z_1' w_{0,\perp,1} + \mu)^5}{40\sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2^5} \right)\Bigg] + O(k^{-4}) \nonumber \\
    &= \frac{1}{\pi} \E_{\mathbf{w},z_1,z_1'}\Bigg[ \frac{z_1^2 (z_1')^2 w_{0,\perp,1}^2}{2\|\mathbf{w}_{0,\perp,-1}\|_2^2}
    - \frac{z_1z_1'(z_1 w_{0,\perp,1} + \mu)(z_1' w_{0,\perp,1} + \mu)\left((z_1 w_{0,\perp,1} + \mu)^2 + (z_1' w_{0,\perp,1} + \mu)^2   \right) }{12\|\mathbf{w}_{0,\perp,-1}\|_2^4} \nonumber \\
    &\quad  + \frac{z_1 z_1'(z_1 w_{0,\perp,1} + \mu)^3(z_1' w_{0,\perp,1} + \mu)^3}{72\|\mathbf{w}_{0,\perp,-1}\|_2^6} + \frac{z_1 z_1'(z_1 w_{0,\perp,1} + \mu)(z_1' w_{0,\perp,1} + \mu)\left( (z_1 w_{0,\perp,1} + \mu)^4 + (z_1' w_{0,\perp,1} + \mu)^4 \right)}{80\|\mathbf{w}_{0,\perp,-1}\|_2^6}\Bigg] \nonumber \\
    &\quad + O(k^{-4}) \nonumber \\
    &= \frac{1}{2\pi (k-r-3)} - \frac{\E[z_1^2 (z_1')^2 w_{0,\perp,1}^2(z_1^2 w_{0,\perp,1}^2 + (z_1')^2 w_{0,\perp,1}^2 ) +  6 z_1^2 (z_1')^2 w_{0,\perp,1}^2 \mu^2       ]}{12 \pi (k-r-3)(k-r-5)}  \nonumber \\
    &\quad + \frac{1}{\pi} \E_{\mathbf{w},z_1,z_1'}\Bigg[ \frac{z_1^4 (z_1')^4 w_{0,\perp,1}^6 + 3z_1^4 (z_1')^2 w_{0,\perp,1}^4 \mu^2 + 3z_1^2 (z_1')^4 w_{0,\perp,1}^4 \mu^2 + 9 z_1^2 (z_1')^2 w_{0,\perp,1}^2 \mu^4}{72\|\mathbf{w}_{0,\perp,-1}\|_2^6}   \Bigg]\nonumber \\
    &\quad + \frac{1}{\pi} \E_{\mathbf{w},z_1,z_1'}\Bigg[ \frac{w_{0,\perp,1}^2 z_1^2 (z_1')^2 ( 2 z_1^4 w_{0,\perp,1}^4 + 12(z_1')^2 w_{0,\perp,1}^2\mu^2  + 2 \mu^4 ) + 2 \mu w_{0,\perp,1} z_1^2 z_1' ( 4 (z_1')^3  w_{0,\perp,1}^3 \mu  + 4  z_1'  w_{0,\perp,1} \mu^3   )
    % (z_1  + \mu)(z_1' w_{0,\perp,1} + \mu)\left( (z_1 w_{0,\perp,1} + \mu)^4 + (z_1' w_{0,\perp,1} + \mu)^4 \right)
    }{80\|\mathbf{w}_{0,\perp,-1}\|_2^6}  \Bigg]\nonumber \\
    &\quad + O(k^{-4}) \nonumber \\
    &= \frac{1}{2\pi (k-r-3)} - \frac{9 +    3r     }{6 \pi (k-r-3)(k-r-5)}   + \frac{1}{\pi} \E_{\mathbf{w},z_1,z_1'}\Bigg[ \frac{135 + 54 r + 27r^2 }{72\|\mathbf{w}_{0,\perp,-1}\|_2^6} \Bigg] + O(k^{-4}) \nonumber \\
    &\quad + \frac{1}{\pi} \E_{\mathbf{w},z_1,z_1'}\Bigg[ \frac{30\times 15 + 108 r + 6 r^2 + 72r + 24r^2 }{80\|\mathbf{w}_{0,\perp,-1}\|_2^6} \Bigg]  + O(k^{-4}) \nonumber \\
    &= \frac{1}{2\pi (k-r-3)} - \frac{9 +    3r     }{6 \pi (k-r-3)(k-r-5)}  + \frac{15 + 6 r + 3r^2 }{8\pi (k-r-3)(k-r-5)(k-r-7)}  \nonumber \\
    &\quad + \frac{45 + 18 r + 3 r^2 }{8\pi (k-r-3)(k-r-5)(k-r-7)}  + O(k^{-4})  \nonumber \\
    &= \frac{1}{2\pi (k-r-3)} - \frac{9 +    3r     }{6 \pi (k-r-3)(k-r-5)}  + \frac{30 + 12 r + 3r^2 }{4\pi (k-r-3)(k-r-5)(k-r-7)}   + O(k^{-4}) 
\end{align}

(Aside) Note that 
\begin{align}
    \E[(\mathbf{u}^\top \w)^4] &= \sum_{i_1,i_2,i_3,i_4=1}^r u_{i_1} u_{i_2} u_{i_3} u_{i_4} \E [w_{i_1} w_{i_2} w_{i_3} w_{i_4} ]\nonumber \\
    &= r  \E [w^4] + 3 r(r-1)\E [w^2 (w')^2] \nonumber \\
    &= 3r^2
\end{align}

% The 6th moment of the inverse chi-square distribution is:
The sum of the $O(k^{-3})$ terms from the first two big terms is:
\begin{align}
 &\frac{1}{ 2 \pi k} + \frac{1}{4 \pi k^2} + \frac{12r^2 - 6r + 23}{24 \pi k^3} +   \frac{1}{2\pi (k-r-3)} - \frac{9 +    2r     }{6 \pi (k-r-3)(k-r-5)}  + \frac{30 + 12 r + 3r^2 }{4\pi (k-r-3)(k-r-5)(k-r-7)}  \nonumber \\
 &= \frac{12 k^2(k-r-3)(k-r-5)(k-r-7)}{ 24 \pi k^3(k-r-3)(k-r-5)(k-r-7)} + \frac{6 k(k-r-3)(k-r-5)(k-r-7)}{ 24 \pi k^3(k-r-3)(k-r-5)(k-r-7)} \nonumber \\
 &\quad + \frac{(12r^2 - 6r + 23)(k-r-3)(k-r-5)(k-r-7)}{24 \pi k^3(k-r-3)(k-r-5)(k-r-7)} +   \frac{12k^3(k-r-5)(k-r-7)}{24 \pi k^3 (k-r-3)(k-r-5)(k-r-7)} \nonumber \\
 &\quad - \frac{(36 +    8r) k^3 (k-r-7)   }{24 \pi k^3 (k-r-3)(k-r-5)(k-r-7)}  + \frac{(180 + 72 r + 18r^2)k^3 }{24\pi k^3 (k-r-3)(k-r-5)(k-r-7)}  \nonumber \\
 &= \frac{ ((2 k+1) 6k + 12r^2 - 6r + 23 )( k^3 - 15 k^2 - 3 k^2 r + 3 k r^2 + 15 k r + 71 k - r^3 - 105 )    
}{ 24 \pi k^3(k-r-3)(k-r-5)(k-r-7)} \nonumber \\
 &\quad + \frac{12k^3 (k^2 -2kr - 12k + r^2 + 12r + 35)}{24 \pi k^3 (k-r-3)(k-r-5)(k-r-7)} \nonumber \\
 &\quad + \frac{ - (36 +    8r) k^3 (k-r-7) + (180 + 72 r + 18r^2)k^3  }{24 \pi k^3 (k-r-3)(k-r-5)(k-r-7)}  \nonumber \\
 &=  \frac{ 12 k^5  + (36r^2  -36r - 174) k^4 + ( 48r^2 + 156r -67   )k^3
}{ 24 \pi k^3(k-r-3)(k-r-5)(k-r-7)} \nonumber \\
 &\quad + \frac{12k^5 - (24r + 144)k^4 + (12r^2+ 144r + 420)k^3 }{24 \pi k^3 (k-r-3)(k-r-5)(k-r-7)} \nonumber \\
 &\quad + \frac{ - (8r + 36)k^4  + (26r^2 + 164r + 432 )k^3 }{24 \pi k^3 (k-r-3)(k-r-5)(k-r-7)}  \nonumber \\
 &= \frac{ 24 k^2  + (36r^2  -68r - 354) k + ( 86r^2 + 464 r +785   )
}{ 24 \pi (k-r-3)(k-r-5)(k-r-7)}  
\end{align}


Finally, the \textbf{third term} is:
\begin{align}
    &2 \E_{\mathbf{v},\mathbf{z}}\left[v_1 z_1 \mathbb{P}_{\mathbf{w}}\left[ \mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} >0 \cap \mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} >0 \right] \right] \nonumber \\
    &= 2 \E_{\mathbf{v},z_1}\left[v_1 z_1 \mathbb{E}_{\mathbf{w}_0}\left[ \mathbb{E}_{\mathbf{z}_{-1}}\left[ \chi\{\mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} >0 \}\chi\{ \mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} >0 \}\right] \right]\right] \nonumber \\
    &= 2 \E_{\mathbf{v},z_1}\left[v_1 z_1 \mathbb{E}_{\mathbf{w}_0}\left[ \chi\{\mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} >0 \}\mathbb{E}_{\mathbf{z}_{-1}}\left[  \mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} >0 \right] \right]\right] \nonumber \\
    &=  \E_{\mathbf{v},z_1}\left[v_1 z_1 \mathbb{E}_{\mathbf{w}_0}\left[ \chi\{\mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} >0 \}\text{erf}\left( \frac{z_1 w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel}}{ \sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2 }  \right) \right]\right] \nonumber \\
    &= \E_{\mathbf{v},z_1}\left[v_1 z_1 \mathbb{E}_{\mathbf{w}_{0}}\left[ \chi\{ v_1 \tfrac{{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2} +\mathbf{v}_{-1}^\top \tfrac{\mathbf{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2} + \mathbf{u}^\top\tfrac{\mathbf{w}_{0,||}}{\|\mathbf{w}_{0,\perp,-1}\|_2} >0\}\text{erf}\left( \frac{z_1 w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel}}{ \sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2 }  \right) \right]\right] \nonumber 
\end{align}
%\mathbb{E}_{\mathbf{w}_{0,\parallel}, w_{0,\perp,1}, \tfrac{\w_{0,\perp,-1}}{\|\w_{0,\perp,-1}\|_2},\|\w_{0,\perp,-1}\|_2}
Since the norm and direction of a standard normal random vector are independent, we have
\begin{align}
    &\mathbb{E}_{\mathbf{w}_{0}}\left[ \chi\{ v_1 \tfrac{{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2} +\mathbf{v}_{-1}^\top \tfrac{\mathbf{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2} + \mathbf{u}^\top\tfrac{\mathbf{w}_{0,||}}{\|\mathbf{w}_{0,\perp,-1}\|_2} >0\}\text{erf}\left( \frac{z_1 w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel}}{ \sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2 }  \right) \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{w}_{0,\parallel}, w_{0,\perp,1},\|\w_{0,\perp,-1}\|_2}\left[ \mathbb{P}_{ \tfrac{\w_{0,\perp,-1}}{\|\w_{0,\perp,-1}\|_2}} \left[v_1 \tfrac{{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2} +\mathbf{v}_{-1}^\top \tfrac{\mathbf{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2} + \mathbf{u}^\top\tfrac{\mathbf{w}_{0,||}}{\|\mathbf{w}_{0,\perp,-1}\|_2} >0\right]\text{erf}\left( \frac{z_1 w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel}}{ \sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2 }  \right) \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{w}_{0,\parallel}, w_{0,\perp,1},\|\w_{0,\perp,-1}\|_2}\left[ CDF(unif_{1,k-r-1}, v_1 \tfrac{{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2 \sqrt{k-r-1}} +   \mathbf{u}^\top\tfrac{\mathbf{w}_{0,||}}{\|\mathbf{w}_{0,\perp,-1}\|_2\sqrt{k-r-1}})\text{erf}\left( \frac{z_1 w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel}}{ \sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2 }  \right) \right] \nonumber %\\
    % &= \mathbb{E}_{\mathbf{w}_{0,\parallel}, w_{0,\perp,1},\|\w_{0,\perp,-1}\|_2}\Bigg[ \left( 1-  \frac{B\left(1 - (v_1 \tfrac{{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2 \sqrt{k}}  + \mathbf{u}^\top\tfrac{\mathbf{w}_{0,||}}{\|\mathbf{w}_{0,\perp,-1}\|_2\sqrt{k}})^2; \tfrac{k-r-2}{2}, \tfrac{1}{2} \right)}{2 B(\tfrac{k-r-2}{2}, \tfrac{1}{2})}   \right)\nonumber \\
    % \mathbb{E}_{\mathbf{w}_{0,\parallel}, w_{0,\perp,1},\|\w_{0,\perp,-1}\|_2}\Bigg[ \left( 1-  \frac{B\left(1 - (v_1 \tfrac{{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2 \sqrt{k}}  + \mathbf{u}^\top\tfrac{\mathbf{w}_{0,||}}{\|\mathbf{w}_{0,\perp,-1}\|_2\sqrt{k}})^2; \tfrac{k-r-2}{2}, \tfrac{1}{2} \right)}{2 B(\tfrac{k-r-2}{2}, \tfrac{1}{2})}   \right)\nonumber \\
    % &\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \text{erf}\left( \frac{z_1 w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel}}{ \sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2 }  \right) \Bigg] \nonumber \\
\end{align}
Let $x = v_1 \tfrac{{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2 \sqrt{k-r-1}} +  \mathbf{u}^\top\tfrac{\mathbf{w}_{0,||}}{\|\mathbf{w}_{0,\perp,-1}\|_2\sqrt{k-r-1}}$. We have
% \begin{align}
%     (1 - CDF(unif_{1,k-r-1}, x) &= \chi\{x <0\} + \tfrac{1}{2} \text{sign}(x)I_{1-x^2}( \tfrac{k-r-2}{2}, \tfrac{1}{2} ) \nonumber \\
%     &= \chi\{x <0\}\tfrac{1}{2}(1 -  I_{1-x^2}( \tfrac{k-r-2}{2}, \tfrac{1}{2} ))  +\chi\{x >0\} \tfrac{1}{2} I_{1-x^2}( \tfrac{k-r-2}{2}, \frac{1}{2} )\nonumber \\
%     &= \chi\{x <0\}\tfrac{1}{2}I_{x^2}( \tfrac{1}{2}, \tfrac{k-r-2}{2}  ))  +\chi\{x >0\} \tfrac{1}{2} I_{1-x^2}( \tfrac{k-r-2}{2}, \tfrac{1}{2} ) \label{regb} \\
%     &= 
% \end{align}
\begin{align}
PDF(unif_{1,k-r-1}, x) &= \frac{\Gamma(\tfrac{k-r-1}{2})}{\sqrt{\pi} \Gamma(\tfrac{k-r-2}{2})}(1 - x^2)^{\tfrac{k-r-4}{2}} \nonumber \\
    CDF(unif_{1,k-r-1}, x) &= \tfrac{1}{2} + \frac{\Gamma(\tfrac{k-r-1}{2})}{\sqrt{\pi} \Gamma(\tfrac{k-r-2}{2})} x \;{}_2F_1\left( \tfrac{1}{2}, \tfrac{3 - (k-r-1)}{2}; \tfrac{3}{2}; x^2  \right)   \nonumber \\
    &= \tfrac{1}{2} + \frac{\Gamma(\tfrac{k-r-1}{2})}{\sqrt{\pi} \Gamma(\tfrac{k-r-2}{2})} x \left(1 + \frac{ (4 - (k-r))x^2 }{6} + \frac{(4 - (k-r))(5 - (k-r)) x^4}{40} +\dots\right)
    % {}_2F_1\left( \tfrac{1}{2}, \tfrac{3 - (k-r-1)}{2}; \tfrac{3}{2}; x  \right)   \nonumber \\
\end{align}
where ${}_2F_1\left( a,b; c; d  \right)$ is the hypergeometric function of the second kind.
Thus we have 
\begin{align}
    &\mathbb{E}_{\mathbf{w}_{0}}\left[ \chi\{ v_1 \tfrac{{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2} +\mathbf{v}_{-1}^\top \tfrac{\mathbf{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2} + \mathbf{u}^\top\tfrac{\mathbf{w}_{0,||}}{\|\mathbf{w}_{0,\perp,-1}\|_2} >0\}\text{erf}\left( \frac{z_1 w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel}}{ \sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2 }  \right) \right] \nonumber \\
    &=  \frac{\Gamma(\tfrac{k-r-1}{2})}{\sqrt{\pi} \Gamma(\tfrac{k-r-2}{2})}  \mathbb{E}_{\mathbf{w}_{0,\parallel}, w_{0,\perp,1},\|\w_{0,\perp,-1}\|_2}\Bigg[\left(v_1 \tfrac{{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2 \sqrt{k-r-1}} +   \mathbf{u}^\top\tfrac{\mathbf{w}_{0,||}}{\|\mathbf{w}_{0,\perp,-1}\|_2\sqrt{k-r-1}}\right)\nonumber \\
    &\quad \times \left( 1 + \frac{ (4 - (k-r))x^2 }{6} + \frac{(4 - (k-r))(5 - (k-r)) x^4}{{40}} +\dots  \right)\text{erf}\left( \frac{z_1 w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel}}{ \sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2 }  \right) \Bigg] \nonumber 
\end{align}

Let $\mu = \mathbf{u}^\top\mathbf{w}_{0,\parallel}$, $\nu = v_1 w_{0,\perp,1}$ and $\zeta = z_1 w_{0,\perp,1}$. We have
\begin{align}
    &\mathbb{E}_{\mathbf{w}_{0}}\left[ \chi\{ v_1 \tfrac{{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2} +\mathbf{v}_{-1}^\top \tfrac{\mathbf{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2} + \mathbf{u}^\top\tfrac{\mathbf{w}_{0,||}}{\|\mathbf{w}_{0,\perp,-1}\|_2} >0\}\text{erf}\left( \frac{z_1 w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel}}{ \sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2 }  \right) \right] \nonumber \\
    &=  \frac{\Gamma(\tfrac{k-r-1}{2})}{\sqrt{\pi} \Gamma(\tfrac{k-r-2}{2})}  \mathbb{E}_{\mathbf{w}_{0,\parallel}, w_{0,\perp,1},\|\w_{0,\perp,-1}\|_2}\Bigg[\frac{\nu + \mu}{\|\mathbf{w}_{0,\perp,-1}\|_2 \sqrt{k-r-1}} \nonumber \\
    &\quad \times \left( 1 + \frac{ (4 - (k-r))(\nu+\mu)^2 }{6 \|\mathbf{w}_{0,\perp,-1}\|_2^2 {(k-r-1)}} + \frac{(4 - (k-r))(5 - (k-r)) (\nu+\mu)^4}{{40\|\mathbf{w}_{0,\perp,-1}\|_2^4 {(k-r-1)}^2}} +\dots  \right)\text{erf}\left( \frac{\zeta + \mu}{ \sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2 }  \right) \Bigg] \nonumber \\
    &= \frac{2 \Gamma(\tfrac{k-r-1}{2})}{{\pi} \Gamma(\tfrac{k-r-2}{2})}  \mathbb{E}_{\mathbf{w}_{0,\parallel}, w_{0,\perp,1},\|\w_{0,\perp,-1}\|_2}\Bigg[\frac{\nu + \mu}{\|\mathbf{w}_{0,\perp,-1}\|_2 \sqrt{k-r-1}} \nonumber \\
    &\quad \times \left( 1 + \frac{ (4 - (k-r))(\nu+\mu)^2 }{6 \|\mathbf{w}_{0,\perp,-1}\|_2^2 ({k-r-1})} + \frac{(4 - (k-r))(5 - (k-r)) (\nu+\mu)^4}{{40\|\mathbf{w}_{0,\perp,-1}\|_2^4 {(k-r-1)}^2}} +\dots  \right)\nonumber\\
    &\quad \times \left( \frac{\zeta + \mu}{ \sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2 } - \frac{(\zeta + \mu)^3}{ 6\sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2^3 } +  \frac{(\zeta + \mu)^5}{ 40\sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2^5 } \right) \Bigg] \nonumber \\
    &= \frac{\sqrt{2} \Gamma(\tfrac{k-r-1}{2})}{{\pi} \Gamma(\tfrac{k-r-2}{2})} \Bigg( \frac{ v_1 z_1 +r}{\sqrt{k-r-1}(k-r-3)}   -  \frac{ v_1 z_1^3 +  v_1 z_1 r +  z_1^2 +r^2}{2\sqrt{k-r-1}(k-r-3)(k-r-5)} \nonumber \\
    &\quad + \frac{15 v_1 z_1^5 + 30 v_1 z_1^3 r + 15 v_1 z_1 r^2 + 15 z_1^4 r + 30 z_1^2 r^2 + 15 r^3  }{40\sqrt{k-r-1}(k-r-3)(k-r-5)(k-r-7)}  \nonumber \\
    &\quad -  \frac{(k-r-4) ( v_1^3 z_1 +  v_1 z_1 r +  v_1^2 +r^2) }{2(k-r-1)^{3/2} (k-r-3)(k-r-5) }   \nonumber\\
    &\quad + \frac{(k-r-4) ( 15r^3 + 27 v_1 z_1 r^2 +  9 (z_1^2+1) r^2 + 27 z_1^2 r+ 9(v_1^3 z_1 + v_1 z_1^3  )r + 15 v_1^3 z_1^3  ) }{36(k-r-1)^{3/2} (k-r-3)(k-r-5)(k-r-7) }  \nonumber \\
    &\quad + \frac{(k-r-4)(k-r-5) ( 15 v_1^5 z_1 + 30 v_1^3 z_1 r + 15 v_1 z_1 r^2 + 15  r + 30  r^2 + 15 r^3  ) }{40(k-r-1)^{5/2} (k-r-3)(k-r-5)(k-r-7) }  + \dots  \Bigg) \nonumber \\
    &=:(\ast) \nonumber
\end{align}
% {\color{red} arg why flipping mu for erf doesn't change anything: terms with odd mu from erf are the only ones that change. for passing through the 1 term for hyper, these odd terms must be multiplied by the one mu in the outer term. but this means they will have only one v1 in total, so they are zero. for passing through the second order hyper term, by the same argument we only need to consider the odd term in that second order hyper term. this contributes one v1. so now we have even mu and even v1 (counting the outer one) and we still need to multiply by (nu+mu). so one of v1,mu will be odd for both terms. likewise for the fourth order hyper term: if the mu from erf is odd, then either mu or v1 will be odd in the final product.

% to show that flipping mu for the hyper does not change anything: passing through the 1 term is the same: if it uses the -mu in nu-mu then v1 will ultimately be odd. if it uses odd mu from other hyper, it has two options: 1) use -mu from nu-mu. but this will make mu again positive, so nothing changes. 2) use nu from nu-mu, but then v1 will ultimately be odd.
% }

Taking the expectation of the RHS over $v_1$ and $z_1$ yields
\begin{align}
    &\E_{\mathbf{v},z_1}\left[v_1 z_1 \mathbb{E}_{\mathbf{w}_{0}}\left[ \chi\{ v_1 \tfrac{{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2} +\mathbf{v}_{-1}^\top \tfrac{\mathbf{w}_{0,\perp,-1}}{\|\mathbf{w}_{0,\perp,-1}\|_2} + \mathbf{u}^\top\tfrac{\mathbf{w}_{0,||}}{\|\mathbf{w}_{0,\perp,-1}\|_2} >0\}\text{erf}\left( \frac{z_1 w_{0,\perp,1} + \mathbf{u}^\top\mathbf{w}_{0,\parallel}}{ \sqrt{2}\|\mathbf{w}_{0,\perp,-1}\|_2 }  \right) \right]\right] \nonumber\\
    &= \E_{\mathbf{v},z_1}\left[v_1 z_1 (\ast)\right] \nonumber \\
    &= \frac{\sqrt{2} \Gamma(\tfrac{k-r-1}{2})}{{\pi} \Gamma(\tfrac{k-r-2}{2})} \Bigg( \frac{ 1}{\sqrt{k-r-1}(k-r-3)}   -  \frac{ 3 + r }{2\sqrt{k-r-1}(k-r-3)(k-r-5)} \nonumber \\
    &\quad + \frac{225 + 90 r + 15  r^2  }{40\sqrt{k-r-1}(k-r-3)(k-r-5)(k-r-7)}  \nonumber \\
    &\quad -  \frac{(k-r-4) ( 1 +   r ) }{2(k-r-1)^{3/2} (k-r-3)(k-r-5) }   \nonumber\\
    &\quad + \frac{(k-r-4) ( 27  r^2 + 9(1+3)r + 45  ) }{36(k-r-1)^{3/2} (k-r-3)(k-r-5)(k-r-7) }  \nonumber \\
    &\quad + \frac{(k-r-4)(k-r-5) ( 15 + 30 r + 15 r^2   ) }{40(k-r-1)^{5/2} (k-r-3)(k-r-5)(k-r-7) }  + \dots  \Bigg) \nonumber \\
    &= \frac{\sqrt{2} \Gamma(\tfrac{k-r-1}{2})}{{\pi} \Gamma(\tfrac{k-r-2}{2})} \Bigg( \frac{ 1}{\sqrt{k-r-1}(k-r-3)}   -  \frac{ 3 + r}{2\sqrt{k-r-1}(k-r-3)(k-r-5)} \nonumber \\
    &\quad + \frac{45 + 18 r + 3  r^2  }{8\sqrt{k-r-1}(k-r-3)(k-r-5)(k-r-7)}  \nonumber \\
    &\quad -  \frac{(k-r-4) ( 1 +   r ) }{2(k-r-1)^{3/2} (k-r-3)(k-r-5) }   \nonumber\\
    &\quad + \frac{(k-r-4) ( 3 r^2 +4r+  5  ) }{4(k-r-1)^{3/2} (k-r-3)(k-r-5)(k-r-7) }  \nonumber \\
    &\quad + \frac{(k-r-4) ( 3 + 6 r + 3 r^2   ) }{8(k-r-1)^{5/2} (k-r-3)(k-r-7) }  + \dots  \Bigg) \nonumber \\
    &\approx  \frac{\sqrt{k-r-2.5} }{{\pi}} \Bigg( \frac{ 1}{\sqrt{k-r-1}(k-r-3)}   -  \frac{ 3 + r }{2\sqrt{k-r-1}(k-r-3)(k-r-5)} \nonumber \\
    &\quad + \frac{45 + 18 r + 3  r^2  }{8\sqrt{k-r-1}(k-r-3)(k-r-5)(k-r-7)}  \nonumber \\
    &\quad -  \frac{(k-r-4) ( 1 +   r ) }{2(k-r-1)^{3/2} (k-r-3)(k-r-5) }   \nonumber\\
    &\quad + \frac{(k-r-4) ( 3 r^2 +4r+  5  ) }{4(k-r-1)^{3/2} (k-r-3)(k-r-5)(k-r-7) }  \nonumber \\
    &\quad + \frac{(k-r-4) ( 3 + 6 r + 3 r^2   ) }{8(k-r-1)^{5/2} (k-r-3)(k-r-7) }  + \dots  \Bigg)
\end{align}
which further reduces to 
\begin{align}
    &= \frac{\sqrt{k-r-2.5} }{{8 \pi \sqrt{k-r-1}} (k-r-1)^2(k-r-3)(k-r-5)(k-r-7)} \Bigg( { 8(k-r-1)^2(k-r-5)(k-r-7)}   \nonumber \\
    &\quad -  { (12+4r) }(k-r-1)^2(k-r-7) + ({45 + 18 r + 3  r^2  })(k-r-1)^2 \nonumber \\
    &\quad -  4(k-r-1){(k-r-4)(k-r-7) ( 1 +   r ) } + 2(k-r-1){(k-r-4) ( 3 r^2 + 4r+ 5  ) } \nonumber \\
    &\quad +  (k-r-5){(k-r-4) ( 3 + 6 r + 3 r^2   ) }  + \dots  \Bigg) \nonumber \\
    &= \frac{\sqrt{k-r-2.5} }{{8 \pi \sqrt{k-r-1}} (k-r-1)^2(k-r-3)(k-r-5)(k-r-7)} \Bigg( { 8(k-r-1)^2(k-r-5)(k-r-7)}   \nonumber \\
    &\quad -  { }(k-r-1)^2 \left( (12+4r)k  -  r^2 - 22 r  -129  \right) \nonumber \\ % difference was -(4rk -4r2 - 28r)
    &\quad -   (k-r-1)(k-r-4) \left( (4+4r) k +2r^2 - 24 r - 38  \right) \nonumber \\
    &\quad +  (k-r-5){(k-r-4) ( 3 + 6 r + 3 r^2   ) }  + \dots  \Bigg) \nonumber \\
    &= \frac{\sqrt{k-r-2.5} }{{8 \pi \sqrt{k-r-1}} (k-r-1)^2(k-r-3)(k-r-5)(k-r-7)} \Bigg( \nonumber \\
    &\quad { }(k-r-1)^2 \left( 8k^2 -20rk - 96k  + 12 r^2 + 124 r+280    - 12k  - 3  r^2 - 6 r +129  \right) \nonumber \\
    &\quad -   (k-r-1)(k-r-4) \left( (4+4r) k +2r^2 - 24 r - 38  \right) \nonumber \\
    &\quad +  (k-r-5){(k-r-4) ( 3 + 6 r + 3 r^2   ) }  + \dots  \Bigg) \nonumber \\
    &= \frac{\sqrt{k-r-2.5} }{{8 \pi \sqrt{k-r-1}} (k-r-1)^2(k-r-3)(k-r-5)(k-r-7)} \Bigg( \nonumber \\
    &\quad { }(k-r-1)^2 \left( 8k^2 -(20r+108)k + 9r^2 + 118 r+409  \right) \nonumber \\
    &\quad -   (k-r-1)(k-r-4) \left( (4+4r) k +2r^2 - 24 r - 38  \right) \nonumber \\
    &\quad +  (k-r-5){(k-r-4) ( 3 + 6 r + 3 r^2   ) }  + \dots  \Bigg) \nonumber \\
\end{align}
The relevant terms in the interior are:
\begin{align}
    &(k-r-1)^2 \left( 8k^2 -(20r+108)k + 9r^2 + 118 r+409  \right) \nonumber \\
    &\quad -   (k-r-1)(k-r-4) \left( (4+4r) k +2r^2 - 24 r - 38  \right) \nonumber \\
    &\quad +  (k-r-5){(k-r-4) ( 3 + 6 r + 3 r^2   ) } \nonumber \\
    &= (k-r-1)^2 \left( 8k^2 -(16r+108)k + 9r^2 + 118 r+409  \right) \nonumber \\
    &\quad - (k-r-4) \left((4+4r) k^2  - ( 2r^2 + 32r + 22 ) k  - (2r^3  -22r^2 -42r 38 ) - (3r^2 + 6r +3)k + 3r^3 +21r^2 + 33r + 15
    % ( 2r^2 - 24r - 18 -4r- 4r^2) k 
    \right) \nonumber \\ 
    &= (k^2 -(2r+2)k  + r^2 + 2r +1) \left( 8k^2 -(20r+108)k + 9r^2 + 118 r+409  \right) \nonumber \\
    &\quad - (k-r-4) \left((4+4r) k^2  - ( 5r^2 + 38r + 25 ) k   + r^3 + 43r^2 + 75r + 53
    % ( 2r^2 - 24r - 18 -4r- 4r^2) k 
    \right) \nonumber \\ 
    &= 8k^4 + \left( -(20r+108)-(16r+16)  \right) k^3 + \left( (20r+108)(2r+2) + 17r^2 + 134r + 417   \right)k^2 \nonumber\\
    &\quad + \left( -(2r+2)(9r^2 + 118 r+319 ) -(20r+108)(r^2 + 2r +1)  \right)k + (r^2 + 2r +1)(9r^2 + 118 r+409) \nonumber \\
    &\quad - (4+4r)k^3 - \left((-r-4)(4+4r) - ( 5r^2 + 38r + 25 )  \right)k^2\nonumber \\
    &\quad - \left((-r-4)(- ( 5r^2 + 38r + 25 ) + r^3 + 43r^2 + 75r + 33) \right)k - \left( (-r-4)(r^3 + 43r^2 + 75r + 33)\right) \nonumber \\ 
    % &\equiv 8k^4 - \left(36r+ 128  \right) k^3 +\left( 32r^2 +392r + 360  + 22r^2 + 152r + 356   \right)k^2 \nonumber\\
    % &\quad + \left( -(2r+2)( 13r^2 +178r + 327 ) \right)k + (r^2 + 2r +1)(5r^2 + 90 r+319) \nonumber \\
    % &\quad - \left((r+4) ( 5r^2 + 38r + 25 ) + r^3 + 43r^2 + 75r + 33) \right)k + \left( (r+4)(r^3 + 43r^2 + 75r + 33)\right)\nonumber \\
    % &= 8k^4 - \left(36r+128  \right) k^3 +\left( 32r^2 +392r + 360  + 22r^2 + 152r + 356   \right)k^2 \nonumber\\
    % &\quad - \left( 26 r^3 + 382r^2 + 1010r + 654 \right)k + 6r^4 + 147r^3 + 751r^2 + 1061r + 451 \nonumber \\
    % &\quad - \left( 6r^3 + 101r^2 + 252 r + 133 \right)k \nonumber \\
    % &= 8k^4 - \left(36r+128  \right) k^3 +\left( 54r^2 +544r + 716    \right)k^2 \nonumber\\
    % &\quad - \left( 32 r^3 + 483r^2 + 1262r + 787 \right)k + 6r^4 + 147r^3 + 751r^2 + 1061r + 451  \nonumber \\
    &\equiv 8k^4 - \left(40r+128  \right) k^3 +\left( 58r^2 +440r + 694    \right)k^2
\end{align}
% {\color{red} need to check the above}


\vspace{4mm}

\begin{align}
    \frac{ 24 k^2  + (36r^2  -68r - 354) k + ( 86r^2 + 464 r +785   )
}{ 24 \pi (k-r-3)(k-r-5)(k-r-7)}  
\end{align}

\end{proof}






% $I_x(a,b)$ is the regularized Beta function, and in \eqref{regb} we have used a property of this function (https://dlmf.nist.gov/8.17).



\begin{lemma}
    \begin{align}
   \Pr_{\w}\left[\left\|\E_{\mathbf{v}}[\mathbf{v} \sigma'( \mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )] - \E_{\mathbf{z}}[\mathbf{z} \sigma'( \mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )]\right\|_2 \geq \frac{c\sqrt{r}}{\sqrt{k}} \right] &\leq 
\end{align}
\end{lemma}

\begin{proof}
    
\end{proof}


% \begin{lemma}
%     \begin{align}
%    \Pr_{\w}\left[\left\|\E_{\mathbf{v}}[\mathbf{v} \sigma'( \mathbf{v}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )] \right\|_2 \geq c \right] &\leq 
% \end{align}
% \end{lemma}

% \begin{proof}
    
% \end{proof}

\begin{lemma}
    \begin{align}
   \E_{\mathbf{z}}[\mathbf{z} \sigma'( \mathbf{z}^\top \mathbf{w}_{0,\perp} + \mathbf{u}^\top\mathbf{w}_{0,||} )] =
\end{align}
\end{lemma}

\begin{proof}
    
\end{proof}

==> Proof_Gaussian.tex <==
\section{Proof of Theorem }


\begin{align}  
&  \frac{1}{\lambda_{1} n n_{1}n_{2} }\sum_{i=1}^n \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}) \nonumber \\
&=  \frac{1}{\lambda_{1} n n_{1}n_{2} }  \sum_{i=1}^n \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1}\chi\{\text{sign}(\bar{\mathbf{x}}_{i,j'})  =  \text{sign}(\mathbf{x}_{i,j}) \} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}) \nonumber \\
&\quad +  \frac{1}{\lambda_{1} n n_{1}n_{2} }  \sum_{i=1}^n \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1}\chi\{\text{sign}(\bar{\mathbf{x}}_{i,j'}) \neq  \text{sign}(\mathbf{x}_{i,j}) \}y_{i,j} \bar{y}_{i,j'}\bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})  \nonumber \\
% \sum_{i=1}^n \frac{1}{n_1n_2}\sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}) 
\end{align} 

\begin{align}  
&  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{i,\mathbf{x}_{i,j},\bar{\mathbf{x}}_{i,j'}}\left[ y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})\right] \nonumber \\
&=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{i,\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[ y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
&=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}}  \left[\mathbb{E}_i \left[ y_{i,j}(\bar{\mathbf{x}}_{j'})  \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'}) \right] \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
&=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}}  \left[\mathbb{E}_i \left[ 1 - 2\chi\{  y_{i,j}({\mathbf{x}}_{j}) \neq \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'})\} \right] \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
&=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[ \left( 1 - 2\mathbb{P}_i \left[ y_{i,j}({\mathbf{x}}_{j}) \neq \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'}) \right]\right) \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
&=  -\frac{2^{-r}}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[  \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j}) | \text{sign}(\bar{\mathbf{x}}_{i,j',:r})=\text{sign}({\mathbf{x}}_{i,j,:r})   \right] \nonumber \\
&\quad + \frac{2^{r} - 1}{2^{r}\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[ \left( 1 - 2\mathbb{P}_i \left[ y_{i,j}({\mathbf{x}}_{j}) \neq \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'}) \right]\right) \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j}) | \text{sign}(\bar{\mathbf{x}}_{i,j',:r})\neq \text{sign}({\mathbf{x}}_{i,j,:r})   \right] \nonumber \\
&= -\frac{2^{-r}}{\lambda_{1}} \mathbb{E}_{\mathbf{x},\bar{\mathbf{x}}} \left[  \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}})^\top \sigma(\mathbf{W}\mathbf{x}) | \text{sign}(\bar{\mathbf{x}}_{:r})=\text{sign}({\mathbf{x}}_{:r})   \right] \nonumber \\
&\quad + \frac{2^{r} - 1}{2^{r}\lambda_{1} n_{1}n_{2} } \mathbb{E}_{\mathbf{x},\bar{\mathbf{x}}} \left[ \left( 1 - 2\mathbb{P}_i \left[ y_{i}({\mathbf{x}}) \neq \bar{y}_{i}(\bar{\mathbf{x}}) \right]\right) \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}})^\top \sigma(\mathbf{W}\mathbf{x}) | \text{sign}(\bar{\mathbf{x}}_{:r})\neq \text{sign}({\mathbf{x}}_{:r})   \right] \nonumber 
\end{align} 




% \begin{align}
%     & \frac{2^{-r}}{\lambda_{1} n_{1}n_{2} }  \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1}  \mathbb{E}_{\bar{\mathbf{x}}_{i,j'},{\mathbf{x}}_{i,j}}\left[ \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}) | \text{sign}(\bar{\mathbf{x}}_{i,j',:r})=\text{sign}({\mathbf{x}}_{i,j,:r})  \right] \nonumber \\
% &\quad +  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \int_{\mathbf{x}_{i,j},\bar{\mathbf{x}}_{i,j'}} \int_{i} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})  p(\mathbf{x}_{i,j},\bar{\mathbf{x}}_{i,j'}) 
% \end{align}



% is infinite tasks the same as sampling a random pair of gaussians, then sampling the number of tasks for which they have the same label? yes but does not equal zero... yes because opposite pairs?


Differentiating with respect to the neuron weight $\mathbf{w}$ leads to the following 
\begin{align}
   & \nabla_{\mathbf{w}_j}  \mathbb{E}_{\mathbf{x},\bar{\mathbf{x}}} \left[  \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}})^\top \sigma(\mathbf{W}\mathbf{x}) | \text{sign}(\bar{\mathbf{x}}_{:r})=\text{sign}({\mathbf{x}}_{:r})   \right]\nonumber \\
   &=  \nabla_{\mathbf{w}_j}  \mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}} \left[  \bar{\sigma}(\mathbf{w}_j^\top\mathbf{M}\bar{\mathbf{z}}) \sigma(\mathbf{w}_j^\top \mathbf{Mz}) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  \nonumber \\
    &=\mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}} \left[  \mathbf{Mz} {\sigma}(\mathbf{w}_j^\top\mathbf{M}\bar{\mathbf{z}}) \sigma'(\mathbf{w}_j^\top \mathbf{Mz}) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  \nonumber \\
    &= \mathbf{M}\mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}} \left[  \mathbf{z}\bar{\mathbf{z}}^\top {\sigma}'(\mathbf{w}_j^\top  \mathbf{M}\bar{\mathbf{z}}) \sigma'(\mathbf{w}_j^\top \mathbf{Mz}) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \mathbf{M}^\top \mathbf{w}_j  \nonumber \\
    % \mathbf{A} =  \begin{bmatrix}
    %     \mathbf{A}_{.}
    % \end{bmatrix}
\end{align}
Now, for ease of notation we drop the subscript $j$.
Analyzing the matrix $\mathbf{A}(\mathbf{w}) \coloneqq \mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}} \left[  \mathbf{z}\bar{\mathbf{z}}^\top  {\sigma}'(\mathbf{w}^\top  \mathbf{M}\bar{\mathbf{z}}) \sigma'(\mathbf{w}^\top \mathbf{Mz}) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]$ is the key to the proof.
We have 
\begin{align}
    \mathbf{A}(\mathbf{w}) = \begin{bmatrix}
\mathbf{A}_{\parallel,\parallel}(\mathbf{w}) & \mathbf{A}_{\parallel,\perp}(\mathbf{w}) \\
\mathbf{A}_{\perp,\parallel}(\mathbf{w}) & \mathbf{A}_{\perp,\perp}(\mathbf{w}) \\
    \end{bmatrix}
\end{align}
where 
\begin{align}
    \mathbf{A}_{\parallel,\parallel}(\mathbf{w}) &= \mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top {\sigma}'(\mathbf{w}^\top  \mathbf{M}\bar{\mathbf{z}}) \sigma'(\mathbf{w}^\top \mathbf{Mz}) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top 
 \mathbb{E}_{\mathbf{z}_{r:},\bar{\mathbf{z}_{r:}}} \left[{\sigma}'(\mathbf{w}^\top  \mathbf{M}\bar{\mathbf{z}}) \sigma'(\mathbf{w}^\top \mathbf{Mz})\right] | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \nonumber \\
 &=  \mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top 
 \mathbb{P}_{\mathbf{z}_{r:}} \left[\mathbf{w}^\top  \mathbf{M}_{r:}\mathbf{z}_{r:} > -\mathbf{w}^\top  \mathbf{M}_{:r}{\mathbf{z}}_{:r}  \right]  \mathbb{P}_{\bar{\mathbf{z}_{r:}}} \left[ \mathbf{w}^\top \mathbf{M}_{r:}\bar{\mathbf{z}}_{r:} > -\mathbf{w}^\top \mathbf{M}_{:r}\bar{\mathbf{z}}_{:r}  \right] | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  \nonumber \\
 &= \mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top 
 \left(\frac{1}{2} + \frac{1}{2}\erf\left(\frac{\mathbf{w}^\top  \mathbf{M}_{:r}{\mathbf{z}}_{:r} }{ \sqrt{2}\| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \right) \right)  \left(\frac{1}{2} + \frac{1}{2}\erf\left(\frac{\mathbf{w}^\top  \mathbf{M}_{:r}\bar{\mathbf{z}}_{:r} }{\sqrt{2} \| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \right) \right)| \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \nonumber \\
 &= \frac{1}{4}\mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \nonumber \\
 &\quad + \frac{1}{2}\mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top 
\erf\left(\frac{\mathbf{w}^\top  \mathbf{M}_{:r}{\mathbf{z}}_{:r} }{ \sqrt{2}\| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \right) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  \nonumber \\
 &\quad + \frac{1}{4}\mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top 
 \erf\left(\frac{\mathbf{w}^\top  \mathbf{M}_{:r}{\mathbf{z}}_{:r} }{ \sqrt{2}\| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \right) \erf\left(\frac{\mathbf{w}^\top  \mathbf{M}_{:r}\bar{\mathbf{z}}_{:r} }{ \sqrt{2}\| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \right)| \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] 
\end{align}
For the first term, we have
\begin{align}
     \frac{1}{4}\mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]
     &= \frac{1}{2\pi}\mathbf{I}_r
\end{align}
(diagonal element is average of product of aligned half-normals, off diagonals are averaged of non-aligned)
For the cross term, we have
\begin{align}
     &\frac{1}{2}\mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top 
\erf\left(\frac{\mathbf{w}^\top  \mathbf{M}_{:r}{\mathbf{z}}_{:r} }{ \sqrt{2}\| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \right) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \nonumber \\
&= \frac{1}{\sqrt{\pi}} \Bigg( \frac{1}{ \sqrt{2} \| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}}_{:r}}\left[  \mathbf{z}_{:r}{\mathbf{z}}_{:r}^\top \mathbf{M}_{:r}^\top \mathbf{w} \bar{\mathbf{z}}_{:r}^\top  | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  \nonumber \\
&\quad + \frac{1}{ 2 \sqrt{2} \| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2^3 } \mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  ({\mathbf{z}}_{:r}^\top \mathbf{M}_{:r}^\top \mathbf{w})^3\mathbf{z}_{:r} \bar{\mathbf{z}}_{:r}^\top  | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  + \dots \Bigg) \nonumber \\
&=\frac{1}{{\pi}} \Bigg( \frac{1}{  \| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \mathbb{E}_{\mathbf{v},\mathbf{z}_{:r}} \left[  \mathbf{z}_{:r}{\mathbf{z}}_{:r}^\top \mathbf{M}_{:r}^\top \mathbf{w} {\mathbf{v}}^\top  | \text{sign}({\mathbf{z}}_{:r}) =\mathbf{v}   \right]  \nonumber \\
&\quad + \frac{1}{ 2  \| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2^3 } \mathbb{E}_{\mathbf{v},\mathbf{z}_{:r}} \left[  ({\mathbf{z}}_{:r}^\top \mathbf{M}_{:r}^\top \mathbf{w})^3\mathbf{z}_{:r}  {\mathbf{v}}^\top  | \text{sign}({\mathbf{z}}_{:r}) =\mathbf{v}   \right]  + \dots \Bigg) \nonumber \\
&= \mathbf{0}
\end{align}
because there is always an odd number of $\mathbf{v}$'s (write z as |z| sign(v)
- remember there is the other cross term too



The final term is 
\begin{align}
    &\mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top 
 \erf\left(\frac{\mathbf{w}^\top  \mathbf{M}_{:r}{\mathbf{z}}_{:r} }{ \sqrt{2}\| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \right) \erf\left(\frac{\mathbf{w}^\top  \mathbf{M}_{:r}\bar{\mathbf{z}}_{:r} }{ \sqrt{2}\| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \right)| \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  \nonumber \\
 &= \mathbb{E}_{\mathbf{v}} \left[\mathbb{E}_{\mathbf{z}_{:r}} \left[  \mathbf{z}_{:r} 
 \erf\left(\frac{\mathbf{w}^\top  \mathbf{M}_{:r}{\mathbf{z}}_{:r} }{ \sqrt{2}\| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \right) \bigg| \text{sign}({\mathbf{z}}_{:r})=\mathbf{v}\right] \mathbb{E}_{\bar{\mathbf{z}}_{:r}}\left[\bar{\mathbf{z}}_{:r}^\top\erf\left(\frac{\mathbf{w}^\top  \mathbf{M}_{:r}\bar{\mathbf{z}}_{:r} }{ \sqrt{2}\| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \right)\bigg| \text{sign}(\bar{\mathbf{z}}_{:r})=\mathbf{v}\right] \right]
\end{align}


\begin{align}
    \mathbf{A}_{\perp,\perp}(\mathbf{w}) &=  \mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}} \left[  \mathbf{z}_{r:}\bar{\mathbf{z}}_{r:}^\top {\sigma}'(\mathbf{w}^\top  \mathbf{M}\bar{\mathbf{z}}) \sigma'(\mathbf{w}^\top \mathbf{Mz}) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}}_{:r}} \left[ \mathbb{E}_{\mathbf{z}_{r:},\bar{\mathbf{z}}_{r:}} \left[ \mathbf{z}_{r:}\bar{\mathbf{z}}_{r:}^\top {\sigma}'(\mathbf{w}^\top  \mathbf{M}\bar{\mathbf{z}}) \sigma'(\mathbf{w}^\top \mathbf{Mz}) \right] | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})  \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}}_{:r}} \left[ \mathbb{E}_{\mathbf{z}_{r:}} \left[ \mathbf{z}_{r:} \sigma'(\mathbf{w}^\top \mathbf{Mz})  \right] \mathbb{E}_{\bar{\mathbf{z}}_{r:}} \left[\bar{\mathbf{z}}_{r:}^\top {\sigma}'(\mathbf{w}^\top  \mathbf{M}\bar{\mathbf{z}}) \right] | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})  \right] \nonumber \\
    &=  \mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}}_{:r}} \left[ \exp\left( -\frac{(\mathbf{z}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w})^2+ (\bar{\mathbf{z}}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w})^2}{2\|\mathbf{M}_{r:}^\top \mathbf{w}\|_2^2} \right)    \bigg| \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})  \right] \nonumber \\
    &\quad \times 2^{-2} \frac{2}{\pi \|\mathbf{M}_{r:}^\top \mathbf{w}\|_2^2}\mathbf{M}_{r:}^\top \mathbf{w} \mathbf{w}^\top \mathbf{M}_{r:}   \nonumber 
\end{align}
We have
\begin{align}
&\mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}}_{:r}} \left[ \exp\left( -\frac{(\mathbf{z}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w})^2+ (\bar{\mathbf{z}}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w})^2}{2\|\mathbf{M}_{r:}^\top \mathbf{w}\|_2^2} \right)    \bigg| \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})  \right] \nonumber \\
    &= 2^{-r} \sum_{\mathbf{v}\in \mathcal{H}^r} \mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}}_{:r}} \left[ \exp\left( -\frac{(\mathbf{z}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w})^2+ (\bar{\mathbf{z}}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w})^2}{2\|\mathbf{M}_{r:}^\top \mathbf{w}\|_2^2} \right)    \bigg| \text{sign}(\bar{\mathbf{z}}_{:r})= \mathbf{v}, \text{sign}({\mathbf{z}}_{:r}) = \mathbf{v}  \right] \nonumber \\
    &= 2^{-r} \sum_{\mathbf{v}\in \mathcal{H}^r} \mathbb{E}_{\mathbf{z}_{:r}} \left[ \exp\left( -\frac{(\mathbf{z}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w})^2}{2\|\mathbf{M}_{r:}^\top \mathbf{w}\|_2^2} \right)    \bigg| \text{sign}({\mathbf{z}}_{:r}) = \mathbf{v}  \right] \mathbb{E}_{\bar{\mathbf{z}}_{:r}} \left[ \exp\left( -\frac{(\bar{\mathbf{z}}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w})^2}{2\|\mathbf{M}_{r:}^\top \mathbf{w}\|_2^2} \right)    \bigg| \text{sign}(\bar{\mathbf{z}}_{:r})= \mathbf{v} \right] \nonumber \\
    &= 2^{-r} \sum_{\mathbf{v}\in \mathcal{H}^r} \mathbb{E}_{\mathbf{z}_{:r}} \left[ \exp\left( -\frac{(\mathbf{z}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w})^2}{2\|\mathbf{M}_{r:}^\top \mathbf{w}\|_2^2} \right)    \bigg| \text{sign}({\mathbf{z}}_{:r}) = \mathbf{v}  \right]^2 \nonumber \\
    &\leq \left( 2^{-r} \sum_{\mathbf{v}\in \mathcal{H}^r} \mathbb{E}_{\mathbf{z}_{:r}} \left[ \exp\left( -\frac{(\mathbf{z}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w})^2}{2\|\mathbf{M}_{r:}^\top \mathbf{w}\|_2^2} \right)    \bigg| \text{sign}({\mathbf{z}}_{:r}) = \mathbf{v}  \right] \right)^2 \nonumber \\
    &=  \mathbb{E}_{\mathbf{z}_{:r}} \left[ \exp\left( -\frac{(\mathbf{z}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w})^2}{2\|\mathbf{M}_{r:}^\top \mathbf{w}\|_2^2} \right)   \right] ^2 \nonumber \\
    &= \frac{ \| \mathbf{M}_{r:}^\top \mathbf{w} \|_2^2  }{\| \mathbf{M}^\top \mathbf{w} \|_2^2 }
\end{align}










\begin{align}
    \mathbf{A}_{\parallel,\perp}(\mathbf{w}) &= \mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{r:}^\top {\sigma}'(\mathbf{w}^\top  \mathbf{M}\bar{\mathbf{z}}) \sigma'(\mathbf{w}^\top \mathbf{Mz}) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}_{:r}} \left[  \mathbf{z}_{:r} \sigma'(\mathbf{w}^\top \mathbf{Mz}) \E_{,\bar{\mathbf{z}}_{r:}} \left[\bar{\mathbf{z}}_{r:}^\top {\sigma}'(\mathbf{w}^\top  \mathbf{M}\bar{\mathbf{z}})\right] | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \nonumber \\
    &=  \sqrt{\frac{2}{\pi}}\mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}_{:r}} \left[  \mathbf{z}_{:r} \sigma'(\mathbf{w}^\top \mathbf{Mz}) \exp\left( - \frac{(\bar{\mathbf{z}}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w})^2}{2\|\mathbf{M}_{r:}^\top \mathbf{w}\|_2^2} \right)| \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  \frac{ \mathbf{w}^\top {\mathbf{M}}_{r:} }{\|{\mathbf{M}}_{r:}^\top\mathbf{w}\|_2}  \nonumber \\
    &=  \sqrt{\frac{2}{\pi}}\mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}_{:r}} \left[  \mathbf{z}_{:r} \left(\frac{1}{2} + \frac{1}{2} \erf\left( \frac{{\mathbf{z}}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w}}{\sqrt{2}\|\mathbf{M}_{r:}^\top \mathbf{w}\|_2} \right) \right) \exp\left( - \frac{(\bar{\mathbf{z}}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w})^2}{2\|\mathbf{M}_{r:}^\top \mathbf{w}\|_2^2} \right)| \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  \frac{ \mathbf{w}^\top {\mathbf{M}}_{r:} }{\|{\mathbf{M}}_{r:}^\top\mathbf{w}\|_2}  \nonumber \\
    &=  \frac{1}{\sqrt{2\pi}}\mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}_{:r}} \left[  \mathbf{z}_{:r} \erf\left( \frac{{\mathbf{z}}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w}}{\sqrt{2}\|\mathbf{M}_{r:}^\top \mathbf{w}\|_2} \right)  \exp\left( - \frac{(\bar{\mathbf{z}}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w})^2}{2\|\mathbf{M}_{r:}^\top \mathbf{w}\|_2^2} \right)| \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  \frac{ \mathbf{w}^\top {\mathbf{M}}_{r:} }{\|{\mathbf{M}}_{r:}^\top\mathbf{w}\|_2} \nonumber \\
    &= \frac{1}{\sqrt{2\pi}}\mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}_{:r}} \left[  \mathbf{z}_{:r} \erf\left( \frac{{\mathbf{z}}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w}}{\sqrt{2}\|\mathbf{M}_{r:}^\top \mathbf{w}\|_2} \right)  \exp\left( - \frac{(\bar{\mathbf{z}}_{:r}^\top\mathbf{M}_{:r}^\top \mathbf{w})^2}{2\|\mathbf{M}_{r:}^\top \mathbf{w}\|_2^2} \right)| \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  \frac{ \mathbf{w}^\top {\mathbf{M}}_{r:} }{\|{\mathbf{M}}_{r:}^\top\mathbf{w}\|_2} 
\end{align}
to get last line: condition on sign(z) = v and sign(z)= - v 






\begin{align}
    \mathbf{w}_{t+1} &= (1 - \eta \lambda)\mathbf{w}_t  + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{M} \mathbf{A}(\mathbf{w}_t)\mathbf{M}^\top \mathbf{w}_t \nonumber \\
    \mathbf{M}_{:r}^\top \mathbf{w}_{t+1} &= (1 - \eta \lambda) \mathbf{M}_{:r}^\top\mathbf{w}_t  + \frac{\eta 2^{-r}}{\lambda_1}  \begin{bmatrix}
        \mathbf{I}_r & \mathbf{0}_{r,k-r} \\
    \end{bmatrix} \mathbf{A}(\mathbf{w}_t)\mathbf{M}^\top \mathbf{w}_t  \nonumber \\
    &= (1 - \eta \lambda) \mathbf{M}_{:r}^\top\mathbf{w}_t  + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\parallel,\parallel}(\mathbf{w}_t)\mathbf{M}_{:r}^\top \mathbf{w}_t + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\parallel,\perp}(\mathbf{w}_t)\mathbf{M}_{r:}^\top \mathbf{w}_t \nonumber \\
    \mathbf{M}_{r:}^\top \mathbf{w}_{t+1} &= (1 - \eta \lambda) \mathbf{M}_{r:}^\top\mathbf{w}_t  + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\perp,\parallel}(\mathbf{w}_t)\mathbf{M}_{:r}^\top \mathbf{w}_t + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\perp,\perp}(\mathbf{w}_t)\mathbf{M}_{r:}^\top \mathbf{w}_t \nonumber \\
\end{align}
% \begin{align}
%     \mathbf{w}_t = \mathbf{M}_{:r}^\top \mathbf{w}_t + \mathbf{M}_{r:}^\top \mathbf{w}_t + (\mathbf{I}- \mathbf{MM}^\top)  \mathbf{w}_t = a_t  \mathbf{M}_{:r}^\top \mathbf{w}_0 + b_t\mathbf{M}_{r:}^\top \mathbf{w}_0 + c_t (\mathbf{I}- \mathbf{MM}^\top)  \mathbf{w}_0 
% \end{align}

\begin{align}
    a_{t} &:=  \frac{ 1 }{ \| \mathbf{M}_{:r}^\top \mathbf{w}_0\|_2 } \mathbf{w}_{0}^\top \mathbf{M}_{:r} \mathbf{M}_{:r}^\top \mathbf{w}_t \nonumber \\
    b_{t} &:= \frac{ 1 }{ \| \mathbf{M}_{r:}^\top \mathbf{w}_0\|_2 } \mathbf{w}_{0}^\top \mathbf{M}_{r:} \mathbf{M}_{r:}^\top \mathbf{w}_t \nonumber \\
    \mathbf{w}_t &:=  \frac{ a_t }{ \| \mathbf{M}_{:r}^\top \mathbf{w}_0\|_2 }  \mathbf{M}_{:r} \mathbf{M}_{:r}^\top \mathbf{w}_0   +  \frac{ b_t }{ \| \mathbf{M}_{r:}^\top \mathbf{w}_0\|_2 }  \mathbf{M}_{r:} \mathbf{M}_{r:}^\top \mathbf{w}_0 \nonumber \\
    &\quad + \left( \mathbf{I} - \frac{ 1 }{ \| \mathbf{M}_{:r}^\top \mathbf{w}_0\|_2^2 } \mathbf{M}_{:r} \mathbf{M}_{:r}^\top \mathbf{w}_{0} \mathbf{w}_{0}^\top \mathbf{M}_{:r} \mathbf{M}_{:r}^\top  - \frac{ 1 }{ \| \mathbf{M}_{:r}^\top \mathbf{w}_0\|_2^2 } \mathbf{M}_{r:} \mathbf{M}_{r:}^\top \mathbf{w}_{0} \mathbf{w}_{0}^\top \mathbf{M}_{r:} \mathbf{M}_{r:}^\top \right) \mathbf{w}_t \nonumber 
\end{align}


\begin{align}
    {a}_{t+1} &= (1 - \eta \lambda ) a_t +   \nonumber \\
    b_{t+1} &= (1 - \eta \lambda ) b_t +  \eta 2^{-r-2} \frac{2 f_t }{\pi}
\end{align}





% Since this loss is strongly convex in $\mathbf{a}$, we can find its minimizer by examining the elements of its subgradient and equating them with zero. Doing so yields:

% \begin{align}
%     \lambda_{\mathbf{a}} \mathbf{a} = \frac{1}{|\mathcal{D}_i|}\sum_{(y_{i,j},\mathbf{x}_{i,j})\in \mathcal{D}_i}y_{i,j} \sigma(\mathbf{W}\mathbf{x}_{i,j}) \chi\{\mathbf{a}^\top \sigma(\mathbf{W}\mathbf{x}_{i,j} )<1 \} \nonumber \\
%     \implies \mathbf{a}^\ast = \frac{1}{\lambda_{\mathbf{a}}|\mathcal{D}_i|}\sum_{(y_{i,j},\mathbf{x}_{i,j})\in \mathcal{D}_i}y_{i,j} \sigma(\mathbf{W}\mathbf{x}_{i,j}) 
% \end{align}
% as one can check that this choice of $\mathbf{a}^\ast$ gives $\mathbf{a}^\top \sigma(\mathbf{W}\mathbf{x}_{i,j} )<1$ for all $j$.


% As long as there are almost equal numbers of samples per vertex, the label factor can be appoximated with finite samples


For ease of notation we drop the subscript $j$. 
The inductive argument is as follows:
\begin{enumerate}
    \item $\|\mathbf{w}_{t+1}\|_2 \leq \frac{c_1}{k\sqrt{m}}$.
    \item 
\end{enumerate}



==> Proof_Hypercube.tex <==
\section{Data on hypercube (sparse coding model)}

Throughout, let $\mathbf{u}_i \in \mathcal{H}^{r}$ denote prefixes and $\mathbf{v}_j \in \mathcal{H}^{k-r}$ denote suffixes. 





In this section we prove Theorem \ref{thm:1}. For convenience, we restate the theorem here.

\begin{theorem}
    
\end{theorem}
\begin{proof}
    
\end{proof}

% need to show that for every task, there exists a good network with the same set of features
% just need one feature in each orthant, then can learn any function by adding biases
% bias should be between closest vertex sum and second closest vertex sum (flip one coord)

% with random features you could still get one feature closest to each vertex with only r2^r features. but the issue is that changing one coordinate of the perp would deactivate the neuron. should be able to build a lower bound out of this -- the lower bound should be k2^k neurons required. we want features that are robust to changes in the perp.

\begin{lemma}
    the biases and weights are in a nice set at initialization whp

    each is initialized at the same scale
\end{lemma}

\begin{proof}
    
\end{proof}



% \begin{lemma}
%     for all j, the hypercube to gaussian error vector has expected norm squared at most c/k2
% \end{lemma}

% \begin{proof}
    
% \end{proof}

% \begin{lemma}
%     for all j, the other error vectors have expected norm squared sufficiently small
% \end{lemma}

% \begin{proof}
    
% \end{proof}


\input{Proof_Errors}



\begin{lemma}
    with high probability, a constant fraction of neurons are good, in the sense that 

    1. error vector is less than c/k, other errors are sufficiently small

    2. w|| is large enough

    3. bias is in the correct range
    
\end{lemma}

\begin{proof}
chebyshev to upper bound probability of bad neuron, then
    hoeffding
\end{proof}



\begin{lemma}
    since the number of neurons is large enough, this set covers all $2^r$ vertices
\end{lemma}

\begin{proof}
    balls and bins. but being in the set changes the distribution? should still work.
\end{proof}

\begin{lemma}
    Suppose $\lambda \geq $. On the first iteration, the locally updated head for task $i$ is:
    \begin{align}
        \mathbf{a}_{1,i} = \frac{1}{\lambda_1}
    \end{align}
    for all tasks $i\in \mathcal{T}$.
\end{lemma}

\begin{proof}
    
\end{proof}


\begin{lemma}\label{lem:compute_grad}
    The gradient of the global loss with respect to the representation after updating the task-specific heads on the first iteration is $-\frac{1}{2^{r}\lambda_1}\mathbf{A}(\w)\w$, where
%     \begin{align}
%     \w^+ &= \w(1 - \eta \lambda) + \eta \begin{bmatrix}
%         \mathbf{A}_{||,||}(\w) &  \mathbf{A}_{||,\perp}(\w) \\
%         \mathbf{A}_{\perp,||}(\w) & \mathbf{A}_{\perp,\perp}(\w) \\
%     \end{bmatrix}\w
% \end{align}
    \begin{align}
    \mathbf{A}(\w) \coloneqq \begin{bmatrix}
        \mathbf{A}_{||,||}(\w) &  \mathbf{A}_{||,\perp}(\w) \\
        \mathbf{A}_{\perp,||}(\w) & \mathbf{A}_{\perp,\perp}(\w) \\
    \end{bmatrix}
\end{align}
and
\begin{align}
    \mathbf{A}_{||,||}(\w) &= \mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[ \mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2 \mathbf{uu}^\top  \right] \\
    \mathbf{A}_{||,\perp}(\w) &= \mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[ \mathbb{E}_{\mathbf{v}\sim \text{Unif}( \mathcal{H}^{k-r})} \left[\sigma'( \mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right] \mathbf{u} \mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^{k-r})}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right] \\
    \mathbf{A}_{\perp,||}(\w) &=  \mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[  \mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^{k-r})}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right] \mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^{k-r})} \left[\sigma'( \mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\right] \mathbf{u}^\top  \right] \\
    \mathbf{A}_{\perp,\perp}(\w) &=  \mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[  \mathbb{E}_{\mathbf{v}\sim \text{Unif}( \mathcal{H}^{k-r})}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]  \mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^{k-r})}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right] 
\end{align}
\end{lemma}

\begin{proof}
    
\begin{align}  
&  \frac{1}{\lambda_{1} n n_{1}n_{2} }\sum_{i=1}^n \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}) \nonumber \\
&=  \frac{1}{\lambda_{1} n n_{1}n_{2} }  \sum_{i=1}^n \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1}\chi\{\text{sign}(\bar{\mathbf{x}}_{i,j'})  =  \text{sign}(\mathbf{x}_{i,j}) \} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}) \nonumber \\
&\quad +  \frac{1}{\lambda_{1} n n_{1}n_{2} }  \sum_{i=1}^n \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1}\chi\{\text{sign}(\bar{\mathbf{x}}_{i,j'}) \neq  \text{sign}(\mathbf{x}_{i,j}) \}y_{i,j} \bar{y}_{i,j'}\bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})  \nonumber \\
% \sum_{i=1}^n \frac{1}{n_1n_2}\sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}) 
\end{align} 

\begin{align}  
&  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{i,\mathbf{x}_{i,j},\bar{\mathbf{x}}_{i,j'}}\left[ y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})\right] \nonumber \\
&=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{i,\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[ y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
&=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}}  \left[\mathbb{E}_i \left[ y_{i,j}(\bar{\mathbf{x}}_{j'})  \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'}) \right] \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
&=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}}  \left[\mathbb{E}_i \left[ 1 - 2\chi\{  y_{i,j}({\mathbf{x}}_{j}) \neq \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'})\} \right] \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
&=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[ \left( 1 - 2\mathbb{P}_i \left[ y_{i,j}({\mathbf{x}}_{j}) \neq \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'}) \right]\right) \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
&=  -\frac{2^{-r}}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[  \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j}) | \text{sign}(\bar{\mathbf{x}}_{i,j',:r})=\text{sign}({\mathbf{x}}_{i,j,:r})   \right] \nonumber \\
&\quad + \frac{2^{r} - 1}{2^{r}\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[ \left( 1 - 2\mathbb{P}_i \left[ y_{i,j}({\mathbf{x}}_{j}) \neq \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'}) \right]\right) \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j}) | \text{sign}(\bar{\mathbf{x}}_{i,j',:r})\neq \text{sign}({\mathbf{x}}_{i,j,:r})   \right] \nonumber \\
&= -\frac{2^{-r}}{\lambda_{1}} \mathbb{E}_{\mathbf{x},\bar{\mathbf{x}}} \left[  \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}})^\top \sigma(\mathbf{W}\mathbf{x}) | \text{sign}(\bar{\mathbf{x}}_{:r})=\text{sign}({\mathbf{x}}_{:r})   \right] \nonumber \\
&\quad + \frac{2^{r} - 1}{2^{r}\lambda_{1} n_{1}n_{2} } \mathbb{E}_{\mathbf{x},\bar{\mathbf{x}}} \left[ \left( 1 - 2\mathbb{P}_i \left[ y_{i}({\mathbf{x}}) \neq \bar{y}_{i}(\bar{\mathbf{x}}) \right]\right) \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}})^\top \sigma(\mathbf{W}\mathbf{x}) | \text{sign}(\bar{\mathbf{x}}_{:r})\neq \text{sign}({\mathbf{x}}_{:r})   \right] \nonumber 
\end{align} 



% \begin{align}
%     & \frac{2^{-r}}{\lambda_{1} n_{1}n_{2} }  \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1}  \mathbb{E}_{\bar{\mathbf{x}}_{i,j'},{\mathbf{x}}_{i,j}}\left[ \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}) | \text{sign}(\bar{\mathbf{x}}_{i,j',:r})=\text{sign}({\mathbf{x}}_{i,j,:r})  \right] \nonumber \\
% &\quad +  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \int_{\mathbf{x}_{i,j},\bar{\mathbf{x}}_{i,j'}} \int_{i} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})  p(\mathbf{x}_{i,j},\bar{\mathbf{x}}_{i,j'}) 
% \end{align}



% is infinite tasks the same as sampling a random pair of gaussians, then sampling the number of tasks for which they have the same label? yes but does not equal zero... yes because opposite pairs?


Differentiating with respect to the neuron weight $\mathbf{w}$ leads to the following 
\begin{align}
   & \nabla_{\mathbf{w}_j}  \mathbb{E}_{\mathbf{x},\bar{\mathbf{x}}} \left[  \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}})^\top \sigma(\mathbf{W}\mathbf{x}) | \text{sign}(\bar{\mathbf{x}}_{:r})=\text{sign}({\mathbf{x}}_{:r})   \right]\nonumber \\
   &=  \nabla_{\mathbf{w}_j}  \mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}} \left[  \bar{\sigma}(\mathbf{w}_j^\top\mathbf{M}\bar{\mathbf{z}}) \sigma(\mathbf{w}_j^\top \mathbf{Mz}) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  \nonumber \\
    &=\mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}} \left[  \mathbf{Mz} {\sigma}(\mathbf{w}_j^\top\mathbf{M}\bar{\mathbf{z}}) \sigma'(\mathbf{w}_j^\top \mathbf{Mz}) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  \nonumber \\
    &= \mathbf{M}\mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}} \left[  \mathbf{z}\bar{\mathbf{z}}^\top {\sigma}'(\mathbf{w}_j^\top  \mathbf{M}\bar{\mathbf{z}}) \sigma'(\mathbf{w}_j^\top \mathbf{Mz}) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \mathbf{M}^\top \mathbf{w}_j  \nonumber \\
    % \mathbf{A} =  \begin{bmatrix}
    %     \mathbf{A}_{.}
    % \end{bmatrix}
\end{align}
Now, for ease of notation we drop the subscript $j$.
Analyzing the matrix $\mathbf{A}(\mathbf{w}) \coloneqq \mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}} \left[  \mathbf{z}\bar{\mathbf{z}}^\top  {\sigma}'(\mathbf{w}^\top  \mathbf{M}\bar{\mathbf{z}}) \sigma'(\mathbf{w}^\top \mathbf{Mz}) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]$ is the key to the proof.
We have 
\begin{align}
    \mathbf{A}(\mathbf{w}) = \begin{bmatrix}
\mathbf{A}_{\parallel,\parallel}(\mathbf{w}) & \mathbf{A}_{\parallel,\perp}(\mathbf{w}) \\
\mathbf{A}_{\perp,\parallel}(\mathbf{w}) & \mathbf{A}_{\perp,\perp}(\mathbf{w}) \\
    \end{bmatrix}
\end{align}
where 
\begin{align}
    \mathbf{A}_{\parallel,\parallel}(\mathbf{w}) &= \mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top {\sigma}'(\mathbf{w}^\top  \mathbf{M}\bar{\mathbf{z}}) \sigma'(\mathbf{w}^\top \mathbf{Mz}) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top 
 \mathbb{E}_{\mathbf{z}_{r:},\bar{\mathbf{z}_{r:}}} \left[{\sigma}'(\mathbf{w}^\top  \mathbf{M}\bar{\mathbf{z}}) \sigma'(\mathbf{w}^\top \mathbf{Mz})\right] | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \nonumber \\
\end{align}



\end{proof}

\begin{lemma}\label{lem:apara}
    For all $j: \w_{0,j}\in \mathcal{G}_{w}$, we have 
    \begin{align}
        \|\mathbf{A}_{\parallel,\parallel}(\mathbf{w}_{0,j}) - (\tfrac{1}{4} + \sqrt{\tfrac{r}{k-r}})\mathbf{I}_r\|_2 &\leq O(k^{-1})
    \end{align}
\end{lemma}

\begin{proof}
We drop the subscript $0$ indicating time zero for ease of notation. We have 
\begin{align}
    &\mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[ \mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{z} )\right]^2 \mathbf{uu}^\top  \right] \nonumber \\
    &=  \mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[ \mathbb{E}_{\mathbf{z}\sim N(\mathbf{0}_{k-r},\mathbf{I}_{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2  \mathbf{uu}^\top  \right] \nonumber \\
    &\quad + \mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[ \left(\mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2 - \mathbb{E}_{\mathbf{z}\sim N(\mathbf{0}_{k-r},\mathbf{I}_{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{z} )\right]^2\right)  \mathbf{uu}^\top  \right] \nonumber 
\end{align}
Since each $\mathbf{uu}^\top$ is positive semi-definite, we have
\begin{align}
    &\left\|\mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[ \left(\mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2 - \mathbb{E}_{\mathbf{z}\sim N(\mathbf{0}_{k-r},\mathbf{I}_{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{z} )\right]^2\right)  \mathbf{uu}^\top  \right] \right\|_2 \nonumber \\
    &\leq \left\|\mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[ \left|\mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2 - \mathbb{E}_{\mathbf{z}\sim N(\mathbf{0}_{k-r},\mathbf{I}_{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{z} )\right]^2\right|  \mathbf{uu}^\top  \right] \right\|_2\label{prd} \\
    &\leq \left\|\mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[ b \mathbf{uu}^\top  \right] \right\|_2\nonumber \\
    &= b \nonumber 
\end{align}
where \eqref{prd} follows from Lemma \ref{lem:} and the fact that $\w\in \mathcal{G}_w$.

Next, 
\begin{align}
    &\mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[ \mathbb{E}_{\mathbf{z}\sim N(\mathbf{0}_{k-r},\mathbf{I}_{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2  \mathbf{uu}^\top  \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[ \mathbb{E}_{\mathbf{z}\sim N(\mathbf{0}_{k-r},\mathbf{I}_{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2  \mathbf{uu}^\top  \right] \nonumber \\
\end{align}

\begin{align}
    \mathbf{A}_{\parallel,\parallel}(\mathbf{w}) &= \mathbb{E}_{\mathbf{z},\bar{\mathbf{z}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top {\sigma}'(\mathbf{w}^\top  \mathbf{M}\bar{\mathbf{z}}) \sigma'(\mathbf{w}^\top \mathbf{Mz}) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top 
 \mathbb{E}_{\mathbf{z}_{r:},\bar{\mathbf{z}_{r:}}} \left[{\sigma}'(\mathbf{w}^\top  \mathbf{M}\bar{\mathbf{z}}) \sigma'(\mathbf{w}^\top \mathbf{Mz})\right] | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \nonumber \\
 &=  \mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top 
 \mathbb{P}_{\mathbf{z}_{r:}} \left[\mathbf{w}^\top  \mathbf{M}_{r:}\mathbf{z}_{r:} > -\mathbf{w}^\top  \mathbf{M}_{:r}{\mathbf{z}}_{:r}  \right]  \mathbb{P}_{\bar{\mathbf{z}_{r:}}} \left[ \mathbf{w}^\top \mathbf{M}_{r:}\bar{\mathbf{z}}_{r:} > -\mathbf{w}^\top \mathbf{M}_{:r}\bar{\mathbf{z}}_{:r}  \right] | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  \nonumber \\
 &= \mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top 
 \left(\frac{1}{2} + \frac{1}{2}\erf\left(\frac{\mathbf{w}^\top  \mathbf{M}_{:r}{\mathbf{z}}_{:r} }{ \sqrt{2}\| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \right) \right)  \left(\frac{1}{2} + \frac{1}{2}\erf\left(\frac{\mathbf{w}^\top  \mathbf{M}_{:r}\bar{\mathbf{z}}_{:r} }{\sqrt{2} \| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \right) \right)| \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \nonumber \\
 &= \frac{1}{4}\mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right] \nonumber \\
 &\quad + \frac{1}{2}\mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top 
\erf\left(\frac{\mathbf{w}^\top  \mathbf{M}_{:r}{\mathbf{z}}_{:r} }{ \sqrt{2}\| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \right) | \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  \nonumber \\
 &\quad + \frac{1}{4}\mathbb{E}_{\mathbf{z}_{:r},\bar{\mathbf{z}_{:r}}} \left[  \mathbf{z}_{:r}\bar{\mathbf{z}}_{:r}^\top 
 \erf\left(\frac{\mathbf{w}^\top  \mathbf{M}_{:r}{\mathbf{z}}_{:r} }{ \sqrt{2}\| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \right) \erf\left(\frac{\mathbf{w}^\top  \mathbf{M}_{:r}\bar{\mathbf{z}}_{:r} }{ \sqrt{2}\| \mathbf{M}_{r:}^\top {\mathbf{w}} \|_2 } \right)| \text{sign}(\bar{\mathbf{z}}_{:r})=\text{sign}({\mathbf{z}}_{:r})   \right]  \label{apara3}
\end{align}


\begin{align}
    
\end{align}





\end{proof}



\begin{lemma} \label{lem:aperp}
    For all $j: \w_{0,j}\in \mathcal{G}_{w}$, we have 
    \begin{align}
        \|\mathbf{A}_{\perp,\perp}(\mathbf{w}_{0,j}) - \|_2 &\leq 
    \end{align}
\end{lemma}


\begin{proof}
We have
\begin{align}
    \mathbf{A}_{\perp,\perp}(\w) &=  \mathbb{E}_{\mathbf{u}}\left[  \mathbb{E}_{\mathbf{v}}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]  \mathbb{E}_{\mathbf{v}}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right] \nonumber \\
    &=  \mathbb{E}_{\mathbf{u}}\left[  \mathbb{E}_{\mathbf{z}}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{z})\mathbf{z} \right]  \mathbb{E}_{\mathbf{z}}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{z})\mathbf{z} \right]^\top  \right] \nonumber \\
    &\quad +  \mathbb{E}_{\mathbf{u}}\left[  \mathbb{E}_{\mathbf{v}}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right] \left(  \mathbb{E}_{\mathbf{v}}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right] -  \mathbb{E}_{\mathbf{z}}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{z})\mathbf{z} \right]\right)^\top  \right] \nonumber \\
    &\quad +  \mathbb{E}_{\mathbf{u}}\left[\left(  \mathbb{E}_{\mathbf{v}}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right] -  \mathbb{E}_{\mathbf{z}}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{z})\mathbf{z} \right]\right)  \mathbb{E}_{\mathbf{z}}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{z})\mathbf{z} \right] ^\top  \right] \nonumber \nonumber
\end{align}
For the second and third terms, we have
\begin{align}
    
\end{align}

% prefix issue: just define f(wperp). changing u doesn't change distribution of wpara times u so it doesnt change f(wperp)
things tried: 
- frob norm of matrix - then you get fourth sigmoid
- bounding the other vector (c(mu)) - this vector has norm 1
- making the error vector smaller than k**-3 - nope this is tight
- bounding product with w - error is ultimately the same
- bounding sum over u, then product with w.
- add and subtract one good one good prefix



% \begin{align}
%     &\left\|\mathbf{A}_{\perp,\perp} - \mathbf{A}^\circ_{\perp,\perp}\right\|_2 \nonumber\\
%     &= 2^{-r}\left\|2^{-r}\sum_{\mathbf{u} \in \mathcal{H}^r} \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]^\top   - \aaa\aaa^\top\right\|_2 \nonumber \\
%     &\leq 
%     % 2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}\left\|\left( 2^{-(k-r)}\sum_{\vv \in \mathcal{H}^{k-r}} \sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right)\left(2^{-(k-r)}\sum_{\vv \in \mathcal{H}^{k-r}} \sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right)^\top   - \aaa\aaa^\top\right\|_2 \nonumber \\
%     % &= 
%     2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}\left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]^\top   - \aaa\aaa^\top\right\|_2 \label{pre} \\
%     &= 2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}  \sup_{\y : \|\y\|_2=1} \left| \left\langle \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right], \y \right\rangle^2   - \left\langle\aaa,\y\right\rangle^2\right| \nonumber \\
%         &= 2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}  \sup_{\y : \|\y\|_2=1} \left|\left( \left\langle \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right], \y \right\rangle+\left\langle\aaa,\y\right\rangle \right)\left( \left\langle \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right], \y \right\rangle  - \left\langle\aaa,\y\right\rangle\right)\right| \nonumber \\
%         &\leq  2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}  \sup_{\y : \|\y\|_2=1} \left| \left\langle \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right], \y \right\rangle+\left\langle\aaa,\y\right\rangle \right|\sup_{\y' : \|\y'\|_2=1} \left| \left\langle \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right], \y' \right\rangle  - \left\langle\aaa,\y'\right\rangle\right| \nonumber \\ 
%         &=  2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}  \left\| \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]+\aaa \right\|_2 \left\|  \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]  - \aaa\right\|_2 \nonumber \\ 
%         &= 2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r} \left(\|\aaa\|_2 + \left\| \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]-\aaa \right\|_2\right) \left\|  \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]  - \aaa\right\|_2 \label{186} 
%     % &\leq 2^{-r}\max_{\mathbf{u} \in \mathcal{H}^r} \left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] + \aaa\right\|_2 \left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa\right\|_2 
% \end{align}
% &=  2^{-r} \sup_{\y : \|\y\|_2=1} | \langle \y, \aaa\rangle^2 - \langle \y, \bbb\rangle^2 |\nonumber \\
        % &=  2^{-r}\sup_{\y : \|\y\|_2=1} | (\langle \y, \aaa\rangle - \langle \y, \bbb\rangle)(\langle \y, \aaa\rangle + \langle \y, \bbb\rangle) |\nonumber \\
        % &\leq  2^{-r}\sup_{\y : \|\y\|_2=1} | \langle \y, \aaa\rangle - \langle \y, \bbb\rangle| \sup_{\y' : \|\y'\|_2=1}|\langle \y', \aaa\rangle + \langle \y, \bbb\rangle |\nonumber \\
% Thus we can upper bound $\left\|\mathbf{A}_{\perp,\perp} - \mathbf{A}^\circ_{\perp,\perp}\right\|_2 $ by upper bounding $\|\aaa\|_2$ and $\left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa\right\|_2$ for all $\uu \in \uH^r$. We start by controlling $\left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa\right\|_2$. We will upper bound $\|\aaa\|_2$ {\color{red}later}.   


    
\end{proof}




\begin{lemma}\label{lem:aparaperp}
    For all $j: \w_{0,j}\in \mathcal{G}_{w}$, we have 
    \begin{align}
        \|\mathbf{A}_{\parallel,\perp}(\mathbf{w}_{0,j}) - \|_2 &\leq 
    \end{align}
\end{lemma}

\begin{proof}
    
\end{proof}

\input{Proof_Rep2}





\begin{lemma}
    compute w1 for any neuron in the good set
    
    Consider any neuron $\mathbf{w}_{0,j} \in \mathcal{G}_{w}$ and omit the subscript $j$. Let $\w_{0,\parallel}\in \mathbb{R}^r$ denote the first $r$ elements of $\w_0$, and $\w_{0,\perp}\in \mathbb{R}^{k-r}$ denote the remaining $k-r$ elements, and likewise let $\w_{1,\parallel}\in \mathbb{R}^r$ and $\w_{0,\perp}\in \mathbb{R}^{k-r}$ denote the first $r$ and last $k-r$ elements of $\w_1$, respectively. Set $\eta = $ and $\lambda_2=$. 
    We have
    \begin{align}
        \w_{1,\parallel} &= \eta \w_{0,\parallel} + \nonumber \\
        \w_{1,\perp} &= \eta  \nonumber \\
    \end{align}
\end{lemma}

\begin{proof}
From Lemma \ref{lem:compute_grad},  we have 
\begin{align}
    % \mathbf{w}_{1} &= (1 - \eta \lambda)\mathbf{w}_0  + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{M} \mathbf{A}(\mathbf{w}_t)\mathbf{M}^\top \mathbf{w}_t \nonumber \\
    % \mathbf{M}_{:r}^\top \mathbf{w}_{t+1} &= (1 - \eta \lambda) \mathbf{M}_{:r}^\top\mathbf{w}_t  + \frac{\eta 2^{-r}}{\lambda_1}  \begin{bmatrix}
    %     \mathbf{I}_r & \mathbf{0}_{r,k-r} \\
    % \end{bmatrix} \mathbf{A}(\mathbf{w}_t)\mathbf{M}^\top \mathbf{w}_t  \nonumber \\
    % &= (1 - \eta \lambda) \mathbf{M}_{:r}^\top\mathbf{w}_t  + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\parallel,\parallel}(\mathbf{w}_t)\mathbf{M}_{:r}^\top \mathbf{w}_t + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\parallel,\perp}(\mathbf{w}_t)\mathbf{M}_{r:}^\top \mathbf{w}_t \nonumber \\
    % \mathbf{M}_{r:}^\top \mathbf{w}_{t+1} &= (1 - \eta \lambda) \mathbf{M}_{r:}^\top\mathbf{w}_t  + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\perp,\parallel}(\mathbf{w}_t)\mathbf{M}_{:r}^\top \mathbf{w}_t + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\perp,\perp}(\mathbf{w}_t)\mathbf{M}_{r:}^\top \mathbf{w}_t \nonumber \\
        \mathbf{w}_{1} &= (1 - \eta \lambda)\mathbf{w}_0  + \frac{\eta 2^{-r}}{\lambda_1}   \mathbf{A}(\mathbf{w}_0) \mathbf{w}_0 \nonumber 
\end{align}
For the first $r$ elements, since  $\mathbf{w}_{0} \in \mathcal{G}_{w}$ by Lemmas \ref{lem:apara} and \ref{lem:aparaperp} we have 
\begin{align}
    \mathbf{w}_{1,\parallel} &= (1 - \eta \lambda) \mathbf{w}_{0,\parallel}  + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\parallel,\parallel}(\mathbf{w}_0) \mathbf{w}_{0,\parallel} + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\parallel,\perp}(\mathbf{w}_0) \mathbf{w}_{0,\perp}  \nonumber \\
    &=  \nonumber \\
\end{align}
For the last $k-r$ elements, again using $\mathbf{w}_{0} \in \mathcal{G}_{w}$ by Lemmas \ref{lem:aperp} and \ref{lem:aparaperp} we have
\begin{align}
    \mathbf{w}_{1,\perp} &= (1 - \eta \lambda) \mathbf{w}_{1,\perp}  + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\perp,\parallel}(\mathbf{w}_{0})\mathbf{w}_{0,\parallel} + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\perp,\perp}(\mathbf{w}_0)\mathbf{w}_{0,\perp} \nonumber \\
    &= 
\end{align}




\end{proof}


\begin{lemma}
    compute b1, show it doesn't really change
\end{lemma}

\begin{proof}
    
\end{proof}

\begin{lemma}
    argue that now for any task, there exists a good head on top of the weights and biases that can get zero loss 
\end{lemma}

\begin{proof}
    
\end{proof}

\begin{lemma}
    apply result from shi et al showing that GD finds such a head? can play with how the updates for the head are computed. with infinite samples, gd is the same as min. 
    
    should need 2**r samples for finite? need to say that rep learning is better than random features.
\end{lemma}

\begin{proof}

with multitask trained features: information theoretically, for every bad neuron, need at least two samples with that neuron activated but different labels

with random features: should need Theta(exp(k)) neurons to guarantee 2r good ones
    
\end{proof}

We drop the subscript $0$ indicating time zero for ease of notation. We have 
\begin{align}
    &\mathbb{E}_{\mathbf{u}\sim \Unif(\mathcal{H}^{r})}\left[ \mathbb{E}_{\mathbf{v}\sim \Unif(\mathcal{H}^{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{z} )\right]^2 \mathbf{uu}^\top  \right] \nonumber \\
    &=  \mathbb{E}_{\mathbf{u}\sim \Unif(\mathcal{H}^{r})}\left[ \mathbb{E}_{\mathbf{z}\sim N(\mathbf{0}_{k-r},\mathbf{I}_{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2  \mathbf{uu}^\top  \right] \nonumber \\
    &\quad + \mathbb{E}_{\mathbf{u}\sim \Unif(\mathcal{H}^{r})}\left[ \left(\mathbb{E}_{\mathbf{v}\sim \Unif(\mathcal{H}^{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2 - \mathbb{E}_{\mathbf{z}\sim N(\mathbf{0}_{k-r},\mathbf{I}_{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{z} )\right]^2\right)  \mathbf{uu}^\top  \right] \nonumber 
\end{align}
Since each $\mathbf{uu}^\top$ is positive semi-definite, we have
\begin{align}
    &\left\|\mathbb{E}_{\mathbf{u}\sim \Unif(\mathcal{H}^{r})}\left[ \left(\mathbb{E}_{\mathbf{v}\sim \Unif(\mathcal{H}^{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2 - \mathbb{E}_{\mathbf{z}\sim N(\mathbf{0}_{k-r},\mathbf{I}_{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{z} )\right]^2\right)  \mathbf{uu}^\top  \right] \right\|_2 \nonumber \\
    &\leq \left\|\mathbb{E}_{\mathbf{u}\sim \Unif(\mathcal{H}^{r})}\left[ \left|\mathbb{E}_{\mathbf{v}\sim \Unif(\mathcal{H}^{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2 - \mathbb{E}_{\mathbf{z}\sim N(\mathbf{0}_{k-r},\mathbf{I}_{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{z} )\right]^2\right|  \mathbf{uu}^\top  \right] \right\|_2\label{prd} \\
    &\leq \left\|\mathbb{E}_{\mathbf{u}\sim \Unif(\mathcal{H}^{r})}\left[ b \mathbf{uu}^\top  \right] \right\|_2\nonumber \\
    &= b \nonumber 
\end{align}
where \eqref{prd} follows from Lemma \ref{lem:} and the fact that $\w\in \mathcal{G}_w$.
Next, 
\begin{align}
    &\mathbb{E}_{\mathbf{u}\sim \Unif(\mathcal{H}^{r})}\left[ \mathbb{E}_{\mathbf{z}\sim N(\mathbf{0}_{k-r},\mathbf{I}_{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2  \mathbf{uu}^\top  \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{u}\sim \Unif(\mathcal{H}^{r})}\left[ \mathbb{E}_{\mathbf{z}\sim N(\mathbf{0}_{k-r},\mathbf{I}_{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2  \mathbf{uu}^\top  \right] \nonumber \\
\end{align}

==> Proof_Lower.tex <==
\section{Lower Bound: GD in multitask setting with many simple tasks cannot learn good features.}

% Consider the following simple setting. There are two tasks. 
% Fix some column-orthonormal dictionary matrix $\mathbf{M}\in \mathbb{R}^{d \times k}$. The $j$-th sample for task $i$ is generated as:
% \begin{align}
%     \boldsymbol{\phi}_{i,j} \sim \mathcal{D}_k, \quad \mathbf{x}_{i,j} = \mathbf{M}\boldsymbol{\phi}_{i,j}, \quad y_{i,j} = g_i({\phi}_{i,j,1}, {\phi}_{i,j,2})
% \end{align}
% where $\mathcal{D}_k$ is the distribution over $\{0,1\}^k$ such that each element is drawn i.i.d. from Bern(0.5), and ${\phi}_{i,j,1}$ and ${\phi}_{i,j,2}$ are the first and second elements of $\boldsymbol{\phi}_{i,j}$, respectively. 
% % 
% The link function for task 1 is given by
% \begin{align}
%     g_1({\phi}_{i,j,1}, {\phi}_{i,j,2}) = \begin{cases}1 & {\phi}_{i,j,1} = 1 \\
%     -1 & {\phi}_{i,j,1} = 0 \\
%     \end{cases}
% \end{align}
% and the link function for task 2 is
% \begin{align}
%     g_2({\phi}_{i,j,1}, {\phi}_{i,j,2}) = \begin{cases}1 & {\phi}_{i,j,2} = 1 \\
%     -1 & {\phi}_{i,j,2} = 0 \\
%     \end{cases}
% \end{align}
% We ignore for now that these two tasks do not share important features (although, they do share $D-2$ spurious features). Our results should generalize to cases in which the tasks do share important features. 

Consider the following simple setting. There are two tasks. 
Fix some column-orthonormal dictionary matrix $\mathbf{M}\in \mathbb{R}^{d \times k}$. The $j$-th sample for task $i$ is generated as:
\begin{align}
    \boldsymbol{\phi}_{i,j} \sim \mathcal{D}_k, \quad \mathbf{x}_{i,j} = \mathbf{M}\boldsymbol{\phi}_{i,j}, \quad y_{i,j} = g_i({\phi}_{i,j,1}, {\phi}_{i,j,2})
\end{align}
where $\mathcal{D}_k$ is the distribution over $\{-1,1\}^k$ such that each element is an i.i.d. Rademacher random variable, and ${\phi}_{i,j,1}$ and ${\phi}_{i,j,2}$ are the first and second elements of $\boldsymbol{\phi}_{i,j}$, respectively. 
Note that this setting is equivalent to the setting considered in \cite{shi2022theoretical} where the $\phi_{i,j,\ell}$ are i.i.d. Bern(0.5) random variables but the data is normalized by subtracting the mean (and dividing by the standard deviation).

% 
The link function for task 1 is given by
\begin{align}
    g_1({\phi}_{i,j,1}, {\phi}_{i,j,2}) = \begin{cases}1 & {\phi}_{i,j,1} = 1 \\
    -1 & {\phi}_{i,j,1} = -1 \\
    \end{cases}
\end{align}
and the link function for task 2 is
\begin{align}
    g_2({\phi}_{i,j,1}, {\phi}_{i,j,2}) = \begin{cases}1 & {\phi}_{i,j,2} = 1 \\
    -1 & {\phi}_{i,j,2} = -1 \\
    \end{cases}
\end{align}
We ignore for now that these two tasks do not share important features (although, they do share $D-2$ spurious features). Our results should generalize to cases in which the tasks do share important features. 

Empirically, GD learns only the average while Local Heads and FedAvg learn the average and the difference.

% Proof sketch:

% % - Throughout: we anything that is true for task 1 must analogously be true for task 2. -- not true-depends on init W

% \begin{enumerate}
%     \item Show that GD converges to planted soln
    
%     \item 
% \end{enumerate}
% GD parameters: step size - must show GD fails for all step sizes.
max: the same samples will be chopped in both cases so it's fine

The gradient for neuron weight $\mathbf{w}_j$ is:
\begin{align}
 \nabla_{\mathbf{w}_j}\mathcal{L}(\mathbf{W},\mathbf{a})&=  \frac{a_j}{2}\bigg( \mathbb{E}[\chi\{ f(\mathbf{x}_1)<1\}\mathbf{x}_1\sigma'(\mathbf{w}_j^\top \mathbf{x}_1)|y_1 = 1]\mathbb{P}[y_1=1] \nonumber \\
 &\quad \quad \quad \quad - \mathbb{E}[\chi\{ f(\mathbf{x}_1)>-1\}\mathbf{x}_1\sigma'(\mathbf{w}_j^\top \mathbf{x}_1)|y_1 = -1]\mathbb{P}[y_1=-1]\bigg)\nonumber \\
 &\quad +  \frac{a_j}{2}\bigg(\mathbb{E}[\chi\{ f(\mathbf{x}_2)<1\}\mathbf{x}_2\sigma'(\mathbf{w}_j^\top \mathbf{x}_2)|y_2 = 1]\mathbb{P}[y_2=1] \nonumber \\
 &\quad \quad \quad \quad - \mathbb{E}[ \chi\{ f(\mathbf{x}_2)>-1 \} \mathbf{x}_2\sigma'(\mathbf{w}_j^\top \mathbf{x}_2)|y_2 = -1]\mathbb{P}[y_2 =-1]\bigg) \nonumber \\
 &\quad + \lambda \mathbf{w}_j
\end{align}
Consider first the term due to task 1. Let $\mathbf{z}= \sum_{\ell=2}^{k} \phi_\ell \mathbf{m}_{\ell}$. (need to remove mu's) We have 
\begin{align}
    &\mathbb{E}[\chi\{ f(\mathbf{x}_1)<1\} \mathbf{x}_1\sigma'(\mathbf{w}_j^\top \mathbf{x}_1)|y_1 = 1] \nonumber \\
    &= \mathbf{m}_1\mathbb{E}[\chi\{ f(\mathbf{x}_1)<1\} \sigma'(\mathbf{w}_j^\top (\mathbf{m}_1 + \mathbf{z}))] +  \mathbb{E}[\chi\{ f(\mathbf{x}_1)<1\} \mathbf{z}\sigma'(\mathbf{w}_j^\top (\mathbf{m}_1 + \mathbf{z}))] \\ 
    % - \boldsymbol{\mu}\mathbb{E}[\sigma'(\mathbf{w}_j^\top (\mathbf{m}_1 + \mathbf{z}- \boldsymbol{\mu}))]\\
    &= c_{1,1}\mathbf{m}_1 +  \mathbb{E}[\chi\{ f(\mathbf{x}_1)<1\}\mathbf{z}\sigma'(\mathbf{w}_j^\top (\mathbf{m}_1 + \mathbf{z}))] \\
    % - c^*\boldsymbol{\mu}\\ 
    &= c_{1,1}\mathbf{m}_1 +  \sum_{\ell=2}^k \mathbf{m}_\ell \mathbb{E}_{\phi_2,\dots,\phi_k}\left[\chi\{ f(\mathbf{x}_1)<1\}\phi_\ell\sigma'\left(\mathbf{w}_j^\top \mathbf{m}_1  + \sum_{\ell'=2}^k \phi_{\ell'} \mathbf{w}_j^\top \mathbf{m}_{\ell'}\right)\right]\\
    % -c^*\boldsymbol{\mu} \\ 
    &= c_{1,1} \mathbf{m}_1  + \frac{1}{2} \sum_{\ell=2}^k \mathbf{m}_\ell \Bigg(\mathbb{E}_{\phi_2,\dots,\phi_k}\left[\chi\{ f(\mathbf{x}_1)<1\} \sigma'\left(\mathbf{w}_j^\top \mathbf{m}_1  + \mathbf{w}_j^\top \mathbf{m}_{\ell}+  \sum_{\ell'=2,\ell'\neq \ell}^k \phi_{\ell'} \mathbf{w}_j^\top \mathbf{m}_{\ell'}\right)\right] \nonumber \\
    &\quad\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad -\mathbb{E}_{\phi_2,\dots,\phi_k}\left[\chi\{ f(\mathbf{x}_1)<1\}\sigma'\left(\mathbf{w}_j^\top \mathbf{m}_1  - \mathbf{w}_j^\top \mathbf{m}_{\ell}+  \sum_{\ell'=2,\ell'\neq \ell}^k \phi_{\ell'} \mathbf{w}_j^\top \mathbf{m}_{\ell'}\right)\right] \Bigg)  \\
    &= c_{1,1} \mathbf{m}_1 + \sum_{\ell=2}^k c_{1,\ell} \mathbf{m}_\ell
    % &= \frac{1}{2}c^*\mathbf{m}_1 + \frac{1}{2} \sum_{\ell=2}^k \mathbf{m}_\ell \left(\mathbb{E}_{\phi_2,\dots,\phi_k\setminus \phi_\ell}\left[\sigma'\left(0.5 \mathbf{w}_j^\top \mathbf{m}_1 + 0.5\mathbf{w}_j^\top \mathbf{m}_{\ell}+  \sum_{\ell'=2,\ell'\neq \ell}^k (\phi_{\ell'} - 0.5) \mathbf{w}_j^\top \mathbf{m}_{\ell'}\right)\right] - 1\right) \\ 
\end{align}
where % $c_{1,1} = \mathbb{E}[\sigma'(\mathbf{w}_j^\top (\mathbf{m}_1 + \mathbf{z}))]$, and
% Each of the terms in the sum from $\ell=2,\dots,k$ is small due to Berry-Esseen, but the sum is a constant... doesn't matter
for each $\ell = 2,...,k$, the coefficient of $\mathbf{m}_\ell$ is \begin{align}|c_{1,\ell}| &\coloneqq \bigg|\frac{1}{2}\mathbb{E}_{\phi_2,\dots,\phi_k}\bigg[\chi\{ f(\mathbf{x}_1)<1\}\sigma'\bigg(\mathbf{w}_j^\top \mathbf{m}_1  + \mathbf{w}_j^\top \mathbf{m}_{\ell}+  \sum_{\ell'=2,\ell'\neq \ell}^k \phi_{\ell'} \mathbf{w}_j^\top \mathbf{m}_{\ell'}\bigg)\bigg]\nonumber \\
&\quad -\frac{1}{2}\mathbb{E}_{\phi_2,\dots,\phi_k}\bigg[\chi\{ f(\mathbf{x}_1)<1\} \sigma'\bigg(\mathbf{w}_j^\top \mathbf{m}_1  - \mathbf{w}_j^\top \mathbf{m}_{\ell}+  \sum_{\ell'=2,\ell'\neq \ell}^k \phi_{\ell'} \mathbf{w}_j^\top \mathbf{m}_{\ell'}\bigg)\bigg]\bigg|  \nonumber \\
&= O(1/\sqrt{k})
\end{align}
by Berry-Esseen. (yes this still holds with max)
{\color{blue}
\begin{align}|c_{1,\ell}| &\coloneqq \frac{1}{2}\bigg|\mathbb{E}_{\mathbf{v}}\bigg[\sigma'\bigg({w}_1  + {w}_{\ell}+  \mathbf{v}^\top  \mathbf{w}_{-1,\ell}\bigg)\bigg] -\mathbb{E}_{\mathbf{v}}\bigg[\sigma'\bigg({w}_1  - {w}_{\ell}+  \mathbf{v}^\top  \mathbf{w}_{-1,\ell}\bigg)\bigg]\bigg|  \nonumber \\
&= O(1/\sqrt{k})
\end{align}
by Gaussian approximation and incoherence of $\w$.}
On the other hand,
% \begin{align}
%     &\mathbb{E}[(\mathbf{x}_1-\boldsymbol{\mu})\sigma'(\mathbf{w}_j^\top \mathbf{x}_1 )|y_1 = 1] \nonumber \\
%     &= \mathbf{m}_1\mathbb{E}[\sigma'(\mathbf{w}_j^\top (\mathbf{m}_1 + \mathbf{z} ))] +  \mathbb{E}[\mathbf{z}\sigma'(\mathbf{w}_j^\top (\mathbf{m}_1 + \mathbf{z}))] \nonumber \\
%     &= c^*\mathbf{m}_1 +  \mathbb{E}[\mathbf{z}\sigma'(\mathbf{w}_j^\top (\mathbf{m}_1 + \mathbf{z}))] \\ 
%     &= c^*\mathbf{m}_1 +  \sum_{\ell=2}^k \mathbf{m}_\ell \mathbb{E}_{\phi_2,\dots,\phi_k}\left[\phi_\ell\sigma'\left(\mathbf{w}_j^\top \mathbf{m}_1 + \sum_{\ell'=2}^k \phi_{\ell'} \mathbf{w}_j^\top \mathbf{m}_{\ell'}\right)\right]  \\ 
%     &= c^*\mathbf{m}_1 + \frac{1}{2} \sum_{\ell=2}^k \mathbf{m}_\ell \mathbb{E}_{\phi_2,\dots,\phi_k}\left[\sigma'\left(\mathbf{w}_j^\top \mathbf{m}_1  + \mathbf{w}_j^\top \mathbf{m}_{\ell}+  \sum_{\ell'=2,\ell'\neq \ell}^k \phi_{\ell'} \mathbf{w}_j^\top \mathbf{m}_{\ell'}\right)\right] \\ 
% \end{align}
\begin{align}
    c_{1,1} &= \mathbb{E}\left[\chi\{ f(\mathbf{x}_1)<1\} \sigma'\left(\mathbf{w}_j^\top \mathbf{m}_1 
    % - \mathbf{w}_j^\top \boldsymbol{\mu} 
    + \sum_{\ell'=2}^k \phi_{\ell'} \mathbf{w}_j^\top \mathbf{m}_{\ell'}\right)\right] = \mathbb{P}\left[ f(\mathbf{x}_1)<1 \cap \mathbf{w}_j^\top \mathbf{m}_1 + \sum_{\ell'=2}^k \phi_{\ell'}  \mathbf{w}_j^\top \mathbf{m}_{\ell'} > 0\right]  \geq 1/2
    % &\geq  \mathbb{P}\left[ \sum_{\ell'=2}^k \phi_{\ell'}  \mathbf{w}_j^\top \mathbf{m}_{\ell'} > O()\right]
\end{align}
% where $c^* = \mathbb{E}\left[\sigma'\left(\mathbf{w}_j^\top \mathbf{m}_1 + \sum_{\ell'=2}^k \phi_{\ell'} \mathbf{w}_j^\top \mathbf{m}_{\ell'}\right)\right]$
% if $\mathbf{w}_j^\top \mathbf{m}_1 >0$, then $c^* \geq 0.5$. 
at initialization.
% On initialization, the inner product may be negative, but sum should have variance $\Omega(k)$ larger. So we should be fine.
% \begin{align}
% & \mathbb{E}_{\phi_2,\dots,\phi_k}\left[\sigma'\left(\mathbf{w}_j^\top \mathbf{m}_1  + \mathbf{w}_j^\top \mathbf{m}_{\ell}+  \sum_{\ell'=2,\ell'\neq \ell}^k \phi_{\ell'} \mathbf{w}_j^\top \mathbf{m}_{\ell'}\right)\right] 
% \end{align}
% which is similar to $c*$.
Similarly, 
\begin{align}
    &\mathbb{E}[\mathbf{x}_1\sigma'(\mathbf{w}_j^\top \mathbf{x}_1)|y_1 = -1] \nonumber \\
      &= -\mathbf{m}_1\mathbb{E}[\sigma'(-\mathbf{w}_j^\top \mathbf{m}_1 + \mathbf{w}_j^\top \mathbf{z})] +  \mathbb{E}[\mathbf{z}\sigma'(-\mathbf{w}_j^\top \mathbf{m}_1 + \mathbf{w}_j^\top \mathbf{z})] \\ 
    % - \boldsymbol{\mu}\mathbb{E}[\sigma'(\mathbf{w}_j^\top (\mathbf{m}_1 + \mathbf{z}- \boldsymbol{\mu}))]\\
    &= -c_{1,1}'\mathbf{m}_1 +  \mathbb{E}[\mathbf{z}\sigma'(-\mathbf{w}_j^\top \mathbf{m}_1 + \mathbf{w}_j^\top \mathbf{z}))] \\
    % - c^*\boldsymbol{\mu}\\ 
    &= -c_{1,1}'\mathbf{m}_1 +  \sum_{\ell=2}^k \mathbf{m}_\ell \mathbb{E}_{\phi_2,\dots,\phi_k}\left[\phi_\ell\sigma'\left(-\mathbf{w}_j^\top \mathbf{m}_1  + \sum_{\ell'=2}^k \phi_{\ell'} \mathbf{w}_j^\top \mathbf{m}_{\ell'}\right)\right]\\
    % -c^*\boldsymbol{\mu} \\ 
    &= -c_{1,1}' \mathbf{m}_1  + \frac{1}{2} \sum_{\ell=2}^k \mathbf{m}_\ell \Bigg(\mathbb{E}_{\phi_2,\dots,\phi_k}\left[\sigma'\left(-\mathbf{w}_j^\top \mathbf{m}_1  + \mathbf{w}_j^\top \mathbf{m}_{\ell}+  \sum_{\ell'=2,\ell'\neq \ell}^k \phi_{\ell'} \mathbf{w}_j^\top \mathbf{m}_{\ell'}\right)\right] \nonumber \\
    &\quad\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad -\mathbb{E}_{\phi_2,\dots,\phi_k}\left[\sigma'\left(-\mathbf{w}_j^\top \mathbf{m}_1 - \mathbf{w}_j^\top \mathbf{m}_{\ell}+  \sum_{\ell'=2,\ell'\neq \ell}^k \phi_{\ell'} \mathbf{w}_j^\top \mathbf{m}_{\ell'}\right)\right] \Bigg) \\
    &= -c_{1,1}' \mathbf{m}_1  + \sum_{\ell=2}^k c_{1,\ell}' \mathbf{m}_\ell %\\
    % &= \mathbb{E}[\mathbf{z}\sigma'(\mathbf{w}_j^\top  \mathbf{z})]  \\
    % &=  \mathbb{E}[\mathbf{z}\sigma'(\mathbf{w}_j^\top \mathbf{z})] \\ 
    % &= -\frac{1}{2}c'\mathbf{m}_1 + \frac{1}{2} \sum_{\ell=2}^k \mathbf{m}_\ell \left(\mathbb{E}_{\phi_2,\dots,\phi_k\setminus \phi_\ell}\left[\sigma'\left(\mathbf{w}_j^\top \mathbf{m}_1 + \mathbf{w}_j^\top \mathbf{m}_{\ell}+  \sum_{\ell'=2,\ell'\neq \ell}^k \phi_{\ell'} \mathbf{w}_j^\top \mathbf{m}_{\ell'}\right)\right] - c'\right) \\ 
\end{align}
where $c_{1,1}' \geq 1/2$ and $|c_{1,\ell}'| = O(1/\sqrt{k})$. 
\begin{align}
   &\mathbb{E}[\mathbf{x}_1\sigma'(\mathbf{w}_j^\top \mathbf{x}_1)|y_1 = 1] - \mathbb{E}[\mathbf{x}_1\sigma'(\mathbf{w}_j^\top \mathbf{x}_1)|y_1 = -1] \nonumber \\
   &= (c_{1,1} + c_{1,1}') \mathbf{m}_1 + \sum_{\ell=2}^k (c_{1,\ell} - c_{1,\ell}')\mathbf{m}_\ell 
\end{align}
By symmetry, the same argument holds for the terms in the gradient from task 2.
Now we have
% Thus we have
\begin{align}
    \nabla_{\mathbf{w}_j}\mathcal{L}(\mathbf{W},\mathbf{a}) &= \frac{a_j}{2}(c_{1,1} + c_{1,1}' + c_{2,1} - c_{2,1}') \mathbf{m}_1 + \frac{a_j}{2}(c_{1,2} - c_{1,2}' + c_{2,2} + c_{2,2}') \mathbf{m}_2 + \frac{a_j}{2}\sum_{\ell=3}^k (c_{1,\ell} - c_{1,\ell}' + c_{2,\ell} - c_{2,\ell}') \mathbf{m}_\ell  
\end{align}
where 
\begin{align}
    c_{1,1} + c_{1,1}' + c_{2,1} - c_{2,1}' &\geq 1 - O(1/k) \nonumber \\
    c_{1,2} - c_{1,2}' + c_{2,2} + c_{2,2}' &\geq 1 - O(1/k) \nonumber \\
    |c_{1,\ell} - c_{1,\ell}' + c_{2,\ell} - c_{2,\ell}'| &= O(1/k) \quad \forall \ell = 3,\dots,k
\end{align}

The update for $\mathbf{a}_1$ is:
\begin{align}
    \mathbf{a}_1 &= \mathbf{a}_0 - \frac{\alpha}{2} \left( -\mathbb{E}_{\mathbf{x}_1}\left[y_1\sigma\left(\mathbf{W}_0 \mathbf{x}_1\right)\right] - \mathbb{E}_{\mathbf{x}_2}\left[y_2\sigma\left(\mathbf{W}_0 \mathbf{x}_2\right)\right] + 2 \lambda \mathbf{a}_0 \right) \nonumber \\
    &= (1 - \alpha \lambda)\mathbf{a}_0 + \frac{\alpha}{2}  \mathbb{E}_{\mathbf{x}}\left[(y_1+y_2)\sigma\left(\mathbf{W}_0 \mathbf{x}\right)\right]  \nonumber \\
    &= (1 - \alpha \lambda)\mathbf{a}_0 + \frac{\alpha}{8}  \left(2\mathbb{E}_{\mathbf{x}}\left[\sigma\left(\mathbf{W}_0 \mathbf{x}\right) |y_1+y_2 = 2 \right] - 2\mathbb{E}_{\mathbf{x}}\left[\sigma\left(\mathbf{W}_0 \mathbf{x}\right) |y_1+y_2 = -2 \right] \right)\nonumber \\
    &= (1 - \alpha \lambda)\mathbf{a}_0 + \frac{\alpha}{4}  \mathbb{E}_{\mathbf{z}}\left[\sigma\left(\mathbf{W}_0 \mathbf{m}_1 + \mathbf{W}_0 \mathbf{m}_2 + \mathbf{W}_0 \mathbf{z}\right) \right]\nonumber \\
    &\quad \quad - \frac{\alpha}{4}  \mathbb{E}_{\mathbf{z}}\left[\sigma\left(-\mathbf{W}_0 \mathbf{m}_1 - \mathbf{W}_0 \mathbf{m}_2 + \mathbf{W}_0 \mathbf{z}\right)  \right]
    % &= (1 - \alpha \lambda)\mathbf{a}_0 + \frac{\alpha}{4} \big[ \mathbb{P}(\sigma (\mathbf{w}_j^\top \mathbf{z}))\big]_{j=1,\dots,m}
\end{align}

{\color{blue}

\begin{align}
    c_{1,1} + c_{1,1}' &= \mathbb{E}\left[\chi\{ f(\mathbf{x}_1)<1\}\sigma'\left({w}_1 
    + \mathbf{v}^\top \mathbf{w}_{-1}\right)\right] + \mathbb{E}\left[\chi\{ f(\mathbf{x}_1)>-1\}\sigma'\left(-{w}_1 
    + \mathbf{v}^\top \mathbf{w}_{-1}\right)\right] \nonumber \\
    &= 2\mathbb{E}\left[\chi\{ v_1 f(\mathbf{x})<1\}\sigma'\left(
    \mathbf{v}^\top \mathbf{w}\right)\right] \nonumber 
 %    &= 2 \mathbb{E}\left[\sigma'\left(
 %     \mathbf{v}^\top \mathbf{w}_{}\right)\right]\nonumber \\
 % &= 1
\end{align}
and 
\begin{align}
    c_{2,2} + c_{2,2}' &= 
    % \mathbb{E}\left[\chi\{ f(\mathbf{x}_2)<1\}\sigma'\left({w}_1 
    % + \mathbf{v}^\top \mathbf{w}_{-1}\right)\right] + \mathbb{E}\left[\chi\{ f(\mathbf{x}_1)>-1\}\sigma'\left(-{w}_1 
    % + \mathbf{v}^\top \mathbf{w}_{-1}\right)\right] \nonumber \\
     2\mathbb{E}\left[\chi\{ v_2 f(\mathbf{x})<1\}\sigma'\left(
     \mathbf{v}^\top \mathbf{w}\right)\right] \nonumber 
 %    &= 2 \mathbb{E}\left[\sigma'\left(
 %     \mathbf{v}^\top \mathbf{w}_{}\right)\right]\nonumber \\
 % &= 1
\end{align}
Also,
\begin{align}
    &c_{1,2} - c_{1,2}' \nonumber \\ 
    &= \frac{1}{2}\mathbb{E}_{\mathbf{v}}\bigg[\chi\{ f(\mathbf{x}_1)<1\}\sigma'\bigg({w}_1  + {w}_{2}+  \mathbf{v}^\top  \mathbf{w}_{-1,2}\bigg)\bigg] -\frac{1}{2}\mathbb{E}_{\mathbf{v}}\bigg[\chi\{ f(\mathbf{x}_1)<1\}\sigma'\bigg({w}_1  - {w}_{2}+  \mathbf{v}^\top  \mathbf{w}_{-1,2}\bigg)\bigg] \nonumber \\
    &\quad - \frac{1}{2}\mathbb{E}_{\mathbf{v}}\bigg[\chi\{ f(\mathbf{x}_1)>-1\}\sigma'\bigg(-{w}_1  + {w}_{2}+  \mathbf{v}^\top  \mathbf{w}_{-1,2}\bigg)\bigg] + \frac{1}{2}\mathbb{E}_{\mathbf{v}}\bigg[\chi\{ f(\mathbf{x}_1)>-1\}\sigma'\bigg(-{w}_1  - {w}_{2}+  \mathbf{v}^\top  \mathbf{w}_{-1,2}\bigg)\bigg] \nonumber \\
    &= \mathbb{E}_{\mathbf{v}}\bigg[\chi\{ f(\mathbf{x}_1)<1\} v_1\sigma'\bigg(v_1 {w}_1  + {w}_{2}+  \mathbf{v}^\top  \mathbf{w}_{-1,2}\bigg)\bigg] -\mathbb{E}_{\mathbf{v}}\bigg[\chi\{ f(\mathbf{x}_1)>-1\}v_1 \sigma'\bigg(v_1 {w}_1  - {w}_{2}+  \mathbf{v}^\top  \mathbf{w}_{-1,2}\bigg)\bigg] \nonumber \\
    &= \mathbb{E}_{\mathbf{v}}\bigg[\chi\{ v_2f(\mathbf{x}_1)<1\}v_1v_2 \sigma'\bigg(\mathbf{v}^\top  \mathbf{w}\bigg)\bigg]
\end{align}
and
\begin{align}
    &c_{2,1} - c_{2,1}' 
    % &= \frac{1}{2}\mathbb{E}_{\mathbf{v}}\bigg[\chi\{ f(\mathbf{x}_1)<1\}\sigma'\bigg({w}_1  + {w}_{2}+  \mathbf{v}^\top  \mathbf{w}_{-1,2}\bigg)\bigg] -\frac{1}{2}\mathbb{E}_{\mathbf{v}}\bigg[\chi\{ f(\mathbf{x}_1)>-1\}\sigma'\bigg({w}_1  - {w}_{2}+  \mathbf{v}^\top  \mathbf{w}_{-1,2}\bigg)\bigg] \nonumber \\
    % &\quad - \frac{1}{2}\mathbb{E}_{\mathbf{v}}\bigg[\chi\{ f(\mathbf{x}_1)<1\}\sigma'\bigg(-{w}_1  + {w}_{2}+  \mathbf{v}^\top  \mathbf{w}_{-1,2}\bigg)\bigg] + \frac{1}{2}\mathbb{E}_{\mathbf{v}}\bigg[\chi\{ f(\mathbf{x}_1)>-1\}\sigma'\bigg(-{w}_1  - {w}_{2}+  \mathbf{v}^\top  \mathbf{w}_{-1,2}\bigg)\bigg] \nonumber \\
    % &= \mathbb{E}_{\mathbf{v}}\bigg[\chi\{ f(\mathbf{x}_1)<1\} v_1\sigma'\bigg(v_1 {w}_1  + {w}_{2}+  \mathbf{v}^\top  \mathbf{w}_{-1,2}\bigg)\bigg] -\mathbb{E}_{\mathbf{v}}\bigg[\chi\{ f(\mathbf{x}_1)>-1\}v_1 \sigma'\bigg(v_1 {w}_1  - {w}_{2}+  \mathbf{v}^\top  \mathbf{w}_{-1,2}\bigg)\bigg] \nonumber \\
    = \mathbb{E}_{\mathbf{v}}\bigg[\chi\{ v_1f(\mathbf{x}_1)<1\}v_1v_2 \sigma'\bigg(\mathbf{v}^\top  \mathbf{w}\bigg)\bigg]
\end{align}




and 
\begin{align}
    c_{1,\ell} - c_{1,\ell}' + c_{2,\ell} - c_{2,\ell}' &= \mathbb{E}_{\mathbf{v}}\bigg[(v_1+v_2) v_\ell \sigma'\bigg(  \mathbf{v}^\top  \mathbf{w}_{}\bigg)\bigg] 
\end{align}
Then 
\begin{align}
    \nabla_{\mathbf{w}_j}\mathcal{L}(\mathbf{W},\mathbf{a}) &= \frac{a_j}{2}\mathbb{E}_{\mathbf{v}}[\chi\{ v_1f(\mathbf{x})<1\}( 1 + v_1v_2) \sigma'(\mathbf{v}^\top  \mathbf{w})] \mathbf{e}_1+\frac{a_j}{2}\mathbb{E}_{\mathbf{v}}[\chi\{ v_2f(\mathbf{x})<1\}( 1 + v_1v_2) \sigma'(\mathbf{v}^\top  \mathbf{w})] \mathbf{e}_2 \nonumber \\
    % v_1v_2 \sigma'(\mathbf{v}^\top  \mathbf{w})]) (\mathbf{e}_1 +\mathbf{e}_2) \nonumber \\
    &\quad + \frac{a_j}{2}\sum_{\ell=3}^k \mathbb{E}_{\mathbf{v}}[(v_1+v_2) v_\ell \sigma'(  \mathbf{v}^\top  \mathbf{w}_{})] \mathbf{e}_\ell   \nonumber \\
    &=  {a_j}\mathbb{E}_{\mathbf{v}}[\chi\{ f(\mathbf{x})<1, v_1=v_2\}\sigma'(\mathbf{v}^\top  \mathbf{w})] (\mathbf{e}_1+\mathbf{e}_2) + \frac{a_j}{2}\sum_{\ell=3}^k \mathbb{E}_{\mathbf{v}}[(v_1+v_2) v_\ell \sigma'(  \mathbf{v}^\top  \mathbf{w}_{})] \mathbf{e}_\ell 
\end{align}
% {\color{red} (plus regularization) can have stationary point at e1 or e2.

% relevant cases are when v1 = v2. 

% say v1 = 1 and f(w1 + w2 + junk) > 1
% }

------

error is:
\begin{align}
    \frac{a_j}{2}\mathbb{E}_{\mathbf{v}}[(\chi\{ v_2f(\mathbf{x})<1\} - \chi\{ v_1f(\mathbf{x})<1\})( 1 + v_1v_2) \sigma'(\mathbf{v}^\top  \mathbf{w})] \mathbf{e}_2 
\end{align}
if w1 is large then v1 f1 is likely to be too large whenever v1 is 1. so that coefficient may be near zero all the time..second coefficient will contain only v1=v2=1 terms.
If w is proportional to the ones vector then there is no issue (coeffs are the same)
but in other basis it must have same projection on all directions.
cannot initialize like this. need to say that...large params cause some other issue





note that there exists a good solution to this problem in the multitask case
may be able to adopt shi analysis directly, slight change in params


thus the gradient only depends on $\mathbf{e}_1, \mathbf{e}_2$ through $\mathbf{e}_1 + \mathbf{e}_2$ (this would also hold for more general features).

For $a_{1,j}$:
\begin{align}
    {a}_{1,j} 
    &= (1 - \alpha \lambda){a}_{0,j} + \frac{\alpha}{4}  \mathbb{E}_{\mathbf{z}}\left[\sigma\left({w}_{0,j,1}  + {w}_{0,j,2}  + \mathbf{v}^\top \mathbf{w}_{0,j,-1,2}\right) \right]\nonumber \\
    &\quad \quad - \frac{\alpha}{4}  \mathbb{E}_{\mathbf{z}}\left[\sigma\left(-{w}_{0,j,1}  - {w}_{0,j,2}  + \mathbf{v}^\top \mathbf{w}_{0,j,-1,2}\right)  \right] \nonumber \\
    &= (1 - \alpha \lambda){a}_{0,j} + \frac{\alpha}{2}  \mathbb{E}_{\mathbf{v}}\left[v\sigma\left(v({w}_{0,j,1}  + {w}_{0,j,2})  + \mathbf{v}^\top \mathbf{w}_{0,j,-1,2}\right) \right]
    % &= (1 - \alpha \lambda)\mathbf{a}_0 + \frac{\alpha}{4} \big[ \mathbb{P}(\sigma (\mathbf{w}_j^\top \mathbf{z}))\big]_{j=1,\dots,m}
\end{align}

can show contraction of perp part on first step due to regularization, move towards e1+e2. aj fixes sign alignment.on subsequent steps, gradient always only depends on sum so this immediately implies... but initialization could cause it to go to one or the other... but then no stationary point... what is the stationary points... yes the only? stationary point is e1 + e2 times a constant (with regularization) and likewise for a. 

yes only. because gradient for w has components on e1+e2, e3, e4, etc. So if gradient is zero (including regularization), w has to be some linear combination of  e1+e2, e3, e4, etc.

and for a, c(e1+e2) is a stationary point. done.
}

Let $\mathbf{x} = \mathbf{Mv}$. Let $\mathbf{M}=\mathbf{I}_d$. 

The gradient for neuron weight $\mathbf{w}_j$ is:
\begin{align}
 \nabla_{\mathbf{w}_j}\mathcal{L}(\mathbf{W},\mathbf{b},\mathbf{a})&=  \frac{a_j}{2}\bigg( \mathbb{E}[\chi\{ f(\mathbf{v})<1\}\mathbf{v}\sigma'(\mathbf{w}_j^\top \mathbf{v})|f_1^*(\mathbf{v})=1]\mathbb{P}[f_1^*(\mathbf{v})=1] \nonumber \\
 &\quad \quad \quad \quad - \mathbb{E}[\chi\{ f(\mathbf{v})>-1\}\mathbf{v}\sigma'(\mathbf{w}_j^\top \mathbf{v})|f_1^*(\mathbf{v})=-1]\mathbb{P}[y_1=-1]\bigg)\nonumber \\
 &\quad +  \frac{a_j}{2}\bigg(\mathbb{E}[\chi\{ f(\mathbf{v})<1\}\mathbf{v}\sigma'(\mathbf{w}_j^\top \mathbf{v})|f_2^*(\mathbf{v})=-1]\mathbb{P}[f_2^*(\mathbf{v})=-1] \nonumber \\
 &\quad \quad \quad \quad - \mathbb{E}[ \chi\{ f(\mathbf{v})>-1 \} \mathbf{v}\sigma'(\mathbf{w}_j^\top \mathbf{v})|f_2^*(\mathbf{v})=-1]\mathbb{P}[f_2^*(\mathbf{v})=-1]\bigg) \nonumber \\
 &\quad + \lambda \mathbf{w}_j \nonumber \\
 &= [\alpha_{\ell,1}]_\ell + [\alpha_{\ell,2}]_\ell + \lambda \mathbf{w}_j
\end{align}

For task 1, the first coordinate is (dropping $j$ subscript):
\begin{align}
    \alpha_{1,1} &\coloneqq  \frac{a_j}{2}\bigg( \mathbb{E}[\chi\{ f(\mathbf{v})<1\}v_1\sigma'(\mathbf{w}^\top \mathbf{v})|f_1^*(\mathbf{v})=1]\mathbb{P}[f_1^*(\mathbf{v})=1] \nonumber \\
 &\quad \quad \quad \quad - \mathbb{E}[\chi\{ f(\mathbf{v})>-1\}v_1\sigma'(\mathbf{w}^\top \mathbf{v})|f_1^*(\mathbf{v})=-1]\mathbb{P}[f_1^*(\mathbf{v})=-1]\bigg)\nonumber \\
 &=  \frac{a_j}{4}\bigg( \mathbb{E}[\chi\{f(\mathbf{v},v_1=1)<1\}\sigma'(w_1 + \mathbf{w}_{2:}^\top \mathbf{v}_{2:}+ b_j)]\nonumber \\
 &\quad \quad \quad \quad + \mathbb{E}[\chi\{ f(\mathbf{v},v_1=-1)>-1\}\sigma'(-w_1 + \mathbf{w}_{2:}^\top \mathbf{v}_{2:} + b_j)]\bigg)\nonumber \\
 &= \frac{a_j}{2} \mathbb{E}[\chi\{ v_1f(\mathbf{v})<1\}\sigma'(\mathbf{w}^\top \mathbf{v}+ b_j)]\nonumber 
\end{align}
While the first coordinate for task two is:
\begin{align}
    \alpha_{1,2} &\coloneqq \frac{a_j}{2}\bigg(\mathbb{E}[\chi\{ f(\mathbf{v})<1\}{v}_1\sigma'(\mathbf{w}_j^\top \mathbf{v} + b_j)|f_2^*(\mathbf{v})=-1]\mathbb{P}[f_2^*(\mathbf{v})=-1] \nonumber \\
 &\quad \quad \quad \quad - \mathbb{E}[ \chi\{ f(\mathbf{v})>-1 \} {v}_1\sigma'(\mathbf{w}_j^\top \mathbf{v} + b_j)|f_2^*(\mathbf{v})=-1]\mathbb{P}[f_2^*(\mathbf{v})=-1]\bigg) \nonumber \\
 &=  \frac{a_j}{4}\bigg(\mathbb{E}[\chi\{ f(\mathbf{v},v_2=1)<1\}{v}_1\sigma'(w_2 + \mathbf{w}_{j,-2}^\top \mathbf{v}_{j,-2} + b_j)] \nonumber \\
 &\quad \quad \quad \quad - \mathbb{E}[ \chi\{ f(\mathbf{v},v_2=-1)>-1 \} v_1 \sigma'( -w_2 +  \mathbf{w}_{j,-2}^\top \mathbf{v}_{-2} + b_j)]\bigg) \nonumber \\
 &= \frac{a_j}{2} \mathbb{E}[\chi\{ v_2f(\mathbf{v})<1\}v_1 v_2 \sigma'(\mathbf{w}^\top \mathbf{v}+ b_j)]\nonumber 
\end{align}

So the sum of these is:
\begin{align}
    g_1 &\coloneqq  \alpha_{1,1} +  \alpha_{1,2} \nonumber \\
    &= \frac{a_j}{2} \mathbb{E}[\left(\chi\{ v_1f(\mathbf{v})<1\} + \chi\{ v_2f(\mathbf{v})<1\}v_1 v_2 \right)\sigma'(\mathbf{w}^\top \mathbf{v}+ b_j)]\nonumber
\end{align}
For coordinate 2, we have by symmetry
\begin{align}
    g_2 &\coloneqq  \alpha_{2,1} +  \alpha_{2,2} \nonumber \\
    &= \frac{a_j}{2} \mathbb{E}[\left(\chi\{ v_2f(\mathbf{v})<1\} + \chi\{ v_1 f(\mathbf{v})<1\}v_1 v_2 \right)\sigma'(\mathbf{w}^\top \mathbf{v}+ b_j)]\nonumber
\end{align}


If $v_1 = v_2 = 1$, then $g_1 = g_2$.
If $v_1 = v_2 = -1$, then $g_1 = g_2$.
If $v_1 =1,  v_2 = -1$, then $g_1 = \frac{a_j}{2} \mathbb{E}[\left(\chi\{ f(\mathbf{v})<1\} - \chi\{ f(\mathbf{v})>-1\}\right)\sigma'(\mathbf{w}^\top \mathbf{v}+ b_j)] = - g_2$ .


% Let $q_{t,j,\ell}\coloneqq \langle \mathbf{w}_{t,j}^\top, \mathbf{m}_\ell \rangle$. We have 
% \begin{align}
%     |q_{1,j,1}| &\geq |q_{0,j,1}|(1 - \lambda) + \frac{\alpha |a_{0,j}|}{2} (1 - O(1/\sqrt{k})) \nonumber \\
%     |q_{1,j,2}| &\geq |q_{0,j,2}|(1 - \lambda) + \frac{\alpha |a_{0,j}|}{2} (1 - O(1/\sqrt{k})) \nonumber \\
%     |q_{1,j,\ell}| &\leq |q_{0,j,\ell}|(1 - \lambda) + \frac{\alpha |a_{0,j}|}{2}  O(1/\sqrt{k}) \quad \forall \ell = 3,\dots,k
%     \nonumber 
% \end{align}

% Each coordinate of $\mathbf{a}$ can flip sign on the first round, but if it does so, then it must have previously been small, which means the corresponding neuron did not change much from its initialization. Once the magnitude of the coordinate and the neurons becomes large, the coordinate does not flip sign. Note $a_j$ will be negative for ${w}_{j,1},w_{j,2}\rightarrow(-1,-1)$ and positive for ${w}_{j,1},w_{j,2}\rightarrow(1,1)$
% Now on round 2,
% \begin{align}
%     \mathbf{w}_{2,j}
% \end{align}

% Show that either $(q_{t,j,1},q_{t,j,2})$ goes to quadrant 1 or quadrant 3 depending on the sign of $a_{t,j}$. Need to show that the sign of $a_{t,j}$
% does not change.


% -------
% \begin{align}
%     \nabla &= \frac{1}{2}(c^* + c')\mathbf{m}_1 \nonumber \\
%     &\quad + \frac{1}{2} \sum_{\ell=2}^k \mathbf{m}_\ell \Bigg(\mathbb{E}_{\phi_2,\dots,\phi_k\setminus \phi_\ell}\left[\sigma'\left(0.5 \mathbf{w}_j^\top \mathbf{m}_1 + 0.5\mathbf{w}_j^\top \mathbf{m}_{\ell}+  \sum_{\ell'=2,\ell'\neq \ell}^k (\phi_{\ell'} - 0.5) \mathbf{w}_j^\top \mathbf{m}_{\ell'}\right)\right] \nonumber \\
%     &\quad - \mathbb{E}_{\phi_2,\dots,\phi_k\setminus \phi_\ell}\left[\sigma'\left(-0.5 \mathbf{w}_j^\top \mathbf{m}_1 + 0.5\mathbf{w}_j^\top \mathbf{m}_{\ell}+  \sum_{\ell'=2,\ell'\neq \ell}^k (\phi_{\ell'} - 0.5) \mathbf{w}_j^\top \mathbf{m}_{\ell'}\right)\right] + c'-c^* \Bigg) 
% \end{align}
% we want coeff of ml to be zero. at init, each prob is roughly 1/2, so sum is zero. 
% when wj approx m1 + m2 and ell = 2. then first term is 1, -second term is -0.5 , c'-c* is 0.5(0.5 - 1) + 0.5(0 - 0.5) -- thus sum = 1 - 0.5 + 0.5(0.5 - 1) + 0.5(0 - 0.5) = 0
% when ell neq 2, again c'-c* is 0.5(0.5 - 1) + 0.5(0 - 0.5) = -0.5. first term is 0.5(0.5 + 1), -second term is -0.5(0+0.5) -- sum first two terms is 0.5 as desired.

% and 
% \begin{align}
%     c^* + c' &= \mathbb{P}\left[  \sum_{\ell'=2}^k (\phi_{\ell'} - 0.5) \mathbf{w}_j^\top \mathbf{m}_{\ell'} > -0.5 \mathbf{w}_j^\top \mathbf{m}_1\right] + \mathbb{P}\left[ \sum_{\ell'=2}^k (\phi_{\ell'} - 0.5) \mathbf{w}_j^\top \mathbf{m}_{\ell'} > 0.5 \mathbf{w}_j^\top \mathbf{m}_1\right] %\\
%     % &= 
% \end{align}
% we want sum to be 1
% initially: reduces to sum of k-1 gaussians being larger than one gaussian - each probability is roughly 1/2
% later: when wj is mostly m1 + m2 the 
% % term with negative on 
% RHS is 1 whp: if phi2 is 1, then sum of conditional probs is 1+0.5. if phi2 is 0, then sum is 0.5+0. 0.5*(1.5)+0.5*0.5 = 1.


% Proof will be: GD with no regularization diverges, and GD with regularization converges linearly to average.

% The crux here is that the gradient loses dependence on wj. Meaning it lies in a single line regardless of wj. So all neurons go to that line (can we show this holds more generally? no because lack of symmetry). In the standard model, even with symmetry, the gradients depended on wj, due to isotropic data?, so we had diversity.

% empirically: even if w1 starts close to m1, it will move in the direction m1+m2...roughly



==> Proof_Rep2.tex <==


\begin{lemma} \label{lem:final}
 % Let $\mathbf{w}_{1,0},\dots,\mathbf{w}_{m,0}$ denote the initial neuron weights.   
    % Let $\w_{0,\parallel}\in \mathbb{R}^r$ denote the first $r$ elements of $\w_0$, and $\w_{0,\perp}\in \mathbb{R}^{d-r}$ denote the remaining $d-r$ elements, and likewise let $\w_{1,\parallel}\in \mathbb{R}^r$ and $\w_{0,\perp}\in \mathbb{R}^{d-r}$ denote the first $r$ and last $d-r$ elements of $\w_1$, respectively. 
    Set $\eta = \Theta(1)$ and $\lambda_{\mathbf{w}}=\frac{2^{-r-2}\pi+ \eta}{\eta 2^{-r-2}\pi}$. 
    We have, for any   $\mathbf{w}_{j}^0 \in \mathcal{G}_{\mathbf{w}}$, there are absolute constants $c,c'$ such that
    % \begin{align}
    %     \w_{1,\parallel} &= \eta \w_{0,\parallel} +  \nonumber \\
    %     \w_{1,\perp} &= \eta  \nonumber \\
    % \end{align}
    \begin{align}
       \left \|\mathbf{w}_{j,:r}^0 - \frac{\eta^2  }{2^{r+2} }\mathbf{w}_{j,:r}^0  \right\|_2 &\leq  c \nu_{\mathbf{w}} \left( \frac{r^4 + \log^4(m)}{2^r d} + de^{-c' d } +  d \frac{\sqrt{r}}{\sqrt{T}} \right)\nonumber \\
        \left\| \mathbf{w}_{j,r:}^0 \right\|_2 &\leq c \nu_{\mathbf{w}}\left( \frac{r^{3.5} + \log^{3.5}(m)}{2^{r}d^{1.5}} +  de^{-c' d } + d \frac{\sqrt{r}}{\sqrt{T}}\right) \nonumber
    \end{align}
\end{lemma}

\begin{proof}
 Due to the computation of the gradient in Lemma \ref{lem:compute_grad}, we have
\begin{align}
    \mathbf{w}_{j}^+ &= (1 - \eta \lambda_{\mathbf{w}})\mathbf{w}_{j}^0 - \eta \nabla_{\mathbf{w}_{j}} \mathcal{L}(\mathbf{W}^0, \mathbf{b}^0,\{\mathbf{a}_{i}^+\}_{i\in [n]}) \nonumber \\
    &=  (1 - \eta \lambda_{\mathbf{w}})\mathbf{w}_{j}^0  + {\eta^2 2^{-r}}  \mathbf{A}(\mathbf{w}_{j}^0) \mathbf{w}_{j}^0 +\eta \tilde{\mathbf{e}}\nonumber  \\
    \mathbf{w}_{j,:r}^+ 
    % &= 
    % (1 - \eta \lambda_{\mathbf{w}}) \mathbf{w}_{j,:r}^0  + {\eta^2 2^{-r}}  \begin{bmatrix}
    %     \mathbf{I}_r & \mathbf{0}_{r,d-r} \\
    % \end{bmatrix} \mathbf{A}(\mathbf{w}_{j}^0)\mathbf{w}_{j}^0  \nonumber \\
    &= (1 - \eta \lambda_{\mathbf{w}}) \mathbf{w}_{j,:r}^0  + {\eta^2 2^{-r}}\mathbf{A}_{\parallel,\parallel}(\mathbf{w}_{j}^0)\mathbf{w}_{j,:r}^0 + {\eta^2 2^{-r}}\mathbf{A}_{\parallel,\perp}(\mathbf{w}_{j}^0)\mathbf{w}_{j,r:}^0 + \eta \tilde{\mathbf{e}}_{:r} \nonumber \\
    \mathbf{w}_{{j,r:}}^+ &= (1 - \eta \lambda_{\mathbf{w}}) \mathbf{w}_{j,r:}^0  + {\eta^2 2^{-r}} \mathbf{A}_{\perp,\parallel}(\mathbf{w}_{j}^0)\mathbf{w}_{j,:r}^0 + {\eta^2 2^{-r}}  \mathbf{A}_{\perp,\perp}(\mathbf{w}_{j}^0)\mathbf{w}_{j,r:}^0 + \eta \tilde{\mathbf{e}}_{r:} \nonumber 
\end{align}
where $\|\tilde{\mathbf{e}} \|_2 \leq O( \nu_{\mathbf{w}} de^{-c d } + \nu_{\mathbf{w}} d \frac{\sqrt{r}}{\sqrt{T}} )$.

Next, 
% since $\mathbf{w}_{j}^0 \in \mathcal{G}_{\mathbf{w}}$,  to obtain
\begin{align}
    \mathbf{w}_{j,:r}^+ &= (1 - \eta \lambda_{\mathbf{w}})\mathbf{w}_{j,:r}^0  + {\eta^2 2^{-r}} \mathbf{w}_{j,:r}^0 + \frac{ {\eta^2 2^{-r}} }{2{\pi} \|\mathbf{w}_{j,r:}^0\|_2^2} \mathbf{w}_{j,:r}^0(\mathbf{w}_{j,r:}^0)^\top  \mathbf{w}_{j,r:}^0 \nonumber \\
    &\quad + {\eta^2 2^{-r}}\left(   \mathbf{A}_{\parallel,\parallel}(\mathbf{w}_{j}^0) - \tfrac{1}{4}\mathbf{I}_r \right)\mathbf{w}_{j,:r}^0 \nonumber \\
    &\quad + {\eta^2 2^{-r}} \left( \mathbf{A}_{\parallel,\perp}(\mathbf{w}_{j}^0) -  \frac{1 }{2{\pi} \|\mathbf{w}_{j,r:}^0\|_2^2} \mathbf{w}_{j,:r}^0(\mathbf{w}_{j,r:}^0)^\top   \right)\mathbf{w}_{j,r:}^0 + \eta \tilde{\mathbf{e}}_{:r} \nonumber \\
    &= \left(1 - \eta \lambda_{\mathbf{w}} + {\eta^2 2^{-r-2}}\left(1 + \frac{2}{\pi}\right) \right) \mathbf{w}_{j,:r}^0  + {\eta^2 2^{-r}}\mathbf{e}_{\parallel} + \eta \tilde{\mathbf{e}}_{:r}
\end{align}
where 
\begin{align}
    \|\mathbf{e}_{\parallel}\|_2&=  \left\| \left(   \mathbf{A}_{\parallel,\parallel}(\mathbf{w}_{j}^0) - \tfrac{1}{4}\mathbf{I}_r \right)\mathbf{w}_{j,:r}^0  +  \left( \mathbf{A}_{\parallel,\perp}(\mathbf{w}_{j}^0) -  \frac{1 }{2{\pi} \|\mathbf{w}_{j,r:}^0\|_2^2} \mathbf{w}_{j,:r}^0(\mathbf{w}_{j,r:}^0)^\top   \right)\mathbf{w}_{j,r:}^0   \right\|_2 \nonumber \\
    &\leq \left\| \left(   \mathbf{A}_{\parallel,\parallel}(\mathbf{w}_{j}^0) - \tfrac{1}{4}\mathbf{I}_r \right)\mathbf{w}_{j,:r}^0 \right\|_2 \nonumber \\
    &\quad +   \left\| \left( \mathbf{A}_{\parallel,\perp}(\mathbf{w}_{j}^0) -  \frac{1 }{2{\pi} \|\mathbf{w}_{j,r:}^0\|_2^2} \mathbf{w}_{j,:r}^0(\mathbf{w}_{j,r:}^0)^\top   \right)\mathbf{w}_{j,r:}^0   \right\|_2  \nonumber \\
    &\leq  \left\|    \mathbf{A}_{\parallel,\parallel}(\mathbf{w}_{j}^0) - \tfrac{1}{4}\mathbf{I}_r \right\|_2\left\|\mathbf{w}_{j,:r}^0 \right\|_2 \nonumber \\
    &\quad +  \left\|  \mathbf{A}_{\parallel,\perp}(\mathbf{w}_{j}^0) -  \frac{1 }{2{\pi} \|\mathbf{w}_{j,r:}^0\|_2^2} \mathbf{w}_{j,:r}^0(\mathbf{w}_{j,r:}^0)^\top   \right\|_2 \left\|\mathbf{w}_{j,r:}^0   \right\|_2  \nonumber \\
    &= O\left(\nu_{\mathbf{w}}\frac{r^4 + \log^4(m)}{d} \right)  \label{xvx}
\end{align} where \eqref{xvx} follows by  Lemmas \ref{lem:apara} and \ref{lem:aparaperp} and the fact that $\mathbf{w}\in \mathcal{G}_{\mathbf{w}}$. 

Similarly, 
\begin{align}
    \mathbf{w}_{j,r:}^{+} &= (1 - \eta \lambda_{\mathbf{w}}) \mathbf{w}_{j,r:}^0  + {\eta^2 2^{-r}}  \frac{ \mathbf{w}_{j,r:}^0 (\mathbf{w}_{j,:r}^0)^\top }{2{\pi}\|\mathbf{w}_{j,r:}^0\|_2^2}\mathbf{w}_{j,:r}^0 \nonumber \\
    &\quad + \left( 1 - \frac{\|\mathbf{w}_{j,:r}^0\|_2^2}{\|\mathbf{w}_{j,r:}^0\|_2^2}  \right) {\eta^2 2^{-r}}  \frac{ \mathbf{w}_{j,r:}^0(\mathbf{w}_{j,r:}^0)^\top }{2{\pi}\|\mathbf{w}_{j,r:}^0\|_2^2}\mathbf{w}_{j,r:}^0 \nonumber \\
    &\quad + {\eta^2 2^{-r}}\left(\mathbf{A}_{\perp,\parallel}(\mathbf{w}_{j}^0)- \frac{ \mathbf{w}_{j,r:}^0(\mathbf{w}^0_{j,:r})^\top }{2{\pi}\|\mathbf{w}_{j,r:}^0\|_2^2} \right)\mathbf{w}_{j,:r}^0 \nonumber \\
    &\quad + {\eta^2 2^{-r}}\left( \mathbf{A}_{\perp,\perp}(\mathbf{w}_{j}^0)  -  \left( 1 - \frac{\|\mathbf{w}_{j,:r}^0\|_2^2}{\|\mathbf{w}_{j,r:}^0\|_2^2}  \right) \frac{ \mathbf{w}_{j,r:}^0(\mathbf{w}_{j,r:}^0)^\top }{2{\pi}\|\mathbf{w}_{j,r:}^0\|_2^2} \right)\mathbf{w}_{j,r:}^0 + \eta \tilde{\mathbf{e}}_{r:}\nonumber \\
    &=  (1 - \eta \lambda_{\mathbf{w}}) \mathbf{w}_{j,r:}^0  +  {\eta^2 2^{-r}}  \frac{ \mathbf{w}_{j,r:}^0(\mathbf{w}_{j,r:}^0)^\top }{2{\pi}\|\mathbf{w}_{j,r:}^0\|_2^2}\mathbf{w}_{j,r:}^0 \nonumber \\
    &\quad + {\eta^2 2^{-r}}\left(\mathbf{A}_{\perp,\parallel}(\mathbf{w}_{j}^0)- \frac{ \mathbf{w}_{j,r:}^0(\mathbf{w}_{j,:r}^0)^\top }{2{\pi}\|\mathbf{w}_{j,r:}^0\|_2^2} \right)\mathbf{w}_{j,:r}^0 \nonumber \\
    &\quad + {\eta^2 2^{-r}}\left( \mathbf{A}_{\perp,\perp}(\mathbf{w}_{j}^0)  -  \left( 1 - \frac{\|\mathbf{w}_{j,:r}^0\|_2^2}{\|\mathbf{w}_{j,r:}^0\|_2^2}  \right) \frac{ \mathbf{w}_{j,r:}^0(\mathbf{w}_{j,r:}^0)^\top }{2{\pi}\|\mathbf{w}_{j,r:}^0\|_2^2} \right)\mathbf{w}_{j,r:}^0 + \eta \tilde{\mathbf{e}}_{r:}\nonumber \\
    &= \left(1 - \eta \lambda_{\mathbf{w}} + {\eta^2 2^{-r-2}}\frac{2}{\pi} \right) \mathbf{w}_{j,r:}^0  + {\eta^2 2^{-r}}\mathbf{e}_\perp + \eta \tilde{\mathbf{e}}_{r:} 
\end{align}
where 
\begin{align}
  \|  \mathbf{e}_{\perp}\| &= \Bigg\|\left(\mathbf{A}_{\perp,\parallel}(\mathbf{w}_{j}^0)- \frac{ \mathbf{w}_{j,r:}^0(\mathbf{w}_{j,:r}^0)^\top }{2{\pi}\|\mathbf{w}_{j,r:}^0\|_2^2} \right)\mathbf{w}_{j,:r}^0 \nonumber \\
  &\quad \quad + \left( \mathbf{A}_{\perp,\perp}(\mathbf{w}_{j}^0)  -  \left( 1 - \frac{\|\mathbf{w}_{j,:r}^0\|_2^2}{\|\mathbf{w}_{j,r:}^0\|_2^2}  \right) \frac{ \mathbf{w}_{j,r:}^0(\mathbf{w}_{j,r:}^0)^\top }{2{\pi}\|\mathbf{w}_{j,r:}^0\|_2^2} \right)\mathbf{w}_{j,r:}^0 \Bigg\|_2 \nonumber \\
  &\leq \left\|\mathbf{A}_{\perp,\parallel}(\mathbf{w}_{j}^0)- \frac{ \mathbf{w}_{j,r:}^0(\mathbf{w}_{j,:r}^0)^\top }{2{\pi}\|\mathbf{w}_{j,r:}^0\|_2^2} \right\|_2\|\mathbf{w}_{j,:r}^0 \|_2\nonumber \\
  &\quad \quad + \left\| \mathbf{A}_{\perp,\perp}(\mathbf{w}_{j}^0)  -  \left( 1 - \frac{\|\mathbf{w}_{j,:r}^0\|_2^2}{\|\mathbf{w}_{j,r:}^0\|_2^2}  \right) \frac{ \mathbf{w}_{j,r:}^0(\mathbf{w}_{j,r:}^0)^\top }{2{\pi}\|\mathbf{w}_{j,r:}^0\|_2^2} \right\|_2 \|\mathbf{w}_{j,r:}^0\|_2 \nonumber \\
  &= O\left( \nu_{\mathbf{w}}\frac{r^{3.5} + \log^{3.5}(m)}{d^{1.5}} \right) \label{rfr}
\end{align}
where \eqref{rfr} follows by  Lemmas \ref{lem:aperp} and \ref{lem:aparaperp} and the fact that $\mathbf{w}\in \mathcal{G}_{\mathbf{w}}$.
% \begin{align}
%     \mathbf{w}_{j,:r}^0_{j,1} 
%     &= \left(1 - \eta \lambda_{\mathbf{w}} + \frac{\eta^2 }{2^{r+2}} + \frac{\eta^2 }{2^{r+1}\pi }  \right) \mathbf{M}_{:r}^\top\mathbf{w}_{j}^0  + O(k^{-1/2}) \nonumber \\
%     (\mathbf{w}_{j,r:}^0)^\top_{{j,1}} &= \left(1 - \eta \lambda_{\mathbf{w}}  + \frac{\eta^2 }{2^{r+1}\pi}  \right) \mathbf{w}_{j,r:}^0 + O(k^{-1/2}) \nonumber 
% \end{align}
Applying the choice of $\lambda_{\mathbf{w}}$ completes the proof.
% From Lemma \ref{lem:compute_grad},  we have 
% \begin{align}
%     % \mathbf{w}_{1} &= (1 - \eta \lambda)\mathbf{w}_0  + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{M} \mathbf{A}(\mathbf{w}_t)\mathbf{M}^\top \mathbf{w}_t \nonumber \\
%     % \mathbf{w}_{j,:r}^0_{t+1} &= (1 - \eta \lambda) \mathbf{M}_{:r}^\top\mathbf{w}_t  + \frac{\eta 2^{-r}}{\lambda_1}  \begin{bmatrix}
%     %     \mathbf{I}_r & \mathbf{0}_{r,d-r} \\
%     % \end{bmatrix} \mathbf{A}(\mathbf{w}_t)\mathbf{M}^\top \mathbf{w}_t  \nonumber \\
%     % &= (1 - \eta \lambda) \mathbf{M}_{:r}^\top\mathbf{w}_t  + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\parallel,\parallel}(\mathbf{w}_t)\mathbf{w}_{j,:r}^0_t + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\parallel,\perp}(\mathbf{w}_t)\mathbf{M}_{r:}^\top \mathbf{w}_t \nonumber \\
%     % \mathbf{M}_{r:}^\top \mathbf{w}_{t+1} &= (1 - \eta \lambda) \mathbf{M}_{r:}^\top\mathbf{w}_t  + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\perp,\parallel}(\mathbf{w}_t)\mathbf{w}_{j,:r}^0_t + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\perp,\perp}(\mathbf{w}_t)\mathbf{M}_{r:}^\top \mathbf{w}_t \nonumber \\
%         \mathbf{w}_{1} &= (1 - \eta \lambda)\mathbf{w}_0  + \frac{\eta 2^{-r}}{\lambda_1}   \mathbf{A}(\mathbf{w}_0) \mathbf{w}_0 \nonumber 
% \end{align}
% For the first $r$ elements, since  $\mathbf{w}_{0} \in \mathcal{G}_{\mathbf{w}}$ by Lemmas \ref{lem:apara} and \ref{lem:aparaperp} we have 
% \begin{align}
%     \mathbf{w}_{1,\parallel} &= (1 - \eta \lambda) \mathbf{w}_{0,\parallel}  + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\parallel,\parallel}(\mathbf{w}_0) \mathbf{w}_{0,\parallel} + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\parallel,\perp}(\mathbf{w}_0) \mathbf{w}_{0,\perp}  \nonumber \\
%     &=  \nonumber \\
% \end{align}
% For the last $d-r$ elements, again using $\mathbf{w}_{0} \in \mathcal{G}_{\mathbf{w}}$ by Lemmas \ref{lem:aperp} and \ref{lem:aparaperp} we have
% \begin{align}
%     \mathbf{w}_{1,\perp} &= (1 - \eta \lambda) \mathbf{w}_{1,\perp}  + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\perp,\parallel}(\mathbf{w}_{0})\mathbf{w}_{0,\parallel} + \frac{\eta 2^{-r}}{\lambda_1}  \mathbf{A}_{\perp,\perp}(\mathbf{w}_0)\mathbf{w}_{0,\perp} \nonumber \\
%     &= 
% \end{align}
\end{proof}
Finally we are ready to prove Proposition \ref{prop:1} and Theorem \ref{thm:1}. For convenience, we restate the statements here.



\begin{proposition} \label{prop:1:app}
    Consider the gradient-based multi-task algorithm described in Section~\ref{sec:alg} and suppose Assumption \ref{assump:diversity} holds. Further assume $d=\Omega( r^4)$,
and let $\eta = \Theta(1)$, $\lambda_{\mathbf{a}} = 1/\eta $, $\lambda_{\mathbf{w}} = (1+(\eta^2 2^{-r-1})/\pi)/\eta$, and $\nu_{\mathbf{w}} = O(d^{-1.25})$. % and $\sigma_b = O(d^{-1.25})$. 
%$m = \Omega(r 2^r)$, 
% For a subset ${S}\subseteq [m]$, let $\mathbf{W}_{1,S}\in \mathbb{R}^{|S|\times d}$ denote the sub-matrix of $\mathbf{W}$ with rows selected by $S$.
Then for any $m= O(d)$,  with probability at least $0.99$ over the random initialization we have
% there is a subset of neurons ${S}\subseteq [m]$ of size $|{S}| \geq m/4$ such that for all $j \in {S}$:
% the following two properties are satisfied by the representation learned by MTRL:
\begin{enumerate}
\item $\frac{1}{\nu_{\mathbf{w}}\sqrt{\bar{m}}}\|\Pi_{\parallel}(\mathbf{W}^+) -  \Omega(\frac{1}{2^r}) % \frac{\eta^2}{2^{r+2}} 
\Pi_{\parallel}(\mathbf{W}^{0}) \|_2 = O\left(  
\frac{r^4 + \log^4(m)}{2^r d} 
+  \frac{\sqrt{r}d}{\sqrt{T}}
\right) $,
% (and scales with init)
% $\|\mathbf{W}_1 - \eta 2^{-r-2} \mathbf{M}_{:r}\mathbf{M}_{:r}^\top \mathbf{W}_0\| =  +  O\left(\sqrt{\frac{r}{d-r}}\right)$
    \item $\frac{1}{\nu_{\mathbf{w}}\sqrt{\bar{m}}}\|\Pi_{\perp}(\mathbf{W}^{+}) \|_2 = O\left(
\frac{r^{3.5} + \log^{3.5}(m)}{2^r d^{1.5}} %+ \eta\nu_{\mathbf{w}} d^{1.5} e^{-d^2/8} 
    + \frac{\sqrt{r}d}{\sqrt{T}}
    \right)$
    %     \eta^2 \nu_{\mathbf{w}}\frac{r^{3.5}}{d^{1.5}2^r} %+ \eta\nu_{\mathbf{w}} d^{1.5} e^{-d^2/8} 
    % + \eta \nu_{\mathbf{w}}\frac{\sqrt{r}d}{\sqrt{n}}
    % \item For all $\mathbf{v}\in \{-1,1\}^r$, $\exists j \in \mathcal{S}$ such that $\mathbf{w}_{1,j}^\top \mathbf{v} + b_{1,j} > 0$
    % $\sigma_{\min}(\mathbf{W}_1)$
\end{enumerate}
\end{proposition}

\begin{proof}
By Lemma \ref{lem:init}, $\mathbf{w}_j^0\in \mathcal{G}_{\mathbf{w}}$ for all $j\in [m]$ with probability at least 0.99. 
 Conditioned on this event, we can directly apply Lemma \ref{lem:final} along with the fact that $\|\mathbf{B}\|_2\leq \|\mathbf{B}\|_F \sqrt{\bar{m}}\max_{j\in [m]} \|\mathbf{b}_j\|_2$ for any matrix $\mathbf{B}\in \mathbb{R}^{m \times d}$, where $\mathbf{b}_j$ is the $j$-th row of $\mathbf{B}$. We also use that $\frac{r^4 + \log^4(m)}{2^r d} \gg de^{-c' d } $ and $\frac{r^{3.5} + \log^{3.5}(m)}{2^r d^{1.5}} \gg de^{-c' d } $ as $d$ is sufficiently large.
\end{proof}


\begin{theorem}[  ]\label{thm:1:app}
    Consider the setting in Proposition \ref{prop:1} and let $d =\Omega( r^4 + \log^4(m))$, $m = \Omega(r)$,  and $ T = \Omega( r 2^{2r} d^2) $. Let $\sigma_r(\mathbf{B})$ denote the $r$-th singular value of a matrix $\mathbf{B}$.
Then with probability at least $0.99$ over the random initialization, we have 
\begin{align}  
    \frac{\| \Pi_{\perp}(\mathbf{W}^+) \|_2}{\sigma_{r}( \Pi_{\parallel}(\mathbf{W}^+) )} = O\left( \frac{ {r^{3.5}} + \log^{3.5}(m) }{ d^{1.5} } + \frac{  2^r \sqrt{r} d  }{ \sqrt{T}} \right). \nonumber
\end{align}
\end{theorem}

\begin{proof}
By Lemmas \ref{lem:init} and \ref{lem:init2} and a union bound, we have that  $\mathbf{w}_j^0\in \mathcal{G}_{\mathbf{w}}$ for all $j\in [m]$, and $\nu_{\mathbf{w}}\sqrt{\bar{m}}\left(1 - c\frac{\sqrt{r}}{\sqrt{\bar{m}}}\right)$ with probability at least $0.99$.
Conditioned on these events, we can invoke Lemma \ref{lem:final} to obtain
\begin{align}
    \sigma_{r}( \Pi_{\parallel}(\mathbf{W}^+) ) &\geq \eta 2^{-r-2}\sigma_{r}( \Pi_{\parallel}(\mathbf{W}^0) ) - \nu_{\mathbf{w}} \sqrt{\bar{m}} O\left(  
\frac{r^4 + \log^4(m)}{2^r d} 
+  \frac{\sqrt{r}d}{\sqrt{T}}
\right) \nonumber \\
&\geq \eta 2^{-r-2} \nu_{\mathbf{w}} \sqrt{\bar{m}}   - \nu_{\mathbf{w}} \sqrt{\bar{m}} O\left( \frac{\sqrt{r}}{2^r \sqrt{\bar{m}}} -   
\frac{r^4 + \log^4(m)}{2^r d} 
+  \frac{\sqrt{r}d}{\sqrt{T}}
\right)  \nonumber \\
&= \Omega(2^{-r} \nu_{\mathbf{w}} \sqrt{\bar{m}}) \label{zm}
\end{align}
 % with probability at least 0.99. 
 Likewise,  conditioned again on the event that $\mathbf{w}_j^0\in \mathcal{G}_{\mathbf{w}} $ for all $j\in [m]$,
\begin{align}
    \|\Pi_{\perp}(\mathbf{W}^+)\|_2 &= \nu_{\mathbf{w}} \sqrt{\bar{m}}  O\left(
\frac{r^{3.5} + \log^{3.5}(m)}{2^r d^{1.5}} 
    + \frac{\sqrt{r}d}{\sqrt{T}}
    \right). \label{nz}
\end{align}
Combining \eqref{zm} and \eqref{nz} completes the proof.
\end{proof}

% \begin{lemma}
%     compute b1, show it doesn't really change
% \end{lemma}

% \begin{proof}
    
% \end{proof}

% \begin{lemma}
%     argue that now for any task, there exists a good head on top of the weights and biases that can get zero loss 
% \end{lemma}

% \begin{proof}
% For any fixed vertex $\mathbf{v}\in \{-1,1\}^r$ and $j \in [m]$, $\mathbf{w}_{j,0}^\top \mathbf{M}_{:r}^\top \mathbf{M}_{:r}\mathbf{v}$ is a Gaussian random variable with mean 0 and variance $\|  \mathbf{M}_{:r}^\top \mathbf{M}_{:r}\mathbf{v}\|_2^2$ 

% No, for each vertex $\mathbf{v}\in \{-1,1\}^r$, there is some w that is close

% cos Angle is mean 0 and variance $\|  \mathbf{M}_{:r}^\top \mathbf{M}_{:r}\mathbf{v}\|_2^2/r$. 

% But $\mathbf{w}_{j,:r}^0_{j,0}$ has norm approx

% this means l1 norm $\|\mathbf{w}_{j,:r}^0_{j,0}\|_1\geq ...$
% meanwhile l1 norm of perp is small
% so changing them cannot change the output
% noooo not tight enough

% \end{proof}
\newpage
\section{Proof of Downstream Guarantees.}\label{app:down}
In this section we prove Theorem \ref{thm:downstream} and Corollary \ref{cor:set}. Given a function $\bar{f}^*:\{-\frac{1}{\sqrt{r}},\frac{1}{\sqrt{r}}\}^r \rightarrow \{-1,1\}$, we refer to the sets $\mathcal{V}^+ \coloneqq \{ \mathbf{v}_{:r} \in \{-\frac{1}{\sqrt{r}},\frac{1}{\sqrt{r}}\}^r: \bar{f}^* = 1 \}$ and $\mathcal{V}^- \coloneqq \{ \mathbf{v}_{:r} \in \{-\frac{1}{\sqrt{r}},\frac{1}{\sqrt{r}}\}^r: \bar{f}^* = -1 \}$ as the inverse sets of $\bar{f}^*$. Note that solving the task described by $\bar{f}^*$ entails finding a classifier that separates the inverse sets of $\bar{f}^*$. As in \ref{app:thrm1}, we will abuse notation by reusing $c,c',c''$ and $C$ as absolute constants independent of all other parameters. The notations $O(\cdot)$, $\Theta(\cdot)$, and $\Omega(\cdot)$ describe scalings up to absolute constants independent of all other parameters.

\textbf{Proof summary.} Informally, the proof of Theorem \ref{thm:downstream}
 follows six steps:
 \begin{enumerate}
     \item Construct a two-layer ReLU network embedding using the weights output by the during multi-task pretraining algorithm for the first-layer weights, then randomly sampling first-layer biases and second layer weights and biases (calling this the ``learned'' embedding),
     \item Construct a nearby two-layer ReLU network embedding that is ``purified'' in the sense that it is only a function of the the $r$ label-relevant features of the input,
     \item Show that the ``purified'' network linearly separates the pair of inverse sets corresponding to any binary function on the $r$-dimensional hypercube with high probability as long as the number of neurons in each layer  is larger than some function of $r$,
     \item Prove that the outputs of the learned embedding are very close to the outputs of the ``purified'' embedding, meaning the learned embedding has the same linear separation capability with only slightly smaller margin,
     \item Prove that the learned embedding linearly separates the inverse sets with lower bounded margin, and
     \item Apply a standard generalization result for linear classification showing that the empirically-optimal head achieves loss close to the minimal loss (zero).
 \end{enumerate} 

\textbf{Step 1: Construct downstream embedding.} We start by stating the construction of the downstream classifier as described first in Section \ref{sec:alg}. Let $\mathbf{W}^+$ be the model weights resulting from one step of the multitask representation learning algorithm. For simplicity, here we discard the last half of the weights and consider a network with $\bar{m}\coloneqq m/2$ neurons in the first layer (this means that all neurons are independent, which was originally not the case due to the symmetric initialization, and thereby alleviates technical issues but is not necessary). 
%Note that this slightly differs from the construction in Section \ref{sec:alg} but 

Let  $\bar{\mathbf{W}}^+\in \mathbb{R}^{\bar{m} \times d}$ denote the submatrix of $\mathbf{W}^+$ obtained by taking its top $\bar{m}$ rows. Similarly,  let $\bar{\mathbf{W}}^0\in \mathbb{R}^{\bar{m} \times d}$ denote the submatrix of $\mathbf{W}^0$ obtained by taking its top $\bar{m}$ rows.

The downstream classifier is a linear head composed with a two-layer ReLU network embedding 
% three-layer ReLU network $F(\mathbf{x}; )$
with $\bar{m}$ neurons in the first layer and $\hat{m}$ neurons in the second layer. For now, we focus on the embedding itself, excluding the linear classification head. The weights of the first layer of the embedding are equal to the weights in $\bar{\mathbf{W}}^+$ up to rescaling. The biases of the first layer and weights and biases of the second layer are contained in $\mathbf{b}$,
 $\hat{\mathbf{W}} := [\hat{\mathbf{w}}_1,\dots,\hat{\mathbf{w}}_{\hat{m}}]^\top $ and $ \hat{\mathbf{b}}$, respectively, where
    % Consider a two-layer ReLU network $F:\mathbb{R}^{d}\rightarrow \mathbb{R}^{\hat{m}}$ constructed as follows:
    \begin{align}
        % \hat{\mathbf{w}}_j &\sim \mathcal{N}\left(\mathbf{0}_d,\frac{2}{\hat{m}}\mathbf{I}_d\right)\quad j = 1,\dots,\hat{m} \nonumber\\
        \mathbf{b} &\sim \text{Unif}\left(\left[-\frac{\sqrt{2}\gamma}{\sqrt{\bar{m}}},\frac{\sqrt{2}\gamma}{\sqrt{\bar{m}}}\right]^m\right) \nonumber \\
         \hat{\mathbf{w}}_j &\sim \mathcal{N}\left(\mathbf{0}_d, \frac{2}{\hat{m}}\mathbf{I}_d\right) \quad \forall \; j = 1,\dots, \hat{m} \nonumber\\
        \hat{\mathbf{b}} &\sim \text{Unif}\left(\left[-\frac{\sqrt{2}\hat{\gamma}}{\sqrt{\hat{m}}},\frac{\sqrt{2}\hat{\gamma}}{\sqrt{\hat{m}}}\right]^{\hat{m}}\right) \nonumber 
        % F(\mathbf{x};\boldsymbol{\theta}) &= \sigma( \hat{\mathbf{W}}\sigma(\mathbf{Wx}+ \mathbf{b}) + \hat{\mathbf{b}} ) \quad \forall \mathbf{x} \in \mathbb{R}^r \label{net}
    \end{align}
    for some $\gamma,\hat{\gamma}>0$.
The full embedding is given by:
    \begin{align}
    % F(\mathbf{v},\bar{\mathbf{W}}^+,  \alpha ) &:= 
    % \mathbf{a}^\top 
    g(\mathbf{v}; \alpha\bar{\mathbf{W}}^+, \mathbf{b}, \hat{\mathbf{W}}, \hat{\mathbf{b}}) :=  \sigma( \hat{\mathbf{W}}\sigma(\alpha \bar{\mathbf{W}}^+\mathbf{v}+ \bar{\mathbf{b}}) + \hat{\mathbf{b}} ) \quad \forall \;\mathbf{v} \in \{-1,1\}^d \label{qw}
\end{align}
where $\alpha := \frac{2^{r+2.5}}{\sqrt{\bar{m}} \eta^2 }$ is a rescaling factor.  

For ease of notation we denote $g(\mathbf{v}):= g(\mathbf{v}; \alpha\bar{\mathbf{W}}^+, \mathbf{b}, \hat{\mathbf{W}}, \hat{\mathbf{b}}) $.
    % $ {\mathbf{W}} = [{\mathbf{w}}_1,\dots,{\mathbf{w}}_{{m}}]^\top $,  $ \hat{\mathbf{W}} = [\hat{\mathbf{w}}_1,\dots,\hat{\mathbf{w}}_{\hat{m}}]^\top $ 
    % and $\boldsymbol{\theta} = \{{\mathbf{W}},{\mathbf{b}},\hat{\mathbf{W}},\hat{\mathbf{b}} \}$ 


\textbf{Step 2: Construct purified downstream embedding.} Next, the ``purified'' embedding also has $\bar{m}$ neurons in the first layer and $\hat{m}$ neurons in the second layer, and is also parameterized by $\mathbf{b}$,
 ${\mathbf{W}} $ and $ \mathbf{b}$, for the first layer biases and second layer weights and biases, respectively, but has a different construction of the first layer weights. 
 % In particular, the first layer only takes as input the $r$ label-relevant coordinates in $\mathbf{x}$. 
 In particular, the first-layer weights are equal to the first $r$ coordinates of the corresponding weights in $\mathbf{W}^0$, up to rescaling, and zero on all other coordinates.
 % zero on all the spurious coordinates and 
 % The neuron weights are 
 % maps from $\mathbb{R}^r$ to $\mathbb{R}^{\bar{m}}$
 Formally, this embedding is given by 
 \begin{align}
 {g}(\mathbf{v}; [\bar{\mathbf{W}}^0_{:r},\mathbf{0}_{\bar{m}\times (d-r) }, ], \mathbf{b}, \hat{\mathbf{W}}, \hat{\mathbf{b}} ) := \sigma( \hat{\mathbf{W}}\sigma(\hat{\alpha}\bar{\mathbf{W}}^0_{:r}\mathbf{v}_{:r}+ {\mathbf{b}}) + \hat{\mathbf{b}} ) \quad \forall \;\mathbf{v} \in \{-1,1\}^d
 \end{align}
 where $\hat{\alpha} = \frac{2}{\nu_{\mathbf{w}}\sqrt{\bar{m}}} $.

For ease of notation we denote $\tilde{g}(\mathbf{v}_{:r}):= g([\mathbf{v}_{:r},\mathbf{0}_{d-r}]; [\hat{\alpha}\bar{\mathbf{W}}^0_{:r},\mathbf{0}_{\bar{m}\times (d-r) }, ], \mathbf{b}, \hat{\mathbf{W}}, \hat{\mathbf{b}} )  $.
 
 \textbf{Step 3: Purified embedding linearly separates two classes.} We start by showing that for any function $\bar{f}^*:\{-1,1\}^r\rightarrow \{-1,1\}$, with high probability $\tilde{g}$ linearly separates the pair of inverse sets $\mathcal{V}^+ \coloneqq \{ \mathbf{v} \in \{-{1},{1}\}^r: \bar{f}^* = 1 \}$ and $ \mathcal{V}^- \coloneqq \{ \mathbf{v} \in \{-1,1\}^r: \bar{f}^* = -1 \} $ with lower bounded margin
 by adapting a result of \cite{dirksen2022separation}. Note that we have not optimized the dependence of $\bar{m}$ on $\log()$ and the dependence of $\hat{m}$ on $\log()$ factors in the exponent.
 % among the first $r$ coordinates.
 % The idea
% For analysis purposes, we also consider the following three-layer ReLU network whose parameters are coupled with $ $.
% \begin{align}
%     \tilde{F}(\mathbf{x}; )
% \end{align}

\begin{lemma}[Adapted from Theorem 1 in \cite{dirksen2022separation}] \label{lem:pure}
% Consider the network $F(\cdot;\boldsymbol{\theta})$ constructed in \eqref{net}.
% with constants
    % Let $\gamma \gtrsim \sqrt{\log(e  \sqrt{r} \gamma/2)}$, $m \gtrsim \frac{\gamma^8 r^5}{128} + \frac{\gamma^8 r^4 \log(1/\nu)}{256}$, $\hat{\gamma} \gtrsim \frac{\gamma^4 r^2}{16}(\sqrt{r} +\gamma)$. Further define
    % \begin{align}
    %     \omega \coloneqq \exp\left( C( r + \gamma^2 ) \gamma^6 ...     \right)
    % \end{align}
% without constants
    Let  $\delta \in (0,0.05]$, 
    % $\gamma \gtrsim \sqrt{\log(\sqrt{r} \gamma)}$, $m \gtrsim  {\gamma^8 r^5} + {\gamma^8 r^4 \log(1/\delta)}$, $\hat{\gamma} \gtrsim {\gamma^4 r^2}(\sqrt{r} +\gamma)$. 
$\gamma = \Theta(\log({r}))$, $\hat{\gamma} = \Theta( r^{2.5} \log^4(r))$,
% \begin{align}
%     \mu &= \Omega (r^{-2.5} \log^{-3}(r) \exp( -C \log^6(r) r^5 \log(\log(r)/\delta) )) \nonumber \\
%     m &= O( r^4\log^8(r) ({ r} + {\log(1/\delta)})) \nonumber \\
%     \hat{m} &= O\left(r^{3.5} \log^4(r) \exp\left( C \log^6(r) r^5 \log(\log(r)/\delta) ) \right) \log(1/\delta)\right)
% \end{align} for an absolute constant $c$.
    % Further define
    % \begin{align}
    %     \omega \coloneqq \exp\left( C( \gamma^6  r^5 + \gamma^8  r^4 )  \log(\gamma/\delta)  \right)
    % \end{align}
    % for an absolute constant $C$, and let 
    % $\bar{m} = \Omega( r^4\log^8(r) ({ r} + {\log(1/\delta)}))$
    $\bar{m} = \Omega( r^5\log^8(r) {\log(1/\delta)})$, and
    % $\hat{m} \gtrsim \frac{\hat{\gamma}}{\gamma} r \omega \log(1/\delta)$.
    $\hat{m} = %r^{3.5} \log^4(r) 
    \exp\left(\Omega\left( \bar{m}
    % r^5 \log^6(r)  \log(\log(r)/\delta) ) 
    \right) \right)
    % \log(1/\delta)
    $.
    Consider any function $\bar{f}^*:\{-\frac{1}{\sqrt{r}},\frac{1}{\sqrt{r}}\}^r \rightarrow \{-1,1\}$. With probability at least $1 - \delta$, $\tilde{g}$ makes the classes $\mathcal{V}^+ \coloneqq \{ \mathbf{v}_{:r} \in \{-\frac{1}{\sqrt{r}},\frac{1}{\sqrt{r}}\}^r: \bar{f}^* = 1 \}$ and $\mathcal{V}^- \coloneqq \{ \mathbf{v}_{:r} \in \{-\frac{1}{\sqrt{r}},\frac{1}{\sqrt{r}}\}^r: \bar{f}^* = -1 \}$ linearly separable with margin 
    % $\mu = c \sqrt{r} \gamma^2/(\hat{\gamma}\omega)$, 
    $\mu = \exp \left(- O(r^5 \log^6(r)  \log(\log(r)/\delta) )\right)$,
    i.e. there exists a vector $\mathbf{a}\in \mathbb{R}^{\hat{m} }$ with $\|\mathbf{a}\|_2=1$ and bias $\tau\in \mathbb{R}$ such that for all $\mathbf{v}_{:r}\in \left\{-\frac{1}{\sqrt{r}},\frac{1}{\sqrt{r}}\right\}^r,$
    \begin{align}
       \bar{f}^\ast(\mathbf{v}) = 1 &\implies  \mathbf{a}^\top \tilde{g}( \mathbf{v}_{:r})+ \tau > \mu    \nonumber\\
        \bar{f}^\ast(\mathbf{v}) = -1 &\implies  \mathbf{a}^\top \tilde{g}( \mathbf{v}_{:r}) + \tau < -\mu \nonumber   
    \end{align}
\end{lemma}


\begin{proof}
% To apply Theorem 1 in \cite{dirksen2022separation}, we need to normalize the data, 
The above statement is a special case of Theorem 1 in \cite{dirksen2022separation} with 
 positive and negative sets  ${\mathcal{V}}^+ \coloneqq \{ \mathbf{v}_{:r} \in \{-\frac{1}{\sqrt{r}},\frac{1}{\sqrt{r}}\}^r: \bar{f}^* = 1 \}$ and ${\mathcal{V}}^- \coloneqq \{ \mathbf{v}_{:r} \in \{-\frac{1}{\sqrt{r}},\frac{1}{\sqrt{r}}\}^r:  \bar{f}^* = -1 \}$, respectively. Note that the distance between these sets is $\frac{2}{\sqrt{r}}$, and we have used $|\mathcal{V}^+||\mathcal{V}^-|\leq 2^{2r}$.
 % Now we apply Theorem 1 in \cite{dirksen2022separation} to obtain that $\tilde{g}$ linearly separates $\bar{\mathcal{V}}^+$ and $\bar{\mathcal{V}}^-$ with margin at least $c\gamma^2/(\hat{\gamma}\omega)$ with probability at least $1-\delta$. Note that we have used $|\mathcal{V}^+||\mathcal{V}^-|\leq 2^{2r}$.
\end{proof}


\begin{lemma} \label{lem:pure2}
% Consider the network $F(\cdot;\boldsymbol{\theta})$ constructed in \eqref{net}.
% with constants
    % Let $\gamma \gtrsim \sqrt{\log(e  \sqrt{r} \gamma/2)}$, $m \gtrsim \frac{\gamma^8 r^5}{128} + \frac{\gamma^8 r^4 \log(1/\nu)}{256}$, $\hat{\gamma} \gtrsim \frac{\gamma^4 r^2}{16}(\sqrt{r} +\gamma)$. Further define
    % \begin{align}
    %     \omega \coloneqq \exp\left( C( r + \gamma^2 ) \gamma^6 ...     \right)
    % \end{align}
% without constants
    Let 
$\gamma = \Theta(\sqrt{r}\log({r}))$, $\hat{\gamma} = \Theta( r^{3} \log^4(r))$,
and $\bar{m}$, $\hat{m}$ satisfy the same conditions as in Lemma \ref{lem:pure}, for any $\delta \in (0,0.05]$.
    Consider any function $\bar{f}^*:\{-1,1\}^r \rightarrow \{-1,1\}$. With probability at least $1 - \delta$, $\tilde{g}$ makes the classes $\mathcal{V}^+ \coloneqq \{ \mathbf{v}_{:r} \in \{-{1},{1}\}^r: \bar{f}^* = 1 \}$ and $\mathcal{V}^- \coloneqq \{ \mathbf{v}_{:r} \in \{-{1},{1}\}^r: \bar{f}^* = -1 \}$ linearly separable with margin 
    % $\mu = c \sqrt{r} \gamma^2/(\hat{\gamma}\omega)$, 
    $\mu = %r^{-2} \log^{-3}(r) 
    \exp( -O ( r^5 \log^6(r)  \log(\log(r)/\delta) ))$.
\end{lemma}
\begin{proof}
    The result follows from Lemma \ref{lem:pure} and the fact that $g([\sqrt{r}\mathbf{v}_{:r},\mathbf{0}_{d-r}]; [\bar{\mathbf{W}}^0_{:r},\mathbf{0}_{\bar{m}\times (d-r) }, ], \sqrt{r}\mathbf{b}, \hat{\mathbf{W}}, \sqrt{r}\hat{\mathbf{b}} ) = \sqrt{r}\tilde{g}(\mathbf{v}_{:r}) $, thus if $\bar{\mathcal{V}}^+ \coloneqq \{ \mathbf{v}_{:r} \in \{-\frac{1}{\sqrt{r}},\frac{1}{\sqrt{r}}\}^r: \bar{f}^* = 1 \}$ and $\bar{\mathcal{V}}^- \coloneqq \{ \mathbf{v}_{:r} \in \{-\frac{1}{\sqrt{r}},\frac{1}{\sqrt{r}}\}^r: \bar{f}^* = -1 \}$ are linearly separated with margin $\mu'$ by $\tilde{g}$, then after rescaling the biases, $\mathcal{V}^+ \coloneqq \{ \mathbf{v}_{:r} \in \{-\frac{1}{\sqrt{r}},\frac{1}{\sqrt{r}}\}^r: \bar{f}^* = 1 \}$ and $\mathcal{V}^- \coloneqq \{ \mathbf{v}_{:r} \in \{-\frac{1}{\sqrt{r}},\frac{1}{\sqrt{r}}\}^r: \bar{f}^* = -1 \}$ are linearly separated with margin $\sqrt{r}\mu'$.
\end{proof}


% In particular, Lemma \ref{lem:pure} is satisfied with $\gamma = \Theta(\log({r}))$, $\hat{\gamma} = \Theta( r^{2.5} \log^4(r))$, and
% \begin{align}
%     \mu &= \Omega (r^{-2.5} \log^{-3}(r) \exp( -C \log^6(r) r^5 \log(\log(r)/\delta) )) \nonumber \\
%     m &= O( r^4\log^8(r) ({ r} + {\log(1/\delta)})) \nonumber \\
%     \hat{m} &= O\left(r^{3.5} \log^4(r) \exp\left( C \log^6(r) r^5 \log(\log(r)/\delta) ) \right) \log(1/\delta)\right)
% \end{align} for an absolute constant $c$.
% Note these are sufficient conditions -- Lemma \ref{lem:pure} would also hold with larger $m$ and $\hat{m}$ and smaller $\mu$.



% \begin{lemma} 
%     % apply result from shi et al showing that GD finds such a head? can play with how the updates for the head are computed. with infinite samples, gd is the same as min. 
    
%     % should need 2**r samples for finite? need to say that rep learning is better than random features.

%     with random second layer and purified first layer, with high probability the network linearly separates
% \end{lemma}

% \begin{proof}

% % with multitask trained features: information theoretically, for every bad neuron, need at least two samples with that neuron activated but different labels

% % with random features: should need Theta(exp(k)) neurons to guarantee 2r good ones
    
% \end{proof}

\textbf{Step 4: Downstream embedding is close to purified embedding.} Next we compare the outputs of the ``purified'' embedding $\tilde{g}$  to those of the learned embedding ${g}$. 
% In particular, let $\mathbf{W}^+ \in \mathbb{R}^{m\times d}$ be the first layer weights learned by MTRL. Then, let  $\boldsymbol{\theta}_1 = \{{\mathbf{W}}_1,{\mathbf{b}},\hat{\mathbf{W}},\hat{\mathbf{b}} \}$ and let
% \begin{align}
%     F(\mathbf{x};\boldsymbol{\theta}) &= \sigma( \hat{\mathbf{W}}\sigma(\frac{2}{\sqrt{\bar{m}}\nu_{\mathbf{w}} \eta^2 }\mathbf{W}_{1,(:m/2)}\mathbf{x}+ \mathbf{b}) + \hat{\mathbf{b}} )  \label{net1}
% \end{align}
% for all $\mathbf{x}\in \mathbb{R}^d$.

% Note that ${F}(\cdot;{\boldsymbol{\theta}})$ and $F^+(\cdot;\boldsymbol{\theta}^+)$ have different domains; this is not a problem.

    % true network output is close to purified network. so if purified has margin delta', true has margin delta''
\begin{lemma} \label{lem:true}
% Let $\bar{\mathbf{W}}^{0}\in \mathbb{R}^{(m/2) \times d}$ be the first layer weights initialized by MTRL.
% Let $F(\cdot;\boldsymbol{\theta}): \mathbb{R}^r\rightarrow \mathbb{R}^{\hat{m}}$ be the network constructed in \eqref{net}, with one exception: set $\mathbf{W} = \frac{2}{\nu_{\mathbf{w}}\sqrt{\bar{m}}}\bar{\mathbf{W}}^{0}\mathbf{M}_{:r}$.  
% Let $F_1(\cdot;\boldsymbol{\theta}_1): \mathbb{R}^d\rightarrow \mathbb{R}^{\hat{m}}$ be the network constructed in \eqref{net1}. 
% Let $\mathbf{M}\in\mathbb{R}^{d\times d}$ be a column-orthonormal matrix. 
% Suppose $\bar{m} = \Theta( r^4\log^8(r) ({ r} + {\log(1/\delta)}))$ and $
%     \hat{m} = \Omega\left(r^{3.5} \log^4(r) \exp\left( c r^5 \log^6(r)  \log(\log(r)/\delta) ) \right) \log(1/\delta)\right)$ for an absolute constant $c$, and set $\gamma = \Theta(\log({r}))$, $\hat{\gamma} = \Theta( r^{2.5} \log^4(r))$ and $\eta=\Theta(1)$.
    Under the same conditions as Lemma \ref{lem:pure2} hold. Additionally, suppose $\eta=\Theta(1)$, $\lambda_{\mathbf{a}} = 1/\eta$, $\lambda_{\mathbf{w}} = (1+(\eta^2 2^{-r-1})/\pi)/\eta$, and Assumption \ref{assump:diversity} holds,
then  with probability at least $0.99$,  for all $\mathbf{v}\in \{-1,1\}^d$, 
\begin{align}
    \| \tilde{g}( \mathbf{v}_{:r}) - g( \mathbf{v})\|_2 &= O\left(\frac{r^{3.5} + \log^{3.5}(\bar{m})}{2^r \sqrt{d}} + \frac{\sqrt{r}d^{1.5}}{\sqrt{T}}\right). \nonumber 
\end{align}
\end{lemma}

\begin{proof}
For any $\mathbf{v}\in \{-1,1\}^d$, we have
\begin{align}
    &\|\tilde{g}( \mathbf{v}_{:r}) - g( \mathbf{v})\|_2 \nonumber \\
    &= \left\|\sigma\left( \hat{\mathbf{W}}\sigma\left(\frac{2}{\sqrt{\bar{m}}\nu_{\mathbf{w}} }\bar{\mathbf{W}}^0_{:r}\mathbf{v}_{:r} + \mathbf{b}\right) + \hat{\mathbf{b}} \right) -  \sigma\left( \hat{\mathbf{W}}\sigma\left(\frac{2}{\sqrt{\bar{m}}\nu_{\mathbf{w}} \eta^2 2^{-r-2} }\bar{\mathbf{W}}^+\mathbf{v}+ \mathbf{b}\right) + \hat{\mathbf{b}} \right)  \right\|_2 \nonumber \\
    &\leq \left\| \hat{\mathbf{W}}\sigma\left(\frac{2}{\sqrt{\bar{m}}\nu_{\mathbf{w}}  }\bar{\mathbf{W}}^{0}\mathbf{v}+ \mathbf{b}\right)  -   \hat{\mathbf{W}}\sigma(\frac{2}{\sqrt{\bar{m}}\nu_{\mathbf{w}} \eta^2 2^{-r-2} }\bar{\mathbf{W}}^{+}\mathbf{v}+ \mathbf{b})   \right\|_2 \label{lip1} \\
    &\leq \|\hat{\mathbf{W}}\|_2 \left\| \frac{2}{\sqrt{\bar{m}}\nu_{\mathbf{w}}  }\bar{\mathbf{W}}_{:r}^{0}\mathbf{v}_{:r} -   \frac{2}{\sqrt{\bar{m}}\nu_{\mathbf{w}} \eta^2 2^{-r-2}}\bar{\mathbf{W}}^{+}\mathbf{v}   \right\|_2 \label{lip2}\\
    &=  \frac{2}{\sqrt{\bar{m}}\nu_{\mathbf{w}}  }\|\hat{\mathbf{W}}\|_2 \left\|\bar{\mathbf{W}}^{0}_{:r}\mathbf{v}_{:r} -   \frac{1}{\eta^2 2^{-r-2}}\bar{\mathbf{W}}^{+}_{:r}\mathbf{v}_{:r} -  \frac{1}{\eta^2 2^{-r-2}}\bar{\mathbf{W}}^{+}_{r:}\mathbf{v}_{r:}  \right\|_2 \label{lip22} \\
    &\leq \frac{2}{\sqrt{\bar{m}}\nu_{\mathbf{w}}  }\|\hat{\mathbf{W}}\|_2 \left\|\bar{\mathbf{W}}^{0}_{:r}\mathbf{v}_{:r} -   \frac{1}{\eta^2 2^{-r-2} }\bar{\mathbf{W}}^{+}_{:r}\mathbf{v}_{:r} \right\|_2  + \frac{2}{\sqrt{\bar{m}}\nu_{\mathbf{w}}  }\|\hat{\mathbf{W}}\|_2 \left\| \frac{1}{\eta^2 2^{-r-2} }\bar{\mathbf{W}}^{+}_{r:}\mathbf{v}_{r:}  \right\|_2 \label{lip3} \\
    &\leq \frac{2}{\sqrt{\bar{m}}\nu_{\mathbf{w}}  }\|\hat{\mathbf{W}}\|_2 \left\|\bar{\mathbf{W}}^{0}_{:r} -   \frac{1}{\eta^2 2^{-r-2} }\bar{\mathbf{W}}^{+}_{:r}\right\|_2 \|\mathbf{v}_{:r}\|_2  + \frac{2}{\sqrt{\bar{m}}\nu_{\mathbf{w}} {\eta^22^{-r-2} } }\|\hat{\mathbf{W}}\|_2 \left\| \bar{\mathbf{W}}^{+}_{r:}  \right\|_2 \|\mathbf{v}_{r:}\|_2 \label{lip4} \\
    &= \frac{2\sqrt{r}}{\sqrt{\bar{m}}\nu_{\mathbf{w}}  }\|\hat{\mathbf{W}}\|_2 \left\|\bar{\mathbf{W}}^{0}_{:r} -   \frac{1}{\eta^2 2^{-r-2} }\bar{\mathbf{W}}^{+}_{:r}\right\|_2  + \frac{2\sqrt{d-r}}{\sqrt{\bar{m}}\nu_{\mathbf{w}} {\eta^22^{-r-2} } }\|\hat{\mathbf{W}}\|_2 \left\| \bar{\mathbf{W}}^{+}_{r:}  \right\|_2\nonumber \\
    &=  O\left(  \frac{r^{4.5} + \sqrt{r}\log^4(\bar{m})}{2^r {d}} +    \frac{{r}d}{\sqrt{T}}\right) \|\hat{\mathbf{W}}\|_2  + O\left(\frac{r^{3.5}+\log^{3.5}(\bar{m})}{2^r\sqrt{d}} +  \frac{\sqrt{r}d^{1.5}}{\sqrt{T}}\right)\|\hat{\mathbf{W}}\|_2\label{lip5} \\ 
    &=  O\left(\frac{r^{3.5}+\log^{3.5}(\bar{m})}{2^r\sqrt{d}} +   \frac{\sqrt{r}d^{1.5}}{\sqrt{T}}\right)\label{lip6} 
\end{align}
where \eqref{lip1} and \eqref{lip2} follow since $\sigma()$ is $1$-Lipschitz and by the Cauchy-Schwarz Inequality, \eqref{lip4} follows by the Cauchy-Schwarz Inequality, \eqref{lip5} follows by Proposition \ref{prop:1:app} with probability at least $0.999$, and \eqref{lip6} follows with probability at least 0.99 (since with high probability, $\|\hat{\mathbf{W}}\|_2\leq O\left(1 + \frac{\bar{m}}{\hat{m}} \right) = O(1)$).
\end{proof}
% with probability at least $1-$.  $(\frac{\sqrt{\bar{m}}}{\sqrt{\hat{m}}})$
% want to say that $\mathbf{w}^\top \mathbf{M}_{:r}$ is isotopic  gaussian in r. need to couple these inits.

% need to upscale mtrl first layer by 1/sigmaw after pre-training. this is fine. only reason for sigmaw being small is to avoid max during pretrainning. fine after.

% We have 
% \begin{align}
%     n
% \end{align}

% issues:


\textbf{Step 5: Downstream embedding linearly separates two classes.} Now we reason that $\bar{f}^*$ linearly separates the two classes with high probability.
\begin{lemma} \label{lem:sep}
% Choose 
% \begin{align}
%     \mu &= \Theta (r^{-2.5} \log^{-3}(r) \exp( -C \log^6(r) r^5 \log(\log(r)/\delta) )) \nonumber \\
%     m &= \Theta( r^4\log^8(r) ({ r} + {\log(1/\delta)})) \nonumber \\
%     \hat{m} &= \Omega\left(r^{3.5} \log^4(r) \exp\left( C \log^6(r) r^5 \log(\log(r)/\delta) ) \right) \log(1/\delta)\right)
% \end{align}
Suppose the same conditions as Lemma \ref{lem:true} hold. Additionally, suppose \\
$d = \Omega( \log^{7}(\bar{m})\exp( c r^5 \log^6(r)\log(\log(r)/\delta) )  )$ and $T=\Omega( d^3 \exp( c r^5 \log^6(r)\log(\log(r)/\delta) ) )$ for an absolute constant $c$.
Consider any function $\bar{f}^*:\{-1,1\}^r \rightarrow \{-1,1\}$. With probability at least $0.99 - \delta$, ${g}$ makes the classes $\mathcal{V}^+ \coloneqq \{ \mathbf{v} \in \{-{1},{1}\}^r: \bar{f}^* = 1 \}$ and $\mathcal{V}^- \coloneqq \{ \mathbf{v} \in \{-1,1\}^r: \bar{f}^* = -1 \}$ linearly separable with margin 
% $\Omega (r^{-2} \log^{-3}(r) \exp( -C \log^6(r) r^5 \log(\log(r)/\delta) ))$  r^{-2} \log^{-3}(r) 
$$\mu = \exp(-O( r^5 \log^6(r) \log(\log(r)/\delta) ))$$ 
% - O\left(\frac{r^{3.5}+\log^{3.5}(m)}{\sqrt{d}} +  d^{1.5} e^{-c'd} + \frac{\sqrt{r}d^{1.5}}{\sqrt{T}}\right),$$ 
i.e. there exists a vector $\mathbf{a}\in \mathbb{R}^{\hat{m} }$ with $\|\mathbf{a}\|_2=1$ and bias $\tau\in \mathbb{R}$ such that for all $\mathbf{v}\in \left\{-{1},{1}\right\}^d,$
    \begin{align}
       % \bar{f}^\ast(\mathbf{v}) = 1 &\implies  \mathbf{a}_{:m}^\top g(\mathbf{v}) + a_{m+1} > \mu    \nonumber\\
       \bar{f}^\ast(\mathbf{v}) = 1 &\implies  \mathbf{a}^\top {g}( \mathbf{v})+ \tau > \mu   \nonumber \\
        \bar{f}^\ast(\mathbf{v}) = -1 &\implies  \mathbf{a}^\top g(\mathbf{v}) + \tau < -\mu \nonumber   
    \end{align}
\end{lemma}



\begin{proof}
% Note that setting $\mathbf{W} = \frac{{2}}{\nu_{\mathbf{w}}\sqrt{\bar{m}}}\bar{\mathbf{W}}^{0}\mathbf{M}_{:r}$ does not change the marginal distribution of $\mathbf{W}$; it only couples it with $\bar{\mathbf{W}}^{0}$. 
The proof follows from Lemmas \ref{lem:pure2} and \ref{lem:true}. In particular, for any point $\mathbf{v}\in \{-1,1\}^d$, from Lemma \ref{lem:pure2} we have with probability at least $1-\delta$, for absolute constants $c,c'$, there exists $\mathbf{a}\in \mathbb{R}^{\hat{m} }$ with $\|\mathbf{a}\|_2=1$ and  $\tau\in \mathbb{R}$ such that
    \begin{align}
       \bar{f}^\ast(\mathbf{v}) = 1 &\implies  \mathbf{a}^\top \tilde{g}( \mathbf{v}_{:r})+ \tau >  \exp(-c r^5 \log^6(r) \log(\log(r)/\delta) )   \nonumber \\
       &\implies  \mathbf{a}^\top {g}( \mathbf{v})+ \tau >  \exp(-cr^5 \log^6(r) \log(\log(r)/\delta) )    \nonumber \\
       &\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad -c'\left(\frac{r^{3.5}+\log^{3.5}(\bar{m})}{2^r\sqrt{d}} +   \frac{\sqrt{r}d^{1.5}}{\sqrt{T}}\right) \label{vcvc}\\
       &\implies  \mathbf{a}^\top {g}( \mathbf{v}_{:r})+ \tau > \exp(-O( r^5 \log^6(r) \log(\log(r)/\delta) ))     \label{cdcd}    
    \end{align}
where \eqref{vcvc} follows with probability at least $0.99-\delta$   by Lemma \ref{lem:true} and a union bound, and \eqref{cdcd} follows since $d$ and $T$ are sufficiently large. Repeating the same argument for the case  $\bar{f}^\ast(\mathbf{v}) = -1$ with the same $\mathbf{a},\tau$ completes the proof.
\end{proof}

% We now want to solve a linear classification problem in $\mathbb{R}^{\hat{m}}$.



% \begin{proof}
% By Lemma \ref{lem:pure}

    
% \end{proof}


% \begin{theorem}[Lower Bound]\label{thm:lower_app}
    
% \end{theorem}

% \begin{proof}
 
% \end{proof}

\textbf{Step 6: Complexity of learning the linear head.}
Now that we have shown that for any binary function on the $r$-dimensional hypercube, $g$ makes its inverse sets linearly separable with high probability, we complete the proof by bounding the sample complexity of finding a linear separator. For convenience, we restate the theorem here in full detail. Recall that in the previous proofs we have used $\bar{m}=m/2$ in place of $m$; here we give the statements in terms of $m$.
\begin{theorem}[End-to-end Guarantee] \label{thm:downstream:app}
% Let $\mathbf{W}^+$ be the outcome of the multi-task representation learning algorithm described in Section \ref{sec:alg}, and suppose Assumption \ref{assump:diversity} holds. 
Consider a downstream task with labeling function $\bar{f}_{T+1}^*$.
Construct the two-layer ReLU embedding $g:\{-1,1\}^d \rightarrow \mathbb{R}^{\hat{m}}$ using the rescaled $\mathbf{W}^+$ for first layer weights as in  \eqref{qw}, and train the task-adapted head $(\mathbf{a}_{T+1},\tau_{T+1})$ using $n$ i.i.d. samples from the downstream task, as in \eqref{ada},  with regularization parameter $\hat{\lambda}_{\mathbf{a}} = {\exp(-c r^5 \log^6(r) \log(\log(r)/\delta) )}$ for an absolute constant $c$.
% If $ d = \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  )) $, $n = \Omega( d^3 \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  ))  )$,
% $m = \Theta(r^4\log^8(r) ({ r} + {\log(1/\delta)}))$,  $\hat{m}= \Omega( r^{3.5} \log^4(r) \exp\left( C \log^6(r) r^5 \log(\log(r)/\delta) ) \right) \log(1/\delta) )$, and 
 Further, suppose Assumption \ref{assump:diversity} holds, 
${m} = \Omega( r^5\log^8(r) {\log(1/\delta)})$,
    $\hat{m} =\exp\left(\Omega\left( {m}\right) \right)$,
$d = \Omega( \log^{7}({m})\exp( c r^5 \log^6(r)\log(\log(r)/\delta) )  )$, and \\
$T=\Omega( d^3 \exp( c r^5 \log^6(r)\log(\log(r)/\delta) ) )$, and set  $\gamma = \Theta(\sqrt{r}\log({r}))$, $\hat{\gamma} = \Theta( r^{3} \log^4(r))$, $\eta = \Theta(1)$, $\lambda_{\mathbf{a}} = 1/\eta$ and $\lambda_{\mathbf{w}} = (1 - (\eta^2 2^{-r-1})/\pi )/\eta$.


Then for any $\delta \in (0,0.05]$, with probability at least $0.99-\delta$ over the random  initializations, draw of $T$ pretraining tasks, and draw of $n$ samples, we have
\begin{align}
        \mathcal{L}^{(\text{eval})}_{T+1} 
        &= 
       \frac{ \exp(-O( r^5 \log^6(r) \log(\log(r)/\delta) )) }{ \sqrt{n}}. 
    \end{align}
    % where $\tilde{\Omega}(\cdot),\tilde{\Theta}(\cdot)$ and $\tilde{O}(\cdot)$ hide logarithmic factors in $r$ and $\delta^{-1}$.
\end{theorem}

\begin{proof}
We know that there is an absolute constant $c$ such that with probability at least 0.999, $ \max(\|\hat{\mathbf{W}}\|_2 ,\| \hat{\alpha} \bar{\mathbf{W}}^0\|_2) \leq c$. Thus, by Lemma \ref{lem:true}, for any $\mathbf{v}\in\{-1,1\}^d$, $\|g(\mathbf{v})\|_2\leq 2 \|\tilde{g}(\mathbf{v}_{:r})\|_2 \leq c'(\gamma + \hat{\gamma})\leq c'' r^{2.5}\log^4(r)$ for absolute constants $c',c''$. 


Let $ (\mathbf{a}_{T+1}^*,\tau^*_{T+1})$ be the linear head that separates the inverse sets of $\bar{f}^*_{T+1}$ with margin $\mu := \exp(-O( r^5 \log^6(r) \log(\log(r)/\delta) ))$, whose existence is guaranteed with high probability by Lemma \ref{lem:sep}. 
We have $|\tau^*_{T+1}|\leq \max_{\mathbf{v}\in \{\pm 1\}^d} |(\mathbf{a}^*)^\top {g}(\mathbf{v})|\leq c'' r^{2.5}\log^4(r)$. Thus, $\sqrt{\|\mathbf{a}^*_{T+1}\|_2^2 + (\tau^*_{T+1})^2}\leq c''' r^{1.25}\log^2(r)=: B$. Since $(\mathbf{a}^*_{T+1},\tau^*_{T+1})$ linearly separates the two inverse sets with margin $\mu$, $(\mathbf{a}^*_{T+1}/\mu,\tau^*_{T+1}/\mu)$ linearly separates them with margin 1. Define $\mathcal{H}:= \{(\mathbf{a}, \tau): \mathbf{a}\in \mathbb{R}^{\hat{m}}, \tau\in \mathbb{R},\sqrt{\|\mathbf{a}^*_{T+1}\|_2^2 + (\tau^*_{T+1})^2} \leq B/\mu\}$. 
% Define  By Lemma \ref{lem:sep}, 
\begin{align}
 \mathcal{L}^*_{T+1}  \coloneqq &\min_{(\mathbf{a},\tau)\in \mathcal{H}} \frac{1}{2^d}\sum_{\mathbf{v}\in \{\pm 1\}^d} \ell( f_{T+1}^*(\mathbf{v}_{:r}), \mathbf{a}^\top g(\mathbf{v}) + \tau )\nonumber\\
    &\leq \frac{1}{2^d}\sum_{\mathbf{v}\in \{\pm 1\}^d} \ell((\mathbf{a}_{T+1}^*)^\top g(\mathbf{v})/\mu + \tau^*_{T+1}/\mu , \bar{f}_{T+1}^*(\mathbf{v}_{:r}) )  \nonumber \\
    &= 0 \label{zer}
\end{align}
where $\ell$ is the hinge loss, as usual.
% where $B = $. 
Recall that 
    \begin{align}
    ( \mathbf{a}_{T+1}, \tau_{T+1}) \in\  \argmin_{ \mathbf{a}\in \mathbb{R}^{\hat{m}}, \tau \in \mathbb{R}}  \frac{1}{n}\sum_{l=1}^n \ell(\mathbf{a}^\top g(\mathbf{v}_l )+\tau , \bar{f}_{T+1}^*(\mathbf{v}_{l,:r})  ) + \frac{\hat{\lambda}_{\mathbf{a}}}{2}(\|\mathbf{a}\|_2^2+\tau^2) \label{adaa}
\end{align}
for a set of $n$ random samples $\{\mathbf{v}_l,f_{T+1}^*(\mathbf{v}_l) \}_{l=1}^n$, where each $\mathbf{v}_l$ is drawn independently uniformly  from $\{-1,1\}^d$. Equivalently, for $\hat{\lambda}_{\mathbf{a}} = \mu/B$  we have
    \begin{align}
    ( \mathbf{a}_{T+1}, \tau_{T+1}) \in\  \argmin_{ (\mathbf{a}, \tau)\in \mathcal{H}}  \frac{1}{n}\sum_{l=1}^n \ell(\mathbf{a}^\top g(\mathbf{v}_l )+\tau , \bar{f}_{T+1}^*(\mathbf{v}_{l,:r})  )  \label{adaaa}
\end{align}

Thus, by applying a standard generalization bound for $1$-Lipschitz loss functions \cite{Livni_2017}, we obtain, for an absolute constant $C$,
\begin{align}
   \mathcal{L}^{(\text{eval})}_{T+1} &:=  \frac{1}{2^d}\sum_{\mathbf{v}\in \{\pm 1\}^d} \ell( \mathbf{a}_{T+1}^\top g(\mathbf{v}) + \tau_{T+1}, \bar{f}_{T+1}^*(\mathbf{v}_{:r}) ) \nonumber \\
   &\leq \mathcal{L}^*_{T+1}  + C\frac{B\sqrt{\log(1/\delta')}}{\mu\sqrt{n}} \nonumber \\
    &= C\frac{B\sqrt{\log(1/\delta')}}{\mu\sqrt{n}} \nonumber \\
    &= O\left(\frac{\exp(O( r^5 \log^6(r) \log(\log(r)/\delta) ))}{\sqrt{n}}\sqrt{\log(1/\delta')} \right).
\end{align}
with probability at least $0.99 - \delta - \delta'$. Setting $\delta' = \delta^{\text{new}}/2$ and $\delta = \delta^{\text{new}}/2$ for some $\delta^{\text{new}}\in (0,0.05]$ completes the proof. 
% \begin{theorem}  \label{lem:head}
% \begin{align}
%         \mathcal{L}^{(\text{eval})}_{n+1}(\boldsymbol{\theta}_1,\mathbf{a}_{n+1}) &= O\left(\frac{ r^{5} \log^8(r) \log(1/\delta) --- no, margin}{ \sqrt{N}}\right)
%     \end{align}
%     with probability at least $1-\delta $ over choice of $\mathcal{S}$. $\mathcal{L}^*=0$ because $\lambda_{\mathbf{a}}=1$ and linearly separable. constrained loss equiv to regularized. but how large is tau? can't be larger than $\hat{\gamma}$. so actually need $\lambda_{\mathbf{a}}=1/(1+\hat{\gamma})$ to get zero loss. no, margin
% \end{theorem}
\end{proof}

To conclude, we state and prove the full version of Corollary \ref{cor:set}.
\begin{corollary}[Generalization to set of tasks] \label{cor:set:app}
Consider a set  of possible downstream tasks $\mathcal{T}^{(\text{eval})}$ with cardinality $|\mathcal{T}^{(\text{eval})}| = D$. 
% Suppose $ d = \exp(\tilde{\Omega}( r^5 \log(D) )) $, $T = d^3 \exp(\tilde{\Omega}( r^5 \log(D)  )  )$,
% $m = \tilde{\Theta}(r^5 \log(D) )$,  and $\hat{m}= \exp\left( \tilde{\Omega}(r^5 \log(D) )  \right)$. Construct the two-layer ReLU embedding as in \eqref{F}. 
Construct the two-layer ReLU embedding $g:\{-1,1\}^d \rightarrow \mathbb{R}^{\hat{m}}$ using the rescaled $\mathbf{W}^+$ for first layer weights as in  \eqref{qw}, and train the task-adapted head $(\mathbf{a}_{T+1},\tau_{T+1})$ using $n$ i.i.d. samples from the downstream task, as in \eqref{ada},  with regularization parameter $\hat{\lambda}_{\mathbf{a}} = {\exp(-c r^5 \log^6(r) \log(\log(r)/\delta) )}$ for an absolute constant $c$.
% If $ d = \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  )) $, $n = \Omega( d^3 \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  ))  )$,
% $m = \Theta(r^4\log^8(r) ({ r} + {\log(1/\delta)}))$,  $\hat{m}= \Omega( r^{3.5} \log^4(r) \exp\left( C \log^6(r) r^5 \log(\log(r)/\delta) ) \right) \log(1/\delta) )$, and 
 Further, suppose Assumption \ref{assump:diversity} holds,
${m} = \Omega( r^5\log^8(r) {\log(1/\delta)})$,
    $\hat{m} =\exp\left(\Omega\left( {m}\right) \right)$,
$d = \Omega( \log^{7}({m})\exp( c r^5 \log^6(r)\log(\log(r)/\delta) )  )$, and $T=\Omega( d^3 \exp( c r^5 \log^6(r)\log(\log(r)/\delta) ) )$, and set  $\gamma = \Theta(\sqrt{r}\log({r}))$, $\hat{\gamma} = \Theta( r^{3} \log^4(r))$, $\eta = \Theta(1)$, $\lambda_{\mathbf{a}} = 1/\eta$ and $\lambda_{\mathbf{w}} = (1 - (\eta^2 2^{-r-1})/\pi )/\eta$.

Then with probability at least $0.99-\delta$,  any task $T+1$ in $\mathcal{T}^{(\text{eval})}$ 
satisfies
% compute $(\mathbf{a}_{T+1},\tau_{T+1})$ using $n$ samples from task $T+1$,
\begin{align}
        \mathcal{L}^{(\text{eval})}_{T+1} %(\boldsymbol{\theta}_1,\mathbf{a}_{T+1}) 
        &= 
        % \tilde{O}\left(\frac{ r^{5} \log^8(r) \log(1/\delta')}{ \sqrt{N}}\right).
       \frac{\exp(O( r^5 \log^6(r) \log(D\log(r)/\delta) ))}{\sqrt{n}}, 
    \end{align}
    % where $\tilde{\Omega}(\cdot),\tilde{\Theta}(\cdot)$ and $\tilde{O}(\cdot)$ hide logarithmic factors in $r$ and $\delta^{-1}$. 
    % \textcolor{blue}{same comment as above about $\delta$}
\end{corollary}

\begin{proof}
Note that in the proof of Theorem \ref{thm:downstream:app}, $\delta$ upper bounds the probability of a bad event occurring that depends on the choice of downstream task (while 0.01 upper bounds the probability of a bad event occurring that is independent of the downstream task, namely the event that any $\w_j^0\notin \mathcal{G}_{\mathbf{w}}$). 
Thus, setting setting $\delta^{\text{new}} = \delta/D$ applying a union bound over all tasks implies $$\mathcal{L}^{(\text{eval})}_{T+1} 
        = 
       \frac{\exp(O( r^5 \log^6(r) \log(\log(r)/\delta^{\text{new}}) ))}{\sqrt{n}} =\frac{\exp(O( r^5 \log^6(r) \log(D\log(r)/\delta) ))}{\sqrt{n}} $$ for all tasks $T+1\in \mathcal{T}^{\text{eval}}$ with probability at least $0.99 - \delta^{\text{new}} D = 0.99 - \delta$, as desired.
\end{proof}


\input{Notes_sample_complexity}

==> Proof_RepLearn-ICML.tex <==





\section{Proofs of Proposition \ref{prop:1} and Theorem \ref{thm:1}} \label{app:thrm1}


In this section we prove Proposition \ref{prop:1} and Theorem \ref{thm:1}. Throughout, we will slightly abuse notation by reusing $c,c',c''$ and $C$ as absolute constants independent of all other parameters. The notations $O(\cdot)$, $\Theta(\cdot)$, and $\Omega(\cdot)$ describe scalings up to absolute constants independent of all other parameters. 
% We start by establishing that each neuron is in general position with high probability at initialization.
% For convenience, we restate Proposition \ref{prop:1} here.

% \begin{theorem}
    
% \end{theorem}
% \begin{proof}
    
% \end{proof}
% need to show that for every task, there exists a good network with the same set of features
% just need one feature in each orthant, then can learn any function by adding biases
% bias should be between closest vertex sum and second closest vertex sum (flip one coord)

% with random features you could still get one feature closest to each vertex with only r2^r features. but the issue is that changing one coordinate of the perp would deactivate the neuron. should be able to build a lower bound out of this -- the lower bound should be k2^k neurons required. we want features that are robust to changes in the perp.

% \begin{lemma}
%     the biases and weights are in a nice set at initialization whp

%     each is initialized at the same scale
% \end{lemma}

% \begin{proof}
    
% \end{proof}





% 1. compute A

% 2. w+ has the right norm and points in the right direction in parallel space

% 3. so we can again say that with high probability, there exists a subset of good indicators

% 4. how does bias affect analysis?


% \begin{lemma}
%     for all j, the hypercube to gaussian error vector has expected norm squared at most c/k2
% \end{lemma}

% \begin{proof}
    
% \end{proof}

% \begin{lemma}
%     for all j, the other error vectors have expected norm squared sufficiently small
% \end{lemma}

% \begin{proof}
    
% \end{proof}

% \input{Proof_Errors}



% \begin{lemma}[Initialization I] \label{lem:init}
%     % With probability at least $1-\delta$, all neuron weights satisfy:
%     % \begin{align}
%     %     \leq \|\mathbf{w}_{j}^0\|_2 \leq  \nonumber \\
%     % \end{align}
%     % a constant fraction of neurons are good, in the sense that 

%     % 1. error vector is less than c/k, other errors are sufficiently small

%     % 2. w|| is large enough

%     % 3. need bias in an interval like [rt(r) - 1/rt(r), rt(r)]. which occurs with prob 1/rt(r). too small. but still a good network exists. so can jointly optimize a,b. to get a good network...no. not jointly convex in a,b

%     % or, make different generalization arguement... 
%     Define the set 
%     \begin{align}
%         \mathcal{G}_{\mathbf{w}} \coloneqq \big\{&\mathbf{w}\in \mathbb{R}^d :  \|\mathbf{Mw}\|_2 \leq c \nu_{\mathbf{w}}( \sqrt{r} + \sqrt{\log(m)}), \nonumber \\
%         &\quad  c\nu_{\mathbf{w}}(\sqrt{d-r} - \sqrt{\log(m)}) \leq \|\mathbf{M}_\perp \mathbf{w} \|_2 \leq c\nu_{\mathbf{w}}(\sqrt{d-r} + \sqrt{\log(m)}), \nonumber \\
%         &\quad c\nu_{\mathbf{w}}(\sqrt{d} - \sqrt{\log(m)}) \leq \|\mathbf{w} \|_2 \leq c\nu_{\mathbf{w}}(\sqrt{d} + \sqrt{\log(m)}) \big\}
%     \end{align} for an absolute constant $c$
%     with probability at least $0.999$, $\mathbf{w}_{j}\in \mathcal{G}_{\mathbf{w}}$ for all $j\in [m]$.
% \end{lemma}

% \begin{proof}
% % chebyshev to upper bound probability of bad neuron, then
%     % hoeffding
% Since each $\mathbf{w}_j\sim \mathcal{N}(\mathbf{0}_d,\nu_{\mathbf{w}}^2\mathbf{I}_d)$, each $\|\mathbf{Mw}\|_2$, $\|\mathbf{M}_\perp \mathbf{w}\|_2$, and $\|\mathbf{w}\|_2$ are sub-gaussian with parameter $\nu_{\mathbf{w}}$, i.e.
% \begin{align}
%     \mathbb{P}_{\mathbf{w}_{j,:r}}[| \|\mathbf{w}_{j,:r}\|_2 - \nu_{\mathbf{w}}\sqrt{r}| \leq t] \leq e^{-c' t^2/\nu_{\mathbf{w}}^2}
% \end{align}
% Choosing $t = c'' \nu_{\mathbf{w}}\sqrt{\log(m)}$ and union bounding over all $j\in [m]$ completes the proof.
% \end{proof}


\subsection{General lemmas}


\begin{lemma} \label{lem:exp1}
Suppose $\mathbf{x} \sim \mathcal{N}(\mathbf{0}_d,\mathbf{I}_d)$. Then for any $\mathbf{w}\in \mathbb{R}^d$,
    $$\mathbb{E}_{\mathbf{x}}\left[
\sigma'(\mathbf{w}^\top \mathbf{x}) \mathbf{x}\right] = \sqrt{\frac{2}{\pi}} \frac{\mathbf{w}}{\|\mathbf{w}\|_2}.$$
\end{lemma}

\begin{proof}
 For any $\mathbf{u}: \mathbf{w}^\top\mathbf{u}=0$, we have
 \begin{align}
     \mathbf{u}^\top (\mathbb{E}_{\mathbf{x}}\left[
\sigma'(\mathbf{w}^\top \mathbf{x}) \mathbf{x}\right]) &= \mathbb{E}_{\mathbf{x}}\left[
\sigma'(\mathbf{w}^\top \mathbf{x}) \mathbf{u}^\top\mathbf{x}\right]\nonumber \\
&= \mathbb{E}_{\mathbf{x}}\left[
\sigma'(\mathbf{w}^\top \mathbf{x})\right]  \mathbb{E}_{\mathbf{x}}\left[\mathbf{u}^\top\mathbf{x}\right]\nonumber \\
&= 0
 \end{align}
 by the independence of orthogonal projections of isotropic Gaussian vectors. So, $\mathbb{E}_{\mathbf{x}}\left[
\sigma'(\mathbf{w}^\top \mathbf{x}) \mathbf{x}\right]$ is parallel to $\mathbf{w}$. Thus,
\begin{align}
    \mathbb{E}_{\mathbf{x}}\left[
\sigma'(\mathbf{w}^\top \mathbf{x}) \mathbf{x}\right] &= \frac{\mathbf{ww}^\top}{\|\mathbf{w}\|_2^2}  \mathbb{E}_{\mathbf{x}}\left[
\sigma'(\mathbf{w}^\top \mathbf{x}) \mathbf{x}\right]\nonumber \\
&= \frac{\mathbf{w}}{\|\mathbf{w}\|_2^2}  \mathbb{E}_{\mathbf{x}}\left[
\sigma'(\mathbf{w}^\top \mathbf{x}) \mathbf{w}^\top\mathbf{x}\right]\nonumber \\
&= \frac{\mathbf{w}}{\|\mathbf{w}\|_2^2}  \mathbb{E}_{\mathbf{x}}\left[
\sigma(\mathbf{w}^\top \mathbf{x}) \right]
\end{align}
where $\sigma(\mathbf{w}^\top \mathbf{x})$ is a half-normal random variable with parameter $\|\mathbf{w}\|_2$, so it has mean $\|\mathbf{w}\|_2\sqrt{\frac{2}{\pi}}$, completing the proof.
\end{proof}

\begin{lemma}
    \label{lem:exp-perp}
Suppose $\mathbf{x} \sim \mathcal{N}(\mathbf{0}_d,\mathbf{I}_d)$ and $\mathbf{M}_\perp \in \mathbb{O}^{(d-r)\times d}$ and $\mathbf{M} \in \mathbb{O}^{r \times d}$ such that $\mathbf{M}_{\perp}\mathbf{M}^\top = \mathbf{0}_{(d-r)\times r}$, i.e.  the rowspaces of $\mathbf{M}$ and $\mathbf{M}_{\perp}$ are orthogonal. Then for any $\mathbf{w}\in \mathbb{R}^d$,
\begin{align}
    \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} \; \sigma'(\mathbf{w}^\top \mathbf{x})  \right] = {\frac{1}{\sqrt{2\pi}} \exp\left(-\frac{(\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x})^2}{2} \right) }\frac{\mathbf{M}_\perp \mathbf{w} }{ \| \mathbf{M}_\perp \mathbf{w} \|_2} 
\end{align}
\end{lemma}

\begin{proof}
  We have
\begin{align}
    &\mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} \; \sigma'(\mathbf{w}^\top \mathbf{x})  \right]\nonumber \\
    &= \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} \; \sigma'(\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} + \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x})  \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} + \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} > 0 \right] \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}}[\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} + \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} > 0] \nonumber \\
    &= \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} \bigg|\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > | \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} |\right] \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}}[\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} >| \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}| ] \label{bh} 
\end{align}
where the last line follows by considering two cases: (i) $\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} <0$ and (ii) $\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} >0$.
If case (i) holds, then $ - \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} = |\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}|$ so  $\mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} + \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} > 0 \right]= \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} \bigg|\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > | \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} |\right]$ and 
$\mathbb{P}_{\mathbf{M}_\perp \mathbf{x}}[\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} + \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} > 0]=\mathbb{P}_{\mathbf{M}_\perp \mathbf{x}}[\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} >| \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}| ]$.
Alternatively, if case (ii) holds,  then by the law of total expectation,
\begin{align}
   &\mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} + \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} > 0 \right] \nonumber \\
   &= \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}  \right] \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}  |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > -\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} \right] \nonumber \\
   &\quad + \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} |\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}> \mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > -\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}  \right] \nonumber \\
   &\quad \quad \quad \quad \times \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}> \mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > -\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}  |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > -\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} \right]  \nonumber \\
   &= \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}  \right] \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}  |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > -\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} \right] \nonumber  \\
   &= \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > |\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}|  \right] \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}  |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > -\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} \right] \label{bnv}  \\
   &= \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > |\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}|  \right]\frac{ \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > |\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}|\right] }{ \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}} \left[\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > -\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} \right]}  \nonumber
\end{align}
where \eqref{bnv} follows since $\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} = |\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}| $. 
Now we return to \eqref{bh}. 
Note that
\begin{align}
&\mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} \bigg|\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > | \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} |\right] \nonumber \\
&=\mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} - 2 \sigma\left( -\frac{\mathbf{w}^\top \mathbf{M}_\perp^\top  }{ \| \mathbf{M}_\perp \mathbf{w} \|_2}\mathbf{M}_\perp \mathbf{x}\right)\frac{\mathbf{M}_\perp \mathbf{w} }{ \| \mathbf{M}_\perp \mathbf{w} \|_2} \bigg||\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x}| > | \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} |\right]
\end{align}
by the symmetry of the Gaussian distribution and the fact that $$\mathbf{M}_\perp \mathbf{x} - 2 \sigma\left( -\frac{\mathbf{w}^\top \mathbf{M}_\perp^\top  }{ \| \mathbf{M}_\perp \mathbf{w} \|_2}\mathbf{M}_\perp \mathbf{x}\right)\frac{\mathbf{M}_\perp \mathbf{w} }{ \| \mathbf{M}_\perp \mathbf{w} \|_2} $$ is the flip of $\mathbf{M}_\perp \mathbf{x}$ across the hyperplane with normal vector $\frac{\mathbf{w}^\top \mathbf{M}_\perp^\top  }{ \| \mathbf{M}_\perp \mathbf{w} \|_2}$ when $\mathbf{w}^\top \mathbf{M}_\perp^\top \mathbf{M}_\perp \mathbf{x} < - | \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} |$.
Using this, we obtain
\begin{align}
    &\mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} \sigma'(\mathbf{w}^\top \mathbf{x})  \right]\nonumber \\
    % &=  \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} \bigg|\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} > | \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} |\right] \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}}[\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x} >| \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}| ] \nonumber \\
    &= \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} - 2  \sigma\left( -\frac{\mathbf{w}^\top \mathbf{M}_\perp^\top  }{ \| \mathbf{M}_\perp \mathbf{w} \|_2}\mathbf{M}_\perp \mathbf{x}\right)\frac{\mathbf{M}_\perp \mathbf{w} }{ \| \mathbf{M}_\perp \mathbf{w} \|_2} \bigg| |\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}|  > |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x}| \right] \nonumber \\
    &\quad \quad \times \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}}\left[\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} > |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x}| \right]\nonumber \\
    % &\quad \quad \times  \nonumber \\
    &= 2\mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \sigma\left( -\frac{\mathbf{w}^\top \mathbf{M}_\perp^\top \mathbf{M}_\perp \mathbf{x} }{ \| \mathbf{M}_\perp \mathbf{w} \|_2}\right)\bigg| |\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} | > |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x}| \right]  \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}}\left[\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} > |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x}| \right] \frac{\mathbf{M}_\perp \mathbf{w} }{ \| \mathbf{M}_\perp \mathbf{w} \|_2}  \nonumber \\
    &=\mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \sigma\left( -\frac{\mathbf{w}^\top \mathbf{M}_\perp^\top \mathbf{M}_\perp \mathbf{x} }{ \| \mathbf{M}_\perp \mathbf{w} \|_2}\right)\bigg| \mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x}  < - |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x}| \right]  \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}}\left[\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} > |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x}| \right] \frac{\mathbf{M}_\perp \mathbf{w} }{ \| \mathbf{M}_\perp \mathbf{w} \|_2}  \nonumber \\
    % &\quad \quad \times \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}}\left[\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} > |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x}| \right] \nonumber \\
    &= \frac{\frac{1}{\sqrt{2\pi}} \exp(-(\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x})^2/2 ) }{\mathbb{P}_{\mathbf{M}_\perp \mathbf{x}}\left[\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} <- |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x}| \right]} \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}}\left[\mathbf{w}^\top \mathbf{M}_\perp^\top\mathbf{M}_\perp \mathbf{x} > |\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x}| \right] \frac{\mathbf{M}_\perp \mathbf{w} }{ \| \mathbf{M}_\perp \mathbf{w} \|_2}  \label{ddw} \\
    &= {\frac{1}{\sqrt{2\pi}} \exp(-(\mathbf{w}^\top \mathbf{M}^\top\mathbf{M}\mathbf{x})^2/2 ) }\frac{\mathbf{M}_\perp \mathbf{w} }{ \| \mathbf{M}_\perp \mathbf{w} \|_2}  \label{mn}
\end{align}
where \eqref{ddw} follows by the definition of the inverse Mills ratio.
\end{proof}


\begin{lemma} \label{lem:exp2}
For any function $f:\mathbb{R}^d\rightarrow \{-1,1\}$ such that $f(\mathbf{x}) = g(\mathbf{Mx})$ for some row-orthonormal matrix $\mathbf{M}\in \mathbb{O}^{r\times d}$ and some function $g: \mathbb{R}^r \rightarrow \{-1,1\}$ for all $\mathbf{x}\in \mathbb{R}^d$. Then for any vector $\mathbf{w} \in \mathbb{R}^d$,
\begin{align}
    \|\mathbb{E}_{\mathbf{x}}\left[
f(\mathbf{x}) \sigma'(\mathbf{w}^\top \mathbf{x}) \mathbf{x}\right] \|_2 \leq \frac{\sqrt{r}}{2}\left( 1 + \frac{\sqrt{\pi}}{2} \frac{\|\mathbf{Mw}\|_2}{\|\mathbf{M}_\perp\mathbf{w}\|_2} \right) +  \left( \frac{1 + \|\mathbf{Mw}\|_2^2 }{2\pi } \right)^{1/2}.
\end{align}
\end{lemma}

\begin{proof}
%     By Lemma \ref{lem:exp1}, we have $\mathbb{E}_{\mathbf{x}}\left[
% \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h\right] = \sqrt{\frac{2}{\pi}} \frac{w_{j,h}}{\|\mathbf{w}_j\|_2
% }$. Now, 
Let $\mathbf{M}_{\perp}\in \mathbb{O}^{(d-r)\times d}$ be a row-orthonormal matrix whose rowspace is orthogonal to that of $\mathbf{M}$. Using that $\mathbf{M}^\top\mathbf{M} + \mathbf{M}_\perp^\top\mathbf{M}_\perp = \mathbf{I}_d$ and $\mathbf{Mx}$ and $\mathbf{M}_{\perp}\mathbf{x}$ are independent standard normal multivariate random vectors,  we have 
\begin{align}
    \mathbb{E}_{\mathbf{x}}\left[f(\mathbf{x})
\sigma'(\mathbf{w}^\top \mathbf{x}) \mathbf{x}\right] 
% &=  
% \mathbb{E}_{\mathbf{x}}\left[g(\mathbf{Mx})
% \sigma'(\mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx} + \mathbf{w}^\top \mathbf{M}_\perp^\top \mathbf{M}_\perp \mathbf{x}) (\mathbf{M}^\top\mathbf{M}\mathbf{x} + \mathbf{M}_\perp^\top\mathbf{M}_\perp\mathbf{x})\right] \nonumber \\
&= \mathbb{E}_{\mathbf{x}}\left[g(\mathbf{Mx})
\sigma'(\mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx} + \mathbf{w}^\top \mathbf{M}_\perp^\top \mathbf{M}_\perp \mathbf{x}) \mathbf{M}^\top\mathbf{M}\mathbf{x} \right] \nonumber \\
&\quad + \mathbb{E}_{\mathbf{x}}\left[g(\mathbf{Mx})
\sigma'(\mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx} + \mathbf{w}^\top \mathbf{M}_\perp^\top \mathbf{M}_\perp \mathbf{x})  \mathbf{M}_\perp^\top\mathbf{M}_\perp\mathbf{x})\right] \nonumber \\
&= \underbrace{\mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx})\mathbb{E}_{\mathbf{M}_\perp\mathbf{x}}\left[
\sigma'(\mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx} + \mathbf{w}^\top \mathbf{M}_\perp^\top \mathbf{M}_\perp \mathbf{x})\right] \mathbf{M}^\top\mathbf{M}\mathbf{x} \right]}_{\circled{1}} \nonumber \\
&\quad + \underbrace{\mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx})
 \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}}\left[\sigma'(\mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx} + \mathbf{w}^\top \mathbf{M}_\perp^\top \mathbf{M}_\perp \mathbf{x})  \mathbf{M}_\perp^\top\mathbf{M}_\perp\mathbf{x})\right] \right]}_{\circled{2}} \nonumber 
\end{align}
so  $ \|   \mathbb{E}_{\mathbf{x}}\left[f(\mathbf{x})
\sigma'(\mathbf{w}^\top \mathbf{x}) \mathbf{x}\right]\|_2 \leq \left\| \circled{1} \right\|_2 +  \left\| \circled{2} \right\|_2$ by the triangle inequality.  First we consider $\circled{1}$. We have
\begin{align}
& \mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx})\mathbb{E}_{\mathbf{M}_\perp\mathbf{x}}\left[
\sigma'(\mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx} + \mathbf{w}^\top \mathbf{M}_\perp^\top \mathbf{M}_\perp \mathbf{x})\right] \mathbf{M}^\top\mathbf{M}\mathbf{x} \right] \nonumber \\
 &=  \mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx})\mathbb{P}_{\mathbf{M}_\perp\mathbf{x}}\left[
\mathbf{w}^\top \mathbf{M}_\perp^\top \mathbf{M}_\perp \mathbf{x} > - \mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx}\right] \mathbf{M}^\top\mathbf{M}\mathbf{x} \right] \nonumber \\
  &=  \mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx})\left(\frac{1}{2} + \frac{1}{2}\erf\left( \frac{\mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx} }{  \sqrt{2}\|\mathbf{M}_{\perp}\mathbf{w}\|_2  } \right) \right)\mathbf{M}^\top\mathbf{M}\mathbf{x} \right]  \label{hnfv} \\
 &= \frac{1}{2}\mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx}) \mathbf{M}^\top\mathbf{M}\mathbf{x} \right]  + \frac{1}{2}\mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx}) \erf\left( \frac{\mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx} }{  \sqrt{2}\|\mathbf{M}_{\perp}\mathbf{w}\|_2  }  \right)\mathbf{M}^\top\mathbf{M}\mathbf{x} \right] \nonumber
\end{align}
where \eqref{hnfv} is due to the Gaussian CDF. Thus by the triangle inequality,
\begin{align}
    \left\|\circled{1}\right\|_2 &\leq  \frac{1}{2}\left\|\mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx}) \mathbf{M}^\top\mathbf{M}\mathbf{x} \right] \right\|_2 + \frac{1}{2}\left\|\mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx}) \erf\left( \frac{\mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx} }{  \sqrt{2}\|\mathbf{M}_{\perp}\mathbf{w}\|_2  }  \right)\mathbf{M}^\top\mathbf{M}\mathbf{x}\right] \right\|_2 \label{dfg} \end{align}
For the first term,
\begin{align}
    \left\|\mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx}) \mathbf{M}^\top\mathbf{M}\mathbf{x} \right] \right\|_2 &\leq \mathbb{E}_{\mathbf{Mx}}\left[\left\|g(\mathbf{Mx}) \mathbf{M}^\top\mathbf{M}\mathbf{x}\right\|_2   \right] \label{jen1} \\
    &= \mathbb{E}_{\mathbf{Mx}}\left[\left\| \mathbf{M}\mathbf{x}\right\|_2   \right] \nonumber \\
    &\leq  \mathbb{E}_{\mathbf{Mx}}\left[\left\| \mathbf{M}\mathbf{x}\right\|_2^2   \right]^{1/2} \label{jen2} \\
    &= \sqrt{r}  \label{bhg}
\end{align}
where \eqref{jen1} and \eqref{jen2} follow by Jensen's inequality.
For the second term in \eqref{dfg}, we have
\begin{align}
&\left\|\mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx}) \erf\left( \frac{\mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx} }{  \sqrt{2}\|\mathbf{M}_{\perp}\mathbf{w}\|_2  }  \right)\mathbf{M}^\top\mathbf{M}\mathbf{x}\right] \right\|_2  \nonumber \\
    &\leq \mathbb{E}_{\mathbf{Mx}}\left[\left\|g(\mathbf{Mx}) \erf\left( \frac{\mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx} }{  \sqrt{2}\|\mathbf{M}_{\perp}\mathbf{w}\|_2  }  \right)\mathbf{M}^\top\mathbf{M}\mathbf{x}\right\|_2\right]  \label{kiy} \\
    &\leq  \left(\mathbb{E}_{\mathbf{Mx}}\left[\left|g(\mathbf{Mx}) \erf\left( \frac{\mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx} }{  \sqrt{2}\|\mathbf{M}_{\perp}\mathbf{w}\|_2  }  \right) \right|^2 \right] \mathbb{E}_{\mathbf{Mx}}\left[ \left\|\mathbf{M}^\top\mathbf{M}\mathbf{x}\right\|_2^2\right]\right)^{1/2}  \label{fv} \\
    &= {\sqrt{r}} \mathbb{E}_{\mathbf{Mx}}\left[\left|g(\mathbf{Mx}) \erf\left( \frac{\mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx} }{  \sqrt{2}\|\mathbf{M}_{\perp}\mathbf{w}\|_2  }  \right) \right|^2 \right]^{1/2}  \label{fv} \\
    &\leq {\sqrt{r}} \mathbb{E}_{\mathbf{Mx}}\left[\left( \frac{\sqrt{\pi}\mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx} }{ 2\|\mathbf{M}_{\perp}\mathbf{w}\|_2  }  \right) ^2 \right]^{1/2}  \label{xs} \\
    &= \frac{\sqrt{\pi r}}{2} \frac{\|\mathbf{Mw}\|_2}{\|\mathbf{M}_\perp\mathbf{w}\|_2} \label{xa}
\end{align}
where \eqref{kiy} follows by Jensen's inequality, \eqref{fv} follows by the Cauchy-Schwarz inequality, and \eqref{xs} follows since $|\erf(x)|\leq |\sqrt{\pi/2} \; x|$. Combining \eqref{dfg}, \eqref{bhg} and \eqref{xa} yields
\begin{align}
    \left\|\circled{1}\right\|_2 \leq \frac{\sqrt{r}}{2}\left( 1 + \frac{\sqrt{\pi}}{2} \frac{\|\mathbf{Mw}\|_2}{\|\mathbf{M}_\perp\mathbf{w}\|_2} \right)
\end{align}

Next we consider $\circled{2}$. We have
\begin{align}
&\mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx})
 \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}}\left[\sigma'(\mathbf{w}^\top \mathbf{M}^\top  \mathbf{Mx} + \mathbf{w}^\top \mathbf{M}_\perp^\top \mathbf{M}_\perp \mathbf{x})  \mathbf{M}_\perp^\top\mathbf{M}_\perp\mathbf{x})\right] \right] \nonumber \\
 &= \frac{1}{\sqrt{2\pi}} \mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx})
 \exp\left( -\frac{(\mathbf{w}^\top \mathbf{M}^\top \mathbf{Mx})^2 }{2} \right) 
  \right] \frac{\mathbf{M}_\perp^\top \mathbf{M}_\perp \mathbf{w}}{\| \mathbf{M}_\perp \mathbf{w}\|_2 } \label{hnv}  
\end{align}
by Lemma \ref{lem:exp-perp}, thus
\begin{align}
\left\|\circled{2} \right\|_2 = \frac{1}{\sqrt{2\pi}} \left|\mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx})
 \exp\left( -\frac{(\mathbf{w}^\top \mathbf{M}^\top \mathbf{Mx})^2 }{2} \right) 
  \right]\right|.
  \end{align}
  Next we upper bound $\left|\mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx})
 \exp\left( -\frac{(\mathbf{w}^\top \mathbf{M}^\top \mathbf{Mx})^2 }{2} \right) 
  \right]\right|$. We have
\begin{align}
     &\left|\mathbb{E}_{\mathbf{Mx}}\left[g(\mathbf{Mx})
 \exp\left( -\frac{(\mathbf{w}^\top \mathbf{M}^\top \mathbf{Mx})^2 }{2} \right) 
  \right]\right| \nonumber \\
  &\leq  \mathbb{E}_{\mathbf{Mx}}\left[
 \exp\left( -\frac{(\mathbf{w}^\top \mathbf{M}^\top \mathbf{Mx})^2 }{2} \right) 
  \right] \label{tgd} \\
  &=  \int_{\mathbb{R}^r} \frac{1}{(2\pi)^{r/2} } \exp\left(- \frac{( \mathbf{w}^\top \mathbf{M}^\top \mathbf{Mx} )^2}{2} - \frac{\mathbf{x}^\top \mathbf{M}^\top \mathbf{Mx}}{2} \right) d \mathbf{Mx} \label{wes} \\
  &= \int_{\mathbb{R}^r} \frac{1}{(2\pi)^{r/2} } \exp\left(- \frac{\mathbf{x}^\top \mathbf{M}^\top  \left(  \mathbf{I}_r + \mathbf{Mww}^\top \mathbf{M}^\top \right) \mathbf{Mx}}{2} \right) d \mathbf{Mx} \nonumber \\
  &= {\text{det}( \mathbf{I}_r + \mathbf{Mww}^\top \mathbf{M}^\top )^{1/2} }\nonumber \\
  &\quad \times \int_{\mathbb{R}^r} \frac{1}{(2\pi)^{r/2} \text{det}( \mathbf{I}_r + \mathbf{Mww}^\top \mathbf{M}^\top )^{1/2} } \exp\left(- \frac{\mathbf{x}^\top \mathbf{M}^\top  \left(  \mathbf{I}_r + \mathbf{Mww}^\top \mathbf{M}^\top \right) \mathbf{Mx}}{2} \right) d \mathbf{Mx} \label{gz} \\
  &= {\text{det}( \mathbf{I}_r + \mathbf{Mww}^\top \mathbf{M}^\top )^{1/2} } \nonumber \\
  % &= {\left( 1 + \mathbf{w}^\top \mathbf{M}^\top\mathbf{Mw} \right)^{1/2} } \label{wqp} \\
  &= \left( 1 + \|\mathbf{Mw}\|_2^2 \right)^{1/2}\label{wqp} 
\end{align}
where \eqref{tgd} follows since $\exp()$ is positive, \eqref{wes} follows since $\mathbf{w}^\top \mathbf{M}^\top \mathbf{Mx}$ is a Gaussian random variable with mean zero and variance $\|\mathbf{Mw}\|_2^2$, and \eqref{gz} follows due to  the multivariate normal distribution, and \eqref{wqp} follows by the matrix determinant lemma. Therefore,
\begin{align}
  \left\| \circled{2} \right\|_2 &\leq \left( \frac{1 + \|\mathbf{Mw}\|_2^2 }{2\pi } \right)^{1/2},
\end{align}
completing the proof.
\end{proof}



% \begin{align}
%     \mathbb{E}_{\mathbf{x}}\left[f_i(\mathbf{x})
% \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h\right] &= \mathbb{E}_{\mathbf{x}}\left[
% \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h | f_i(\mathbf{x}) =1 \right]\mathbb{P}_{\mathbf{x}}(f_i(\mathbf{x})=1) - \mathbb{E}_{\mathbf{x}}\left[
% \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h | f_i(\mathbf{x}) =-1 \right]\mathbb{P}_{\mathbf{x}}(f_i(\mathbf{x})=-1)\nonumber \\
% &\leq   \mathbb{E}_{\mathbf{x}}\left[f_i(\mathbf{x})
% \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h\right] &= \mathbb{E}_{\mathbf{x}}\left[
% \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h | f_i(\mathbf{x}) =1 \right]\mathbb{P}_{\mathbf{x}}(f_i(\mathbf{x})=1) - \mathbb{E}_{\mathbf{x}}\left[
% \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h | f_i(\mathbf{x}) =-1 \right]\mathbb{P}_{\mathbf{x}}(f_i(\mathbf{x})=-1)\nonumber \\
% \end{align}





\subsection{Finite-task and finite-sample concentration results}


\begin{lemma}[Initialization I] \label{lem:init}
    % With probability at least $1-\delta$, all neuron weights satisfy:
    % \begin{align}
    %     \leq \|\mathbf{w}_{j}^0\|_2 \leq  \nonumber \\
    % \end{align}
    % a constant fraction of neurons are good, in the sense that 

    % 1. error vector is less than c/k, other errors are sufficiently small

    % 2. w|| is large enough

    % 3. need bias in an interval like [rt(r) - 1/rt(r), rt(r)]. which occurs with prob 1/rt(r). too small. but still a good network exists. so can jointly optimize a,b. to get a good network...no. not jointly convex in a,b

    % or, make different generalization arguement... 
    For any $\delta\in (0,1)$, define the set 
    \begin{align}
        \mathcal{G}_{\mathbf{w}}(\delta) \coloneqq \big\{&\mathbf{w}\in \mathbb{R}^d :  \|\mathbf{M}\mathbf{w}\|_2 \leq c \nu_{\mathbf{w}}( \sqrt{r} + \sqrt{\log(m/\delta)}), \nonumber \\
        &\quad c\nu_{\mathbf{w}}(\sqrt{d-r} - \sqrt{\log(m/\delta)}) \leq \|\mathbf{M}_\perp\mathbf{w} \|_2 \leq c \nu_{\mathbf{w}}(\sqrt{d-r} + \sqrt{\log(m/\delta)}), \nonumber \\
        &\quad c\nu_{\mathbf{w}}(\sqrt{d} - \sqrt{\log(m/\delta)}) \leq \|\mathbf{w} \|_2 \leq c\nu_{\mathbf{w}}(\sqrt{d} + \sqrt{\log(m/\delta)}) \big\}
    \end{align} for an absolute constant $c$.
    Then with probability at least $1-\delta$, $\mathbf{w}_{j}\in \mathcal{G}_{\mathbf{w}}(\delta)$ for all $j\in [m]$.
\end{lemma}

\begin{proof}
% chebyshev to upper bound probability of bad neuron, then
    % hoeffding
Since each $\mathbf{w}_j\sim \mathcal{N}(\mathbf{0}_d,\nu_{\mathbf{w}}^2\mathbf{I}_d)$, each $\|\mathbf{M}\mathbf{w}_j\|_2$, $\|\mathbf{M}_\perp\mathbf{w}_j\|_2$, and $\|\mathbf{w}_j\|_2$ are sub-Gaussian with parameters $\nu_{\mathbf{w}}\sqrt{r}$, $\nu_{\mathbf{w}}\sqrt{d-r}$, and $\nu_{\mathbf{w}}\sqrt{d}$. That is, 
\begin{align}
    \mathbb{P}_{\mathbf{w}_{j}}[| \|\mathbf{Mw}_{j}\|_2 - \nu_{\mathbf{w}}\sqrt{r}| \leq t] \leq e^{-c' t^2/\nu_{\mathbf{w}}^2}
\end{align}
for any $t>0$, and likewise for $ \|\mathbf{M}_\perp\mathbf{w}_{j}\|_2$ and  $\|\mathbf{w}_{j}\|_2$ (with $ \nu_{\mathbf{w}}\sqrt{r}$ replaced by $ \nu_{\mathbf{w}}\sqrt{d-r}$ and $ \nu_{\mathbf{w}}\sqrt{d}$, respectively).
Choosing $t = c'' \nu_{\mathbf{w}}\sqrt{\log(m/\delta)}$ and union bounding over all $j\in [m]$ completes the proof.
\end{proof}

\begin{lemma}[Initialization II] \label{lem:init2}
    % With probability at least $1-\delta$, all neuron weights satisfy:
    % \begin{align}
    %     \leq \|\mathbf{w}_{j}^0\|_2 \leq  \nonumber \\
    % \end{align}
    % a constant fraction of neurons are good, in the sense that 

    % 1. error vector is less than c/k, other errors are sufficiently small

    % 2. w|| is large enough

    % 3. need bias in an interval like [rt(r) - 1/rt(r), rt(r)]. which occurs with prob 1/rt(r). too small. but still a good network exists. so can jointly optimize a,b. to get a good network...no. not jointly convex in a,b

    % or, make different generalization arguement... 
Suppose $m >r$. For an absolute constant $c$ and any $\delta\in (0,1)$,
    \begin{align}
        \sigma_{\min}(\mathbf{M}\mathbf{W}^0) \geq \nu_{\mathbf{w}}\sqrt{m}\left(1 - c\frac{\sqrt{r} + \sqrt{\log(1/\delta)}}{\sqrt{m}}  \right)
    \end{align}
    with probability at least $1-\delta$.
\end{lemma}

\begin{proof}
% Since each $\mathbf{w}_j\sim \mathcal{N}(\mathbf{0}_d,\nu_{\mathbf{w}}^2\mathbf{I}_d)$, each $\|\mathbf{Mw}\|_2$, $\|\mathbf{M}_\perp \mathbf{w}\|_2$, and $\|\mathbf{w}\|_2$ are sub-gaussian with parameter $\nu_{\mathbf{w}}$, i.e.
% \begin{align}
%     \mathbb{P}_{\mathbf{w}_{j,:r}}[| \|\mathbf{w}_{j,:r}\|_2 - \sqrt{r}| \leq t] \leq e^{-c' t^2/\nu_{\mathbf{w}}^2}
% \end{align}
% Choosing $t = c'' \nu_{\mathbf{w}}\sqrt{\log(m)}$ and union bounding over all $j\in [m]$ completes the proof.
The result follows from the fact that each row of $\mathbf{W}^0$ is drawn independently from $\mathcal{N}(\mathbf{0}_d,\nu_{\mathbf{w}}^2\mathbf{I}_d)$, so each of the $r$ rows of $\mathbf{M}\mathbf{W}^0$ are drawn i.i.d. from $\mathcal{N}(\mathbf{0}_m,\nu_{\mathbf{w}}^2\mathbf{I}_m)$ (recalling that the rows of $\mathbf{M}$ are orthogonal, so $\mathbf{u}_i^\top \mathbf{w}_j$ and $\mathbf{u}_{i'}^\top \mathbf{w}_j$ are independent for any two distinct rows $\mathbf{u}_i$ and $\mathbf{u}_{i'}$ of $\mathbf{M}$). A standard (sub-)Gaussian matrix concentration  inequality yields the result (e.g. Equation 4.21 in \cite{vershynin2018high}).
\end{proof}

\begin{lemma}[Initialization III] \label{lem:init3}
For an absolute constant $c$ and any $\delta \in (0,1)$,
    \begin{align}
        \|\mathbf{W}^0\|_2 \leq \nu_{\mathbf{w}}\sqrt{m}\left(1 + \frac{\sqrt{d}+\sqrt{\log(1/\delta)}}{\sqrt{m}}\right)
    \end{align}
    for some absolute constant with probability at least $1-\delta$.
\end{lemma}
\begin{proof}
    As in Lemma \ref{lem:init2}, the proof follows by standard (sub-)Gaussian matrix concentration (e.g. Equation 4.21 in \cite{vershynin2018high}).
\end{proof}

% \begin{lemma}
%     since the number of neurons is large enough, this set covers all $2^r$ vertices
% \end{lemma}

% \begin{proof}
%     balls and bins. but being in the set changes the distribution? should still work.
% \end{proof}

% We use $\hat{\mathbb{E}}_{\mathbf{x}\sim \mathcal{D}}[h(\mathbf{x})]$ to denote the empirical mean of $h(\mathbf{x})$ over the data in $\mathcal{D}$.
\begin{lemma}\label{lem:all}
    For any $\delta\in (0,1)$ define the event $E_{\mathbf{w}}(\delta)$ as follows: 
\begin{align}
    E_{\mathbf{w}}(\delta) :=\Bigg\{ &\mathbf{w}_j^0 \in \mathcal{G}_{\mathbf{x}}(\delta), \quad 
     \sigma_{\min}(\mathbf{M}\mathbf{W}^0) \geq \nu_{\mathbf{w}}\sqrt{m}\left(1 - c\frac{\sqrt{r} - \sqrt{\log(1/\delta)}}{\sqrt{m}}  \right),\nonumber \\
     &\|\mathbf{W}^0\|_2 \leq \nu_{\mathbf{w}}\sqrt{m}\left(1 + \frac{\sqrt{d}+\sqrt{\log(1/\delta)}}{\sqrt{m}}\right)
    \Bigg\}.
\end{align}
Then $\mathbb{P}(E_{\mathbf{w}}(\delta))\geq 1 - 3\delta$. 
\end{lemma}

\begin{proof}
    The proof follows immediately from Lemmas \ref{lem:init}, \ref{lem:init2}, \ref{lem:init3} and a union bound.
\end{proof}

Next we begin to analyze the first gradient-based update of the algorithm.
Throughout, let $ \hat{\mathcal{D}}_{i,\mathbf{a}} = \{(\mathbf{x}_{i,k}, f_i(\mathbf{x}_{i,k}))\}_{k=1}^{n_1}$ and $ \hat{\mathcal{D}}_{i,\mathbf{W}} = \{(\mathbf{x}_{i,l}, f_i(\mathbf{x}_{i,l}))\}_{l=1}^{n_2}$, where all samples are drawn i.i.d. from $\mathcal{D}_i$, for each $i \in [T]$.

\begin{lemma}\label{lem:a1}
    Let $\lambda_{\mathbf{a}} = \frac{1}{\eta}$ and $\mathbf{x}\sim \mathcal{N}(\mathbf{0}_d,\mathbf{I}_d)$. On the first iteration of the multitask learning algorithm described in Section \ref{sec:alg}, the locally updated head for task $i$ is:
    \begin{align}
        \mathbf{a}_{i}^1 = \frac{\eta}{n_1} 
        \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) {\sigma}(\mathbf{W}^0\mathbf{x}_{i,k}) 
    \end{align}
    for all tasks $i\in [T]$.
\end{lemma}

\begin{proof}
% For ease of notation we let $\mathbf{a}_i = \mathbf{a}_i^0$. 
% and $\hat{\mathbb{E}}_{\mathbf{x}\sim \hat{\mathcal{D}}_{i,\mathbf{a}}}[g(\mathbf{x})]$ denote the empirical mean of $g$ on samples in $\hat{\mathcal{D}}_{i,\mathbf{a}}$. 
Since $\mathbf{a}_{i}^0 = \mathbf{0}_m$ for all $i$,
$(\mathbf{a}_{i}^0)^\top  \sigma(\mathbf{W}^0\mathbf{x} + \mathbf{b}^0)=0$ for all $\mathbf{x}$ and $i$.
Therefore, 
$\max(1 - f_{i}(\mathbf{x})( \mathbf{a}_i^0)^\top  \sigma(\mathbf{W}^0\mathbf{x} + \mathbf{b}^0) , 0) = 1 - f_{i}(\mathbf{x}) (\mathbf{a}_i^0)^\top  \sigma(\mathbf{W}^0\mathbf{x} )$, and
\begin{align} %_{\mathbf{a},0}
\mathbf{a}_{i}^1 &= \mathbf{a}_i^0 - \eta \nabla_{\mathbf{a}} \hat{\mathcal{L}}_i(\mathbf{W}^0,\mathbf{b}^0,\mathbf{a}_i^0; \hat{\mathcal{D}}_{i,\mathbf{a}}) \nonumber \\
&= %(1 - \eta \lambda_{\mathbf{a}}) \mathbf{a}_i - 
-\frac{\eta}{n_1} \sum_{k=1}^{n_1}\nabla_{\mathbf{a}} ( \max(1 - f_{i}(\mathbf{x}_{i,k}) (\mathbf{a}_i^0)^\top  \sigma(\mathbf{W}^0\mathbf{x}_{i,k} + \mathbf{b}^0) , 0) )\nonumber \\
&= %(1 - \eta \lambda_{\mathbf{a}}) \mathbf{a}_i - 
-\frac{\eta}{n_1} \sum_{k=1}^{n_1}\nabla_{\mathbf{a}} (1 - f_{i}(\mathbf{x}_{i,k}) (\mathbf{a}_i^0)^\top  \sigma(\mathbf{W}^0\mathbf{x}_{i,k} + \mathbf{b}^0)  )\nonumber \\
% -\eta \nabla_{\mathbf{a}} \hat{\mathbb{E}}_{\mathbf{x}\sim \hat{\mathcal{D}}_{i, \mathbf{a}}}[ 1 - f_{i}(\mathbf{x}) \mathbf{a}_i^\top  \sigma(\mathbf{W}^0\mathbf{x}) ]\nonumber \\
&= %(1 - \eta \lambda_{\mathbf{a}}) \mathbf{a}_i + 
\frac{\eta}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k})  \sigma(\mathbf{W}^0\mathbf{x}_{i,k})  \nonumber 
% \eta \hat{\mathbb{E}}_{\mathbf{x}\sim \hat{\mathcal{D}}_{i, \mathbf{a}}}[ f_{i}(\mathbf{x}) \sigma(\mathbf{W}^0\mathbf{x} ) ] \nonumber %\\  %\label{sym} \\
% &= \eta \hat{\mathbb{E}}_{\mathbf{x}\sim \hat{\mathcal{D}}_{i,\mathbf{a}}} [f_{i}(\mathbf{x}) \sigma(\mathbf{W}^0\mathbf{x} + \mathbf{b}^0) ]  \label{lam}
\end{align}
where in the last equality we have used $\mathbf{b}^0= \mathbf{0}_m$ by choice of initialization.
% where \eqref{sym} follows by the symmetric initialization and \eqref{lam} follows by choice of $\lambda_{\mathbf{a}}$.
\end{proof}


% \begin{lemma}
%     \label{lem:mag_a}
    
% \end{lemma}
% \begin{proof}
    
% \end{proof}

Next, we substitute the updated heads in the global empirical loss. Since the gradient computation for the update of $\mathbf{W}$ does not backpropagate through the update of the heads,  we use $\bar{\sigma}(\cdot)$ to denote the stop-gradient ReLU activation, meaning all model parameters inside are treated as constants for the purposes of later gradient updates. In particular, from Lemma \ref{lem:a1} we have
\begin{align}
        \mathbf{a}_{i}^1 = \frac{\eta}{n_1} 
        \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) {\sigma}(\mathbf{W}^0\mathbf{x}_{i,k}) \label{jkj}
    \end{align}
    for all $i \in [T]$.
\begin{lemma}\label{lem:upd_loss}
    After updating the heads on the first iteration, the empirical loss averaged across the task datasets $\{\hat{\mathcal{D}}_{i,\mathbf{W}}\}_{i=1}^T$ used for updating the neuron weights is given by
        \begin{align}
        \hat{\mathcal{L}}(\mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{i}^1 \}_{i=1}^T;\{\hat{\mathcal{D}}_{i,\mathbf{W}}\}_{i=1}^T) &\coloneqq \frac{1}{T}\sum_{i=1}^T \hat{\mathcal{L}}_i(\mathbf{W}^0, \mathbf{b}^0, \mathbf{a}_{i}^1 ;\hat{\mathcal{D}}_{i,\mathbf{W}}) \nonumber \\
&=  1 -   
\frac{\eta}{T n_1 n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1} 
f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\bar{\sigma}(\mathbf{W}^0\mathbf{x}_{i,k})^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l})   \nonumber \\
&\quad - \frac{1}{T n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}    \chi\left\{ \eta f_{i}(\mathbf{x}_{i,l}) \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1\right\}   \nonumber \\
&\quad \quad \quad \quad \quad \quad \quad \; \times  \left( 1 - \eta f_{i}(\mathbf{x}_{i,l}) \left(\frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{W}^0\mathbf{x}_{i,k})\right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) \right)  \nonumber 
    \end{align}
\end{lemma}

\begin{proof}
First, by the fact that $\mathbf{b}^0 = \mathbf{0}_m$ by choice of initialization, we have
\begin{align}
    \hat{\mathcal{L}}(\mathbf{W}^0,\mathbf{b}^0,\{\mathbf{a}^1_{i}\}_{i=1}^T; \{\hat{\mathcal{D}}_{i,\mathbf{W}}\}_{i=1}^T) 
   &= \frac{1}{T} \sum_{i=1}^T \hat{\mathcal{L}}_i(\mathbf{W}^0,\mathbf{b}^0,\{\mathbf{a}_{i}^1\}_{i=1}^T; \hat{\mathcal{D}}_{i,\mathbf{W}} )
    \nonumber \\
    &=\frac{1}{Tn_2 } \sum_{i=1}^T \sum_{l=1}^{n_2}   \max\left( 1- f_i(\mathbf{x}_{i,l}) (\mathbf{a}_i^1)^\top\sigma(\mathbf{W}^0\mathbf{x}_{i,l}), 0 \right) 
    \nonumber \\
    &= \frac{1}{Tn_2 } \sum_{i=1}^T \sum_{l=1}^{n_2}   \chi\left\{ f_i(\mathbf{x}_{i,l})  (\mathbf{a}_i^1)^\top\sigma(\mathbf{W}^0\mathbf{x}_{i,l}) < 1   \right\}
    \left( 1- f_i(\mathbf{x}_{i,l}) (\mathbf{a}_i^1)^\top\sigma(\mathbf{W}^0\mathbf{x}_{i,l}) \right)  \nonumber\\
    &= 1 - \frac{1}{Tn_2 } \sum_{i=1}^T \sum_{l=1}^{n_2}  
     f_i(\mathbf{x}_{i,l}) (\mathbf{a}_i^1)^\top\sigma(\mathbf{W}^0\mathbf{x}_{i,l})  \nonumber \\
    &\quad -  \frac{1}{Tn_2 } \sum_{i=1}^T \sum_{l=1}^{n_2} \chi\left\{ f_i(\mathbf{x}_{i,l})  (\mathbf{a}_i^1)^\top\sigma(\mathbf{W}^0\mathbf{x}_{i,l}) > 1   \right\} \left( 1- f_i(\mathbf{x}_{i,l}) (\mathbf{a}_i^1)^\top\sigma(\mathbf{W}^0\mathbf{x}_{i,l}) \right) \nonumber %  \nonumber \\
    % &= \frac{1}{Tn_2 } \sum_{i=1}^T \sum_{l=1}^{n_2}  \E_{\mathbf{x} }  \left[ \max\left( 1- (\mathbf{a}_i^1)^\top\sigma(\mathbf{W}^0\mathbf{x}_{i,l}), 0 \right) \right]  \nonumber \\
%     &= \E_{\mathbf{x} }  \left[ \max\left( 1- \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}'} [ f_{i}(\mathbf{x}') g(\mathbf{x}';\mathbf{W}^0,\mathbf{b}^0 ) ]^\top g(\mathbf{x}; \mathbf{W}^0,\mathbf{b}^0)  , 0 \right) 
% %     \frac{1}{n_2}\sum_{j=1}^{n_2}\max \left(1 - y_{i,j} \left(\frac{1}{\lambda_{1}n_1}\sum_{j'=1}^{n_1}\bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})  \right)^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}), 0\right) \right] \nonumber\\
% % &= 1 -  \E_{i }  \left[ \frac{1}{\lambda_{1} n_1n_2}\sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})
% \right] \label{14} \nonumber \\
% &=\frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) <1\right\} \nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - \etaf_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber \\
% &=  1 -   \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[   \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right) \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})  \right]  \nonumber \\
% &\quad + \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\right\} \nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - \eta f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber 
\end{align}
% Next, using the computation of each $\mathbf{a}_{i}^1$ from Lemma \ref{lem:a1}, we have
% \begin{align}
% \end{align}
Substituting the value of $\mathbf{a}_i^1$ from \eqref{jkj} completes the proof.
\end{proof}

Next we show that after one update of the heads, the model predictions are still close to zero, so $\max()$ in the hinge loss is mostly inactive.
\begin{lemma}
    \label{lem:err_a} Suppose $\nu_{\mathbf{w}}^2 = O( \frac{1}{\eta^2 dm\log(T) (d+m)} )$.
    With probability at least $1 -\delta$, 
    \begin{align}
    &\frac{\eta}{T n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}    \chi\left\{ \eta f_{i}(\mathbf{x}_{i,l}) \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) {\sigma}'(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1\right\}\nonumber \\
    &=\eta O\left(  \exp \left( -\frac{ c }{\eta^2  \nu_{\mathbf{w}}^2 {m\log(T/\delta)}({d} + {\log(m/\delta)}) ({d} + {m} )} \right)\right) + \eta \; O\left(  \frac{  \sqrt{\log(1/\delta)} }{ \sqrt{Tn_2} } \right) 
    % \eta m\;  O\left( \max_{j\in [m]}  \exp \left(-\frac{ {1}}{ c\eta m \|\mathbf{w}_j\|_2^2 }     \right) \right)  +   \eta O\left(  \frac{  1 }{ \sqrt{Tn_2} } \right)
    % &=  \eta \; O(  \exp (- m \max_{j\in [m]}(\|\mathbf{w}_j\|_2^2) /(2\eta^2) ))  +O\left( \frac{\eta \sqrt{\log(m)} }{\sqrt{Tn_2}}\right)
\end{align}
for an absolute constant $c$.
\end{lemma}


\begin{proof} 
Consider any fixed $\mathbf{W}^0$ satisfying $E_{\mathbf{w}}(\delta_1)$ for $\delta_1\in (0,1)$, 
% such that $\delta_1 = \Omega(me^-d)$, 
which occurs with probability at least $1-3 \delta_1$ by Lemma \ref{lem:all}. 
For ease of notation we replace $\mathbf{w}_j^0$ with $\mathbf{w}_j.$ 
Recall that 
\begin{align}
  \eta f_{i}(\mathbf{x}_{i,l}) \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) {\sigma}'(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l})  &=    f_{i}(\mathbf{x}_{i,l}) (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) 
\end{align}
by the computation of $\mathbf{a}_i^1$ in Lemma \ref{lem:a1}.
For any fixed $f_i$ and fixed $\mathbf{a}_i^1$, $  \chi\left\{  f_{i}(\mathbf{x}_{i,l}) (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1\right\}$ is a Bernoulli random variable with parameter
\begin{align}
    &\mathbb{P}_{\mathbf{x_{i,l}}}\left(  f_{i}(\mathbf{x}_{i,l}) (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1 \right) \nonumber \\ %&\leq \nonumber \\
    % &= \mathbb{P}_{\mathbf{x_{i,l}}}\left( f_{i}(\mathbf{x}_{i,l}) \sum_{j=1}^m a_{i,j} \sigma(\mathbf{w}_j^\top\mathbf{x}_{i,l}) > \frac{1}{\eta} \right) \nonumber \\
    % &\leq \mathbb{P}_{\mathbf{x_{i,l}}}\left(  \left| \sum_{j=1}^m a_{i,j} \sigma(\mathbf{w}_j^\top\mathbf{x}_{i,l}) \right| > \frac{1}{\eta \|\mathbf{a}_i^1\|_2} \right) \label{aaq} \\
    &\leq \mathbb{P}_{\mathbf{x}_{i,l}}\left(  \left| (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) \right| > {1}{ } \right) \label{aaq}\\
    &\leq \mathbb{P}_{\mathbf{x}_{i,l}}\left(  \left| (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) - \mathbb{E}_{\mathbf{x}_{i,l}}[(\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l})] \right| > {1}{} -  \mathbb{E}_{\mathbf{x}_{i,l}}[(\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l})]  \right) \label{aaaq} \\
    &\leq 2 \exp \left( -\frac{ \left(1 -  \mathbb{E}_{\mathbf{x}_{i,l}}[(\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l})] \right)^2 }{  c\|\mathbf{a}_i^1\|_2^2 \|\mathbf{W}_0\|_2^2 } \right) \nonumber \\
    &\leq 2 \exp \left( -\frac{ \left( 1 -  \|\mathbf{a}_i^1\|_2 \|\mathbf{W}^0\|_2 \right)^2 }{  c\|\mathbf{a}_i^1\|_2^2 \|\mathbf{W}_0\|_2^2 } \right) \nonumber \\
    &\leq 2 \exp \left( -\frac{  1 -  2\|\mathbf{a}_i^1\|_2 \|\mathbf{W}^0\|_2 }{  c\|\mathbf{a}_i^1\|_2^2 \|\mathbf{W}_0\|_2^2 } \right) \nonumber \\
    &=: \gamma_i \label{gmm}
\end{align}
for some absolute constant $c$, where \eqref{aaq} follows since $ f_{i}(\mathbf{x}_{i,l}) \in \{-1,1\}$, and \eqref{aaaq} follows since $(\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) - \mathbb{E}_{\mathbf{x}_{i,l}}[(\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l})]$ is sub-Gaussian with mean $0$ and variance $O(\|\mathbf{a}_i^1\|_2^2 \|\mathbf{W}_0\|_2^2 )$. Next, since for fixed $\mathbf{a}_i^1$ and $f_i$, the random variables $\{\chi\{ \eta f_{i}(\mathbf{x}_{i,l}) (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) > 1 \} \}_{l=1}^{n_1}$ are i.i.d., we have by Hoeffding's inequality
\begin{align}
&\mathbb{P}_{\mathbf{x}_{i,l}}\left( \left|\frac{1}{n_2} \sum_{l=1}^{n_2} \chi\{  f_{i}(\mathbf{x}_{i,l}) (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) > 1 \} - 
\mathbb{P}_{\mathbf{x}}( f_{i}(\mathbf{x}) (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}) > 1 )\right| > t
\right)\nonumber \\
&\leq  2\exp\left( -2 n_2t^2 \right)
\end{align}
for any $t>0$. So $\frac{1}{n_2} \sum_{l=1}^{n_2} \chi\{  f_{i}(\mathbf{x}_{i,l}) (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) > 1 \} - 
\mathbb{P}_{\mathbf{x}}(\eta f_{i}(\mathbf{x}) (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}) > 1 )$ is sub-Gaussian with mean zero and variance proxy $\frac{1}{n_2}$. Also, each random variable in $\{\frac{1}{n_2} \sum_{l=1}^{n_2} \chi\{  f_{i}(\mathbf{x}_{i,l}) (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) > 1 \} - 
\mathbb{P}_{\mathbf{x}}(\eta f_{i}(\mathbf{x}) (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}) > 1 ) \}_{i=1}^T $ is independent, so again by Hoeffding's inequality,
% $O(\|\mathbf{a}_i^1\|_2\|\mathbf{W}^0\|_F)$ and variance $O()$.
\begin{align}
   & \mathbb{P}_{\mathbf{x}_{i,l}}\left( \left|\frac{1}{Tn_2}\sum_{i=1}^T \sum_{l=1}^{n_2} \chi\{  f_{i}(\mathbf{x}_{i,l}) (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) > 1 \} - \frac{1}{T}\sum_{i=1}^T
\mathbb{P}_{\mathbf{x}}( f_{i}(\mathbf{x}) (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}) > 1 )\right| > t
\right)\nonumber\\
&\leq 2\exp\left( -{2Tn_2 t^2} \right)
\end{align}
Set $t = O(\frac{\sqrt{\log(1/\delta_2)}}{\sqrt{Tn_2}})$, then we have 
\begin{align}
    \frac{1}{Tn_2}\sum_{i=1}^T \sum_{l=1}^{n_2} \chi\{  f_{i}(\mathbf{x}_{i,l}) (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) > 1 \} &= \frac{1}{T}\sum_{i=1}^T \mathbb{P}_{\mathbf{x}}( f_{i}(\mathbf{x}) (\mathbf{a}_i^1)^\top \sigma(\mathbf{W}^0\mathbf{x}) > 1 ) + O\left( \frac{\sqrt{\log(1/\delta)}}{\sqrt{Tn_2}}\right) \nonumber \\
    &\leq \frac{1}{T}\sum_{i=1}^T \gamma_i + O\left( \frac{\sqrt{\log(1/\delta_2)}}{\sqrt{Tn_2}}\right)  \label{30}
\end{align}
with probability at least $1-\delta_2$ over the sampling of $\{\mathbf{x}_{i,l}\}_{i,l}$. It remains to bound each $\gamma_i$. 
% By Lemma \ref{lem:init3} and the fact that $E_{\mathbf{w}}(\delta_1)$ holds, we have $\|\mathbf{W}^0\|_2 = O(\nu_{\mathbf{w}}(\sqrt{d} + \sqrt{m} + \sqrt{\log(1/\delta_1)}))$. 
Next, for any $i\in [T]$, we have 
\begin{align}
    \|\mathbf{a}_i^1\|_2 &= \left\|\frac{\eta}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) {\sigma}(\mathbf{W}^0\mathbf{x}_{i,k} ) \right\|_2
    \leq \eta \sqrt{m } \max_{j\in[m]} \left| \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) {\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} )\right|
\end{align}
Each $ f_{i}(\mathbf{x}_{i,k}) {\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} ) $ is sub-Gaussian with mean $O(\|\mathbf{w}_j\|_2)$ and variance $O(\|\mathbf{w}_j\|_2^2)$. Also, for fixed $f_i$, the random variables $ \{f_{i}(\mathbf{x}_{i,k}) {\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} )\}_{k=1}^{n_1}$ are independent. So, we have $\|\mathbf{a}_i^1\|_2 = O(\eta \sqrt{m} t \max_{j\in[m]}\|\mathbf{w}_j\|_2 )$ with probability at least $1 - e^{-t^2}$ for any $t>0$. Union bounding over all $i\in [T]$ and setting $t = \Theta(\sqrt{\log(T)} + \sqrt{\log(1/\delta_3)})$ yields $\max_{i\in [T]}\|\mathbf{a}_i^1\|_2= O (\eta  \sqrt{m \log(T/\delta_3)} \max_{j\in[m]}\|\mathbf{w}_j\|_2 )$, with probability at least $1-\delta_3$. Now applying Lemma \ref{lem:init} and the fact that $E_{\mathbf{w}}(\delta)$ holds results in $\max_{i\in [T]}\|\mathbf{a}_i^1\|_2= O (\eta  \nu_{\mathbf{w}}\sqrt{m\log(T/\delta_3)}(\sqrt{d} + \sqrt{\log(m/\delta_1)}) )$
and \begin{align}
    \max_{i\in [T]}\|\mathbf{a}_i^1\|_2\|\mathbf{W}^0\|_2 &= O\left(  \eta  \nu_{\mathbf{w}}\sqrt{m\log(T/\delta_3)}(\sqrt{d} + \sqrt{\log(m/\delta_1)}) (\sqrt{d} + \sqrt{m} + \sqrt{\log(1/\delta_1)
    } )\right)\nonumber \\
    &=  O\left(  \eta  \nu_{\mathbf{w}}\sqrt{m\log(T/\delta_3)}(\sqrt{d} + \sqrt{\log(m/\delta_1)}) (\sqrt{d} + \sqrt{m} )\right)
\end{align}
with probability at least $1-\delta_3-3\delta_1$. 
% Next, note that from \eqref{gmm}, 
% \begin{align}
% \end{align}
Set $\delta_3+3\delta_1 + \delta_2 \leq \delta$,
% Since $m/\delta_1 = O(e^d)$, we have $\max_{i\in [T]}\|\mathbf{a}_i^1\|_2= O (\eta  \nu_{\mathbf{w}}\sqrt{dm\log(T/\delta)} )$ with probability at least $1-\delta$.
% (where we have also used that the choice of $m$ is $o(e^d)$). 
then from \eqref{gmm} and using $\nu_{\mathbf{w}} = O( \frac{1}{ \eta  \sqrt{m\log(T/\delta)}(\sqrt{d} + \sqrt{\log(m/\delta)}) (\sqrt{d} + \sqrt{m} )} )$, we have $\max_{i\in [T]}\|\mathbf{a}_i^1\|_2\|\mathbf{W}^0\|_2 = O(1)$ and
\begin{align}
    \frac{1}{T}\sum_{i=1}^T\gamma_i \leq \max_{i\in [T]}\gamma_i &= \frac{2}{T} \sum_{i=1}^T \exp\left( -\frac{  1 -  2\|\mathbf{a}_i^1\|_2 \|\mathbf{W}^0\|_2 }{  c\|\mathbf{a}_i^1\|_2^2 \|\mathbf{W}_0\|_2^2 } \right)\nonumber \\
    &\leq 2 \exp\left( -\frac{  1 -  2 \max_{i\in [T]}\|\mathbf{a}_i^1\|_2 \|\mathbf{W}^0\|_2 }{  c\max_{i\in [T]}\|\mathbf{a}_i^1\|_2^2 \|\mathbf{W}_0\|_2^2 } \right) \nonumber \\
    &\leq 2 c'\exp\left( -\frac{  1}{  c\max_{i\in [T]}\|\mathbf{a}_i^1\|_2^2 \|\mathbf{W}_0\|_2^2 } \right) \nonumber \\
    &\leq 2 c'  \exp \left( -\frac{ c'' }{\eta^2  \nu_{\mathbf{w}}^2 {m\log(T/\delta)}({d} + {\log(m/\delta)}) ({d} + {m} )} \right)\nonumber 
\end{align}
with probability at least $1-\delta$,
completing the proof in light of \eqref{30}.
\end{proof}
% as long as $\eta^2  \nu_{\mathbf{w}}^2{dm\log(T)} (d+m) \leq 1/2$, 
% We first bound the norm of each  $\mathbf{a}_i^1$
% Each indicator $  \chi\left\{ \eta f_{i}(\mathbf{x}_{i,l}) \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1\right\}$ is a Bernoulli random variable with parameter
% \begin{align}
%     &\mathbb{P}_{f_i, \mathbf{x}_{i,k}, \mathbf{x}_{i,l}}\left(  \eta f_{i}(\mathbf{x}_{i,l}) \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1\right)  \nonumber \\
%     &= \mathbb{P}_{f_i, \mathbf{x}_{i,k}, \mathbf{x}_{i,l}}\left(  \eta f_{i}(\mathbf{x}_{i,l})  \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \sum_{j=1}^m \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} )  \sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l}) >1\right)  \nonumber \\
%     &\leq  \mathbb{P}_{f_i, \mathbf{x}_{i,k}, \mathbf{x}_{i,l}}\left(  \left| \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \sum_{j=1}^m \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} )  \sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l})\right| >\frac{1}{\eta}  \right)  \nonumber \\
%     % &\leq \mathbb{P}_{f_i, \mathbf{x}_{i,k}, \mathbf{x}_{i,l}}\left( \max_{j\in [m]} \left| \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} )  \sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l}) \right| >\frac{1}{\eta m}\right)  \nonumber \\
%     &\leq \sum_{j=1}^m \mathbb{P}_{f_i, \mathbf{x}_{i,k}, \mathbf{x}_{i,l}}\left( \left|   \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} ) \sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l})  \right| >\frac{1}{\eta m}\right)  \nonumber \\
%     &\leq \sum_{j=1}^m \mathbb{P}_{f_i, \mathbf{x}_{i,k}, \mathbf{x}_{i,l}}\left( \left|   \frac{1}{n_1} \sum_{k=1}^{n_1}  \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} )  \sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l}) \right| >\frac{1}{\eta m}\right)   \label{pos} \\ 
%     &\leq \sum_{j=1}^m \mathbb{P}_{f_i, \mathbf{x}_{i,k}, \mathbf{x}_{i,l}}\left( \left|  \frac{1}{n_1} \sum_{k=1}^{n_1}  \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} )\sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l})   - c\|\mathbf{w}_j\|_2^2 \right| >\frac{1}{\eta m} - c\|\mathbf{w}_j\|_2^2 \right)   \nonumber \\
%     % &\leq   \nonumber \\
%     % &\leq \mathbb{P}\left( \left|  \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) {\sigma}'(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \mathbf{W}^0\mathbf{x}_{i,l} \right| >1/\eta \right)  \nonumber \\
%     % &\leq \mathbb{P}_{f_i, \mathbf{x}_{i,k}, \mathbf{x}_{i,l}}\left( \left|  \mathbf{1}_m^\top \mathbf{W}^0\mathbf{x}_{i,l} \right| >1/\eta \right)  \nonumber \\
%     % &= \mathbb{P}_{f_i, \mathbf{x}_{i,k}, \mathbf{x}_{i,l}}\left( \left| \sum_{j=1}^m \mathbf{w}^\top_j\mathbf{x}_{i,l} \right| >1/\eta \right) \nonumber \\
%     &= m \;O\left( \max_{j\in [m]}  \exp \left(-\frac{ \frac{1}{\eta m} - c\|\mathbf{w}_j\|_2^2 }{ c'\|\mathbf{w}_j\|_2^2 }     \right) \right) \label{bnbn} \\
%     &=  m\;  O\left( \max_{j\in [m]}  \exp \left(-\frac{ {1}}{ c'\eta m \|\mathbf{w}_j\|_2^2 }     \right) \right) \nonumber\\
%     &=  m\;  O\left(   \exp \left(-\frac{ {1}}{ c'' \eta m d^2 \nu_{\mathbf{w}}^2 }     \right) \right) \label{vvf}
%     % &\leq m\;  O\left( \max_{j\in [m]}  \exp \left(-\frac{ {1}}{ c'\eta m \|\mathbf{w}_j\|_2^2 }     \right) \right)
%     % &\leq O(  \exp (- m \max_{j\in [m]}(\|\mathbf{w}_j\|_2^2) /(2\eta^2) )) \label{bnbn}
%     % \exp\left( O \left( \min\left( \frac{1}{\eta^2 \sigma_{w}^2 m }, \frac{1}{\eta \sigma_{w} } \right)\right)  \right)  \label{bnbn}
% \end{align}
% where $c$ is an absolute constant defined by $\mathbb{E}[\sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l})] = \sqrt{c}\|\mathbf{w}_j\|_2$, in particular $c= 2/\pi$.
% Equation \eqref{pos} follows since $\bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} ) $ and $  \sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l})$ are nonnegative, and
% \eqref{bnbn} follows by noting that $  \sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l}) $ is sub-Gaussian with mean $c\|\mathbf{w}_j\|_2^2$ and variance $O({\|\mathbf{w}_j\|_2^2})$, and $ \frac{1}{n_1} \sum_{k=1}^{n_1}  \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} )$ is independently sub-Gaussian 
% with mean $c\|\mathbf{w}_j\|_2^2$ and variance $O(\frac{\|\mathbf{w}_j\|_2^2}{n_1})$, so $\sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l})  \frac{1}{n_1} \sum_{k=1}^{n_1}  \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} ) - c\|\mathbf{w}_j\|_2^2$ is sub-exponential with mean $O(\|\mathbf{w}_j\|_2^2)$ and variance:
% \begin{align}
%     &\text{Var}\left(\sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l})  \frac{1}{n_1} \sum_{k=1}^{n_1}  \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} ) -c\|\mathbf{w}_j\|_2^2\right)\nonumber \\
%     &= \mathbb{E}\left[\left(\sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l})  \frac{1}{n_1} \sum_{k=1}^{n_1}  \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} ) -c\|\mathbf{w}_j\|_2^2\right)^2\right]\nonumber \\
%     &= \frac{1}{n_1^2} \sum_{k=1}^{n_1}  \mathbb{E}_{\mathbf{x}_{i,l},\mathbf{x}_{i,k}}[(\sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} ) -c\|\mathbf{w}_j\|_2^2)^2] \nonumber \\
%     &\quad \quad \quad \quad + \frac{1}{n_1^2} \sum_{k=1}^{n_1} \sum_{k'=1,k'\neq k}^{n_1}\mathbb{E}_{\mathbf{x}_{i,l}}[\mathbb{E}_{\mathbf{x}_{i,k}}[(\sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} ) -c\|\mathbf{w}_j\|_2^2)]\mathbb{E}_{\mathbf{x}_{i,k'}}[(\sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k'} ) -c\|\mathbf{w}_j\|_2^2)]] \nonumber \\
%     &= \frac{1}{n_1^2} \sum_{k=1}^{n_1}  \mathbb{E}_{\mathbf{x}_{i,l},\mathbf{x}_{i,k}}[(\sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k} ) -c\|\mathbf{w}_j\|_2^2)^2] +  \frac{c\|\mathbf{w}_j\|^2(n_1-1)}{n_1} \mathbb{E}_{\mathbf{x}_{i,l}}[(\sigma(\mathbf{w}^\top_j\mathbf{x}_{i,l})  -\sqrt{c}\|\mathbf{w}_j\|_2)^2]\nonumber \\
%     &= O(\|\mathbf{w}_j\|_2^4)
% \end{align}


% Lastly, \eqref{vvf} follows with probability at least $1-2000^{-1}$ by Lemma \ref{lem:init}.
% % note: we cannot get hoeffding-slike concentration over n1 because the same fi is used for all k. also the relu prevents better concentration because the mean of the sum is not zero.
% % where \eqref{bnbn} follows by Bernstein's Inequality, % since , considering randomness over both $\mathbf{W}^0$ and $\mathbf{x}_{i,l}$ each 
% % as each $\mathbf{w}^\top_j\mathbf{x}_{i,l}$ is an independent mean-zero  Gaussian random variable with variance $\|\mathbf{w}_j\|_2^2$.
% % sub-exponential with mean zero and variance proxy $O(\sigma_{\mathbf{w}}^2)$.
% % , and each $f_{i}(\mathbf{x}_{i,k}) {\sigma}'(\mathbf{w}^\top_j\mathbf{x}_{i,k} ) $ is a discrete random variable that is 0 with probability 1/2, 1 with probability 1/4, and $-1$ with probability 1/4.  
% Thus, we can now invoke Hoeffding's inequality to obtain
% \begin{align}
%     &\frac{\eta}{T n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}    \chi\left\{ \eta f_{i}(\mathbf{x}_{i,l}) \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) {\sigma}'(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1\right\}\nonumber \\
%     &= \eta m\;  O\left(  \exp \left(-\frac{ {1}}{ c''\eta m d^2 \nu_{\mathbf{w}}^2 }     \right) \right)  +   \eta\;  O\left(  \frac{  1 }{ \sqrt{Tn_2} } \right) \nonumber %\\
%     % &=  \eta m\;  O\left( \max_{j\in [m]}  \exp \left(-\frac{ {1}}{ c'\eta m \|\mathbf{w}_j\|_2^2 }     \right) \right)  +   \eta\;  O\left(  \frac{  1 }{ \sqrt{Tn_2} } \right) 
%     % &=  \eta \; O(  \exp (- m \max_{j\in [m]}(\|\mathbf{w}_j\|_2^2) /(2\eta^2) ))  +O\left( \frac{\eta \sqrt{\log(m)} }{\sqrt{Tn_2}}\right)
% \end{align}
% with probability  at least $1 - 1000^{-1}$. 
% Note that this holds for all $j \in [m]$.     



% Next, using the fact that $\sign(\mathbf{M}\mathbf{x}) = \sign(\mathbf{M}\mathbf{x}')$ implies $f_{i}(\mathbf{x}) = f_{i}(\mathbf{x}')$ for all $i\in [n]$, we have 
% \begin{align}
% &=  1 -   \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[ \chi\{\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})  \right] \nonumber \\
% % &\quad -  \E_{\mathbf{x}, \mathbf{x}' }  \left[\{\sign(\mathbf{x}_{:r}) = - \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
% &\quad -  \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{x}_{:r}) \neq   \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
% &\quad + \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\right\} \nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - \eta f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber \\
% &=  1 -   \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[ \chi\{\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}_{:r}') \} \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})  \right] \nonumber \\
% &\quad - \eta  \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
% &\quad + \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\right\} \nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - \eta f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber 
% \end{align}



% Using the computation of each $\mathbf{a}_{i}^1$ from Lemma \ref{lem:a1}, and the fact that $\mathbf{b}^0 = \mathbf{0}$ by choice of initialization, we have
% \begin{align}
%     \hat{\mathcal{L}}(\mathbf{W}^0,\mathbf{b}^0,\{\mathbf{a}^+_{i}\}_{i=1}^T; \{\hat{\mathcal{D}}_{i,\mathbf{W}}\}_{i=1}^T) 
%    &= \frac{1}{T} \sum_{i=1}^T \hat{\mathcal{L}}_i(\mathbf{W}^0,\mathbf{b}^0,\{\mathbf{a}_{i}^1\}_{i=1}^T; \hat{\mathcal{D}}_{i,\mathbf{W}})
%     \nonumber \\
%     &=\frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x} }  \left[ \max\left( 1- (\mathbf{a}_i^1)^\top\sigma(\mathbf{W}^0\mathbf{x}) , 0 \right) \right]   
%     \nonumber \\
%     &= \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x} }  \left[ \max\left( 1- \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}'} [ f_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}') ]^\top \sigma(\mathbf{W}^0\mathbf{x}) , 0 \right) \right]     \nonumber \\
% %     &= \E_{\mathbf{x} }  \left[ \max\left( 1- \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}'} [ f_{i}(\mathbf{x}') g(\mathbf{x}';\mathbf{W}^0,\mathbf{b}^0 ) ]^\top g(\mathbf{x}; \mathbf{W}^0,\mathbf{b}^0)  , 0 \right) 
% % %     \frac{1}{n_2}\sum_{j=1}^{n_2}\max \left(1 - y_{i,j} \left(\frac{1}{\lambda_{1}n_1}\sum_{j'=1}^{n_1}\bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})  \right)^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}), 0\right) \right] \nonumber\\
% % % &= 1 -  \E_{i }  \left[ \frac{1}{\lambda_{1} n_1n_2}\sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})
% % \right] \label{14} \nonumber \\
% &=\frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) <1\right\} \nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - \etaf_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber \\
% &=  1 -   \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[   \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right) \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})  \right]  \nonumber \\
% &\quad + \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\right\} \nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - \eta f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber 
% \end{align}
% Next, using the fact that $\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}_{:r}')$ implies $f_{i}(\mathbf{x}) = f_{i}(\mathbf{x}')$ for all $i\in [n]$, we have 
% \begin{align}
% &=  1 -   \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[ \chi\{\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})  \right] \nonumber \\
% % &\quad -  \E_{\mathbf{x}, \mathbf{x}' }  \left[\{\sign(\mathbf{x}_{:r}) = - \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
% &\quad -  \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{x}_{:r}) \neq   \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
% &\quad + \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\right\} \nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - \eta f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber \\
% &=  1 -   \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[ \chi\{\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}_{:r}') \} \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})  \right] \nonumber \\
% &\quad - \eta  \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
% &\quad + \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\right\} \nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - \eta f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber 
% \end{align}







% \begin{lemma} \label{lem:loss}
% The loss after updating the heads on the first iteration is given by
% %     \begin{align}
% %      &   \mathcal{L}(\mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{1,i} \}_{i\in \mathcal{T}}) \nonumber \\
% % &=  \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) <1\}\nonumber \\
% % &\quad \quad \quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \}  \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz}) \Big] \nonumber 
% %     \end{align}
%         \begin{align}
%      &   \mathcal{L}(\mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{i}^1 \}_{i=1}^T) \nonumber \\
% %      \nonumber \\
% % &=  \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) <1\}\nonumber \\
% % &\quad \quad \quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \}  \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz}) \Big] \nonumber 
% &=  1 -   \E_{\mathbf{x}, \mathbf{x}' }  \left[ \chi\{\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}_{:r}') \} \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})  \right] \nonumber \\
% &\quad -  \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
% &\quad + \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\right\} \nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber 
%     \end{align}
% \end{lemma}

% \begin{proof}
% % Let $g(\mathbf{x}; \mathbf{W}^0) \coloneqq $

% \end{proof}



\begin{lemma}\label{lem:emp_grad}
  For any $\delta \in (0,1)$, with probability at least $1 -  \delta$,   for all neurons $j\in [m]$,  the gradient used to compute $\mathbf{w}_{j}^1$ %, 
    % that is the gradient with respect to $\mathbf{w}_j$ of the average  empirical loss across tasks after the first update of the heads, 
    satisfies
\begin{align}
    &\left\|\nabla_{\mathbf{w}_j} \hat{\mathcal{L}}( \mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{i}^1\}_{i=1}^T; \{\hat{\mathcal{D}}_{i,\mathbf{W}}\}_{i=1}^T ) + \frac{\eta}{T n_1 n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1}
f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) \mathbf{x}_{i,l}\mathbf{x}_{i,k}^\top\mathbf{w}_j^0\right\|_2 \nonumber \\
&=   
% \eta \;  O\left(  d^2 \nu_{\mathbf{w}}^2  \exp \left(-\frac{ {c}}{ \eta^2  \nu_{\mathbf{w}}^2{dm} (d+m) \log(T)}     \right) \right)  +   \eta\;  O\left(  {   }{ \frac{ d \nu_{\mathbf{w}} }{ \sqrt{ Tn_2}} } \right) 
 O\Bigg( \eta \nu_{\mathbf{w}} (\sqrt{d} + \sqrt{\log(m/\delta)}) \sqrt{d\log(Tn_2/\delta)} \left(1 + {\frac{ \sqrt{\log(T/\delta)}}{\sqrt{n_1}}}\right) \nonumber \\
     &\quad \quad \quad \quad \times \left(   \exp \left( -\frac{ c }{\eta^2  \nu_{\mathbf{w}}^2 {m\log(T/\delta)}({d} + {\log(m/\delta)}) ({d} + {m} )} \right) + \frac{\sqrt{\log(1/\delta)}}{\sqrt{Tn_2}}\right) \Bigg)\nonumber
% O\left( 
% \eta d \nu_{\mathbf{w}}  \exp \left(-\frac{ {c}}{ \eta^2  \nu_{\mathbf{w}}^2{dm} (d+m) \log(T)}     \right) \right)  +   \;  O\left(  {   }{ \frac{ \eta d \nu_{\mathbf{w}} }{ { T^{1/4}n_2^{1/4}}} } \right) 
% \eta m\;  O\left(  \exp \left(-\frac{ {1}}{ c\eta m d^2 \nu_{\mathbf{w}}^2 }     \right) \right)  +   \eta\;  O\left(  \frac{  1 }{ \sqrt{Tn_2} } \right),
\end{align}
 %-O( (Tn_1^2 + Tn_2)^{-1}) 
where $c$ is an absolute constant and $\sigma'(x) = \chi\{x>0\}$ denotes the derivative of the ReLU.
\end{lemma}

\begin{proof}
Consider any fixed $\mathbf{W}^0$ satisfying $E_{\mathbf{w}}(\delta_1)$ for $\delta_1\in (0,1)$, 
% such that $\delta_1 = \Omega(me^-d)$, 
which occurs with probability at least $1-3 \delta_1$ by Lemma \ref{lem:all}. 
For ease of notation we write $\mathbf{w}_j =\mathbf{w}_j^0$.  
Using Lemma \ref{lem:upd_loss} and the chain rule, 
\begin{align}
 &\nabla_{\mathbf{w}_j} \hat{\mathcal{L}}( \mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{i}^1\}_{i=1}^T; \{\hat{\mathcal{D}}_{i,\mathbf{W}}\}_{i=1}^T ) \nonumber \\
 &=    - \frac{\eta}{T n_1 n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1}
f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\bar{\sigma}(\mathbf{w}_j^\top \mathbf{x}_{i,k}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l})\mathbf{x}_{i,l}   \nonumber \\
&\quad +\frac{\eta}{T n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}    \chi\left\{ \eta f_{i}(\mathbf{x}_{i,l}) \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1\right\}   \nonumber \\
&\quad \quad \quad \quad \quad \quad \quad \; \times  f_{i}(\mathbf{x}_{i,l}) \left(\frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})\right) \sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,l}) \mathbf{x}_{i,l}
 \nonumber \\
 &=   \underbrace{- \frac{\eta}{T n_1 n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1}
f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k}){\sigma}'(\mathbf{w}_j^\top \mathbf{x}_{i,k}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l})\mathbf{x}_{i,l}\mathbf{x}_{i,k}^\top \mathbf{w}_j}_{\circled{1}}    \nonumber \\
&\quad +\underbrace{\frac{\eta}{T n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}    \chi\left\{ \eta f_{i}(\mathbf{x}_{i,l}) \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1\right\}}_{\circled{2}}   \nonumber \\
&\quad \quad \quad \quad \quad \quad \quad \; \underbrace{\times  f_{i}(\mathbf{x}_{i,l}) \left(\frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})\right) \sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,l}) \mathbf{x}_{i,l}}_{\circled{2}}
 \label{full} 
\end{align}
where \eqref{full} follows since $\bar{\sigma}(x) = \sigma'(x)x$ when $\bar{\sigma}$ is the ReLU activation. By  \eqref{full} and the triangle inequality we have $\|\nabla_{\mathbf{w}_j} \hat{\mathcal{L}}( \mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{i}^1\}_{i=1}^T; \{\hat{\mathcal{D}}_{i,\mathbf{W}}\}_{i=1}^T ) - \circled{1}\|_2 \leq \|\circled{2}\|_2  $, so the result follows by bounding $\|\circled{2}\|_2$. To do this, note that by Hölder's inequality,
% \begin{align}
%  \| \circled{2}\|_2  &\leq \Bigg\| \frac{\eta}{T n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}    \chi\left\{ \eta f_{i}(\mathbf{x}_{i,l}) \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1\right\}   \nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \; \times  f_{i}(\mathbf{x}_{i,l}) \left(\frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})\right) \sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,l}) \mathbf{x}_{i,l} \Bigg\|_2 \nonumber \\
% &\leq  \eta \left(\frac{1}{T n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}    \chi\left\{ \eta f_{i}(\mathbf{x}_{i,l}) \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1\right\} \right)^{1/2} \nonumber\\
% &\quad \times \left(\frac{1}{T n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}   \left\|   \left(\frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})\right) \sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,l}) \mathbf{x}_{i,l}  \right\|_2^2 \right)^{1/2} \nonumber \\
% &\leq  \eta \left(\underbrace{\frac{1}{T n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}    \chi\left\{ \eta f_{i}(\mathbf{x}_{i,l}) \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1\right\}}_{\circled{2a}} \right)^{1/2} \nonumber\\
% &\quad \times \left( \underbrace{\frac{1}{T} \sum_{i=1}^T  \left(   \frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})\right)^2  \frac{1}{n_2}\sum_{l=1}^{n_2} \left\|  \mathbf{x}_{i,l}  \right\|_2^2 }_{\circled{2b}} \right)^{1/2}\label{brea} 
% \end{align}
\begin{align}
 \| \circled{2}\|_2  &\leq \Bigg\| \frac{\eta}{T n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}    \chi\left\{ \eta f_{i}(\mathbf{x}_{i,l}) \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1\right\}   \nonumber \\
&\quad \quad \quad \quad \quad \quad \quad \; \times  f_{i}(\mathbf{x}_{i,l}) \left(\frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})\right) \sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,l}) \mathbf{x}_{i,l} \Bigg\|_2 \nonumber \\
&\leq  \eta {\frac{1}{T n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}    \chi\left\{ \eta f_{i}(\mathbf{x}_{i,l}) \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1\right\}}  \nonumber\\
&\quad \times {\max_{i\in [T], l\in [n_2]}  \left\|   \left(\frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})\right) \sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,l}) \mathbf{x}_{i,l}  \right\|_2 }\nonumber\\
&\leq  \eta \underbrace{\frac{1}{T n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}    \chi\left\{ \eta f_{i}(\mathbf{x}_{i,l}) \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1\right\}}_{\circled{2a}}  \nonumber\\
&\quad \times \underbrace{\max_{i\in [T]}  \left|\frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})\right| \max_{i\in [T], l\in [n_2]}  \left\|   \mathbf{x}_{i,l}  \right\|_2 }_{\circled{2b}} \label{brea}
% &\leq  \eta \left(\underbrace{\frac{1}{T n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}    \chi\left\{ \eta f_{i}(\mathbf{x}_{i,l}) \left( \frac{1}{n_1} \sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{W}^0\mathbf{x}_{i,k} ) \right)^\top \sigma(\mathbf{W}^0\mathbf{x}_{i,l}) >1\right\}}_{\circled{2a}} \right)^{1/2} \nonumber\\
% &\quad \times \left( \underbrace{\frac{1}{T} \sum_{i=1}^T  \left(   \frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})\right)^2  \frac{1}{n_2}\sum_{l=1}^{n_2} \left\|  \mathbf{x}_{i,l}  \right\|_2^2 }_{\circled{2b}} \right)^{1/2}\label{brea} 
\end{align}
By Lemma \ref{lem:err_a}, we have 
\begin{align}
    \circled{2a} = \eta O\left(  \exp \left( -\frac{ c }{\eta^2  \nu_{\mathbf{w}}^2 {m\log(T/\delta_3)}({d} + {\log(m/\delta_3)}) ({d} + {m} )} \right)\right) + \eta \; O\left(  \frac{  \sqrt{\log(1/\delta_3)} }{ \sqrt{Tn_2} } \right) 
    % \eta m\;  O\left(   \exp \left(-\frac{ {1}}{ c\eta m d^2 \nu_{\mathbf{w}}^2 }     \right) \right)  +   \eta\;  O\left(  \frac{  1 }{ \sqrt{Tn_2} } \right).
\end{align}
with probability at least $1 - \delta_3$. 
It remains to control $\circled{2b}$.
Fix $\mathbf{w}_j$, $i$, and $l$, then each random variable $ f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})$ is sub-Gaussian with mean $O(\|\mathbf{w}_j\|_2)$
and variance $O(\|\mathbf{w}_j\|_2^2)$,
% sub-Gaussian random variable with norm $c \|\mathbf{w}_j\|_2$, 
and each random variable in $\{ f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \}_{k=1}^{n_1}$ is i.i.d. Thus, 
% \begin{align}
      $\frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k}) $
% \end{align}
is sub-Gaussian with mean $O(\|\mathbf{w}_j\|_2)$
and variance $O\left(\frac{\|\mathbf{w}_j\|_2^2}{n_1}\right)$, so, by a union bound over all $i\in [T]$,
\begin{align}
   \max_{i\in [T]} \left|\frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})\right| &= O\left(\|\mathbf{w}_j\|_2\left( 1 +  \sqrt{\frac{\log(T/\delta_2)}{n_1}} \right)\right) \nonumber \\
   &= O\left( \nu_{\mathbf{w}} ( \sqrt{d} + \sqrt{\log(m/\delta_1)}) \left( 1 +  \sqrt{\frac{\log(T/\delta_2)}{n_1}} \right)\right)
\end{align}
with probability at least $1-3\delta_1 - \delta_2$. %, where we have used $m/\delta = o(e^d)$. 
Next, $ \left\| \mathbf{x}_{i,l}  \right\|_2^2 $ is sub-exponential with 
mean $O\left({d}\right)$ and variance 
% is sub-exponential with norm 
$O\left(d^2\right)$. So, with probability at least $1-\delta_4$, 
\begin{align}
    \max_{i\in[T],l\in [n_2]} \|\mathbf{x}_{i,l}  \|_2^2 &= O\left(d(1 +  \log(Tn_2/\delta_4) ) \right)  = O\left(d \log(Tn_2/\delta_4)  \right)  \implies \max_{i\in[T],l\in [n_2]} \|\mathbf{x}_{i,l}  \|_2  = O\left(\sqrt{d \log(Tn_2/\delta_4)}  \right) 
\end{align}
% % is sub-Gaussian with norm $ O\left(\frac{\|\mathbf{w}_j\|_2}{\sqrt{n_1}} \right)$, 
% and  $\left(\frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \right)^2$ 
% is sub-exponential with mean $O(\|\mathbf{w}_j\|_2^2)$
% and variance $O\left(\frac{\|\mathbf{w}_j\|_2^4}{n_1^2}\right)$.
% So, 
% \begin{align}
%     \left(\frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \right)^2 &\leq O\left( \|\mathbf{w}_j\|_2^2\left(1 + \frac{1}{n_1}\right) \right)= O(\|\mathbf{w}_j\|_2^2).
% \end{align}
% with probability at least $1 - 1000^{-1}$. 
% is sub-exponential with norm $ O\left(\frac{\|\mathbf{w}_j\|_2^2}{{n_1}} \right)$. 
% with probability at least $1- $.
% Next, due to Lemma \ref{lem:half},  $\mathbb{E}_{ \mathbf{x}_{i,l}}[{\sigma}'(\mathbf{w}_j^\top\mathbf{x}_{i,l}) \mathbf{x}_{i,l} ] = \sqrt{\frac{2}{\pi}}\frac{\mathbf{w}_j}{\|\mathbf{w}_j\|_2}$, and has variance
% \begin{align}
%     \mathbb{E}_{ \mathbf{x}_{i,l}} \left[  \right]
% \end{align}
% Thus, since $\{ \}_{l=1}^T$ are i.i.d., we have that $\frac{1}{n_2}\sum_{l=1}^{n_2} \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}  )  \mathbf{x}_{i,l}  -  \sqrt{\frac{2}{\pi}}\frac{\mathbf{w}_j}{\|\mathbf{w}_j\|_2}$ is a sub-Gaussian random vector with mean zero and variance proxy $O(\frac{  }{n_1})$. So,
% \begin{align}
%     \left\| \frac{1}{n_2}\sum_{l=1}^{n_2} \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}  )  \mathbf{x}_{i,l}  \right\|_2 &\leq \sqrt{\frac{2}{\pi}} + \frac{}{\sqrt{n_1}}
% \end{align}
% with probability at least $1-1000^{-1}$.
% % \begin{align}
%     $ \frac{1}{n_2}\sum_{l=1}^{n_2}  \left\| \mathbf{x}_{i,l}  \right\|_2^2$
% % \end{align}
% Similarly, $ \frac{1}{n_2}\sum_{l=1}^{n_2}  \left\| \mathbf{x}_{i,l}  \right\|_2^2 $
% has mean $O\left({d}\right)$ and variance 
% % is sub-exponential with norm 
% $O\left({\frac{d^2}{n_2}}\right)$.
% % with probability at least .
% Therefore, since $\left(\frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})\right)^2$ and $\frac{1}{n_2}\sum_{l=1}^{n_2}  \left\| \mathbf{x}_{i,l}  \right\|_2^2$ are independent,  for each $i \in [T]$, $ \left(\frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})\right)^2 \frac{1}{n_2}\sum_{l=1}^{n_2}  \left\| \mathbf{x}_{i,l}  \right\|_2^2 $ has 
% mean $O(d \|\mathbf{w}_j\|_2^2)$ and variance $O\left(\|\mathbf{w}_j\|_2^4 d^2\left( \frac{1}{n_1^2} + \frac{1}{n_2}\right) \right)$.
% Moreover, since each random variable in  $ \left\{  \left(   \frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})\right)^2 \frac{1}{n_2}\sum_{l=1}^{n_2}  \left\| \mathbf{x}_{i,l}  \right\|_2^2  \right\}_{i=1}^{T}$ 
% % and
% % $ \left\{\left( \frac{1}{n_2}\sum_{l=1}^{n_2}  \left\| \mathbf{x}_{i,l}  \right\|_2^2 \right) \right\}_{i=1}^T $
% is i.i.d, the random variable
% \begin{align}
%     \frac{1}{T} \sum_{i=1}^T  \left(   \frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) \bar{\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})\right)^2 \left( \frac{1}{n_2}\sum_{l=1}^{n_2}  \left\| \mathbf{x}_{i,l}  \right\|_2^2 \right) \nonumber
% \end{align}
% has mean $O(\|\mathbf{w}_j\|_2^2 d)$ and variance  $O\left( \|\mathbf{w}_j\|_2^4 d^2\left( \frac{1}{Tn_1^2} + \frac{1}{Tn_2}\right)\right)$. 
% Therefore, by Chebyshev's inequality and Lemma \ref{lem:init}, we have
% \begin{align}
%     \frac{1}{T} \sum_{i=1}^T  \left(   \frac{1}{n_1} \sum_{k=1}^{n_1}   f_{i}(\mathbf{x}_{i,k}) {\sigma}(\mathbf{w}_j^\top\mathbf{x}_{i,k})\right)^2 \left( \frac{1}{n_2}\sum_{l=1}^{n_2}  \left\| \mathbf{x}_{i,l}  \right\|_2^2 \right) = O( d \|\mathbf{w}_j\|_2^2  ) = O(d^2 \nu_{\mathbf{w}}^2 )
% \end{align}
% with probability at least $1 - O( (Tn_1^2)^{-1} + (Tn_2)^{-1}) - 2000^{-1}\geq  1 - 1000^{-1}$  .

Combining these bounds via a union bound,  applying \eqref{brea},  and setting $\delta_1, \delta_2, \delta_3, \delta_4=\Theta( \delta)$ yields
\begin{align}
    \circled{2} &=  
    % O\left( \eta d \|\mathbf{w}_{j}\|_2^2 \exp \left(- m \max_{j'\in [m]}(\|\mathbf{w}_{j'}\|_2^2) /(2\eta^2) \right)\right)  +O\left( \eta  d \|\mathbf{w}_{j}\|_2^2  \frac{  \sqrt{\log(m)} }{\sqrt{Tn_2}}\right)
     \;  O\Bigg( \eta \nu_{\mathbf{w}} (\sqrt{d} + \sqrt{\log(m/\delta)}) \sqrt{d\log(Tn_2/\delta)} \left(1 + {\tfrac{ \sqrt{\log(T/\delta)}}{\sqrt{n_1}}}\right) \nonumber \\
     &\quad \quad \quad \quad \times \left(   \exp \left( -\frac{ c }{\eta^2  \nu_{\mathbf{w}}^2 {m\log(T/\delta)}({d} + {\log(m/\delta)}) ({d} + {m} )} \right) + \frac{\sqrt{\log(1/\delta)}}{\sqrt{Tn_2}}\right) \Bigg) \nonumber  
\end{align} for an absolute constant $c$ 
with probability at least $1 -\delta$, completing the proof.
\end{proof}
% note: check whether model in 3-layer paper is learnable by linear models



% Next we upper bound the noise in the gradient due to having finite samples.
\begin{lemma} \label{lem:grad_concen1}
    % The gradient computed in Lemma \ref{lem:emp_grad} satisfies
    For any $\delta\in (0,1)$, with probability at least $1 - \delta$, for all $j\in [m]$, 
    \begin{align}
        &\Bigg\| 
        % \nabla_{\mathbf{w}_j} \hat{\mathcal{L}}( \mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{i}^1\}_{i=1}^T; \{\hat{\mathcal{D}}_{i,\mathbf{W}}\}_{i=1}^T )  
        \frac{1}{T n_1 n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1}
f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\sigma'((\mathbf{w}_j^0)^\top\mathbf{x}_{i,k}) \sigma'((\mathbf{w}_j^0)^\top \mathbf{x}_{i,l}) \mathbf{x}_{i,l}\mathbf{x}_{i,k}^\top\mathbf{w}_j^0
       \nonumber \\
       &-  \mathbb{E}_{i\sim \mathcal{T}}\mathbb{E}_{(\mathbf{x}, f_i(\mathbf{x}))\sim \mathcal{D}_{i}} \mathbb{E}_{(\mathbf{x}', f_i(\mathbf{x}'))\sim \mathcal{D}_{i}}\left[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'((\mathbf{w}_j^0)^\top\mathbf{x}') \sigma'((\mathbf{w}_j^0)^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j^0\right] 
        % \eta  2^{-r}  \mathbf{A}(\mathbf{w}_{j}^0) \mathbf{w}_{j}^0 
        \Bigg\|_2 \nonumber \\
        % &= O\left( \frac{\sqrt{d} \log(d/\delta) \nu_{\mathbf{w}} }{\sqrt{T}} \right)
        &= O\left(\nu_{\mathbf{w}} \sqrt{\frac{d + \log(m/\delta)}{T} \log(d/\delta)}  \left(  \sqrt{r\log(m/\delta)} + \sqrt{\frac{d}{n_2}} \right) \right). \nonumber
    \end{align}
\end{lemma}

% $\epsilon$

\begin{proof} 
For ease of notation we replace $\mathbb{E}_{(\mathbf{x}, f_i(\mathbf{x}))\sim \mathcal{D}_{i}} \mathbb{E}_{(\mathbf{x}', f_i(\mathbf{x}'))\sim \mathcal{D}_{i}}$ with $\mathbb{E}_{\mathbf{x},\mathbf{x}'}$ and $\mathbb{E}_{i\sim \mathcal{T}}$ with $\mathbb{E}_i$, and write $\mathbf{w}_j=\mathbf{w}_j^0$. Consider any fixed $\mathbf{W}^0$ satisfying $E_{\mathbf{w}}(\delta_1)$ for $\delta_1\in (0,1)$, 
% such that $\delta_1 = \Omega(me^-d)$, 
which occurs with probability at least $1-3 \delta_1$ by Lemma \ref{lem:all}. 
We have
\begin{align}
 &\Bigg\| 
        % \nabla_{\mathbf{w}_j} \hat{\mathcal{L}}( \mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{i}^1\}_{i=1}^T; \{\hat{\mathcal{D}}_{i,\mathbf{W}}\}_{i=1}^T )  
        \frac{1}{T n_1 n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1}
f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) \mathbf{x}_{i,l}\mathbf{x}_{i,k}^\top\mathbf{w}_j
       \nonumber \\
       &-  \mathbb{E}_{i}\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right] 
        % \eta  2^{-r}  \mathbf{A}(\mathbf{w}_{j}^0) \mathbf{w}_{j}^0 
        \Bigg\|_2 \nonumber \\
        &= \left\| \frac{1}{T} \sum_{i=1}^T \mathbf{q}_i -  \mathbb{E}_{i}\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right]  \right\|_2
%         &\leq  \underbrace{\Bigg\| 
%         \frac{1}{T n_1 n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1}
% f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) \mathbf{x}_{i,l}\mathbf{x}_{i,k}^\top\mathbf{w}_j}_{\circled{1}}
%        \nonumber \\
%        &\quad \underbrace{- 
%         \frac{1}{T } \sum_{i=1}^T \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right]
%         \Bigg\|_2}_{\circled{1}} \nonumber \\
%         & +  \underbrace{\Bigg\| 
%         \frac{1}{T } \sum_{i=1}^T \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right]}_{\circled{2}}
%        \nonumber \\
%        &\quad \underbrace{-  \mathbb{E}_{i}\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right] 
%         \Bigg\|_2}_{\circled{2}} 
        \label{twonorms}
\end{align}
where $\mathbf{q}_i \coloneqq \frac{1}{n_1n_2} \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1}
f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) \mathbf{x}_{i,l}\mathbf{x}_{i,k}^\top\mathbf{w}_j$. By the linearity of the expectation, 
\begin{align}
    % \mathbb{E}_i \mathbb{E}_{\hat{\mathcal{D}}_i,\hat{\mathcal{D}}_i'}[\mathbf{q}_i]
    \mathbb{E}[\mathbf{q}_i]
    &= \frac{1}{n_1n_2} \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1} \mathbb{E}_i \mathbb{E}_{\mathbf{x}_{i,l},\mathbf{x}_{i,k}}[ f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) \mathbf{x}_{i,l}\mathbf{x}_{i,k}^\top\mathbf{w}_j ]  \nonumber \\
    &= \mathbb{E}_{i}\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right] 
\end{align}
which means that the random vectors $\mathbf{q}_i -  \mathbb{E}_{i}\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right] = \mathbf{q}_i - \mathbb{E}[\mathbf{q}_i ]$ in \eqref{twonorms} are mean zero. 
% They are also independent (and identically distributed). 
Next we bound $ \|\frac{1}{T}\sum_{i=1}^T \mathbf{q}_i - \mathbb{E}[\mathbf{q}_i ]\|_2 $
by bounding each coordinate of $\frac{1}{T}\sum_{i=1}^T \mathbf{q}_i - \mathbb{E}[\mathbf{q}_i ]$ separately. Let $q_{i,h}$ denote the $h$-th entry of $\mathbf{q}_i$, and $x_{i,l,h}$ denote the $h$-th entry of $\mathbf{x}_{i,l}$. Note that each $q_{i,h}$ is the sum of products of two sub-Gaussian random variables ($f_{i}(\mathbf{x}_{i,l}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) {x}_{i,l,h} $ and $ f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \mathbf{x}_{i,k}^\top\mathbf{w}_j $), so $q_{i,h}$ is the sum of sub-exponential random variables and is therefore sub-exponential. Its variance is upper bounded by:
% where \eqref{heff} follows by the fact that each $\diag(\mathbf{q}_i - \mathbb{E}[\mathbf{q}_i])$ is an independent symmetric sub-exponential matrix with mean 0 and variance proxy $O(d^2 \nu_{\mathbf{w}}^2)$ 
% so we can show concentration of the sum in \eqref{twonorms} once we bound the variance of each $\mathbf{q}_i$
% To do this, note that
\begin{align}
    &\mathbb{E}\left[({q}_{i,h} - \mathbb{E}[{q}_{i,h} ])^2 \right]  \nonumber \\
    &=  \mathbb{E}\left[\left(\left(\frac{1}{n_2} \sum_{l=1}^{n_2} 
f_{i}(\mathbf{x}_{i,l}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) {x}_{i,l,h} \right) \left(\frac{1}{n_1}\sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \mathbf{x}_{i,k}^\top\mathbf{w}_j\right) - \mathbb{E}[{q}_{i,h} ]\right)^2 \right]\nonumber \\
&\leq 4 \underbrace{  \mathbb{E}_{i,\hat{\mathcal{D}}_i,\hat{\mathcal{D}}_i' }\Bigg[\Bigg(\left(\frac{1}{n_2} \sum_{l=1}^{n_2} 
f_{i}(\mathbf{x}_{i,l}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) {x}_{i,l,h} \right) \left(\frac{1}{n_1}\sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \mathbf{x}_{i,k}^\top\mathbf{w}_j\right)}_{\circled{1}}\nonumber\\
&\quad \quad \quad \quad \underbrace{ - 
\mathbb{E}_{\mathbf{x}}\left[
f_{i}(\mathbf{x}) \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h \right] \left(\frac{1}{n_1}\sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \mathbf{x}_{i,k}^\top\mathbf{w}_j\right) \Bigg)^2 \Bigg]}_{\circled{1}}\nonumber \\
&\quad + 4\underbrace{ \mathbb{E}_{i,\hat{\mathcal{D}}_i' }\Bigg[\Bigg(\mathbb{E}_{\mathbf{x}}\left[
f_{i}(\mathbf{x}) \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h\right] \left(\frac{1}{n_1}\sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \mathbf{x}_{i,k}^\top\mathbf{w}_j\right)}_{\circled{2}} \nonumber \\
&\quad \quad \quad \quad \underbrace{ - \mathbb{E}_{\mathbf{x}}\left[
f_{i}(\mathbf{x}) \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h\right] \mathbb{E}_{\mathbf{x}'} \left[f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right]\Bigg)^2 \Bigg]}_{\circled{2}} \nonumber \\
&\quad + 2 \underbrace{ \mathbb{E}_i\Big[\Big(\mathbb{E}_{\mathbf{x}}\left[
f_{i}(\mathbf{x}) \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h\right] \mathbb{E}_{\mathbf{x}'} \left[f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right]}_{\circled{3}}\nonumber \\
&\quad \quad \quad \quad \underbrace{ - \mathbb{E}_{i}\left[\mathbb{E}_{\mathbf{x}}\left[
f_{i}(\mathbf{x}) \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h \right] \mathbb{E}_{\mathbf{x}'} \left[f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right]\right] \Big)^2 \Big]}_{\circled{3}} \label{3re}
% - \mathbb{E}[\mathbf{q}_i ]\right\|_2^2 \right]\nonumber \\
\end{align}
where \eqref{3re} follows from the triangle inequality and the fact that $(a+b)^2\leq 2a^2 + 2b^2$.
To bound $\circled{1}$, first let $\mathbf{s}_i \coloneqq \mathbb{E}_{\mathbf{x}}\left[
f_{i}(\mathbf{x}) \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h\right]$ and $s_{i,h}$ be its $h$-th element. Also denote $\overline{{s}_h^2} \coloneqq \mathbb{E}_i [s_{i,h}^2]$.
Observe that\begin{align}
    \circled{1} &=\mathbb{E}_{i,\hat{\mathcal{D}}_i,\hat{\mathcal{D}}_i' }\Bigg[\Bigg(\frac{1}{n_2} \sum_{l=1}^{n_2} 
f_{i}(\mathbf{x}_{i,l}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) {x}_{i,l,h} - s_{i,h} \Bigg)^2\left(\frac{1}{n_1}\sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \mathbf{x}_{i,k}^\top\mathbf{w}_j\right)^2\Bigg] \nonumber \\
&\leq \mathbb{E}_{i,{\mathcal{D}}_i}\Bigg[\Bigg(\frac{1}{n_2} \sum_{l=1}^{n_2} 
f_{i}(\mathbf{x}_{i,l}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) {x}_{i,l,h} - s_{i,h} \Bigg)^{4} \Bigg]^{1/2} \nonumber \\
&\quad \quad \quad \quad \times \mathbb{E}_{\hat{\mathcal{D}}_i}\Bigg[\left(\frac{1}{n_1}\sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \mathbf{x}_{i,k}^\top\mathbf{w}_j\right)^4\Bigg]^{1/2} \label{cs4} \\
&= \mathbb{E}_{i,{\mathcal{D}}_i}\Bigg[\Bigg(\frac{1}{n_2} \sum_{l=1}^{n_2} 
f_{i}(\mathbf{x}_{i,l}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) {x}_{i,l,h} - s_{i,h} \Bigg)^{4} \Bigg]^{1/2}\; O \left( \|\mathbf{w}_j\|_2^2 \right)\label{jnjn}\\
&= O\left( \frac{ \|\mathbf{w}_j\|_2^2}{n_2} \right) \label{mnm}\\
&= O\left( \nu_{\mathbf{w}}^2 \frac{d + \log(m/\delta_1) }{n_2} \right)
\end{align}
where \eqref{cs4} follows by the Cauchy-Schwarz inequality,
\eqref{jnjn} follows since
$\frac{1}{n_1}\sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \mathbf{x}_{i,k}^\top\mathbf{w}_j$ is sub-Gaussian with mean $O(\|\mathbf{w}_j\|_2)$ and variance $O(\frac{\|\mathbf{w}_j\|_2^2}{n_1}
)$, and \eqref{mnm} follows since  $\frac{1}{n_2} \sum_{l=1}^{n_2} 
f_{i}(\mathbf{x}_{i,l}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) {x}_{i,l,h} - s_{i,h}$ is sub-Gaussian with mean zero and variance $O(\frac{1}{n_2} \mathbb{E}_{\mathbf{x}}[ f_i(\mathbf{x})^2 \sigma'(\mathbf{w}_j^\top \mathbf{x})x_h^2 ] )= O(\frac{1}{n_2})$.
To bound $\circled{2}$, consider that 
\begin{align}
    \circled{2} &= \mathbb{E}_{i,\hat{\mathcal{D}}_i' }\Bigg[\mathbb{E}_{\mathbf{x}}\left[
f_{i}(\mathbf{x}) \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h \right]^2 \left(\frac{1}{n_1}\sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \mathbf{x}_{i,k}^\top\mathbf{w}_j- \mathbb{E}_{\mathbf{x}'}\left[
f_{i}(\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right]\right)^2\Bigg]\nonumber \\
 &= \mathbb{E}_{i}\left[s_{i,h}^2 \mathbb{E}_{\hat{\mathcal{D}}_i' } \left[ \left(\frac{1}{n_1}\sum_{k=1}^{n_1} f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \mathbf{x}_{i,k}^\top\mathbf{w}_j- \mathbb{E}_{\mathbf{x}'}\left[
f_{i}(\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right]\right)^2\right]\right]\nonumber \\
&\leq \mathbb{E}_{i}\left[s_{i,h}^2 \max_{i'} \mathbb{E}_{\hat{\mathcal{D}}_{i'}' } \left[ \left(\frac{1}{n_1}\sum_{k=1}^{n_1} f_{i'}(\mathbf{x}_{i',k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i',k}) \mathbf{x}_{i',k}^\top\mathbf{w}_j- \mathbb{E}_{\mathbf{x}'}\left[
f_{i'}(\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right]\right)^2\right]\right]\label{frf}\\
&= \mathbb{E}_{i}\left[s_{i,h}^2 \right] \max_{i'} \mathbb{E}_{\hat{\mathcal{D}}_{i'}' } \left[ \left(\frac{1}{n_1}\sum_{k=1}^{n_1} f_{i'}(\mathbf{x}_{i',k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i',k}) \mathbf{x}_{i',k}^\top\mathbf{w}_j- \mathbb{E}_{\mathbf{x}'}\left[
f_{i'}(\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right]\right)^2\right]\nonumber \\
 &=  \mathbb{E}_{i}\left[s_{i,h}^2 \right] O\left( \nu_{\mathbf{w}}^2 \frac{d +\log(m/\delta_1)}{n_1} \right) \label{rdr} \\
&=O\left( \overline{s_h^2}\nu_{\mathbf{w}}^2 \frac{d +\log(m/\delta_1) }{n_1} \right)  \nonumber 
\end{align}
where \eqref{frf} follows since $s_{i,h}^2\geq 0$ and \\
$ \mathbb{E}_{\hat{\mathcal{D}}_{i'}' } \left[ \left(\frac{1}{n_1}\sum_{k=1}^{n_1} f_{i'}(\mathbf{x}_{i',k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i',k}) \mathbf{x}_{i',k}^\top\mathbf{w}_j- \mathbb{E}_{\mathbf{x}'}\left[
f_{i'}(\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right]\right)^2\right]\geq 0$, and \eqref{rdr} follows since for all $i'$, $\frac{1}{n_1}\sum_{k=1}^{n_1} f_{i'}(\mathbf{x}_{i',k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i',k}) \mathbf{x}_{i',k}^\top\mathbf{w}_j- \mathbb{E}_{\mathbf{x}'}\left[
f_{i'}(\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right]$ is sub-Gaussian with mean zero and variance $O(\frac{\|\mathbf{w}_j\|_2^2}{n_1}) = O(\frac{d\nu_{\mathbf{w}}^2}{n_1})$. 
To control $\circled{3}$, note that
\begin{align}
    \circled{3} &= \mathbb{E}_i\Big[\Big(\mathbb{E}_{\mathbf{x}}\left[
f_{i}(\mathbf{x}) \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h\right] \mathbb{E}_{\mathbf{x}'} \left[f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right]\Big)^2\Big] \nonumber \\
&\quad \quad - \mathbb{E}_i\left[\mathbb{E}_{\mathbf{x}}\left[
f_{i}(\mathbf{x}) \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h\right] \mathbb{E}_{\mathbf{x}'} \left[f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right]\right]^2 \nonumber \\
&= \mathbb{E}_i\Big[s_{i,h}^2 \mathbb{E}_{\mathbf{x}'} \left[f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right]^2\Big]  \nonumber \\
&\leq  \mathbb{E}_i\Big[s_{i,h}^2 \max_{i'} \mathbb{E}_{\mathbf{x}'} \left[f_{i'}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right]^2\Big]  \nonumber \\
&=  \mathbb{E}_i[s_{i,h}^2]  \max_{i'} \mathbb{E}_{\mathbf{x}'} \left[f_{i'}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right]^2\Big]  \nonumber \\
&= \mathbb{E}_i\Big[s_{i,h}^2\Big] O( \nu_{\mathbf{w}}^2( d+ \log(m/\delta_1))  )  \nonumber \\
&= O( \overline{s_h^2}\nu_{\mathbf{w}}^2 (d + \log(m/\delta_1)  ) )
\end{align}
% \begin{align}
%     \circled{3} &= \mathbb{E}_i\Big[\Big(\mathbb{E}_{\mathbf{x}}\left[
% f_{i}(\mathbf{x}) \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h\right] \mathbb{E}_{\mathbf{x}'} \left[f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right] \nonumber \\
% &\quad \quad \quad \quad - \mathbb{E}_{i}\left[\mathbb{E}_{\mathbf{x}}\left[
% f_{i}(\mathbf{x}) \sigma'(\mathbf{w}_j^\top \mathbf{x}) {x}_h \right] \mathbb{E}_{\mathbf{x}'} \left[f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') (\mathbf{x}')^\top\mathbf{w}_j\right]\right] \Big)^2 \Big] \nonumber \\
% &=  \mathbb{E}_i\Big[\mathbb{E}_{\mathbf{x},\mathbf{x}'}\left[
% (f_{i}(\mathbf{x}) f_{i}(\mathbf{x}') -  \mathbb{E}_i[f_{i}(\mathbf{x}) f_{i}(\mathbf{x}')] )\sigma'(\mathbf{w}_j^\top \mathbf{x}) \sigma'(\mathbf{w}_j^\top\mathbf{x}') {x}_h (\mathbf{x}')^\top\mathbf{w}_j \right]^2\Big]  \nonumber \\
% &\leq  \mathbb{E}_{i,\mathbf{x},\mathbf{x}'}\left[
% (f_{i}(\mathbf{x}) f_{i}(\mathbf{x}') -  \mathbb{E}_i[f_{i}(\mathbf{x}) f_{i}(\mathbf{x}')] )^2 \right] \mathbb{E}_{\mathbf{x},\mathbf{x}'}\left[\sigma'(\mathbf{w}_j^\top \mathbf{x}) \sigma'(\mathbf{w}_j^\top\mathbf{x}') ( {x}_h (\mathbf{x}')^\top\mathbf{w}_j )^2\right]  \nonumber \\
% &= \mathbb{E}_{i,\mathbf{x},\mathbf{x}'}\left[
% (f_{i}(\mathbf{x}) f_{i}(\mathbf{x}') -  \mathbb{E}_i[f_{i}(\mathbf{x}) f_{i}(\mathbf{x}')] )^2 \right] O( d \nu_{\mathbf{w}}^2 )
% \end{align}
Combining the bounds on $\circled{1},\circled{2}$ and $\circled{3}$ yields $\mathbb{E}\left[({q}_{i,h} - \mathbb{E}[{q}_{i,h} ]  )^2 \right] = O(\nu_{\mathbf{w}}^2 (d+\log(m/\delta_1)) (\overline{s^2_h} + \frac{1}{n_2}) )$, therefore, since each random variable in $\{{q}_{i,h}\}_{i=1}^T$ is i.i.d.,
% $ \frac{1}{T}\sum_{i=1}^T {q}_{i,h} $ is sub-exponential with variance proxy $O(\frac{d \nu_{\mathbf{w}}^2 }{T})$. 
Bernstein's inequality gives
\begin{align}
   & \mathbb{P}_{\{{q}_{i,h}\}_i}\left(\left| \frac{1}{T}\sum_{i=1}^T {q}_{i,h} - \mathbb{E}[{q}_{i,h} ] \right| > t_h \right) \nonumber \\
   &\leq 2 \exp\left(- cT \min\left( \frac{t_h^2}{\nu_{\mathbf{w}}^2(d + \log(m/\delta_1)) ( \overline{s_h^2} + \frac{1}{n_2} )}, \frac{t_h}{\nu_{\mathbf{w}} \sqrt{d + \log(m/\delta_1)} \sqrt{ \overline{s_h^2} + \frac{1}{n_2} } }\right) \right) \label{berno}
    % \left(- \frac{ t \sqrt{T} }{ \nu_{\mathbf{w}}\sqrt{d} } \right) 
\end{align}
with probability at least $1- 3 \delta_1$ over the selection of $\mathbf{W}^0$ for an absolute constant $c$ and  any $t_h\geq 0$.
% as ${q}_{i,h}$ is sub-exponential with variance proxy $O( d \nu_{\mathbf{w}}^2 )$. 
Set $t_h=O\left(\nu_{\mathbf{w}} \sqrt{\frac{d + \log(m/\delta_1)}{T} (\overline{s_h^2} + \frac{1}{n_2}) \log(d/\delta) } \right)$ for all $h\in [d]$, then as long as $T \geq \log(d/\delta_2)$, via a union bound over all $h\in [d]$
we have
\begin{align}
    \left\| \frac{1}{T}\sum_{i=1}^T \mathbf{q}_i - \mathbb{E}[\mathbf{q}_i]  \right\|_2 &= \left( \sum_{h=1}^d \left( \frac{1}{T}\sum_{i=1}^T {q}_{i,h} - \mathbb{E}[{q}_{i,h}] \right)^2 \right)^{1/2} \nonumber \\
    &\leq  c \left( \sum_{h=1}^d \nu_{\mathbf{w}}^2 {\frac{d + \log(m/\delta_1)}{T} \left(\overline{s_h^2} + \frac{1}{n_2}\right) \log(d/\delta_2) }\right)^{1/2}  \label{bern} \\
    &= c \nu_{\mathbf{w}} \sqrt{\frac{d + \log(m/\delta_1)}{T} \log(d/\delta_2)} \left( \sum_{h=1}^d \overline{s_h^2} + \frac{d}{n_2} \right)^{1/2} \nonumber \\
    &= c \nu_{\mathbf{w}} \sqrt{\frac{d + \log(m/\delta_1)}{T} \log(d/\delta_2)} \left( \mathbb{E}_i\left[\sum_{h=1}^d s_{i,h}^2\right] + \frac{d}{n_2} \right)^{1/2} \nonumber \\
    &= c \nu_{\mathbf{w}} \sqrt{\frac{d + \log(m/\delta_1)}{T} \log(d/\delta_2)} \left( \mathbb{E}_i\left[\|\mathbf{s}_i\|_2^2\right] + \frac{d}{n_2} \right)^{1/2} \nonumber \\
    &\leq c' \nu_{\mathbf{w}} \sqrt{\frac{d + \log(m/\delta_1)}{T} \log(d/\delta_2)} \left(  r  +  \frac{r\|\mathbf{Mw}_j\|_2^2}{\|\mathbf{M}_\perp\mathbf{w}_j\|_2^2}  +  {\|\mathbf{Mw}_j\|_2^2 }+ \frac{d}{n_2} \right)^{1/2} \label{ou} \\
     &\leq c' \nu_{\mathbf{w}} \sqrt{\frac{d + \log(m/\delta_1)}{T} \log(d/\delta_2)} \left(  r (1+ \log(m/\delta_1) )  + \frac{d}{n_2} \right)^{1/2} \label{ouu} \\
    % &\leq O\left(\left( \frac{d^2 \log^2(d/\delta) \nu_{\mathbf{w}}^2 }{T} \right)^{1/2}\right) \nonumber \\
    &= O\left(\nu_{\mathbf{w}} \sqrt{\frac{d + \log(m/\delta_1)}{T} \log(d/\delta_2)}  \left(  \sqrt{r\log(m/\delta_1)} + \sqrt{\frac{d}{n_2}} \right) \right) \nonumber %\\
    % &\leq   \nonumber \\
    % &\leq  \exp\left(    \right)
\end{align}
with probability at least $1-3\delta_1-\delta_2$  for absolute constants $c,c'$, where \eqref{bern} follows with probability at least $1-3\delta_1-\delta_2$ due to \eqref{berno} and our choice of $t_h$, \eqref{ou} follows by Lemma \ref{lem:exp2} and the fact that $(a+b)^2\leq 2a^2+2b^2$, and \eqref{ouu} follows since $\mathbf{w}_j \in \mathcal{G}_{\mathbf{w}}$. Setting $\delta_1, \delta_2 = \Theta( \delta)$ completes the proof.
\end{proof}



% Finally, we use a truncated version of the matrix Bernstein inequality 
% to upper bound the RHS of \eqref{twonorms}, which is equivalent to $\|\frac{1}{T}\sum_{i=1}^T \mathbf{q}_i - \mathbb{E}[\mathbf{q}_i]\|_2$. Matrix Bernstein alone is insufficient because each $\mathbf{q}_i$ is unbounded. However, we 


% We have that since each $\mathbf{q}_i$ is sub-exponential, 
% Let $\diag(\mathbf{u})$ denote the diagonal matrix in $\mathbb{R}^{d\times d}$ whose diagonal elements are the elements of the vector $\mathbf{u}\in \mathbb{R}^d$. 

% We have






% Will ultimately get sth like min( d/T, r/T + d/n1 + d/n2 ) = r/T + d/(T+n1) + d/(T+n2) 

% ------

% We control ${\circled{1}}$ in \eqref{twonorms} using the truncated matrix (vector) Bernstein inequality from Lemma \ref{lem:trunc}.
% First, we need to bound the variance statistic. For ease of notation we define $\mathbf{q}_{i,k,l} \coloneqq f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) \mathbf{x}_{i,l}\mathbf{x}_{i,k}^\top\mathbf{w}_j \in \mathbb{R}^d$. We have
% \begin{align}
%     \mathbb{E}_{\mathbf{x}_{i,k},\mathbf{x}_{i,l}}[\|\mathbf{q}_{i,k,l} - \mathbb{E}_{\mathbf{x}_{i,k},\mathbf{x}_{i,l}}[\mathbf{q}_{i,k,l}]\|_2^2]&\leq 
% \end{align}

% Next, we apply with truncation level $\tau = \Omega()$ to obtain
% \begin{align}
%     \circled{1}\leq   \label{1w}
% \end{align}
% with probability at least $1 - $.

% fixing the selection of tasks, have a sum of Tn1n2 independent random matrices (not identically distributed, but thats fine). to get matrix variancce statistic, take max over any task (even beyond T).
% not totally independent


% instead, write as 
% Ei [ Ex[fi(x) x] Ex'[fi(x') x'] ]

% sum-i [ sum-x( fi(x) x) Ex'[fi(x') x'] ] - sum sum sum .... no this is n1

% with one sample/task you would get T concent

% so how to show more samples/task is better?

% sum-i (Ehat Ehat)

% we have sum of T random variables
% if there was one sample/task they would be mean zero

% should hope for 1/T(c + 1/n1 + 1/n2)

% Choose $\gamma = \Omega()$.

% \begin{align}
    
% \end{align}
% For term $\circled{1a}$, we have

% For term $\circled{1c}$, we have


% Now we apply the matrix Bernstein inequality to control $\circled{1b}$. We

% Note that for a fixed selection of tasks 




% \begin{align}
%     {\circled{1}}&\leq  \underbrace{\Bigg\| 
%         \frac{1}{T n_1 n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1}
% f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) \mathbf{x}_{i,l}\mathbf{x}_{i,k}^\top\mathbf{w}_j^0}_{\circled{1a}}
%        \nonumber \\
%        &\underbrace{- 
%         \frac{1}{T n_1 n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1}
% \tau_{\gamma}(f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) \mathbf{x}_{i,l}\mathbf{x}_{i,k}^\top\mathbf{w}_j^0)
%         \Bigg\|_2}_{\circled{1a}} \nonumber \\
%         & +  \underbrace{\Bigg\| \frac{1}{T n_1 n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1}
% \tau_{\gamma}(f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) \mathbf{x}_{i,l}\mathbf{x}_{i,k}^\top\mathbf{w}_j^0)}_{\circled{1b}}
%        \nonumber \\
%        &\underbrace{- 
%         \frac{1}{T } \sum_{i=1}^T \mathbb{E}_{(\mathbf{x}, f_i(\mathbf{x}))\sim \mathcal{D}_{i}} \mathbb{E}_{(\mathbf{x}', f_i(\mathbf{x}'))\sim \mathcal{D}_{i}}\left[ \tau_{\gamma}(f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j^0)\right]
%         \Bigg\|_2}_{\circled{1b}} \nonumber \\
%         & +  \underbrace{\Bigg\| \frac{1}{T n_1 n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1}
% \tau_{\gamma}(f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) \mathbf{x}_{i,l}\mathbf{x}_{i,k}^\top\mathbf{w}_j^0)}_{\circled{1c}}
%        \nonumber \\
%        &\underbrace{- 
%         \frac{1}{T } \sum_{i=1}^T \mathbb{E}_{(\mathbf{x}, f_i(\mathbf{x}))\sim \mathcal{D}_{i}} \mathbb{E}_{(\mathbf{x}', f_i(\mathbf{x}'))\sim \mathcal{D}_{i}}\left[ f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j^0\right]
%         \Bigg\|_2}_{\circled{1c}} \nonumber 
% \end{align}
% Maybe make a generic truncated matrix ebern lemma....


% \begin{lemma}[Truncated Matrix Bernstein]\label{lem:trunc}
% Suppose $Z_1,\dots,Z_n$ are $n$ independent random matrices.
% For some threshold $\tau$, 
% % 

% truncate only the centered r.v.'s

% Then
% \begin{align}
%     \mathbb{P}\left(\left|\sum_{i=1} \right| > t\right) &\leq 
% \end{align}

% \end{lemma}

% \begin{proof}
% define the truncation operator $ \tau_\gamma : \mathbb{R}^d\rightarrow \gamma\mathbb{B}^d $, where $\gamma\mathbb{B}^d$ is the Euclidean ball around the origin in $\mathbb{R}^d$ of radius $\gamma$, such that  $\tau_\gamma(\mathbf{v}) =  \frac{\min(\|\mathbf{v}\|_2, \gamma )}{\|\mathbf{v}\|_2}\mathbf{v}$. 

% \begin{align}
    
% \end{align}
% \end{proof}

\begin{comment}
Note that Lemma \ref{lem:grad_concen1} gives an upper bound on the error in the finite-sample gradient error that is small when $T$ is large, but does not decay with $n_1$ or $n_2$. Next we give an alternative bound that accounts for the regime in which $T$ may be smaller but $n_1$ and $n_2$ are large. 
\begin{lemma}

\end{lemma}


\begin{proof}
\begin{align}
 &\Bigg\| 
        % \nabla_{\mathbf{w}_j} \hat{\mathcal{L}}( \mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{i}^1\}_{i=1}^T; \{\hat{\mathcal{D}}_{i,\mathbf{W}}\}_{i=1}^T )  
        \frac{1}{T n_1 n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1}
f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) \mathbf{x}_{i,l}\mathbf{x}_{i,k}^\top\mathbf{w}_j
       \nonumber \\
       &-  \mathbb{E}_{i}\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right] 
        % \eta  2^{-r}  \mathbf{A}(\mathbf{w}_{j}^0) \mathbf{w}_{j}^0 
        \Bigg\|_2 \nonumber \\
        % &= \left\| \frac{1}{T} \sum_{i=1}^T \mathbf{q}_i -  \mathbb{E}_{i}\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right]  \right\|_2
        &\leq  \underbrace{\Bigg\| 
        \frac{1}{T n_1 n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1}
f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) \mathbf{x}_{i,l}\mathbf{x}_{i,k}^\top\mathbf{w}_j}_{\circled{1}}
       \nonumber \\
       &\quad \underbrace{- 
        \frac{1}{T } \sum_{i=1}^T \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right]
        \Bigg\|_2}_{\circled{1}} \nonumber \\
        & +  \underbrace{\Bigg\| 
        \frac{1}{T } \sum_{i=1}^T \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right]}_{\circled{2}}
       \nonumber \\
       &\quad \underbrace{-  \mathbb{E}_{i}\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right] 
        \Bigg\|_2}_{\circled{2}} 
        \label{twonorms}
\end{align}
    To control $\circled{2}$, observe that by rearranging the expectations and applying Assumption \ref{assump:diversity},
\begin{align}
    \circled{2} &= \left\|\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[ \left( \frac{1}{T}\sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')   -  \mathbb{E}_{i}[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')]\right)\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right] 
        \right\|_2 \nonumber \\
        &= \left\|\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[\chi\{ \sign(\mathbf{Mx})\neq \sign(\mathbf{Mx}') \} \left( \frac{1}{T}\sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')   -  \frac{1}{2}\right)\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right] 
        \right\|_2 \nonumber  \\
        &\leq \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[\left\| \chi\{ \sign(\mathbf{Mx})\neq \sign(\mathbf{Mx}') \} \left( \frac{1}{T}\sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')   -  \frac{1}{2}\right)\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}  (\mathbf{x}')^\top\mathbf{w}_j \right\|_2 \right] 
        \label{fnf}  \\
        &\leq \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[ \chi\{ \sign(\mathbf{Mx})\neq \sign(\mathbf{Mx}') \} \left| \frac{1}{T}\sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')   -  \frac{1}{2}\right| \left\| \sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}  (\mathbf{x}')^\top\mathbf{w}_j \right\|_2 \right] 
        \label{fnf2}  \\
        &\leq \left(\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[ \chi\{ \sign(\mathbf{Mx})\neq \sign(\mathbf{Mx}') \} \left| \frac{1}{T}\sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')   -  \frac{1}{2}\right|^2\right] \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[ \left\| \sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}  (\mathbf{x}')^\top\mathbf{w}_j \right\|_2^2 \right] \right)^{1/2}
        \label{fnf3}  %\\
        % &\leq  \left\|\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[\chi\{ \sign(\mathbf{Mx})\neq \sign(\mathbf{Mx}') \} \left( \frac{1}{T}\sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')   -  \frac{1}{2}\right) \right] \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[ \sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j^0\right] 
        % \right\|_2 \nonumber 
        % &=  \left\|\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[\chi\{ \sign(\mathbf{Mx})\neq \sign(\mathbf{Mx}') \} \left( \frac{1}{T}\sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')   -  \mathbb{E}_{i}[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')]\right)\sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j^0\right] 
        % \right\|_2 \nonumber \\
\end{align}
where \eqref{fnf} follows by Jensen's inequality,  and \eqref{fnf2} and \eqref{fnf3} follow by the Cauchy-Schwarz inequality.  
By  Lemma \ref{lem:tasks}, for all $(\mathbf{x},\mathbf{x}')$ such that $ \sign(\mathbf{Mx})\neq \sign(\mathbf{Mx}') $, we have that 
\begin{align}
  \left|  \frac{1}{T}\sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')   -  \frac{1}{2}\right| = O\left(\sqrt{\frac{r}{T}}\right)
\end{align}
with probability at least $1-1000^{-1}$, which implies
\begin{align}
    \circled{2} &\leq \sqrt{\frac{r}{T}} \left(  \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[ \left\| \sigma'(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}  (\mathbf{x}')^\top\mathbf{w}_j \right\|_2^2 \right] \right)^{1/2} \label{bg} \\
    &= O\left( \sqrt{\frac{rd}{T}}  \; \|\mathbf{w}_j\|_2\right) \label{bgh} \\
    &= O\left( \sqrt{\frac{r}{T}}  \;d \nu_{\mathbf{w}} \right) \label{bghn}
\end{align}
where \eqref{bg} follows with probability at least $1 - 1000^{-1}$, \eqref{bgh} follows by Cauchy-Schwarz and \eqref{bghn} follows with probability at least $1-1000^{-1}$ by Lemma \ref{lem:init}.
Combining \eqref{1w} and \eqref{bghn} via a union bound yields
\begin{align}
    \circled{1} + \circled{2} =  + \; O\left( \sqrt{\frac{r}{T}}  \; d\nu_{\mathbf{w}} \right)
\end{align}
with probability at least $1-1000^{-1}$, which completes the proof in light of \eqref{twonorms}.
\end{proof}

% \begin{align}
%     \nabla_{\mathbf{w}_{j,0}}\mathcal{L}(\mathbf{W}^0,\mathbf{b}^0,\{\mathbf{a}_{0,i}\}_{i}) &=
%     % \E_{i, \mathbf{x} }  \left[ \max\left( 1- \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}'} [ f_{i}(\mathbf{x}') g(\mathbf{x}';\mathbf{W}^0,\mathbf{b}^0 ) ]^\top g(\mathbf{x}; \mathbf{W}^0,\mathbf{b}^0)  , 0 \right) 
% %     \frac{1}{n_2}\sum_{j=1}^{n_2}\max \left(1 - y_{i,j} \left(\frac{1}{\lambda_{1}n_1}\sum_{j'=1}^{n_1}\bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})  \right)^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}), 0\right) \right] \nonumber\\
% % &= 1 -  \E_{i }  \left[ \frac{1}{\lambda_{1} n_1n_2}\sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})
% % \right] \label{14} \nonumber \\
%  -\E_{\mathbf{x}, \mathbf{x}' }  \left[  \mathbb{E}_i[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')] \mathbf{zz}'T \sigma'((\mathbf{w}_{j}^0)^\top \mathbf{x} + b_{j,0})\sigma'((\mathbf{w}_{j}^0)^\top \mathbf{x}' + b_{j,0})  \right]
% \end{align}

\begin{lemma}\label{lem:tasks}
    % Suppose the set of tasks $\mathcal{T}$ is defined as:
    % \begin{align}
    %     \mathcal{T} \coloneqq \{ f_i^*:\{-1,1\}^r \rightarrow \{-1,1\} | f_i^*(\mathbf{v}) = \prod_{j \in A} v_j, \; A \subseteq [r]  \}.
    % \end{align}
    % Then 
    Under Assumption \ref{assump:diversity}, for all $(\mathbf{v},\mathbf{v}')\in \{-1,1\}^r \times  \{-1,1\}^r$ such that $\mathbf{v}\neq  \mathbf{v}'$,
    \begin{align}
       \left| \frac{1}{T}\sum_{i=1}^T \chi\{\bar{f}_i(\mathbf{v}) \neq \bar{f}_i(\mathbf{v}')\} - \frac{1}{2}\right| &= O\left(\frac{\sqrt{r}}{\sqrt{T}}\right)
    \end{align}
    with probability at least $0.999$ over the random draw of $T$ tasks from $\mathcal{T}$.
\end{lemma}

\begin{proof}
% Let $\mathbf{v}_1,\dots,\mathbf{v}_{2^r}$ denote an ordering of the $2^r$ vertices on the $r$-dimensional hypercube $\{-1,1\}^r$.
% Note that any task $f_i^*: \{-1,1\}^r \rightarrow \{-1,1\}$ can be represented as a vector $f_i$ in $ \{ -1, 1\}^{2^r}$. 
% Note that for any differing v,v', 
Under Assumption \ref{assump:diversity}, each $\chi\{\bar{f}_i(\mathbf{v}) \neq \bar{f}_i(\mathbf{v}')\}$ is an i.i.d. Bernoulli random variable with parameter $\frac{1}{2}$. Thus, for any particular $(\mathbf{v},\mathbf{v}')\in \{-1,1\}^r \times  \{-1,1\}^r$ such that $\mathbf{v}\neq \pm \mathbf{v}'$, we have by Hoeffding's inequality
\begin{align}
    \mathbb{P}\left[ \left| \frac{1}{T}\sum_{i=1}^T \chi\{\bar{f}_i(\mathbf{v}) \neq \bar{f}_i(\mathbf{v}')\} - \frac{1}{2}\right|   \geq t\right] \leq \exp\left( - \frac{T t^2}{2} \right) 
\end{align}
for any $t\geq 0$.  
Union bounding over all $O\left(2^{2r}\right)$ pairs $(\mathbf{v},\mathbf{v}')\in \{-1,1\}^r \times  \{-1,1\}^r$ and choosing $t = \frac{\sqrt{c'\log(2^{2r})}}{\sqrt{T}}$ completes the proof.
% {\color{red}
% For linear tasks to work:
% Need number of points that cover unit sphere such that angle is small (like o(2**-r)) is small (O(2**r)). maybe too much to hope for. ignore until end.
% if inputs are on cube: then use hoeffding, again
% }
\end{proof}

\end{comment}


\begin{lemma}\label{lem:compute_grad}
For any $\delta\in (0,1)$, with probability at least $1- \delta$, for all  $j\in [m]$,
% such that $\mathbf{w}_{j}^0\in \mathcal{G}_{\mathbf{w}}$, then 
% $\nabla_{\mathbf{w}_j}\mathcal{L}(\mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{1,i} \}_{i\in \mathcal{T}})$
    % The gradient of the global loss with respect to the representation after updating the task-specific heads on the first iteration is $-\frac{1}{2^{r}\lambda_1}\mathbf{A}(\w)\w$, where
%     \begin{align}
%     \w^+ &= \w(1 - \eta \lambda) + \eta \begin{bmatrix}
%         \mathbf{A}_{||,||}(\w) &  \mathbf{A}_{||,\perp}(\w) \\
%         \mathbf{A}_{\perp,||}(\w) & \mathbf{A}_{\perp,\perp}(\w) \\
%     \end{bmatrix}\w
% \end{align}
    \begin{align}
\nabla_{\mathbf{w}_j} \hat{\mathcal{L}}( \mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{i}^1\}_{i=1}^T; \{\hat{\mathcal{D}}_{i,\mathbf{W}}\}_{i=1}^T )  &=  - \eta  2^{-r}  \mathbf{A}(\mathbf{w}_{j}^0) \mathbf{w}_{j}^0 + \eta \mathbf{e}  %\\\lambda_{\mathbf{w}}\mathbf{w}_{j,0} 
 % & \coloneqq \begin{bmatrix}
 %        \mathbf{A}_{||,||}(\w) &  \mathbf{A}_{||,\perp}(\w) \\
 %        \mathbf{A}_{\perp,||}(\w) & \mathbf{A}_{\perp,\perp}(\w) \\
 %    \end{bmatrix} 
\end{align} 
where 
% \begin{align}\|\mathbf{e} \|_2 &=  \eta\nu_{\mathbf{w}}
% % O( \nu_{\mathbf{w}} de^{-c d } + \nu_{\mathbf{w}} d \frac{\sqrt{r}}{\sqrt{T}} )
%   O\left( d  \sqrt{\log(Tn_2)} \left(1 + {\tfrac{ \sqrt{\log(T)}}{\sqrt{n_1}}}\right) \left(  \exp \left(-\frac{ {c}}{ \eta^2  \nu_{\mathbf{w}}^2{dm} (d+m) \log(T)}     \right) + \frac{1}{\sqrt{Tn_2}}\right) \right)\nonumber \\
%   &\quad  +O\left( \sqrt{\frac{d}{T} \log(d/\delta)}  \left(  \sqrt{r\log(m/\delta)} + \sqrt{\frac{d}{n_2}} \right) \right), \nonumber
%   % O\left( \frac{ \eta \sqrt{d} \log(d)\nu_{\mathbf{w}}}{\sqrt{T}} 
%   % \right)
%  % O\left( m \exp \left(-\frac{ {1}}{ c\eta m d^2 \nu_{\mathbf{w}}^2 }     \right) \right)  +   O\left(  \frac{  1 }{ \sqrt{Tn_2} } \right) + O\left( \frac{\sqrt{d} \log(d) \nu_{\mathbf{w}} }{\sqrt{T}} \right)
% \end{align} 
\begin{align}\|\mathbf{e} \|_2 &=  \nu_{\mathbf{w}}\;
% O( \nu_{\mathbf{w}} de^{-c d } + \nu_{\mathbf{w}} d \frac{\sqrt{r}}{\sqrt{T}} )
O\Bigg( (\sqrt{d} + \sqrt{\log(m/\delta)}) \sqrt{d\log(Tn_2/\delta)} \left(1 + {\frac{ \sqrt{\log(T/\delta)}}{\sqrt{n_1}}}\right) \nonumber \\
     &\quad \quad \quad \quad \times \left(   \exp \left( -\frac{ c }{\eta^2  \nu_{\mathbf{w}}^2 {m\log(T/\delta)}({d} + {\log(m/\delta)}) ({d} + {m} )} \right) + \frac{\sqrt{\log(1/\delta)}}{\sqrt{Tn_2}}\right) \Bigg) \nonumber \\
     &\quad + \nu_{\mathbf{w}}\; O\left( \sqrt{\frac{d + \log(m/\delta)}{T} \log(d/\delta)}  \left(  \sqrt{r\log(m/\delta)} + \sqrt{\frac{d}{n_2}} \right) \right)
  % O\left( \frac{ \eta \sqrt{d} \log(d)\nu_{\mathbf{w}}}{\sqrt{T}} 
  % \right)
 % O\left( m \exp \left(-\frac{ {1}}{ c\eta m d^2 \nu_{\mathbf{w}}^2 }     \right) \right)  +   O\left(  \frac{  1 }{ \sqrt{Tn_2} } \right) + O\left( \frac{\sqrt{d} \log(d) \nu_{\mathbf{w}} }{\sqrt{T}} \right)
\end{align} 
and  for a vector $\mathbf{w}\in \mathbb{R}^d$,
\begin{align}
    \mathbf{A}(\mathbf{w}) \coloneqq  \mathbb{E}_{\mathbf{u}} \Big[ \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[{\sigma}'(\mathbf{w}^\top\mathbf{x}')\sigma'(\mathbf{w}^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top | \sign(\mathbf{M}\mathbf{x})  =  \sign(\mathbf{M}\mathbf{x}') = \mathbf{u}\Big] \Big]
\end{align}
where $\mathbf{u}\sim \text{Unif}(\mathcal{H}^r)$ is a  random vector  drawn uniformly from the Rademacher hypercube in $r$ dimensions.
\end{lemma}



\begin{proof}
% Using  Lemma \ref{lem:loss}, we have  
% % \begin{align}  
% % % &  \frac{1}{\lambda_{1}  } \mathbb{E}_{\mathbf{x},\mathbf{x}',i} \left[  f_{i}(\mathbf{x}) f_{i}(\mathbf{x}') \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz})\right] \nonumber \\
% % &\mathcal{L}(\mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{1,i} \}_{i\in \mathcal{T}})\nonumber \\
% % &=  \eta  \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) <1\}\nonumber \\
% % &\quad\quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \}  \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz}) \Big] \nonumber \\
% % &= \eta  \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \}  \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz}) \Big] \nonumber \\
% % &\quad  - \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\}\nonumber \\
% % &\quad\quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \}  \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz}) \Big] \nonumber  
% % \end{align} 
% \begin{align}
% &\mathcal{L}(\mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{i}^1 \}_{i\in [T]})\nonumber \\
% &=  1 -  \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[ \chi\{\sign(\mathbf{M}\mathbf{x}) = \sign(\mathbf{M}\mathbf{x}') \} \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})  \right] \nonumber \\
% &\quad - \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{M}\mathbf{x}) \neq  \sign(\mathbf{M}\mathbf{x}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
% &\quad + \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\right\} \nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - \eta f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber 
% \end{align}
Let $\mathbf{w}_j = \mathbf{w}_{j}^0$. We have
\begin{align}
    &\nabla_{\mathbf{w}_j} \hat{\mathcal{L}}( \mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{i}^1\}_{i=1}^T; \{\hat{\mathcal{D}}_{i,\mathbf{W}}\}_{i=1}^T ) \nonumber \\
    &= -\frac{\eta}{T n_1 n_2} \sum_{i=1}^T \sum_{l=1}^{n_2}  \sum_{k=1}^{n_1}
f_{i}(\mathbf{x}_{i,l})  f_{i}(\mathbf{x}_{i,k})\sigma'(\mathbf{w}_j^\top\mathbf{x}_{i,k}) \sigma'(\mathbf{w}_j^\top \mathbf{x}_{i,l}) \mathbf{x}_{i,l}\mathbf{x}_{i,k}^\top\mathbf{w}_j  + \eta \mathbf{e}_1\label{rdr} \\
&= - \eta \mathbb{E}_{i\sim \mathcal{T}}\mathbb{E}_{(\mathbf{x}, f_i(\mathbf{x}))\sim \mathcal{D}_{i}} \mathbb{E}_{(\mathbf{x}', f_i(\mathbf{x}'))\sim \mathcal{D}_{i}}\left[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}) \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right] 
        % \eta  2^{-r}  \mathbf{A}(\mathbf{w}_{j}^0) \mathbf{w}_{j}^0 
        + \eta \mathbf{e}_1 + \eta \mathbf{e}_2
\end{align} 
where \begin{align}
\|\mathbf{e}_1\|_2 &=  O\Bigg( \nu_{\mathbf{w}} (\sqrt{d} + \sqrt{\log(m/\delta_1)}) \sqrt{d\log(Tn_2/\delta_1)} \left(1 + {\frac{ \sqrt{\log(T/\delta_1)}}{\sqrt{n_1}}}\right) \nonumber \\
     &\quad \quad \quad \quad \times \left(   \exp \left( -\frac{ c }{\eta^2  \nu_{\mathbf{w}}^2 {m(\log(T/\delta_1))}({d} + {\log(m/\delta_1)}) ({d} + {m} )} \right) + \frac{\sqrt{\log(1/\delta_1)}}{\sqrt{Tn_2}}\right) \Bigg)\nonumber \end{align}
with probability at least $1-\delta_1$ by Lemma \ref{lem:emp_grad} and \begin{align}
\|\mathbf{e}_2\|_2 = O\left(\nu_{\mathbf{w}} \sqrt{\frac{d + \log(m/\delta_2)}{T} \log(d/\delta_2)}  \left(  \sqrt{r\log(m/\delta_2)} + \sqrt{\frac{d}{n_2}} \right) \right)\end{align} with probability at least $1-\delta_2$ by Lemma \ref{lem:grad_concen1}. Set $\delta_1,\delta_2=\Theta(\delta)$ and apply the triangle inequality to complete the bound on $\| \mathbf{e}\|_2=\|\mathbf{e}_1+\mathbf{e}_2\|_2$ in the theorem statement. 

Next, for ease of notation we replace $\mathbb{E}_{(\mathbf{x}, f_i(\mathbf{x}))\sim \mathcal{D}_{i}} \mathbb{E}_{(\mathbf{x}', f_i(\mathbf{x}'))\sim \mathcal{D}_{i}}$ with $\mathbb{E}_{\mathbf{x},\mathbf{x}'}$ and $\mathbb{E}_{i\sim \mathcal{T}}$ with $\mathbb{E}_i$. Also, let $\mathbf{u} \sim \text{Unif}(\mathcal{H}^r)$ be uniformly drawn from the $r$-dimensional Rademacher hypercube $\mathcal{H}^r=\{-1,1\}^r$.
We have
\begin{align}
  &  \mathbb{E}_{i}\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\sigma'(\mathbf{w}_j^\top\mathbf{x}) \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right]  \nonumber \\
  &= \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[  \mathbb{E}_{i}[f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')]\sigma'(\mathbf{w}_j^\top\mathbf{x}) \sigma'(\mathbf{w}_j^\top \mathbf{x}') \mathbf{x}(\mathbf{x}')^\top\mathbf{w}_j\right]  \nonumber \\
  &= \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{\sign(\mathbf{M}\mathbf{x})  =  \sign(\mathbf{M}\mathbf{x}') \} {\sigma}'(\mathbf{w}_{j}^\top\mathbf{x}') \sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top \mathbf{w}_j \Big] \nonumber \\
  &= 2^{-r}  \mathbb{E}_{\mathbf{u}} \Big[ \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[{\sigma}'(\mathbf{w}_{j}^\top\mathbf{x}')\sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top | \sign(\mathbf{M}\mathbf{x})  =  \sign(\mathbf{M}\mathbf{x}') = \mathbf{u}\Big] \Big] \mathbf{w}_{j} \nonumber \\
  &= - 2^{-r}\mathbf{A}(\mathbf{w}_{j}) \mathbf{w}_{j} \label{shm}
\end{align}
where \eqref{shm} follows by the definition of $\mathbf{A}(\mathbf{w})$.
\end{proof}


\subsection{Analysis of the population gradient}

Next we define matrices capturing the energy of $\mathbf{A}(\mathbf{w}_j)$ in the ground-truth subspace and its perpendicular complement. 
% $\mathbf{A}(\mathbf{w}_{j}^0) \coloneqq \begin{bmatrix}
%          \mathbf{A}_{||,||}(\mathbf{w}_{j}^0) &  \mathbf{A}_{||,\perp}(\mathbf{w}_{j}^0) \\
%          \mathbf{A}_{\perp,||}(\mathbf{w}_{j}^0) & \mathbf{A}_{\perp,\perp}(\mathbf{w}_{j}^0) \\
%    \end{bmatrix} $ 
   % for matrices $\mathbf{A}_{\parallel,\parallel}(\mathbf{w}_{j}^0) \in \mathbb{R}^{r \times r}$, $\mathbf{A}_{\parallel,\perp}(\mathbf{w}_{j}^0) \in \mathbb{R}^{r \times (d-r)}$,  $\mathbf{A}_{\perp,\parallel}(\mathbf{w}_{j}^0) \in \mathbb{R}^{r \times (d-r)}$, $\mathbf{A}_{\perp,\perp}(\mathbf{w}_{j}^0) \in \mathbb{R}^{(d-r) \times (d-r)}$. 
   Again let  $\mathbf{u}\sim \text{Unif}(\mathcal{H}^r)$ be a random variable drawn uniformly from the Rademacher hypercube in $r$ dimensions, and $\mathbf{x}$ and $\mathbf{x}'$ be drawn independently from $\mathcal{N}(\mathbf{0}_d,\mathbf{I}_d)$, then for any $\mathbf{w}\in \mathbb{R}^d$ the matrices $\mathbf{A}_{||,||}(\w)$, $\mathbf{A}_{||,\perp}(\w)$, $\mathbf{A}_{\perp,||}(\w)$, and $\mathbf{A}_{\perp,\perp}(\w)$ are defined as
\begin{align}
    \mathbf{A}_{||,||}(\w) &= \mathbf{M}\mathbf{A}(\mathbf{w})\mathbf{M}^\top =
    % \mathbb{E}_{\mathbf{x}} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2 \mathbf{uu}^\top  
    \mathbb{E}_{\mathbf{u}} \left[   \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[
    {\sigma}'(\mathbf{w}^\top  \mathbf{x}) \sigma'(\mathbf{w}^\top \mathbf{x}') \mathbf{M}\mathbf{x}(\mathbf{x}')^\top\mathbf{M}^\top |\sign(\mathbf{M}\mathbf{x})  =  \sign(\mathbf{M}\mathbf{x}') = \mathbf{u}
    \right] \right]\\
    \mathbf{A}_{||,\perp}(\w) &= \mathbf{M}\mathbf{A}(\mathbf{w})\mathbf{M}_\perp^\top = \mathbb{E}_{\mathbf{u}} \left[   \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[\sigma'( \mathbf{w}^\top \mathbf{x})  \sigma'(\mathbf{w}^\top \mathbf{x})\mathbf{M}\mathbf{x} (\mathbf{x}')^\top \mathbf{M}_\perp^\top | \sign(\mathbf{M}\mathbf{x})  =  \sign(\mathbf{M}\mathbf{x}') = \mathbf{u} \right]\right] \\
    \mathbf{A}_{\perp,||}(\w) &= \mathbf{M}_\perp\mathbf{A}(\mathbf{w})\mathbf{M}^\top =  \mathbb{E}_{\mathbf{u}}\left[\mathbb{E}_{\mathbf{x},\mathbf{x}'}\left[\sigma'( \mathbf{w}^\top \mathbf{x} )\sigma'( \mathbf{w}^\top \mathbf{x}' ) \mathbf{M}_\perp \mathbf{x}(\mathbf{x}')^\top \mathbf{M}^\top  |\sign(\mathbf{M}\mathbf{x})  =  \sign(\mathbf{M}\mathbf{x}') = \mathbf{u}\right] \right]   \\
    \mathbf{A}_{\perp,\perp}(\w) &= \mathbf{M}_\perp\mathbf{A}(\mathbf{w})\mathbf{M}_\perp^\top =  \mathbb{E}_{\mathbf{u}}\left[ \mathbb{E}_{,\mathbf{x},\mathbf{x}'}\left[ \sigma'( \mathbf{w}^\top \mathbf{x} )\sigma'( \mathbf{w}^\top \mathbf{x}' ) \mathbf{M}_\perp \mathbf{x}(\mathbf{x}')^\top \mathbf{M}_\perp^\top |  \sign(\mathbf{M}\mathbf{x})  =  \sign(\mathbf{M}\mathbf{x}') = \mathbf{u}\right]\right]
    % \mathbf{A}_{||,\perp}(\w) &= \mathbb{E}_{\mathbf{}\sim \Unif(\mathcal{H}^{r})}\left[ \mathbb{E}_{\mathbf{v}\sim \Unif( \mathcal{H}^{d-r})} \left[\sigma'( \mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right] \mathbf{u} \mathbb{E}_{\mathbf{v}\sim \Unif(\mathcal{H}^{d-r})}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right] \\
    % \mathbf{A}_{\perp,||}(\w) &=  \mathbb{E}_{\mathbf{u}\sim \Unif(\mathcal{H}^{r})}\left[  \mathbb{E}_{\mathbf{v}\sim \Unif(\mathcal{H}^{d-r})}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right] \mathbb{E}_{\mathbf{v}\sim \Unif(\mathcal{H}^{d-r})} \left[\sigma'( \mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\right] \mathbf{u}^\top  \right] \\
    % \mathbf{A}_{\perp,\perp}(\w) &=  \mathbb{E}_{\mathbf{u}\sim \Unif(\mathcal{H}^{r})}\left[  \mathbb{E}_{\mathbf{v}\sim \Unif( \mathcal{H}^{d-r})}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]  \mathbb{E}_{\mathbf{v}\sim \Unif(\mathcal{H}^{d-r})}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right] 
\end{align}


% Taking the gradient of both terms with respect to $\mathbf{w}_j$ yields
% \begin{align}  
% % &  \frac{1}{\lambda_{1}  } \mathbb{E}_{\mathbf{x},\mathbf{x}',i} \left[  f_{i}(\mathbf{x}) f_{i}(\mathbf{x}') \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz})\right] \nonumber \\
% &\nabla_{\mathbf{w}_j}\mathcal{L}(\mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{i}^1 \}_{i\in [T]})\nonumber \\
% &= -  \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{\sign(\mathbf{M}\mathbf{x})  =  \sign(\mathbf{M}\mathbf{x}') \} {\sigma}(\mathbf{w}_{j}^\top\mathbf{x}') \sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x} \Big] \nonumber \\
% &\quad - \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{M}\mathbf{x}) \neq  \sign(\mathbf{M}\mathbf{x}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x} \right]   \nonumber \\
% &\quad - \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{w}_{j}^\top\mathbf{x}'' ) ]^\top \sigma(\mathbf{w}_{j}^\top\mathbf{x}) >1\} {\sigma}(\mathbf{w}_{j}^\top\mathbf{x}') \sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x} \Big] \nonumber  \\
% &= \eta 2^{-r}  \mathbb{E}_{\mathbf{u}} \Big[ \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[{\sigma}'(\mathbf{w}_{j}^\top\mathbf{x}')\sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top | \sign(\mathbf{M}\mathbf{x})  =  \sign(\mathbf{M}\mathbf{x}') = \mathbf{u}\Big] \Big] \mathbf{w}_{j}^0\nonumber \\
% &\quad - \eta  \E_{\mathbf{x}, \mathbf{x}' }  \Bigg[\chi\{\sign(\mathbf{M}\mathbf{x}) \neq  \sign(\mathbf{M}\mathbf{x}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right) \nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \times \sigma'(\mathbf{w}_{j}^\top\mathbf{x}')^\top \sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top \Bigg] \mathbf{w}_{j}^0   \nonumber \\
% &\quad - \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\}\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{M}\mathbf{x})  =  \sign(\mathbf{M}\mathbf{x}') \} {\sigma}'(\mathbf{w}_{j}^\top\mathbf{x}')\sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top\Big]\mathbf{w}_{j} \label{shm} \\
% &= \eta 2^{-r}\mathbf{A}(\mathbf{w}_{j}^0) \mathbf{w}_{j}^0 \nonumber \\
% &\quad - \eta  \E_{\mathbf{x}, \mathbf{x}' }  \Bigg[\chi\{\sign(\mathbf{M}\mathbf{x}) \neq  \sign(\mathbf{M}\mathbf{x}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \times \sigma'(\mathbf{w}_{j}^\top\mathbf{x}')^\top \sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top \Bigg] \mathbf{w}_{j}^0   \nonumber \\
% &\quad - \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\}\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{M}\mathbf{x})  =  \sign(\mathbf{M}\mathbf{x}') \} {\sigma}'(\mathbf{w}_{j}^\top\mathbf{x}')\sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top\Big]\mathbf{w}_{j}^0 \label{shmm} 
% \end{align} 
% where we have used $\sigma(x)= \sigma'(x)x$ in \eqref{shm}. It is easy to check that the first term in \eqref{shm} is equal to $\eta 2^{-r}\mathbf{A}(\mathbf{w}_{j}) \mathbf{w}_{j}$ by definition of $\mathbf{A}(\mathbf{w}_{j})$. Now we show that the remaining terms are small.
% The norm of the second term in \eqref{shmm} can be bounded using Jensen's Inequality (which implies $\|\mathbb{E}_{\mathbf{x}}[\mathbf{x}]\|_2\leq \mathbb{E}_{\mathbf{x}}[\|\mathbf{x}\|_2]$  for any random vector $\mathbf{x}$) and the Cauchy-Schwarz Inequality as:
% % \begin{align}
% %     & \left\|\eta \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top \right] \mathbf{w}_{j}^0   \right\|_2 \nonumber \\
% %     &\leq  \eta \|\mathbf{w}_{j}^0 \|_2 \E_{\mathbf{x}, \mathbf{x}' }  \left[ \left\| \chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')^\top \sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top   \right\|_2\right]  \nonumber \\
% %     &\leq \eta \|\mathbf{w}_{j}^0 \|_2 \sqrt{ \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)^2 \right]\E_{\mathbf{x}, \mathbf{x}' }  \left[\| \mathbf{x}\|_2^4 \right] } \nonumber \\
% %     &\leq \eta \|\mathbf{w}_{j}^0 \|_2 \sqrt{ \frac{ c' r d^2 }{T} } \nonumber \\
% %     &= \eta \nu_{\mathbf{w}} c''\frac{\sqrt{r}d^{1.5}}{\sqrt{T}}
% % \end{align}
% \begin{align}
%     & \Big\|\eta \E_{\mathbf{x}, \mathbf{x}' }  \big[\chi\{\sign(\mathbf{M}\mathbf{x}) \neq  \sign(\mathbf{M}\mathbf{x}') \} \left(\tfrac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma'(\mathbf{w}_{j}^\top\mathbf{x}')\sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top \big]\mathbf{w}_{j}^0   \Big\|_2 \nonumber \\
%     &\leq \eta \Bigg(\E_{\mathbf{x}, \mathbf{x}' }  \left[\left\| \chi\{\sign(\mathbf{M}\mathbf{x}) \neq  \sign(\mathbf{M}\mathbf{x}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma'(\mathbf{w}_{j}^\top\mathbf{x}')\sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x}\right\|_2^2 \right] \nonumber \\
%     &\quad \quad \quad \E_{\mathbf{x}, \mathbf{x}' }  \left[((\mathbf{x}')^\top \mathbf{w}_{j}^0)^2 \right] \Bigg)^{1/2} \nonumber \\
%     &= \eta \| \mathbf{w}_{j}^0\|_2 \nonumber \\
%     &\quad \times \E_{\mathbf{x}, \mathbf{x}' }  \left[\left\| \chi\{\sign(\mathbf{M}\mathbf{x}) \neq  \sign(\mathbf{M}\mathbf{x}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma'(\mathbf{w}_{j}^\top\mathbf{x}')\sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x}\right\|_2^2 \right]^{1/2}  \nonumber \\
%     &\leq \eta \| \mathbf{w}_{j}^0\|_2  \E_{\mathbf{x}, \mathbf{x}' } \left[\left\| \chi\{\sign(\mathbf{M}\mathbf{x}) \neq  \sign(\mathbf{M}\mathbf{x}') \}\sigma'(\mathbf{w}_{j}^\top\mathbf{x}')\sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x} \right\|_2^4 \right]^{1/4} \nonumber
%     \\
%     &\quad \quad \times \E_{\mathbf{x}, \mathbf{x}' } \left[ \left( \frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}')\right)^4 \right]^{1/4} \nonumber \\
%     &\leq  \eta \| \mathbf{w}_{j}^0\|_2  \E_{\mathbf{x}, \mathbf{x}' } \left[\left\| \chi\{\sign(\mathbf{M}\mathbf{x}) \neq  \sign(\mathbf{M}\mathbf{x}') \}\sigma'(\mathbf{w}_{j}^\top\mathbf{x}')\sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x} \right\|_2^4 \right]^{1/4} c \sqrt{\frac{r}{T}} \nonumber
%     \\
%     &\leq \eta \| \mathbf{w}_{j}^0\|_2  \E_{\mathbf{x}, \mathbf{x}' } \left[\chi\{\sign(\mathbf{M}\mathbf{x}) \neq  \sign(\mathbf{M}\mathbf{x}') \}\sigma'(\mathbf{w}_{j}^\top\mathbf{x}')\sigma'(\mathbf{w}_{j}^\top\mathbf{x})\right]^{1/8} \E_{\mathbf{x}} \left[ \left\|\mathbf{x} \right\|_2^8 \right]^{1/8} c \sqrt{\frac{r}{T}}\label{gh}
%     \\
%     % &\leq \eta \| \mathbf{w}_{j}^0\|_2  \E_{\mathbf{x}, \mathbf{x}' } \left[\chi\{\sign(\mathbf{M}\mathbf{x}) \neq  \sign(\mathbf{M}\mathbf{x}') \}\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\right]^{1/8} \E_{\mathbf{x}} \left[ \left\|\mathbf{x} \right\|_2^8 \right]^{1/8} c \sqrt{\frac{r}{T}} \nonumber \\
%     &\leq 
%     \eta \| \mathbf{w}_{j}^0\|_2 \E_{\mathbf{x}} \left[ \left\|\mathbf{x} \right\|_2^8 \right]^{1/8} c \sqrt{\frac{r}{T}} \nonumber \\
%     &= 
%     \eta \| \mathbf{w}_{j}^0\|_2 (d(d+2)(d+4)(d+6))^{1/8} c \sqrt{\frac{r}{T}} \nonumber\\
%     &\leq c' \eta \nu_{\mathbf{w}} \sqrt{\frac{r(d^2+d\log(m))}{T}}\label{gfg} \\
%     &\leq c'' \nu_{\mathbf{w}} d \sqrt{\frac{r}{T}}  \nonumber
%     % \eta \|c' \eta  \sqrt{\frac{r(d^2+d\log(m))}{T}}\mathbf{w}_{j}^0 \|_2 \E_{\mathbf{x}, \mathbf{x}' }  \left[ \left\| \chi\{\sign(\mathbf{M}\mathbf{x}) \neq  \sign(\mathbf{M}\mathbf{x}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')^\top \sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top   \right\|_2\right]  \nonumber \\
%     % &\leq \eta \|\mathbf{w}_{j}^0 \|_2 \sqrt{ \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{M}\mathbf{x}) \neq  \sign(\mathbf{M}\mathbf{x}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}(\mathbf{x})  f_{i}(\mathbf{x}') \right)^2 \right]\E_{\mathbf{x}, \mathbf{x}' }  \left[\| \mathbf{x}\|_2^4 \right] } \nonumber \\
%     % &\leq \eta \|\mathbf{w}_{j}^0 \|_2 \sqrt{ \frac{ c' r d^2 }{T} } \nonumber \\
%     % &= \eta \nu_{\mathbf{w}} c''\frac{\sqrt{r}d^{1.5}}{\sqrt{T}}
% \end{align}
% %https://math.stackexchange.com/questions/2945294/expectation-of-the-norm-of-a-gaussian-vector-raised-to-a-power
% where \eqref{gh} follows with probability at least 0.999 by Lemma \ref{lem:tasks} and \eqref{gfg} follows deterministically since $\mathbf{w}_{j}^0\in \mathcal{G}_{\mathbf{w}}$ and $\eta=\Theta(1)$.

%     The norm of the third term in \eqref{shm} can similarly be bounded as:
% \begin{align}
%     &\Big\|\eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\}\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{M}\mathbf{x})  =  \sign(\mathbf{M}\mathbf{x}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'(\mathbf{w}_{j}^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top\Big]\mathbf{w}_{j}^0 \Big\|_2 \nonumber \\
% &\leq \eta  \mathbb{E}_{\mathbf{x}'}[\chi\{ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'') ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\}]^{1/2}\nonumber \\
% &\quad \times \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{\sign(\mathbf{M}\mathbf{x})  =  \sign(\mathbf{M}\mathbf{x}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'(\mathbf{w}_{j}^\top\mathbf{x})\|\mathbf{x}\|_2^2 ((\mathbf{x}')^\top\mathbf{w}_{j}^0)^2\Big]^{1/2} \nonumber \\
% &\leq \eta \mathbb{P}_{\mathbf{x}} \big[ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\big]^{1/2}  \nonumber \\
% &\quad \quad \times \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{\sign(\mathbf{M}\mathbf{x})  =  \sign(\mathbf{M}\mathbf{x}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'(\mathbf{w}_{j}^\top\mathbf{x})\|\mathbf{x}\|_2^4 \Big]^{1/4} \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[((\mathbf{x}')^\top\mathbf{w}_{j}^0)^4 \Big]^{1/4} \nonumber \\
% &\leq \eta \mathbb{P}_{\mathbf{x}} \big[ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\big]^{1/2}  \nonumber \\
% &\quad \quad \times \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{\sign(\mathbf{M}\mathbf{x})  =  \sign(\mathbf{M}\mathbf{x}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'(\mathbf{w}_{j}^\top\mathbf{x})\|\mathbf{x}\|_2^4 \Big]^{1/4} \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[((\mathbf{x}')^\top\mathbf{w}_{j}^0)^4 \Big]^{1/4} \nonumber \\
% &= c \;\nu_{\mathbf{w}} \;d \;\mathbb{P}_{\mathbf{x}} \big[ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\big]  \label{56}
% \end{align}
% where the last line follows since $\eta=\Theta(1)$.
% % where \eqref{cs1} follows by the Cauchy-Schwarz Inequality, \eqref{less} follows by Jensen's Inequality, and 
% % \eqref{bbb} follows with probability at least $1-$ over the initialization of $\mathbf{w}_{j}^0$. 
% Conditioned on $\mathbf{w}_{j}^0\in \mathcal{G}_{\mathbf{w}}$ for all $j\in [m]$, we have $\|\mathbf{W}^0\|_2 \leq c\nu_{\mathbf{w}}(\sqrt{d}+\sqrt{m})$. % and $\|\mathbf{b}^0\|_2 \leq c\sigma_b\sqrt{m}$. Conditioned on  this event,
% Thus, we have
% \begin{align}
%     &\mathbb{P}_{\mathbf{x}} \big[ \eta f_{i}(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\big] \nonumber \\
%     &\leq \mathbb{P}_{\mathbf{x}} \left[ \|\mathbb{E}_{\mathbf{x}''} [ \sigma(\mathbf{W}^0\mathbf{x}'') ]\|_2 \|\sigma(\mathbf{W}^0\mathbf{x})\|_2 > \frac{1}{\eta}\right] \nonumber \\
%     &\leq \mathbb{P}_{\mathbf{x}} \left[ \mathbb{E}_{\mathbf{x}''} [\| \sigma(\mathbf{W}^0\mathbf{x}'') \|_2] \|\sigma(\mathbf{W}^0\mathbf{x})\|_2 > \frac{1}{\eta}\right] \nonumber \\
%     &\leq \mathbb{P}_{\mathbf{x}} \left[ c \|\mathbf{W}^0\|_2^2\mathbb{E}_{\mathbf{x}''} [\|\mathbf{x}'' \|_2] \|\mathbf{x}\|_2 > \frac{1}{\eta}\right] \nonumber \\
%     &\leq \mathbb{P}_{\mathbf{x}} \left[ \|\mathbf{x}\|_2  > \frac{1}{c\eta\|\mathbf{W}^0\|_2^2 \sqrt{d}} \right] \nonumber \\
%     &\leq \mathbb{P}_{\mathbf{x}} \left[ \|\mathbf{x}\|_2  > \frac{1}{c'\eta\nu_{\mathbf{w}}^2(d+m)\sqrt{d}} \right] \nonumber \\
%     &\leq \mathbb{P}_{\mathbf{x}} \left[ \|\mathbf{x}\|_2  > \frac{d}{c''\eta} \right]  \nonumber \\
%     &\leq \exp\left(-c'''d^2 \right) \label{38}
%     % &\leq \mathbb{P}_{\mathbf{x}} \left[ \|\mathbf{x}\|_2  > \frac{c}{\eta(d+m)\sqrt{d}\nu_{\mathbf{w}}^2 + \eta (\sqrt{d}+\sqrt{m})\sqrt{m} \nu_{\mathbf{w}}\sigma_b } \right] \nonumber \\
%     % &\leq \mathbb{P}_{\mathbf{x}} \left[ \|\mathbf{x}\|_2  > \frac{c}{\eta(d+m)^{1.5}\nu_{\mathbf{w}}^2 } \right] \nonumber \\
%     % &\leq  \mathbb{P}_{\mathbf{x}} \left[ \|\mathbf{x}\|_2  > c' d \right] \nonumber \\
%     % &\leq  \exp\left( - \frac{d^2}{8}\right)
% \end{align}
% using $\nu_{\mathbf{w}} = O(d^{-1.25})$, $m=O(d)$ and $\eta = \Theta(1)$. Combining \eqref{38} with \eqref{56} and \eqref{shm} completes the proof.


% \begin{align}  
% % &  \frac{1}{\lambda_{1}  } \mathbb{E}_{\mathbf{x},\mathbf{x}',i} \left[  f_{i}(\mathbf{x}) f_{i}(\mathbf{x}') \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz})\right] \nonumber \\
% \mathcal{L}(\mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{1,i} \}_{i\in \mathcal{T}})&=  \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \}  \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz}) \Big] \nonumber \\
% &\quad +   \nonumber \\
% &= 
% % \chi\{\sign(\bar{\mathbf{x}}_{i,j'}) \neq  \sign(\mathbf{x}_{i,j}) \}y_{i,j} \bar{y}_{i,j'}\bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz})  \Big] \nonumber
% % \sum_{i=1}^T \frac{1}{n_1n_2}\sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}) 
% \end{align} 
% where $\bar{\sigma}()$ denotes the stop-gradient applied to the ReLU. 
% \begin{align}  
% &  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{i,\mathbf{x}_{i,j},\bar{\mathbf{x}}_{i,j'}}\left[ y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})\right] \nonumber \\
% &=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{i,\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[ y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
% &=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}}  \left[\mathbb{E}_i \left[ y_{i,j}(\bar{\mathbf{x}}_{j'})  \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'}) \right] \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
% &=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}}  \left[\mathbb{E}_i \left[ 1 - 2\chi\{  y_{i,j}({\mathbf{x}}_{j}) \neq \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'})\} \right] \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
% &=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[ \left( 1 - 2\mathbb{P}_i \left[ y_{i,j}({\mathbf{x}}_{j}) \neq \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'}) \right]\right) \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
% &=  -\frac{2^{-r}}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[  \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j}) | \sign(\bar{\mathbf{x}}_{i,j',:r})=\sign({\mathbf{x}}_{i,j,:r})   \right] \nonumber \\
% &\quad + \frac{2^{r} - 1}{2^{r}\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[ \left( 1 - 2\mathbb{P}_i \left[ y_{i,j}({\mathbf{x}}_{j}) \neq \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'}) \right]\right) \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j}) | \sign(\bar{\mathbf{x}}_{i,j',:r})\neq \sign({\mathbf{x}}_{i,j,:r})   \right] \nonumber \\
% &= -\frac{2^{-r}}{\lambda_{1}} \mathbb{E}_{\mathbf{x},\bar{\mathbf{x}}} \left[  \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}})^\top \sigma(\mathbf{W}\mathbf{x}) | \sign(\bar{\mathbf{Mx}})=\sign({\mathbf{Mx}})   \right] \nonumber \\
% &\quad + \frac{2^{r} - 1}{2^{r}\lambda_{1} n_{1}n_{2} } \mathbb{E}_{\mathbf{x},\bar{\mathbf{x}}} \left[ \left( 1 - 2\mathbb{P}_i \left[ y_{i}({\mathbf{x}}) \neq \bar{y}_{i}(\bar{\mathbf{x}}) \right]\right) \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}})^\top \sigma(\mathbf{W}\mathbf{x}) | \sign(\bar{\mathbf{Mx}})\neq \sign({\mathbf{Mx}})   \right] \nonumber 
% \end{align} 

% \begin{align}
%     & \frac{2^{-r}}{\lambda_{1} n_{1}n_{2} }  \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1}  \mathbb{E}_{\bar{\mathbf{x}}_{i,j'},{\mathbf{x}}_{i,j}}\left[ \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}) | \sign(\bar{\mathbf{x}}_{i,j',:r})=\sign({\mathbf{x}}_{i,j,:r})  \right] \nonumber \\
% &\quad +  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \int_{\mathbf{x}_{i,j},\bar{\mathbf{x}}_{i,j'}} \int_{i} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})  p(\mathbf{x}_{i,j},\bar{\mathbf{x}}_{i,j'}) 
% \end{align}

%ideas: 

% is infinite tasks the same as sampling a random pair of gaussians, then sampling the number of tasks for which they have the same label? yes but does not equal zero... yes because opposite pairs?


% Differentiating with respect to the neuron weight $\mathbf{w}$ leads to the following 
% \begin{align}
%    & \nabla_{\mathbf{w}_j}  \mathbb{E}_{\mathbf{x},\bar{\mathbf{x}}} \left[  \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz}) | \sign({\mathbf{Mx}}')=\sign({\mathbf{Mx}})   \right]\nonumber \\
%    &=  \nabla_{\mathbf{w}_j}  \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[  \bar{\sigma}(\mathbf{w}_j^\top\mathbf{M}{\mathbf{x}}') \sigma(\mathbf{w}_j^\top \mathbf{x}) | \sign({\mathbf{Mx}}')=\sign({\mathbf{Mx}})   \right]  \nonumber \\
%     &=\mathbb{E}_{\mathbf{x},{\mathbf{x}}'} \left[  \mathbf{x} {\sigma}(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}) | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})   \right]  \nonumber \\
%     &= \mathbf{M}\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[  \mathbf{x}(\mathbf{x}')^\top {\sigma}'(\mathbf{w}_j^\top  \mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}) | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})   \right] \mathbf{w}_j  \nonumber \\
%     % \mathbf{A} =  \begin{bmatrix}
%     %     \mathbf{A}_{.}
%     % \end{bmatrix}
% \end{align}
% Now, for ease of notation we drop the subscript $j$.
% Analyzing the matrix $\mathbf{A}(\mathbf{w}) \coloneqq \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[  \mathbf{x}(\mathbf{x}')^\top  {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x}) | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})   \right]$ is the key to the proof.
% We have 
% \begin{align}
%     \mathbf{A}(\mathbf{w}) = \begin{bmatrix}
% \mathbf{A}_{\parallel,\parallel}(\mathbf{w}) & \mathbf{A}_{\parallel,\perp}(\mathbf{w}) \\
% \mathbf{A}_{\perp,\parallel}(\mathbf{w}) & \mathbf{A}_{\perp,\perp}(\mathbf{w}) \\
%     \end{bmatrix}
% \end{align}
% where 
% \begin{align}
%     \mathbf{A}_{\parallel,\parallel}(\mathbf{w}) &= \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[  \mathbf{x}_{:r}(\mathbf{x}')^\top \mathbf{M}^\top {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x}) | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})   \right] \nonumber \\
%     &= \mathbb{E}_{\mathbf{x}_{:r},\mathbf{x}_{:r}'} \left[  \mathbf{x}_{:r}(\mathbf{x}')^\top \mathbf{M}^\top 
%  \mathbb{E}_{\mathbf{M}_\perp \mathbf{x},\bar{\mathbf{M}_\perp \mathbf{x}}} \left[{\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x})\right] | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})   \right] \nonumber \\
% \end{align}






Next we control the matrices  $\mathbf{A}_{||,||}(\w)$, $\mathbf{A}_{||,\perp}(\w)$, $\mathbf{A}_{\perp,||}(\w)$, and $\mathbf{A}_{\perp,\perp}(\w)$. 

\begin{lemma}\label{lem:apara}
    % For all $j: \mathbf{w}_{j}^0\in \mathcal{G}_{\mathbf{w}}$, we have 
    For any $\delta \in (0,1)$ such that $\delta = \Omega(me^{-d})$, then if $ \mathbf{w}\in \mathcal{G}_{\mathbf{w}}(\delta)$, we have 
    \begin{align}
       \left\|\mathbf{A}_{\parallel,\parallel}(\mathbf{w}) - \frac{1}{2\pi} \mathbf{I}_r\right\|_2 &=  O\left( \frac{ r^{3} + \log^3(m/\delta) }{d }\right).
    \end{align}
\end{lemma}

\begin{proof}
% We drop the neuron index subscript and time index superscript on $\mathbf{w}_{j}^0$ for ease of notation. 
Recall that $\mathbf{u}$ is drawn uniformly from $\mathcal{H}^r$.
From Lemma \ref{lem:compute_grad}, we have
\begin{align}
    &\mathbf{A}_{\parallel,\parallel}(\mathbf{w}) \nonumber \\
    &= \mathbb{E}_{\mathbf{u}} \left[ \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[   {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x})  \mathbf{M}\mathbf{x}(\mathbf{Mx}')^\top |\sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})=\mathbf{u}\right] \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{u}} \left[
 \mathbb{E}_{\mathbf{M}\mathbf{x},{\mathbf{M}\mathbf{x}'}} \left[\mathbb{E}_{\mathbf{M}_\perp \mathbf{x},{\mathbf{M}_\perp \mathbf{x}'}} \left[{\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x})\right] \mathbf{M}\mathbf{x}(\mathbf{M}\mathbf{x}')^\top   | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}}) =\mathbf{u}\right] \right]  \nonumber \\
 &=  \mathbb{E}_{\mathbf{u}} \Big[ \mathbb{E}_{\mathbf{M}\mathbf{x},{\mathbf{M}\mathbf{x}'}} \Big[  \mathbf{M}\mathbf{x}(\mathbf{x}')^\top\mathbf{M}^\top \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}} \left[\mathbf{w}^\top \mathbf{M}_\perp^\top  \mathbf{M}_\perp \mathbf{x} > -\mathbf{w}^\top\mathbf{M}^\top \mathbf{Mx}  \right]   \nonumber \\
 &\quad \quad \quad \quad \quad  \times 
 \mathbb{P}_{{\mathbf{M}_\perp \mathbf{x}}'} \left[ \mathbf{w}^\top \mathbf{M}_\perp^\top  \mathbf{M}_\perp \mathbf{x}' > -\mathbf{w}^\top\mathbf{M}^\top \mathbf{Mx}'  \right] |\sign(\mathbf{Mx}')=\sign({\mathbf{Mx}}) =\mathbf{u}  \Big]\Big]  \nonumber \\
 &= \mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},{\mathbf{M}\mathbf{x}'}} \Bigg[  \mathbf{M}\mathbf{x}(\mathbf{x}')^\top \mathbf{M}^\top \left(\frac{1}{2} + \frac{1}{2}\erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top  {\mathbf{Mx}} }{ \sqrt{2}\| {\mathbf{M}_\perp \mathbf{w}} \|_2 } \right) \right) \nonumber \\
&\quad \quad \quad \quad \quad    \left(\frac{1}{2} + \frac{1}{2}\erf\left(\frac{\mathbf{w}^\top  \mathbf{Mx}' }{\sqrt{2} \| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) \right) |\sign(\mathbf{Mx}')=\sign({\mathbf{Mx}}) =\mathbf{u}  \Bigg] \label{gu} \\
 &= \frac{1}{4}\mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},{\mathbf{M}\mathbf{x}'}} \left[   \mathbf{M}\mathbf{x}(\mathbf{x}')^\top \mathbf{M}^\top  |\sign(\mathbf{Mx}')=\sign({\mathbf{Mx}}) =\mathbf{u} \right] \nonumber \\
 &\quad + \frac{1}{2}\mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},\mathbf{M}\mathbf{x}'} \left[  \mathbf{M}\mathbf{x}(\mathbf{x}')^\top \mathbf{M}^\top 
\erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top{\mathbf{Mx}} }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) |\sign(\mathbf{Mx}')=\sign({\mathbf{Mx}}) =\mathbf{u} \right]  \nonumber \\
 &\quad + \frac{1}{4}\mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},{\mathbf{M}\mathbf{x}'}} \left[   \mathbf{M}\mathbf{x}(\mathbf{x}')^\top \mathbf{M}^\top 
 \erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top{\mathbf{Mx}} }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) \erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top\mathbf{Mx}' }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) |\sign(\mathbf{Mx}')=\sign({\mathbf{Mx}}) =\mathbf{u}  \right]  \label{apara3}
\end{align}
where \eqref{gu} follows using the Gaussian CDF.
For the first term in \eqref{apara3}, we can re-write $\mathbf{M}\mathbf{x}$ conditioned on $\sign({\mathbf{Mx}}) =\mathbf{u}$ as $\diag(\mathbf{u}) |\mathbf{M}\mathbf{x}|$, where $|\cdot|$ denotes element-wise absolute value, to obtain
\begin{align}
     % &\frac{1}{4}\mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},{\mathbf{M}\mathbf{x}'}} \left[ \chi\{ \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}}) =\mathbf{u}\}  \mathbf{M}\mathbf{x}(\mathbf{x}')^\top \mathbf{M}^\top \right] \nonumber \\
     &\frac{1}{4}\mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},{\mathbf{M}\mathbf{x}'}} \left[  \mathbf{M}\mathbf{x}(\mathbf{x}')^\top \mathbf{M}^\top | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}}) =\mathbf{u} \right]   \nonumber \\
     &=  \frac{1}{4}\mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},{\mathbf{M}\mathbf{x}'}} \left[  \diag(\mathbf{u})|\mathbf{M}\mathbf{x}||\mathbf{Mx}'|^\top \diag(\mathbf{u}) \right]  \nonumber \\
     &=   \frac{1}{4}\mathbb{E}_{\mathbf{u}} \left[  \diag(\mathbf{u})\mathbb{E}_{\mathbf{M}\mathbf{x}} \left[  |\mathbf{M}\mathbf{x}|\right] \mathbb{E}_{{\mathbf{M}\mathbf{x}'}} \left[|\mathbf{Mx}'|\right]^\top \diag(\mathbf{u}) \right]    \nonumber \\
      &=  \frac{1}{2\pi}\mathbb{E}_{\mathbf{u}} \left[  \diag(\mathbf{u})\mathbf{1}_r\mathbf{1}_{r}^\top \diag(\mathbf{u}) \right]       \label{halkn} \\
      &=  \frac{1}{2\pi}\mathbb{E}_{\mathbf{u}} \left[  \mathbf{u}\mathbf{u}^\top \right]       \nonumber \\
     % &=  \frac{1}{4}\mathbb{E}_{\mathbf{u}} \left[  \diag(\mathbf{u})\left( \frac{2}{\pi} \mathbf{1}_r\mathbf{1}_{r}^\top + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_r  \right)\diag(\mathbf{u}) \right]       \nonumber \\
     % &=  \frac{1}{4}\left( \frac{2}{\pi} \mathbb{E}_{\mathbf{u}} \left[  \mathbf{u}\mathbf{u}^\top  \right] + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_r \right)       \nonumber \\
     &= \frac{1}{2\pi} \mathbf{I}_r      \label{dfc} 
\end{align}
% (diagonal element is average of product of aligned half-normals, off diagonals are averaged of non-aligned)
where \eqref{halkn} follows since each element of $|\mathbf{M}\mathbf{x}|$ and $|\mathbf{M}\mathbf{x}'|$ is a standard half-normal random variable.
For the second term in \eqref{apara3}, we have
\begin{align}
     &\frac{1}{2}\mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},\mathbf{M}\mathbf{x}'} \left[  \mathbf{M}\mathbf{x}(\mathbf{x}')^\top \mathbf{M}^\top 
\erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top{\mathbf{Mx}} }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})=\mathbf{u}   \right] \nonumber \\
&= \frac{1}{2}\mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},\mathbf{M}\mathbf{x}'} \left[  \diag(\mathbf{u})|\mathbf{M}\mathbf{x}||\mathbf{Mx}'|^\top \diag(\mathbf{u}) 
\erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top \diag(\mathbf{u})|{\mathbf{Mx}}| }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right)   \right]\label{jn} \\
&= \frac{1}{2}\mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},\mathbf{M}\mathbf{x}'} \left[  \diag(-\mathbf{u})|\mathbf{M}\mathbf{x}||\mathbf{Mx}'|^\top \diag(-\mathbf{u}) 
\erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top \diag(-\mathbf{u})|{\mathbf{Mx}}| }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right)   \right] \label{jj}\\
&= -\frac{1}{2}\mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},\mathbf{M}\mathbf{x}'} \left[  \diag(\mathbf{u})|\mathbf{M}\mathbf{x}||\mathbf{Mx}'|^\top \diag(\mathbf{u}) 
\erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top \diag(\mathbf{u})|{\mathbf{Mx}}| }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right)   \right] \label{nnj} \\
% &= \frac{1}{\sqrt{\pi}} \Bigg( \frac{1}{ \sqrt{2} \| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \mathbb{E}_{\mathbf{M}\mathbf{x},\mathbf{Mx}'}\left[  \mathbf{M}\mathbf{x}\mathbf{x}^\top\mathbf{M}^\top \mathbf{Mw} (\mathbf{x}')^\top \mathbf{M}^\top  | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})   \right]  \nonumber \\
% &\quad + \frac{1}{ 2 \sqrt{2} \| {\mathbf{M}_{\perp}\mathbf{w}} \|_2^3 } \mathbb{E}_{\mathbf{x}_{:r},\mathbf{x}_{:r}'} \left[  (\mathbf{x}^\top\mathbf{M}^\top \mathbf{Mw})^3\mathbf{x}_{:r} (\mathbf{x}')^\top \mathbf{M}^\top  | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})   \right]  + \dots \Bigg) \nonumber \\
% &=\frac{1}{{\pi}} \Bigg( \frac{1}{  \| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \mathbb{E}_{\mathbf{v},\mathbf{x}_{:r}} \left[  \mathbf{x}_{:r}\mathbf{x}^\top\mathbf{M}^\top \mathbf{Mw} {\mathbf{v}}^\top  | \sign({\mathbf{Mx}}) =\mathbf{v}   \right]  \nonumber \\
% &\quad + \frac{1}{ 2  \| {\mathbf{M}_{\perp}\mathbf{w}} \|_2^3 } \mathbb{E}_{\mathbf{v},\mathbf{x}_{:r}} \left[  (\mathbf{x}^\top\mathbf{M}^\top \mathbf{Mw})^3\mathbf{x}_{:r}  {\mathbf{v}}^\top  | \sign({\mathbf{Mx}}) =\mathbf{v}   \right]  + \dots \Bigg) \nonumber \\
&= \mathbf{0} \label{lst}
\end{align}
where \eqref{jj} follows from the fact that $\mathbf{u}$ and $-\mathbf{u}$ have the same distribution, \eqref{nnj} follows since $\erf()$ is an odd function, and \eqref{lst} follows since $x=-x\iff x=0$.
% since each term always has an odd number of v/s (write z as abs(z)v

The final term in \eqref{apara3} is 
\begin{align}
&\mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},\mathbf{M}\mathbf{x}'} \left[  \mathbf{M}\mathbf{x}(\mathbf{x}')^\top \mathbf{M}^\top 
 \erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top{\mathbf{Mx}} }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) \erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top\mathbf{Mx}' }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right)| \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})  =\mathbf{u} \right]  \nonumber \\
 % &= \mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}_{:r}'} \left[  \mathbf{x}_{:r}(\mathbf{x}')^\top \mathbf{M}^\top 
 % \erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top{\mathbf{Mx}} }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) \erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top\mathbf{Mx}' }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right)| \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})  =\mathbf{u} \right]  \nonumber \\
 &= \mathbb{E}_{\mathbf{u}}
 % \sim \Unif(\mathcal{H}^{r})} 
 \Bigg[\mathbb{E}_{\mathbf{M}\mathbf{x}} \left[  \mathbf{M}\mathbf{x} 
 \erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top{\mathbf{Mx}} }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) \bigg| \sign({\mathbf{Mx}})=\mathbf{u}\right] \nonumber \\
 &\quad \quad \times \mathbb{E}_{\mathbf{Mx}'}\left[(\mathbf{x}')^\top \mathbf{M}^\top\erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top\mathbf{Mx}' }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right)\bigg| \sign(\mathbf{Mx}')=\mathbf{u}\right] \Bigg] \label{46}
\end{align}
% where $\mathcal{H}^{r} = \{-1,1\}^r$ is the $r$-dimensional Rademacher hypercube. 
Again to remove the conditioning, we can equivalently write $\mathbb{E}_{\mathbf{M}\mathbf{x}} \left[  \mathbf{M}\mathbf{x} 
 \erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top{\mathbf{Mx}} }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) \bigg| \sign({\mathbf{Mx}})=\mathbf{u}\right]$ as 
 \begin{align}
     \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[  \mathbf{M}\mathbf{x} 
 \erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top{\mathbf{Mx}} }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) \bigg| \sign({\mathbf{Mx}})=\mathbf{u}\right] 
 &= \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[ \text{diag}(\mathbf{u}) |\mathbf{M}\mathbf{x} |
 \erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top  \text{diag}(\mathbf{u}) | {\mathbf{Mx}}| }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) \right] 
 \end{align}
% where $| {\mathbf{Mx}}| \in \mathbb{R}^r$ denotes the element-wise absolute value of $\mathbf{M}\mathbf{x}$. 
For all $\mathbf{u}\in \mathcal{H}^r$, we have 
\begin{align}
   & \left\|\mathbb{E}_{\mathbf{M}\mathbf{x}} \left[ \text{diag}(\mathbf{u}) |\mathbf{M}\mathbf{x} |
 \erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top  \text{diag}(\mathbf{u}) | {\mathbf{Mx}}| }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) \right] \right\|_2 \nonumber \\
    &\leq  \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[\left\| \text{diag}(\mathbf{u}) |\mathbf{M}\mathbf{x} |
 \erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top  \text{diag}(\mathbf{u}) | {\mathbf{Mx}}| }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) \right\|_2 \right]  \nonumber \\
 &\leq \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[\left\| \text{diag}(\mathbf{u}) |\mathbf{M}\mathbf{x} |\right\|_2
\left|\erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top  \text{diag}(\mathbf{u}) | {\mathbf{Mx}}| }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) \right|\right]  \nonumber \\
 &\leq \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[\left\| \text{diag}(\mathbf{u}) |\mathbf{M}\mathbf{x} |\right\|_2
\left|\frac{\mathbf{w}^\top \mathbf{M}^\top  \text{diag}(\mathbf{u}) | {\mathbf{Mx}}| }{ \| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right|\right]  \label{jhj} \\
 &\leq \left\|\text{diag}(\mathbf{u})\right\|_2  \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[ \|\mathbf{M}\mathbf{x}\|_2^2\right]
\frac{\|\mathbf{w}^\top \mathbf{M}^\top  \text{diag}(\mathbf{u}) \|_2 }{ \| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 }  \nonumber \\
% &\leq  \nonumber \\
 &\leq \frac{c r (\sqrt{r} +\sqrt{\log(m/\delta)}) }{\sqrt{d} } \label{wb}
\end{align}
for an absolute constant $c$, where \eqref{jhj} follows since $|\erf(x)|\leq \sqrt{2}|x| $, and \eqref{wb} follows
since $\mathbf{w}\in \mathcal{G}_{\mathbf{w}}(\delta)$ 
and $m/\delta = O(e^d)$, thus $\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 = \Omega(\sqrt{d})$.
Therefore, using \eqref{46},
\begin{align}
    &\left\|\mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},\mathbf{M}\mathbf{x}'} \left[  \mathbf{M}\mathbf{x}(\mathbf{x}')^\top \mathbf{M}^\top 
 \erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top{\mathbf{Mx}} }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) \erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top\mathbf{Mx}' }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right)| \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})  =\mathbf{u} \right]  \right\|_2 \nonumber \\
 &\leq \frac{c' r^{3} + c'\log^3(m/\delta) }{d }
\end{align}
completing the proof.
\end{proof}
\begin{comment}
Next we use the Taylor series of $\text{erf}(\cdot)$ around zero to write
\begin{align}
    &\mathbb{E}_{\mathbf{M}\mathbf{x}} \left[ \text{diag}(\mathbf{u}) |\mathbf{M}\mathbf{x} |
 \erf\left(\frac{\mathbf{w}^\top \mathbf{M}^\top  \text{diag}(\mathbf{u}) | {\mathbf{Mx}}| }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \right) \right] \nonumber \\
 &= \frac{2}{\sqrt{\pi}} \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[ \text{diag}(\mathbf{u}) |\mathbf{M}\mathbf{x} |
 \left(\frac{\mathbf{w}^\top \mathbf{M}^\top  \text{diag}(\mathbf{u}) | {\mathbf{Mx}}| }{ \sqrt{2}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 }  - \frac{(\mathbf{w}^\top \mathbf{M}^\top  \text{diag}(\mathbf{u}) | {\mathbf{Mx}}|)^3 }{ 6\sqrt{2} \| {\mathbf{M}_{\perp}\mathbf{w}} \|_2^3 }  + \frac{(\mathbf{w}^\top \mathbf{M}^\top  \text{diag}(\mathbf{u}) | {\mathbf{Mx}}|)^5 }{ 40 \| {\mathbf{M}_{\perp}\mathbf{w}} \|_2^5 } +\dots \right) \right] \nonumber \\
 &=  \frac{\sqrt{2}}{\sqrt{\pi}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 }\text{diag}(\mathbf{u})  \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[ |\mathbf{M}\mathbf{x} |  | {\mathbf{Mx}}|^\top \right] \text{diag}(\mathbf{u}) \mathbf{Mw} + \mathbf{E}_1 
  % - \frac{1}{ 6 \| {\mathbf{M}_{\perp}\mathbf{w}} \|_2^3 } \mathbb{E}_{\mathbf{M}\mathbf{x}}\left[   \text{diag}(\mathbf{v}) | {\mathbf{Mx}}| (\mathbf{w}^\top \mathbf{M}^\top  \text{diag}(\mathbf{v}) | {\mathbf{Mx}}|)^3 \right]   +\dots \right) 
  \nonumber 
\end{align}
where $\|\mathbf{E}_1\|_2=O\left({(d-r)^{-1.5}}\right) $. This follows since $\mathbf{w}\in \mathcal{G}_{\mathbf{w}}$, thus $\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 = \Omega(\sqrt{d-r})$, and 
\begin{align}
\|    \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[ \text{diag}(\mathbf{u}) |\mathbf{M}\mathbf{x} |
 \left( - \frac{(\mathbf{w}^\top \mathbf{M}^\top  \text{diag}(\mathbf{u}) | {\mathbf{Mx}}|)^3 }{ 6\sqrt{2} \| {\mathbf{M}_{\perp}\mathbf{w}} \|_2^3 }  + \frac{(\mathbf{w}^\top \mathbf{M}^\top  \text{diag}(\mathbf{u}) | {\mathbf{Mx}}|)^5 }{ 40 \| {\mathbf{M}_{\perp}\mathbf{w}} \|_2^5 } +\dots \right) \right] \|_2 \nonumber \\
 &\leq c
\end{align}
for an absolute constant $c$. 
\end{comment}

% with probability at least $1-$ since $\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 = \Omega(\sqrt{d-r})$ with probability at least $1-$. 

% For the first term, we note that each element of $|\mathbf{M}\mathbf{x} | $ is an i.i.d. half-normal random variable, and thus obtain
% \begin{align}
%     &\frac{\sqrt{2}}{\sqrt{\pi}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 }\text{diag}(\mathbf{v})  \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[ |\mathbf{M}\mathbf{x} |  | {\mathbf{Mx}}|^\top \right] \text{diag}(\mathbf{v}) \mathbf{Mw}\nonumber \\
%     &= \frac{\sqrt{2}}{\sqrt{\pi}\| {\mathbf{M}_{\perp}\mathbf{w}} \|_2 } \left( \frac{2}{\pi} \mathbf{v}\mathbf{v}^\top + \left( 1  - \frac{2}{\pi}\right)\mathbf{I}_r \right)\mathbf{Mw}
% \end{align}






\begin{lemma} \label{lem:aperp}
    For any $\delta \in (0,1)$ such that $\delta = \Omega(me^{-d})$, then if $ \mathbf{w}\in \mathcal{G}_{\mathbf{w}}(\delta)$, we have 
    \begin{align}
        \left\|\mathbf{A}_{\perp,\perp}(\mathbf{w}) - \left(1 - \frac{\|\mathbf{Mw}\|_2^2}{\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right) \frac{\mathbf{M}_\perp \mathbf{w} \mathbf{w}^\top \mathbf{M}_\perp^\top }{2\pi \|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right\|_2 &\leq O\left(\frac{r^4 + \log^4(m/\delta)}{d^2}\right).
    \end{align}
    % for an absolute constant $c$.
\end{lemma}


\begin{proof}
% \begin{align}
%     \mathbf{W} &= \mathbf{W}
% \end{align}
% Next we analyze $\mathbf{A}_{\perp,\perp}(\mathbf{w}_{})$.
% Again we drop the subscript and superscript on $\mathbf{w}_j^0$ for ease of notation.
We have
\begin{align}
    \mathbf{A}_{\perp,\perp}(\mathbf{w}) &=  \mathbb{E}_{\mathbf{u}} \left[\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[  \mathbf{M}_\perp \mathbf{x}(\mathbf{M}_{\perp}\mathbf{x}')^\top {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x}) | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}}) =\mathbf{u}  \right]\right] \nonumber \\
    &= \mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},\mathbf{Mx}'} \left[ \mathbb{E}_{\mathbf{M}_\perp \mathbf{x},\mathbf{M}_{\perp}\mathbf{x}'} \left[ \mathbf{M}_\perp \mathbf{x}(\mathbf{M}_{\perp}\mathbf{x}')^\top {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x}) \right] | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})=\mathbf{u}  \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},\mathbf{Mx}'} \left[ \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} \sigma'(\mathbf{w}^\top \mathbf{x})  \right] \mathbb{E}_{\mathbf{M}_{\perp}\mathbf{x}'} \left[(\mathbf{M}_{\perp}\mathbf{x}')^\top {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \right] | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}}) =\mathbf{u} \right] \label{cb}  
   %  \\
   % &=  \mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},\mathbf{Mx}'} \left[ \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} \sigma'(\mathbf{w}^\top \mathbf{x})  \right] \mathbb{E}_{\mathbf{M}_{\perp}\mathbf{x}'} \left[(\mathbf{M}_{\perp}\mathbf{x}')^\top {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \right] | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}}) =\mathbf{u} \right] \nonumber
\end{align}
Using Lemma \ref{lem:exp-perp} to compute $\mathbb{E}_{\mathbf{M}_\perp \mathbf{x}} \left[ \mathbf{M}_\perp \mathbf{x} \sigma'(\mathbf{w}^\top \mathbf{x})  \right] $ and $\mathbb{E}_{\mathbf{M}_{\perp}\mathbf{x}'} \left[(\mathbf{M}_{\perp}\mathbf{x}')^\top {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \right]$  yields 
\begin{align}
   \mathbf{A}_{\perp,\perp}(\mathbf{w})   &=  \mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},\mathbf{Mx}'} \left[ \exp\left( -\frac{(\mathbf{x}^\top\mathbf{M}^\top \mathbf{Mw})^2+ ((\mathbf{x}')^\top \mathbf{M}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)    \bigg| \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}}) =\mathbf{u} \right] \nonumber \\
    &\quad \times \frac{1}{2\pi \|\mathbf{M}_\perp\mathbf{w}\|_2^2}\mathbf{M}_\perp \mathbf{w} \mathbf{w}^\top \mathbf{M}_\perp^\top   \label{where}
\end{align}
We analyze the scalar term in the top line. We have
\begin{align}
&\mathbb{E}_{\mathbf{u}} \left[\mathbb{E}_{\mathbf{M}\mathbf{x},\mathbf{Mx}'} \left[ \exp\left( -\frac{(\mathbf{x}^\top\mathbf{M}^\top \mathbf{Mw})^2+ ((\mathbf{x}')^\top \mathbf{M}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)    \bigg| \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}}) =\mathbf{u} \right]\right] \nonumber \\
    % &= %2^{-r} \sum_{\mathbf{v}\in \mathcal{H}^r} 
    % \mathbb{E}_{\mathbf{u}} \left[\mathbb{E}_{\mathbf{M}\mathbf{x},\mathbf{Mx}'} \left[ \exp\left( -\frac{(\mathbf{M}\mathbf{x}^\top\mathbf{Mw})^2+ ((\mathbf{x}')^\top \mathbf{M}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)    \bigg| \sign(\mathbf{Mx}')= \mathbf{u}, \sign({\mathbf{Mx}}) = \mathbf{u}  \right]\right] \nonumber \\
    &= %2^{-r} \sum_{\mathbf{v}\in \mathcal{H}^r} 
    \mathbb{E}_{\mathbf{u}}\Bigg[ \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[ \exp\left( -\frac{(\mathbf{x}^\top \mathbf{M}^\top \mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)    \bigg| \sign({\mathbf{Mx}}) = \mathbf{u}  \right] \nonumber \\
    &\quad \quad \quad \quad \times \mathbb{E}_{\mathbf{Mx}'} \left[ \exp\left( -\frac{((\mathbf{x}')^\top \mathbf{M}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)    \bigg| \sign(\mathbf{Mx}')= \mathbf{u} \right]\Bigg] \nonumber \\
    &= %2^{-r} \sum_{\mathbf{v}\in \mathcal{H}^r} 
    \mathbb{E}_{\mathbf{u}} \left[ \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[ \exp\left( -\frac{(\mathbf{x}^\top\mathbf{M}^\top \mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)    \bigg| \sign({\mathbf{Mx}}) = \mathbf{u}  \right]^2 \right] \label{f}
    % &\leq \left( 2^{-r} \sum_{\mathbf{v}\in \mathcal{H}^r} \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[ \exp\left( -\frac{(\mathbf{M}\mathbf{x}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)    \bigg| \sign({\mathbf{Mx}}) = \mathbf{v}  \right] \right)^2 \nonumber \\
    % &=  \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[ \exp\left( -\frac{(\mathbf{M}\mathbf{x}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)   \right] ^2 \nonumber \\
    % &= \frac{ \| \mathbf{M}_\perp \mathbf{w} \|_2^2  }{\| \mathbf{w} \|_2^2 }
\end{align}
where, using the Taylor expansion of $\exp({-x^2})$ and  re-writing $\mathbf{M}\mathbf{x}$ conditioned on $\{\sign({\mathbf{Mx}}) =\mathbf{u}\}$ as $\diag(\mathbf{u}) |\mathbf{M}\mathbf{x}|$,
\begin{align}
    &\mathbb{E}_{\mathbf{M}\mathbf{x}} \left[ \exp\left( -\frac{(\mathbf{x}^\top\mathbf{M}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)    \bigg| \sign({\mathbf{Mx}}) = \mathbf{u}  \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[ \exp\left( -\frac{(|\mathbf{M}\mathbf{x}|^\top \text{diag}(\mathbf{u}) \mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)    \right] \nonumber \\
    &= 1 - \frac{1}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[(|\mathbf{M}\mathbf{x}|^\top \diag(\mathbf{u}) \mathbf{Mw})^2\right]  + O\left( \frac{r^4 + \log^4(m/\delta)}{ d^2} \right) \label{fb}
    % + \frac{1}{\|\mathbf{M}_\perp \mathbf{w}\|_2^4} \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[(|\mathbf{M}\mathbf{x}|^\top \diag(\mathbf{v}) \mathbf{Mw})^4\right]  + O( (d-r)^{-3} ).
\end{align}
where \eqref{fb} follows since  $\|\mathbf{M}_\perp\mathbf{w}\|_2^2 = \Omega( (\sqrt{d} - \sqrt{\log(m/\delta)})^4) = \Omega(d^2)$ and $\mathbb{E}_{\mathbf{M}\mathbf{x}}[ (|\mathbf{M}\mathbf{x}|^\top \text{diag}(\mathbf{u}) \mathbf{Mw})^4 ]\leq \mathbb{E}_{\mathbf{M}\mathbf{x}}[ \|\mathbf{M}\mathbf{x}\|_2^4 ]\|\mathbf{Mw}\|_2^4 = O(r^4 + \log^4(m/\delta))$ since $\mathbf{w}\in \mathcal{G}_{\mathbf{w}}$. To compute the second term in \eqref{fb}, note that
\begin{align}
    \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[(|\mathbf{M}\mathbf{x}|^\top \text{diag}(\mathbf{u}) \mathbf{Mw})^2\right]  &=   \mathbf{w}^\top \mathbf{M}^\top \text{diag}(\mathbf{u})\mathbb{E}_{\mathbf{M}\mathbf{x}}  \left[|\mathbf{M}\mathbf{x}||\mathbf{M}\mathbf{x}|^\top \right]\text{diag}(\mathbf{u}) \mathbf{Mw} \nonumber \\
    &= \mathbf{w}^\top \mathbf{M}^\top \text{diag}(\mathbf{u})\left(\frac{2}{\pi}\mathbf{1}_{r}\mathbf{1}_{r}^\top + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_{r}\right)\text{diag}(\mathbf{u}) \mathbf{Mw} \nonumber \\               
    &=  \mathbf{w}^\top \mathbf{M}^\top \left(\frac{2}{\pi}\mathbf{uu}^\top + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_{r}\right)\mathbf{Mw} \nonumber 
\end{align}
therefore
\begin{align}
   &\mathbb{E}_{\mathbf{u}} \left[ \mathbb{E}_{\mathbf{M}\mathbf{x}} \left[ \exp\left( -\frac{(\mathbf{x}^\top\mathbf{M}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)    \bigg| \sign({\mathbf{Mx}}) = \mathbf{u}  \right]^2 \right] \nonumber \\
   &= \mathbb{E}_{\mathbf{u}} \left[\left( 1 -  \frac{1}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2}\mathbf{w}^\top \mathbf{M}^\top \left(\frac{2}{\pi}\mathbf{uu}^\top + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_{r}\right)\mathbf{Mw} + O\left( \frac{r^4 + \log^4(m/\delta)}{ d^{2}} \right) \right)^2 \right] \nonumber \\
   &= 1 -  \frac{1}{\|\mathbf{M}_\perp\mathbf{w}\|_2^2}\mathbf{w}^\top \mathbf{M}^\top \left(\frac{2}{\pi}\mathbb{E}_{\mathbf{u}}[\mathbf{uu}^\top] + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_{r}\right)\mathbf{Mw} \nonumber \\
   &\quad + \frac{1}{4\|\mathbf{M}_\perp \mathbf{w}\|_2^4}\mathbf{w}^\top \mathbf{M}^\top \mathbb{E}_{\mathbf{u}}\left[ \left(\frac{2}{\pi}\mathbf{uu}^\top + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_{r}\right)\mathbf{Mw}\mathbf{w}^\top \mathbf{M}^\top \left(\frac{2}{\pi}\mathbf{uu}^\top + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_{r}\right)\right] \mathbf{Mw} \nonumber \\
   &\quad +  O\left(\frac{r^4 + \log^4(m/\delta)}{ d^{2}} \right) \nonumber \\
   &=  1 -  \frac{\|\mathbf{Mw}\|_2^2}{\|\mathbf{M}_\perp\mathbf{w}\|_2^2} + \frac{\left((1- \frac{2}{\pi})^2 + \frac{4}{\pi}\left(1 - \frac{2}{\pi}\right) \right)\|\mathbf{M} \mathbf{w}\|_2^4     }{4\|\mathbf{M}_\perp \mathbf{w}\|_2^4} \nonumber \\
   &\quad  + \frac{4}{\pi^2}
   \mathbf{w}^\top \mathbf{M}^\top \mathbb{E}_{\mathbf{u}}\left[ \mathbf{uu}^\top \mathbf{Mw} \mathbf{w}^\top \mathbf{M}^\top  \mathbf{uu}^\top \right] \mathbf{Mw}  +  O\left(\frac{r^4 + \log^4(m/\delta)}{ d^{2}}  \right) \nonumber \\
   &=  1 -  \frac{\|\mathbf{Mw}\|_2^2}{\|\mathbf{M}_\perp\mathbf{w}\|_2^2} + \frac{\left((1- \frac{2}{\pi})^2 + \frac{4}{\pi}\left(1 - \frac{2}{\pi}\right) \right)\|\mathbf{M} \mathbf{w}\|_2^4     }{4\|\mathbf{M}_\perp \mathbf{w}\|_2^4}  \nonumber \\
   &\quad + \frac{1}{\pi^2 \|\mathbf{M}_\perp \mathbf{w}\|_2^4 } 
   \mathbf{w}^\top \mathbf{M}^\top \mathbb{E}_{\mathbf{u}}\left[ \mathbf{uu}^\top (\mathbf{u}^\top\mathbf{Mw})^2 \right] \mathbf{Mw}  +  O\left(\frac{r^4 + \log^4(m/\delta)}{ d^{2} } \right) \nonumber \\
   &=  1 -  \frac{\|\mathbf{Mw}\|_2^2}{\|\mathbf{M}_\perp\mathbf{w}\|_2^2} + \frac{\left((1- \frac{2}{\pi})^2 + \frac{4}{\pi}\left(1 - \frac{2}{\pi}\right) \right)\|\mathbf{M} \mathbf{w}\|_2^4     }{4\|\mathbf{M}_\perp \mathbf{w}\|_2^4}  \nonumber \\
   &\quad + \frac{1}{\pi^2 \|\mathbf{M}_\perp \mathbf{w}\|_2^4 } 
   \mathbf{w}^\top \mathbf{M}^\top \left( \|\mathbf{Mw}\|_2^2\mathbf{I}_r + 2 \mathbf{Mw}\mathbf{w}^\top \mathbf{M}^\top - \diag( \mathbf{Mw} )^2 \right) \mathbf{Mw}  +  O\left(\frac{r^4 + \log^4(m/\delta)}{ d^{2}} \right) \nonumber \\
   &= 1 -  \frac{\|\mathbf{Mw}\|_2^2}{\|\mathbf{M}_\perp\mathbf{w}\|_2^2} + \frac{\left((1- \frac{2}{\pi})^2 + \frac{4}{\pi}\left(1 - \frac{2}{\pi}\right) \right)\|\mathbf{M} \mathbf{w}\|_2^4     }{4\|\mathbf{M}_\perp \mathbf{w}\|_2^4} + \frac{3\|\mathbf{Mw}\|_2^4 - \|\mathbf{Mw}\|_4^4 }{\pi^2 \|\mathbf{M}_\perp \mathbf{w}\|_2^4 }  +  O\left(\frac{r^4 + \log^4(m/\delta)}{ d^{2}} \right) \nonumber \\
   &= 1 - \frac{\|\mathbf{Mw}\|_2^2}{\|\mathbf{M}_\perp\mathbf{w}\|_2^2} + O\left(\frac{r^4 + \log^4(m/\delta)}{ d^{2}} \right), \nonumber 
\end{align}
where we have used $\w\in \mathcal{G}_{\mathbf{w}}(\delta)$ and $m/\delta = O(e^d)$. Combining this with \eqref{where} and \eqref{f} completes the proof.
% error after 1 step for this term will be (with $\lambda $ set pessimistically) $ \eta\frac{2}{\pi} ( 1  - \frac{\|\mathbf{M}_{r:}^\top \w\|_2^2}{\|\w\|_2^2} ) {\mathbf{M}_{r:}^\top \w} $ which has norm $\approx \frac{r}{k} \sqrt{d-r} $ (if $r$ is approximately $k$, then this is again zero).
% which isn't tight enough, but we can approximate to arbitrary order to get arbitrarily tight bound
% easy to get up to 1/k2 error in approximating this constant
% which means the matrix will have spectral norm 1/k 
% prod with w has norm 1/rt(k)
% prod with new x will have norm O(1times rt(r 2r log(k))) which is still too large, needs to be o(1)
% is there a way to get rid of 2r union bound?
% is it ok if only a subset of the neurons are good?
% with subset (hoeffding) argument, we get rid of union bound, and good part and bad part have the same norm up to constants
% with tight analysis of error variance we can make the bad constat very small.
% but is this good enough?
% it is good enough for there to exist a good network?
% yes, with bias.
% can add very small bias before first step and I think the proof should work. basically you're just fixing a u0 coordinate. think of b as part of w.
% make learning rate for b very small
% then we should be able to say that the loss after one step is small for some choice of a...
\end{proof}






\begin{lemma}\label{lem:aparaperp}
    % For all $j: \mathbf{w}_{j}^0\in \mathcal{G}_{\mathbf{w}}$, we have 
   For any $\delta \in (0,1)$ such that $\delta = \Omega(me^{-d})$, then if $ \mathbf{w}\in \mathcal{G}_{\mathbf{w}}(\delta)$, we have 
    \begin{align}
        \left\|\mathbf{A}_{\parallel,\perp}(\mathbf{w}) - \frac{ \mathbf{Mw}\mathbf{w}^\top \mathbf{M}_\perp^\top }{2{\pi}\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right\|_2 &\leq O\left(\frac{r^{3.5} + \log^{3.5}(m/\delta)}{d^{1.5}}\right)
    \end{align}
\end{lemma}



\begin{proof}
Arguing similarly to the previous two lemmas, we obtain
\begin{align}
    \mathbf{A}_{\parallel,\perp}(\mathbf{w}) &= \mathbb{E}_{\mathbf{u},\mathbf{x},\mathbf{x}'} \left[  \mathbf{M}\mathbf{x}(\mathbf{M}_{\perp}\mathbf{x}')^\top {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x}) | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}}) =\mathbf{u}  \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{u},\mathbf{x},\mathbf{Mx}'} \left[  \mathbf{M}\mathbf{x} \sigma'(\mathbf{w}^\top \mathbf{x}) \E_{\mathbf{M}_{\perp}\mathbf{x}'} \left[(\mathbf{M}_{\perp}\mathbf{x}')^\top {\sigma}'(\mathbf{w}^\top  \mathbf{x}')\right] | \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}}) = \mathbf{u}  \right] \nonumber \\
    &=  \mathbb{E}_{\mathbf{u},\mathbf{x},\mathbf{Mx}'} \left[  \mathbf{M}\mathbf{x} \sigma'(\mathbf{w}^\top \mathbf{x}) \exp\left( - \frac{((\mathbf{x}')^\top \mathbf{M}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)| \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})=\mathbf{u}   \right] \nonumber \\
    &\quad \times  \frac{ \mathbf{w}^\top \mathbf{M}_{\perp}^\top }{\sqrt{2 \pi}\|\mathbf{M}_\perp \mathbf{w}\|_2}  \label{nm} %\\
\end{align}
where \eqref{nm} follows by Lemma \ref{lem:exp-perp}.
Next, since the only term that depends on $\mathbf{M}_\perp \mathbf{x}$ is $\sigma'(\mathbf{w}^\top \mathbf{x})$, we have
\begin{align}
\nonumber \\
 &=  \mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},\mathbf{Mx}'} \left[  \mathbf{M}\mathbf{x} \mathbb{E}_{\mathbf{M}_\perp \mathbf{x}}[\sigma'(\mathbf{w}^\top \mathbf{x})] \exp\left( - \frac{((\mathbf{x}')^\top \mathbf{M}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)| \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})=\mathbf{u}   \right] \nonumber \\
    &\quad \times  \frac{ \mathbf{w}^\top \mathbf{M}_{\perp}^\top }{\sqrt{2 \pi}\|\mathbf{M}_\perp \mathbf{w}\|_2}  \nonumber \\
     &=  \mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},\mathbf{Mx}'} \left[  \mathbf{M}\mathbf{x} \mathbb{P}_{\mathbf{M}_\perp \mathbf{x}}[\mathbf{w}^\top \mathbf{M}_\perp^\top \mathbf{M}_\perp \mathbf{x} > - \mathbf{w}^\top \mathbf{M}^\top \mathbf{M}\mathbf{x} ] \exp\left( - \frac{((\mathbf{x}')^\top \mathbf{M}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)| \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})=\mathbf{u}   \right] \nonumber \\
    &\quad \times  \frac{ \mathbf{w}^\top \mathbf{M}_\perp^\top }{\sqrt{2 \pi}\|\mathbf{M}_\perp \mathbf{w}\|_2}  \nonumber \\
    &=  \mathbb{E}_{\mathbf{u},\mathbf{Mx},\mathbf{Mx}'} \left[  \mathbf{M}\mathbf{x} \left(\frac{1}{2} + \frac{1}{2} \erf\left( \frac{\mathbf{x}^\top\mathbf{M}^\top\mathbf{Mw}}{\sqrt{2}\|\mathbf{M}_\perp \mathbf{w}\|_2} \right) \right) \exp\left( \! - \frac{((\mathbf{x}')^\top \mathbf{M}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)| \sign(\mathbf{Mx}')\!=\!\sign({\mathbf{Mx}})\!  =\! \mathbf{u}  \right] \nonumber \\
    &\quad \times \frac{ \mathbf{w}^\top \mathbf{M}_\perp^\top }{\sqrt{2 \pi}\|\mathbf{M}_\perp \mathbf{w}\|_2}   \label{hhj} 
    \end{align}
where \eqref{hhj} is due to the Gaussian CDF.
Note that
\begin{align}
    &\mathbb{E}_{\mathbf{u},\mathbf{Mx},\mathbf{Mx}'} \left[  \mathbf{M}\mathbf{x}  \exp\left( - \frac{((\mathbf{x}')^\top \mathbf{M}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)| \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})  = \mathbf{u}  \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{u},\mathbf{M}\mathbf{x},\mathbf{Mx}'} \left[ \diag(\mathbf{u}) |\mathbf{M}\mathbf{x} | \exp\left( - \frac{(|\mathbf{Mx}'|^\top\diag(\mathbf{u})\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right) \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{M}\mathbf{x},\mathbf{Mx}'} \left[ \mathbb{E}_{\mathbf{u}}\left[ \diag(\mathbf{u}) |\mathbf{M}\mathbf{x} | \left(1  - \frac{(|\mathbf{Mx}'|^\top\diag(\mathbf{u})\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} + \frac{(|\mathbf{Mx}'|^\top\diag(\mathbf{u})\mathbf{Mw})^4}{2\|\mathbf{M}_\perp \mathbf{w}\|_2^4} -\dots \right)\right] \right] \label{aza} \\
    &= \mathbf{0} \label{ewe}
\end{align}
where \eqref{ewe} follows since each term in \eqref{aza} is an odd power of $\mathbf{u}$.
  Thus, from \eqref{hhj} we have
  \begin{align}
\mathbf{A}_{\parallel,\perp}(\mathbf{w})     &=  \mathbb{E}_{\mathbf{u},\mathbf{Mx},\mathbf{Mx}'} \left[  \mathbf{M}\mathbf{x} \erf\left( \frac{\mathbf{x}^\top\mathbf{M}^\top\mathbf{Mw}}{\sqrt{2}\|\mathbf{M}_\perp \mathbf{w}\|_2} \right)  \exp\left( - \frac{((\mathbf{x}')^\top \mathbf{M}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)| \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})  =\mathbf{u}  \right] \nonumber \\
    &\quad \times \frac{ \mathbf{w}^\top \mathbf{M}_\perp^\top }{2\sqrt{2\pi}\|\mathbf{M}_\perp \mathbf{w}\|_2} \label{sds}
    % &= \mathbb{E}_{\mathbf{x},\mathbf{Mx}'} \left[  \mathbf{M}\mathbf{x} \erf\left( \frac{\mathbf{x}^\top\mathbf{M}^\top\mathbf{Mw}}{\sqrt{2}\|\mathbf{M}_\perp \mathbf{w}\|_2} \right)  \exp\left( - \frac{((\mathbf{x}')^\top \mathbf{M}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} \right)| \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})   = \mathbf{u} \right]\nonumber\\
    % &\quad \times \frac{ \mathbf{w}^\top \mathbf{M}^\top }{2\sqrt{2\pi}\|\mathbf{M}_\perp \mathbf{w}\|_2} \nonumber \\
    \end{align}
Next we take the Taylor expansions of $\erf(x)$ and $\exp(-x^2)$ to obtain 
    \begin{align}
\mathbf{A}_{\parallel,\perp}(\mathbf{w}) 
&= \mathbb{E}_{\mathbf{u},\mathbf{Mx},\mathbf{Mx}'} \Bigg[  \mathbf{M}\mathbf{x} \left( \frac{\mathbf{x}^\top\mathbf{M}^\top\mathbf{Mw}}{\|\mathbf{M}_\perp \mathbf{w}\|_2} 
 - \frac{ (\mathbf{x}^\top\mathbf{M}^\top\mathbf{Mw})^3 }{6\|\mathbf{M}_\perp \mathbf{w}\|_2^3} + \dots \right)\nonumber \\
 &\quad \quad \quad \quad \times \left(1  - \frac{((\mathbf{x}')^\top \mathbf{M}^\top\mathbf{Mw})^2}{2\|\mathbf{M}_\perp\mathbf{w}\|_2^2} + \dots \right)| \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})   = \mathbf{u} \Bigg]\frac{ \mathbf{w}^\top \mathbf{M}_\perp^\top }{2{\pi}\|\mathbf{M}_\perp \mathbf{w}\|_2} \nonumber\\
    % &\quad \times \frac{ \mathbf{w}^\top \mathbf{M}^\top }{2{\pi}\|\mathbf{M}_\perp \mathbf{w}\|_2} \nonumber \\
    &= \mathbb{E}_{\mathbf{u},\mathbf{Mx},\mathbf{Mx}'} \left[  \mathbf{M}\mathbf{x}\mathbf{x}^\top\mathbf{M}^\top | 
 \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})  = \mathbf{u} \right]\frac{ \mathbf{Mw}\mathbf{w}^\top \mathbf{M}_\perp^\top }{2{\pi}\|\mathbf{M}_\perp\mathbf{w}\|_2^2}  + \mathbf{E} \nonumber \\
 &= \mathbb{E}_{\mathbf{Mx}} \left[  \mathbf{M}\mathbf{x}\mathbf{x}^\top\mathbf{M}^\top \right]\frac{ \mathbf{Mw}\mathbf{w}^\top \mathbf{M}_\perp^\top }{2{\pi}\|\mathbf{M}_\perp\mathbf{w}\|_2^2}  + \mathbf{E} \nonumber \\
 &=   \frac{ \mathbf{Mw}\mathbf{w}^\top \mathbf{M}_\perp^\top }{2{\pi}\|\mathbf{M}_\perp\mathbf{w}\|_2^2}  + \mathbf{E} \nonumber 
\end{align}
where $\|\mathbf{E}\|_2 = O\left( \frac{r^{3.5}+\log^{3.5}(m/\delta)}{d^{1.5}} \right)$ since $\|\mathbf{M}_\perp \mathbf{w}\|_2 = \Omega(\sqrt{d})$ and $\|\mathbf{Mw}\|_2 = O(\sqrt{r} + \sqrt{\log(m/\delta)})$ as $\mathbf{w} \in \mathcal{G}_{\mathbf{w}}(\delta)$ and $m/\delta = O(e^d)$.
% and $\mathbb{E}_{\mathbf{u},\mathbf{x},\mathbf{Mx}'} \left[  \mathbf{M}\mathbf{x}\mathbf{x}^\top\mathbf{M}^\top | 
 % \sign(\mathbf{Mx}')=\sign({\mathbf{Mx}})  = \mathbf{u} \right] = \mathbf{I}_r$ due to the same argument as in \eqref{dfc}.
% Using the Taylor expansions of $\erf$ and $\exp$ 
% to get last line: condition on sign(z) = v and sign(z)= - v 
\end{proof}


% \textbf{Extension to other losses.} We have only considered the hinge loss for simplicity. However, our observation that multitasking with task-specific heads induces a contrastive loss that encourages feature learning extends to other loss functions as well. If we instead use the logistic loss function for binary classification, we find that the task-specific head for task $i$  updated after step of gradient descent starting from zero has the same form as \eqref{head1} up to an absolute constant, 
% % $\mathbf{a}_{1,i} = \frac{1}{2}\mathbb{E}_{(\mathbf{x}_i,y_i)}[y_i \sigma(\mathbf{W}_0 \mathbf{x})]$
% % the logistic loss $\ell(\hat{y}, y) \coloneqq \log(1 + e^{-y\hat{y}})$ satisfies that
% and the global loss induced by the updated heads has the form
% \begin{align}
%     \mathcal{L} = \mathbb{E}_{i,\mathbf{x}_i,y_i}[\log(1 + \exp(- \mathbb{E}_{\mathbf{x}_i,y_i}))]
% \end{align}
% This loss again encourages 
% We verify empirically in Section \ref{sec:sims} that multi-tasking with the logistic loss on sparse parity tasks indeed learns the correct representation, while running on only a single task fails to do so. 
% For regression with the squared loss, we again have that starting from $\mathbf{a}_{i,0}$ and executing one GD update for task $i$'s  head results in $\mathbf{a}_{i,1} = \eta \mathbb{E}[y_i\sigma (\mathbf{W}\mathbf{x}_i)]$, which is the same form as the updates for the hinge and logistic loss. The resulting global loss is thus again a function of inner products between the representations of pairs of samples, but its connection with contrastive learning is less clear, as contrastive learning is motivated by data with class structure, not regression data.




\input{Proof_Rep2-ICML}




==> Proof_RepLearn.tex <==
\section{Proofs of Proposition \ref{prop:1} and Theorem \ref{thm:1}} \label{app:thrm1}


In this section we prove Proposition \ref{prop:1} and Theorem \ref{thm:1}. Throughout, we will abuse notation by reusing $c,c',c''$ and $C$ as absolute constants independent of all other parameters. The notations $O(\cdot)$, $\Theta(\cdot)$, and $\Omega(\cdot)$ describe scalings up to absolute constants independent of all other parameters. We start by establishing that each neuron is in general position with high probability at initialization.
% For convenience, we restate Proposition \ref{prop:1} here.

% \begin{theorem}
    
% \end{theorem}
% \begin{proof}
    
% \end{proof}
% need to show that for every task, there exists a good network with the same set of features
% just need one feature in each orthant, then can learn any function by adding biases
% bias should be between closest vertex sum and second closest vertex sum (flip one coord)

% with random features you could still get one feature closest to each vertex with only r2^r features. but the issue is that changing one coordinate of the perp would deactivate the neuron. should be able to build a lower bound out of this -- the lower bound should be k2^k neurons required. we want features that are robust to changes in the perp.

% \begin{lemma}
%     the biases and weights are in a nice set at initialization whp

%     each is initialized at the same scale
% \end{lemma}

% \begin{proof}
    
% \end{proof}





% 1. compute A

% 2. w+ has the right norm and points in the right direction in parallel space

% 3. so we can again say that with high probability, there exists a subset of good indicators

% 4. how does bias affect analysis?


% \begin{lemma}
%     for all j, the hypercube to gaussian error vector has expected norm squared at most c/k2
% \end{lemma}

% \begin{proof}
    
% \end{proof}

% \begin{lemma}
%     for all j, the other error vectors have expected norm squared sufficiently small
% \end{lemma}

% \begin{proof}
    
% \end{proof}

% \input{Proof_Errors}



\begin{lemma}[Initialization I] \label{lem:init}
    % With probability at least $1-\delta$, all neuron weights satisfy:
    % \begin{align}
    %     \leq \|\mathbf{w}_{j}^0\|_2 \leq  \nonumber \\
    % \end{align}
    % a constant fraction of neurons are good, in the sense that 

    % 1. error vector is less than c/k, other errors are sufficiently small

    % 2. w|| is large enough

    % 3. need bias in an interval like [rt(r) - 1/rt(r), rt(r)]. which occurs with prob 1/rt(r). too small. but still a good network exists. so can jointly optimize a,b. to get a good network...no. not jointly convex in a,b

    % or, make different generalization arguement... 
    Define the set 
    \begin{align}
        \mathcal{G}_{\mathbf{w}} \coloneqq \big\{&\mathbf{w}\in \mathbb{R}^d :  \|\mathbf{w}_{:r}\|_2 \leq c \nu_{\mathbf{w}}( \sqrt{r} + \sqrt{\log(m)}), \nonumber \\
        &\quad  c\nu_{\mathbf{w}}(\sqrt{d-r} - \sqrt{\log(m)}) \leq \|\mathbf{w}_{r:} \|_2 \leq c\nu_{\mathbf{w}}(\sqrt{d-r} + \sqrt{\log(m)}), \nonumber \\
        &\quad c\nu_{\mathbf{w}}(\sqrt{d} - \sqrt{\log(m)}) \leq \|\mathbf{w} \|_2 \leq c\nu_{\mathbf{w}}(\sqrt{d} + \sqrt{\log(m)}) \big\}
    \end{align} for an absolute constant $c$
    with probability at least $0.999$, $\mathbf{w}_{j}\in \mathcal{G}_{\mathbf{w}}$ for all $j\in [m]$.
\end{lemma}

\begin{proof}
% chebyshev to upper bound probability of bad neuron, then
    % hoeffding
Since each $\mathbf{w}_j\sim \mathcal{N}(\mathbf{0}_d,\nu_{\mathbf{w}}^2\mathbf{I}_d)$, each $\|\mathbf{w}_{:r}\|_2$, $\|\mathbf{w}_{r:}\|_2$, and $\|\mathbf{w}\|_2$ are sub-gaussian with parameter $\nu_{\mathbf{w}}$, i.e.
\begin{align}
    \mathbb{P}_{\mathbf{w}_{j,:r}}[| \|\mathbf{w}_{j,:r}\|_2 - \nu_{\mathbf{w}}\sqrt{r}| \leq t] \leq e^{-c' t^2/\nu_{\mathbf{w}}^2}
\end{align}
Choosing $t = c'' \nu_{\mathbf{w}}\sqrt{\log(m)}$ and union bounding over all $j\in [m]$ completes the proof.
\end{proof}

\begin{lemma}[Initialization II] \label{lem:init2}
    % With probability at least $1-\delta$, all neuron weights satisfy:
    % \begin{align}
    %     \leq \|\mathbf{w}_{j}^0\|_2 \leq  \nonumber \\
    % \end{align}
    % a constant fraction of neurons are good, in the sense that 

    % 1. error vector is less than c/k, other errors are sufficiently small

    % 2. w|| is large enough

    % 3. need bias in an interval like [rt(r) - 1/rt(r), rt(r)]. which occurs with prob 1/rt(r). too small. but still a good network exists. so can jointly optimize a,b. to get a good network...no. not jointly convex in a,b

    % or, make different generalization arguement... 
Suppose $m >r$. For an absolute constant $c$,
    \begin{align}
        \sigma_{\min}(\mathbf{W}^0) \geq \nu_{\mathbf{w}}\sqrt{m}\left(1 - c\frac{\sqrt{r}}{\sqrt{m}}\right)
    \end{align}
    With probability at least $0.999$.
\end{lemma}

\begin{proof}
% Since each $\mathbf{w}_j\sim \mathcal{N}(\mathbf{0}_d,\nu_{\mathbf{w}}^2\mathbf{I}_d)$, each $\|\mathbf{w}_{:r}\|_2$, $\|\mathbf{w}_{r:}\|_2$, and $\|\mathbf{w}\|_2$ are sub-gaussian with parameter $\nu_{\mathbf{w}}$, i.e.
% \begin{align}
%     \mathbb{P}_{\mathbf{w}_{j,:r}}[| \|\mathbf{w}_{j,:r}\|_2 - \sqrt{r}| \leq t] \leq e^{-c' t^2/\nu_{\mathbf{w}}^2}
% \end{align}
% Choosing $t = c'' \nu_{\mathbf{w}}\sqrt{\log(m)}$ and union bounding over all $j\in [m]$ completes the proof.
The result follows by the fact that each row of $\mathbf{W}^0$ is drawn independently from $\mathcal{N}(\mathbf{0}_d,\nu_{\mathbf{w}}^2\mathbf{I}_d)$ and applying a standard sub-Gaussian matrix concentration inequality (e.g. Equation 4.22 in \cite{vershynin2018high}).
\end{proof}

% \begin{lemma}
%     since the number of neurons is large enough, this set covers all $2^r$ vertices
% \end{lemma}

% \begin{proof}
%     balls and bins. but being in the set changes the distribution? should still work.
% \end{proof}

W e use $\hat{\mathbb{E}}_{\mathbf{x}\sim \mathcal{D}}[h(\mathbf{x})]$ to denote the empirical mean of $h(\mathbf{x})$ over the data in $\mathcal{D}$.

\begin{lemma}
    Let $\lambda_{\mathbf{a}} = \frac{1}{\eta}$ and $\mathbf{x}\sim \mathcal{N}(\mathbf{0}_d,\mathbf{I}_d)$ On the first iteration of the multi-task learning algorithm described in Section \ref{sec:alg}, the locally updated head for task $i$ is:
    \begin{align}
        \mathbf{a}_{i}^1 = \eta \hat{\mathbb{E}}_{\mathbf{x}\sim \mathcal{D}_{\mathbf{a}_i^1}} [ {f}^*_{i}(\mathbf{x}) \sigma(\mathbf{W}^0\mathbf{x}) ]
    \end{align}
    for all tasks $i\in [T]$.
\end{lemma}

\begin{proof}
For ease of notation we let $\mathbf{a}_i = \mathbf{a}_i^0$. Due to the symmetric initialization, $\mathbf{a}_{i}^\top  \sigma(\mathbf{W}^0\mathbf{x} + \mathbf{b}^0)=0$ for all $\mathbf{x}$ and all tasks $i$.
Therefore, $\max(1 - f^*_{i}(\mathbf{x}) \mathbf{a}_i^\top  \sigma(\mathbf{W}^0\mathbf{x} + \mathbf{b}^0) , 0) = 1 - f^*_{i}(\mathbf{x}) \mathbf{a}_i^\top  \sigma(\mathbf{W}^0\mathbf{x} )$, and
\begin{align} %_{\mathbf{a},0}
\mathbf{a}_{i}^1 &= \mathbf{a}_i - \eta \nabla \mathcal{L}_i(\mathbf{W}^0,\mathbf{b}^0,\mathbf{a}_i) \nonumber \\
&= (1 - \eta \lambda_{\mathbf{a}}) \mathbf{a}_i - \eta \nabla_{\mathbf{a}} \hat{\mathbb{E}}_{\mathbf{x}\sim \mathcal{D}_{\mathbf{a}_i^0}}[ \max(1 - f^*_{i}(\mathbf{x}) \mathbf{a}_i^\top  \sigma(\mathbf{W}^0\mathbf{x} + \mathbf{b}^0) , 0) ]\nonumber \\
&= (1 - \eta \lambda_{\mathbf{a}}) \mathbf{a}_i + \eta \hat{\mathbb{E}}_{\mathbf{x}\sim \mathcal{D}_{\mathbf{a}_i^1}}[ f^*_{i}(\mathbf{x}) \sigma(\mathbf{W}^0\mathbf{x} ) ] \label{sym} \\
&= \eta \hat{\mathbb{E}}_{\mathbf{x}\sim \mathcal{D}_{\mathbf{a}_i^1}} [{f}^*_{i}(\mathbf{x}) \sigma(\mathbf{W}^0\mathbf{x} + \mathbf{b}^0) ]  \label{lam}
\end{align}
where \eqref{sym} follows by the symmetric initialization and \eqref{lam} follows by choice of $\lambda_{\mathbf{a}}$.
\end{proof}


\begin{lemma} \label{lem:loss}
The loss after updating the heads one the first iteration is given by
%     \begin{align}
%      &   \mathcal{L}(\mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{1,i} \}_{i\in \mathcal{T}}) \nonumber \\
% &=  \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) <1\}\nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \}  \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz}) \Big] \nonumber 
%     \end{align}
        \begin{align}
     &   \mathcal{L}(\mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{i}^1 \}_{i=1}^T) \nonumber \\
%      \nonumber \\
% &=  \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) <1\}\nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \}  \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz}) \Big] \nonumber 
&=  1 -   \E_{\mathbf{x}, \mathbf{x}' }  \left[ \chi\{\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}_{:r}') \} \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})  \right] \nonumber \\
&\quad -  \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
&\quad + \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\right\} \nonumber \\
&\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber 
    \end{align}
\end{lemma}

\begin{proof}
% Let $g(\mathbf{x}; \mathbf{W}^0) \coloneqq $
Using the computation of each $\mathbf{a}_{i}^+$ from Lemma \ref{lem:loss}, and the fact that $\mathbf{b}^0 = \mathbf{0}$ by choice of initialization, 
\begin{align}
   & \mathcal{L}(\mathbf{W}^0,\mathbf{b}^0,\{\mathbf{a}^+_{i}\}_{i=1}^T) \nonumber \\
   &= \frac{1}{T} \sum_{i=1}^T \mathcal{L}_i(\mathbf{W}^0,\mathbf{b}^0,\{\mathbf{a}_{i}^+\}_{i=1}^T)
    \nonumber \\
    &= \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x} }  \left[ \max\left( 1- \eta {f}_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}'} [ {f}^*_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}') ]^\top \sigma(\mathbf{W}^0\mathbf{x}) , 0 \right) \right]     \nonumber \\
%     &= \E_{\mathbf{x} }  \left[ \max\left( 1- \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}'} [ f^*_{i}(\mathbf{x}') g(\mathbf{x}';\mathbf{W}^0,\mathbf{b}^0 ) ]^\top g(\mathbf{x}; \mathbf{W}^0,\mathbf{b}^0)  , 0 \right) 
% %     \frac{1}{n_2}\sum_{j=1}^{n_2}\max \left(1 - y_{i,j} \left(\frac{1}{\lambda_{1}n_1}\sum_{j'=1}^{n_1}\bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})  \right)^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}), 0\right) \right] \nonumber\\
% % &= 1 -  \E_{i }  \left[ \frac{1}{\lambda_{1} n_1n_2}\sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})
% \right] \label{14} \nonumber \\
&=\frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta {f}_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ {f}^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) <1\right\} \nonumber \\
&\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - \eta{f}_{i}^*(\mathbf{x})  {f}^*_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber \\
&=  1 -   \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[   \left(\frac{1}{T} \sum_{i=1}^T {f}_{i}^*(\mathbf{x})  {f}^*_{i}(\mathbf{x}') \right) \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})  \right]  \nonumber \\
&\quad + \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta {f}_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ {f}^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\right\} \nonumber \\
&\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - \eta f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber 
\end{align}
Next, using the fact that $\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}_{:r}')$ implies $f_{i}^*(\mathbf{x}) = f^*_{i}(\mathbf{x}')$ for all $i\in [n]$, we have 
% \begin{align}
% &=  1 -   \E_{\mathbf{x}, \mathbf{x}' }  \left[ \{\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})  \right] \nonumber \\
% &\quad -  \E_{\mathbf{x}, \mathbf{x}' }  \left[\{\sign(\mathbf{x}_{:r}) = - \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
% &\quad -  \E_{\mathbf{x}, \mathbf{x}' }  \left[\{\sign(\mathbf{x}_{:r}) \neq  \pm \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
% &\quad - \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\right\} \nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber \\
% &=  1 -   \E_{\mathbf{x}, \mathbf{x}' }  \left[ \{\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}_{:r}') \} \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})  \right] \nonumber \\
% &\quad -  \E_{\mathbf{x}, \mathbf{x}' }  \left[\{\sign(\mathbf{x}_{:r}) = - \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
% &\quad -  \E_{\mathbf{x}, \mathbf{x}' }  \left[\{\sign(\mathbf{x}_{:r}) \neq  \pm \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
% &\quad - \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\right\} \nonumber \\
% &\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber \\
% \end{align}
\begin{align}
&=  1 -   \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[ \chi\{\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})  \right] \nonumber \\
% &\quad -  \E_{\mathbf{x}, \mathbf{x}' }  \left[\{\sign(\mathbf{x}_{:r}) = - \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
&\quad -  \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{x}_{:r}) \neq   \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
&\quad + \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\right\} \nonumber \\
&\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - \eta f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber \\
&=  1 -   \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[ \chi\{\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}_{:r}') \} \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})  \right] \nonumber \\
&\quad - \eta  \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
&\quad + \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\right\} \nonumber \\
&\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - \eta f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber 
\end{align}
\end{proof}




% \begin{align}
%     \nabla_{\mathbf{w}_{j,0}}\mathcal{L}(\mathbf{W}^0,\mathbf{b}^0,\{\mathbf{a}_{0,i}\}_{i}) &=
%     % \E_{i, \mathbf{x} }  \left[ \max\left( 1- \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}'} [ f^*_{i}(\mathbf{x}') g(\mathbf{x}';\mathbf{W}^0,\mathbf{b}^0 ) ]^\top g(\mathbf{x}; \mathbf{W}^0,\mathbf{b}^0)  , 0 \right) 
% %     \frac{1}{n_2}\sum_{j=1}^{n_2}\max \left(1 - y_{i,j} \left(\frac{1}{\lambda_{1}n_1}\sum_{j'=1}^{n_1}\bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})  \right)^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}), 0\right) \right] \nonumber\\
% % &= 1 -  \E_{i }  \left[ \frac{1}{\lambda_{1} n_1n_2}\sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})
% % \right] \label{14} \nonumber \\
%  -\E_{\mathbf{x}, \mathbf{x}' }  \left[  \mathbb{E}_i[f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}')] \mathbf{zz}'T \sigma'((\mathbf{w}_{j}^0)^\top \mathbf{x} + b_{j,0})\sigma'((\mathbf{w}_{j}^0)^\top \mathbf{x}' + b_{j,0})  \right]
% \end{align}



\begin{lemma}\label{lem:tasks}
    % Suppose the set of tasks $\mathcal{T}$ is defined as:
    % \begin{align}
    %     \mathcal{T} \coloneqq \{ f_i^*:\{-1,1\}^r \rightarrow \{-1,1\} | f_i^*(\mathbf{v}) = \prod_{j \in A} v_j, \; A \subseteq [r]  \}.
    % \end{align}
    % Then 
    Under Assumption \ref{assump:diversity}, for all $(\mathbf{v},\mathbf{v}')\in \{-1,1\}^r \times  \{-1,1\}^r$ such that $\mathbf{v}\neq \pm \mathbf{v}'$,
    \begin{align}
       \left| \frac{1}{T}\sum_{i=1}^T \chi\{\bar{f}_i^*(\mathbf{v}) \neq \bar{f}_i^*(\mathbf{v}')\} - \frac{1}{2}\right| &= c\frac{\sqrt{r}}{\sqrt{T}}
    \end{align}
    with probability at least $0.999$ over the random draw of $T$ tasks from $\mathcal{T}$, for an absolute constant $c$.
\end{lemma}

\begin{proof}
% Let $\mathbf{v}_1,\dots,\mathbf{v}_{2^r}$ denote an ordering of the $2^r$ vertices on the $r$-dimensional hypercube $\{-1,1\}^r$.
% Note that any task $f_i^*: \{-1,1\}^r \rightarrow \{-1,1\}$ can be represented as a vector $f_i$ in $ \{ -1, 1\}^{2^r}$. 
% Note that for any differing v,v', 
Under Assumption \ref{assump:diversity}, each $\chi\{\bar{f}_i^*(\mathbf{v}) \neq \bar{f}_i^*(\mathbf{v}')\}$ is an i.i.d. Bernoulli random variable with parameter $\frac{1}{2}$. Thus, for any particular $(\mathbf{v},\mathbf{v}')\in \{-1,1\}^r \times  \{-1,1\}^r$ such that $\mathbf{v}\neq \pm \mathbf{v}'$, we have 
\begin{align}
    \mathbb{P}\left[ \left| \frac{1}{T}\sum_{i=1}^T \chi\{\bar{f}_i^*(\mathbf{v}) \neq \bar{f}_i^*(\mathbf{v}')\} - \frac{1}{2}\right|   \geq t\right] \leq \exp\left( - \frac{T t^2}{2} \right) 
\end{align}
for any $t\geq 0$.  
Union bounding over all $O\left(2^{2r}\right)$ pairs $(\mathbf{v},\mathbf{v}')\in \{-1,1\}^r \times  \{-1,1\}^r$ and choosing $t = \frac{\sqrt{c'\log(2^{2r})}}{\sqrt{T}}$ completes the proof.
\end{proof}



\begin{lemma}\label{lem:compute_grad}
For any  $j\in [m]$ such that $\mathbf{w}_{j}^0\in \mathcal{G}_{\mathbf{w}}$, then 
% $\nabla_{\mathbf{w}_j}\mathcal{L}(\mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{1,i} \}_{i\in \mathcal{T}})$
    % The gradient of the global loss with respect to the representation after updating the task-specific heads on the first iteration is $-\frac{1}{2^{r}\lambda_1}\mathbf{A}(\w)\w$, where
%     \begin{align}
%     \w^+ &= \w(1 - \eta \lambda) + \eta \begin{bmatrix}
%         \mathbf{A}_{||,||}(\w) &  \mathbf{A}_{||,\perp}(\w) \\
%         \mathbf{A}_{\perp,||}(\w) & \mathbf{A}_{\perp,\perp}(\w) \\
%     \end{bmatrix}\w
% \end{align}
    \begin{align}
 \nabla_{\mathbf{w}_j} \mathcal{L}( \mathbf{W}^0, \mathbf{b}^0, \{ \mathbf{a}_{i}^0 \}_{i\in [T]} )  &=  - \eta^2  2^{-r}  \mathbf{A}(\mathbf{w}_{j}^0) \mathbf{w}_{j}^0 + \eta \mathbf{e}  %\\\lambda_{\mathbf{w}}\mathbf{w}_{j,0} 
 % & \coloneqq \begin{bmatrix}
 %        \mathbf{A}_{||,||}(\w) &  \mathbf{A}_{||,\perp}(\w) \\
 %        \mathbf{A}_{\perp,||}(\w) & \mathbf{A}_{\perp,\perp}(\w) \\
 %    \end{bmatrix} 
\end{align} 
where $\|\mathbf{e} \|_2 \leq O( \nu_{\mathbf{w}} de^{-c d } + \nu_{\mathbf{w}} d \frac{\sqrt{r}}{\sqrt{T}} )$ and  $\mathbf{A}(\mathbf{w}_{j}^0) \coloneqq \begin{bmatrix}
         \mathbf{A}_{||,||}(\mathbf{w}_{j}^0) &  \mathbf{A}_{||,\perp}(\mathbf{w}_{j}^0) \\
         \mathbf{A}_{\perp,||}(\mathbf{w}_{j}^0) & \mathbf{A}_{\perp,\perp}(\mathbf{w}_{j}^0) \\
   \end{bmatrix} $ for matrices $\mathbf{A}_{\parallel,\parallel}(\mathbf{w}_{j}^0) \in \mathbb{R}^{r \times r}$, $\mathbf{A}_{\parallel,\perp}(\mathbf{w}_{j}^0) \in \mathbb{R}^{r \times (d-r)}$,  $\mathbf{A}_{\perp,\parallel}(\mathbf{w}_{j}^0) \in \mathbb{R}^{r \times (d-r)}$, $\mathbf{A}_{\perp,\perp}(\mathbf{w}_{j}^0) \in \mathbb{R}^{(d-r) \times (d-r)}$. Let  $\mathbf{u}\sim \text{Unif}(\{-1,1\}^r)$ be a random variable drawn uniformly from the Rademacher hypercube in $r$ dimensions, and $\mathbf{x}$ and $\mathbf{x}'$ be drawn independently from $\mathcal{N}(\mathbf{0}_d,\mathbf{I}_d)$, then for any $\mathbf{w}\in \mathbb{R}^d$ the matrices $\mathbf{A}_{||,||}(\w)$, $\mathbf{A}_{||,\perp}(\w)$, $\mathbf{A}_{\perp,||}(\w)$, and $\mathbf{A}_{\perp,\perp}(\w)$ are defined as
\begin{align}
    \mathbf{A}_{||,||}(\w) &= 
    % \mathbb{E}_{\mathbf{x}} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2 \mathbf{uu}^\top  
    \mathbb{E}_{\mathbf{u}} \left[   \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[
    {\sigma}'(\mathbf{w}^\top  \mathbf{x}) \sigma'(\mathbf{w}^\top \mathbf{x}') \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top |\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') = \mathbf{u}
    \right] \right]\\
    \mathbf{A}_{||,\perp}(\w) &= \mathbb{E}_{\mathbf{u}} \left[   \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[\sigma'( \mathbf{w}^\top \mathbf{x})  \sigma'(\mathbf{w}^\top \mathbf{x})\mathbf{x}_{:r} (\mathbf{x}_{r:}')^\top | \sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') = \mathbf{u} \right]\right] \\
    \mathbf{A}_{\perp,||}(\w) &=  \mathbb{E}_{\mathbf{u}}\left[\mathbb{E}_{\mathbf{x},\mathbf{x}'}\left[\sigma'( \mathbf{w}^\top \mathbf{x} )\sigma'( \mathbf{w}^\top \mathbf{x}' ) \mathbf{x}_{r:}(\mathbf{x}_{:r}')^\top |\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') = \mathbf{u}\right] \right]   \\
    \mathbf{A}_{\perp,\perp}(\w) &=  \mathbb{E}_{\mathbf{u}}\left[ \mathbb{E}_{,\mathbf{x},\mathbf{x}'}\left[ \sigma'( \mathbf{w}^\top \mathbf{x} )\sigma'( \mathbf{w}^\top \mathbf{x}' ) \mathbf{x}_{r:}(\mathbf{x}_{r:}')^\top |  \sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') = \mathbf{u}\right]\right]
    % \mathbf{A}_{||,\perp}(\w) &= \mathbb{E}_{\mathbf{}\sim \Unif(\mathcal{H}^{r})}\left[ \mathbb{E}_{\mathbf{v}\sim \Unif( \mathcal{H}^{d-r})} \left[\sigma'( \mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right] \mathbf{u} \mathbb{E}_{\mathbf{v}\sim \Unif(\mathcal{H}^{d-r})}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right] \\
    % \mathbf{A}_{\perp,||}(\w) &=  \mathbb{E}_{\mathbf{u}\sim \Unif(\mathcal{H}^{r})}\left[  \mathbb{E}_{\mathbf{v}\sim \Unif(\mathcal{H}^{d-r})}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right] \mathbb{E}_{\mathbf{v}\sim \Unif(\mathcal{H}^{d-r})} \left[\sigma'( \mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\right] \mathbf{u}^\top  \right] \\
    % \mathbf{A}_{\perp,\perp}(\w) &=  \mathbb{E}_{\mathbf{u}\sim \Unif(\mathcal{H}^{r})}\left[  \mathbb{E}_{\mathbf{v}\sim \Unif( \mathcal{H}^{d-r})}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]  \mathbb{E}_{\mathbf{v}\sim \Unif(\mathcal{H}^{d-r})}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right] 
\end{align}
\end{lemma}



\begin{proof}
Using  Lemma \ref{lem:loss}, we have  
% \begin{align}  
% % &  \frac{1}{\lambda_{1}  } \mathbb{E}_{\mathbf{x},\mathbf{x}',i} \left[  f_{i}^*(\mathbf{x}) f_{i}^*(\mathbf{x}') \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz})\right] \nonumber \\
% &\mathcal{L}(\mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{1,i} \}_{i\in \mathcal{T}})\nonumber \\
% &=  \eta  \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) <1\}\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \}  \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz}) \Big] \nonumber \\
% &= \eta  \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \}  \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz}) \Big] \nonumber \\
% &\quad  - \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\}\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \}  \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz}) \Big] \nonumber  
% \end{align} 
\begin{align}
&\mathcal{L}(\mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{i}^+ \}_{i\in [T]})\nonumber \\
&=  1 -  \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[ \chi\{\sign(\mathbf{x}_{:r}) = \sign(\mathbf{x}_{:r}') \} \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})  \right] \nonumber \\
&\quad - \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x})\right]   \nonumber \\
&\quad + \frac{1}{T} \sum_{i=1}^T \E_{\mathbf{x}, \mathbf{x}' }  \Big[  \chi\left\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\right\} \nonumber \\
&\quad \quad \quad \quad \quad \quad \quad \quad \quad \times \left( 1 - \eta f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma(\mathbf{W}^0\mathbf{x}) \right) \Big] \nonumber 
\end{align}

Let $\mathbf{u} \sim \text{Unif}(\{-1,1\}^r)$ be uniformly drawn from the $r$-dimensional hypercube. Taking the gradient of both terms with respect to $\mathbf{w}_j$ yields
\begin{align}  
% &  \frac{1}{\lambda_{1}  } \mathbb{E}_{\mathbf{x},\mathbf{x}',i} \left[  f_{i}^*(\mathbf{x}) f_{i}^*(\mathbf{x}') \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz})\right] \nonumber \\
&\nabla_{\mathbf{w}_j}\mathcal{L}(\mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{i}^+ \}_{i\in [T]})\nonumber \\
&= -  \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}((\mathbf{w}_{j}^0)^\top\mathbf{x}') \sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x} \Big] \nonumber \\
&\quad - \eta \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma(\mathbf{W}^0\mathbf{x}')^\top \sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x} \right]   \nonumber \\
&\quad - \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma((\mathbf{w}_{j}^0)^\top\mathbf{x}'' ) ]^\top \sigma((\mathbf{w}_{j}^0)^\top\mathbf{x}) >1\} {\sigma}((\mathbf{w}_{j}^0)^\top\mathbf{x}') \sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x} \Big] \nonumber  \\
&= \eta 2^{-r}  \mathbb{E}_{\mathbf{u}} \Big[ \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[{\sigma}'((\mathbf{w}_{j}^0)^\top\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top | \sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') = \mathbf{u}\Big] \Big] \mathbf{w}_{j}^0\nonumber \\
&\quad - \eta  \E_{\mathbf{x}, \mathbf{x}' }  \Bigg[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right) \nonumber \\
&\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \times \sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')^\top \sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top \Bigg] \mathbf{w}_{j}^0   \nonumber \\
&\quad - \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\}\nonumber \\
&\quad\quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}'((\mathbf{w}_{j}^0)^\top\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top\Big]\mathbf{w}_{j}^0 \label{shm} \\
&= \eta 2^{-r}\mathbf{A}(\mathbf{w}_{j}^0) \mathbf{w}_{j}^0 \nonumber \\
&\quad - \eta  \E_{\mathbf{x}, \mathbf{x}' }  \Bigg[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\nonumber \\
&\quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \quad \times \sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')^\top \sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top \Bigg] \mathbf{w}_{j}^0   \nonumber \\
&\quad - \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\}\nonumber \\
&\quad\quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}'((\mathbf{w}_{j}^0)^\top\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top\Big]\mathbf{w}_{j}^0 \label{shmm} 
\end{align} 
where we have used $\sigma(x)= \sigma'(x)x$ in \eqref{shm}. It is easy to check that the first term in \eqref{shm} is equal to $\eta 2^{-r}\mathbf{A}(\mathbf{w}_{j}^0) \mathbf{w}_{j}^0$ by definition of $\mathbf{A}(\mathbf{w}_{j}^0)$. Now we show that the remaining terms are small.
The norm of the second term in \eqref{shmm} can be bounded using Jensen's Inequality (which implies $\|\mathbb{E}_{\mathbf{x}}[\mathbf{x}]\|_2\leq \mathbb{E}_{\mathbf{x}}[\|\mathbf{x}\|_2]$  for any random vector $\mathbf{x}$) and the Cauchy-Schwarz Inequality as:
% \begin{align}
%     & \left\|\eta \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top \right] \mathbf{w}_{j}^0   \right\|_2 \nonumber \\
%     &\leq  \eta \|\mathbf{w}_{j}^0 \|_2 \E_{\mathbf{x}, \mathbf{x}' }  \left[ \left\| \chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')^\top \sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top   \right\|_2\right]  \nonumber \\
%     &\leq \eta \|\mathbf{w}_{j}^0 \|_2 \sqrt{ \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)^2 \right]\E_{\mathbf{x}, \mathbf{x}' }  \left[\| \mathbf{x}\|_2^4 \right] } \nonumber \\
%     &\leq \eta \|\mathbf{w}_{j}^0 \|_2 \sqrt{ \frac{ c' r d^2 }{T} } \nonumber \\
%     &= \eta \nu_{\mathbf{w}} c''\frac{\sqrt{r}d^{1.5}}{\sqrt{T}}
% \end{align}
\begin{align}
    & \Big\|\eta \E_{\mathbf{x}, \mathbf{x}' }  \big[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\tfrac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top \big]\mathbf{w}_{j}^0   \Big\|_2 \nonumber \\
    &\leq \eta \Bigg(\E_{\mathbf{x}, \mathbf{x}' }  \left[\left\| \chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}\right\|_2^2 \right] \nonumber \\
    &\quad \quad \quad \E_{\mathbf{x}, \mathbf{x}' }  \left[((\mathbf{x}')^\top \mathbf{w}_{j}^0)^2 \right] \Bigg)^{1/2} \nonumber \\
    &= \eta \| \mathbf{w}_{j}^0\|_2 \nonumber \\
    &\quad \times \E_{\mathbf{x}, \mathbf{x}' }  \left[\left\| \chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}\right\|_2^2 \right]^{1/2}  \nonumber \\
    &\leq \eta \| \mathbf{w}_{j}^0\|_2  \E_{\mathbf{x}, \mathbf{x}' } \left[\left\| \chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \}\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x} \right\|_2^4 \right]^{1/4} \nonumber
    \\
    &\quad \quad \times \E_{\mathbf{x}, \mathbf{x}' } \left[ \left( \frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}')\right)^4 \right]^{1/4} \nonumber \\
    &\leq  \eta \| \mathbf{w}_{j}^0\|_2  \E_{\mathbf{x}, \mathbf{x}' } \left[\left\| \chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \}\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x} \right\|_2^4 \right]^{1/4} c \sqrt{\frac{r}{T}} \nonumber
    \\
    &\leq \eta \| \mathbf{w}_{j}^0\|_2  \E_{\mathbf{x}, \mathbf{x}' } \left[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \}\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\right]^{1/8} \E_{\mathbf{x}} \left[ \left\|\mathbf{x} \right\|_2^8 \right]^{1/8} c \sqrt{\frac{r}{T}}\label{gh}
    \\
    % &\leq \eta \| \mathbf{w}_{j}^0\|_2  \E_{\mathbf{x}, \mathbf{x}' } \left[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \}\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\right]^{1/8} \E_{\mathbf{x}} \left[ \left\|\mathbf{x} \right\|_2^8 \right]^{1/8} c \sqrt{\frac{r}{T}} \nonumber \\
    &\leq 
    \eta \| \mathbf{w}_{j}^0\|_2 \E_{\mathbf{x}} \left[ \left\|\mathbf{x} \right\|_2^8 \right]^{1/8} c \sqrt{\frac{r}{T}} \nonumber \\
    &= 
    \eta \| \mathbf{w}_{j}^0\|_2 (d(d+2)(d+4)(d+6))^{1/8} c \sqrt{\frac{r}{T}} \nonumber\\
    &\leq c' \eta \nu_{\mathbf{w}} \sqrt{\frac{r(d^2+d\log(m))}{T}}\label{gfg} \\
    &\leq c'' \nu_{\mathbf{w}} d \sqrt{\frac{r}{T}}  \nonumber
    % \eta \|c' \eta  \sqrt{\frac{r(d^2+d\log(m))}{T}}\mathbf{w}_{j}^0 \|_2 \E_{\mathbf{x}, \mathbf{x}' }  \left[ \left\| \chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}')^\top \sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top   \right\|_2\right]  \nonumber \\
    % &\leq \eta \|\mathbf{w}_{j}^0 \|_2 \sqrt{ \E_{\mathbf{x}, \mathbf{x}' }  \left[\chi\{\sign(\mathbf{x}_{:r}) \neq  \sign(\mathbf{x}_{:r}') \} \left(\frac{1}{T} \sum_{i=1}^T f_{i}^*(\mathbf{x})  f^*_{i}(\mathbf{x}') \right)^2 \right]\E_{\mathbf{x}, \mathbf{x}' }  \left[\| \mathbf{x}\|_2^4 \right] } \nonumber \\
    % &\leq \eta \|\mathbf{w}_{j}^0 \|_2 \sqrt{ \frac{ c' r d^2 }{T} } \nonumber \\
    % &= \eta \nu_{\mathbf{w}} c''\frac{\sqrt{r}d^{1.5}}{\sqrt{T}}
\end{align}
%https://math.stackexchange.com/questions/2945294/expectation-of-the-norm-of-a-gaussian-vector-raised-to-a-power
where \eqref{gh} follows with probability at least 0.999 by Lemma \ref{lem:tasks} and \eqref{gfg} follows deterministically since $\mathbf{w}_{j}^0\in \mathcal{G}_{\mathbf{w}}$ and $\eta=\Theta(1)$.

The norm of the third term in \eqref{shm} can similarly be bounded as:
% \begin{align}
%     &\Big\|\eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\}\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top\Big]\mathbf{w}_{j}^0 \Big\|_2 \nonumber \\
% &\leq \eta \|\mathbf{w}_{j}^0\|_2 \nonumber \\
% &\quad \times \Big\|\mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\}\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top\Big]\Big\|_2 \nonumber \\
% &\leq \eta \|\mathbf{w}_{j}^0\|_2 \nonumber \\
% &\quad \times \Big(\mathbb{E}_{\mathbf{x}} \big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\}\big]\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \Big\|\mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[\chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}) \mathbf{zz}^\top\mathbf{x}'(\mathbf{x}')^\top\Big]\Big\|_2\Big)^{1/2} \label{cs1} \\
% &\leq \eta \|\mathbf{w}_{j}^0\|_2 \nonumber \\
% &\quad \times \Big(\mathbb{P}_{\mathbf{x},\mathbf{x}'} \big[ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\big]\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \Big\|\mathbb{E}_{\mathbf{x},\mathbf{x}'} \big[\|\mathbf{x}\|_2^2 \|\mathbf{x}'\|_2^2\big]\Big\|_2\Big)^{1/2} \label{less} \\
% &= \eta \|\mathbf{w}_{j}^0\|_2 d \; \mathbb{P}_{\mathbf{x}} \big[ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\big]^{1/2}\nonumber \\
% &= \eta c \nu_{\mathbf{w}} d^{1.5} \; \mathbb{P}_{\mathbf{x}} \big[ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\big]^{1/2}\label{bbb}
% \end{align}
% \begin{align}
%     &\Big\|\eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\}\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top\Big]\mathbf{w}_{j}^0 \Big\|_2 \nonumber \\
% &\leq \eta \mathbb{E}_{\mathbf{x}'}[((\mathbf{x}')^\top\mathbf{w}_{j}^0)^2]^{1/2}\nonumber \\
% &\quad \times \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\}\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\|\mathbf{x}\|_2^2\Big]^{1/2} \nonumber \\
% &\leq \eta \|\mathbf{w}_{j}^0\|_2 \nonumber \\
% &\quad \times \Big(\mathbb{E}_{\mathbf{x}} \big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\}\big]\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[\chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}) \|\mathbf{x}\|_2^4\Big]\Big)^{1/4} \label{cs1} \\
% &= \eta \|\mathbf{w}_{j}^0\|_2 \nonumber \\
% &\quad \times \Big(\mathbb{E}_{\mathbf{x}} \big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\}\big]\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \Big\|\mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[\chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}) \mathbf{zz}^\top\mathbf{x}'(\mathbf{x}')^\top\Big]\Big\|_2\Big)^{1/2}  \nonumber \\
% &\leq \eta \|\mathbf{w}_{j}^0\|_2 \nonumber \\
% &\quad \times \Big(\mathbb{P}_{\mathbf{x},\mathbf{x}'} \big[ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\big]\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \Big\|\mathbb{E}_{\mathbf{x},\mathbf{x}'} \big[\|\mathbf{x}\|_2^2 \|\mathbf{x}'\|_2^2\big]\Big\|_2\Big)^{1/2} \label{less} \\
% &= \eta \|\mathbf{w}_{j}^0\|_2 d \; \mathbb{P}_{\mathbf{x}} \big[ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\big]^{1/2}\nonumber \\
% &= \eta c \nu_{\mathbf{w}} d^{1.5} \; \mathbb{P}_{\mathbf{x}} \big[ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\big]^{1/2}\label{bbb}
% \end{align}
\begin{align}
    &\Big\|\eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\}\nonumber \\
&\quad\quad \quad \quad \quad \quad \times \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\mathbf{x}(\mathbf{x}')^\top\Big]\mathbf{w}_{j}^0 \Big\|_2 \nonumber \\
&\leq \eta  \mathbb{E}_{\mathbf{x}'}[\chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'') ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\}]^{1/2}\nonumber \\
&\quad \times \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\|\mathbf{x}\|_2^2 ((\mathbf{x}')^\top\mathbf{w}_{j}^0)^2\Big]^{1/2} \nonumber \\
&\leq \eta \mathbb{P}_{\mathbf{x}} \big[ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\big]^{1/2}  \nonumber \\
&\quad \quad \times \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\|\mathbf{x}\|_2^4 \Big]^{1/4} \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[((\mathbf{x}')^\top\mathbf{w}_{j}^0)^4 \Big]^{1/4} \nonumber \\
&\leq \eta \mathbb{P}_{\mathbf{x}} \big[ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\big]^{1/2}  \nonumber \\
&\quad \quad \times \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x})\|\mathbf{x}\|_2^4 \Big]^{1/4} \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[((\mathbf{x}')^\top\mathbf{w}_{j}^0)^4 \Big]^{1/4} \nonumber \\
&= c \;\nu_{\mathbf{w}} \;d \;\mathbb{P}_{\mathbf{x}} \big[ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\big]  \label{56}
% &\leq \eta \|\mathbf{w}_{j}^0\|_2 \nonumber \\
% &\quad \times \Big(\mathbb{E}_{\mathbf{x}} \big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\}\big]\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[\chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}) \|\mathbf{x}\|_2^4\Big]\Big)^{1/4} \label{cs1} \\
% &= \eta \|\mathbf{w}_{j}^0\|_2 \nonumber \\
% &\quad \times \Big(\mathbb{E}_{\mathbf{x}} \big[ \chi\{ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\}\big]\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \Big\|\mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[\chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \} {\sigma}'(\mathbf{w}_{j}^0\mathbf{x}')\sigma'((\mathbf{w}_{j}^0)^\top\mathbf{x}) \mathbf{zz}^\top\mathbf{x}'(\mathbf{x}')^\top\Big]\Big\|_2\Big)^{1/2}  \nonumber \\
% &\leq \eta \|\mathbf{w}_{j}^0\|_2 \nonumber \\
% &\quad \times \Big(\mathbb{P}_{\mathbf{x},\mathbf{x}'} \big[ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\big]\nonumber \\
% &\quad\quad \quad \quad \quad \quad \times \Big\|\mathbb{E}_{\mathbf{x},\mathbf{x}'} \big[\|\mathbf{x}\|_2^2 \|\mathbf{x}'\|_2^2\big]\Big\|_2\Big)^{1/2} \label{less} \\
% &= \eta \|\mathbf{w}_{j}^0\|_2 d \; \mathbb{P}_{\mathbf{x}} \big[ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\big]^{1/2}\nonumber \\
% &= \eta c \nu_{\mathbf{w}} d^{1.5} \; \mathbb{P}_{\mathbf{x}} \big[ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' + \mathbf{b}^0) ]^\top \sigma(\mathbf{W}^0\mathbf{x}+\mathbf{b}^0) >1\big]^{1/2}\label{bbb}
\end{align}
where the last line follows since $\eta=\Theta(1)$.
% where \eqref{cs1} follows by the Cauchy-Schwarz Inequality, \eqref{less} follows by Jensen's Inequality, and 
% \eqref{bbb} follows with probability at least $1-$ over the initialization of $\mathbf{w}_{j}^0$. 
Conditioned on $\mathbf{w}_{j}^0\in \mathcal{G}_{\mathbf{w}}$ for all $j\in [m]$, we have $\|\mathbf{W}^0\|_2 \leq c\nu_{\mathbf{w}}(\sqrt{d}+\sqrt{m})$. % and $\|\mathbf{b}^0\|_2 \leq c\sigma_b\sqrt{m}$. Conditioned on  this event,
Thus, we have
\begin{align}
    &\mathbb{P}_{\mathbf{x}} \big[ \eta f_{i}^*(\mathbf{x}) \mathbb{E}_{\mathbf{x}''} [ f^*_{i}(\mathbf{x}'') \sigma(\mathbf{W}^0\mathbf{x}'' ) ]^\top \sigma(\mathbf{W}^0\mathbf{x}) >1\big] \nonumber \\
    &\leq \mathbb{P}_{\mathbf{x}} \left[ \|\mathbb{E}_{\mathbf{x}''} [ \sigma(\mathbf{W}^0\mathbf{x}'') ]\|_2 \|\sigma(\mathbf{W}^0\mathbf{x})\|_2 > \frac{1}{\eta}\right] \nonumber \\
    &\leq \mathbb{P}_{\mathbf{x}} \left[ \mathbb{E}_{\mathbf{x}''} [\| \sigma(\mathbf{W}^0\mathbf{x}'') \|_2] \|\sigma(\mathbf{W}^0\mathbf{x})\|_2 > \frac{1}{\eta}\right] \nonumber \\
    &\leq \mathbb{P}_{\mathbf{x}} \left[ c \|\mathbf{W}^0\|_2^2\mathbb{E}_{\mathbf{x}''} [\|\mathbf{x}'' \|_2] \|\mathbf{x}\|_2 > \frac{1}{\eta}\right] \nonumber \\
    &\leq \mathbb{P}_{\mathbf{x}} \left[ \|\mathbf{x}\|_2  > \frac{1}{c\eta\|\mathbf{W}^0\|_2^2 \sqrt{d}} \right] \nonumber \\
    &\leq \mathbb{P}_{\mathbf{x}} \left[ \|\mathbf{x}\|_2  > \frac{1}{c'\eta\nu_{\mathbf{w}}^2(d+m)\sqrt{d}} \right] \nonumber \\
    &\leq \mathbb{P}_{\mathbf{x}} \left[ \|\mathbf{x}\|_2  > \frac{d}{c''\eta} \right]  \nonumber \\
    &\leq \exp\left(-c'''d^2 \right) \label{38}
    % &\leq \mathbb{P}_{\mathbf{x}} \left[ \|\mathbf{x}\|_2  > \frac{c}{\eta(d+m)\sqrt{d}\nu_{\mathbf{w}}^2 + \eta (\sqrt{d}+\sqrt{m})\sqrt{m} \nu_{\mathbf{w}}\sigma_b } \right] \nonumber \\
    % &\leq \mathbb{P}_{\mathbf{x}} \left[ \|\mathbf{x}\|_2  > \frac{c}{\eta(d+m)^{1.5}\nu_{\mathbf{w}}^2 } \right] \nonumber \\
    % &\leq  \mathbb{P}_{\mathbf{x}} \left[ \|\mathbf{x}\|_2  > c' d \right] \nonumber \\
    % &\leq  \exp\left( - \frac{d^2}{8}\right)
\end{align}
using $\nu_{\mathbf{w}} = O(d^{-1.25})$, $m=O(d)$ and $\eta = \Theta(1)$. Combining \eqref{38} with \eqref{56} and \eqref{shm} completes the proof.
\end{proof}
% \begin{align}  
% % &  \frac{1}{\lambda_{1}  } \mathbb{E}_{\mathbf{x},\mathbf{x}',i} \left[  f_{i}^*(\mathbf{x}) f_{i}^*(\mathbf{x}') \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz})\right] \nonumber \\
% \mathcal{L}(\mathbf{W}^0, \mathbf{b}^0, \{\mathbf{a}_{1,i} \}_{i\in \mathcal{T}})&=  \eta \mathbb{E}_{\mathbf{x},\mathbf{x}'} \Big[ \chi\{\sign(\mathbf{x}_{:r})  =  \sign(\mathbf{x}_{:r}') \}  \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz}) \Big] \nonumber \\
% &\quad +   \nonumber \\
% &= 
% % \chi\{\sign(\bar{\mathbf{x}}_{i,j'}) \neq  \sign(\mathbf{x}_{i,j}) \}y_{i,j} \bar{y}_{i,j'}\bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz})  \Big] \nonumber
% % \sum_{i=1}^T \frac{1}{n_1n_2}\sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}) 
% \end{align} 
% where $\bar{\sigma}()$ denotes the stop-gradient applied to the ReLU. 
% \begin{align}  
% &  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{i,\mathbf{x}_{i,j},\bar{\mathbf{x}}_{i,j'}}\left[ y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})\right] \nonumber \\
% &=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{i,\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[ y_{i,j} \bar{y}_{i,j'} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
% &=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}}  \left[\mathbb{E}_i \left[ y_{i,j}(\bar{\mathbf{x}}_{j'})  \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'}) \right] \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
% &=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}}  \left[\mathbb{E}_i \left[ 1 - 2\chi\{  y_{i,j}({\mathbf{x}}_{j}) \neq \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'})\} \right] \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
% &=  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[ \left( 1 - 2\mathbb{P}_i \left[ y_{i,j}({\mathbf{x}}_{j}) \neq \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'}) \right]\right) \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j})\right] \nonumber \\
% &=  -\frac{2^{-r}}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[  \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j}) | \sign(\bar{\mathbf{x}}_{i,j',:r})=\sign({\mathbf{x}}_{i,j,:r})   \right] \nonumber \\
% &\quad + \frac{2^{r} - 1}{2^{r}\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \mathbb{E}_{\mathbf{x}_{j},\bar{\mathbf{x}}_{j'}} \left[ \left( 1 - 2\mathbb{P}_i \left[ y_{i,j}({\mathbf{x}}_{j}) \neq \bar{y}_{i,j'}(\bar{\mathbf{x}}_{j'}) \right]\right) \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{j'})^\top \sigma(\mathbf{W}\mathbf{x}_{j}) | \sign(\bar{\mathbf{x}}_{i,j',:r})\neq \sign({\mathbf{x}}_{i,j,:r})   \right] \nonumber \\
% &= -\frac{2^{-r}}{\lambda_{1}} \mathbb{E}_{\mathbf{x},\bar{\mathbf{x}}} \left[  \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}})^\top \sigma(\mathbf{W}\mathbf{x}) | \sign(\bar{\mathbf{x}}_{:r})=\sign({\mathbf{x}}_{:r})   \right] \nonumber \\
% &\quad + \frac{2^{r} - 1}{2^{r}\lambda_{1} n_{1}n_{2} } \mathbb{E}_{\mathbf{x},\bar{\mathbf{x}}} \left[ \left( 1 - 2\mathbb{P}_i \left[ y_{i}({\mathbf{x}}) \neq \bar{y}_{i}(\bar{\mathbf{x}}) \right]\right) \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}})^\top \sigma(\mathbf{W}\mathbf{x}) | \sign(\bar{\mathbf{x}}_{:r})\neq \sign({\mathbf{x}}_{:r})   \right] \nonumber 
% \end{align} 

% \begin{align}
%     & \frac{2^{-r}}{\lambda_{1} n_{1}n_{2} }  \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1}  \mathbb{E}_{\bar{\mathbf{x}}_{i,j'},{\mathbf{x}}_{i,j}}\left[ \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j}) | \sign(\bar{\mathbf{x}}_{i,j',:r})=\sign({\mathbf{x}}_{i,j,:r})  \right] \nonumber \\
% &\quad +  \frac{1}{\lambda_{1} n_{1}n_{2} } \sum_{j=1}^{n_2}\sum_{j'=1}^{n_1} \int_{\mathbf{x}_{i,j},\bar{\mathbf{x}}_{i,j'}} \int_{i} \bar{\sigma}(\mathbf{W}\bar{\mathbf{x}}_{i,j'})^\top \sigma(\mathbf{W}\mathbf{x}_{i,j})  p(\mathbf{x}_{i,j},\bar{\mathbf{x}}_{i,j'}) 
% \end{align}

%ideas: 

% is infinite tasks the same as sampling a random pair of gaussians, then sampling the number of tasks for which they have the same label? yes but does not equal zero... yes because opposite pairs?


% Differentiating with respect to the neuron weight $\mathbf{w}$ leads to the following 
% \begin{align}
%    & \nabla_{\mathbf{w}_j}  \mathbb{E}_{\mathbf{x},\bar{\mathbf{x}}} \left[  \bar{\sigma}(\mathbf{WMz}')^\top \sigma(\mathbf{WMz}) | \sign({\mathbf{x}}_{:r}')=\sign({\mathbf{x}}_{:r})   \right]\nonumber \\
%    &=  \nabla_{\mathbf{w}_j}  \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[  \bar{\sigma}(\mathbf{w}_j^\top\mathbf{M}{\mathbf{x}}') \sigma(\mathbf{w}_j^\top \mathbf{x}) | \sign({\mathbf{x}}_{:r}')=\sign({\mathbf{x}}_{:r})   \right]  \nonumber \\
%     &=\mathbb{E}_{\mathbf{x},{\mathbf{x}}'} \left[  \mathbf{x} {\sigma}(\mathbf{w}_j^\top\mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}) | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})   \right]  \nonumber \\
%     &= \mathbf{M}\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[  \mathbf{x}(\mathbf{x}')^\top {\sigma}'(\mathbf{w}_j^\top  \mathbf{x}') \sigma'(\mathbf{w}_j^\top \mathbf{x}) | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})   \right] \mathbf{w}_j  \nonumber \\
%     % \mathbf{A} =  \begin{bmatrix}
%     %     \mathbf{A}_{.}
%     % \end{bmatrix}
% \end{align}
% Now, for ease of notation we drop the subscript $j$.
% Analyzing the matrix $\mathbf{A}(\mathbf{w}) \coloneqq \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[  \mathbf{x}(\mathbf{x}')^\top  {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x}) | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})   \right]$ is the key to the proof.
% We have 
% \begin{align}
%     \mathbf{A}(\mathbf{w}) = \begin{bmatrix}
% \mathbf{A}_{\parallel,\parallel}(\mathbf{w}) & \mathbf{A}_{\parallel,\perp}(\mathbf{w}) \\
% \mathbf{A}_{\perp,\parallel}(\mathbf{w}) & \mathbf{A}_{\perp,\perp}(\mathbf{w}) \\
%     \end{bmatrix}
% \end{align}
% where 
% \begin{align}
%     \mathbf{A}_{\parallel,\parallel}(\mathbf{w}) &= \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[  \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x}) | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})   \right] \nonumber \\
%     &= \mathbb{E}_{\mathbf{x}_{:r},\mathbf{x}_{:r}'} \left[  \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top 
%  \mathbb{E}_{\mathbf{x}_{r:},\bar{\mathbf{x}_{r:}}} \left[{\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x})\right] | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})   \right] \nonumber \\
% \end{align}






Next we control the matrices  $\mathbf{A}_{||,||}(\w)$, $\mathbf{A}_{||,\perp}(\w)$, $\mathbf{A}_{\perp,||}(\w)$, and $\mathbf{A}_{\perp,\perp}(\w)$. 

\begin{lemma}\label{lem:apara}
    % For all $j: \mathbf{w}_{j}^0\in \mathcal{G}_{\mathbf{w}}$, we have 
    For any $ \mathbf{w}\in \mathcal{G}_{\mathbf{w}}$, we have 
    \begin{align}
       \left\|\mathbf{A}_{\parallel,\parallel}(\mathbf{w}) - \tfrac{1}{4} \mathbf{I}_r\right\|_2 &\leq c \frac{ r^{3} + \log^3(m) }{d }
    \end{align}
    for an absolute constant $c$.
\end{lemma}

\begin{proof}
% We drop the neuron index subscript and time index superscript on $\mathbf{w}_{j}^0$ for ease of notation. 
Recall that $\mathbf{u}$ is drawn uniformly from $\{-1,1\}^r$.
From Lemma \ref{lem:compute_grad}, we have
\begin{align}
    &\mathbf{A}_{\parallel,\parallel}(\mathbf{w}) \nonumber \\
    &= \mathbb{E}_{\mathbf{u}} \left[ \mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[   {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x})  \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top |\sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})=\mathbf{u}\right] \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{u}} \left[
 \mathbb{E}_{\mathbf{x}_{:r},{\mathbf{x}_{:r}'}} \left[\mathbb{E}_{\mathbf{x}_{r:},{\mathbf{x}_{r:}'}} \left[{\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x})\right] \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top   | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r}) =\mathbf{u}\right] \right]  \nonumber \\
 &=  \mathbb{E}_{\mathbf{u}} \Big[ \mathbb{E}_{\mathbf{x}_{:r},{\mathbf{x}_{:r}'}} \Big[  \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top \mathbb{P}_{\mathbf{x}_{r:}} \left[\mathbf{w}_{r:}^\top  \mathbf{x}_{r:} > -\mathbf{w}_{:r}^\top  {\mathbf{x}}_{:r}  \right]   \nonumber \\
 &\quad \quad \quad \quad \quad  \times 
 \mathbb{P}_{{\mathbf{x}_{r:}}'} \left[ \mathbf{w}_{r:}^\top \mathbf{x}'_{r:} > -\mathbf{w}_{:r}^\top \mathbf{x}'_{:r}  \right] |\sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r}) =\mathbf{u}  \Big]\Big]  \nonumber \\
 &= \mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},{\mathbf{x}_{:r}'}} \Bigg[  \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top \left(\frac{1}{2} + \frac{1}{2}\erf\left(\frac{\mathbf{w}_{:r}^\top  {\mathbf{x}}_{:r} }{ \sqrt{2}\| {\mathbf{w}_{r:}} \|_2 } \right) \right) \nonumber \\
&\quad \quad \quad \quad \quad    \left(\frac{1}{2} + \frac{1}{2}\erf\left(\frac{\mathbf{w}^\top  \mathbf{x}'_{:r} }{\sqrt{2} \| {\mathbf{w}}_{r:} \|_2 } \right) \right) |\sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r}) =\mathbf{u}  \Bigg] \label{gu} \\
 &= \frac{1}{4}\mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},{\mathbf{x}_{:r}'}} \left[   \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top  |\sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r}) =\mathbf{u} \right] \nonumber \\
 &\quad + \frac{1}{2}\mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}_{:r}'} \left[  \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top 
\erf\left(\frac{\mathbf{w}_{:r}^\top{\mathbf{x}}_{:r} }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right) |\sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r}) =\mathbf{u} \right]  \nonumber \\
 &\quad + \frac{1}{4}\mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},{\mathbf{x}_{:r}'}} \left[   \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top 
 \erf\left(\frac{\mathbf{w}_{:r}^\top{\mathbf{x}}_{:r} }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right) \erf\left(\frac{\mathbf{w}_{:r}^\top\mathbf{x}'_{:r} }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right) |\sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r}) =\mathbf{u}  \right]  \label{apara3}
\end{align}
where \eqref{gu} follows using the Gaussian CDF.
For the first term in \eqref{apara3}, we can re-write $\mathbf{x}_{:r}$ conditioned on $\sign({\mathbf{x}}_{:r}) =\mathbf{u}$ as $\diag(\mathbf{u}) |\mathbf{x}_{:r}|$, where $|\cdot|$ denotes element-wise absolute value, to obtain
\begin{align}
     % &\frac{1}{4}\mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},{\mathbf{x}_{:r}'}} \left[ \chi\{ \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r}) =\mathbf{u}\}  \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top \right] \nonumber \\
     &\frac{1}{4}\mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},{\mathbf{x}_{:r}'}} \left[  \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r}) =\mathbf{u} \right]   \nonumber \\
     &=  \frac{1}{4}\mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},{\mathbf{x}_{:r}'}} \left[  \diag(\mathbf{u})|\mathbf{x}_{:r}||\mathbf{x}'_{:r}|^\top \diag(\mathbf{u}) \right]  \nonumber \\
     &=   \frac{1}{4}\mathbb{E}_{\mathbf{u}} \left[  \diag(\mathbf{u})\mathbb{E}_{\mathbf{x}_{:r},{\mathbf{x}_{:r}'}} \left[  |\mathbf{x}_{:r}||\mathbf{x}'_{:r}|^\top \right]\diag(\mathbf{u}) \right]    \nonumber \\
     &=  \frac{1}{4}\mathbb{E}_{\mathbf{u}} \left[  \diag(\mathbf{u})\left( \frac{2}{\pi} \mathbf{1}_r\mathbf{1}_{r}^\top + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_r  \right)\diag(\mathbf{u}) \right]       \nonumber \\
     &=  \frac{1}{4}\left( \frac{2}{\pi} \mathbb{E}_{\mathbf{u}} \left[  \mathbf{u}\mathbf{u}^\top  \right] + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_r \right)       \nonumber \\
     &= \frac{1}{4} \mathbf{I}_r      \label{dfc} 
\end{align}
% (diagonal element is average of product of aligned half-normals, off diagonals are averaged of non-aligned)
For the second term in \eqref{apara3}, we have
\begin{align}
     &\frac{1}{2}\mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}_{:r}'} \left[  \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top 
\erf\left(\frac{\mathbf{w}_{:r}^\top{\mathbf{x}}_{:r} }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right) | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})=\mathbf{u}   \right] \nonumber \\
&= \frac{1}{2}\mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}_{:r}'} \left[  \diag(\mathbf{u})|\mathbf{x}_{:r}||\mathbf{x}'_{:r}|^\top \diag(\mathbf{u}) 
\erf\left(\frac{\mathbf{w}_{:r}^\top \diag(\mathbf{u})|{\mathbf{x}}_{:r}| }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right)   \right]\label{jn} \\
&= \frac{1}{2}\mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}_{:r}'} \left[  \diag(-\mathbf{u})|\mathbf{x}_{:r}||\mathbf{x}'_{:r}|^\top \diag(-\mathbf{u}) 
\erf\left(\frac{\mathbf{w}_{:r}^\top \diag(-\mathbf{u})|{\mathbf{x}}_{:r}| }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right)   \right] \label{jj}\\
&= -\frac{1}{2}\mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}_{:r}'} \left[  \diag(\mathbf{u})|\mathbf{x}_{:r}||\mathbf{x}'_{:r}|^\top \diag(\mathbf{u}) 
\erf\left(\frac{\mathbf{w}_{:r}^\top \diag(\mathbf{u})|{\mathbf{x}}_{:r}| }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right)   \right] \label{nnj} \\
% &= \frac{1}{\sqrt{\pi}} \Bigg( \frac{1}{ \sqrt{2} \| {\mathbf{w}}_{r:} \|_2 } \mathbb{E}_{\mathbf{x}_{:r},\mathbf{x}'_{:r}}\left[  \mathbf{x}_{:r}{\mathbf{x}}_{:r}^\top \mathbf{w}_{:r} (\mathbf{x}'_{:r})^\top  | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})   \right]  \nonumber \\
% &\quad + \frac{1}{ 2 \sqrt{2} \| {\mathbf{w}}_{r:} \|_2^3 } \mathbb{E}_{\mathbf{x}_{:r},\mathbf{x}_{:r}'} \left[  ({\mathbf{x}}_{:r}^\top \mathbf{w}_{:r})^3\mathbf{x}_{:r} (\mathbf{x}'_{:r})^\top  | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})   \right]  + \dots \Bigg) \nonumber \\
% &=\frac{1}{{\pi}} \Bigg( \frac{1}{  \| {\mathbf{w}}_{r:} \|_2 } \mathbb{E}_{\mathbf{v},\mathbf{x}_{:r}} \left[  \mathbf{x}_{:r}{\mathbf{x}}_{:r}^\top \mathbf{w}_{:r} {\mathbf{v}}^\top  | \sign({\mathbf{x}}_{:r}) =\mathbf{v}   \right]  \nonumber \\
% &\quad + \frac{1}{ 2  \| {\mathbf{w}}_{r:} \|_2^3 } \mathbb{E}_{\mathbf{v},\mathbf{x}_{:r}} \left[  ({\mathbf{x}}_{:r}^\top \mathbf{w}_{:r})^3\mathbf{x}_{:r}  {\mathbf{v}}^\top  | \sign({\mathbf{x}}_{:r}) =\mathbf{v}   \right]  + \dots \Bigg) \nonumber \\
&= \mathbf{0} \label{lst}
\end{align}
where \eqref{jj} follows from the fact that $\mathbf{u}$ and $-\mathbf{u}$ have the same distribution, \eqref{nnj} follows since $\erf()$ is an odd function, and \eqref{lst} follows since $x=-x\iff x=0$.
% since each term always has an odd number of v/s (write z as abs(z)v

The final term in \eqref{apara3} is 
\begin{align}
&\mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}_{:r}'} \left[  \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top 
 \erf\left(\frac{\mathbf{w}_{:r}^\top{\mathbf{x}}_{:r} }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right) \erf\left(\frac{\mathbf{w}_{:r}^\top\mathbf{x}'_{:r} }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right)| \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})  =\mathbf{u} \right]  \nonumber \\
 % &= \mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}_{:r}'} \left[  \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top 
 % \erf\left(\frac{\mathbf{w}_{:r}^\top{\mathbf{x}}_{:r} }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right) \erf\left(\frac{\mathbf{w}_{:r}^\top\mathbf{x}'_{:r} }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right)| \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})  =\mathbf{u} \right]  \nonumber \\
 &= \mathbb{E}_{\mathbf{u}}
 % \sim \Unif(\mathcal{H}^{r})} 
 \Bigg[\mathbb{E}_{\mathbf{x}_{:r}} \left[  \mathbf{x}_{:r} 
 \erf\left(\frac{\mathbf{w}_{:r}^\top{\mathbf{x}}_{:r} }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right) \bigg| \sign({\mathbf{x}}_{:r})=\mathbf{u}\right] \nonumber \\
 &\quad \quad \times \mathbb{E}_{\mathbf{x}'_{:r}}\left[(\mathbf{x}'_{:r})^\top\erf\left(\frac{\mathbf{w}_{:r}^\top\mathbf{x}'_{:r} }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right)\bigg| \sign(\mathbf{x}'_{:r})=\mathbf{u}\right] \Bigg] \label{46}
\end{align}
% where $\mathcal{H}^{r} = \{-1,1\}^r$ is the $r$-dimensional Rademacher hypercube. 
Again to remove the conditioning, we can equivalently write $\mathbb{E}_{\mathbf{x}_{:r}} \left[  \mathbf{x}_{:r} 
 \erf\left(\frac{\mathbf{w}_{:r}^\top{\mathbf{x}}_{:r} }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right) \bigg| \sign({\mathbf{x}}_{:r})=\mathbf{u}\right]$ as 
 \begin{align}
     \mathbb{E}_{\mathbf{x}_{:r}} \left[  \mathbf{x}_{:r} 
 \erf\left(\frac{\mathbf{w}_{:r}^\top{\mathbf{x}}_{:r} }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right) \bigg| \sign({\mathbf{x}}_{:r})=\mathbf{u}\right] 
 &= \mathbb{E}_{\mathbf{x}_{:r}} \left[ \text{diag}(\mathbf{u}) |\mathbf{x}_{:r} |
 \erf\left(\frac{\mathbf{w}_{:r}^\top  \text{diag}(\mathbf{u}) | {\mathbf{x}}_{:r}| }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right) \right] 
 \end{align}
where $| {\mathbf{x}}_{:r}| \in \mathbb{R}^r$ denotes the element-wise absolute value of $\mathbf{x}_{:r}$. For all $\mathbf{u}\in \{-1,1\}^r$, we have 
\begin{align}
   & \left\|\mathbb{E}_{\mathbf{x}_{:r}} \left[ \text{diag}(\mathbf{u}) |\mathbf{x}_{:r} |
 \erf\left(\frac{\mathbf{w}_{:r}^\top  \text{diag}(\mathbf{u}) | {\mathbf{x}}_{:r}| }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right) \right] \right\|_2 \nonumber \\
    &\leq  \mathbb{E}_{\mathbf{x}_{:r}} \left[\left\| \text{diag}(\mathbf{u}) |\mathbf{x}_{:r} |
 \erf\left(\frac{\mathbf{w}_{:r}^\top  \text{diag}(\mathbf{u}) | {\mathbf{x}}_{:r}| }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right) \right\|_2 \right]  \nonumber \\
 &\leq \mathbb{E}_{\mathbf{x}_{:r}} \left[\left\| \text{diag}(\mathbf{u}) |\mathbf{x}_{:r} |\right\|_2
\left|\erf\left(\frac{\mathbf{w}_{:r}^\top  \text{diag}(\mathbf{u}) | {\mathbf{x}}_{:r}| }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right) \right|\right]  \nonumber \\
 &\leq \mathbb{E}_{\mathbf{x}_{:r}} \left[\left\| \text{diag}(\mathbf{u}) |\mathbf{x}_{:r} |\right\|_2
\left|\frac{\mathbf{w}_{:r}^\top  \text{diag}(\mathbf{u}) | {\mathbf{x}}_{:r}| }{ \| {\mathbf{w}}_{r:} \|_2 } \right|\right]  \label{jhj} \\
 &\leq \left\|\text{diag}(\mathbf{u})\right\|_2  \mathbb{E}_{\mathbf{x}_{:r}} \left[ \|\mathbf{x}_{:r}\|_2^2\right]
\frac{\|\mathbf{w}_{:r}^\top  \text{diag}(\mathbf{u}) \|_2 }{ \| {\mathbf{w}}_{r:} \|_2 }  \nonumber \\
% &\leq  \nonumber \\
 &\leq \frac{c r (\sqrt{r} +\sqrt{\log(m)}) }{\sqrt{d} } \label{wb}
\end{align}
for an absolute constant $c$, where \eqref{jhj} follows since $|\erf(x)|\leq \sqrt{2}|x| $, and \eqref{wb} follows
since $\mathbf{w}\in \mathcal{G}_{\mathbf{w}}$ and $m=O(d)$, thus $\| {\mathbf{w}}_{r:} \|_2 = \Omega(\sqrt{d})$.
Therefore, using \eqref{46},
\begin{align}
    &\left\|\mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}_{:r}'} \left[  \mathbf{x}_{:r}(\mathbf{x}'_{:r})^\top 
 \erf\left(\frac{\mathbf{w}_{:r}^\top{\mathbf{x}}_{:r} }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right) \erf\left(\frac{\mathbf{w}_{:r}^\top\mathbf{x}'_{:r} }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right)| \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})  =\mathbf{u} \right]  \right\|_2 \nonumber \\
 &\leq \frac{c' r^{3} + c'\log^3(m) }{d }
\end{align}
completing the proof.
\end{proof}
\begin{comment}
Next we use the Taylor series of $\text{erf}(\cdot)$ around zero to write
\begin{align}
    &\mathbb{E}_{\mathbf{x}_{:r}} \left[ \text{diag}(\mathbf{u}) |\mathbf{x}_{:r} |
 \erf\left(\frac{\mathbf{w}_{:r}^\top  \text{diag}(\mathbf{u}) | {\mathbf{x}}_{:r}| }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 } \right) \right] \nonumber \\
 &= \frac{2}{\sqrt{\pi}} \mathbb{E}_{\mathbf{x}_{:r}} \left[ \text{diag}(\mathbf{u}) |\mathbf{x}_{:r} |
 \left(\frac{\mathbf{w}_{:r}^\top  \text{diag}(\mathbf{u}) | {\mathbf{x}}_{:r}| }{ \sqrt{2}\| {\mathbf{w}}_{r:} \|_2 }  - \frac{(\mathbf{w}_{:r}^\top  \text{diag}(\mathbf{u}) | {\mathbf{x}}_{:r}|)^3 }{ 6\sqrt{2} \| {\mathbf{w}}_{r:} \|_2^3 }  + \frac{(\mathbf{w}_{:r}^\top  \text{diag}(\mathbf{u}) | {\mathbf{x}}_{:r}|)^5 }{ 40 \| {\mathbf{w}}_{r:} \|_2^5 } +\dots \right) \right] \nonumber \\
 &=  \frac{\sqrt{2}}{\sqrt{\pi}\| {\mathbf{w}}_{r:} \|_2 }\text{diag}(\mathbf{u})  \mathbb{E}_{\mathbf{x}_{:r}} \left[ |\mathbf{x}_{:r} |  | {\mathbf{x}}_{:r}|^\top \right] \text{diag}(\mathbf{u}) \mathbf{w}_{:r} + \mathbf{E}_1 
  % - \frac{1}{ 6 \| {\mathbf{w}}_{r:} \|_2^3 } \mathbb{E}_{\mathbf{x}_{:r}}\left[   \text{diag}(\mathbf{v}) | {\mathbf{x}}_{:r}| (\mathbf{w}_{:r}^\top  \text{diag}(\mathbf{v}) | {\mathbf{x}}_{:r}|)^3 \right]   +\dots \right) 
  \nonumber 
\end{align}
where $\|\mathbf{E}_1\|_2=O\left({(d-r)^{-1.5}}\right) $. This follows since $\mathbf{w}\in \mathcal{G}_{\mathbf{w}}$, thus $\| {\mathbf{w}}_{r:} \|_2 = \Omega(\sqrt{d-r})$, and 
\begin{align}
\|    \mathbb{E}_{\mathbf{x}_{:r}} \left[ \text{diag}(\mathbf{u}) |\mathbf{x}_{:r} |
 \left( - \frac{(\mathbf{w}_{:r}^\top  \text{diag}(\mathbf{u}) | {\mathbf{x}}_{:r}|)^3 }{ 6\sqrt{2} \| {\mathbf{w}}_{r:} \|_2^3 }  + \frac{(\mathbf{w}_{:r}^\top  \text{diag}(\mathbf{u}) | {\mathbf{x}}_{:r}|)^5 }{ 40 \| {\mathbf{w}}_{r:} \|_2^5 } +\dots \right) \right] \|_2 \nonumber \\
 &\leq c
\end{align}
for an absolute constant $c$. 
\end{comment}

% with probability at least $1-$ since $\| {\mathbf{w}}_{r:} \|_2 = \Omega(\sqrt{d-r})$ with probability at least $1-$. 

% For the first term, we note that each element of $|\mathbf{x}_{:r} | $ is an i.i.d. half-normal random variable, and thus obtain
% \begin{align}
%     &\frac{\sqrt{2}}{\sqrt{\pi}\| {\mathbf{w}}_{r:} \|_2 }\text{diag}(\mathbf{v})  \mathbb{E}_{\mathbf{x}_{:r}} \left[ |\mathbf{x}_{:r} |  | {\mathbf{x}}_{:r}|^\top \right] \text{diag}(\mathbf{v}) \mathbf{w}_{:r}\nonumber \\
%     &= \frac{\sqrt{2}}{\sqrt{\pi}\| {\mathbf{w}}_{r:} \|_2 } \left( \frac{2}{\pi} \mathbf{v}\mathbf{v}^\top + \left( 1  - \frac{2}{\pi}\right)\mathbf{I}_r \right)\mathbf{w}_{:r}
% \end{align}






\begin{lemma} \label{lem:aperp}
    For any $\mathbf{w}\in \mathcal{G}_{\mathbf{w}}$, we have 
    \begin{align}
        \left\|\mathbf{A}_{\perp,\perp}(\mathbf{w}) - \left(1 - \frac{\|\mathbf{w}_{:r}\|_2^2}{\|\mathbf{w}_{r:}\|_2^2} \right) \frac{\mathbf{w}_{r:} \mathbf{w}_{r:}^\top }{2\pi \|\mathbf{w}_{r:}\|_2^2} \right\|_2 &\leq c\frac{r^4 + \log^4(m)}{d^2}
    \end{align}
    for an absolute constant $c$.
\end{lemma}


\begin{proof}
% \begin{align}
%     \mathbf{W} &= \mathbf{W}
% \end{align}
% Next we analyze $\mathbf{A}_{\perp,\perp}(\mathbf{w}_{})$.
% Again we drop the subscript and superscript on $\mathbf{w}_j^0$ for ease of notation.
We have
\begin{align}
    \mathbf{A}_{\perp,\perp}(\mathbf{w}) &=  \mathbb{E}_{\mathbf{u}} \left[\mathbb{E}_{\mathbf{x},\mathbf{x}'} \left[  \mathbf{x}_{r:}(\mathbf{x}'_{r:})^\top {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x}) | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r}) =\mathbf{u}  \right]\right] \nonumber \\
    &= \mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}'_{:r}} \left[ \mathbb{E}_{\mathbf{x}_{r:},\mathbf{x}'_{r:}} \left[ \mathbf{x}_{r:}(\mathbf{x}'_{r:})^\top {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x}) \right] | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})=\mathbf{u}  \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}'_{:r}} \left[ \mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} \sigma'(\mathbf{w}^\top \mathbf{x})  \right] \mathbb{E}_{\mathbf{x}'_{r:}} \left[(\mathbf{x}'_{r:})^\top {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \right] | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r}) =\mathbf{u} \right] \label{cb}  
   %  \\
   % &=  \mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}'_{:r}} \left[ \mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} \sigma'(\mathbf{w}^\top \mathbf{x})  \right] \mathbb{E}_{\mathbf{x}'_{r:}} \left[(\mathbf{x}'_{r:})^\top {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \right] | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r}) =\mathbf{u} \right] \nonumber
\end{align}
Next, 
% let $b= \mathbf{w}_{r:}^\top\mathbf{x}_{r:}$. 
% For any $\mathbf{z}\sim \mathcal{N}(\mathbf{0}_r,\mathbf{I}_r)$ and fixed $\mathbf{q}\in\mathbb{R}^r$, $\mathbb{E}_{\mathbf{z}}[\mathbf{z}\chi\{\mathbf{q}^\top\mathbf{z} + b>0\}] = \mathbb{E}_{\mathbf{z}}[\mathbf{z}\chi\{\mathbf{q}^\top\mathbf{z} + b>0\}] $ 
we have 
\begin{align}
    \mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} \sigma'(\mathbf{w}^\top \mathbf{x})  \right] &= \mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} \sigma'(\mathbf{w}_{:r}^\top\mathbf{x}_{:r} + \mathbf{w}_{r:}^\top\mathbf{x}_{r:})  \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} |\mathbf{w}_{:r}^\top\mathbf{x}_{:r} + \mathbf{w}_{r:}^\top\mathbf{x}_{r:} > 0 \right] \mathbb{P}_{\mathbf{x}_{r:}}[\mathbf{w}_{:r}^\top\mathbf{x}_{:r} + \mathbf{w}_{r:}^\top\mathbf{x}_{r:} > 0] \nonumber \\
    &= \mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} \bigg|\mathbf{w}_{:r}^\top\mathbf{x}_{:r} > | \mathbf{w}_{r:}^\top\mathbf{x}_{r:} |\right] \mathbb{P}_{\mathbf{x}_{r:}}[\mathbf{w}_{:r}^\top\mathbf{x}_{:r} >| \mathbf{w}_{r:}^\top\mathbf{x}_{r:}| ] \label{bh} 
\end{align}
where the last line follows since if $\mathbf{w}_{r:}^\top\mathbf{x}_{r:} <0$, then $ - \mathbf{w}_{r:}^\top\mathbf{x}_{r:} = |\mathbf{w}_{r:}^\top\mathbf{x}_{r:}|$ so $\mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} |\mathbf{w}_{:r}^\top\mathbf{x}_{:r} + \mathbf{w}_{r:}^\top\mathbf{x}_{r:} > 0 \right]= \mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} \bigg|\mathbf{w}_{:r}^\top\mathbf{x}_{:r} > | \mathbf{w}_{r:}^\top\mathbf{x}_{r:} |\right]$ and $\mathbb{P}_{\mathbf{x}_{r:}}[\mathbf{w}_{:r}^\top\mathbf{x}_{:r} + \mathbf{w}_{r:}^\top\mathbf{x}_{r:} > 0]=\mathbb{P}_{\mathbf{x}_{r:}}[\mathbf{w}_{:r}^\top\mathbf{x}_{:r} >| \mathbf{w}_{r:}^\top\mathbf{x}_{r:}| ]$, and if $\mathbf{w}_{r:}^\top\mathbf{x}_{r:} >0$, then by the law of total expectation,
\begin{align}
   &\mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} |\mathbf{w}_{:r}^\top\mathbf{x}_{:r} + \mathbf{w}_{r:}^\top\mathbf{x}_{r:} > 0 \right] \nonumber \\
   &= \mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} |\mathbf{w}_{:r}^\top\mathbf{x}_{:r} > \mathbf{w}_{r:}^\top\mathbf{x}_{r:}  \right] \mathbb{P}_{\mathbf{x}_{r:}} \left[ \mathbf{w}_{:r}^\top\mathbf{x}_{:r} > \mathbf{w}_{r:}^\top\mathbf{x}_{r:}  |\mathbf{w}_{:r}^\top\mathbf{x}_{:r} > -\mathbf{w}_{r:}^\top\mathbf{x}_{r:} \right] \nonumber \\
   &\quad + \mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} |\mathbf{w}_{r:}^\top\mathbf{x}_{r:}> \mathbf{w}_{:r}^\top\mathbf{x}_{:r} > -\mathbf{w}_{r:}^\top\mathbf{x}_{r:}  \right] \nonumber \\
   &\quad \quad \quad \quad \times \mathbb{P}_{\mathbf{x}_{r:}} \left[ \mathbf{w}_{r:}^\top\mathbf{x}_{r:}> \mathbf{w}_{:r}^\top\mathbf{x}_{:r} > -\mathbf{w}_{r:}^\top\mathbf{x}_{r:}  |\mathbf{w}_{:r}^\top\mathbf{x}_{:r} > -\mathbf{w}_{r:}^\top\mathbf{x}_{r:} \right]  \nonumber \\
   &= \mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} |\mathbf{w}_{:r}^\top\mathbf{x}_{:r} > \mathbf{w}_{r:}^\top\mathbf{x}_{r:}  \right] \mathbb{P}_{\mathbf{x}_{r:}} \left[ \mathbf{w}_{:r}^\top\mathbf{x}_{:r} > \mathbf{w}_{r:}^\top\mathbf{x}_{r:}  |\mathbf{w}_{:r}^\top\mathbf{x}_{:r} > -\mathbf{w}_{r:}^\top\mathbf{x}_{r:} \right] \nonumber  \\
   &= \mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} |\mathbf{w}_{:r}^\top\mathbf{x}_{:r} > |\mathbf{w}_{r:}^\top\mathbf{x}_{r:}|  \right] \mathbb{P}_{\mathbf{x}_{r:}} \left[ \mathbf{w}_{:r}^\top\mathbf{x}_{:r} > \mathbf{w}_{r:}^\top\mathbf{x}_{r:}  |\mathbf{w}_{:r}^\top\mathbf{x}_{:r} > -\mathbf{w}_{r:}^\top\mathbf{x}_{r:} \right] \label{bnv}  \\
   &= \mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} |\mathbf{w}_{:r}^\top\mathbf{x}_{:r} > |\mathbf{w}_{r:}^\top\mathbf{x}_{r:}|  \right]\frac{ \mathbb{P}_{\mathbf{x}_{r:}} \left[ \mathbf{w}_{:r}^\top\mathbf{x}_{:r} > |\mathbf{w}_{r:}^\top\mathbf{x}_{r:}|\right] }{ \mathbb{P}_{\mathbf{x}_{r:}} \left[\mathbf{w}_{:r}^\top\mathbf{x}_{:r} > -\mathbf{w}_{r:}^\top\mathbf{x}_{r:} \right]}  \nonumber
\end{align}
where \eqref{bnv} follows since $\mathbf{w}_{r:}^\top\mathbf{x}_{r:} = |\mathbf{w}_{r:}^\top\mathbf{x}_{r:}| $. 
Now we return to \eqref{bh}. 

Note that
$$\mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} \bigg|\mathbf{w}_{:r}^\top\mathbf{x}_{:r} > | \mathbf{w}_{r:}^\top\mathbf{x}_{r:} |\right]=\mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} - 2 \sigma\left( -\frac{\mathbf{w}_{r:}^\top  }{ \| \mathbf{w}_{r:} \|_2}\mathbf{x}_{r:}\right)\frac{\mathbf{w}_{r:} }{ \| \mathbf{w}_{r:} \|_2} \bigg||\mathbf{w}_{:r}^\top\mathbf{x}_{:r}| > | \mathbf{w}_{r:}^\top\mathbf{x}_{r:} |\right] $$ by the symmetry of the Gaussian distribution (and the fact that $$\mathbf{x}_{r:} - 2 \sigma\left( -\frac{\mathbf{w}_{r:}^\top  }{ \| \mathbf{w}_{r:} \|_2}\mathbf{x}_{r:}\right)\frac{\mathbf{w}_{r:} }{ \| \mathbf{w}_{r:} \|_2} $$ is the flip of $\mathbf{x}_{r:}$ across the hyperplane with normal vector $\frac{\mathbf{w}_{r:}^\top  }{ \| \mathbf{w}_{r:} \|_2}$ when $\mathbf{w}_{r:}^\top \mathbf{x}_{r:} < - | \mathbf{w}_{r:}^\top\mathbf{x}_{r:} |$.
Using this, we obtain
\begin{align}
    &\mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} \sigma'(\mathbf{w}^\top \mathbf{x})  \right]\nonumber \\
    % &=  \mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} \bigg|\mathbf{w}_{:r}^\top\mathbf{x}_{:r} > | \mathbf{w}_{r:}^\top\mathbf{x}_{r:} |\right] \mathbb{P}_{\mathbf{x}_{r:}}[\mathbf{w}_{:r}^\top\mathbf{x}_{:r} >| \mathbf{w}_{r:}^\top\mathbf{x}_{r:}| ] \nonumber \\
    &= \mathbb{E}_{\mathbf{x}_{r:}} \left[ \mathbf{x}_{r:} - 2  \sigma\left( -\frac{\mathbf{w}_{r:}^\top  }{ \| \mathbf{w}_{r:} \|_2}\mathbf{x}_{r:}\right)\frac{\mathbf{w}_{r:} }{ \| \mathbf{w}_{r:} \|_2} \bigg| |\mathbf{w}_{r:}^\top\mathbf{x}_{r:}|  > |\mathbf{w}_{:r}^\top\mathbf{x}_{:r}| \right] \mathbb{P}_{\mathbf{x}_{r:}}\left[\mathbf{w}_{r:}^\top\mathbf{x}_{r:} > |\mathbf{w}_{:r}^\top\mathbf{x}_{:r}| \right]\nonumber \\
    % &\quad \quad \times  \nonumber \\
    &= 2\mathbb{E}_{\mathbf{x}_{r:}} \left[ \sigma\left( -\frac{\mathbf{w}_{r:}^\top \mathbf{x}_{r:} }{ \| \mathbf{w}_{r:} \|_2}\right)\bigg| |\mathbf{w}_{r:}^\top\mathbf{x}_{r:} | > |\mathbf{w}_{:r}^\top\mathbf{x}_{:r}| \right]  \mathbb{P}_{\mathbf{x}_{r:}}\left[\mathbf{w}_{r:}^\top\mathbf{x}_{r:} > |\mathbf{w}_{:r}^\top\mathbf{x}_{:r}| \right] \frac{\mathbf{w}_{r:} }{ \| \mathbf{w}_{r:} \|_2}  \nonumber \\
    &=\mathbb{E}_{\mathbf{x}_{r:}} \left[ \sigma\left( -\frac{\mathbf{w}_{r:}^\top \mathbf{x}_{r:} }{ \| \mathbf{w}_{r:} \|_2}\right)\bigg| \mathbf{w}_{r:}^\top\mathbf{x}_{r:}  < - |\mathbf{w}_{:r}^\top\mathbf{x}_{:r}| \right]  \mathbb{P}_{\mathbf{x}_{r:}}\left[\mathbf{w}_{r:}^\top\mathbf{x}_{r:} > |\mathbf{w}_{:r}^\top\mathbf{x}_{:r}| \right] \frac{\mathbf{w}_{r:} }{ \| \mathbf{w}_{r:} \|_2}  \nonumber \\
    % &\quad \quad \times \mathbb{P}_{\mathbf{x}_{r:}}\left[\mathbf{w}_{r:}^\top\mathbf{x}_{r:} > |\mathbf{w}_{:r}^\top\mathbf{x}_{:r}| \right] \nonumber \\
    &= \frac{\frac{1}{\sqrt{2\pi}} \exp(-(\mathbf{w}_{:r}^\top\mathbf{x}_{:r})^2/2 ) }{\mathbb{P}_{\mathbf{x}_{r:}}\left[\mathbf{w}_{r:}^\top\mathbf{x}_{r:} <- |\mathbf{w}_{:r}^\top\mathbf{x}_{:r}| \right]} \mathbb{P}_{\mathbf{x}_{r:}}\left[\mathbf{w}_{r:}^\top\mathbf{x}_{r:} > |\mathbf{w}_{:r}^\top\mathbf{x}_{:r}| \right] \frac{\mathbf{w}_{r:} }{ \| \mathbf{w}_{r:} \|_2}  \label{ddw} \\
    &= {\frac{1}{\sqrt{2\pi}} \exp(-(\mathbf{w}_{:r}^\top\mathbf{x}_{:r})^2/2 ) }\frac{\mathbf{w}_{r:} }{ \| \mathbf{w}_{r:} \|_2}  \label{mn}
\end{align}
where \eqref{ddw} follows by the definition of the inverse Mills ratio.
Repeating the same argument for $\mathbf{x}_{r:}'$ and using \eqref{cb} yields 
\begin{align}
   \mathbf{A}_{\perp,\perp}(\mathbf{w})   &=  \mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}'_{:r}} \left[ \exp\left( -\frac{(\mathbf{x}_{:r}^\top\mathbf{w}_{:r})^2+ ((\mathbf{x}'_{:r})^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)    \bigg| \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r}) =\mathbf{u} \right] \nonumber \\
    &\quad \times \frac{1}{2\pi \|\mathbf{w}_{r:}\|_2^2}\mathbf{w}_{r:} \mathbf{w}_{r:}^\top   \label{where}
\end{align}
We analyze the scalar term in the top line. We have
\begin{align}
&\mathbb{E}_{\mathbf{u}} \left[\mathbb{E}_{\mathbf{x}_{:r},\mathbf{x}'_{:r}} \left[ \exp\left( -\frac{(\mathbf{x}_{:r}^\top\mathbf{w}_{:r})^2+ ((\mathbf{x}'_{:r})^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)    \bigg| \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r}) =\mathbf{u} \right]\right] \nonumber \\
    % &= %2^{-r} \sum_{\mathbf{v}\in \mathcal{H}^r} 
    % \mathbb{E}_{\mathbf{u}} \left[\mathbb{E}_{\mathbf{x}_{:r},\mathbf{x}'_{:r}} \left[ \exp\left( -\frac{(\mathbf{x}_{:r}^\top\mathbf{w}_{:r})^2+ ((\mathbf{x}'_{:r})^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)    \bigg| \sign(\mathbf{x}'_{:r})= \mathbf{u}, \sign({\mathbf{x}}_{:r}) = \mathbf{u}  \right]\right] \nonumber \\
    &= %2^{-r} \sum_{\mathbf{v}\in \mathcal{H}^r} 
    \mathbb{E}_{\mathbf{u}}\Bigg[ \mathbb{E}_{\mathbf{x}_{:r}} \left[ \exp\left( -\frac{(\mathbf{x}_{:r}^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)    \bigg| \sign({\mathbf{x}}_{:r}) = \mathbf{u}  \right] \nonumber \\
    &\quad \quad \times \mathbb{E}_{\mathbf{x}'_{:r}} \left[ \exp\left( -\frac{((\mathbf{x}'_{:r})^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)    \bigg| \sign(\mathbf{x}'_{:r})= \mathbf{u} \right]\Bigg] \nonumber \\
    &= %2^{-r} \sum_{\mathbf{v}\in \mathcal{H}^r} 
    \mathbb{E}_{\mathbf{u}} \left[ \mathbb{E}_{\mathbf{x}_{:r}} \left[ \exp\left( -\frac{(\mathbf{x}_{:r}^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)    \bigg| \sign({\mathbf{x}}_{:r}) = \mathbf{u}  \right]^2 \right] \label{f}
    % &\leq \left( 2^{-r} \sum_{\mathbf{v}\in \mathcal{H}^r} \mathbb{E}_{\mathbf{x}_{:r}} \left[ \exp\left( -\frac{(\mathbf{x}_{:r}^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)    \bigg| \sign({\mathbf{x}}_{:r}) = \mathbf{v}  \right] \right)^2 \nonumber \\
    % &=  \mathbb{E}_{\mathbf{x}_{:r}} \left[ \exp\left( -\frac{(\mathbf{x}_{:r}^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)   \right] ^2 \nonumber \\
    % &= \frac{ \| \mathbf{w}_{r:} \|_2^2  }{\| \mathbf{w} \|_2^2 }
\end{align}
where, using the Taylor expansion of $\exp({-x^2})$ and  re-writing $\mathbf{x}_{:r}$ conditioned on $\sign({\mathbf{x}}_{:r}) =\mathbf{u}$ as $\diag(\mathbf{u}) |\mathbf{x}_{:r}|$,
\begin{align}
    &\mathbb{E}_{\mathbf{x}_{:r}} \left[ \exp\left( -\frac{(\mathbf{x}_{:r}^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)    \bigg| \sign({\mathbf{x}}_{:r}) = \mathbf{u}  \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{x}_{:r}} \left[ \exp\left( -\frac{(|\mathbf{x}_{:r}|^\top \text{diag}(\mathbf{u}) \mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)    \right] \nonumber \\
    &= 1 - \frac{1}{2\|\mathbf{w}_{r:}\|_2^2} \mathbb{E}_{\mathbf{x}_{:r}} \left[(|\mathbf{x}_{:r}|^\top \diag(\mathbf{u}) \mathbf{w}_{:r})^2\right]  + O\left( \frac{r^4 + \log^4(m)}{ d^2} \right) \label{fb}
    % + \frac{1}{\|\mathbf{w}_{r:}\|_2^4} \mathbb{E}_{\mathbf{x}_{:r}} \left[(|\mathbf{x}_{:r}|^\top \diag(\mathbf{v}) \mathbf{w}_{:r})^4\right]  + O( (d-r)^{-3} ).
\end{align}
where \eqref{fb} follows since  $\|\mathbf{w}_{r:}\|_2^2 = \Omega( (\sqrt{d} - \sqrt{\log(m)})^4) = \Omega(d^2)$ and $\mathbb{E}_{\mathbf{x}_{:r}}[ (|\mathbf{x}_{:r}|^\top \text{diag}(\mathbf{u}) \mathbf{w}_{:r})^4 ]\leq \mathbb{E}_{\mathbf{x}_{:r}}[ \|\mathbf{x}_{:r}\|_2^4 ]\|\mathbf{w}_{:r}\|_2^4 = O(r^4 + \log^4(m))$ since $\mathbf{w}\in \mathcal{G}_{\mathbf{w}}$. To compute the second term in \eqref{fb}, note that
\begin{align}
    \mathbb{E}_{\mathbf{x}_{:r}} \left[(|\mathbf{x}_{:r}|^\top \text{diag}(\mathbf{u}) \mathbf{w}_{:r})^2\right]  &=   \mathbf{w}_{:r}^\top \text{diag}(\mathbf{u})\mathbb{E}_{\mathbf{x}_{:r}}  \left[|\mathbf{x}_{:r}||\mathbf{x}_{:r}|^\top \right]\text{diag}(\mathbf{u}) \mathbf{w}_{:r} \nonumber \\
    &= \mathbf{w}_{:r}^\top \text{diag}(\mathbf{u})\left(\frac{2}{\pi}\mathbf{1}_{d-r}\mathbf{1}_{d-r}^\top + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_{d-r}\right)\text{diag}(\mathbf{u}) \mathbf{w}_{:r} \nonumber \\               
    &=  \mathbf{w}_{:r}^\top \left(\frac{2}{\pi}\mathbf{uu}^\top + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_{d-r}\right)\mathbf{w}_{:r} \nonumber 
\end{align}
therefore
\begin{align}
   &\mathbb{E}_{\mathbf{u}} \left[ \mathbb{E}_{\mathbf{x}_{:r}} \left[ \exp\left( -\frac{(\mathbf{x}_{:r}^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)    \bigg| \sign({\mathbf{x}}_{:r}) = \mathbf{u}  \right]^2 \right] \nonumber \\
   &= \mathbb{E}_{\mathbf{u}} \left[\left( 1 -  \frac{1}{2\|\mathbf{w}_{r:}\|_2^2}\mathbf{w}_{:r}^\top \left(\frac{2}{\pi}\mathbf{uu}^\top + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_{d-r}\right)\mathbf{w}_{:r} + O\left( \frac{r^4 + \log^4(m)}{ d^{2}} \right) \right)^2 \right] \nonumber \\
   &= 1 -  \frac{1}{\|\mathbf{w}_{r:}\|_2^2}\mathbf{w}_{:r}^\top \left(\frac{2}{\pi}\mathbb{E}_{\mathbf{u}}[\mathbf{uu}^\top] + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_{d-r}\right)\mathbf{w}_{:r} \nonumber \\
   &\quad + \frac{1}{4\|\mathbf{w}_{r:}\|_2^4}\mathbf{w}_{:r}^\top \mathbb{E}_{\mathbf{u}}\left[ \left(\frac{2}{\pi}\mathbf{uu}^\top + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_{d-r}\right)\mathbf{w}_{:r}\mathbf{w}_{:r}^\top \left(\frac{2}{\pi}\mathbf{uu}^\top + \left(1 - \frac{2}{\pi}\right)\mathbf{I}_{d-r}\right)\right] \mathbf{w}_{:r} \nonumber \\
   &\quad +  O\left(\frac{r^4 + \log^4(m)}{ d^{2}} \right) \nonumber \\
   &=  1 -  \frac{\|\mathbf{w}_{:r}\|_2^2}{\|\mathbf{w}_{r:}\|_2^2} + \frac{\left((1- \frac{2}{\pi})^2 + \frac{4}{\pi}\left(1 - \frac{2}{\pi}\right) \right)\|\mathbf{w}_{r:}\|_2^4     }{4\|\mathbf{w}_{r:}\|_2^4} \nonumber \\
   &\quad  + \frac{4}{\pi^2}
   \mathbf{w}_{:r}^\top \mathbb{E}_{\mathbf{u}}\left[ \mathbf{uu}^\top \mathbf{w}_{:r} \mathbf{w}_{:r}^\top  \mathbf{uu}^\top \right] \mathbf{w}_{:r}  +  O\left(\frac{r^4 + \log^4(m)}{ d^{2}}  \right) \nonumber \\
   &=  1 -  \frac{\|\mathbf{w}_{:r}\|_2^2}{\|\mathbf{w}_{r:}\|_2^2} + \frac{\left((1- \frac{2}{\pi})^2 + \frac{4}{\pi}\left(1 - \frac{2}{\pi}\right) \right)\|\mathbf{w}_{r:}\|_2^4     }{4\|\mathbf{w}_{r:}\|_2^4}  \nonumber \\
   &\quad + \frac{1}{\pi^2 \|\mathbf{w}_{r:}\|_2^4 } 
   \mathbf{w}_{:r}^\top \mathbb{E}_{\mathbf{u}}\left[ \mathbf{uu}^\top (\mathbf{u}^\top\mathbf{w}_{:r})^2 \right] \mathbf{w}_{:r}  +  O\left(\frac{r^4 + \log^4(m)}{ d^{2}} \right) \nonumber \\
   &=  1 -  \frac{\|\mathbf{w}_{:r}\|_2^2}{\|\mathbf{w}_{r:}\|_2^2} + \frac{\left((1- \frac{2}{\pi})^2 + \frac{4}{\pi}\left(1 - \frac{2}{\pi}\right) \right)\|\mathbf{w}_{r:}\|_2^4     }{4\|\mathbf{w}_{r:}\|_2^4}  \nonumber \\
   &\quad + \frac{1}{\pi^2 \|\mathbf{w}_{r:}\|_2^4 } 
   \mathbf{w}_{:r}^\top \left( \|\mathbf{w}_{:r}\|_2^2\mathbf{I}_r + 2 \mathbf{w}_{:r}\mathbf{w}_{:r}^\top - \diag( \mathbf{w}_{:r} )^2 \right) \mathbf{w}_{:r}  +  O\left(\frac{r^4 + \log^4(m)}{ d^{2}} \right) \nonumber \\
   &= 1 -  \frac{\|\mathbf{w}_{:r}\|_2^2}{\|\mathbf{w}_{r:}\|_2^2} + \frac{\left((1- \frac{2}{\pi})^2 + \frac{4}{\pi}\left(1 - \frac{2}{\pi}\right) \right)\|\mathbf{w}_{r:}\|_2^4     }{4\|\mathbf{w}_{r:}\|_2^4} + \frac{3\|\mathbf{w}_{:r}\|_2^4 - \|\mathbf{w}_{:r}\|_4^4 }{\pi^2 \|\mathbf{w}_{r:}\|_2^4 }  +  O\left(\frac{r^4 + \log^4(m)}{ d^{2}} \right) \nonumber \\
   &= 1 - \frac{\|\mathbf{w}_{:r}\|_2^2}{\|\mathbf{w}_{r:}\|_2^2} + O\left(\frac{r^4 + \log^4(m)}{ d^{2}} \right) \nonumber 
\end{align}
for an absolute constant $c$, where we have used $\w\in \mathcal{G}_{\mathbf{w}}$. Combining this with \eqref{where} and \eqref{f} completes the proof.
% error after 1 step for this term will be (with $\lambda $ set pessimistically) $ \eta\frac{2}{\pi} ( 1  - \frac{\|\mathbf{M}_{r:}^\top \w\|_2^2}{\|\w\|_2^2} ) {\mathbf{M}_{r:}^\top \w} $ which has norm $\approx \frac{r}{k} \sqrt{d-r} $ (if $r$ is approximately $k$, then this is again zero).
% which isn't tight enough, but we can approximate to arbitrary order to get arbitrarily tight bound
% easy to get up to 1/k2 error in approximating this constant
% which means the matrix will have spectral norm 1/k 
% prod with w has norm 1/rt(k)
% prod with new x will have norm O(1times rt(r 2r log(k))) which is still too large, needs to be o(1)
% is there a way to get rid of 2r union bound?
% is it ok if only a subset of the neurons are good?
% with subset (hoeffding) argument, we get rid of union bound, and good part and bad part have the same norm up to constants
% with tight analysis of error variance we can make the bad constat very small.
% but is this good enough?
% it is good enough for there to exist a good network?
% yes, with bias.
% can add very small bias before first step and I think the proof should work. basically you're just fixing a u0 coordinate. think of b as part of w.
% make learning rate for b very small
% then we should be able to say that the loss after one step is small for some choice of a...
\end{proof}




\begin{lemma}\label{lem:aparaperp}
    % For all $j: \mathbf{w}_{j}^0\in \mathcal{G}_{\mathbf{w}}$, we have 
    For any $ \mathbf{w}\in \mathcal{G}_{\mathbf{w}}$, we have 
    \begin{align}
        \left\|\mathbf{A}_{\parallel,\perp}(\mathbf{w}) - \frac{ \mathbf{w}_{:r}\mathbf{w}_{:r}^\top }{2{\pi}\|\mathbf{w}_{r:}\|_2^2} \right\|_2 &\leq c\frac{r^{3.5} + \log^{3.5}(m)}{d^{1.5}}
    \end{align}
\end{lemma}



\begin{proof}
Arguing similarly to the previous two lemmas, we obtain
\begin{align}
    \mathbf{A}_{\parallel,\perp}(\mathbf{w}) &= \mathbb{E}_{\mathbf{u},\mathbf{x},\mathbf{x}'} \left[  \mathbf{x}_{:r}(\mathbf{x}'_{r:})^\top {\sigma}'(\mathbf{w}^\top  \mathbf{x}') \sigma'(\mathbf{w}^\top \mathbf{x}) | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r}) =\mathbf{u}  \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{u},\mathbf{x},\mathbf{x}'_{:r}} \left[  \mathbf{x}_{:r} \sigma'(\mathbf{w}^\top \mathbf{x}) \E_{\mathbf{x}'_{r:}} \left[(\mathbf{x}'_{r:})^\top {\sigma}'(\mathbf{w}^\top  \mathbf{x}')\right] | \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r}) = \mathbf{u}  \right] \nonumber \\
    &=  \mathbb{E}_{\mathbf{u},\mathbf{x},\mathbf{x}'_{:r}} \left[  \mathbf{x}_{:r} \sigma'(\mathbf{w}^\top \mathbf{x}) \exp\left( - \frac{((\mathbf{x}'_{:r})^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)| \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})=\mathbf{u}   \right] \nonumber \\
    &\quad \times  \frac{ \mathbf{w}_{:r}^\top }{\sqrt{2 \pi}\|\mathbf{w}_{r:}\|_2}  \label{nm} %\\
\end{align}
where \eqref{nm} follows by the same calculation as in \eqref{mn}.
Next, since the only term that depends on $\mathbf{x}_{r:}$ is $\sigma'(\mathbf{w}^\top \mathbf{x})$, we have
\begin{align}
\nonumber \\
 &=  \mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}'_{:r}} \left[  \mathbf{x}_{:r} \mathbb{E}_{\mathbf{x}_{r:}}[\sigma'(\mathbf{w}^\top \mathbf{x})] \exp\left( - \frac{((\mathbf{x}'_{:r})^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)| \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})=\mathbf{u}   \right] \nonumber \\
    &\quad \times  \frac{ \mathbf{w}_{:r}^\top }{\sqrt{2 \pi}\|\mathbf{w}_{r:}\|_2}  \nonumber \\
     &=  \mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}'_{:r}} \left[  \mathbf{x}_{:r} \mathbb{P}_{\mathbf{x}_{r:}}[\mathbf{w}_{r:}^\top \mathbf{x}_{r:} > - \mathbf{w}_{:r}^\top \mathbf{x}_{:r} ] \exp\left( - \frac{((\mathbf{x}'_{:r})^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)| \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})=\mathbf{u}   \right] \nonumber \\
    &\quad \times  \frac{ \mathbf{w}_{:r}^\top }{\sqrt{2 \pi}\|\mathbf{w}_{r:}\|_2}  \nonumber \\
    &=  \mathbb{E}_{\mathbf{u},\mathbf{x},\mathbf{x}'_{:r}} \left[  \mathbf{x}_{:r} \left(\frac{1}{2} + \frac{1}{2} \erf\left( \frac{{\mathbf{x}}_{:r}^\top\mathbf{w}_{:r}}{\sqrt{2}\|\mathbf{w}_{r:}\|_2} \right) \right) \exp\left( \! - \frac{((\mathbf{x}'_{:r})^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)| \sign(\mathbf{x}'_{:r})\!=\!\sign({\mathbf{x}}_{:r})\!  =\! \mathbf{u}  \right] \nonumber \\
    &\quad \times \frac{ \mathbf{w}_{:r}^\top }{\sqrt{2 \pi}\|\mathbf{w}_{r:}\|_2}   \label{hhj} 
    \end{align}
where \eqref{hhj} follows by the Gaussian CDF.
Note that
\begin{align}
    &\mathbb{E}_{\mathbf{u},\mathbf{x},\mathbf{x}'_{:r}} \left[  \mathbf{x}_{:r}  \exp\left( - \frac{((\mathbf{x}'_{:r})^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)| \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})  = \mathbf{u}  \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{u},\mathbf{x}_{:r},\mathbf{x}'_{:r}} \left[ \diag(\mathbf{u}) |\mathbf{x}_{:r} | \exp\left( - \frac{(|\mathbf{x}'_{:r}|^\top\diag(\mathbf{u})\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right) \right] \nonumber \\
    &= \mathbb{E}_{\mathbf{x}_{:r},\mathbf{x}'_{:r}} \left[ \mathbb{E}_{\mathbf{u}}\left[ \diag(\mathbf{u}) |\mathbf{x}_{:r} | \left(1  - \frac{(|\mathbf{x}'_{:r}|^\top\diag(\mathbf{u})\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} + \frac{(|\mathbf{x}'_{:r}|^\top\diag(\mathbf{u})\mathbf{w}_{:r})^4}{2\|\mathbf{w}_{r:}\|_2^4} -\dots \right)\right] \right] \label{aza} \\
    &= \mathbf{0} \label{ewe}
\end{align}
where \eqref{ewe} follows since each term in \eqref{aza} is an odd power of $\mathbf{u}$.
  Thus, from \eqref{hhj} we have
  \begin{align}
\mathbf{A}_{\parallel,\perp}(\mathbf{w})     &=  \mathbb{E}_{\mathbf{x},\mathbf{x}'_{:r}} \left[  \mathbf{x}_{:r} \erf\left( \frac{{\mathbf{x}}_{:r}^\top\mathbf{w}_{:r}}{\sqrt{2}\|\mathbf{w}_{r:}\|_2} \right)  \exp\left( - \frac{((\mathbf{x}'_{:r})^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)| \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})  =\mathbf{u}  \right] \nonumber \\
    &\quad \times \frac{ \mathbf{w}_{:r}^\top }{2\sqrt{2\pi}\|\mathbf{w}_{r:}\|_2} \label{sds}
    % &= \mathbb{E}_{\mathbf{x},\mathbf{x}'_{:r}} \left[  \mathbf{x}_{:r} \erf\left( \frac{{\mathbf{x}}_{:r}^\top\mathbf{w}_{:r}}{\sqrt{2}\|\mathbf{w}_{r:}\|_2} \right)  \exp\left( - \frac{((\mathbf{x}'_{:r})^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} \right)| \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})   = \mathbf{u} \right]\nonumber\\
    % &\quad \times \frac{ \mathbf{w}_{:r}^\top }{2\sqrt{2\pi}\|\mathbf{w}_{r:}\|_2} \nonumber \\
    \end{align}
Next we take the Taylor expansions of $\erf(x)$ and $\exp(-x^2)$ to obtain 
    \begin{align}
&\mathbf{A}_{\parallel,\perp}(\mathbf{w}) \nonumber \\
&= \mathbb{E}_{\mathbf{u},\mathbf{x},\mathbf{x}'_{:r}} \Bigg[  \mathbf{x}_{:r} \left( \frac{{\mathbf{x}}_{:r}^\top\mathbf{w}_{:r}}{\|\mathbf{w}_{r:}\|_2} 
 - \frac{ ({\mathbf{x}}_{:r}^\top\mathbf{w}_{:r})^3 }{6\|\mathbf{w}_{r:}\|_2^3} + \dots \right)\nonumber \\
 &\quad \quad \quad \quad \times \left(1  - \frac{((\mathbf{x}'_{:r})^\top\mathbf{w}_{:r})^2}{2\|\mathbf{w}_{r:}\|_2^2} + \dots \right)| \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})   = \mathbf{u} \Bigg]\frac{ \mathbf{w}_{:r}^\top }{2{\pi}\|\mathbf{w}_{r:}\|_2} \nonumber\\
    % &\quad \times \frac{ \mathbf{w}_{:r}^\top }{2{\pi}\|\mathbf{w}_{r:}\|_2} \nonumber \\
    &= \mathbb{E}_{\mathbf{u},\mathbf{x},\mathbf{x}'_{:r}} \left[  \mathbf{x}_{:r}{\mathbf{x}}_{:r}^\top | 
 \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})  = \mathbf{u} \right]\frac{ \mathbf{w}_{:r}\mathbf{w}_{:r}^\top }{2{\pi}\|\mathbf{w}_{r:}\|_2^2}  + \mathbf{E} \nonumber \\
 &=   \frac{ \mathbf{w}_{:r}\mathbf{w}_{:r}^\top }{2{\pi}\|\mathbf{w}_{r:}\|_2^2}  + \mathbf{E} \nonumber 
\end{align}
where $\|\mathbf{E}\|_2 = O\left( \frac{r^{3.5}+\log^{3.5}(m)}{d^{1.5}} \right)$ since $\|\mathbf{w}_{r:}\|_2 = \Omega(\sqrt{d})$ and $\|\mathbf{w}_{:r}\|_2 = O(\sqrt{r} + \sqrt{\log(m)})$ as $\mathbf{w} \in \mathcal{G}_{\mathbf{w}}$, and $\mathbb{E}_{\mathbf{u},\mathbf{x},\mathbf{x}'_{:r}} \left[  \mathbf{x}_{:r}{\mathbf{x}}_{:r}^\top | 
 \sign(\mathbf{x}'_{:r})=\sign({\mathbf{x}}_{:r})  = \mathbf{u} \right] = \mathbf{I}_r$ due to the same argument as in \eqref{dfc}.
% Using the Taylor expansions of $\erf$ and $\exp$ 
% to get last line: condition on sign(z) = v and sign(z)= - v 
\end{proof}

\input{Proof_Rep2}




==> Proof_old.tex <==

\newpage

\section{old}

We have reduced the first gradient descent update for each weight vector to:
\begin{align}
    \mathbf{w}^+ &= \mathbf{w}(1-\eta \lambda) + \eta \begin{bmatrix}
        \mathbf{A}_{||,||} & \mathbf{A}_{||,\perp} \\
        \mathbf{A}_{\perp,||} & \mathbf{A}_{\perp,\perp} \\
    \end{bmatrix} \w
\end{align}



% differences with shi analysis: 
% - -1,1 vs 0,1, and normalization
% - non-smooth activations
% otherwise there's is more general and should be readily applicable

% can 




% but parallel part has a true r/(k-r) error that we should fix










% \begin{align}
%     \mathbf{w}_t = \mathbf{M}_{:r}^\top \mathbf{w}_t + \mathbf{M}_{r:}^\top \mathbf{w}_t + (\mathbf{I}- \mathbf{MM}^\top)  \mathbf{w}_t = a_t  \mathbf{M}_{:r}^\top \mathbf{w}_0 + b_t\mathbf{M}_{r:}^\top \mathbf{w}_0 + c_t (\mathbf{I}- \mathbf{MM}^\top)  \mathbf{w}_0 
% \end{align}

\begin{align}
    a_{t} &:=  \frac{ 1 }{ \| \mathbf{M}_{:r}^\top \mathbf{w}_0\|_2 } \mathbf{w}_{0}^\top \mathbf{M}_{:r} \mathbf{M}_{:r}^\top \mathbf{w}_t \nonumber \\
    b_{t} &:= \frac{ 1 }{ \| \mathbf{M}_{r:}^\top \mathbf{w}_0\|_2 } \mathbf{w}_{0}^\top \mathbf{M}_{r:} \mathbf{M}_{r:}^\top \mathbf{w}_t \nonumber \\
    \mathbf{w}_t &:=  \frac{ a_t }{ \| \mathbf{M}_{:r}^\top \mathbf{w}_0\|_2 }  \mathbf{M}_{:r} \mathbf{M}_{:r}^\top \mathbf{w}_0   +  \frac{ b_t }{ \| \mathbf{M}_{r:}^\top \mathbf{w}_0\|_2 }  \mathbf{M}_{r:} \mathbf{M}_{r:}^\top \mathbf{w}_0 \nonumber \\
    &\quad + \left( \mathbf{I} - \frac{ 1 }{ \| \mathbf{M}_{:r}^\top \mathbf{w}_0\|_2^2 } \mathbf{M}_{:r} \mathbf{M}_{:r}^\top \mathbf{w}_{0} \mathbf{w}_{0}^\top \mathbf{M}_{:r} \mathbf{M}_{:r}^\top  - \frac{ 1 }{ \| \mathbf{M}_{:r}^\top \mathbf{w}_0\|_2^2 } \mathbf{M}_{r:} \mathbf{M}_{r:}^\top \mathbf{w}_{0} \mathbf{w}_{0}^\top \mathbf{M}_{r:} \mathbf{M}_{r:}^\top \right) \mathbf{w}_t \nonumber 
\end{align}


\begin{align}
    {a}_{t+1} &= (1 - \eta \lambda ) a_t +   \nonumber \\
    b_{t+1} &= (1 - \eta \lambda ) b_t +  \eta 2^{-r-2} \frac{2 f_t }{\pi}
\end{align}





\begin{lemma} \label{lem:first}
After step $t=1$, the learned weight matrix satisfies 

\begin{align}
    \mathbf{W}_1 = \mathbf{M}_{:r}\mathbf{M}_{:r}^\top \mathbf{W}_0 + \mathbf{N}
\end{align}
where each row of $\mathbf{N}$ satisfies $\|\mathbf{n}_j\|_2=O(\sqrt{m}/\sqrt{k})$.
\end{lemma}






\begin{proof}
Consider any neuron $j$ with weight vector $\mathbf{w}_{j,0}$ at time $0$. We will compute $\mathbf{w}_{j,1}$, i.e. the updated weight vector for neuron $j$ after one step of gradient descent:
\begin{align}
    \mathbf{w}_{j,1} = \mathbf{w}_{j,0} - \eta  \nabla_{\mathbf{w}_{j}} \mathbb{E}_i[\mathcal{L}_i(\mathbf{W}, \mathbf{a}_i(\mathbf{W}))] - \eta \lambda \mathbf{w}_{j,0}
\end{align}
where $\mathbf{a}_i(\mathbf{W}) \in \arg\min_{\mathbf{a}\in \mathbb{R}^m}  \mathcal{L}_i(\mathbf{W}, \mathbf{a})$.
For ease of notation, we drop the time and node index  subscripts in subsequent analysis, letting $\mathbf{w}\equiv \mathbf{w}_{j,0}$ and $\mathbf{w}^+\equiv \mathbf{w}_{j,1}$.

We show in Lemma \ref{lem:compute_grad} that
\begin{align}
    \w^+ &= \w(1 - \eta \lambda) + \eta \begin{bmatrix}
        \mathbf{A}_{||,||}(\w) &  \mathbf{A}_{||,\perp}(\w) \\
        \mathbf{A}_{\perp,||}(\w) & \mathbf{A}_{\perp,\perp}(\w) \\
    \end{bmatrix}\w
\end{align}
where 
\begin{align}
    \mathbf{A}_{||,||}(\w) &= 2^{-r} \mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[ \mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^{k-r})} \left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2 \mathbf{uu}^\top  \right] \\
    \mathbf{A}_{||,\perp}(\w) &= 2^{-r} \mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[ \mathbb{E}_{\mathbf{v}\in \mathcal{H}^{k-r}} \left[\sigma'( \mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v} )\right] \mathbf{u} \mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^{k-r})}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right] \\
    \mathbf{A}_{\perp,||}(\w) &= 2^{-r} \mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[  \mathbb{E}_{\mathbf{v}\in \mathcal{H}^{k-r}}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right] \mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^{k-r})} \left[\sigma'( \mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\right] \mathbf{u}^\top  \right] \\
    \mathbf{A}_{\perp,\perp}(\w) &= 2^{-r} \mathbb{E}_{\mathbf{u}\sim \text{Unif}(\mathcal{H}^{r})}\left[  \mathbb{E}_{\mathbf{v}\in \mathcal{H}^{k-r}}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]  \mathbb{E}_{\mathbf{v}\in \mathcal{H}^{k-r}}\left[\sigma'(\mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right] 
\end{align}

We approximate each of these matrices with their analogues in the case that the 

% Let $s(\mathbf{w},\mathbf{u}) \coloneqq \sum_{\mathbf{v}\in \mathcal{H}^{k-r}} \sigma'( \mathbf{w}_{||}^\top \mathbf{u}+ \mathbf{w}_{\perp}^\top \mathbf{v})$.
Let $\mathbf{A}\coloneqq \begin{bmatrix}
        \mathbf{A}_{||,||} &  \mathbf{A}_{||,\perp} \\
        \mathbf{A}_{\perp,||} & \mathbf{A}_{\perp,\perp} \\
    \end{bmatrix}$. 
Observe that
\begin{align}
    \w^+ &= \w(1 - \eta \lambda) + \eta 2^{-r-2} \begin{bmatrix}
       \mathbf{I}_{r} &  \mathbf{0}_{r,k-r} \\
        \mathbf{0}_{k-r,r} & \frac{2}{\pi \|\w_{\perp}\|_2^2}\mathbf{w}_{\perp}\mathbf{w}_{\perp}^\top  \\
    \end{bmatrix}\w + \eta  \left( 
        \mathbf{A} -  2^{-r-2}\begin{bmatrix}
        \mathbf{I}_{r} &  \mathbf{0}_{r,k-r} \\
        \mathbf{0}_{k-r,r} & \frac{2}{\pi \|\w_{\perp}\|_2^2}\mathbf{w}_{\perp}\mathbf{w}_{\perp}^\top  \\
    \end{bmatrix}\right)\w
\end{align}
By Lemmas \ref{}, with probability at least..., we have

\begin{align}
    \w^+_{\parallel} &= \left(1 - \eta \lambda + \eta 2^{-r-2} \left(1 + \frac{2}{\pi}\right)\right)\w_{\parallel}  + O\left(\frac{\eta}{\sqrt{k}}\right) \nonumber \\
    \w^+_{\perp} &= \left(1 - \eta \lambda + \eta 2^{-r-2}\frac{2}{\pi}\right)\w_{\perp}  + O\left(\frac{\eta}{\sqrt{k}}\right) \nonumber
\end{align}

Choose $\eta = \Theta(1)$ and $\lambda = \tfrac{1+\eta 2^{-r-2} \tfrac{2}{\pi}}{\eta}$.


Union bounding over all neurons completes the proof.

\end{proof}













% For each $i\in [2^r]$, define
% \begin{align}
%     x_i \coloneqq \sum_{\mathbf{v}_j} \chi\{ [\mathbf{u}_i^\top, \mathbf{v}^\top] \mathbf{w} > 0\}
% \end{align}


% \begin{lemma}
%     \begin{align}
%        \Pr_{\w}\left[ \|\mathbf{A}_{||,||} - 2^{-r-2}\mathbf{I}_r\|_2\geq \right] \leq 
%     \end{align}
%     {\color{red}note: need to union bound over all neurons, will linearly weaken the bound, but this is ok}
% \end{lemma}

% \begin{proof}

% % We have 
% % \begin{align}
% % \mathbf{A}_{||,||}&= \sum_{i=1}^{2^r} x_i^2 \mathbf{u}_i \mathbf{u}_i^\top
% % \end{align}



% % Outline: 
% % \begin{enumerate}
% % \item Compute mean and almost sure lower bound.
% %     \item Upper bound variance of $x_i$ as $1/k$. Use this to get upper bound on maximum singular value. Since $x_i$ close to its mean implies that $\mathbf{A}_{||,||}$ is close to its mean.
% %     \item Compute matrix variance statistic, show it is $1/\sqrt{k}$.
% %     \item Use this combined with upper bound on difference from mean to apply truncated matrix Bernstein inequality to get tight upper bound on  $\|\mathbf{A}_{||,||} - 2^{2k-r-2}\mathbf{I}_r\|_2 = O(\frac{\sqrt{r}}{\sqrt{k}})2^{2k-r-2}$.
% % \end{enumerate}


% \end{proof}


\begin{lemma}
With probability at least 0.99 over the Gaussian initialization of $\mathbf{w}$, 
    % \begin{align}
    %     \left\|\mathbf{A}_{\perp,\perp}(\w) - 2^{r-2} {\frac{2}{\pi}} \; \frac{\mathbf{w}_{\perp}\mathbf{w}_{\perp}^\top }{\|\mathbf{w}_{\perp}\|_2^2} \right\|_2 = O(rk^{-1/2})
    % \end{align}
  \begin{align}
        \left\|\mathbf{A}(\w) - \mathbf{A}^\star(\w) \right\|_2 = O(rk^{-1/2})
    \end{align}

    
\end{lemma}

\begin{proof}
Recall 
\begin{align}
\mathbf{A}_{\perp,\perp} &= 2^{-2k} \sum_{\mathbf{u} \in \mathcal{H}^r} \left(\sum_{\vv \in \mathcal{H}^{k-r}} \sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right)\left(\sum_{\vv \in \mathcal{H}^{k-r}} \sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right)^\top  \nonumber \\
&= 2^{-2r}\sum_{\mathbf{u} \in \mathcal{H}^r} 
\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]^\top 
% \left( 2^{-(k-r)}\sum_{\vv \in \mathcal{H}^{k-r}} \sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right)\left(2^{-(k-r)}\sum_{\vv \in \mathcal{H}^{k-r}} \sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right)^\top  
\end{align}


\begin{itemize}
    \item \textbf{Step 1: $\mathbf{A}^{\circ,{\mathcal{N}}}_{\perp,\perp} = 2^{-r-2} {\frac{2}{\pi}} \; \frac{\mathbf{w}_{\perp}\mathbf{w}_{\perp}^\top }{\|\mathbf{w}_{\perp}\|_2^2}$.} We have 
\begin{align}
    \mathbf{A}^{\circ,{\mathcal{N}}}_{\perp,\perp} = 2^{-r} \E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top\z) \z]\E_{\z'\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top\z') \z']^\top
\end{align}
which is $ 2^{-r}$ times the outer product of the vector $\E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top\z) \z]$ with itself. 
Note that 
\begin{align}
    \E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top\z) \z] &= \frac{1}{2}\E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}\left[\z - 2 \sigma\left(-\left(\frac{\w_\perp}{\|\w_\perp\|_2}\right)^\top\z\right) \frac{\w_\perp}{\|\w_\perp\|_2}\right]   \label{flip}\\
    &= \E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}\left[ \sigma\left(-\left(\frac{\w_\perp}{\|\w_\perp\|_2}\right)^\top\z \right) \right]  \frac{\w_\perp}{\|\w_\perp\|_2} \nonumber\\
    &= \frac{1}{2}\sqrt{\frac{2}{\pi}} \frac{\w_\perp}{\|\w_\perp\|_2} \label{halfnormal}
\end{align}
where \eqref{flip} follows since  and \eqref{halfnormal} follows since $\left(\frac{\w_\perp}{\|\w_\perp\|_2}\right)^\top\z$ is a Gaussian r.v. with mean 0 and variance 1.




    \item \textbf{Step 2: $\left\|\mathbf{A}_{\perp,\perp} - \mathbf{A}^\circ_{\perp,\perp}\right\|_2 = O(2^{r/2}r k^{-1/2})$ with probability at least $1 - 10^{-4}$.}
% Let $\aaa := \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]$, thus $\mathbf{A}_{\perp,\perp} = $   
We have $\mathbf{A}^\circ_{\perp,\perp} :=  2^{-r}\aaa \aaa^\top$, 
    % \begin{align}
    %     \mathbf{A}^\circ_{\perp,\perp}&:=\E_{\vv \sim \text{Unif}(\mathcal{H}^{k-r})}[\sigma'(\w_\perp^\top \vv)\vv]\E_{\vv \sim \text{Unif}(\mathcal{H}^{k-r})}[\sigma'(\w_\perp^\top \vv)\vv ]^\top \\
    % \mathbf{A}^{\circ,\mathcal{N}}_{\perp,\perp}&:= \E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top \z)\z]\E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top \z)\z]^\top
    % \end{align}
where 
% $b_i:= \E_{v_i \sim \text{Unif}(\{-1,1\}),\z_{-1}\sim \mathcal{N}(\mathbf{0}_{k-r-1},\mathbf{I}_{k-r-1})}[\sigma'(w_{\perp,i} v_i + \w_{\perp,-i}^\top\z_{-1}) v_i]$ for all $i \in [k-r]$. 
$\aaa = \E_{\vv\sim \text{Unif}(\mathcal{H}^{k-r})}[\sigma'(\w_\perp^\top \vv)\vv]$. 
We have
\begin{align}
    &\left\|\mathbf{A}_{\perp,\perp} - \mathbf{A}^\circ_{\perp,\perp}\right\|_2 \nonumber\\
    &= 2^{-r}\left\|2^{-r}\sum_{\mathbf{u} \in \mathcal{H}^r} \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]^\top   - \aaa\aaa^\top\right\|_2 \nonumber \\
    &\leq 
    % 2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}\left\|\left( 2^{-(k-r)}\sum_{\vv \in \mathcal{H}^{k-r}} \sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right)\left(2^{-(k-r)}\sum_{\vv \in \mathcal{H}^{k-r}} \sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right)^\top   - \aaa\aaa^\top\right\|_2 \nonumber \\
    % &= 
    2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}\left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]^\top   - \aaa\aaa^\top\right\|_2 \label{pre} \\
    &= 2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}  \sup_{\y : \|\y\|_2=1} \left| \left\langle \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right], \y \right\rangle^2   - \left\langle\aaa,\y\right\rangle^2\right| \nonumber \\
        &= 2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}  \sup_{\y : \|\y\|_2=1} \left|\left( \left\langle \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right], \y \right\rangle+\left\langle\aaa,\y\right\rangle \right)\left( \left\langle \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right], \y \right\rangle  - \left\langle\aaa,\y\right\rangle\right)\right| \nonumber \\
        &\leq  2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}  \sup_{\y : \|\y\|_2=1} \left| \left\langle \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right], \y \right\rangle+\left\langle\aaa,\y\right\rangle \right|\sup_{\y' : \|\y'\|_2=1} \left| \left\langle \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right], \y' \right\rangle  - \left\langle\aaa,\y'\right\rangle\right| \nonumber \\ 
        &=  2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}  \left\| \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]+\aaa \right\|_2 \left\|  \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]  - \aaa\right\|_2 \nonumber \\ 
        &= 2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r} \left(\|\aaa\|_2 + \left\| \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]-\aaa \right\|_2\right) \left\|  \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]  - \aaa\right\|_2 \label{186} 
    % &\leq 2^{-r}\max_{\mathbf{u} \in \mathcal{H}^r} \left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] + \aaa\right\|_2 \left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa\right\|_2 
\end{align}
% &=  2^{-r} \sup_{\y : \|\y\|_2=1} | \langle \y, \aaa\rangle^2 - \langle \y, \bbb\rangle^2 |\nonumber \\
        % &=  2^{-r}\sup_{\y : \|\y\|_2=1} | (\langle \y, \aaa\rangle - \langle \y, \bbb\rangle)(\langle \y, \aaa\rangle + \langle \y, \bbb\rangle) |\nonumber \\
        % &\leq  2^{-r}\sup_{\y : \|\y\|_2=1} | \langle \y, \aaa\rangle - \langle \y, \bbb\rangle| \sup_{\y' : \|\y'\|_2=1}|\langle \y', \aaa\rangle + \langle \y, \bbb\rangle |\nonumber \\
Thus we can upper bound $\left\|\mathbf{A}_{\perp,\perp} - \mathbf{A}^\circ_{\perp,\perp}\right\|_2 $ by upper bounding $\|\aaa\|_2$ and $\left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa\right\|_2$ for all $\uu \in \uH^r$. We start by controlling $\left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa\right\|_2$. We will upper bound $\|\aaa\|_2$ {\color{red}later}.

For any $\uu \in \uH^r$, we will control $\left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa\right\|_2$ by controlling each of the  coordinates of $\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa$. Note that each coordinate is identically distributed. The first coordinate is:
\begin{align}
    \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) v_1 \right] - \E_{\vv} \left[\sigma'(  \mathbf{w}_{\perp}^\top\mathbf{v} ) v_1 \right] =\E_{\vv} \left[(\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} )- \sigma'( \mathbf{w}_{\perp}^\top\mathbf{v} )) v_1 \right]
\end{align}
This is a scalar-valued random variable that is a function of $\w$.
Denote it as $f_1(\w)$, i.e. $f_1(\w):= \E_{\vv} \left[(\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} )- \sigma'( \mathbf{w}_{\perp}^\top\mathbf{v} )) v_1 \right]$.
By symmetry we have that $\E_{\w}[f_1(\w)]=0$, in particular,
\begin{align}
    \E_{\w}[f_1(\w)] &= \frac{1}{2}\E_{\w,\vv_{-1}}[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + {w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1} )- \sigma'( {w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1}))] \nonumber \\
    &\quad - \frac{1}{2}\E_{\w,\vv_{-1}}[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} -{w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1} )- \sigma'( -{w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1} ))] \nonumber \\
    &= \frac{1}{2}(\Pr_{\w,\vv_{-1}}[ \mathbf{w}_{\parallel}^\top \mathbf{u} + {w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1} >0] - \Pr_{\w,\vv_{-1}}[ \mathbf{w}_{\parallel}^\top \mathbf{u} - {w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1} >0] )
    % - \sigma'( {w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1}))] 
    \nonumber \\
    &\quad + \frac{1}{2}(\Pr_{\w,\vv_{-1}}[ -{w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1} >0]- \Pr_{\w,\vv_{-1}}[ {w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1} >0]) \nonumber \\
    &=0+0=0
\end{align}
where the first equality follows by the tower property and the last equality follows by the fact that ${w}_{\perp,-1}$ has the same distribution as $-{w}_{\perp,-1}$.




Next we control the second moment. 

\end{itemize}

This completes the proof.
\end{proof}



\begin{lemma}
    \begin{align}
       \Pr_{\w}\left[ \|\mathbf{A}_{||,\perp}\|_2\geq O(k^{-1/2}) \right] &\leq  \\
       \Pr_{\w}\left[ \|\mathbf{A}_{\perp,||}\|_2\geq O(k^{-1/2}) \right] &\leq  
    \end{align}
\end{lemma}


\begin{proof}
    

Note that $\mathbf{A}_{\perp,||} = \mathbf{A}_{||,\perp}^\top$, so we only need to consider and the proof for $\mathbf{A}_{||,\perp}$. 
We have 
\begin{align}
\|\mathbf{A}_{||,\perp}\|_2&= 2^{-2r}\left\|\sum_{\mathbf{u}\in \mathcal{H}^r}\mathbf{u} \mathbb{E}_{\vv}\left[ \sigma'(\mathbf{w}_{||}^\top \mathbf{u} + \w_{\perp}^\top \vv)  \vv\right]^\top\right\|_2 \nonumber \\
&=  2^{-2r}\left\|\sum_{\mathbf{u}\in \mathcal{H}^r}\mathbf{u} \aaa^\top - \sum_{\mathbf{u}\in \mathcal{H}^r}\mathbf{u}\left(\aaa - \mathbb{E}_{\vv}\left[ \sigma'(\mathbf{w}_{||}^\top \mathbf{u} + \w_{\perp}^\top \vv)  \vv\right]\right)^\top\right\|_2 \nonumber \\
&=  2^{-2r}\left\|\sum_{\mathbf{u}\in \mathcal{H}^r}\mathbf{u}\left(\aaa - \mathbb{E}_{\vv}\left[ \sigma'(\mathbf{w}_{||}^\top \mathbf{u} + \w_{\perp}^\top \vv)  \vv\right]\right)^\top\right\|_2 \nonumber \\
&\leq 2^{-r} \max_{\mathbf{u}\in \mathcal{H}^r} \left\|\mathbf{u}\right\|_2 \left\|\aaa - \mathbb{E}_{\vv}\left[ \sigma'(\mathbf{w}_{||}^\top \mathbf{u} + \w_{\perp}^\top \vv)  \vv\right]\right\|_2 \nonumber \\
&= 2^{-r} \sqrt{r} \max_{\mathbf{u}\in \mathcal{H}^r}  \left\|\aaa - \mathbb{E}_{\vv}\left[ \sigma'(\mathbf{w}_{||}^\top \mathbf{u} + \w_{\perp}^\top \vv)  \vv\right]\right\|_2 \nonumber 
\end{align}
where $\aaa:= \mathbb{E}_{\vv}\left[ \sigma'( \w_{\perp}^\top \vv)  \vv\right] $ as defined in the proof of Lemma \ref{lem:aperp}. By equation \eqref{} in the proof of Lemma \ref{lem:aperp}, we have $  \left\|\aaa - \mathbb{E}_{\vv}\left[ \sigma'(\mathbf{w}_{||}^\top \mathbf{u} + \w_{\perp}^\top \vv)  \vv\right]\right\|_2 \leq $ for all $\mathbf{u}\in \mathcal{H}^r$ with probability at least $1 - $. This completes the proof.
\end{proof}




\begin{align}
    \mathbf{A}_{||,||}([a_t,b_t]\mathbf{w}) &= 2^{-r} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[ \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}} \left[\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v} )\right]^2 \mathbf{uu}^\top  \right] \\
    \mathbf{A}_{||,\perp}([a_t,b_t]\mathbf{w}) &= 2^{-r} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[ \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}} \left[\sigma'( a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v} )\right] \mathbf{u} \; \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}}\left[\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right] \\
    \mathbf{A}_{\perp,||}([a_t,b_t]\mathbf{w}) &= 2^{-r} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[  \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}}\left[\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right] \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}} \left[\sigma'( a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v})\right] \mathbf{u}^\top  \right] \\
    \mathbf{A}_{\perp,\perp}([a_t,b_t]\mathbf{w}) &= 2^{-r} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[  \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}}\left[\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]  \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}}\left[\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right] 
\end{align}




If $a_t \mathbf{w}_{||}^\top \mathbf{u} < 0$:

\begin{align}
    &\mathbb{E}_{\mathbf{z}\sim \mathcal{N}}\left[\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{z})\mathbf{z} \right] \nonumber\\
    &= \frac{1}{2}\left(1 + \text{erf}\left( \frac{a_t \mathbf{w}_{||}^\top \mathbf{u}}{ \sqrt{2} b_t \|\mathbf{w}_{\perp}\|_2 } \right) \right) \mathbb{E}_{\mathbf{z}\sim \mathcal{N}}\left[ \mathbf{z} | a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{z} > 0 \right]  \nonumber \\
    &= \frac{1}{2}\left(1 + \text{erf}\left( \frac{a_t \mathbf{w}_{||}^\top \mathbf{u}}{ \sqrt{2} b_t \|\mathbf{w}_{\perp}\|_2 } \right) \right) \mathbb{E}_{\mathbf{z}\sim \mathcal{N}}\left[ \mathbf{z} - 2\sigma\left(-\frac{\mathbf{w}_{\perp}^\top}{\|\mathbf{w}_{\perp}\|_2} \mathbf{z} \right) \frac{\mathbf{w}_{\perp}}{\|\mathbf{w}_{\perp}\|_2}   \bigg| |b_t \mathbf{w}_{\perp}^\top \mathbf{z}| > -a_t \mathbf{w}_{||}^\top \mathbf{u} \right]  \nonumber \\
    % &= \frac{1}{2}\left(1 + \text{erf}\left( \frac{a_t \mathbf{w}_{||}^\top \mathbf{u}}{ \sqrt{2} b_t \|\mathbf{w}_{\perp}\|_2 } \right) \right) \mathbb{E}_{\mathbf{z}\sim \mathcal{N}}\left[ \mathbf{z} | b_t \mathbf{w}_{\perp}^\top \mathbf{z} > |a_t \mathbf{w}_{||}^\top \mathbf{u} |\right]  \nonumber 
    &= -\left(1 + \text{erf}\left( \frac{a_t \mathbf{w}_{||}^\top \mathbf{u}}{ \sqrt{2} b_t \|\mathbf{w}_{\perp}\|_2 } \right) \right) \mathbb{E}_{\mathbf{z}\sim \mathcal{N}}\left[\sigma\left(-\frac{\mathbf{w}_{\perp}^\top}{\|\mathbf{w}_{\perp}\|_2} \mathbf{z} \right)   \bigg| |b_t \mathbf{w}_{\perp}^\top \mathbf{z}| > -a_t \mathbf{w}_{||}^\top \mathbf{u} \right] \frac{\mathbf{w}_{\perp}}{\|\mathbf{w}_{\perp}\|_2}  \nonumber \\
    &= \frac{1}{2}\left(1 + \text{erf}\left( \frac{a_t \mathbf{w}_{||}^\top \mathbf{u}}{ \sqrt{2} b_t \|\mathbf{w}_{\perp}\|_2 } \right) \right) \mathbb{E}_{\mathbf{z}\sim \mathcal{N}}\left[\frac{\mathbf{w}_{\perp}^\top}{\|\mathbf{w}_{\perp}\|_2^2} \mathbf{z}   \bigg| \frac{\mathbf{w}_{\perp}^\top}{\|\mathbf{w}_{\perp}\|_2} \mathbf{z} > -\frac{a_t}{b_t \|\mathbf{w}_{\perp}\|_2} \mathbf{w}_{||}^\top \mathbf{u} \right] \frac{\mathbf{w}_{\perp}}{\|\mathbf{w}_{\perp}\|_2}  \nonumber \\
     &= \frac{1}{2}\left(1 + \text{erf}\left( \frac{a_t \mathbf{w}_{||}^\top \mathbf{u}}{ \sqrt{2} b_t \|\mathbf{w}_{\perp}\|_2 } \right) \right) \frac{\tfrac{1}{\sqrt{2\pi}} \exp\left(-{ \tfrac{a_t^2 (\mathbf{w}_{||}^\top \mathbf{u})^2}{2b_t^2 \|\mathbf{w}_{\perp}\|_2} }\right) }{\tfrac{1}{2} + \tfrac{1}{2}\text{erf}\left( \tfrac{a_t \mathbf{w}_{||}^\top \mathbf{u}}{ \sqrt{2} b_t \|\mathbf{w}_{\perp}\|_2 } \right)} \frac{\mathbf{w}_{\perp}}{\|\mathbf{w}_{\perp}\|^2_2}  \nonumber \\
     &=  \frac{1}{2}\sqrt{\frac{2}{\pi}} \exp\left(-{ \frac{a_t^2 (\mathbf{w}_{||}^\top \mathbf{u})^2}{2b_t^2 \|\mathbf{w}_{\perp}\|_2^2} }\right)  \frac{\mathbf{w}_{\perp}}{\|\mathbf{w}_{\perp}\|_2}  \nonumber 
\end{align}



If $a_t \mathbf{w}_{||}^\top \mathbf{u} > 0$:
\begin{align}
    \mathbb{E}_{\mathbf{z}\sim \mathcal{N}}\left[\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{z})\mathbf{z} \right] &=  0 -  \mathbb{E}_{\mathbf{z}\sim \mathcal{N}}\left[\sigma'(-a_t \mathbf{w}_{||}^\top \mathbf{u} -b_t \mathbf{w}_{\perp}^\top \mathbf{z})\mathbf{z} \right] \nonumber \\
    &=   \mathbb{E}_{\mathbf{z}\sim \mathcal{N}}\left[\sigma'(-a_t \mathbf{w}_{||}^\top \mathbf{u} -b_t \mathbf{w}_{\perp}^\top \mathbf{z})(-\mathbf{z}) \right] \nonumber \\
    &=   \mathbb{E}_{\mathbf{z}\sim \mathcal{N}}\left[\sigma'(-a_t \mathbf{w}_{||}^\top \mathbf{u} +b_t \mathbf{w}_{\perp}^\top \mathbf{z})\mathbf{z} \right] \nonumber \\
     &=  \frac{1}{2}\sqrt{\frac{2}{\pi}}  \exp\left(-{ \frac{a_t^2 (\mathbf{w}_{||}^\top \mathbf{u})^2}{2b_t^2 \|\mathbf{w}_{\perp}\|^2_2} }\right)  \frac{\mathbf{w}_{\perp}}{\|\mathbf{w}_{\perp}\|_2}  \nonumber 
\end{align}
So it is the same in both cases.

\begin{align}
    \mathbf{A}_{\perp,\perp}([a_t,b_t]\mathbf{w}) &= 2^{-r} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[  \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}}\left[\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]  \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}}\left[\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right]  \nonumber \\
    &\approx 2^{-r} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[  \mathbb{E}_{\mathbf{z}\sim \mathcal{N}}\left[\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{z})\mathbf{z} \right]  \mathbb{E}_{\mathbf{z}\sim \mathcal{N}}\left[\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{z})\mathbf{z} \right]^\top  \right]  \nonumber \\
    &= 2^{-r-2} \times \frac{2}{\pi} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[  \exp\left(-{ \frac{a_t^2 (\mathbf{w}_{||}^\top \mathbf{u})^2}{b_t^2 \|\mathbf{w}_{\perp}\|_2^2} }\right)  \right] \frac{\mathbf{w}_{\perp}\mathbf{w}_{\perp}^\top}{\|\mathbf{w}_\perp\|_2^2}  \nonumber \\
    &\approx 2^{-r-2} \times \frac{2}{\pi} \left( 1 - { \frac{a_t^2 \|\mathbf{w}_{||}\|_2^2 }{b_t^2 \|\mathbf{w}_{\perp}\|_2^2} } \right) \frac{\mathbf{w}_{\perp}\mathbf{w}_{\perp}^\top}{\|\mathbf{w}_\perp\|_2^2}  \nonumber
\end{align}




\begin{align}
    \mathbf{A}_{||,\perp}([a_t,b_t]\mathbf{w}) &= 2^{-r} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[ \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}} \left[\sigma'( a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v} )\right] \mathbf{u} \; \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}}\left[\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right] \\
    &\approx 2^{-r} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[ \left(\frac{1}{2} + \frac{1}{2}\text{erf}\left( \frac{ a_t \mathbf{w}_{||}^\top \mathbf{u} }{ \sqrt{2} b_t \|\mathbf{w}_{\perp}\|_2 }   \right) \right) \mathbf{u} \; \mathbb{E}_{\mathbf{v}\sim \mathcal{H}^{k-r}}\left[\sigma'(a_t \mathbf{w}_{||}^\top \mathbf{u}+ b_t \mathbf{w}_{\perp}^\top \mathbf{v})\mathbf{v} \right]^\top  \right] \\
    &\approx 2^{-r} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[ \left(\frac{1}{2} + \frac{1}{2}\text{erf}\left( \frac{ a_t \mathbf{w}_{||}^\top \mathbf{u} }{ \sqrt{2} b_t \|\mathbf{w}_{\perp}\|_2 }   \right) \right) \mathbf{u} \; \exp\left(-\frac{a_t^2 (\mathbf{w}_{||}^\top \mathbf{u})^2 }{ 2b_t^2 \|\mathbf{w}_{\perp}\|_2^2 } \right)   \right] \frac{1}{\sqrt{2 \pi}} \frac{\mathbf{w}_{\perp}^\top}{\|\mathbf{w}_{\perp}\|_2} \\
    &= 2^{-r-2} \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[ \text{erf}\left( \frac{ a_t \mathbf{w}_{||}^\top \mathbf{u} }{\sqrt{2} b_t \|\mathbf{w}_{\perp}\|_2 }   \right) \mathbf{u} \; \exp\left(-\frac{a_t^2 (\mathbf{w}_{||}^\top \mathbf{u})^2 }{ 2b_t^2 \|\mathbf{w}_{\perp}\|_2^2 } \right)   \right] \sqrt{\frac{2}{\pi}} \frac{\mathbf{w}_{\perp}^\top}{\|\mathbf{w}_{\perp}\|_2} \\
    &\approx 2^{-r-2} \frac{2 a_t}{\pi b_t}   \mathbb{E}_{\mathbf{u}\sim \mathcal{H}^{r}}\left[   \mathbf{u}\mathbf{u}^\top \; \exp\left(-\frac{a_t^2 (\mathbf{w}_{||}^\top \mathbf{u})^2 }{ 2b_t^2 \|\mathbf{w}_{\perp}\|_2^2 } \right)   \right]  \frac{\mathbf{w}_{||} \mathbf{w}_{\perp}^\top}{\|\mathbf{w}_{\perp}\|_2^2} \\
    &\approx   2^{-r-2} \frac{2 a_t}{\pi b_t}   \left( 1 - \frac{  a_t^2 \|\mathbf{w}_{||}\|_2^2 }{ 2b_t^2 \|\mathbf{w}_{\perp}\|_2^2 } \right) \frac{\mathbf{w}_{||} \mathbf{w}_{\perp}^\top}{\|\mathbf{w}_{\perp}\|_2^2} 
\end{align}



\begin{align}
    \mathbf{A}_{||,||}^\star([a_t,b_t]\mathbf{w}) &= 2^{-r-2} \mathbf{I}_r  \\
    \mathbf{A}_{||,\perp}^\star([a_t,b_t]\mathbf{w}) &=  2^{-r-2} \frac{2 a_t}{\pi b_t}   \left( 1 - \frac{  a_t^2 \|\mathbf{w}_{||}\|_2^2 }{ 2b_t^2 \|\mathbf{w}_{\perp}\|_2^2 } \right) \frac{\mathbf{w}_{||} \mathbf{w}_{\perp}^\top}{\|\mathbf{w}_{\perp}\|_2^2}  \\
    \mathbf{A}_{\perp,||}^\star([a_t,b_t]\mathbf{w}) &=  2^{-r-2} \frac{2 a_t}{\pi b_t}   \left( 1 - \frac{  a_t^2 \|\mathbf{w}_{||}\|_2^2 }{ 2b_t^2 \|\mathbf{w}_{\perp}\|_2^2 } \right) \frac{\mathbf{w}_{\perp} \mathbf{w}_{||}^\top}{\|\mathbf{w}_{\perp}\|_2^2} \\
    \mathbf{A}_{\perp,\perp}^\star([a_t,b_t]\mathbf{w}) &= 2^{-r-2} \times \frac{2}{\pi} \left( 1 - { \frac{a_t^2 \|\mathbf{w}_{||}\|_2^2 }{b_t^2 \|\mathbf{w}_{\perp}\|_2^2} } \right) \frac{\mathbf{w}_{\perp}\mathbf{w}_{\perp}^\top}{\|\mathbf{w}_\perp\|_2^2} 
\end{align}



\begin{align}
    \mathbf{A}^{\star}([a_t,b_t] \mathbf{w}_0) &= \begin{bmatrix}
       { 2^{-r-2} } \mathbf{I}_r
          & 2^{-r-2} \frac{2 a_t}{\pi b_t}   \left( 1 - \frac{  a_t^2 \|\mathbf{w}_{||}\|_2^2 }{ 2b_t^2 \|\mathbf{w}_{\perp}\|_2^2 } \right) \frac{\mathbf{w}_{||} \mathbf{w}_{\perp}^\top}{\|\mathbf{w}_{\perp}\|_2^2}  \\
          2^{-r-2} \frac{2 a_t}{\pi b_t}   \left( 1 - \frac{  a_t^2 \|\mathbf{w}_{||}\|_2^2 }{ 2b_t^2 \|\mathbf{w}_{\perp}\|_2^2 } \right) \frac{\mathbf{w}_{\perp} \mathbf{w}_{||}^\top}{\|\mathbf{w}_{\perp}\|_2^2}  & 2^{-r-2}  \frac{2}{\pi} \left( 1 - { \frac{a_t^2 \|\mathbf{w}_{||}\|_2^2 }{b_t^2 \|\mathbf{w}_{\perp}\|_2^2} } \right) \frac{\mathbf{w}_{\perp}\mathbf{w}_{\perp}^\top}{\|\mathbf{w}_\perp\|_2^2}   \\
    \end{bmatrix}
\end{align}


\begin{align}
    \mathbf{w}_{t+1} &= (1 - \eta \lambda)\mathbf{w}_t + \eta \mathbf{A}(\w_t)\w_t \nonumber \\
    &= (1 - \eta \lambda)([a_t,b_t] \mathbf{w}_0 +\mathbf{n}_t) + \eta \mathbf{A}([a_t,b_t] \mathbf{w}_0 +\mathbf{n}_t)([a_t,b_t] \mathbf{w}_0 +\mathbf{n}_t)   \nonumber \\
    &= [a_t,b_t](1 - \eta \lambda)\mathbf{w}_0 + (1 - \eta \lambda)\mathbf{n}_t + \eta \mathbf{A}([a_t,b_t] \mathbf{w}_0 )([a_t,b_t] \mathbf{w}_0 +\mathbf{n}_t) \nonumber \\
    &\quad \quad + \eta \left(\mathbf{A}([a_t,b_t]\mathbf{w}_0+\mathbf{n}_t) - \mathbf{A}([a_t,b_t] \mathbf{w}_0 ) \right)([a_t,b_t] \mathbf{w}_0 +\mathbf{n}_t)  \nonumber \\
    &= [a_t,b_t](1 - \eta \lambda)\mathbf{w}_0 + (1 - \eta \lambda)\mathbf{n}_t + \eta [a_t,b_t] \mathbf{A}([a_t,b_t] \mathbf{w}_0 )\mathbf{w}_0  \nonumber \\
    &\quad \quad + \eta \mathbf{A}([a_t,b_t] \mathbf{w}_0 )\mathbf{n}_t + \eta \left(\mathbf{A}([a_t,b_t] \mathbf{w}_0+\mathbf{n}_t) - \mathbf{A}([a_t,b_t] \mathbf{w}_0 ) \right)([a_t,b_t] \mathbf{w}_0 +\mathbf{n}_t)  \nonumber \\
    &= [a_t,b_t](1 - \eta \lambda)\mathbf{w}_0 + (1 - \eta \lambda)\mathbf{n}_t + \eta \mathbf{A}^\star([a_t,b_t] \mathbf{w}_0 )[a_t,b_t]\mathbf{w}_0  + {\color{red}\eta \underbrace{ \left(\mathbf{A}([a_t,b_t] \mathbf{w}_0 ) - \mathbf{A}^\star([a_t,b_t]\mathbf{w}_0 )\right)}_{\mathbf{E}_{1,t}} }[a_t,b_t]\mathbf{w}_0\nonumber \\
    &\quad \quad  {\color{red} + \eta {\mathbf{A}([a_t,b_t] \mathbf{w}_0 )\mathbf{n}_t} +\eta \underbrace{\left(\mathbf{A}([a_t,b_t] \mathbf{w}_0+\mathbf{n}_t) - \mathbf{A}([a_t,b_t]\mathbf{w}_0 ) \right)}_{\mathbf{E}_{2,t}}}([a_t,b_t] \mathbf{w}_0 +\mathbf{n}_t)  \nonumber
\end{align}


% (i think the off diags are should be divided by 4. other consts might be off)

\begin{align}
    \w_{t+1,||} &= a_t(1-\eta \lambda)\w_{0,||} + (1-\eta \lambda)\mathbf{n}_{t,||} + \eta 2^{-r-2} a_t \w_{0,||}  + \eta 2^{-r-2} \tfrac{2}{\pi} a_t \left( 1 - { \frac{a_t^2 \|\mathbf{w}_{||}\|_2^2 }{b_t^2 \|\mathbf{w}_{\perp}\|_2^2} } \right) \w_{0,||}  \nonumber \\
   &\quad  {\color{red} + \eta \frac{c_1}{k} a_t \|\mathbf{w}_0\|_2 + \eta   c_2 \|\mathbf{n}_t\|_2 + \eta c_3 \|\mathbf{n}_t\|_2 (a_t \|\mathbf{w}_0\|_2 + \|\mathbf{n}_t\|_2) }  \nonumber \\
   &= a_t(1-\eta \lambda)\w_{0,||} + (1-\eta \lambda)\mathbf{n}_{t,||} + \eta 2^{-r-2} a_t \w_{0,||}  + \eta 2^{-r-2} \tfrac{2}{\pi} a_t \left( 1 - { \frac{a_t^2 \|\mathbf{w}_{||}\|_2^2 }{b_t^2 \|\mathbf{w}_{\perp}\|_2^2} } \right) \w_{0,||}  \nonumber \\
   &\quad  {\color{red} + \eta c_4 \left(\left(\frac{1}{k}  +\|\mathbf{n}_t\|_2\right)a_t\|\mathbf{w}_0\|_2 + \|\mathbf{n}_t\|_2 \right) } 
\end{align}



==> RelatedWorks.tex <==
\subsection{Related Work} \label{sec:related}


% \textbf{Empirical evidence of the benefit of multi-task pre-training with task-adapted heads.} A number of 

% \cite{lu202012} vision example. Shared representation with task-specific heads for pre-training.

% Pre-training a large language model to do next-word completion using  Wikipedia text can be thought of as multi-task pre-training (each task is to complete the next word in a similar subset of Wikipedia). But the last linear layer is shared by all ``tasks''. However, if pre-training on context-dependent tasks, with bi-directional encoder, encoding of context can be thought of as the task-specific adaptation...


\textbf{Single-task learning with neural networks.} 
A plethora of works have studied the behavior of gradient-based algorithms for optimizing neural networks on single tasks in recent years. 
% Theoretical  analyses of the behavior of gradient descent on neural networks
Many of these studies consider the neural tangent kernel (NTK) regime 
% Such analyses roughly speaking fall into one of two categories: 1) those that consider the 
\citep{jacot2018neural,arora2019exact,du2019gradient,allen2019convergence,oymak2020toward,ji2019polylogarithmic,li2018learning,du2020fewshot,zou2018stochastic,lee2019wide,chizat2019lazy},
in which a large initialization and small step size mean that early layer model weights barely change during training, so the algorithm dynamics reduce to those of linear regression on fixed features. 
% and 2) those that consider the feature learning regime. In the NTK regime, 
We are interested in the feature learning regime of training neural networks, wherein the representation weights change significantly and the dynamics are nonlinear. 

Numerous works study  feature learning in neural networks, but the vast majority consider optimizing only a single task from a particular class of functions \cite{allen2019learning,bai2019beyond,li2020learning,daniely2020learning,barak2022hidden,telgarsky2022feature,akiyama2022excess,zhou2021local,abbe2022merged}. 
% \cite{bai2019beyond} studies gradient dynamics on depth-two neural networks via a quadratic approximation. \cite{daniely2020learning,barak2022hidden,telgarsky2022feature} show that gradient-based methods can learn sparse parities with depth-two neural networks.
% \cite{akiyama2022excess} analyze a two-phase gradient-based algorithm that learns a two-layer ReLU teacher network,
% when the teacher network head parameters are $\pm 1$.
\cite{ba2022high} studies how one step of SGD improves two-layer network performance with respect to a teacher model when compared to random features as long as a large learning rate is used.
% Similarly, \cite{lewkowycz2020large,li2019towards,zhu2022quadratic} argue that large learning rate is the key to feature learning, while \cite{yang2021tensor} proposes that initializing near zero is critical. We adopt the large learning rate and small initialization in our study.
% Moreover, \cite{frei2022random} show that ReLU nonlinearity is instrumental to learning robust features with a two-layer model. 
% \cite{radhakrishnan2022feature} put forth the idea that an expected gradient outer product controls feature learning in deep fully-connected neural networks. 
% A variety of works study  whether neural networks can learn low-dimensional representations that generalize to many tasks via training on a single task.
\cite{mousavi2022neural} shows that stochastic gradient descent on a two-layer ReLU network with arbitrary width can learn a single-index task ($r=1$). \cite{damian2022neural} proves that gradient-based methods on two-layer networks can learn $r$-index  polynomials by learning a projection onto the $r$ relevant directions, and \citet{}. The closest analysis to  ours is due to \cite{shi2022theoretical}, which considers a similar data generative model and loss function to show two layer ReLU networks can learn functions of the parity of $r$ inputs. However, unlike our work, this analysis leverages activation noise and the learned features do not allow for learning more general functions of $r$ inputs.
% to show convergence to the average of the  show they can learn functions of the parity of $r$ inputs. It is not clear how these analyses generalize multi-task settings, and in fact we show in Section \ref{sec:results} that the same behavior that allows gradient descent to succeed in \citep{shi2022theoretical} causes it to fail in an analogous multi-task setting. 
Additional works consider single-task feature learning  in the mean-field regime with infinitely-wide networks \citep{chizat2018global,mei2018mean,sirignano2020mean,nguyen2019mean}.



% xx show that gradient descent on  - layer ReLU networks  can learn ...
% ways to group these:
% -algorithm
% -target function class
% -model class
%     - network width/depth

% large learning rate is the key to feature learning:
% \cite{lewkowycz2020large}
% \cite{li2019towards}
% \cite{zhu2022quadratic}

% initializing near zero is key to feature learning
% \cite{yang2021tensor}

% evaluate evolution of networks layers during GD:
% abbe, damian, shi

% \cite{mousavi2022neural}: Their only feature learning results are for the single-index model, i.e. the link function is a monomial. $O(d)$ samples required to learn single-index model. For multi-index model, they show that the component of the learned features in the orthogonal space to the ground-truth features is decreasing. 
% SGD with simultaneous updates of head and representation.

% \cite{damian2022neural}: Link function is a polynomial of $r$ inputs. $O(d^2)$ samples required to learn polynomial. Symmetric initialization and regularization trick to completely forget initial features after one step. Gaussian data, Stein's Lemma, Hermite expansion. Labels are normalized to ignore 0-th and 1st order terms. Only one step of GD to learn the features, then in subsequent steps only the head is updated. Assumption that Hessian is full-rank is critical.

% \cite{ba2022high}: Analyzes feature learning with one step of SGD. Focus is mostly on statistics induced by this one step of SGD. In proportional limit as samples, neurons, and dimension go to infinity, they show that the gradient w.r.t. W is almost rank 1, which results in the features being aligned with the linear component of the ground-truth model after one gradient step. Also shows that large learning rate is necessary to beat random features model.

% \cite{barak2022hidden}: Considers sparse parity problem: aims to learn function that is the parity of $k\ll n$ input bits, where $n$ is the length of the full input string. Show that on two-layer MLPs and disjoint-polynets, and at least $n^{O(k)}$ batch size, SGD learns the function.

% \cite{abbe2022merged}: provide a necessary and sufficient condition for sparse polynomial functions to be learnable by SGD on a two-layer neural network with $O(d)$ samples. The polynomials must satisfy a staircase property. Note that polynomials that do not satisfy this property can still be learnable with $O(d^p)$ samples where $p$ is the degree of the polynomial.

% \cite{shi2022theoretical}: Data generated from sparse coding model. Two-layer net with truncated relu activation. Hinge loss. Symmetric initialization. Infinite samples. All parameters updated simultaneously -- algorithm is truly gradient descent on the population loss. labels have nontrivial correlation with true features. Every neuron goes to the average of the true features.

% \cite{telgarsky2022feature}: Studies gradient flow and SGD on two-layer ReLU. Shows that these algorithms learn 2-sparse parities.
 
% \cite{akiyama2022excess}: two-phase GD-based algorithm that provably learns two-layer ReLU without overparameterization when teacher head parameters are $\pm 1$. First phase is Langevin dynamics, second phase is GD.

% \cite{bai2019beyond} studies two-layer neural networks with smooth activations

% \cite{daniely2020learning} sparse parities can be learned by gradient descent on depth-two neural networks





% -----------------

% nearly all consider single-task scenarios. 

% how to formally define learning: input distribution, target function class, model.


% \textbf{Multi-task learning optimization dynamics.} To my knowledge, no work has studied the dynamics of multi-task learning algorithms for learning multiple two-layer neural networks.
% Results proving the feature learning abilities of reasonably-wide neural networks trained with gradient-based methods are relatively new. Below is a summary of recent papers on this topic.

% \cite{mousavi2022neural}: Their only feature learning results are for the single-index model, i.e. the link function is a monomial. $O(d)$ samples required to learn single-index model. For multi-index model, they show that the component of the learned features in the orthogonal space to the ground-truth features is decreasing. 
% SGD with simultaneous updates of head and representation.


% \cite{damian2022neural}: Link function is a polynomial of $r$ inputs. $O(d^2)$ samples required to learn polynomial. Symmetric initialization and regularization trick to completely forget initial features after one step. Gaussian data, Stein's Lemma, Hermite expansion. Labels are normalized to ignore 0-th and 1st order terms. Only one step of GD to learn the features, then in subsequent steps only the head is updated. Assumption that Hessian is full-rank is critical.

% \cite{ba2022high}: Analyzes feature learning with one step of SGD. Focus is mostly on statistics induced by this one step of SGD. In proportional limit as samples, neurons, and dimension go to infinity, they show that the gradient w.r.t. W is almost rank 1, which results in the features being aligned with the linear component of the ground-truth model after one gradient step. Also shows that large learning rate is necessary to beat random features model.

% \cite{barak2022hidden}: Considers sparse parity problem: aims to learn function that is the parity of $k\ll n$ input bits, where $n$ is the length of the full input string. Show that on two-layer MLPs and disjoint-polynets, and at least $n^{O(k)}$ batch size, SGD learns the function.


% \cite{abbe2022merged}: provide a necessary and sufficient condition for sparse polynomial functions to be learnable by SGD on a two-layer neural network with $O(d)$ samples. The polynomials must satisfy a staircase property. Note that polynomials that do not satisfy this property can still be learnable with $O(d^p)$ samples where $p$ is the degree of the polynomial.

% \cite{shi2022theoretical}: Data generated from sparse coding model. Two-layer net with truncated relu activation. Hinge loss. Symmetric initialization. Infinite samples. All parameters updated simultaneously -- algorithm is truly gradient descent on the population loss. labels have nontrivial correlation with true features. Every neuron goes to the average of the true features.
% Proof sketch:
% \begin{enumerate}
%     \item First, they show that there exists a ground-truth two-layer truncated ReLU model that can classify the  data exactly.
%     \item Then, they again leverage the symmetric initialization to show that the ground-truth features are roughly learned in the first gradient step. 
%     \begin{itemize}
%         \item Key insight: For components of the gradient along spurious features, the label in independent of the rest of the gradient, so the expected value of this component is zero (since the labels are balanced, expected value of the label is zero). But the label is correlated with the rest of the gradient along true feature directions, so the expectation is non-trivial.
%         \item  In their single-task setting, every neuron goes to $\pm$ the average of the ground-truth features. Thus, the algorithm is only capable of learning functions of the sum of the feature coordinates, not functions of the feature coordinates in general. With multi-task learning, we should be able to disentangle the features such that each neuron goes to an individual feature rather than their sum.
%         % \item {\color{blue} Idea: In their single-task setting, every neuron goes to $\pm$ the average of the ground-truth features. This behavior seems not a product of the analysis but intrinsic to the setting (on average over initialization, the value of each neu 
%     \end{itemize}
%     \item Then they show that the features are refined in the second gradient step.
%     \item In all subsequent steps, the last-layer parameters are learned to form an accurate classifier.
% \end{enumerate}

% \cite{telgarsky2022feature}: Studies gradient flow and SGD on two-layer ReLU. Shows that these algorithms learn 2-sparse parities.
 
% \cite{akiyama2022excess}: two-phase GD-based algorithm that provably learns two-layer ReLU without overparameterization when teacher head parameters are $\pm 1$. First phase is Langevin dynamics, second phase is GD.

% \cite{bai} and lee


\textbf{Feature learning in multi-task settings.} Other works have considered feature learning in multi-task settings.  A popular theme among these works is to assume the existence of a ground-truth low-dimensional data representation shared among all tasks, and to show that the algorithm \cite{thekumparampil2021sample,collins2022maml,collins2021exploiting,saunshi2021representation,sun2021towards,chua2021fine,bullins2019generalize,chen2022active} in consideration recovers this representation. However, all of these of these algorithmic analyses are limited to linear models.
% all showed that fundamental multi-task learning algorithms can learn ground-truth low-dimensional subspaces when training linear models.  
A small number of works have studied nonlinear multitask settings.
% \cite{wu2020understanding} studies a  two-layer ReLU model from statistical perspective and provides a result showing when mutli-task learning on two tasks transfers positively to a third task.
% Depends on data covariances. Introduces covariance alignment layer inspired by result.
\cite{huang2021fl} studied the dynamics of FedAvg \cite{mcmahan2017communication}, a multi-task learning algorithm used for federated learning, but in the NTK regime, meaning they did not consider feature learning, while \cite{collins2022fedavg} demonstrates the FedAvg learns ground-truth features but only considers linear models.
\cite{deng2022local} showed that FedAvg converges to global optima of the training loss for $L$-layer ReLU models, but also did not analyze feature learning. 
% or any generalization properties.
% But does not consider generalization. Results suggest that $\tau=1$ is optimal for convergence to solution of training objective.
\citep{kao2021maml} empirically noticed a similar phenomenon as us in that adapting task-specific heads to each task induces a contrastive loss, albeit in the context of studying a particular meta-learning algorithm.
% Multi-tasking induces a contrastive loss - A previous work empirically noticed a similar phenomenon occurs for a particular meta-learning algorithm . 
Finally, \cite{maurer2016benefit,tripuraneni2020provable,du2020fewshot,tripuraneni2020theory,xu2021representation} gave statistical bounds on the downstream task loss after learning a task-specific head on top of a (possibly nonlinear) representation learned by solving an empirical risk minimization problem over a set of pretraining tasks, but did not consider the transferability of representations returned by gradient-based algorithms.

% These linear analyses can be generalized to non-linear models by lifting to infinite dimensions (e.g., see \cite{}) as in the standard kernel analysis, such as the NTK.
% However, such a lifting requires paying a penalty in terms of the induced infinite-dimensional covariance which may be arbitrarily large.
% Ours is the first analysis without recourse to such lifting.



% \citep{wu2020understanding} 

% \citep{chua2021fine} linear

% \citep{bullins2019generalize} linear

% \cite{wang2021bridging} bo li papr

% \cite{chen2022active} active multitask representation learning - linear

% \cite{maurer2016benefit}



==> Results-ICML-long.tex <==
\section{Theoretical Results} \label{sec:results}

\textbf{Feature learning guarantees.}
% In this section we discuss our main results. 
We start by showing that the gradient-based multitask learning algorithm described in the previous section recovers the ground-truth features.
To do this, we first need the following proposition, which shows that the projection of the initial features $\mathbf{W}_0$ onto the subspace spanned by the label-relevant, or ground-truth, features stays roughly the same after one step, while their projection onto the subspace spanned by the spurious features becomes very small. 

Here, we let $\Pi_{\parallel}(\mathbf{W})\coloneqq \mathbf{W}\mathbf{M}^\top\mathbf{M}$ denote the projection of the rows of the matrix $\mathbf{W}$ onto the ground-truth subspace, and $\Pi_{\perp}(\mathbf{W})\coloneqq \mathbf{W}\mathbf{M}_{\perp}^\top \mathbf{M}_{\perp}$ denote the projection onto the spurious subspace. 
For brevity, we abbreviate the statements of the theoretical results in this section and defer the full versions, along with their proofs, to the Appendix.
\begin{proposition} \label{prop:1}
% {\color{red}{I think it would make the theorems more self-contained if you remind the reader about the definition of $m$, $n_2$, T, ... . at least in this result which is the first formal result. by now the reader for sure don't recall what $n_1$ and $n_2$ stand for}}
    Consider the gradient-based multitask algorithm described in Section~\ref{sec:alg} that uses $T$ tasks and $(n_1,n_2)$ samples per task to update the (head, representation), respectively,  and suppose Assumption \ref{assump:diversity} holds. Further assume  $d=\tilde{\Omega}( r^4)$, $m= o(\exp(d))$,
and define $\epsilon \coloneqq {O}\left(\frac{d \sqrt{\log(Tn_2)}}{\sqrt{Tn_2}} \left(1 + {\tfrac{ \sqrt{\log(T)}}{\sqrt{n_1}}}\right) + \tfrac{  \sqrt{d} \log(d)}{\sqrt{T}}\right)$.
Then there is some setting of the parameters $\eta,   \lambda_{\mathbf{w}}$ and $\nu_{\mathbf{w}}$
% $\eta = \Theta(1)$, $\lambda_{\mathbf{a}} = 1/\eta $, $\lambda_{\mathbf{w}} = (1+(\eta^2 2^{-r-1})/\pi)/\eta$, and $\nu_{\mathbf{w}} = O(d^{-1.25})$. % and $\sigma_b = O(d^{-1.25})$. 
%$m = \Omega(r 2^r)$, 
% For a subset ${S}\subseteq [m]$, let $\mathbf{W}_{1,S}\in \mathbb{R}^{|S|\times d}$ denote the sub-matrix of $\mathbf{W}$ with rows selected by $S$.
such that with probability at least $0.99$,
% over the random initialization,
% there is a subset of neurons ${S}\subseteq [m]$ of size $|{S}| \geq m/4$ such that for all $j \in {S}$:
% the following two properties are satisfied by the representation learned by MTRL:
% \begin{enumerate}[leftmargin=2mm]
% \item 
\vspace{-2mm}
\begin{align}
    &1. \quad  \tfrac{1}{\nu_{\mathbf{w}}\sqrt{m}}\|\Pi_{\parallel}(\mathbf{W}^1) -  \tfrac{1}{2^{r-2}} % \frac{\eta^2}{2^{r+2}} 
\Pi_{\parallel}(\mathbf{W}^{0}) \|_2 \nonumber \\
&\quad \quad \quad\quad \quad \quad \quad \quad \quad \;\;\; =  O\left(  
\tfrac{r^4 + \log^4(m)}{2^r d} + \epsilon\right) \nonumber \\
&2. \quad \tfrac{1}{\nu_{\mathbf{w}}\sqrt{m}}\|\Pi_{\perp}(\mathbf{W}^{1}) \|_2 = O\left(
\tfrac{r^{3.5} + \log^{3.5}(m)}{2^r d^{1.5}} %+ \eta\sigma_w d^{1.5} e^{-d^2/8} 
    + \epsilon\right). \nonumber
\end{align} %+ \eta \sigma_w d^{1.5} e^{-d^2/8}
% +    \frac{d \sqrt{\log(Tn_2)}}{\sqrt{Tn_2}} \left(1 + {\tfrac{ \sqrt{\log(T)}}{\sqrt{n_1}}}\right) + \tfrac{  \sqrt{d} \log(d)}{\sqrt{T}}
% \frac{\sqrt{r}d}{\sqrt{T}}
% \eta^2\frac{r^4}{d} %+ \eta \sigma_w d^{1.5} e^{-d^2/8}
% + \eta \frac{\sqrt{r}d}{\sqrt{n}}


% (and scales with init)
% $\|\mathbf{W}_1 - \eta 2^{-r-2} \mathbf{M}_{:r}\mathbf{M}_{:r}^\top \mathbf{W}_0\| =  +  O\left(\sqrt{\frac{r}{d-r}}\right)$
    % \item $
    % \frac{\sqrt{r}d}{\sqrt{T}}
    % $
    %     \eta^2 \sigma_w\frac{r^{3.5}}{d^{1.5}2^r} %+ \eta\sigma_w d^{1.5} e^{-d^2/8} 
    % + \eta \sigma_w\frac{\sqrt{r}d}{\sqrt{n}}
    % \item For all $\mathbf{v}\in \{-1,1\}^r$, $\exists j \in \mathcal{S}$ such that $\mathbf{w}_{1,j}^\top \mathbf{v} + b_{1,j} > 0$
    % $\sigma_{\min}(\mathbf{W}_1)$
% \end{enumerate}
\end{proposition}
% Note that the error terms in the RHS 
% \textcolor{blue}{I think in the above theorem you should specify what the "poly" is.}
Proposition \ref{prop:1} shows that w.h.p. over the random initialization, the weights learned by the gradient-based multitask learning algorithm satisfy two properties, for sufficiently large $T, n_1, n_2$ and $d$\footnote{A lower bound is required on $d$ to ensure that the projection of the gradient onto the $d\!-\!r$ spurious features approximates its expectation; e.g. see Equation \ref{rowp2} in Section \ref{sec:sketch}.}: (1) the projection of these weights onto the ground-truth subspace is close to a slightly scaled down (by a factor of $2^{-r}$) version of their projection at initialization, and (2) their projection onto the spurious subspace is negligible. These two observations, combined with the fact that the neuron weights have independent standard Gaussian initializations, imply that  the projection of the neuron weights onto the ground-truth subspace dominates their projection onto the spurious subspace. We formalize this observation in the statement below. 

% Let $\sigma_{\min}(\Pi_{\parallel}(\mathbf{W}^+{0}))$ denote the minimum singular value of $\Pi_{\parallel}(\mathbf{W}^{0})$, then since initially the minimum singular value $\sigma_{\min}(\Pi_{\parallel}(\mathbf{W}^{0}))\gtrsim \sigma_w\sqrt{mr}$ with high probability due to the Gaussian initialization, we require that 
%  $d \gg r^4$ and $T \gg d^2 2^{2r}$ 
 
%  in order for the energy in  projection onto the ground-truth spurious subspace to dominate the projection onto the spurious subspace. 


%as long as $d\gg r$ and $n \gg d^2 2^r$
% if you condition on this then you no longer have gaussian
% if you remove thse then you no longer have gaussian
% probability you can't throw away neurons. because you don't know the value of their projections
% say that you have 
% workst case scenariom m e^{c^2r} need to choose $c = sqrt(log(m))/sqrt$  

% have large energy ($\Omega(1)$) in the subspace spanned by the label-relevant features ($\text{col}(\mathbf{M}_{:r})$) and small energy $O(d^{-1/2})$ in the subspace of spurious features ($\text{col}(\mathbf{M}_{r:})$). Moreover, Part 3 of Theorem 1 implies that the learned weights are nearly isotropic within the ground-truth $\text{col}(\mathbf{M}_{:r})$.  Effectively, after one step have a random features model with $m$ features on the $r$ label-relevant inputs rather than the ambient $d$ inputs with $d-r$ of them being spurious. 
% \textcolor{blue}{I feel that you need to expand this in words a bit more -- right now it's not easy for the reader to understand the message exactly. e.g. spurious features vanish, and all the relevant features are recovered (maybe with a scaling)? }
% \begin{proof}
    
% \end{proof}
% pick

% union bound over 2^2^r things. this means m scales up by 2^r. which is fine because complexity of error in first prop is log(m)

\begin{theorem}[  ]\label{thm:1}
    Consider the setting in Proposition \ref{prop:1}  with $d =\tilde{\Omega}( r^4 )$, $m = o(\exp(d))$, and $\epsilon$ defined the same way.
    Further suppose $m = \Omega(r)$, $ T = \tilde{\Omega}( 2^{2r} d ) $ and $Tn_2 = \tilde{\Omega}(2^{2r} d^2)$. Let $\sigma_r(\mathbf{B})$ denote the $r$-th singular value of the matrix $\mathbf{B}$.
Then with probability at least $0.99$ over the random initialization,
% , we have 
\begin{align}  
    \frac{\sigma_1( \Pi_{\perp}(\mathbf{W}^1)) }{\sigma_{r}( \Pi_{\parallel}(\mathbf{W}^1) )} = O\left( \tfrac{ {r^{3.5}} + \log^{3.5}(m) }{ d^{1.5} } +  2^r \epsilon \right). \nonumber
\end{align}
\vspace{-2mm}
\end{theorem}
Theorem \ref{thm:1} characterizes the representation learned by multitask pretraining in an intuitive manner.  For $d \gg r^4$, $ T \gg 2^{2r} d $ and $Tn_2 \gg 2^{2r} d^2$, we have ${\sigma_{r}( \Pi_{\parallel}(\mathbf{W}^1) )} \gg \sigma_1( \Pi_{\perp}(\mathbf{W}^1) )$, meaning that most of the energy in each neuron weight is in the column space of the ground-truth subspace. This is equivalent to saying that applying $\mathbf{W}^1$ to an input $\mathbf{x}$ essentially projects it onto the ground-truth subspace spanned by the rowspace of $\mathbf{M}$, as desired.
% The key mechanism behind the ability of MTRL to recover the ground-truth features is its task-specific adaptation of the heads, as we discuss below and in Section \ref{sec:sketch}.
% characterizes the representation learned by multitask pretraining in an intuitive manner .

% (for hypercube, 2. is $O(\eta 2^r/d^{1/2})$)
% $\lambda_1 = \Theta(1)$ 
% \end{theorem}



% A sketch of the proof is provided in Section \ref{sec:sketch} and the full proof is deferred to Appendix \ref{app:thrm1}. 

% It turns out that 
% 

% Difficulty of finite-sample analysis: dealing with non-smooth objects. can't canoncentrate over tasks without having infinite samples first. but to get infinite samples, need to know something about the finite tasks. doable but not trivial


\begin{comment}

\textbf{The importance of adapting the head to each task.} We show in Section \ref{sec:sketch} that adapting the head to each task prior to updating the representation leads to a contrastive loss that encourages feature learning. Here we provide a negative result, describing a failure case when the head is not adapted to each task and we fail to learn the true features. In particular,  we show that SMGD cannot be guaranteed to recover the ground-truth features. Recall that SMGD solves the single-model objective \eqref{obj_glob} via gradient descent. 
\begin{theorem}[Negative Result]\label{thm:negative} Consider a setting with $r=2$ and two tasks with labelling functions:
\begin{align}
    \bar{f}_1^\ast(\sign(\mathbf{z}_{:2})) &\coloneqq \begin{cases} 1 & \text{if } \; z_1 > 0\\
    -1 & \text{otherwise}\\
    \end{cases}, \quad 
    \bar{f}_2^\ast(\sign(\mathbf{z}_{:2})) \coloneqq \begin{cases} 1 & \text{if } \; z_2 > 0\\
    -1 & \text{otherwise.}\\
    \end{cases} \nonumber 
\end{align}
Note that $\bar{\mathcal{T}} = \{\bar{f}_1^*, \bar{f}_2^*\}$ satisfies Assumption \ref{assump:diversity}. Suppose $(\mathbf{W}_T,\mathbf{b}_T,\mathbf{a}_T)$ is a stationary point of the dynamics of SMGD.
% $\mathbf{w}_{j,0}^{\text{SMGD}}\sim N(\mathbf{0}_d,\nu^2\mathbf{I}_d)$  for all $j \in [m]$, and $\mathbf{a}_0^{\text{SMGD}}\sim N(\mathbf{0}_m,\alpha^2\mathbf{I}_m)$, for any $\nu\geq 0,\alpha\geq0,\eta\geq 0,\lambda_1\geq0,\lambda_2\geq 0$, 
Then, 
\begin{align}
   \mathbf{W}_T\mathbf{e}_{1} &= \mathbf{W}_T\mathbf{e}_{2}.
\end{align}
% with probability at least $1 -$ over the random initialization.
\end{theorem}
% // or argue about stationary points. get rid of initialization
Theorem \ref{thm:negative} shows that SMGD can only learn a strict subset of the ground-truth two-dimensional subspace: its intersection with the (one-dimensional) span of $\mathbf{Me}_1+\mathbf{Me}_2$. The, the features it learns are not sensitive to changes in ..  as long as their sum is the same

 
The key to the proof is to notice that the gradient for any neuron weights can be written as
\begin{align}
    \nabla_{\mathbf{w}_j}\mathcal{L}(\mathbf{W},\mathbf{a}) &= \frac{a_j}{2}(1 + \mathbb{E}_{\mathbf{v}}[v_1v_2 \sigma'(\mathbf{v}^\top  \mathbf{w})]) (\mathbf{e}_1 +\mathbf{e}_2) + \frac{a_j}{2}\sum_{\ell=3}^k \mathbb{E}_{\mathbf{v}}[(v_1+v_2) v_\ell \sigma'(  \mathbf{v}^\top  \mathbf{w}_{})] \mathbf{e}_\ell  
\end{align}
thus the gradient only depends on the ground-truth features $\mathbf{e}_1, \mathbf{e}_2$ through their sum $\mathbf{e}_1 + \mathbf{e}_2$. This observation was also made by \cite{shi2022theoretical}, who showed that gradient descent learns the sum of the ground-truth features in the single-task sparse coding setting, which is sufficient to generalize to tasks whose labels are functions of the sum of the latent coordinates, but not the much larger set of tasks that are functions of individual latent coordinates.

\textcolor{blue}{This part is good.}

\end{comment}

% {\color{red}
% \subsection{Downstream Guarantees}

% From Theorem \ref{thm:1}, we have 
% \begin{align}
%     \mathbf{W}_1 &= \eta \mathbf{M}_{:r}\mathbf{M}_{:r}^\top \mathbf{W}_0 + \eta \mathbf{N}_0
% \end{align}
% where each row of $\mathbf{N}_0$ satisfies $\|\mathbf{n}_{0,j}\|_2 = O\left(\tfrac{\|\w_{0}\|_2}{k}\right)$. 


% We consider
% \begin{align}
%     \mathcal{T}^{\text{eval}} \coloneqq \{f^* : \mathbb{R}^k \rightarrow \{-1,1\} \; \text{s.t.}  \}
% \end{align}

% Need to show improvement over random features and single task learning, thus need to quantify sample complexity and/or neuron complexity.

\textbf{Downstream performance.} Now that we have shown that the learned representation recovers the ground-truth subspace, we use this result to show that the representation generalizes to downstream tasks. We consider downstream tasks with input data sharing the same label-relevant $r$ features as the pretraining tasks, but here the input data is  on the hypercube. In particular, input data points $ ( \mathbf{v}, f_{T+1}(\mathbf{v}) ) $ are generated by the downstream task $T+1$ as follows:
\begin{align}
 \mathbf{v} \sim \text{Unif}(\mathcal{H}^d),\quad   
 % \mathbf{x} = \mathbf{Mv}, \quad 
 {f}_{T+1}(\mathbf{v}) = g_{T+1}(\sign(\mathbf{Mv})) \in \{-1,1\} \nonumber%\label{down}
\end{align}
% where, as for pretraining, $g_{T+1} :\mathcal{H}^r \rightarrow \{-1,1\}$. 
We formally show below that the learned features generalize to {\em any} such link function $g_{T+1}$.



% \begin{theorem}[End-to-end Guarantee] \label{thm:downstream}
% Let $\mathbf{W}_1$ be the weight matrix learned by multitask pretraining with $n$ tasks drawn from a collection of tasks satisfying Assumption \ref{assump:diversity}.
% Construct the three-layer ReLU neural network ${g}(\cdot, \boldsymbol{\theta}_1)$ using re-scaled $\mathbf{W}_1$ for first layer weights as in  \eqref{F} and the task-adapted head $\mathbf{a}_{n+1}$ from \eqref{ada}.
% For any downstream task $\mathcal{D}_{n+1}$ described in \eqref{down}, with labeling function $\bar{f}_{n+1}^*$ being any mapping from $\{-1,1\}^r \rightarrow \{-1,1\}$, sample a set $\mathcal{S}_N \coloneqq \{\mathbf{x}_l, {f}_{n+1}^*(\mathbf{x}_{l})\}_{l=1}^N$ of $N$ i.i.d. samples from $\mathcal{D}_{n+1}$.
% % If $ d = \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  )) $, $n = \Omega( d^3 \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  ))  )$,
% % $m = \Theta(r^4\log^8(r) ({ r} + {\log(1/\delta)}))$,  $\hat{m}= \Omega( r^{3.5} \log^4(r) \exp\left( C \log^6(r) r^5 \log(\log(r)/\delta) ) \right) \log(1/\delta) )$, and 
% For any $\delta,\delta'\in (0,1)$ and $ d = \exp(\tilde{\Omega}( r^6  )) $, $n = d^3 \exp(\tilde{\Omega}( r^6  )  )$,
% $m = \tilde{\Theta}(r^6)$,  and $\hat{m}= \exp\left( \tilde{\Omega}(r^6)  \right)$,
% with probability at least $0.99-\delta - \delta'$ over the random  initializations, draw of $n$ pretraining tasks, and draw of $\mathcal{S}_N$,
% \begin{align} % note: r^6 may be lose. for a single task, it is definitely r^5. but we want to generalize to all 2^r tasks
%         \mathcal{L}^{(\text{eval})}_{n+1}(\boldsymbol{\theta}_1,\mathbf{a}_{n+1}) &= 
%         % \tilde{O}\left(\frac{ r^{5} \log^8(r) \log(1/\delta')}{ \sqrt{N}}\right).
%          \left(\frac{ \exp(\tilde{O}(r^6)) }{ \sqrt{N}}\right), 
%     \end{align}
%     where $\tilde{\Omega}(\cdot),\tilde{\Theta}(\cdot)$ and $\tilde{O}(\cdot)$ hide logarithmic factors in $r$, $\delta^{-1}$ and $(\delta')^{-1}$.
%     % with probability at least $1-\delta - $
% % \frac{(\hat{\gamma}=   r^{2.5} \log^4(r) )\log(1/\delta)}{(\lambda_{\mathbf{a}}=1/\hat{\gamma}) \sqrt{N}}
% \end{theorem}
\begin{theorem}[End-to-end Guarantee] \label{thm:downstream}
Let $\mathbf{W}^1$ be the outcome of the multitask representation learning algorithm described in Section \ref{sec:alg} on the task distribution $\mathcal{T}(\mathbf{M})$, where $\mathcal{T}$ satisfies Assumption \ref{assump:diversity}. 
% \textcolor{blue}{can you be more specific here about what you mean by "learned". I think $W_1$ is just the outcome of the algorithm. If yes, maybe it's better to say it here?}
Consider a downstream task in the support of $\mathcal{T}(\mathbf{M})$ with link function $g_{T+1}$.
% being a mapping from $\{-1,1\}^r \rightarrow \{-1,1\}$. 
% Let $\mathcal{S}_N \coloneqq \{\mathbf{x}_l, {f}_{n+1}^*(\mathbf{x}_{l})\}_{l=1}^N$ be a set of $N$ i.i.d. samples from $\mathcal{D}_{n+1}$.
Construct the two-layer ReLU embedding $\phi$ using the rescaled $\mathbf{W}^1$ for first layer weights as in  \eqref{F}, and train the task-adapted head $(\mathbf{a}_{T+1},\tau_{T+1})$ using $N$ i.i.d. samples from the downstream task.
% , as in \eqref{ada}.
% 
% If $ d = \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  )) $, $n = \Omega( d^3 \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  ))  )$,
% $m = \Theta(r^4\log^8(r) ({ r} + {\log(1/\delta)}))$,  $\hat{m}= \Omega( r^{3.5} \log^4(r) \exp\left( C \log^6(r) r^5 \log(\log(r)/\delta) ) \right) \log(1/\delta) )$, and 
 Further, suppose $ d = \exp(\tilde{\Omega}( r^5  )) $, $T = d^2 \exp(\tilde{\Omega}( r^5  )  )$, $Tn_2 = d^3 \exp(\tilde{\Omega}( r^5  )  )$, $n_1 = \Omega(\log(T))$ % $\min(n_1,n_2)=\Omega(1)$,
$m = \tilde{\Theta}(r^5)$,  and $\hat{m}= \exp\left( \tilde{\Omega}(r^5)  \right)$.
Then for any $\delta \in (0,0.99)$, with probability at least $0.99-\delta$,
% over the random  initializations, draw of $T$ pretraining tasks, and draw of $N$ samples from the downstream task, 
% we have
\begin{align}
\vspace{-2mm}
        \mathcal{L}^{\text{eval}}_{T+1} %(\boldsymbol{\theta}_1,\mathbf{a}_{T+1}) 
        &= 
        % \tilde{O}\left(\frac{ r^{5} \log^8(r) \log(1/\delta')}{ \sqrt{N}}\right).
       \frac{ \exp(\tilde{O}(r^5)) }{ \sqrt{N}}, 
       \vspace{-2mm}
    \end{align}
    where $\tilde{\Omega}(\cdot),\tilde{\Theta}(\cdot)$ and $\tilde{O}(\cdot)$ hide log factors in $r$ and $\delta^{-1}$.
    %and $(\delta')^{-1}$.
    % \textcolor{blue}{don's see why you need both $\delta$ and $\delta'$. CAn you just use a single $\delta$ for $\delta + \delta'$? }
    % with probability at least $1-\delta - $
% \frac{(\hat{\gamma}=   r^{2.5} \log^4(r) )\log(1/\delta)}{(\lambda_{\mathbf{a}}=1/\hat{\gamma}) \sqrt{N}}
\end{theorem}
Theorem \ref{thm:downstream} confirms that the features learned by multitask pretraining generalize to {\em any} downstream task mapping from $\mathcal{H}^d$ to $\{-1,1\}$ that has the same representation as the pretraining tasks, i.e., its labels are a function of the input's projection onto the rowspace of $\mathbf{M}$. In particular,
if we compose the learned representation with  a random ReLU layer, then learn a linear head using $\exp(\tilde{O}(r^5))$ samples from the task, we solve the task with high probability (w.h.p.).
Critically, the number of samples and neurons  needed to solve the downstream task w.h.p. are independent of the ambient dimension  $d$. 
% In other words,  multitask learning reduces the effective dimension of the downstream task  from $d$ to $r$. 
% Since the motivating assumption

 % are generalizable by showing that they can yield a network that 
 % efficiently solves \textit{any} downstream task with latent coordinates on the hypercube, 
 % after adding a random ReLU layer and a trained head. Most importantly, the complexity of solving the new task is independent of dimension

%  \begin{align}
%     \mu &= \Theta (r^{-2.5} \log^{-3}(r) \exp( -C \log^6(r) r^5 \log(\log(r)/\nu) )) \nonumber \\
%     m &= \Theta( r^4\log^8(r) ({ r} + {\log(1/\nu)})) \nonumber \\
%     \hat{m} &= \Theta\left(r^{3.5} \log^4(r) \exp\left( C \log^6(r) r^5 \log(\log(r)/\nu) ) \right) \log(1/\nu)\right) \\
%     &O\left(\left(\frac{r^{4}}{\sqrt{d}} +  d^2 e^{-d^2/8} + \frac{\sqrt{r}d^{1.5}}{\sqrt{n}}\right)(\frac{\sqrt{m}}{\sqrt{\hat{m}}})\right) \\
%     &\rightarrow
% \end{align}


The proof of Theorem \ref{thm:downstream} leverages Proposition \ref{prop:1} to show that the embedding  generated by multitask learning is close to the embedding of a coupled, ``purified'' two-hidden layer random ReLU network whose first layer weights project the input {\em exactly} onto the rowspace of $\mathbf{M}$. Then, the proof applies  Theorem 2 from \citet{dirksen2022separation} which implies that w.h.p. the purified network linearly separates two classes of points on $\mathcal{H}^r$ with margin and neuron complexity scaling as functions of the input dimension $r$. The representation learning error from Proposition \ref{prop:1} is  smaller than this margin due to the lower bounds on $T$, $n_1, n_2$,  and $d$ in Theorem \ref{thm:downstream}, so the learned network also linearly separates the two classes w.h.p. Then, the proof invokes a standard linear classification generalization bound to control the final error in learning the head \cite{Livni_2017}.
% Alternatively, we could apply the results on linear separation capabilities of random two-layer ReLU networks in \cite{ghosal2022randomly} without needing to add an extra hidden layer, but doing so would require $\Omega(\exp(2^r))$ samples and neurons. 
% The full proof is found in Appendix \ref{app:down}.
% \citep{hsu2021approximation}

\begin{comment}
While Theorem \ref{thm:downstream}  ensures generalization to an arbitrary task sharing the ground-truth features, it can only guarantee generalization to a single such task at once. To ensure that the learned embedding generalizes to a larger set of tasks simultaneously, we have the following corollary.
\begin{corollary}[Generalization to set of tasks] \label{cor:set}
Consider a set  of possible downstream tasks $\mathcal{S}^{\text{eval}}$ with $|\mathcal{S}^{\text{eval}}| = D$. Suppose $ d = \exp(\tilde{\Omega}( r^5 \log(D) )) $, $T = d^3 \exp(\tilde{\Omega}( r^5 \log(D)  )  )$,
$m = \tilde{\Theta}(r^5 \log(D) )$,  and $\hat{m}= \exp\left( \tilde{\Omega}(r^5 \log(D) )  \right)$. Construct the two-layer ReLU embedding as in \eqref{F}. Then with probability at least $0.99-\delta$,  any task $T\!+\!1$ in $\mathcal{S}^{\text{eval}}$ 
satisfies
% compute $(\mathbf{a}_{T+1},\tau_{T+1})$ using $n$ samples from task $T+1$,
\begin{align}
        \mathcal{L}^{\text{eval}}_{T+1} %(\boldsymbol{\theta}_1,\mathbf{a}_{T+1}) 
        &= 
        % \tilde{O}\left(\frac{ r^{5} \log^8(r) \log(1/\delta')}{ \sqrt{N}}\right).
       \frac{ \exp(\tilde{O}(r^5 \log(D))) }{ \sqrt{N}}, 
    \end{align}
    where $\tilde{\Omega}(\cdot),\tilde{\Theta}(\cdot)$ and $\tilde{O}(\cdot)$ hide log factors in $r$ and $\delta^{-1}$. 
    % \textcolor{blue}{same comment as above about $\delta$}
\end{corollary}
For example, if $\mathcal{S}^{\text{eval}}$ is the set of all $2^{2^r}$ functions from $\mathcal{H}^r$ to $\{-1,1\}$ (the support of $\mathcal{T}_{\text{all}}$), then Corollary \ref{cor:set} shows that multitask pretraining learns a representation that for all such target functions yields an accurate classifier with $O(\exp(\exp(r)))$ sample and neuron complexity, which is independent of the ambient dimension $d$.
\end{comment}

\subsection{Negative Results}

Next, we present two negative results that underscore the tightness of our findings in the previous section. The first result emphasizes the significance of representation learning in achieving strong generalization guarantees. The second result highlights the importance of multi-task learning by demonstrating that single-task learning may fail to capture all critical features.



\textbf{Random features do not generalize.} A consequence of Theorem \ref{thm:downstream} is that multitask pretraining improves the sample and neuron complexity of solving downstream tasks by an exponential factor in $d$. 
To show this, we consider sparse parity tasks,  and show that learning a linear classifier on top of random features
% not knowing the sparse features on which the task is defined 
entails exponential complexity in $d$ to solve the task.
% We have introduced sparse parity tasks \eqref{sparsepar}, however in \eqref{sparsepar}, $\mathcal{T}_{\text{s.p.}}$ was defined as the set of sparse parity tasks mapping from a {\em fixed} set of $r$ features, that is, the set of sparse parity tasks on a fixed ground-truth representation.
Now, there is no feature learning, so the learner has no knowledge of which few features are relevant and needs to consider tasks on all $d$ inputs.
% We model this by considering the set of sparse parity tasks on $r$-dimensional subsets of $d$ inputs, meaning each task $i$ is associated with a unique  representation $\mathbf{M}_i$ that selects $r$ coordinates of a Boolean input vector
We model this by considering a set of tasks sharing a single link function but having many distinct representations.
We consider a smaller class of representations than in our positive results: here $\mathbf{M}$ belongs to $\mathbb{O}^{r\times d}_{\{0,1\}}\coloneqq \{\mathbf{M}: \mathbf{M}\in \mathbb{O}^{r\times d}, \mathbf{M}\in \{0,1\}^{r\times d} \}$, that is, the rows of $\mathbf{M}$ are standard basis elements. The single link function we consider is the parity function on $r$ inputs, namely $g^{(r)}(\mathbf{v})\coloneqq (-1)^{\sum_{j =1}^r \chi\{{v}_j = -1\}}$.

% \footnote{This restricts the class of possible ground-truth representations $\mathbf{M}$ to matrices whose rows are a subset of the standard basis, whereas our positive results concern the harder problem of learning a continuous representation $\mathbf{M}$.}. This task set is formally defined as:
% \begin{align}
%     \mathcal{S}_{\text{s.p.}}\! &:= \{ g_i\!: g_i(\mathbf{v})= \bar{g}_i(\mathbf{M}_i\mathbf{v}) \!=\! (-1)^{\sum_{j =1}^r \chi\{(M_i{v})_j = -1\}},\nonumber \\
%         &\quad\quad
%         % \mathcal{S}_i \subseteq [d], |\mathcal{S}_i|=r,
%         % 
%         \mathbf{M}_i\in \{0,1\}^{r\times d}, \mathbf{M}_i \in \mathbb{O}^{r\times d},
%         \; \forall \; \mathbf{v}\in \mathcal{H}^d  \}
%         \label{sp2}
% \end{align}
   % \begin{align}
   %      \mathcal{T}_{\text{s.p.}} \coloneqq &\;\text{Unif}(\{ g_i: g_i(\mathbf{v}) = (-1)^{\sum_{j \in \mathcal{S}_i} \chi\{{v}_j = -1\}},\nonumber \\
   %      &\quad\quad \quad \quad \;\; \mathcal{S}_i \subseteq [r],\; \forall \; \mathbf{v}\in \mathcal{H}^r  \}).\label{sparsepar}
   %  \end{align}
% , i.e. the support of the task distribution $\mathcal{T}_{\text{s.p.}}$ defined in \eqref{sparsepar}.
% we consider the well-studied problem of learning sparse parities, which are functions that output the parity of a small subset of input bits. Formally, for  $\mathbf{u}\in \{0,1\}^d$ with $\|\mathbf{u}\|_1 = r$, an $(r,\mathbf{u})$-sparse parity task is defined as follows.
% \begin{definition}
%     [$(r,\mathbf{u})$-sparse parity task]
%     An $(r,\mathbf{u})$-sparse parity task $\mathcal{D}_{\mathbf{u}}$ has data $(\mathbf{v},f_{\mathbf{u}}(\mathbf{v}))$ generated as
% $
%         \mathbf{v}\sim \text{Unif}(\{-1,1\}^d )$ and $f_{\mathbf{u}}(\mathbf{v}) = (-1)^{\mathbf{u}^\top \mathbf{v}},
%     $
%     where $\mathbf{u}\in \{0,1\}^d$ with $\|\mathbf{u}\|_1 = r$.
% \end{definition}
% In other words, an $(r,\mathbf{u})$-sparse parity task has labels being the parity of the number of $-1$'s among the bits selected by the $r$-sparse vector $\mathbf{u}$.
% The sparse parity problem is then 
% Canonical results show that solving an $(r,\mathbf{u})$-sparse parity task requires $\Omega(d^r)$ samples in the Statistical Query (SQ) model \cite{} and $\Omega(\poly(d))$ noiseless samples via Gaussian elimination. 
While there is a large literature demonstrating the hardness of learning sparse parities in various settings \cite{kearns1998efficient,abbe2020poly,telgarsky2022feature,barak2022hidden,malach2022hardness,kamath2020approximate,goel2019time}, the most relevant results to our setting show that any data-independent, $\hat{m}$-dimensional embedding of $d$ inputs can admit linear classifiers that solve all sparse parity tasks on subset only if the dimension $\hat{m}$ and/or the classification margin is exponentially large (small, respectively) in $d$.
% , including the two-layer ReLU representations, as well as the neural tangent kernel \cite{jacot2018neural},  requires 
In particular, the following result adapts Theorem 5 in \cite{barak2022hidden}, which in turn draws on the works of \citet{kamath2020approximate} and \citet{malach2022hardness}.
% Holds for any embedding mapping from $\mathbb{R}^d$ to $\mathbb{R}^{\hat{m}}$, 
\begin{theorem}[] \label{thm:lower}
Consider any embedding $\Psi:\{-1,1\}^d \rightarrow \mathbb{R}^{\hat{m}}$ such that $\|\Psi(\mathbf{v})\|_2 \leq 1 $ for all $\mathbf{v}\in \mathcal{H}^d$. 
For % $\mathbf{v}\sim \text{Unif}(\mathcal{H}^d)$ and 
any $\epsilon >0$, if 
$ \hat{m}B^2 \leq \epsilon^2 \binom{d}{r}, $
then there exists a %n $(r,\mathbf{u})$
representation $\mathbf{M} \in \mathbb{O}^{r\times d}_{\{0,1\}}$
% sparse parity task $g_i\in \mathcal{S}_{\text{s.p.}}$ 
such that: % $\mathcal{D}_{\mathbf{u}}$ s.t.
\vspace{-2mm}
    \begin{align}
        \inf_{\mathbf{a}: \|\mathbf{a}\|_2 \leq B } \mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^d)}
        % {(\mathbf{v},f_{\mathbf{u}}(\mathbf{v}))\sim \mathcal{D}_{\mathbf{u}}} 
        \left[ \ell \left(\mathbf{a}^\top \Psi(\mathbf{v}), g^{(r)}(\mathbf{Mv})\right)   \right]  &\geq 1 - \epsilon.\nonumber
    \end{align}
    \vspace{-3mm}
\end{theorem}
Theorem \ref{thm:lower} implies that any random feature model requires a number of neurons and/or margin that is exponentially large (small, respectively) in $d$ in order to solve a downstream sparse parity task with a linear classifier. Note that the margin (i.e. inverse of $B$ in Theorem \ref{thm:lower}) is inversely proportional to the number of samples that are required to learn the classifier \cite{Livni_2017}. On the other hand, Theorem~\ref{thm:1} guarantees that  after multitask pretraining, the output embedding admits a linear classifier that solves any sparse parity task  on the extracted $r$ features, with the number of neurons and samples of the downstream task of the order of $\exp(\poly(r))$. 


% While our analysis does assume infinite samples for the multitask representation learning phase, it is not required to solve an $r$-sparse parity task during this phase. 

% \textbf{Lower bound: }

% I think we can get rid of second relu layer.... each neuron is the indicator for some input, covers all inputs with r2**r neurons... no, because the bias needs to be exact learned...
\textbf{Single task does not suffice for  feature learning.} Although Theorem \ref{thm:lower} shows that feature learning is essential for generalization in our setting, we have not yet shown that effective feature learning necessitates pretraining on {\em multiple} tasks. We address this issue next.  
% We first show that multitask training is necessary for learning a generalizable representation, since with high probability over a single task drawn from $\mathcal{T}_{\text{s.p.}}$, training on this single task cannot lead to learning all $r$ ground-truth features.
\begin{theorem}\label{thm:single}
    % Suppose $\mathcal{T} = \mathcal{T}_{\text{s.p.}}$.
    % and $\mathcal{S}^{\text{eval}} = \{ g_i: g_i(\mathbf{v}) = v_i,\; i \in [r],\; \forall \; \mathbf{v}\in \mathcal{H}^r\}$. 
    % any algorithm for pretraining with any number of samples cannot produce a model that 
    % contains information about all $r$ ground-truth features, in the sense that this model 
    % requires at least $d$ samples
    % from the downstream task to guarantee loss smaller than $0.5 -\epsilon$ for any $\epsilon>0$ in the worst case over downstream tasks in $\mathcal{S}^{\text{eval}}$.
    % Consider 
    Consider any embedding $\Psi:\{-1,1\}^d \rightarrow \mathbb{R}^{\hat{m}}$ such that $\|\Psi(\mathbf{v})\|_2 \leq 1 $ for all $\mathbf{v}\in \{-1,1\}^d$ that is trained on arbitrarily many samples from a single task drawn from $\mathcal{T}_{\text{s.p.}}(\mathbf{M})$.  Then there exists an $\mathbf{M}\in \mathbb{O}^{r\times d}$ such that for any $k\in[r]$, with probability at least $1 - 2^{-r}\sum_{j=k}^r\binom{r}{k} $ over the single task drawn from $\mathcal{T}_{\text{s.p.}}(\mathbf{M})$, 
for any $\epsilon >0$, 
$ \hat{m}B^2 > \epsilon^2 \binom{d-k+1}{r-k+1}$ is necessary to obtain
 % $\mathcal{D}_{\mathbf{u}}$ s.t.
    \begin{align}
        \inf_{\mathbf{a}: \|\mathbf{a}\|_2 \leq B } \mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^d)}
        % {(\mathbf{v},f_{\mathbf{u}}(\mathbf{v}))\sim \mathcal{D}_{\mathbf{u}}} 
        \left[ \ell \left(\mathbf{a}^\top \Psi(\mathbf{v}), f_i(\mathbf{v})\right)   \right]  &\geq 1 - \epsilon \nonumber
        \vspace{-1mm}
    \end{align}
    on all %n $(r,\mathbf{u})$
sparse parity tasks $f_i\in \mathcal{T}_{\text{s.p.}}(\mathbf{M})$.
    % Otherwise, there exists a bad stationary point. 
    % This is only true for hypercube data, not gaussian data.
\end{theorem}
% can recover in the sense that it can guarantee generalization to all one-hot tasks with fewer than d samples
Theorem \ref{thm:single} shows that w.h.p., a single task drawn from the task distribution $\mathcal{T}_{\text{s.p.}}(\mathbf{M})$ cannot be used to guarantee generalization with downstream neuron and margin complexity smaller than the ambient dimension for all ground-truth representations $\mathbf{M}$. For example, if $k=r$, then with probability at least $1-2^{-r}$, the number of neurons must be $\Omega(d)$ and/or the margin must be $O(d^{-1/2})$ to allow for non-trivial error. The underlying reason is that most tasks in $\mathcal{T}_{\text{s.p.}}(\mathbf{M})$ are ``simple'' in that they only depend on a strict subset of the  $r$ ground-truth features,  thus do not contain information about all the important features (although they are still ``hard'' by virtue of being sparse parity tasks), so single-task pretraining cannot improve upon random features in terms of recovering the remaining important features. Nevertheless, Theorem \ref{thm:1} shows that multitask pretraining aggregates information across the tasks to learn a generalizable model.
% ...Even if you select the one (2) good task(s), you move to the sum of the important features.

% \textbf{Single head.}



% check how yuanzhi generalizes. answer: neurons learn single features. 


 
 % The motivating setting wherein $r\ll d $,
 
 % you might be able to learn a good representation with one hard task, but it would require d samples per task. if you have a small number of easy tasks you can solve them with few samples, but you cannot learn a good representation. here we show that you can learn a good representation with many tasks and amortize the sample complexity across tasks
 
 % $ \rho(\mathbf{W},\mathcal{T}^{\text{eval}}) \coloneqq \sup_{(i+1)\sim \mathcal{T}^{\text{eval}}}  \mathcal{L}_{i+1}(\mathbf{W},\mathbf{a}_{i+1}(\mathbf{W}))$

% address hypercube

% \begin{theorem}[Existence of a Good Network for any task] \label{thm:exist}
%    Let $\mathbf{W}_1$ be the matrix of weights learned by the multitask learning algorithm.  If $m = \Omega(r2^r)$,  $n = \Omega(rd^4)$, then for any downstream task $\bar{f}_{n+1}^\ast \in \{ \bar{f}_i^*:\{-1,1\}^r \rightarrow \{-1,1\}  \}$,  there exists a vector of biases $\mathbf{b}_{n+1}^*\in \mathbb{R}^{m}$ and a head $\mathbf{a}_{n+1}^*\in \mathbb{R}^m$ such that 
%    \begin{align}
%        \mathcal{L}_{n+1}(\mathbf{W}_1, \mathbf{b}_{n+1}^*, \mathbf{a}_{n+1}^*) = 0.
%    \end{align}
% \end{theorem}

% STATUS
% pretraining proof done
% generlaization using RF, the negtive, then experiments

% First need to show existence. Then approximation.

% Existence:

% euclidean balls of radius 1
% need to put another random relu on top (fine)
% need to bound difference between ideal random and empirical
% of course two-layer relu works. no not obvious

% goal: perfectly classify any input on the hypercube 

% with perfect features:
% $\delta=2/rt(r)$
% need $r^2 e^{r^4}$ neurons in last layer

% just need to bound difference between real network output and ideal network output: 

% for any input, the output of the first layer will differ by at most f(r)/d
% thus output of second layer neurons will differ by at most n f(r)/d, n is hidden width
% output of final layer is a distance at most rt( nhat n2 f(r)2/d2 ) 
% just make d large enugh, done.

% 1. sample complexity of linear classification on top. roughly done
% 2. lower bound for random features (hsu).. but applies only for two  layers
% 3. lower bound for gd
% 4. experiments


% option 2: perfectly classify any input in balls around hypercube vertices








% \begin{theorem}[Approximation of smooth functions]
    
% \end{theorem}







% \begin{theorem}[clusters]
    
% \end{theorem}


% }




% todo:
% negative result for linear setting
% negative result for single head
% pictures and experiments
% bias in thrm 1 proof.

%ideas: 
% learning without input structure is hard in single task setting, but not in multitask setting?
% how do they learn parities with all features going to average? implies learning parities doesn't imly generalization to other tasks
% maybe this is only true in presence of input structure
% wihtout input structure, if you learned parities you would generalize
% but you can't learn parities without input structure
% the question remains: how to prove generalization to other tasks even with good features?
% note: parities do satisfy 1/2 assumption as long as they are sampled in a particular way, e.g. r is even and the subset size is first sampled uniformly... no they break this assumption. need to argue that it doesnt make sense to learn parities
% these functions are not sensitive to individual values
% can we say that we learn a rep such that there exists a bias and head that can solve any task (yes)
% while on the other hand, learn any singe task cannot guarantee learning weights that generalize
% no. if the task is very non-smooth, then it can require checking all r vertices to predict label
% but learning any single parity or sum-based function cannot gaurantee to generalize.
% but we can't even learn parity without input structure
% our set of tasks can include parities but it cannot be solely parities
% so maybe we need to say that
% 
% plan A: 1. say that we learn a rep that can generalize if train bias and head with xx samples 2. more tasks, better generalization via delta (under uniform task distribution). 3. but we need super-exponentially-many in r tasks so don't talk abut complexities.  (r choose r/2)
% 4. single task cannot guarantee generalization even if trained with infinite samples... but it can if task is hard it works
% plan B: 1. need to show sample complexity improvement with many tasks. 
% 2. sample complexity for new task 
% 3. but we don't have 

% {\color{red} Problem: we cannot get any reasonable downstream guarantees without adding bias...

% What can be learned:

% Binary latents:
% - any polynomial...

% Gaussian latents:
% - single orthants. but requires the coordinates of the head for most neurons to be minus infinity, which complicates optimization
% - halspaces (easy)
% - i don't think we can learn parities...

% approach: need to show the existence of a good network with gaussian features in the right subspace. optimizing the head is a strongly convex problem, so if a good network exists, then optimizing the head will find it
% }'

% if we use binary data:
% error after one step is too large
% but if we can somehow kill this error and get good features, we can show that a good network exists for any function if bias is added
% can use shi et al proof to show that fine-tuning recovers the good network
% if we use gaussian data with sign: 
% 

% idea:
% use gaussian data, kill most of perp in one step, then use gaussianity to effectively go back to the hypercube for other subsequent steps
% --> the problem is that we really need to convert the prefixes back to hypercube, but we only get concentration with $r$
% , not k. and ifr is large, then error from earlier is also large (proportional to $r/k$.


% before first step:

% perp has norm O(rt(k))
% parallel has norm O(1)

% after one step:

% perp has norm O(1/rt(k)) (not O(1)) and is totally gaussian (original direction)

% parallel has norm Omega(1)
% and is gaussian plus a norm 1/k perturbation




% perp always stays completely gaussian (original direction)


\begin{comment}
\subsection{Negative Result} In this subsection we prove that SMGD cannot recover the ground-truth features, regardless of the choice of hyperparameters.

\begin{theorem}[Negative Result]\label{thm:negative} Consider a setting with $r=2$ and two tasks:
\begin{align}
    f_1^\ast(\sign(\mathbf{z}_{:2})) &\coloneqq \begin{cases} 1 & \text{if } \; z_1 > 0\\
    -1 & \text{otherwise}\\
    \end{cases} \nonumber \\
    f_2^\ast(\sign(\mathbf{z}_{:2})) &\coloneqq \begin{cases} 1 & \text{if } \; z_2 > 0\\
    -1 & \text{otherwise.}\\
    \end{cases} \nonumber 
\end{align}
Note that $\mathcal{T} = \{f_1^*, f_2^*\}$ satisfies Assumption \ref{assump:diversity}. For any $T>0$ iterations of SMGD with $\mathbf{w}_{j,0}^{\text{SMGD}}\sim N(\mathbf{0}_d,\nu^2\mathbf{I}_d)$  for all $j \in [m]$, and $\mathbf{a}_0^{\text{SMGD}}\sim N(\mathbf{0}_m,\alpha^2\mathbf{I}_m)$, for any $\nu\geq 0,\alpha\geq0,\eta\geq 0,\lambda_1\geq0,\lambda_2\geq 0$, we have that 
\begin{align}
    \mathbf{W}_T
\end{align}
with probability at least $1 -$ over the random initialization.
    
\end{theorem}
// or argue about stationary points. get rid of initialization

Theorem \ref{thm:negative} shows that 

The key to the proof is to note that the gradient for any neuron weights can be written as
\begin{align}
    \nabla_{\mathbf{w}_j}\mathcal{L}(\mathbf{W},\mathbf{a}) &= \frac{a_j}{2}(1 + \mathbb{E}_{\mathbf{v}}[v_1v_2 \sigma'(\mathbf{v}^\top  \mathbf{w})]) (\mathbf{e}_1 +\mathbf{e}_2) + \frac{a_j}{2}\sum_{\ell=3}^k \mathbb{E}_{\mathbf{v}}[(v_1+v_2) v_\ell \sigma'(  \mathbf{v}^\top  \mathbf{w}_{})] \mathbf{e}_\ell  
\end{align}
thus the gradient only depends on the ground-truth features $\mathbf{e}_1, \mathbf{e}_2$ through their sum $\mathbf{e}_1 + \mathbf{e}_2$. This observation was also made by \cite{shi2022theoretical}, who showed that gradient descent learns the sum of the ground-truth features in the single-task sparse coding setting, which is sufficient to generalize to tasks whose labels are functions of the sum of the latent coordinates, but not the much larger set of tasks that are functions of individual latent coordinates.
\end{comment}

% Single-task learning can't generalize?





==> Results-ICML.tex <==
\section{Theoretical Results} \label{sec:results}

\textbf{Feature learning guarantees.}
% In this section we discuss our main results. 
We start by showing that the gradient-based multi-task learning algorithm described in the previous section recovers the ground-truth features.
To do this, we first need the following proposition, which shows that the projection of the initial features $\mathbf{W}_0$ onto the subspace spanned by the label-relevant, or ground-truth, features stays roughly the same after one step, while their projection onto the subspace spanned by the spurious features becomes very small. 

Here, we let $\Pi_{\parallel}(\mathbf{W})\coloneqq \mathbf{W}\mathbf{M}^\top\mathbf{M}$ denote the projection of the rows of the matrix $\mathbf{W}$ onto the ground-truth subspace, and $\Pi_{\perp}(\mathbf{W})\coloneqq \mathbf{W}\mathbf{M}_{\perp}^\top \mathbf{M}_{\perp}$ denote the projection onto the spurious subspace. 
For brevity, we abbreviate the statements of the theoretical results in this section and defer the full versions, along with their proofs, to the Appendix.
\begin{proposition} \label{prop:1}
% {\color{red}{I think it would make the theorems more self-contained if you remind the reader about the definition of $m$, $n_2$, T, ... . at least in this result which is the first formal result. by now the reader for sure don't recall what $n_1$ and $n_2$ stand for}}
    Consider the gradient-based multi-task algorithm described in Section~\ref{sec:alg} that uses $T$ tasks and $(n_1,n_2)$ samples per task to update the (head, representation), respectively,  and suppose Assumption \ref{assump:diversity} holds. Further assume\footnote{The $m=O(d)$ condition in Proposition \ref{prop:1} and Theorem \ref{thm:1} is purely for ease of presentation; please see Lemma \ref{lem:final} for a complete statement of the errors for arbitrary $m$.}  %$d=\tilde{\Omega}( r^4)$, 
    $m= O(d)$
and define $\epsilon \coloneqq {O}\left(
% \frac{d \sqrt{\log(Tn_2)}}{\sqrt{Tn_2}} \left(1 + {\tfrac{ \sqrt{\log(T)}}{\sqrt{n_1}}}\right) + \tfrac{  \sqrt{d} \log(d)}{\sqrt{T}}
\frac{d\; {\log(dTn_2/\delta)} }{\sqrt{Tn_2}} \left( 1+ \frac{\sqrt{\log(T/\delta)}}{\sqrt{n_1}} \right) + {\frac{\sqrt{dr} \log(dm/\delta) }{\sqrt{T}}} 
\right)$ for $\delta<1$ and $\delta = \Omega(e^{-d})$.
Then there is a setting of the parameters $\eta,   \lambda_{\mathbf{w}}$ and $\nu_{\mathbf{w}}$
% $\eta = \Theta(1)$, $\lambda_{\mathbf{a}} = 1/\eta $, $\lambda_{\mathbf{w}} = (1+(\eta^2 2^{-r-1})/\pi)/\eta$, and $\nu_{\mathbf{w}} = O(d^{-1.25})$. % and $\sigma_b = O(d^{-1.25})$. 
%$m = \Omega(r 2^r)$, 
% For a subset ${S}\subseteq [m]$, let $\mathbf{W}_{1,S}\in \mathbb{R}^{|S|\times d}$ denote the sub-matrix of $\mathbf{W}$ with rows selected by $S$.
s.t.  %for any $\delta <1$ and $\delta=\Omega(e^{-d})$, 
with probability at least $1-\delta$,
% over the random initialization,
% there is a subset of neurons ${S}\subseteq [m]$ of size $|{S}| \geq m/4$ such that for all $j \in {S}$:
% the following two properties are satisfied by the representation learned by MTRL:
% \begin{enumerate}[leftmargin=2mm]
% \item 
\vspace{-3mm}
\begin{align}
    &1. \quad  \tfrac{1}{\nu_{\mathbf{w}}\sqrt{m}}\|\Pi_{\parallel}(\mathbf{W}^1) -  \tfrac{1}{2^{r+1}\pi} % \frac{\eta^2}{2^{r+2}} 
\Pi_{\parallel}(\mathbf{W}^{0}) \|_2 \nonumber \\
&\quad \quad \quad \quad \;\; =  O\left(  
\tfrac{r^4 + \log^4(m/\delta)}{2^r d} + \epsilon\right), \nonumber \\
&2. \quad \tfrac{1}{\nu_{\mathbf{w}}\sqrt{m}}\|\Pi_{\perp}(\mathbf{W}^{1}) \|_2  = O\left(
\tfrac{r^{3.5} + \log^{3.5}(m/\delta)}{2^r d^{1.5}} %+ \eta\sigma_w d^{1.5} e^{-d^2/8} 
    + \epsilon\right). \nonumber
\end{align} %+ \eta \sigma_w d^{1.5} e^{-d^2/8}
% +    \frac{d \sqrt{\log(Tn_2)}}{\sqrt{Tn_2}} \left(1 + {\tfrac{ \sqrt{\log(T)}}{\sqrt{n_1}}}\right) + \tfrac{  \sqrt{d} \log(d)}{\sqrt{T}}
% \frac{\sqrt{r}d}{\sqrt{T}}
% \eta^2\frac{r^4}{d} %+ \eta \sigma_w d^{1.5} e^{-d^2/8}
% + \eta \frac{\sqrt{r}d}{\sqrt{n}}


% (and scales with init)
% $\|\mathbf{W}_1 - \eta 2^{-r-2} \mathbf{M}_{:r}\mathbf{M}_{:r}^\top \mathbf{W}_0\| =  +  O\left(\sqrt{\frac{r}{d-r}}\right)$
    % \item $
    % \frac{\sqrt{r}d}{\sqrt{T}}
    % $
    %     \eta^2 \sigma_w\frac{r^{3.5}}{d^{1.5}2^r} %+ \eta\sigma_w d^{1.5} e^{-d^2/8} 
    % + \eta \sigma_w\frac{\sqrt{r}d}{\sqrt{n}}
    % \item For all $\mathbf{v}\in \{-1,1\}^r$, $\exists j \in \mathcal{S}$ such that $\mathbf{w}_{1,j}^\top \mathbf{v} + b_{1,j} > 0$
    % $\sigma_{\min}(\mathbf{W}_1)$
% \end{enumerate}
\end{proposition}
% Note that the error terms in the RHS 
% \textcolor{blue}{I think in the above theorem you should specify what the "poly" is.}
Proposition \ref{prop:1} shows that with high probability (w.h.p.) over the random initialization, the weights learned by the gradient-based multi-task learning algorithm satisfy two properties, for sufficiently large $T, n_1,$ and $ n_2$:
% \footnote{A lower bound is required on $d$ to ensure that the projection of the gradient onto the $d\!-\!r$ spurious features approximates its expectation; e.g. see Equation \ref{rowp2} in Section \ref{sec:sketch}.}: 
(1) the projection of these weights onto the ground-truth subspace is close to a slightly scaled down (by a factor of $2^{-r}$) version of their projection at initialization, and (2) their projection onto the spurious subspace is negligible. These two observations, combined with the fact that the neuron weights have independent standard Gaussian initializations, imply that  the projection of the neuron weights onto the ground-truth subspace dominates their projection onto the spurious subspace. We formalize this observation below. 

% Let $\sigma_{\min}(\Pi_{\parallel}(\mathbf{W}^+{0}))$ denote the minimum singular value of $\Pi_{\parallel}(\mathbf{W}^{0})$, then since initially the minimum singular value $\sigma_{\min}(\Pi_{\parallel}(\mathbf{W}^{0}))\gtrsim \sigma_w\sqrt{mr}$ with high probability due to the Gaussian initialization, we require that 
%  $d \gg r^4$ and $T \gg d^2 2^{2r}$ 
 
%  in order for the energy in  projection onto the ground-truth spurious subspace to dominate the projection onto the spurious subspace. 


%as long as $d\gg r$ and $n \gg d^2 2^r$
% if you condition on this then you no longer have gaussian
% if you remove thse then you no longer have gaussian
% probability you can't throw away neurons. because you don't know the value of their projections
% say that you have 
% workst case scenariom m e^{c^2r} need to choose $c = sqrt(log(m))/sqrt$  

% have large energy ($\Omega(1)$) in the subspace spanned by the label-relevant features ($\text{col}(\mathbf{M}_{:r})$) and small energy $O(d^{-1/2})$ in the subspace of spurious features ($\text{col}(\mathbf{M}_{r:})$). Moreover, Part 3 of Theorem 1 implies that the learned weights are nearly isotropic within the ground-truth $\text{col}(\mathbf{M}_{:r})$.  Effectively, after one step have a random features model with $m$ features on the $r$ label-relevant inputs rather than the ambient $d$ inputs with $d-r$ of them being spurious. 
% \textcolor{blue}{I feel that you need to expand this in words a bit more -- right now it's not easy for the reader to understand the message exactly. e.g. spurious features vanish, and all the relevant features are recovered (maybe with a scaling)? }
% \begin{proof}
    
% \end{proof}
% pick

% union bound over 2^2^r things. this means m scales up by 2^r. which is fine because complexity of error in first prop is log(m)

\begin{theorem}[Representation Learning]\label{thm:1}
    Consider the setting in Proposition \ref{prop:1}  with $d =\tilde{\Omega}( r^4 )$, $m = O(d)$, and $\epsilon$ defined the same way.
    Further suppose $m = \tilde{\Omega}(r)$, $ T = \tilde{\Omega}( 2^{2r} d r ) $ and $Tn_2 = \tilde{\Omega}(2^{2r} d^2)$. Let $\sigma_r(\mathbf{B})$ denote the $r$-th singular value of the matrix $\mathbf{B}$.
Then with probability at least $1-\delta$,
% , we have 
\begin{align}  
    \frac{\sigma_1( \Pi_{\perp}(\mathbf{W}^1)) }{\sigma_{r}( \Pi_{\parallel}(\mathbf{W}^1) )} = O\left( \tfrac{ {r^{3.5}} + \log^{3.5}(m/\delta) }{ d^{1.5} } +  2^r \epsilon \right). \nonumber
\end{align}
\vspace{-2mm}
\end{theorem}
Theorem \ref{thm:1} characterizes the representation learned by multi-task pretraining in an intuitive manner.  For $d \gg r^4$, $ T \gg 2^{2r} d $ and $Tn_2 \gg 2^{2r} d^2$, we have ${\sigma_{r}( \Pi_{\parallel}(\mathbf{W}^1) )} \gg \sigma_1( \Pi_{\perp}(\mathbf{W}^1) )$, meaning that most of the energy in each neuron weight is in the column space of the ground-truth subspace. This is equivalent to saying that applying $\mathbf{W}^1$ to an input $\mathbf{x}$ essentially projects it onto the ground-truth subspace spanned by the row space of $\mathbf{M}$, as desired.
% The key mechanism behind the ability of MTRL to recover the ground-truth features is its task-specific adaptation of the heads, as we discuss below and in Section \ref{sec:sketch}.
% characterizes the representation learned by multi-task pretraining in an intuitive manner .

% (for hypercube, 2. is $O(\eta 2^r/d^{1/2})$)
% $\lambda_1 = \Theta(1)$ 
% \end{theorem}



% A sketch of the proof is provided in Section \ref{sec:sketch} and the full proof is deferred to Appendix \ref{app:thrm1}. 

% It turns out that 
% 

% Difficulty of finite-sample analysis: dealing with non-smooth objects. can't canoncentrate over tasks without having infinite samples first. but to get infinite samples, need to know something about the finite tasks. doable but not trivial


\begin{comment}

\textbf{The importance of adapting the head to each task.} We show in Section \ref{sec:sketch} that adapting the head to each task prior to updating the representation leads to a contrastive loss that encourages feature learning. Here we provide a negative result, describing a failure case when the head is not adapted to each task and we fail to learn the true features. In particular,  we show that SMGD cannot be guaranteed to recover the ground-truth features. Recall that SMGD solves the single-model objective \eqref{obj_glob} via gradient descent. 
\begin{theorem}[Negative Result]\label{thm:negative} Consider a setting with $r=2$ and two tasks with labelling functions:
\begin{align}
    \bar{f}_1^\ast(\sign(\mathbf{z}_{:2})) &\coloneqq \begin{cases} 1 & \text{if } \; z_1 > 0\\
    -1 & \text{otherwise}\\
    \end{cases}, \quad 
    \bar{f}_2^\ast(\sign(\mathbf{z}_{:2})) \coloneqq \begin{cases} 1 & \text{if } \; z_2 > 0\\
    -1 & \text{otherwise.}\\
    \end{cases} \nonumber 
\end{align}
Note that $\bar{\mathcal{T}} = \{\bar{f}_1^*, \bar{f}_2^*\}$ satisfies Assumption \ref{assump:diversity}. Suppose $(\mathbf{W}_T,\mathbf{b}_T,\mathbf{a}_T)$ is a stationary point of the dynamics of SMGD.
% $\mathbf{w}_{j,0}^{\text{SMGD}}\sim N(\mathbf{0}_d,\nu^2\mathbf{I}_d)$  for all $j \in [m]$, and $\mathbf{a}_0^{\text{SMGD}}\sim N(\mathbf{0}_m,\alpha^2\mathbf{I}_m)$, for any $\nu\geq 0,\alpha\geq0,\eta\geq 0,\lambda_1\geq0,\lambda_2\geq 0$, 
Then, 
\begin{align}
   \mathbf{W}_T\mathbf{e}_{1} &= \mathbf{W}_T\mathbf{e}_{2}.
\end{align}
% with probability at least $1 -$ over the random initialization.
\end{theorem}
% // or argue about stationary points. get rid of initialization
Theorem \ref{thm:negative} shows that SMGD can only learn a strict subset of the ground-truth two-dimensional subspace: its intersection with the (one-dimensional) span of $\mathbf{Me}_1+\mathbf{Me}_2$. The, the features it learns are not sensitive to changes in ..  as long as their sum is the same

 
The key to the proof is to notice that the gradient for any neuron weights can be written as
\begin{align}
    \nabla_{\mathbf{w}_j}\mathcal{L}(\mathbf{W},\mathbf{a}) &= \frac{a_j}{2}(1 + \mathbb{E}_{\mathbf{v}}[v_1v_2 \sigma'(\mathbf{v}^\top  \mathbf{w})]) (\mathbf{e}_1 +\mathbf{e}_2) + \frac{a_j}{2}\sum_{\ell=3}^k \mathbb{E}_{\mathbf{v}}[(v_1+v_2) v_\ell \sigma'(  \mathbf{v}^\top  \mathbf{w}_{})] \mathbf{e}_\ell  
\end{align}
thus the gradient only depends on the ground-truth features $\mathbf{e}_1, \mathbf{e}_2$ through their sum $\mathbf{e}_1 + \mathbf{e}_2$. This observation was also made by \cite{shi2022theoretical}, who showed that gradient descent learns the sum of the ground-truth features in the single-task sparse coding setting, which is sufficient to generalize to tasks whose labels are functions of the sum of the latent coordinates, but not the much larger set of tasks that are functions of individual latent coordinates.

\textcolor{blue}{This part is good.}

\end{comment}

% {\color{red}
% \subsection{Downstream Guarantees}

% From Theorem \ref{thm:1}, we have 
% \begin{align}
%     \mathbf{W}_1 &= \eta \mathbf{M}_{:r}\mathbf{M}_{:r}^\top \mathbf{W}_0 + \eta \mathbf{N}_0
% \end{align}
% where each row of $\mathbf{N}_0$ satisfies $\|\mathbf{n}_{0,j}\|_2 = O\left(\tfrac{\|\w_{0}\|_2}{k}\right)$. 


% We consider
% \begin{align}
%     \mathcal{T}^{\text{eval}} \coloneqq \{f^* : \mathbb{R}^k \rightarrow \{-1,1\} \; \text{s.t.}  \}
% \end{align}

% Need to show improvement over random features and single task learning, thus need to quantify sample complexity and/or neuron complexity.

\textbf{Downstream performance.} Now that we have shown that the learned representation recovers the ground-truth subspace, we use this result to show that the representation generalizes to downstream tasks. We consider tasks with input data sharing the same label-relevant $r$ features as the pretraining tasks, but here the input data is discrete. In particular, each $\mathbf{v} \in \mathbb{R}^d$ is generated as:
\begin{align}
    \mathbf{v} = \mathbf{M}^\top \mathbf{z} + \mathbf{M}_{\perp}^\top \boldsymbol{\xi}, \; \mathbf{z} \sim \text{Unif}(\mathcal{H}^r), \; \boldsymbol{\xi} \sim  \text{Unif}(\mathcal{H}^{d-r})\nonumber
\end{align}
where $\mathbf{z}$ is a latent vector whose coordinates indicate the activations of the ground-truth features in the input $\mathbf{x}$ and $\boldsymbol{\xi}$ is a noise vector whose coordinates indicate the activation of the spurious features in the input.
% akin to model used in \cite{shi2022theoretical}.
Again, labels for the downstream task $T+1$ are generated by projecting the input onto the row space of $\mathbf{M}$ as follows:
\begin{align} 
 % \mathbf{x} = \mathbf{Mv}, \quad 
 {f}_{T+1}(\mathbf{x}) = g_{T+1}(\sign(\mathbf{Mv})) = g_{T+1}(\mathbf{z}) \in \{-1,1\} \nonumber%\label{down}
\end{align}
% where, as for pretraining, $g_{T+1} :\mathcal{H}^r \rightarrow \{-1,1\}$. 
We formally show below that the features learned during pretraining generalize to {\em any} such link function $g_{T+1}$.
% \begin{theorem}[End-to-end Guarantee] \label{thm:downstream}
% Let $\mathbf{W}_1$ be the weight matrix learned by multi-task pretraining with $n$ tasks drawn from a collection of tasks satisfying Assumption \ref{assump:diversity}.
% Construct the three-layer ReLU neural network ${g}(\cdot, \boldsymbol{\theta}_1)$ using re-scaled $\mathbf{W}_1$ for first layer weights as in  \eqref{F} and the task-adapted head $\mathbf{a}_{n+1}$ from \eqref{ada}.
% For any downstream task $\mathcal{D}_{n+1}$ described in \eqref{down}, with labeling function $\bar{f}_{n+1}^*$ being any mapping from $\{-1,1\}^r \rightarrow \{-1,1\}$, sample a set $\mathcal{S}_N \coloneqq \{\mathbf{x}_l, {f}_{n+1}^*(\mathbf{x}_{l})\}_{l=1}^N$ of $N$ i.i.d. samples from $\mathcal{D}_{n+1}$.
% % If $ d = \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  )) $, $n = \Omega( d^3 \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  ))  )$,
% % $m = \Theta(r^4\log^8(r) ({ r} + {\log(1/\delta)}))$,  $\hat{m}= \Omega( r^{3.5} \log^4(r) \exp\left( C \log^6(r) r^5 \log(\log(r)/\delta) ) \right) \log(1/\delta) )$, and 
% For any $\delta,\delta'\in (0,1)$ and $ d = \exp(\tilde{\Omega}( r^6  )) $, $n = d^3 \exp(\tilde{\Omega}( r^6  )  )$,
% $m = \tilde{\Theta}(r^6)$,  and $\hat{m}= \exp\left( \tilde{\Omega}(r^6)  \right)$,
% with probability at least $0.99-\delta - \delta'$ over the random  initializations, draw of $n$ pretraining tasks, and draw of $\mathcal{S}_N$,
% \begin{align} % note: r^6 may be lose. for a single task, it is definitely r^5. but we want to generalize to all 2^r tasks
%         \mathcal{L}^{(\text{eval})}_{n+1}(\boldsymbol{\theta}_1,\mathbf{a}_{n+1}) &= 
%         % \tilde{O}\left(\frac{ r^{5} \log^8(r) \log(1/\delta')}{ \sqrt{N}}\right).
%          \left(\frac{ \exp(\tilde{O}(r^6)) }{ \sqrt{N}}\right), 
%     \end{align}
%     where $\tilde{\Omega}(\cdot),\tilde{\Theta}(\cdot)$ and $\tilde{O}(\cdot)$ hide logarithmic factors in $r$, $\delta^{-1}$ and $(\delta')^{-1}$.
%     % with probability at least $1-\delta - $
% % \frac{(\hat{\gamma}=   r^{2.5} \log^4(r) )\log(1/\delta)}{(\lambda_{\mathbf{a}}=1/\hat{\gamma}) \sqrt{N}}
% \end{theorem}
\begin{theorem}[End-to-end Guarantee] \label{thm:downstream}
Let $\mathbf{W}^1$ be the outcome of the multi-task representation learning algorithm described in Section \ref{sec:alg} on the task distribution $\mathcal{T}(\mathbf{M})$, where $\mathcal{T}$ satisfies Assumption \ref{assump:diversity}. 
% \textcolor{blue}{can you be more specific here about what you mean by "learned". I think $W_1$ is just the outcome of the algorithm. If yes, maybe it's better to say it here?}
Consider a downstream task in the support of $\mathcal{T}(\mathbf{M})$ with link function $g_{T+1}$.
% being a mapping from $\{-1,1\}^r \rightarrow \{-1,1\}$. 
% Let $\mathcal{S}_N \coloneqq \{\mathbf{x}_l, {f}_{n+1}^*(\mathbf{x}_{l})\}_{l=1}^N$ be a set of $N$ i.i.d. samples from $\mathcal{D}_{n+1}$.
Construct the two-layer ReLU embedding $\phi$ using the rescaled $\mathbf{W}^1$ for first layer weights as in  \eqref{F}, and train the task-adapted head $(\mathbf{a}_{T+1},\tau_{T+1})$ using $N$ i.i.d. samples from the downstream task.
% , as in \eqref{ada}.
% 
% If $ d = \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  )) $, $n = \Omega( d^3 \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  ))  )$,
% $m = \Theta(r^4\log^8(r) ({ r} + {\log(1/\delta)}))$,  $\hat{m}= \Omega( r^{3.5} \log^4(r) \exp\left( C \log^6(r) r^5 \log(\log(r)/\delta) ) \right) \log(1/\delta) )$, and 
 Further, suppose $ d = \exp(\tilde{\Omega}( r^5  )) $, $T = d^2 r \exp(\tilde{\Omega}( r^5  )  )$, $Tn_2 = d^3 \exp(\tilde{\Omega}( r^5  )  )$, $n_1 = \Omega(\log(T))$ % $\min(n_1,n_2)=\Omega(1)$,
$m = \tilde{\Theta}(r^5)$,  and $\hat{m}= \exp\left( \tilde{\Omega}(r^5)  \right)$.
Then there is a setting of the parameters $\eta,   \lambda_{\mathbf{w}}$ and $\nu_{\mathbf{w}}$ such that for any $\delta \in (e^{-d},0.05]$, with probability at least $1-\delta$,
% over the random  initializations, draw of $T$ pretraining tasks, and draw of $N$ samples from the downstream task, 
% we have
\begin{align}
% \vspace{-2mm}
        \mathcal{L}^{\text{eval}}_{T+1} %(\boldsymbol{\theta}_1,\mathbf{a}_{T+1}) 
        &= 
        % \tilde{O}\left(\frac{ r^{5} \log^8(r) \log(1/\delta')}{ \sqrt{N}}\right).
       \frac{ \exp(\tilde{O}(r^5)) }{ \sqrt{N}}. 
       \vspace{-3mm}
    \end{align}
    % where $\tilde{\Omega}(\cdot),\tilde{\Theta}(\cdot)$ and $\tilde{O}(\cdot)$ hide log factors in  $\delta^{-1}$.
    %and $(\delta')^{-1}$.
    % \textcolor{blue}{don's see why you need both $\delta$ and $\delta'$. CAn you just use a single $\delta$ for $\delta + \delta'$? }
    % with probability at least $1-\delta - $
% \frac{(\hat{\gamma}=   r^{2.5} \log^4(r) )\log(1/\delta)}{(\lambda_{\mathbf{a}}=1/\hat{\gamma}) \sqrt{N}}
\end{theorem}
Theorem \ref{thm:downstream} shows that the features learned by multi-task pretraining generalize to {\em any} downstream task 
% mapping from $\mathcal{H}^d$ to $\{-1,1\}$ 
that has the same representation as the pretraining tasks, i.e., its labels are a function of the input's projection onto the row space of $\mathbf{M}$. Specifically,
if we compose the learned representation with  a random ReLU layer, then learn a linear head using $\exp(\tilde{O}(r^5))$ samples from the task, we solve the task w.h.p.
Crucially, the number of samples and neurons  needed to solve the downstream task do not depend on the ambient dimension  $d$. 
% In other words,  multi-task learning reduces the effective dimension of the downstream task  from $d$ to $r$. 
% Since the motivating assumption

 % are generalizable by showing that they can yield a network that 
 % efficiently solves \textit{any} downstream task with latent coordinates on the hypercube, 
 % after adding a random ReLU layer and a trained head. Most importantly, the complexity of solving the new task is independent of dimension

%  \begin{align}
%     \mu &= \Theta (r^{-2.5} \log^{-3}(r) \exp( -C \log^6(r) r^5 \log(\log(r)/\nu) )) \nonumber \\
%     m &= \Theta( r^4\log^8(r) ({ r} + {\log(1/\nu)})) \nonumber \\
%     \hat{m} &= \Theta\left(r^{3.5} \log^4(r) \exp\left( C \log^6(r) r^5 \log(\log(r)/\nu) ) \right) \log(1/\nu)\right) \\
%     &O\left(\left(\frac{r^{4}}{\sqrt{d}} +  d^2 e^{-d^2/8} + \frac{\sqrt{r}d^{1.5}}{\sqrt{n}}\right)(\frac{\sqrt{m}}{\sqrt{\hat{m}}})\right) \\
%     &\rightarrow
% \end{align}


The proof of Theorem \ref{thm:downstream} leverages Proposition \ref{prop:1} to show that the embedding  generated by multi-task learning is close to the embedding of a coupled, ``purified'' two-hidden layer random ReLU network whose first layer weights project the input {\em exactly} onto the row space of $\mathbf{M}$. Then, the proof applies  Theorem 2 from \citet{dirksen2022separation} which implies that w.h.p. the purified network linearly separates two classes of points on $\mathcal{H}^r$ with margin and neuron complexity scaling as functions of the input dimension $r$. The representation learning error from Proposition \ref{prop:1} is  smaller than this margin due to the lower bounds on $T$, $n_1, n_2$,  and $d$ in Theorem \ref{thm:downstream}, so the learned network also linearly separates the two classes w.h.p. Then, the proof invokes a standard linear classification generalization bound to control the final error in learning the head \cite{Livni_2017}. Note that Theorem \ref{thm:downstream} requires $d^3$ training sample complexity rather than the $d^2$ complexity of Theorem \ref{thm:1} because Theorem \ref{thm:1} concerns the spectral norm of the representation learning error, whereas for the generalization result, we require a Frobenius norm bound, which induces an extra $d$ factor. Please see the proof of Lemma C.3 for details.
% Alternatively, we could apply the results on linear separation capabilities of random two-layer ReLU networks in \cite{ghosal2022randomly} without needing to add an extra hidden layer, but doing so would require $\Omega(\exp(2^r))$ samples and neurons. 
% The full proof is found in Appendix \ref{app:down}.
% \citep{hsu2021approximation}

\begin{comment}
While Theorem \ref{thm:downstream}  ensures generalization to an arbitrary task sharing the ground-truth features, it can only guarantee generalization to a single such task at once. To ensure that the learned embedding generalizes to a larger set of tasks simultaneously, we have the following corollary.
\begin{corollary}[Generalization to set of tasks] \label{cor:set}
Consider a set  of possible downstream tasks $\mathcal{S}^{\text{eval}}$ with $|\mathcal{S}^{\text{eval}}| = D$. Suppose $ d = \exp(\tilde{\Omega}( r^5 \log(D) )) $, $T = d^3 \exp(\tilde{\Omega}( r^5 \log(D)  )  )$,
$m = \tilde{\Theta}(r^5 \log(D) )$,  and $\hat{m}= \exp\left( \tilde{\Omega}(r^5 \log(D) )  \right)$. Construct the two-layer ReLU embedding as in \eqref{F}. Then with probability at least $0.99-\delta$,  any task $T\!+\!1$ in $\mathcal{S}^{\text{eval}}$ 
satisfies
% compute $(\mathbf{a}_{T+1},\tau_{T+1})$ using $n$ samples from task $T+1$,
\begin{align}
        \mathcal{L}^{\text{eval}}_{T+1} %(\boldsymbol{\theta}_1,\mathbf{a}_{T+1}) 
        &= 
        % \tilde{O}\left(\frac{ r^{5} \log^8(r) \log(1/\delta')}{ \sqrt{N}}\right).
       \frac{ \exp(\tilde{O}(r^5 \log(D))) }{ \sqrt{N}}, 
    \end{align}
    where $\tilde{\Omega}(\cdot),\tilde{\Theta}(\cdot)$ and $\tilde{O}(\cdot)$ hide log factors in $r$ and $\delta^{-1}$. 
    % \textcolor{blue}{same comment as above about $\delta$}
\end{corollary}
For example, if $\mathcal{S}^{\text{eval}}$ is the set of all $2^{2^r}$ functions from $\mathcal{H}^r$ to $\{-1,1\}$ (the support of $\mathcal{T}_{\text{all}}$), then Corollary \ref{cor:set} shows that multi-task pretraining learns a representation that for all such target functions yields an accurate classifier with $O(\exp(\exp(r)))$ sample and neuron complexity, which is independent of the ambient dimension $d$.
\end{comment}


{
% \color{gray}

\begin{remark}[Necessity of second layer] \label{rem:2}
    % As the reviewer correctly points out, after one gradient descent step we almost have a random two-layer ReLU network that takes as input the $r$-dimensional ground-truth features (which here are vectors on the $r$-dimensional hypercube), and whose first-layer weights are $r$-dimensional Gaussians. 
 % Thus, we should consult the literature on random feature models to 
 % determine the classes of functions that networks with such a first layer are capable of expressing with high probability. 
 In the ideal representation learning scenario, the  first-layer weights are i.i.d. isotropic Gaussians in the ground-truth subspace $\text{row}(\mathbf{M})$. In this scenario we can think of the network as taking an $r$-dimensional input (corresponding to the $r$ ground-truth features of the input) and having first-layer weights that are i.i.d.isotropic Gaussians in $\mathbb{R}^r$. Even in this ideal scenario, existing results have not shown whether such a representation is sufficiently expressive or generalization to all downstream tasks w.h.p.
 % We refer to this first layer as the ``ideal'' representation, and argue that even it requires composition with a second ReLU layer to be sufficiently expressive as to achieve the generalization results of Theorem \ref{thm:downstream} w.h.p.
 There are several positive results for the expressivity of a  random, finite-width ReLU layer, but these concern approximating low-degree polynomials under the squared loss \cite{hsu2021approximation,ji2019neural,yehudai2019power,bach2017breaking}. 
% In our case, we require that the representation linearly separates the ground-truth classes with margin larger than the error between this low-input-dimensional Gaussian network and the noisy Gaussian network we have from starting with high-dimensional Gaussian weights and executing one step of GD. 
However, to our knowledge, there are no analogous positive results showing that one layer of random ReLU neurons can linearly separate  two arbitrary classes of points on the Boolean hypercube  w.h.p., even with  exponentially-many neurons or exponentially-small margin. 
% We leverage the positive result of this kind with, to our knowledge, the cheapest neuron and margin complexity, which requires a second ReLU layer (Dirksen et al., 2022, Theorem 1). 
\end{remark}


\begin{remark}[Tightness of exponential complexity in $r$ in positive results]
% Our Theorem 3.4, which adapts Theorem 5 in Barak et al. 2022, shows that for any fixed representation, at least $d^{\Omega(k)}$ samples or width is necessary to solve all $k$-sparse parity tasks on $d$ inputs. 
Replacing $d$ with $r$, Theorem \ref{thm:lower} implies  that at least $r^{\Omega(k)}$ samples or width is necessary to express all $k$-sparse parity tasks on $r$ inputs. So, even if we learn exactly the correct representation, we require $r^{\Omega(r)}$ samples or width to solve all $\frac{r}{2}$-sparse parity tasks on the $r$ ground-truth features. Please see \cite{malach2022hardness,abbe2020poly,abbe2022merged,abbe2023sgd,shalev2017failures,hsu2021approximation,kamath2020approximate,ghorbani2020neural} 
for similar lower bounds. 
Nevertheless, our complexity of $\exp(\text{poly}(r))$ is larger than such lower bounds. We leave to future work to investigate whether the $\text{poly}(r)$ complexity in the exponent can be reduced.
\end{remark}
% of function classes on $r$ inputs that require exponential sample or width complexity in $r$ to learn with a fixed representation and linear head.

% One might propose that this exponential complexity could be avoided by adapting the representation to each downstream task. However, prior results show that gradient-based algorithms require at least $\Omega(r^k)$ samples to solve $k$-sparse parity tasks on $r$ inputs (Abbe et al., 2023; Abbe and Sandon, 2020; Shalev-Schwartz et al., 2017).
% % classical results give statistical query (SQ) lower bounds for learning $k$-sparse parities on $r$ inputs that are exponential in $r$ when $k$ grows with $r$, implying that gradient descent would require exponentially-many samples in $r$ (Blum et al., 1994; Kearns, 1998). 
% Therefore, since we seek to generalize to all downstream tasks including  sparse parities, exponential sample or neuron complexity in $r$ is inevitable.
% % mention malach and daniely?

% Other works give exponential-width lower bounds for 
% approximating parities with uniform input distribution under the squared loss with random features and task-optimal heads (Hsu et al., 2021; Hsu, 2021; Kamath et al., 2020), and an exponential sample-lower bound for learning the head in the same setting (Kamath et al., 2020). 
% The underlying idea behind  these (and the aforementioned) results is that since the parity functions on subsets of $r$ input bits are orthogonal and  any representation that can express all such functions after composition with a linear mapping must ``span'' them in function space, the representation dimension must be at least the number of tasks, which is $2^r$ for all of the sparse parity tasks on $r$ input bits and  $2^{\Omega(r)}$ for the set of $k$-sparse parity tasks on $r$ inputs where $k$  scales with $r$.
% Additional results lower bounding the complexity of learning polynomials under squared error with any fixed features (Abbe et al., 2022 Proposition 11; Abbe et al., 2023 Proposition 3; Ghorbani et al., 2020 Theorems 2 and 3) imply $r^{\Omega(r)}$ sample- and width lower bounds for learning $\frac{r}{2}$-sparse parities under the squared error.



% (note that the set of such tasks is a set of $\binom{r}{\frac{r}{2}}$ orthogonal polynomials of degree $\frac{r}{2}$).
% While these results do not apply to classification, they suggest that exponential complexity in both samples and width are required in our setting, perhaps even $\exp(\omega_r(r))$ complexity. 
% With that being said, our complexity of $\exp(\text{poly}(r))$ is larger than such lower bounds. We leave to future work to investigate whether the $\text{poly}(r)$ complexity in the exponent can be reduced.
% Nevertheless, it is worth reiterating that by our Theorem 3.4, if we did not learn the correct representation, we would face at least $d^{r}$ sample- or width-complexity for generalization, which could be far worse than our current complexity.



}

% \vspace{-2mm}
\subsection{Negative Results}
% \vspace{-1mm}
Next, we present two negative results that underscore the tightness of our findings in the previous section. The first result emphasizes the significance of representation learning in achieving strong generalization guarantees. The second result highlights the importance of multi-task learning by demonstrating that single-task learning may fail to capture all critical features.

% \vspace{-1mm}

\textbf{Random features do not generalize.} A consequence of Theorem \ref{thm:downstream} is that multi-task pretraining improves the sample and neuron complexity of solving downstream tasks by an exponential factor in $d$. 
To show this, we consider sparse parity tasks,  and show that learning a linear classifier on top of random features
% not knowing the sparse features on which the task is defined 
entails exponential complexity in $d$ to solve the task.
% We have introduced sparse parity tasks \eqref{sparsepar}, however in \eqref{sparsepar}, $\mathcal{T}_{\text{s.p.}}$ was defined as the set of sparse parity tasks mapping from a {\em fixed} set of $r$ features, that is, the set of sparse parity tasks on a fixed ground-truth representation.
Now, there is no feature learning, so the learner has no knowledge of which few features are relevant and needs to consider tasks on all $d$ inputs.
% We model this by considering the set of sparse parity tasks on $r$-dimensional subsets of $d$ inputs, meaning each task $i$ is associated with a unique  representation $\mathbf{M}_i$ that selects $r$ coordinates of a Boolean input vector
We model this by considering a set of tasks sharing a single link function but having many distinct representations.
We consider a smaller class of representations than in our positive results: here $\mathbf{M}$ belongs to $\mathbb{O}^{r\times d}_{\{0,1\}}\coloneqq \{\mathbf{M}: \mathbf{M}\in \mathbb{O}^{r\times d}, \mathbf{M}\in \{0,1\}^{r\times d} \}$, that is, the rows of $\mathbf{M}$ are standard basis elements. The single link function we consider is the parity function on $r$ inputs, namely $g^{(r)}(\mathbf{v})\coloneqq (-1)^{\sum_{j =1}^r \chi\{{v}_j = -1\}}$.

% \footnote{This restricts the class of possible ground-truth representations $\mathbf{M}$ to matrices whose rows are a subset of the standard basis, whereas our positive results concern the harder problem of learning a continuous representation $\mathbf{M}$.}. This task set is formally defined as:
% \begin{align}
%     \mathcal{S}_{\text{s.p.}}\! &:= \{ g_i\!: g_i(\mathbf{v})= \bar{g}_i(\mathbf{M}_i\mathbf{v}) \!=\! (-1)^{\sum_{j =1}^r \chi\{(M_i{v})_j = -1\}},\nonumber \\
%         &\quad\quad
%         % \mathcal{S}_i \subseteq [d], |\mathcal{S}_i|=r,
%         % 
%         \mathbf{M}_i\in \{0,1\}^{r\times d}, \mathbf{M}_i \in \mathbb{O}^{r\times d},
%         \; \forall \; \mathbf{v}\in \mathcal{H}^d  \}
%         \label{sp2}
% \end{align}
   % \begin{align}
   %      \mathcal{T}_{\text{s.p.}} \coloneqq &\;\text{Unif}(\{ g_i: g_i(\mathbf{v}) = (-1)^{\sum_{j \in \mathcal{S}_i} \chi\{{v}_j = -1\}},\nonumber \\
   %      &\quad\quad \quad \quad \;\; \mathcal{S}_i \subseteq [r],\; \forall \; \mathbf{v}\in \mathcal{H}^r  \}).\label{sparsepar}
   %  \end{align}
% , i.e. the support of the task distribution $\mathcal{T}_{\text{s.p.}}$ defined in \eqref{sparsepar}.
% we consider the well-studied problem of learning sparse parities, which are functions that output the parity of a small subset of input bits. Formally, for  $\mathbf{u}\in \{0,1\}^d$ with $\|\mathbf{u}\|_1 = r$, an $(r,\mathbf{u})$-sparse parity task is defined as follows.
% \begin{definition}
%     [$(r,\mathbf{u})$-sparse parity task]
%     An $(r,\mathbf{u})$-sparse parity task $\mathcal{D}_{\mathbf{u}}$ has data $(\mathbf{v},f_{\mathbf{u}}(\mathbf{v}))$ generated as
% $
%         \mathbf{v}\sim \text{Unif}(\{-1,1\}^d )$ and $f_{\mathbf{u}}(\mathbf{v}) = (-1)^{\mathbf{u}^\top \mathbf{v}},
%     $
%     where $\mathbf{u}\in \{0,1\}^d$ with $\|\mathbf{u}\|_1 = r$.
% \end{definition}
% In other words, an $(r,\mathbf{u})$-sparse parity task has labels being the parity of the number of $-1$'s among the bits selected by the $r$-sparse vector $\mathbf{u}$.
% The sparse parity problem is then 
% Canonical results show that solving an $(r,\mathbf{u})$-sparse parity task requires $\Omega(d^r)$ samples in the Statistical Query (SQ) model \cite{} and $\Omega(\poly(d))$ noiseless samples via Gaussian elimination. 
While there is a large literature demonstrating the hardness of learning sparse parities in various settings \cite{kearns1998efficient,abbe2020poly,telgarsky2022feature,barak2022hidden,malach2022hardness,kamath2020approximate,goel2019time}, the most relevant results to our setting show that any data-independent, $\hat{m}$-dimensional embedding of $d$ inputs can admit linear classifiers that solve all sparse parity tasks on subset only if the dimension $\hat{m}$ and/or the classification margin is exponentially large (small, respectively) in $d$.
% , including the two-layer ReLU representations, as well as the neural tangent kernel \cite{jacot2018neural},  requires 
In particular, the following result adapts Theorem 5 in \cite{barak2022hidden}, which in turn draws on the works of \citet{kamath2020approximate} and \citet{malach2022hardness}.
\vspace{-1mm}
% Holds for any embedding mapping from $\mathbb{R}^d$ to $\mathbb{R}^{\hat{m}}$, 
\begin{theorem}[] \label{thm:lower}
Consider any embedding $\Psi:\mathcal{H}^d \rightarrow \mathbb{R}^{\hat{m}}$ such that $\|\Psi(\mathbf{v})\|_2 \leq 1 $ for all $\mathbf{v}\in \mathcal{H}^d$. 
For % $\mathbf{v}\sim \text{Unif}(\mathcal{H}^d)$ and 
any $\epsilon >0$, if 
$ \hat{m}B^2 \leq \epsilon^2 \binom{d}{r}, $
then there exists a %n $(r,\mathbf{u})$
representation $\mathbf{M} \in \mathbb{O}^{r\times d}_{\{0,1\}}$
% sparse parity task $g_i\in \mathcal{S}_{\text{s.p.}}$ 
such that: % $\mathcal{D}_{\mathbf{u}}$ s.t.
\vspace{-2mm}
    \begin{align}
        \inf_{\mathbf{a}: \|\mathbf{a}\|_2 \leq B } \mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^d)}
        % {(\mathbf{v},f_{\mathbf{u}}(\mathbf{v}))\sim \mathcal{D}_{\mathbf{u}}} 
        \left[ \ell \left(\mathbf{a}^\top \Psi(\mathbf{v}), g^{(r)}(\mathbf{Mv})\right)   \right]  &\geq 1 - \epsilon.\nonumber
    \end{align}
    \vspace{-4mm}
\end{theorem}
Theorem \ref{thm:lower} implies that any random feature model requires a number of neurons and/or  inverse margin that is polynomially large in $d^r$ in order to solve a downstream sparse parity task with a linear classifier. Note that the margin (i.e. inverse of $B$ in Theorem \ref{thm:lower}) is inversely proportional to the number of samples that are required to learn the classifier \cite{Livni_2017}. On the other hand, Theorem~\ref{thm:1} guarantees that  after multi-task pretraining, the output embedding admits a linear classifier that solves any sparse parity task  on the extracted $r$ features, with the number of neurons and samples of the downstream task of the order of $\exp(\poly(r))$. 


% While our analysis does assume infinite samples for the multi-task representation learning phase, it is not required to solve an $r$-sparse parity task during this phase. 

% \textbf{Lower bound: }

% I think we can get rid of second relu layer.... each neuron is the indicator for some input, covers all inputs with r2**r neurons... no, because the bias needs to be exact learned...
\textbf{Single task does not suffice for  feature learning.} Although Theorem \ref{thm:lower} shows that feature learning is essential for generalization in our setting, we have not yet shown that effective feature learning necessitates pretraining on {\em multiple} tasks. We address this issue next.  
% We first show that multi-task training is necessary for learning a generalizable representation, since with high probability over a single task drawn from $\mathcal{T}_{\text{s.p.}}$, training on this single task cannot lead to learning all $r$ ground-truth features.
\begin{theorem}\label{thm:single}
%     % Suppose $\mathcal{T} = \mathcal{T}_{\text{s.p.}}$.
%     % and $\mathcal{S}^{\text{eval}} = \{ g_i: g_i(\mathbf{v}) = v_i,\; i \in [r],\; \forall \; \mathbf{v}\in \mathcal{H}^r\}$. 
%     % any algorithm for pretraining with any number of samples cannot produce a model that 
%     % contains information about all $r$ ground-truth features, in the sense that this model 
%     % requires at least $d$ samples
%     % from the downstream task to guarantee loss smaller than $0.5 -\epsilon$ for any $\epsilon>0$ in the worst case over downstream tasks in $\mathcal{S}^{\text{eval}}$.
%     % Consider 
%     Consider any embedding $\Psi:\mathcal{H}^d \rightarrow \mathbb{R}^{\hat{m}}$ such that $\|\Psi(\mathbf{v})\|_2 \leq 1 $ for all $\mathbf{v}\in \mathcal{H}^d$ that is trained on arbitrarily many samples from a single task drawn from $\mathcal{T}_{\text{s.p.}}(\mathbf{M})$.  Then there exists an $\mathbf{M}\in \mathbb{O}^{r\times d}_{\{0,1\}}$ such that for any $k\in[r]$, with probability at least $1 - 2^{-r}\sum_{j=k}^r\binom{r}{j} $ over the single task drawn from $\mathcal{T}_{\text{s.p.}}(\mathbf{M})$, 
% for any $\epsilon >0$, 
% $ \hat{m}B^2 > \epsilon^2 \binom{d-k+1}{r-k+1}$ is necessary to obtain
%  % $\mathcal{D}_{\mathbf{u}}$ s.t.
%     \begin{align}
%         \inf_{\mathbf{a}: \|\mathbf{a}\|_2 \leq B } \mathbb{E}_{\mathbf{v}\sim \text{Unif}(\mathcal{H}^d)}
%         % {(\mathbf{v},f_{\mathbf{u}}(\mathbf{v}))\sim \mathcal{D}_{\mathbf{u}}} 
%         \left[ \ell \left(\mathbf{a}^\top \Psi(\mathbf{v}), f_i(\mathbf{v})\right)   \right]  &\geq 1 - \epsilon \nonumber
%         \vspace{-1mm}
%     \end{align}
%     on all %n $(r,\mathbf{u})$
% sparse parity tasks $f_i\in \mathcal{T}_{\text{s.p.}}(\mathbf{M})$.
%     % Otherwise, there exists a bad stationary point. 
%     % This is only true for hypercube data, not gaussian data.
    Consider any algorithm $\mathcal{A}$ that takes as input infinite samples from any {\em single} task in  $\mathcal{T}_{\text{s.p.}}(\mathbf{M})$ and returns an $\hat{m}$-dimensional representation $\Psi:\mathcal{H}^d \rightarrow \mathbb{R}^{\hat{m}}$. 
Then
 there exists an $\mathbf{M}\in \mathbb{O}^{r\times d}_{\{0,1\}}$ such that for any $k\in[r]$, with probability at least $1 - 2^{-r}\sum_{j=k}^r\binom{r}{j} $ over the draw of a single training task $f_1 \sim \mathcal{T}_{\text{s.p.}}(\mathbf{M})$, the representation $\Psi_{f_1}:= \mathcal{A}(f_1)$ satisfies that
for any $\epsilon >0$, 
$ \hat{m}B^2 > \epsilon^2 \binom{d-k+1}{r-k+1}$ is necessary to obtain
    \begin{align}
   \min_{\mathbf{a}_2: \|\mathbf{a}_2\|_2 \leq B}      \mathbb{E}_{\mathbf{v} \sim \text{Unif}(\mathcal{H}^d)}[\ell( \mathbf{a}_2^\top \Psi_{f_1}(\mathbf{v}), \; f_{2}(\mathbf{v}) )] \geq 1- \epsilon. \nonumber
    \end{align}
\end{theorem}
% can recover in the sense that it can guarantee generalization to all one-hot tasks with fewer than d samples
Theorem \ref{thm:single} shows that w.h.p., a single task drawn from the task distribution $\mathcal{T}_{\text{s.p.}}(\mathbf{M})$ cannot be used to guarantee generalization with downstream neuron and margin complexity smaller than the ambient dimension for all ground-truth representations $\mathbf{M}$. For example, if $k=r$, then with probability at least $1-2^{-r}$, the number of neurons must be $\Omega(d)$ and/or the margin must be $O(d^{-1/2})$ to allow for non-trivial error. The underlying reason is that most tasks in $\mathcal{T}_{\text{s.p.}}(\mathbf{M})$ are ``simple'' in that they only depend on a strict subset of the  $r$ ground-truth features,  thus do not contain information about all the important features (although they are still ``hard'' by virtue of being sparse parity tasks), so single-task pretraining cannot improve upon random features in terms of recovering the remaining important features. Nevertheless, Theorem \ref{thm:1} shows that multi-task pretraining aggregates information across the tasks to learn a generalizable model.
% ...Even if you select the one (2) good task(s), you move to the sum of the important features.

% \textbf{Single head.}

% {\color{red}Liam: below is WIP, will finish merging rebuttal tonight 5/28}
\begin{remark}[Single-task training with highly informative task]
    % As far as showing separations between training with a single task that contains information about all ground-truth features and multi-tasking, 
     Theorem \ref{thm:1}  leaves open the possibility that training on a highly-informative task could perform as well as multi-tasking. Note that  there is one task supported by $\mathcal{T}_{\text{s.p.}}(\mathbf{M})$, the full parity task, that provides information abut all $r$ ground-truth features in $\mathbf{M}$. While gradient-based training on this task may allow for efficient generalization to any downstream task on the $r$ features \cite{barak2022hidden}\footnote{\citet{barak2022hidden} show that SGD on a two-layer ReLU NN with batch size $\tilde{\Omega}(d^r)$ can solve the parity task on $r$ features with unknown $\mathbf{M} \in \mathbb{O}_{{0,1}}^{d\times r}$, which suggests that the representation learned during this process generalizes to simpler tasks on the features in $\mathbf{M}$.}, the sample complexity of this training may be much larger than multi-tasking.
    Additional prior results show that 
    % However,
    % prior results have demonstrated that, even in the setting with possible ground-truth representations limited to subsets of input coordinates (i.e. $\mathbf{M}\in \mathbb{O}_{{0,1}}^{d\times r}$),
    gradient-based algorithms require at least $\Omega(d^r)$ samples to solve the full parity task on $r$ inputs \cite{abbe2023sgd,abbe2020poly,shalev2017failures}. This complexity has worse dependence on $d$ and $T$ than the $n_1+n_2 = \tilde{O}(\frac{d^3}{T})$ training samples per task required by Theorem \ref{thm:downstream} for downstream generalization with the number of downstream samples independent of $d$. In fact,  it is even worse complexity in $d$ than the $T(n_1+n_2) + N = \tilde{O}(d^3)$ total samples across tasks that Theorem \ref{thm:downstream} requires for multi-task pretraining followed by downstream adaptation. Thus multi-tasking reduces feature learning  sample complexity compared to training with {\em any} single task. 

% Beyond sample complexity separations, one may also ask whether we can show learnability separations between training on any single task and multi-tasking. Yet \citet{barak2022hidden} show that the aforementioned lower bounds on the complexity of learning the full parity task are tight by proving that SGD on a two-layer ReLU NN with batch size $\tilde{\Omega}(d^r)$ can solve the parity task on $r$ inputs with unknown $\mathbf{M} \in \mathbb{O}_{{0,1}}^{d\times r}$. This suggests that a single, highly informative task with many samples is sufficient for recovering all the ground-truth features via gradient-based approaches and nonlinear NNs, albeit with larger net sample complexity. 
% So, we do not believe a learnability separation result is possible for single task training with the best-case task vs multi-tasking.
\end{remark}



% check how yuanzhi generalizes. answer: neurons learn single features. 


 
 % The motivating setting wherein $r\ll d $,
 
 % you might be able to learn a good representation with one hard task, but it would require d samples per task. if you have a small number of easy tasks you can solve them with few samples, but you cannot learn a good representation. here we show that you can learn a good representation with many tasks and amortize the sample complexity across tasks
 
 % $ \rho(\mathbf{W},\mathcal{T}^{\text{eval}}) \coloneqq \sup_{(i+1)\sim \mathcal{T}^{\text{eval}}}  \mathcal{L}_{i+1}(\mathbf{W},\mathbf{a}_{i+1}(\mathbf{W}))$

% address hypercube

% \begin{theorem}[Existence of a Good Network for any task] \label{thm:exist}
%    Let $\mathbf{W}_1$ be the matrix of weights learned by the multi-task learning algorithm.  If $m = \Omega(r2^r)$,  $n = \Omega(rd^4)$, then for any downstream task $\bar{f}_{n+1}^\ast \in \{ \bar{f}_i^*:\{-1,1\}^r \rightarrow \{-1,1\}  \}$,  there exists a vector of biases $\mathbf{b}_{n+1}^*\in \mathbb{R}^{m}$ and a head $\mathbf{a}_{n+1}^*\in \mathbb{R}^m$ such that 
%    \begin{align}
%        \mathcal{L}_{n+1}(\mathbf{W}_1, \mathbf{b}_{n+1}^*, \mathbf{a}_{n+1}^*) = 0.
%    \end{align}
% \end{theorem}

% STATUS
% pretraining proof done
% generlaization using RF, the negtive, then experiments

% First need to show existence. Then approximation.

% Existence:

% euclidean balls of radius 1
% need to put another random relu on top (fine)
% need to bound difference between ideal random and empirical
% of course two-layer relu works. no not obvious

% goal: perfectly classify any input on the hypercube 

% with perfect features:
% $\delta=2/rt(r)$
% need $r^2 e^{r^4}$ neurons in last layer

% just need to bound difference between real network output and ideal network output: 

% for any input, the output of the first layer will differ by at most f(r)/d
% thus output of second layer neurons will differ by at most n f(r)/d, n is hidden width
% output of final layer is a distance at most rt( nhat n2 f(r)2/d2 ) 
% just make d large enugh, done.

% 1. sample complexity of linear classification on top. roughly done
% 2. lower bound for random features (hsu).. but applies only for two  layers
% 3. lower bound for gd
% 4. experiments


% option 2: perfectly classify any input in balls around hypercube vertices








% \begin{theorem}[Approximation of smooth functions]
    
% \end{theorem}







% \begin{theorem}[clusters]
    
% \end{theorem}


% }




% todo:
% negative result for linear setting
% negative result for single head
% pictures and experiments
% bias in thrm 1 proof.

%ideas: 
% learning without input structure is hard in single task setting, but not in multi-task setting?
% how do they learn parities with all features going to average? implies learning parities doesn't imly generalization to other tasks
% maybe this is only true in presence of input structure
% wihtout input structure, if you learned parities you would generalize
% but you can't learn parities without input structure
% the question remains: how to prove generalization to other tasks even with good features?
% note: parities do satisfy 1/2 assumption as long as they are sampled in a particular way, e.g. r is even and the subset size is first sampled uniformly... no they break this assumption. need to argue that it doesnt make sense to learn parities
% these functions are not sensitive to individual values
% can we say that we learn a rep such that there exists a bias and head that can solve any task (yes)
% while on the other hand, learn any singe task cannot guarantee learning weights that generalize
% no. if the task is very non-smooth, then it can require checking all r vertices to predict label
% but learning any single parity or sum-based function cannot gaurantee to generalize.
% but we can't even learn parity without input structure
% our set of tasks can include parities but it cannot be solely parities
% so maybe we need to say that
% 
% plan A: 1. say that we learn a rep that can generalize if train bias and head with xx samples 2. more tasks, better generalization via delta (under uniform task distribution). 3. but we need super-exponentially-many in r tasks so don't talk abut complexities.  (r choose r/2)
% 4. single task cannot guarantee generalization even if trained with infinite samples... but it can if task is hard it works
% plan B: 1. need to show sample complexity improvement with many tasks. 
% 2. sample complexity for new task 
% 3. but we don't have 

% {\color{red} Problem: we cannot get any reasonable downstream guarantees without adding bias...

% What can be learned:

% Binary latents:
% - any polynomial...

% Gaussian latents:
% - single orthants. but requires the coordinates of the head for most neurons to be minus infinity, which complicates optimization
% - halspaces (easy)
% - i don't think we can learn parities...

% approach: need to show the existence of a good network with gaussian features in the right subspace. optimizing the head is a strongly convex problem, so if a good network exists, then optimizing the head will find it
% }'

% if we use binary data:
% error after one step is too large
% but if we can somehow kill this error and get good features, we can show that a good network exists for any function if bias is added
% can use shi et al proof to show that fine-tuning recovers the good network
% if we use gaussian data with sign: 
% 

% idea:
% use gaussian data, kill most of perp in one step, then use gaussianity to effectively go back to the hypercube for other subsequent steps
% --> the problem is that we really need to convert the prefixes back to hypercube, but we only get concentration with $r$
% , not k. and ifr is large, then error from earlier is also large (proportional to $r/k$.


% before first step:

% perp has norm O(rt(k))
% parallel has norm O(1)

% after one step:

% perp has norm O(1/rt(k)) (not O(1)) and is totally gaussian (original direction)

% parallel has norm Omega(1)
% and is gaussian plus a norm 1/k perturbation




% perp always stays completely gaussian (original direction)


\begin{comment}
\subsection{Negative Result} In this subsection we prove that SMGD cannot recover the ground-truth features, regardless of the choice of hyperparameters.

\begin{theorem}[Negative Result]\label{thm:negative} Consider a setting with $r=2$ and two tasks:
\begin{align}
    f_1^\ast(\sign(\mathbf{z}_{:2})) &\coloneqq \begin{cases} 1 & \text{if } \; z_1 > 0\\
    -1 & \text{otherwise}\\
    \end{cases} \nonumber \\
    f_2^\ast(\sign(\mathbf{z}_{:2})) &\coloneqq \begin{cases} 1 & \text{if } \; z_2 > 0\\
    -1 & \text{otherwise.}\\
    \end{cases} \nonumber 
\end{align}
Note that $\mathcal{T} = \{f_1^*, f_2^*\}$ satisfies Assumption \ref{assump:diversity}. For any $T>0$ iterations of SMGD with $\mathbf{w}_{j,0}^{\text{SMGD}}\sim N(\mathbf{0}_d,\nu^2\mathbf{I}_d)$  for all $j \in [m]$, and $\mathbf{a}_0^{\text{SMGD}}\sim N(\mathbf{0}_m,\alpha^2\mathbf{I}_m)$, for any $\nu\geq 0,\alpha\geq0,\eta\geq 0,\lambda_1\geq0,\lambda_2\geq 0$, we have that 
\begin{align}
    \mathbf{W}_T
\end{align}
with probability at least $1 -$ over the random initialization.
    
\end{theorem}
// or argue about stationary points. get rid of initialization

Theorem \ref{thm:negative} shows that 

The key to the proof is to note that the gradient for any neuron weights can be written as
\begin{align}
    \nabla_{\mathbf{w}_j}\mathcal{L}(\mathbf{W},\mathbf{a}) &= \frac{a_j}{2}(1 + \mathbb{E}_{\mathbf{v}}[v_1v_2 \sigma'(\mathbf{v}^\top  \mathbf{w})]) (\mathbf{e}_1 +\mathbf{e}_2) + \frac{a_j}{2}\sum_{\ell=3}^k \mathbb{E}_{\mathbf{v}}[(v_1+v_2) v_\ell \sigma'(  \mathbf{v}^\top  \mathbf{w}_{})] \mathbf{e}_\ell  
\end{align}
thus the gradient only depends on the ground-truth features $\mathbf{e}_1, \mathbf{e}_2$ through their sum $\mathbf{e}_1 + \mathbf{e}_2$. This observation was also made by \cite{shi2022theoretical}, who showed that gradient descent learns the sum of the ground-truth features in the single-task sparse coding setting, which is sufficient to generalize to tasks whose labels are functions of the sum of the latent coordinates, but not the much larger set of tasks that are functions of individual latent coordinates.
\end{comment}

% Single-task learning can't generalize?





==> Results.tex <==
\section{Theoretical Results} \label{sec:results}

\textbf{Feature learning guarantees.}
% In this section we discuss our main results. 
We start by showing that the gradient-based multi-task learning algorithm described in the previous section recovers the ground-truth features.
To do this, we first need the following proposition, which shows that the projection of the initial features $\mathbf{W}_0$ onto the subspace spanned by the label-relevant, or ground-truth, features stays roughly the same after one step, while their projection onto the subspace spanned by the spurious features becomes very small. 

Here, we let $\Pi_{\parallel}(\mathbf{W})\coloneqq \mathbf{W}_{:r}$ denote the projection of the rows of the matrix $\mathbf{W}$ onto the ground-truth subspace (i.e., selecting the first $r$ elements of each row), and $\Pi_{\perp}(\mathbf{W})\coloneqq \mathbf{W}_{r:}$ denote the projection onto the spurious subspace (the last $d-r$ elements). 
All proofs are deferred to the Appendix.
\begin{proposition} \label{prop:1}
    Consider the gradient-based multi-task algorithm described in Section~\ref{sec:alg} and suppose Assumption \ref{assump:diversity} holds. Further assume $d=\Omega( r^4)$,
and let $\eta = \Theta(1)$, $\lambda_{\mathbf{a}} = 1/\eta $, $\lambda_{\mathbf{w}} = (1+(\eta^2 2^{-r-1})/\pi)/\eta$, and $\nu_{\mathbf{w}} = O(d^{-1.25})$. % and $\sigma_b = O(d^{-1.25})$. 
%$m = \Omega(r 2^r)$, 
% For a subset ${S}\subseteq [m]$, let $\mathbf{W}_{1,S}\in \mathbb{R}^{|S|\times d}$ denote the sub-matrix of $\mathbf{W}$ with rows selected by $S$.
Then for any $m= o(\exp(d))$,  with probability at least $0.99$ over the random initialization we have
% there is a subset of neurons ${S}\subseteq [m]$ of size $|{S}| \geq m/4$ such that for all $j \in {S}$:
% the following two properties are satisfied by the representation learned by MTRL:
\begin{enumerate}
\item $\frac{1}{\nu_{\mathbf{w}}\sqrt{m}}\|\Pi_{\parallel}(\mathbf{W}^+) -  \Omega(\frac{1}{2^r}) % \frac{\eta^2}{2^{r+2}} 
\Pi_{\parallel}(\mathbf{W}^{0}) \|_2 = O\left(  
\frac{r^4 + \log^4(m)}{2^r d} %+ \eta \sigma_w d^{1.5} e^{-d^2/8}
+  \frac{\sqrt{r}d}{\sqrt{T}}
% \eta^2\frac{r^4}{d} %+ \eta \sigma_w d^{1.5} e^{-d^2/8}
% + \eta \frac{\sqrt{r}d}{\sqrt{n}}
\right) $,
% (and scales with init)
% $\|\mathbf{W}_1 - \eta 2^{-r-2} \mathbf{M}_{:r}\mathbf{M}_{:r}^\top \mathbf{W}_0\| =  +  O\left(\sqrt{\frac{r}{d-r}}\right)$
    \item $\frac{1}{\nu_{\mathbf{w}}\sqrt{m}}\|\Pi_{\perp}(\mathbf{W}^{+}) \|_2 = O\left(
\frac{r^{3.5} + \log^{3.5}(m)}{2^r d^{1.5}} %+ \eta\sigma_w d^{1.5} e^{-d^2/8} 
    + \frac{\sqrt{r}d}{\sqrt{T}}
    \right)$
    %     \eta^2 \sigma_w\frac{r^{3.5}}{d^{1.5}2^r} %+ \eta\sigma_w d^{1.5} e^{-d^2/8} 
    % + \eta \sigma_w\frac{\sqrt{r}d}{\sqrt{n}}
    % \item For all $\mathbf{v}\in \{-1,1\}^r$, $\exists j \in \mathcal{S}$ such that $\mathbf{w}_{1,j}^\top \mathbf{v} + b_{1,j} > 0$
    % $\sigma_{\min}(\mathbf{W}_1)$
\end{enumerate}
\end{proposition}
% Note that the error terms in the RHS 
% \textcolor{blue}{I think in the above theorem you should specify what the "poly" is.}
Proposition \ref{prop:1} shows that with high probability over the random initialization, the weights learned by the gradient-based multi-task learning algorithm satisfy two properties,  for sufficiently large $d$ and $T$: (1) the projection of these weights onto the ground-truth subspace is close to a slightly scaled down (by a factor of $2^{-r}$) version of their projection at initialization, and (2) their projection onto the spurious subspace is negligible. These two observations, combined with the fact that the neuron weights have independent standard Gaussian initializations, imply that  the projection of the neuron weights onto the ground-truth subspace dominates their projection onto the spurious subspace. We formalize this observation in the statement below.

% Let $\sigma_{\min}(\Pi_{\parallel}(\mathbf{W}^+{0}))$ denote the minimum singular value of $\Pi_{\parallel}(\mathbf{W}^{0})$, then since initially the minimum singular value $\sigma_{\min}(\Pi_{\parallel}(\mathbf{W}^{0}))\gtrsim \sigma_w\sqrt{mr}$ with high probability due to the Gaussian initialization, we require that 
%  $d \gg r^4$ and $T \gg d^2 2^{2r}$ 
 
%  in order for the energy in  projection onto the ground-truth spurious subspace to dominate the projection onto the spurious subspace. 


%as long as $d\gg r$ and $n \gg d^2 2^r$
% if you condition on this then you no longer have gaussian
% if you remove thse then you no longer have gaussian
% probability you can't throw away neurons. because you don't know the value of their projections
% say that you have 
% workst case scenariom m e^{c^2r} need to choose $c = sqrt(log(m))/sqrt$  

% have large energy ($\Omega(1)$) in the subspace spanned by the label-relevant features ($\text{col}(\mathbf{M}_{:r})$) and small energy $O(d^{-1/2})$ in the subspace of spurious features ($\text{col}(\mathbf{M}_{r:})$). Moreover, Part 3 of Theorem 1 implies that the learned weights are nearly isotropic within the ground-truth $\text{col}(\mathbf{M}_{:r})$.  Effectively, after one step have a random features model with $m$ features on the $r$ label-relevant inputs rather than the ambient $d$ inputs with $d-r$ of them being spurious. 
% \textcolor{blue}{I feel that you need to expand this in words a bit more -- right now it's not easy for the reader to understand the message exactly. e.g. spurious features vanish, and all the relevant features are recovered (maybe with a scaling)? }
% \begin{proof}
    
% \end{proof}
% pick

% union bound over 2^2^r things. this means m scales up by 2^r. which is fine because complexity of error in first prop is log(m)

\begin{theorem}[  ]\label{thm:1}
    Consider the setting in Proposition \ref{prop:1} and let $d =\Omega( r^4 + \log^4(m))$, $m = \Omega(r)$,  and $ T = \Omega( r 2^{2r} d^2) $. Let $\sigma_r(\mathbf{B})$ denote the $r$-th singular value of a matrix $\mathbf{B}$.
Then with probability at least $0.99$ over the random initialization, we have 
\begin{align}  
    \frac{\| \Pi_{\perp}(\mathbf{W}^+) \|_2}{\sigma_{r}( \Pi_{\parallel}(\mathbf{W}^+) )} = O\left( \frac{ {r^{3.5}} + \log^{3.5}(m) }{ d^{1.5} } + \frac{  2^r \sqrt{r} d  }{ \sqrt{T}} \right). \nonumber
\end{align}
\end{theorem}
Theorem \ref{thm:1} characterizes the representation learned by multi-task pre-training in an intuitive manner.  For $d \gg r^4$ and $ T \gg 2^{2r} d^2 $, we have ${\sigma_{r}( \Pi_{\parallel}(\mathbf{W}^+) )} \gg {\| \Pi_{\perp}(\mathbf{W}^+) \|}$, meaning that most of the energy in each neuron weight is in the column space of the ground-truth subspace. This is equivalent to saying that applying $\mathbf{W}^+$ to an input $\mathbf{x}$ essentially projects it onto the ground-truth subspace spanned by the first $r$ coordinates, as desired.
% The key mechanism behind the ability of MTRL to recover the ground-truth features is its task-specific adaptation of the heads, as we discuss below and in Section \ref{sec:sketch}.
% characterizes the representation learned by multi-task pre-training in an intuitive manner .

% (for hypercube, 2. is $O(\eta 2^r/d^{1/2})$)
% $\lambda_1 = \Theta(1)$ 
% \end{theorem}



% A sketch of the proof is provided in Section \ref{sec:sketch} and the full proof is deferred to Appendix \ref{app:thrm1}. 

% It turns out that 
% 

% Difficulty of finite-sample analysis: dealing with non-smooth objects. can't canoncentrate over tasks without having infinite samples first. but to get infinite samples, need to know something about the finite tasks. doable but not trivial


\begin{comment}

\textbf{The importance of adapting the head to each task.} We show in Section \ref{sec:sketch} that adapting the head to each task prior to updating the representation leads to a contrastive loss that encourages feature learning. Here we provide a negative result, describing a failure case when the head is not adapted to each task and we fail to learn the true features. In particular,  we show that SMGD cannot be guaranteed to recover the ground-truth features. Recall that SMGD solves the single-model objective \eqref{obj_glob} via gradient descent. 
\begin{theorem}[Negative Result]\label{thm:negative} Consider a setting with $r=2$ and two tasks with labelling functions:
\begin{align}
    \bar{f}_1^\ast(\sign(\mathbf{z}_{:2})) &\coloneqq \begin{cases} 1 & \text{if } \; z_1 > 0\\
    -1 & \text{otherwise}\\
    \end{cases}, \quad 
    \bar{f}_2^\ast(\sign(\mathbf{z}_{:2})) \coloneqq \begin{cases} 1 & \text{if } \; z_2 > 0\\
    -1 & \text{otherwise.}\\
    \end{cases} \nonumber 
\end{align}
Note that $\bar{\mathcal{T}} = \{\bar{f}_1^*, \bar{f}_2^*\}$ satisfies Assumption \ref{assump:diversity}. Suppose $(\mathbf{W}_T,\mathbf{b}_T,\mathbf{a}_T)$ is a stationary point of the dynamics of SMGD.
% $\mathbf{w}_{j,0}^{\text{SMGD}}\sim N(\mathbf{0}_d,\nu^2\mathbf{I}_d)$  for all $j \in [m]$, and $\mathbf{a}_0^{\text{SMGD}}\sim N(\mathbf{0}_m,\alpha^2\mathbf{I}_m)$, for any $\nu\geq 0,\alpha\geq0,\eta\geq 0,\lambda_1\geq0,\lambda_2\geq 0$, 
Then, 
\begin{align}
   \mathbf{W}_T\mathbf{e}_{1} &= \mathbf{W}_T\mathbf{e}_{2}.
\end{align}
% with probability at least $1 -$ over the random initialization.
\end{theorem}
% // or argue about stationary points. get rid of initialization
Theorem \ref{thm:negative} shows that SMGD can only learn a strict subset of the ground-truth two-dimensional subspace: its intersection with the (one-dimensional) span of $\mathbf{Me}_1+\mathbf{Me}_2$. The, the features it learns are not sensitive to changes in ..  as long as their sum is the same

 
The key to the proof is to notice that the gradient for any neuron weights can be written as
\begin{align}
    \nabla_{\mathbf{w}_j}\mathcal{L}(\mathbf{W},\mathbf{a}) &= \frac{a_j}{2}(1 + \mathbb{E}_{\mathbf{v}}[v_1v_2 \sigma'(\mathbf{v}^\top  \mathbf{w})]) (\mathbf{e}_1 +\mathbf{e}_2) + \frac{a_j}{2}\sum_{\ell=3}^k \mathbb{E}_{\mathbf{v}}[(v_1+v_2) v_\ell \sigma'(  \mathbf{v}^\top  \mathbf{w}_{})] \mathbf{e}_\ell  
\end{align}
thus the gradient only depends on the ground-truth features $\mathbf{e}_1, \mathbf{e}_2$ through their sum $\mathbf{e}_1 + \mathbf{e}_2$. This observation was also made by \cite{shi2022theoretical}, who showed that gradient descent learns the sum of the ground-truth features in the single-task sparse coding setting, which is sufficient to generalize to tasks whose labels are functions of the sum of the latent coordinates, but not the much larger set of tasks that are functions of individual latent coordinates.

\textcolor{blue}{This part is good.}

\end{comment}

% {\color{red}
% \subsection{Downstream Guarantees}

% From Theorem \ref{thm:1}, we have 
% \begin{align}
%     \mathbf{W}_1 &= \eta \mathbf{M}_{:r}\mathbf{M}_{:r}^\top \mathbf{W}_0 + \eta \mathbf{N}_0
% \end{align}
% where each row of $\mathbf{N}_0$ satisfies $\|\mathbf{n}_{0,j}\|_2 = O\left(\tfrac{\|\w_{0}\|_2}{k}\right)$. 


% We consider
% \begin{align}
%     \mathcal{T}^{\text{eval}} \coloneqq \{f^* : \mathbb{R}^k \rightarrow \{-1,1\} \; \text{s.t.}  \}
% \end{align}

% Need to show improvement over random features and single task learning, thus need to quantify sample complexity and/or neuron complexity.

\textbf{Downstream performance.} Now that we have shown that the learned representation recovers the ground-truth subspace, we use this result to show that the representation generalizes to downstream tasks. We consider downstream tasks with input data sharing the same label-relevant $r$ coordinates as the pre-training tasks, but here the input data is  on the hypercube. In particular, input data points $ ( \mathbf{v}, f_{T+1}^*(\mathbf{v}) ) $ are generated by the downstream task $T+1$ as follows:
\begin{align}
 \mathbf{v} \sim \text{Unif}(\{-1,1\}^d),\quad   
 % \mathbf{x} = \mathbf{Mv}, \quad 
 {f}_{T+1}^*(\mathbf{v}) = \bar{f}_{T+1}^*(\mathbf{v}_{:r}) \in \{-1,1\}\label{down}
\end{align}
where, as for pre-training, $\bar{f}_{T+1}^*:\{-1,1\}^r \rightarrow \{-1,1\}$. We formally show below that the learned features generalize to {\em any} such labeling function $\bar{f}_{T+1}^*$.



% \begin{theorem}[End-to-end Guarantee] \label{thm:downstream}
% Let $\mathbf{W}_1$ be the weight matrix learned by multi-task pre-training with $n$ tasks drawn from a collection of tasks satisfying Assumption \ref{assump:diversity}.
% Construct the three-layer ReLU neural network ${g}(\cdot, \boldsymbol{\theta}_1)$ using re-scaled $\mathbf{W}_1$ for first layer weights as in  \eqref{F} and the task-adapted head $\mathbf{a}_{n+1}$ from \eqref{ada}.
% For any downstream task $\mathcal{D}_{n+1}$ described in \eqref{down}, with labeling function $\bar{f}_{n+1}^*$ being any mapping from $\{-1,1\}^r \rightarrow \{-1,1\}$, sample a set $\mathcal{S}_N \coloneqq \{\mathbf{x}_l, {f}_{n+1}^*(\mathbf{x}_{l})\}_{l=1}^N$ of $N$ i.i.d. samples from $\mathcal{D}_{n+1}$.
% % If $ d = \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  )) $, $n = \Omega( d^3 \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  ))  )$,
% % $m = \Theta(r^4\log^8(r) ({ r} + {\log(1/\delta)}))$,  $\hat{m}= \Omega( r^{3.5} \log^4(r) \exp\left( C \log^6(r) r^5 \log(\log(r)/\delta) ) \right) \log(1/\delta) )$, and 
% For any $\delta,\delta'\in (0,1)$ and $ d = \exp(\tilde{\Omega}( r^6  )) $, $n = d^3 \exp(\tilde{\Omega}( r^6  )  )$,
% $m = \tilde{\Theta}(r^6)$,  and $\hat{m}= \exp\left( \tilde{\Omega}(r^6)  \right)$,
% with probability at least $0.99-\delta - \delta'$ over the random  initializations, draw of $n$ pre-training tasks, and draw of $\mathcal{S}_N$,
% \begin{align} % note: r^6 may be lose. for a single task, it is definitely r^5. but we want to generalize to all 2^r tasks
%         \mathcal{L}^{(\text{eval})}_{n+1}(\boldsymbol{\theta}_1,\mathbf{a}_{n+1}) &= 
%         % \tilde{O}\left(\frac{ r^{5} \log^8(r) \log(1/\delta')}{ \sqrt{N}}\right).
%          \left(\frac{ \exp(\tilde{O}(r^6)) }{ \sqrt{N}}\right), 
%     \end{align}
%     where $\tilde{\Omega}(\cdot),\tilde{\Theta}(\cdot)$ and $\tilde{O}(\cdot)$ hide logarithmic factors in $r$, $\delta^{-1}$ and $(\delta')^{-1}$.
%     % with probability at least $1-\delta - $
% % \frac{(\hat{\gamma}=   r^{2.5} \log^4(r) )\log(1/\delta)}{(\lambda_{\mathbf{a}}=1/\hat{\gamma}) \sqrt{N}}
% \end{theorem}
\begin{theorem}[End-to-end Guarantee] \label{thm:downstream}
Let $\mathbf{W}^+$ be the outcome of the multi-task representation learning algorithm described in Section \ref{sec:alg}, and suppose Assumption \ref{assump:diversity} holds. 
% \textcolor{blue}{can you be more specific here about what you mean by "learned". I think $W_1$ is just the outcome of the algorithm. If yes, maybe it's better to say it here?}
Consider a downstream task with labeling function $\bar{f}_{T+1}^*$.
% being a mapping from $\{-1,1\}^r \rightarrow \{-1,1\}$. 
% Let $\mathcal{S}_N \coloneqq \{\mathbf{x}_l, {f}_{n+1}^*(\mathbf{x}_{l})\}_{l=1}^N$ be a set of $N$ i.i.d. samples from $\mathcal{D}_{n+1}$.
Construct the two-layer ReLU embedding $g$ using the rescaled $\mathbf{W}^+$ for first layer weights as in  \eqref{F}, and train the task-adapted head $(\mathbf{a}_{T+1},\tau_{T+1})$ using $n$ i.i.d. samples from the downstream task, as in \eqref{ada}.
% If $ d = \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  )) $, $n = \Omega( d^3 \exp({\Omega}( r^5 \log^6(r)  \log(\log(r)/\delta)  ))  )$,
% $m = \Theta(r^4\log^8(r) ({ r} + {\log(1/\delta)}))$,  $\hat{m}= \Omega( r^{3.5} \log^4(r) \exp\left( C \log^6(r) r^5 \log(\log(r)/\delta) ) \right) \log(1/\delta) )$, and 
 Further, suppose $ d = \exp(\tilde{\Omega}( r^5  )) $, $T = d^3 \exp(\tilde{\Omega}( r^5  )  )$,
$m = \tilde{\Theta}(r^5)$,  and $\hat{m}= \exp\left( \tilde{\Omega}(r^5)  \right)$.
Then for any $\delta,\delta'\in (0,1)$, with probability at least $0.99-\delta - \delta'$ over the random  initializations, draw of $T$ pre-training tasks, and draw of $n$ samples, we have
\begin{align}
        \mathcal{L}^{(\text{eval})}_{T+1} %(\boldsymbol{\theta}_1,\mathbf{a}_{T+1}) 
        &= 
        % \tilde{O}\left(\frac{ r^{5} \log^8(r) \log(1/\delta')}{ \sqrt{N}}\right).
       \frac{ \exp(\tilde{O}(r^5)) }{ \sqrt{n}}, 
    \end{align}
    where $\tilde{\Omega}(\cdot),\tilde{\Theta}(\cdot)$ and $\tilde{O}(\cdot)$ hide logarithmic factors in $r$ and $\delta^{-1}$.
    %and $(\delta')^{-1}$.
    % \textcolor{blue}{don's see why you need both $\delta$ and $\delta'$. CAn you just use a single $\delta$ for $\delta + \delta'$? }
    % with probability at least $1-\delta - $
% \frac{(\hat{\gamma}=   r^{2.5} \log^4(r) )\log(1/\delta)}{(\lambda_{\mathbf{a}}=1/\hat{\gamma}) \sqrt{N}}
\end{theorem}
Theorem \ref{thm:downstream} confirms that the features learned by multi-task pre-training generalize to {\em any} downstream task mapping from $\{-1,1\}^d$ to $\{-1,1\}$ that has the same representation as the tasks in the training, i.e., its label is a function of the first $r$ coordinates. In particular,
if we compose the learned representation with  a random ReLU layer, then learn a linear head using $\exp(\tilde{O}(r^5))$ samples from the task, we solve the task with high probability.
Critically, the number of samples, pre-training tasks, and neurons  needed to ensure the downstream task is solved with high probability are only functions of $r$ and the high-probability constants.  In other words,  multi-task learning reduces the effective dimension of the downstream task  from $d$ to $r$. 
% Since the motivating assumption

 % are generalizable by showing that they can yield a network that 
 % efficiently solves \textit{any} downstream task with latent coordinates on the hypercube, 
 % after adding a random ReLU layer and a trained head. Most importantly, the complexity of solving the new task is independent of dimension

%  \begin{align}
%     \mu &= \Theta (r^{-2.5} \log^{-3}(r) \exp( -C \log^6(r) r^5 \log(\log(r)/\nu) )) \nonumber \\
%     m &= \Theta( r^4\log^8(r) ({ r} + {\log(1/\nu)})) \nonumber \\
%     \hat{m} &= \Theta\left(r^{3.5} \log^4(r) \exp\left( C \log^6(r) r^5 \log(\log(r)/\nu) ) \right) \log(1/\nu)\right) \\
%     &O\left(\left(\frac{r^{4}}{\sqrt{d}} +  d^2 e^{-d^2/8} + \frac{\sqrt{r}d^{1.5}}{\sqrt{n}}\right)(\frac{\sqrt{m}}{\sqrt{\hat{m}}})\right) \\
%     &\rightarrow
% \end{align}


The proof of Theorem \ref{thm:downstream} leverages Proposition \ref{prop:1} to show that the embedding $g$ generated by multi-task learning is close to the embedding of a coupled, ``purified'' two-hidden layer random ReLU network that takes as input {\em only} the $r$ important coordinates. Then, we apply  Theorem 2 from \cite{dirksen2022separation} which implies that w.h.p. a random two-hidden layer ReLU network makes two classes of points on the $r$-dimensional hypercube linearly separable with margin and neuron complexity scaling as functions of the input dimension $r$. 
% Alternatively, we could apply the results on linear separation capabilities of random two-layer ReLU networks in \cite{ghosal2022randomly} without needing to add an extra hidden layer, but doing so would require $\Omega(\exp(2^r))$ samples and neurons. 
% The full proof is found in Appendix \ref{app:down}.
% \citep{hsu2021approximation}

While Theorem \ref{thm:downstream}  ensures generalization to an arbitrary task sharing the ground-truth important coordinates, it can only guarantee generalization to a single such task at once. To ensure that the learned embedding generalizes to a larger set of tasks simultaneously, we have the following corollary.
\begin{corollary}[Generalization to set of tasks] \label{cor:set}
Consider a set  of possible downstream tasks $\mathcal{T}^{(\text{eval})}$ with $|\mathcal{T}^{(\text{eval})}| = D$. Suppose $ d = \exp(\tilde{\Omega}( r^5 \log(D) )) $, $T = d^3 \exp(\tilde{\Omega}( r^5 \log(D)  )  )$,
$m = \tilde{\Theta}(r^5 \log(D) )$,  and $\hat{m}= \exp\left( \tilde{\Omega}(r^5 \log(D) )  \right)$. Construct the two-layer ReLU embedding as in \eqref{F}. Then with probability at least $0.99-\delta$,  any task $T+1$ in $\mathcal{T}^{(\text{eval})}$ 
satisfies
% compute $(\mathbf{a}_{T+1},\tau_{T+1})$ using $n$ samples from task $T+1$,
\begin{align}
        \mathcal{L}^{(\text{eval})}_{T+1} %(\boldsymbol{\theta}_1,\mathbf{a}_{T+1}) 
        &= 
        % \tilde{O}\left(\frac{ r^{5} \log^8(r) \log(1/\delta')}{ \sqrt{N}}\right).
       \frac{ \exp(\tilde{O}(r^5 \log(D))) }{ \sqrt{n}}, 
    \end{align}
    where $\tilde{\Omega}(\cdot),\tilde{\Theta}(\cdot)$ and $\tilde{O}(\cdot)$ hide logarithmic factors in $r$ and $\delta^{-1}$. 
    % \textcolor{blue}{same comment as above about $\delta$}
\end{corollary}
For example, if $\mathcal{T}^{(\text{eval})}$ is the set of all $2^{2^r}$ functions from $\{-1,1\}^r$ to $\{-1,1\}$, then Corollary \ref{cor:set} shows that multi-task pre-training learns a representation that for all such target functions yields an accurate classifier with $O(\exp(\exp(r)))$ sample and neuron complexity. While this is huge in $r$, it is still independent of the ambient dimension $d$.

\textbf{Lower bound: Random features do not generalize.} A consequence of Theorem \ref{thm:downstream} is that multi-task pre-training (albeit with infinite samples) improves the sample and neuron complexity of solving hard downstream tasks by an exponential factor in $d$. 
To show this, we consider the well-studied problem of learning sparse parities, which are functions that output the parity of a small subset of input bits. Formally, for  $\mathbf{u}\in \{0,1\}^d$ with $\|\mathbf{u}\|_1 = r$, an $(r,\mathbf{u})$-sparse parity task is defined as follows.
\begin{definition}
    [$(r,\mathbf{u})$-sparse parity task]
    An $(r,\mathbf{u})$-sparse parity task $\mathcal{D}_{\mathbf{u}}$ has data $(\mathbf{v},f_{\mathbf{u}}^*(\mathbf{v}))$ generated as
$
        \mathbf{v}\sim \text{Unif}(\{-1,1\}^d )$ and $f_{\mathbf{u}}^*(\mathbf{v}) = (-1)^{\mathbf{u}^\top \mathbf{v}},
    $
    where $\mathbf{u}\in \{0,1\}^d$ with $\|\mathbf{u}\|_1 = r$.
\end{definition}
In other words, an $(r,\mathbf{u})$-sparse parity task has labels being the parity of the bits selected by the $r$-sparse vector $\mathbf{u}$.
% The sparse parity problem is then 
% Canonical results show that solving an $(r,\mathbf{u})$-sparse parity task requires $\Omega(d^r)$ samples in the Statistical Query (SQ) model \cite{} and $\Omega(\poly(d))$ noiseless samples via Gaussian elimination. 
While there is a large literature demonstrating the hardness of learning sparse parities in various settings \cite{kearns1998efficient,abbe2020poly,telgarsky2022feature,barak2022hidden,malach2022hardness,kamath2020approximate,goel2019time}, the most relevant results to our setting show that any data-independent, $\hat{m}$-dimensional embedding of $d$ inputs can admit linear classifiers that solve all $(r,\mathbf{u})$-sparse parity tasks only if the dimension $\hat{m}$ and/or the classification margin is exponentially large in $d$. 
% , including the two-layer ReLU representations, as well as the neural tangent kernel \cite{jacot2018neural},  requires 
In particular, the following result adapts Theorem 5 in \cite{barak2022hidden}, which in turn draws on the works of \cite{kamath2020approximate} and \cite{malach2022hardness}.
% Holds for any embedding mapping from $\mathbb{R}^d$ to $\mathbb{R}^{\hat{m}}$, 
\begin{theorem}[] \label{thm:lower}
Consider any embedding $\Psi:\{-1,1\}^d \rightarrow \mathbb{R}^{\hat{m}}$ such that $\|\Psi(\mathbf{v})\|_2 \leq 1 $ for all $\mathbf{v}\in \{-1,1\}^d$. 
For any $\epsilon >0$, if 
$ \hat{m}B^2 \leq \epsilon^2 \binom{d}{r} $
then there exists an $(r,\mathbf{u})$-sparse parity task $\mathcal{D}_{\mathbf{u}}$ s.t.
    \begin{align}
        \inf_{\mathbf{a}: \|\mathbf{a}\|_2 \leq B } \mathbb{E}_{(\mathbf{v},f_{\mathbf{u}}^*(\mathbf{v}))\sim \mathcal{D}_{\mathbf{u}}} \left[ \ell \left(\mathbf{a}^\top \Psi(\mathbf{v}), {f}_{\mathbf{u}}^*(\mathbf{v})\right)   \right]  &\geq 1 - \epsilon.
    \end{align}
\end{theorem}

Theorem \ref{thm:lower} implies that any random feature model requires a number of neurons and/or samples that is exponentially large in $d$ in order to solve a downstream sparse parity task with a linear classifier. On the other hand, our Theorem~\ref{thm:1} guarantees that  after multi-task pre-training, the output embedding admits a linear classifier that solves the $(r,\mathbf{u})$-sparse parity on the extracted $r$ coordinates, with the number of neurons and samples of the downstream task of the order of $\exp(\poly(r))$.
% While our analysis does assume infinite samples for the multi-task representation learning phase, it is not required to solve an $r$-sparse parity task during this phase. 
 





 
 % The motivating setting wherein $r\ll d $,
 
 % you might be able to learn a good representation with one hard task, but it would require d samples per task. if you have a small number of easy tasks you can solve them with few samples, but you cannot learn a good representation. here we show that you can learn a good representation with many tasks and amortize the sample complexity across tasks
 
 % $ \rho(\mathbf{W},\mathcal{T}^{\text{eval}}) \coloneqq \sup_{(i+1)\sim \mathcal{T}^{\text{eval}}}  \mathcal{L}_{i+1}(\mathbf{W},\mathbf{a}_{i+1}(\mathbf{W}))$

% address hypercube

% \begin{theorem}[Existence of a Good Network for any task] \label{thm:exist}
%    Let $\mathbf{W}_1$ be the matrix of weights learned by the multitask learning algorithm.  If $m = \Omega(r2^r)$,  $n = \Omega(rd^4)$, then for any downstream task $\bar{f}_{n+1}^\ast \in \{ \bar{f}_i^*:\{-1,1\}^r \rightarrow \{-1,1\}  \}$,  there exists a vector of biases $\mathbf{b}_{n+1}^*\in \mathbb{R}^{m}$ and a head $\mathbf{a}_{n+1}^*\in \mathbb{R}^m$ such that 
%    \begin{align}
%        \mathcal{L}_{n+1}(\mathbf{W}_1, \mathbf{b}_{n+1}^*, \mathbf{a}_{n+1}^*) = 0.
%    \end{align}
% \end{theorem}

% STATUS
% pretraining proof done
% generlaization using RF, the negtive, then experiments

% First need to show existence. Then approximation.

% Existence:

% euclidean balls of radius 1
% need to put another random relu on top (fine)
% need to bound difference between ideal random and empirical
% of course two-layer relu works. no not obvious

% goal: perfectly classify any input on the hypercube 

% with perfect features:
% $\delta=2/rt(r)$
% need $r^2 e^{r^4}$ neurons in last layer

% just need to bound difference between real network output and ideal network output: 

% for any input, the output of the first layer will differ by at most f(r)/d
% thus output of second layer neurons will differ by at most n f(r)/d, n is hidden width
% output of final layer is a distance at most rt( nhat n2 f(r)2/d2 ) 
% just make d large enugh, done.

% 1. sample complexity of linear classification on top. roughly done
% 2. lower bound for random features (hsu).. but applies only for two  layers
% 3. lower bound for gd
% 4. experiments


% option 2: perfectly classify any input in balls around hypercube vertices








% \begin{theorem}[Approximation of smooth functions]
    
% \end{theorem}







% \begin{theorem}[clusters]
    
% \end{theorem}


% }




% todo:
% negative result for linear setting
% negative result for single head
% pictures and experiments
% bias in thrm 1 proof.

%ideas: 
% learning without input structure is hard in single task setting, but not in multi-task setting?
% how do they learn parities with all features going to average? implies learning parities doesn't imly generalization to other tasks
% maybe this is only true in presence of input structure
% wihtout input structure, if you learned parities you would generalize
% but you can't learn parities without input structure
% the question remains: how to prove generalization to other tasks even with good features?
% note: parities do satisfy 1/2 assumption as long as they are sampled in a particular way, e.g. r is even and the subset size is first sampled uniformly... no they break this assumption. need to argue that it doesnt make sense to learn parities
% these functions are not sensitive to individual values
% can we say that we learn a rep such that there exists a bias and head that can solve any task (yes)
% while on the other hand, learn any singe task cannot guarantee learning weights that generalize
% no. if the task is very non-smooth, then it can require checking all r vertices to predict label
% but learning any single parity or sum-based function cannot gaurantee to generalize.
% but we can't even learn parity without input structure
% our set of tasks can include parities but it cannot be solely parities
% so maybe we need to say that
% 
% plan A: 1. say that we learn a rep that can generalize if train bias and head with xx samples 2. more tasks, better generalization via delta (under uniform task distribution). 3. but we need super-exponentially-many in r tasks so don't talk abut complexities.  (r choose r/2)
% 4. single task cannot guarantee generalization even if trained with infinite samples... but it can if task is hard it works
% plan B: 1. need to show sample complexity improvement with many tasks. 
% 2. sample complexity for new task 
% 3. but we don't have 

% {\color{red} Problem: we cannot get any reasonable downstream guarantees without adding bias...

% What can be learned:

% Binary latents:
% - any polynomial...

% Gaussian latents:
% - single orthants. but requires the coordinates of the head for most neurons to be minus infinity, which complicates optimization
% - halspaces (easy)
% - i don't think we can learn parities...

% approach: need to show the existence of a good network with gaussian features in the right subspace. optimizing the head is a strongly convex problem, so if a good network exists, then optimizing the head will find it
% }'

% if we use binary data:
% error after one step is too large
% but if we can somehow kill this error and get good features, we can show that a good network exists for any function if bias is added
% can use shi et al proof to show that fine-tuning recovers the good network
% if we use gaussian data with sign: 
% 

% idea:
% use gaussian data, kill most of perp in one step, then use gaussianity to effectively go back to the hypercube for other subsequent steps
% --> the problem is that we really need to convert the prefixes back to hypercube, but we only get concentration with $r$
% , not k. and ifr is large, then error from earlier is also large (proportional to $r/k$.


% before first step:

% perp has norm O(rt(k))
% parallel has norm O(1)

% after one step:

% perp has norm O(1/rt(k)) (not O(1)) and is totally gaussian (original direction)

% parallel has norm Omega(1)
% and is gaussian plus a norm 1/k perturbation




% perp always stays completely gaussian (original direction)


\begin{comment}
\subsection{Negative Result} In this subsection we prove that SMGD cannot recover the ground-truth features, regardless of the choice of hyperparameters.

\begin{theorem}[Negative Result]\label{thm:negative} Consider a setting with $r=2$ and two tasks:
\begin{align}
    f_1^\ast(\sign(\mathbf{z}_{:2})) &\coloneqq \begin{cases} 1 & \text{if } \; z_1 > 0\\
    -1 & \text{otherwise}\\
    \end{cases} \nonumber \\
    f_2^\ast(\sign(\mathbf{z}_{:2})) &\coloneqq \begin{cases} 1 & \text{if } \; z_2 > 0\\
    -1 & \text{otherwise.}\\
    \end{cases} \nonumber 
\end{align}
Note that $\mathcal{T} = \{f_1^*, f_2^*\}$ satisfies Assumption \ref{assump:diversity}. For any $T>0$ iterations of SMGD with $\mathbf{w}_{j,0}^{\text{SMGD}}\sim N(\mathbf{0}_d,\nu^2\mathbf{I}_d)$  for all $j \in [m]$, and $\mathbf{a}_0^{\text{SMGD}}\sim N(\mathbf{0}_m,\alpha^2\mathbf{I}_m)$, for any $\nu\geq 0,\alpha\geq0,\eta\geq 0,\lambda_1\geq0,\lambda_2\geq 0$, we have that 
\begin{align}
    \mathbf{W}_T
\end{align}
with probability at least $1 -$ over the random initialization.
    
\end{theorem}
// or argue about stationary points. get rid of initialization

Theorem \ref{thm:negative} shows that 

The key to the proof is to note that the gradient for any neuron weights can be written as
\begin{align}
    \nabla_{\mathbf{w}_j}\mathcal{L}(\mathbf{W},\mathbf{a}) &= \frac{a_j}{2}(1 + \mathbb{E}_{\mathbf{v}}[v_1v_2 \sigma'(\mathbf{v}^\top  \mathbf{w})]) (\mathbf{e}_1 +\mathbf{e}_2) + \frac{a_j}{2}\sum_{\ell=3}^k \mathbb{E}_{\mathbf{v}}[(v_1+v_2) v_\ell \sigma'(  \mathbf{v}^\top  \mathbf{w}_{})] \mathbf{e}_\ell  
\end{align}
thus the gradient only depends on the ground-truth features $\mathbf{e}_1, \mathbf{e}_2$ through their sum $\mathbf{e}_1 + \mathbf{e}_2$. This observation was also made by \cite{shi2022theoretical}, who showed that gradient descent learns the sum of the ground-truth features in the single-task sparse coding setting, which is sufficient to generalize to tasks whose labels are functions of the sum of the latent coordinates, but not the much larger set of tasks that are functions of individual latent coordinates.
\end{comment}

% Single-task learning can't generalize?





==> old_first_step.tex <==

The proof consists of four steps:
\begin{enumerate}
\item  $\mathbf{A}^{\circ,{\mathcal{N}}}_{\perp,\perp} = {\frac{2}{\pi}} \; \frac{\mathbf{w}_{\perp}\mathbf{w}_{\perp}^\top }{\|\mathbf{w}_{\perp}\|_2^2}$ almost surely,
    \item $\left\|\mathbf{A}_{\perp,\perp} - \mathbf{A}^\circ_{\perp,\perp}\right\|_2 = O(k^{-1/2})$ with constant probability, 
    \item $\left\|\mathbf{A}^\circ_{\perp,\perp} - \mathbf{A}^{\circ,\tilde{\mathcal{N}}}_{\perp,\perp}\right\|_2 = O(k^{-1/2})$ with constant probability, and
    \item $\left\|\mathbf{A}^{\circ,\tilde{\mathcal{N}}}_{\perp,\perp} - \mathbf{A}^{\circ,{\mathcal{N}}}_{\perp,\perp}\right\|_2 = O(k^{-1/2})$ with constant probability.
\end{enumerate}
where ....


Together, these imply that $\left\|\mathbf{A}_{\perp,\perp} - {\frac{2}{\pi}} \; \frac{\mathbf{w}_{\perp}\mathbf{w}_{\perp}^\top }{\|\mathbf{w}_{\perp}\|_2^2} \right\|_2 = O(k^{-1/2})$ with constant probability by the triangle inequality. We complete each of the steps below.

\begin{itemize}
    \item \textbf{Step 1: $\mathbf{A}^{\circ,{\mathcal{N}}}_{\perp,\perp} = 2^{-r-2} {\frac{2}{\pi}} \; \frac{\mathbf{w}_{\perp}\mathbf{w}_{\perp}^\top }{\|\mathbf{w}_{\perp}\|_2^2}$.} We have 
\begin{align}
    \mathbf{A}^{\circ,{\mathcal{N}}}_{\perp,\perp} = 2^{-r} \E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top\z) \z]\E_{\z'\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top\z') \z']^\top
\end{align}
which is $ 2^{-r}$ times the outer product of the vector $\E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top\z) \z]$ with itself. 
Note that 
\begin{align}
    \E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top\z) \z] &= \frac{1}{2}\E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}\left[\z - 2 \sigma\left(-\left(\frac{\w_\perp}{\|\w_\perp\|_2}\right)^\top\z\right) \frac{\w_\perp}{\|\w_\perp\|_2}\right]   \label{flip}\\
    &= \E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}\left[ \sigma\left(-\left(\frac{\w_\perp}{\|\w_\perp\|_2}\right)^\top\z \right) \right]  \frac{\w_\perp}{\|\w_\perp\|_2} \nonumber\\
    &= \frac{1}{2}\sqrt{\frac{2}{\pi}} \frac{\w_\perp}{\|\w_\perp\|_2} \label{halfnormal}
\end{align}
where \eqref{flip} follows since  and \eqref{halfnormal} follows since $\left(\frac{\w_\perp}{\|\w_\perp\|_2}\right)^\top\z$ is a Gaussian r.v. with mean 0 and variance 1.




    \item \textbf{Step 2: $\left\|\mathbf{A}_{\perp,\perp} - \mathbf{A}^\circ_{\perp,\perp}\right\|_2 = O(2^{r/2}r k^{-1/2})$ with probability at least $1 - 10^{-4}$.}
% Let $\aaa := \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]$, thus $\mathbf{A}_{\perp,\perp} = $   
We have $\mathbf{A}^\circ_{\perp,\perp} :=  2^{-r}\aaa \aaa^\top$, 
    % \begin{align}
    %     \mathbf{A}^\circ_{\perp,\perp}&:=\E_{\vv \sim \text{Unif}(\mathcal{H}^{k-r})}[\sigma'(\w_\perp^\top \vv)\vv]\E_{\vv \sim \text{Unif}(\mathcal{H}^{k-r})}[\sigma'(\w_\perp^\top \vv)\vv ]^\top \\
    % \mathbf{A}^{\circ,\mathcal{N}}_{\perp,\perp}&:= \E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top \z)\z]\E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top \z)\z]^\top
    % \end{align}
where 
% $b_i:= \E_{v_i \sim \text{Unif}(\{-1,1\}),\z_{-1}\sim \mathcal{N}(\mathbf{0}_{k-r-1},\mathbf{I}_{k-r-1})}[\sigma'(w_{\perp,i} v_i + \w_{\perp,-i}^\top\z_{-1}) v_i]$ for all $i \in [k-r]$. 
$\aaa = \E_{\vv\sim \text{Unif}(\mathcal{H}^{k-r})}[\sigma'(\w_\perp^\top \vv)\vv]$. 
We have
\begin{align}
    &\left\|\mathbf{A}_{\perp,\perp} - \mathbf{A}^\circ_{\perp,\perp}\right\|_2 \nonumber\\
    &= 2^{-r}\left\|2^{-r}\sum_{\mathbf{u} \in \mathcal{H}^r} \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]^\top   - \aaa\aaa^\top\right\|_2 \nonumber \\
    &\leq 
    % 2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}\left\|\left( 2^{-(k-r)}\sum_{\vv \in \mathcal{H}^{k-r}} \sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right)\left(2^{-(k-r)}\sum_{\vv \in \mathcal{H}^{k-r}} \sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right)^\top   - \aaa\aaa^\top\right\|_2 \nonumber \\
    % &= 
    2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}\left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]^\top   - \aaa\aaa^\top\right\|_2 \label{pre} \\
    &= 2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}  \sup_{\y : \|\y\|_2=1} \left| \left\langle \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right], \y \right\rangle^2   - \left\langle\aaa,\y\right\rangle^2\right| \nonumber \\
        &= 2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}  \sup_{\y : \|\y\|_2=1} \left|\left( \left\langle \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right], \y \right\rangle+\left\langle\aaa,\y\right\rangle \right)\left( \left\langle \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right], \y \right\rangle  - \left\langle\aaa,\y\right\rangle\right)\right| \nonumber \\
        &\leq  2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}  \sup_{\y : \|\y\|_2=1} \left| \left\langle \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right], \y \right\rangle+\left\langle\aaa,\y\right\rangle \right|\sup_{\y' : \|\y'\|_2=1} \left| \left\langle \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right], \y' \right\rangle  - \left\langle\aaa,\y'\right\rangle\right| \nonumber \\ 
        &=  2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r}  \left\| \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]+\aaa \right\|_2 \left\|  \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]  - \aaa\right\|_2 \nonumber \\ 
        &= 2^{-r} \max_{\mathbf{u} \in \mathcal{H}^r} \left(\|\aaa\|_2 + \left\| \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]-\aaa \right\|_2\right) \left\|  \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right]  - \aaa\right\|_2 \label{186} 
    % &\leq 2^{-r}\max_{\mathbf{u} \in \mathcal{H}^r} \left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] + \aaa\right\|_2 \left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa\right\|_2 
\end{align}
% &=  2^{-r} \sup_{\y : \|\y\|_2=1} | \langle \y, \aaa\rangle^2 - \langle \y, \bbb\rangle^2 |\nonumber \\
        % &=  2^{-r}\sup_{\y : \|\y\|_2=1} | (\langle \y, \aaa\rangle - \langle \y, \bbb\rangle)(\langle \y, \aaa\rangle + \langle \y, \bbb\rangle) |\nonumber \\
        % &\leq  2^{-r}\sup_{\y : \|\y\|_2=1} | \langle \y, \aaa\rangle - \langle \y, \bbb\rangle| \sup_{\y' : \|\y'\|_2=1}|\langle \y', \aaa\rangle + \langle \y, \bbb\rangle |\nonumber \\
Thus we can upper bound $\left\|\mathbf{A}_{\perp,\perp} - \mathbf{A}^\circ_{\perp,\perp}\right\|_2 $ by upper bounding $\|\aaa\|_2$ and $\left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa\right\|_2$ for all $\uu \in \uH^r$. We start by controlling $\left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa\right\|_2$. We will upper bound $\|\aaa\|_2$ {\color{red}later}.

For any $\uu \in \uH^r$, we will control $\left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa\right\|_2$ by controlling each of the  coordinates of $\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa$. Note that each coordinate is identically distributed. The first coordinate is:
\begin{align}
    \E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) v_1 \right] - \E_{\vv} \left[\sigma'(  \mathbf{w}_{\perp}^\top\mathbf{v} ) v_1 \right] =\E_{\vv} \left[(\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} )- \sigma'( \mathbf{w}_{\perp}^\top\mathbf{v} )) v_1 \right]
\end{align}
This is a scalar-valued random variable that is a function of $\w$.
Denote it as $f_1(\w)$, i.e. $f_1(\w):= \E_{\vv} \left[(\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} )- \sigma'( \mathbf{w}_{\perp}^\top\mathbf{v} )) v_1 \right]$.
By symmetry we have that $\E_{\w}[f_1(\w)]=0$, in particular,
\begin{align}
    \E_{\w}[f_1(\w)] &= \frac{1}{2}\E_{\w,\vv_{-1}}[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + {w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1} )- \sigma'( {w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1}))] \nonumber \\
    &\quad - \frac{1}{2}\E_{\w,\vv_{-1}}[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} -{w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1} )- \sigma'( -{w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1} ))] \nonumber \\
    &= \frac{1}{2}(\Pr_{\w,\vv_{-1}}[ \mathbf{w}_{\parallel}^\top \mathbf{u} + {w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1} >0] - \Pr_{\w,\vv_{-1}}[ \mathbf{w}_{\parallel}^\top \mathbf{u} - {w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1} >0] )
    % - \sigma'( {w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1}))] 
    \nonumber \\
    &\quad + \frac{1}{2}(\Pr_{\w,\vv_{-1}}[ -{w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1} >0]- \Pr_{\w,\vv_{-1}}[ {w}_{\perp,-1} + \mathbf{w}_{\perp,-1}^\top\mathbf{v}_{-1} >0]) \nonumber \\
    &=0+0=0
\end{align}
where the first equality follows by the tower property and the last equality follows by the fact that ${w}_{\perp,-1}$ has the same distribution as $-{w}_{\perp,-1}$.




Next we control the second moment. 
\begin{align}
    \E_{\w}[f_1(\w)^2] &= \E_{\w}\left[\left(\E_{\vv} \left[(\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} )- \sigma'( \mathbf{w}_{\perp}^\top\mathbf{v} )) v_1 \right]\right)^2\right] \\
    &= \E_{\w}\left[\E_{\vv,\vv'} \left[(\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} )- \sigma'( \mathbf{w}_{\perp}^\top\mathbf{v} ))(\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v}' )- \sigma'( \mathbf{w}_{\perp}^\top\mathbf{v}' )) v_1 v_1' \right]\right] \\
    &= \E_{\vv,\vv'} \left[v_1 v_1' \Pr_{\w}\left[\mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v}>0 \cap \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v}' >0\right]\right] \nonumber \\
    &\quad + \E_{\vv,\vv'} \left[v_1 v_1' \Pr_{\w}\left[ \mathbf{w}_{\perp}^\top\mathbf{v}>0 \cap  \mathbf{w}_{\perp}^\top\mathbf{v}' >0\right]\right]   \nonumber \\
    &\quad - 2 \E_{\vv,\vv'} \left[v_1 v_1' \Pr_{\w}\left[\mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v}>0 \cap  \mathbf{w}_{\perp}^\top\mathbf{v}' >0\right]\right] \nonumber\\
    &= \E_{\vv,\vv'} \left[v_1 v_1' \left(\frac{1}{2}-\frac{1}{2\pi} \cos^{-1}\left(\frac{r + \vv^\top \vv'}{k}\right)\right)\right]  + \E_{\vv,\vv'} \left[v_1 v_1' \left(\frac{1}{2}-\frac{1}{2\pi} \cos^{-1}\left(\frac{\vv^\top \vv'}{k-r}\right)\right)\right]   \nonumber \\
    &\quad - 2 \E_{\vv,\vv'} \left[v_1 v_1' \left(\frac{1}{2}-\frac{1}{2\pi} \cos^{-1}\left(\frac{\vv^\top \vv'}{\sqrt{k}\sqrt{k-r}}\right)\right)\right] \nonumber\\
    &= -\frac{1}{2\pi} \E_{\vv,\vv'} \left[v_1 v_1' \cos^{-1}\left(\frac{r + \vv^\top \vv'}{k}\right)\right] -\frac{1}{2\pi} \E_{\vv,\vv'} \left[v_1 v_1' \cos^{-1}\left(\frac{\vv^\top \vv'}{k-r}\right)\right]   \nonumber \\
    &\quad +\frac{1}{\pi}  \E_{\vv,\vv'} \left[v_1 v_1' \cos^{-1}\left(\frac{\vv^\top \vv'}{\sqrt{k}\sqrt{k-r}}\right)\right] \label{190}
    % \mathbf{w}_{\perp}^\top\mathbf{v} >0 ))(\sigma'( )- \sigma'( \mathbf{w}_{\perp}^\top\mathbf{v}' ))  \right]
\end{align}
% \E_{\vv} \left[(\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} )- \sigma'( \mathbf{w}_{\perp}^\top\mathbf{v} )) v_1 \right]
Note that the term inside each expectation is only a function of $v_1 v_1'$ and the Hamming distance between $\vv_{-1}$ and $\vv'_{-1}$. For any $\vv_{-1}\in \uH^{k-r-1}$, there are ${k-r-1 \choose q}$ vertices $\vv'_{-1}\in \uH^{k-r-1}$ that are Hamming distance $q$ away from $\vv_{-1}$. Thus we can write
\begin{align}
   & \E_{\vv,\vv'} \left[v_1 v_1' \cos^{-1}\left(\frac{r + \vv^\top \vv'}{k}\right)\right] \nonumber \\
   &= \frac{1}{2}\E_{\vv, \vv'_{-1}} \left[ \cos^{-1}\left(\frac{r + 1 + \vv_{-1}^\top \vv'_{-1}}{k}\right)\right] -  \frac{1}{2}\E_{\vv, \vv'_{-1}} \left[ \cos^{-1}\left(\frac{r - 1 + \vv_{-1}^\top \vv'_{-1}}{k}\right)\right] \nonumber\\
   &= \frac{1}{2}\E_{\vv} \left[ 2^{-(k-r-1)}\sum_{q=0}^{k-r-1}{k-r-1 \choose q}\cos^{-1}\left(\frac{r - 1 + k-r-1-2q}{k}\right)\right] \nonumber\\
   &\quad -  \frac{1}{2}\E_{\vv} \left[ 2^{-(k-r-1)}\sum_{q=0}^{k-r-1}{k-r-1 \choose q}\cos^{-1}\left(\frac{r - 1 + k-r-1-2q}{k}\right)\right] \nonumber\\
   &=  2^{-(k-r)}\sum_{q=0}^{k-r-1}{k-r-1 \choose q}\left( \cos^{-1}\left(1 - \frac{2q}{k}\right) - \cos^{-1}\left(1 - \frac{2(q+1)}{k}\right) \right)
\end{align}
Note that the binomial coefficients place largest weight on the terms in the sum with $q\approx (k-r-1)/2$, and for these values of $q$, the inputs to the $\cos^{-1}$ functions are close to zero. We will use the Taylor series approximation of $\cos^{-1}$ around zero to simplify the sum. First assume that $k-r-1$ is even. We have
    \begin{align}
   & \E_{\vv,\vv'} \left[v_1 v_1' \cos^{-1}\left(\frac{r + \vv^\top \vv'}{k}\right)\right] \nonumber \\
   &=  2^{k-r} {k-r-1 \choose \frac{k-r-1}{2}}\left( \cos^{-1}\left(\frac{r +1 }{k}\right) - \cos^{-1}\left(\frac{r-1}{k}\right) \right)\nonumber \\
   &\quad + 2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'}\left( \cos^{-1}\left(\frac{r +1 - 2q'}{k}\right) - \cos^{-1}\left(\frac{r-1-2q'}{k}\right) \right) \nonumber\\
   &\quad + 2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left( \cos^{-1}\left(\frac{r +1 + 2q'}{k}\right) - \cos^{-1}\left(\frac{r-1+2q'}{k}\right) \right) \nonumber %\\
   % &=  2^{k-r} {k-r-1 \choose \frac{k-r-1}{2}}\left( \cos^{-1}\left(\frac{r +1 }{k}\right) - \cos^{-1}\left(\frac{r-1}{k}\right) \right)\nonumber \\
   % &\quad + 2^{k-r} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'}\left( \cos^{-1}\left(\frac{r +1 - 2q'}{k}\right) - \cos^{-1}\left(\frac{r-1-2q'}{k}\right) \right) \nonumber\\
   % &\quad + 2^{k-r} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left( \cos^{-1}\left(\frac{r +1 + 2q'}{k}\right) - \cos^{-1}\left(\frac{r-1+2q'}{k}\right) \right) \nonumber \\
\end{align}
Taking the Taylor series expansion of the $\cos^{-1}$ functions in the first line, we obtain
\begin{align}
    &\cos^{-1}\left(\frac{r +1 }{k}\right) - \cos^{-1}\left(\frac{r-1}{k}\right) \nonumber \\
    &= \frac{\pi}{2} - \left(\frac{r +1 }{k} + \frac{(r +1)^3 }{6 k^3} + O\left(\frac{r^5}{k^5}\right) \right) -  \frac{\pi}{2} + \left(\frac{r -1 }{k} + \frac{(r -1)^3 }{6 k^3} + O\left(\frac{r^5}{k^5}\right) \right) \nonumber \\
    &= -\frac{2}{k} - \frac{ 3r^2+1 }{3k^3}  + O\left(\frac{r^4}{k^5}\right)
\end{align}
Similarly, for any $q' \in \left[\frac{k-r-1}{2}\right]$, 
\begin{align}
    &\cos^{-1}\left(\frac{r +1 - 2q'}{k}\right) - \cos^{-1}\left(\frac{r-1-2q'}{k}\right) \nonumber \\
    &= \frac{\pi}{2} - \left(\frac{r +1 -2q'}{k} + \frac{(r +1 -2q')^3 }{6 k^3} + O\left(\frac{(r-2q')^4}{k^5}\right) \right) -  \frac{\pi}{2} + \left(\frac{r -1 -2q' }{k} + \frac{(r -1 - 2q')^3 }{6 k^3} + O\left(\frac{(r-2q')^4}{k^5}\right) \right) \nonumber \\
    &= -\frac{2}{k} - \frac{ 3(r-2q')^2+1 }{3k^3}  + O\left(\frac{(r-2q')^4}{k^5}\right)
\end{align}
and 
\begin{align}
        \cos^{-1}\left(\frac{r +1 + 2q'}{k}\right) - \cos^{-1}\left(\frac{r-1+2q'}{k}\right)
    &= -\frac{2}{k} - \frac{ 3(r+2q')^2+1 }{3k^3}  + O\left(\frac{(r+2q')^4}{k^5}\right)
\end{align}
Thus
\begin{align}
    & \E_{\vv,\vv'} \left[v_1 v_1' \cos^{-1}\left(\frac{r + \vv^\top \vv'}{k}\right)\right] \nonumber \\
   &=  2^{-(k-r)} {k-r-1 \choose \frac{k-r-1}{2}}\left(  -\frac{2}{k} - \frac{ 3r^2+1 }{3k^3}  + O\left(\frac{r^4}{k^5}\right)  \right)\nonumber \\
   &\quad + 2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'}\left(   -\frac{2}{k} - \frac{ 3(r-2q')^2+1 }{3k^3}  + (r-2q')^4 O\left({k^{-5}}\right)  \right) \nonumber\\
   &\quad + 2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(  -\frac{2}{k} - \frac{ 3(r+2q')^2+1 }{3k^3}  + (r+2q')^4 O\left({k^{-5}}\right)  \right) \nonumber \\
   &= -\frac{1}{k} -  2^{-(k-r)} {k-r-1 \choose \frac{k-r-1}{2}} \frac{ r^2 }{k^3} - 2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \frac{ (r-2q')^2 + (r+2q')^2}{k^3} \nonumber \\
   &\quad + 2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} (q')^4 O\left({k^{-5}}\right)  + O\left({k^{-3}}\right) + O\left(\frac{r^4}{k^5}\right) \nonumber \\
   &= -\frac{1}{k}  - 2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \frac{ 8(q')^2}{k^3}  +2^{-(k-r)} \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} (q')^4 O\left({k^{-5}}\right) + O\left(\frac{r^2}{k^3}\right)  \label{show}
\end{align}
% we will show that the entire expression above is $O(k^{-3})$.

% the sum of $O\left(\frac{(q')^4}{k^5}\right) $ terms is $O(k^{-3})$, and show that the $O(k^{-1})$  and $O(k^{-2})$ terms in the previous sum of 


For the sum of $(q')^2$ terms, we have
% \begin{align}
%     \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} (q')^2 &= \underbrace{\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} + q'\right)^2}_{T_1} - \underbrace{\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2}\right)^2}_{T_2}\nonumber \\
%     &\quad - \underbrace{2\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2}q'\right)^2 }_{T_3}\nonumber 
% \end{align}
% For $T_1$, we have
\begin{align}
     &\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} (q')^2  \nonumber \\
     &= \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} + q'\right)^2\nonumber \\
    &= \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} + q'\right)^2  + \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2} - q'\right)^2  \nonumber \\
    &\quad - \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} \right)^2 - \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \frac{k-r-1}{2} q' \nonumber \\
    &\quad - \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2} \right)^2 + \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \frac{k-r-1}{2} q' \nonumber \\
    &= \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} + q'\right)^2  + \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2} - q'\right)^2  \nonumber \\
    &\quad - \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} \right)^2 - \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2} \right)^2 \nonumber \\
    &= \frac{1}{2}\sum_{q=0}^{{k-r-1}}{k-r-1 \choose q} q^2 - \frac{1}{2}{k-r-1 \choose \frac{k-r-1}{2}}\left(\frac{k-r-1}{2}\right)^2  \nonumber \\
    &\quad - \frac{1}{2}  \left(\frac{k-r-1}{2} \right)^2\sum_{q=0}^{k-r-1}{k-r-1 \choose q} +  \frac{1}{2}{k-r-1 \choose \frac{k-r-1}{2}} \left(\frac{k-r-1}{2} \right)^2 \nonumber \\
    &= (k-r-1 + (k-r-1)^2 )2^{k-r-4} - (k-r-1)^2 2^{k-r-4} \nonumber \\
    &= (k-r-1 )2^{k-r-4}\label{second}
    % \sum_{q=}^{{k-r-1}{k-r-1 \choose q} q^2 - {k-r-1 \choose \frac{k-r-1}{2}}(\frac{k-r-1}{2})^2 - 
\end{align}
% [which gives us the correct result]
Similarly,
\begin{align}
     &\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} (q')^4  \nonumber \\
     &= \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} + q'\right)^2\nonumber \\
    &= \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} + q'\right)^4  + \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2} - q'\right)^4  \nonumber \\
    &\quad - \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2} \right)^4 -\frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2} \right)^4 
    % - \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \frac{k-r-1}{2} q'
    \nonumber \\
    &\quad - 3\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2}\right)^2 (q')^2 - 3\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2}\right)^2 (q')^2
    % \frac{1}{2}\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \left(\frac{k-r-1}{2} \right)^2 + \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}- q'} \frac{k-r-1}{2} q' 
    \nonumber \\
    &= \frac{1}{2} \sum_{q=0}^{k-r-1} {k-r-1 \choose  q} q^4  - \frac{1}{2} {k-r-1 \choose  \frac{k-r-1}{2}} \left(\frac{k-r-1}{2}\right)^4  \nonumber \\
    &\quad - \frac{1}{2}\left(\frac{k-r-1}{2} \right)^4\sum_{q=0}^{{k-r-1}}{k-r-1 \choose q}  + \frac{1}{2} {k-r-1 \choose  \frac{k-r-1}{2}} \left(\frac{k-r-1}{2}\right)^4
    % - \sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \frac{k-r-1}{2} q'
    \nonumber \\
    &\quad - 3 \times (k-r-1 )2^{k-r-4}
    \nonumber \\
    &= 2^{k-r-5}( (k-r-1)^4 + 6 (k-r-1)^3 + 3(k-r-1)^2 - 2(k-r-1)) - 2^{k-r-5}( (k-r-1)^4 + 6 (k-r-1)^3) \nonumber \\
    &= 2^{k-r-5}(  3(k-r-1)^2 - 2(k-r-1)) 
\end{align}
where we have used the computation of $\sum_{q'=1}^{\frac{k-r-1}{2}}{k-r-1 \choose \frac{k-r-1}{2}+ q'} \left(\frac{k-r-1}{2}\right)^2 (q')^2 $ from \eqref{second} and the equality $ \sum_{q=0}^{n} {n \choose  q} q^4  = 2^{n-4}(n^4 + 6 n^3 + 3n^2 - 2n)$ (Boros and Moll 2004, pp. 14-15, and Wolfram).

Combining these two equalities with \eqref{show} yields
\begin{align}
    & \E_{\vv,\vv'} \left[v_1 v_1' \cos^{-1}\left(\frac{r + \vv^\top \vv'}{k}\right)\right] = -\frac{1}{ k} -\frac{1}{2 k^2} + O\left(\frac{r^2}{k^3}\right)
    % = -\frac{1}{2\pi k} -\frac{1}{4\pi k^2} + O\left(\frac{r^2}{k^3}\right)
\end{align}
For the other two terms in \eqref{190}, we argue similarly and obtain % above was a special case of (r' + ...)/(k - r + r') with r' = r. Now r' = 0
\begin{align}
    \E_{\vv,\vv'} \left[v_1 v_1' \cos^{-1}\left(\frac{\vv^\top \vv'}{k-r}\right)\right] &= -\frac{1}{ k-r } -\frac{1}{2 (k-r)^2} + O\left(\frac{1}{(k-r)^3}\right) \label{1990} \\
    \E_{\vv,\vv'} \left[v_1 v_1' \cos^{-1}\left(\frac{\vv^\top \vv'}{\sqrt{k}\sqrt{k-r}}\right)\right] &= -\frac{1}{ \sqrt{k}\sqrt{k-r} } -\frac{1}{2 k(k-r)} + O\left(\frac{1}{k^{3/2}(k-r)^{3/2}}\right) 
\end{align}
This implies that \eqref{190} simplifies to
\begin{align}
    \E_{\w}[f_1(\w)^2] &= \frac{1}{2\pi}\left(\frac{1}{k}+ \frac{1}{k-r} - \frac{2}{\sqrt{k}\sqrt{k-r}}  \right) + \frac{1}{4\pi}\left(  \frac{1}{k^2}+ \frac{1}{(k-r)^2} - \frac{2}{{k}({k-r})} \right)+ O\left(\frac{1}{(k-r)^3}\right) \nonumber \\
    &= \frac{1}{2\pi} \frac{(\sqrt{k} - \sqrt{k-r})^2}{k(k-r)} + \frac{1}{4\pi} \frac{({k} - ({k-r}))^2}{k^2(k-r)^2}+ O\left(\frac{1}{(k-r)^3}\right)\nonumber \\
    &= O\left(\frac{r^2}{k^2(k-r)}\right) \nonumber \\
    &= O\left(\frac{r^2}{k^3}\right) 
\end{align}
where the second-to-last equality follows due to the numerical inequality $0<\sqrt{k}-\sqrt{k-r}\leq \frac{r}{\sqrt{k}}$ for all $k\geq r \geq 0$.
Now that we have bounded the first and second moments of $f_1(\w)$, we can use Chebyshev's Inequality to write
\begin{align}
    \Pr_{\w}\left[|f_1(w)|\geq \frac{2^{r/2}crk^{1/2}}{C k^{3/2}}\right] \leq \frac{1}{2^r c^2 k}
\end{align} for some constants $c,C$.
Since each coordinate of $\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa =  \E_{\vv} \left[(\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} )- \sigma'( \mathbf{w}_{\perp}^\top\mathbf{v} )) \vv \right]$ is identically distributed, 
\begin{align}
    \Pr_{\w}\left[|f_i(w)|\geq \frac{2^{r/2}crk^{1/2}}{Ck^{3/2}}\right] \leq \frac{1}{2^r c^2 k}
\end{align} 
for all $i \in [k-r]$, where $f_i(\w):= \E_{\vv} \left[(\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} )- \sigma'( \mathbf{w}_{\perp}^\top\mathbf{v} )) v_i \right]$.
Thus, by a union bound over all coordinates, we have 
\begin{align}
   \Pr_{\w}\left[\left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa\right\|_2^2 \geq \frac{2^r c^2 r^2}{C^2 k} \right]& \leq \Pr_{\w}\left[\cup_{i=1}^{k-r} |f_i(w)|\geq \frac{2^{r/2} c r}{C k}\right] \nonumber \\ %\frac{c'rk^{1/2}}{k^{3/2}}
   &\leq \sum_{i=1}^{k-r} \Pr_{\w}\left[|f_i(w)|\geq \frac{ 2^{r/2} c rk^{1/2}}{C k^{3/2}}\right]\nonumber \\
   &\leq \frac{1}{2^{r} c^2} 
\end{align}
Finally we union bound over all $\mathbf{u}\in \uH^r$:
\begin{align}
    \Pr_{\w}\left[ \cup_{\mathbf{u} \in \mathcal{H}^r} \left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa\right\|_2^2 \geq \frac{2^r c^2 r^2}{C^2 k} \right] \leq \frac{1}{c^2} 
\end{align}
Choose $c=100$ to complete the proof of this step.




% 
% ---------------
% Similarly, 
% \begin{align}
%     &\E_{\vv,\vv'} \left[v_1 v_1' \cos^{-1}\left(\frac{\vv^\top \vv'}{k-r}\right)\right] \nonumber \\
%     &= 2^{k-r}\sum_{q=0}^{k-r-1}{k-r-1 \choose q}\left( \cos^{-1}\left(1 - \frac{2q}{k-r}\right) - \cos^{-1}\left(1 - \frac{2(q+1)}{k-r}\right) \right) 
% \end{align}
% and 
% \begin{align}
%     &\E_{\vv,\vv'} \left[v_1 v_1' \cos^{-1}\left(\frac{\vv^\top \vv'}{k-r}\right)\right] \nonumber \\
%     &= 2^{k-r}\sum_{q=0}^{k-r-1}{k-r-1 \choose q}\left( \cos^{-1}\left(\frac{k-r-2q}{\sqrt{k}\sqrt{k-r}}\right) - \cos^{-1}\left( \frac{k-r-2(q+1)}{\sqrt{k}\sqrt{k-r}}\right) \right) 
% \end{align}









    \item \textbf{Step 3: $\left\|\mathbf{A}^\circ_{\perp,\perp} - \mathbf{A}^{\circ,\tilde{\mathcal{N}}}_{\perp,\perp}\right\|_2 = O(k^{-1/2})$ with constant probability.}

Recall $ \mathbf{A}^\circ_{\perp,\perp}:=  2^{-r}\aaa \aaa^\top$ and $\mathbf{A}^{\circ,\tilde{\mathcal{N}}}_{\perp,\perp}:=  2^{-r} \bbb\bbb^\top$
    % \begin{align}
    %     \mathbf{A}^\circ_{\perp,\perp}&:=\E_{\vv \sim \text{Unif}(\mathcal{H}^{k-r})}[\sigma'(\w_\perp^\top \vv)\vv]\E_{\vv \sim \text{Unif}(\mathcal{H}^{k-r})}[\sigma'(\w_\perp^\top \vv)\vv ]^\top \\
    % \mathbf{A}^{\circ,\mathcal{N}}_{\perp,\perp}&:= \E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top \z)\z]\E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top \z)\z]^\top
    % \end{align}
where 
% $b_i:= \E_{v_i \sim \text{Unif}(\{-1,1\}),\z_{-1}\sim \mathcal{N}(\mathbf{0}_{k-r-1},\mathbf{I}_{k-r-1})}[\sigma'(w_{\perp,i} v_i + \w_{\perp,-i}^\top\z_{-1}) v_i]$ for all $i \in [k-r]$. 
$\aaa = \E_{\vv\sim \text{Unif}(\mathcal{H}^{k-r})}[\sigma'(\w_\perp^\top \vv)\vv] $ and $\mathbf{b}= [b_1,\dots,b_{k-r}]$, and $b_i:= \E_{v_i \sim \text{Unif}(\{-1,1\}),\z_{-i}\sim \mathcal{N}(\mathbf{0}_{k-r-1},\mathbf{I}_{k-r-1})}[\sigma'(w_{\perp,i} v_i + \w_{\perp,-i}^\top\z_{-i}) v_i]$ for all $i \in [k-r]$. The proof for this step follows the same structure as the proof for Step 2. We first note that 
    \begin{align}
        \left\|\mathbf{A}^\circ_{\perp,\perp} - \mathbf{A}^{\circ,\mathcal{N}}_{\perp,\perp}\right\|_2 &=  2^{-r}\left\|\aaa \aaa^\top - \bbb \bbb^\top \right\|_2 \nonumber \\
        % &=  2^{-r} \sup_{\y : \|\y\|_2=1} | \langle \y, \aaa\rangle^2 - \langle \y, \bbb\rangle^2 |\nonumber \\
        % &=  2^{-r}\sup_{\y : \|\y\|_2=1} | (\langle \y, \aaa\rangle - \langle \y, \bbb\rangle)(\langle \y, \aaa\rangle + \langle \y, \bbb\rangle) |\nonumber \\
        % &\leq  2^{-r}\sup_{\y : \|\y\|_2=1} | \langle \y, \aaa\rangle - \langle \y, \bbb\rangle| \sup_{\y' : \|\y'\|_2=1}|\langle \y', \aaa\rangle + \langle \y, \bbb\rangle |\nonumber \\
        &\leq  2^{-r} \|\aaa +\bbb \|_2 \|\aaa - \bbb\|_2 \label{1866}
    \end{align}
analagously as in \eqref{186}. 

We first bound $\|\aaa - \bbb\|_2$. Note that each coordinate of $\aaa - \bbb$ is identically distributed (although they are not independent). We will bound the first coordinate with high probability then use a union bound to bound all of the coordinates. 

Note that the first coordinate is a random variable that is a function of the random vector $\mathbf{w}_{\perp}$. 

Also, note that we can rewrite $b_1$ as:
\begin{align}
    b_1 &= \E_{v_1,\z_{-1}}[\sigma'(w_{\perp,1} v_1 +\w_{\perp,-1}^\top\z_{-1}) v_1] \nonumber \\
    &= \frac{1}{2}\E_{\z_{-1}}[\sigma'(w_{\perp,1} +\w_{\perp,-1}^\top \z_{-1} )] - \frac{1}{2}\E_{\z_{-1}}[\sigma'(-w_{\perp,1} +\w_{\perp,-1}^\top \z_{-1} )] \nonumber \\
    &= \frac{1}{2}\left(\mathbb{P}_{\z_{-1}}\left( \w_{\perp,-1}^\top \z_{-1} > -  w_{\perp,1} \right) - \mathbb{P}_{\z_{-1}}\left( \w_{\perp,-1}^\top \z_{-1} >   w_{\perp,1} \right)\right)\nonumber \\
    &= \frac{1}{2}\left( \mathbb{P}_{\z_{-1}}\left( \w_{\perp,-1}^\top \z_{-1} <   w_{\perp,1} \right) - \mathbb{P}_{\z_{-1}}\left( \w_{\perp,-1}^\top \z_{-1} <   -w_{\perp,1} \right)\right)\nonumber \\
    &= \frac{1}{4}\left( \erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right) - \erf\left( -\frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right) \right) \label{erf}
     \\
    &= \frac{1}{2} \erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right)  \label{odd}
\end{align}
where \eqref{erf} follows by noting that $\w_{\perp,-1}^\top \z_{-1}$ is a Gaussian r.v. with mean zero and variance $\|\w_{\perp,-1}\|_2^2$, and using its CDF (with erf denoting the error function), and \eqref{odd} follows since the error function is odd.


We have 
\begin{align}
    \E_{\w_\perp} [a_1 - b_1] &=  \E_{\w_\perp}\left[ \E_{\vv}[\sigma'(\w_\perp^\top\vv) v_1]\right] - \E_{\w_\perp}\left[\E_{v_1,\z_{-1}}[\sigma'(w_{\perp,1} v_1 +\w_{\perp,-1}^\top\z_{-1}) v_1]\right]
    \nonumber \\
    &= 0 - 0 = 0
\end{align}
by symmetry of $\w_{\perp},\vv$ and $\z$. 
Next,

\begin{align}
    \E_{\w_\perp} [(a_1 - b_1)^2] 
    % &= \E_{\w_\perp} \left[ \left(\E_{\vv}[\sigma'(\w_\perp^\top\vv) v_1] - \E_{\z}[\sigma'(\w_\perp^\top\z) z_1]\right)^2\right]
    % \nonumber \\
    &= T_1 - T_2 + T_3 \label{3t}
\end{align}
where $T_1 \coloneqq \E_{\w_\perp} \left[ a_1^2\right]$, $T_2 \coloneqq 2\E_{\w_\perp} \left[ a_1 b_1\right]$, and $T_3 \coloneqq \E_{\w_\perp} \left[ b_1^2\right]$. We start with $T_1$.
\begin{align}
    % 
    T_1 &:= \E_{\w_\perp} \left[ a_1^2\right]\nonumber \\ 
    % &=\E_{\w_\perp} \left[ \left(\E_{\vv}[\sigma'(\w_\perp^\top\vv) v_1] \right)^2\right] \nonumber \\
    &= \E_{\w_\perp} \left[ \E_{\vv, \vv'}[\sigma'(\w_\perp^\top\vv) \sigma'(\w_\perp^\top\vv') v_1 v_1' ]\right]  \nonumber \\
    &= \E_{\vv, \vv'} \left[ v_1 v_1' \mathbb{P}_{\w_\perp}[\sigma'(\w_\perp^\top\vv) \sigma'(\w_\perp^\top\vv')  ]\right]  \nonumber \\
    &= -\frac{1}{2\pi} \E_{\vv, \vv'} \left[ v_1 v_1' \cos^{-1}\left(\frac{\vv^\top \vv'}{k-r} \right)\right]  \nonumber \\
    &= \frac{1}{2\pi}\left( \frac{1}{k-r} + \frac{1}{(k-r)^2}\right) + O\left(\frac{1}{(k-r)^3}\right)
    % &\vdots \nonumber \\
    % &= 1/2\pi k + 1/4\pi k^2
\end{align}
where the second equality is obtained using the same analysis as in the proof of Step 2, and the last inequality is due to \eqref{1990}. Next, by \eqref{odd} and the Taylor expansion of the error function around zero, we have
\begin{align}
    T_3 &\coloneqq  \E_{\w_\perp} \left[ b_1^2\right]\nonumber \\
    % &= \E_{\w_\perp} \left[ \left(\E_{\z}[\sigma'(\w_\perp^\top\z) z_1] \right)^2\right]  \nonumber \\
    &=\E_{\w_\perp} \left[ \left( \frac{1}{2} \erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right)\right)^2\right]  \nonumber \\
    &= \frac{1}{2 \pi}\E_{\w_\perp} \left[ \left(  \frac{w_{\perp,1}}{\|\w_{\perp,-1}\|_2} - \frac{w_{\perp,1}^3}{6\|\w_{\perp,-1}\|_2^3} + O\left(\frac{w_{\perp,1}^5}{\|\w_{\perp,-1}\|_2^5}\right) \right)^2\right] \nonumber \\
    &= \frac{1}{2 \pi}\E_{\w_\perp} \left[   \frac{w_{\perp,1}^2}{\|\w_{\perp,-1}\|_2^2} - \frac{w_{\perp,1}^4}{3\|\w_{\perp,-1}\|_2^4} + O\left(\frac{w_{\perp,1}^6}{\|\w_{\perp,-1}\|_2^6}\right)  \right] \nonumber \\
    &= \frac{1}{2 \pi}\left(   \frac{1}{k-r-3} - \frac{1}{(k-r-3)(k-r-5)} \right)  + O\left(\frac{1}{k^3}\right) 
\end{align}
where the last equality follows by properties of the Gaussian and chi-square distribution.

The most difficult term is $T_2$. We have
\begin{align}
    T_2 &:= 2\E_{\w_{\perp}}[a_1b_1] \nonumber \\
    &= 2\E_{\w_{\perp}}\left[ \E_{\vv}[\sigma'(\w_{\perp}^\top\vv) v_1] \erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right) \right]\nonumber \\ \nonumber \\
    &= 2\E_{\w_{\perp}}\left[\E_{\vv}[\sigma'(w_{\perp,1} v_1 +\w_{\perp,-1}^\top\vv_{-1}) v_1] \erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right) \right]\nonumber \\
    &= \E_{\w_{\perp}}\left[\E_{\vv_{-1}}[\sigma'(w_{\perp,1}  +\w_{\perp,-1}^\top\vv_{-1})- \sigma'(-w_{\perp,1}  +\w_{\perp,-1}^\top\vv_{-1})] \erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right) \right]\nonumber \\
    &= \E_{\w_{\perp}}\left[ \E_{\vv_{-1}}[\chi\{-w_{\perp,1} <\w_{\perp,-1}^\top\vv_{-1} <w_{\perp,1}\}]\erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right) \right]\nonumber \\
    &\quad - \E_{\w_{\perp}}\left[\E_{\vv_{-1}}[\chi\{w_{\perp,1} <\w_{\perp,-1}^\top\vv_{-1} <-w_{\perp,1}\}] \erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right) \right]\nonumber \\
    &= \E_{\w_{\perp}}\left[\E_{\vv_{-1}}[\chi\{-w_{\perp,1} <\w_{\perp,-1}^\top\vv_{-1} <w_{\perp,1}\}]\erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right)  \right]\label{odd2} \\
    &= 2\E_{\w_{\perp}}\left[ \E_{\vv_{-1}}[\chi\{-w_{\perp,1} <\w_{\perp,-1}^\top\vv_{-1} <0\}] \erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right)\right]
\end{align}
where \eqref{odd2} follows by the fact that the distribution of $-w_{\perp,1}$ is equivalent to the distribution of $w_{\perp,1}$, and the fact that the error function is an odd function ($f(-w) = -f(w)$). Next, since $\E_{\vv_{-1}}[\chi\{0<\w_{\perp,-1}^\top\vv_{-1} \}] = \frac{1}{2}$ for any $\w_{\perp,-1}$ and $\E_{\w_{\perp}}\left[\erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right) \frac{1}{2} \right] = 0$, we have
\begin{align}
    T_2 &= 2\E_{\w_{\perp}}\left[\E_{\vv_{-1}}[\chi\{-w_{\perp,1} <\w_{\perp,-1}^\top\vv_{-1} <0\} + \chi\{0<\w_{\perp,-1}^\top\vv_{-1} \}] \erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right) \right] \nonumber \\
    &=  2\E_{\w_{\perp}}\left[ \E_{\vv_{-1}}[\chi\{-w_{\perp,1} <\w_{\perp,-1}^\top\vv_{-1} \}] \erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right)\right] \nonumber \\
    &=  2\E_{\vv_{-1}}\left[\E_{\w_{\perp}}\left[\chi\{w_{\perp,1} +\w_{\perp,-1}^\top\vv_{-1}>0 \}\erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right)  \right]\right] \nonumber \\
    &=  2\E_{\w_{\perp}}\left[\chi\{w_{\perp,1} +\w_{\perp,-1}^\top \mathbf{1}_{k-r-1}>0 \} \erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right) \right] \nonumber 
\end{align}
where the last equality follows by the symmetry of the Gaussian distribution.
Next we use the fact that the norm and direction of an isotropic Gaussian random vector are independent:
\begin{align}
     T_2  &= 2\E_{w_{\perp,1},\frac{\w_{\perp,-1}}{\|\w_{\perp,-1}\|_2}, \|\w_{\perp,-1}\|_2}\left[\chi \left\{\frac{w_{\perp,1}}{\|\w_{\perp,-1}\|_2} +\frac{\w_{\perp,-1}^\top}{\|\w_{\perp,-1}\|_2} \mathbf{1}_{k-r-1}>0 \right\} \erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right) \right] \nonumber \\
     &= 2\E_{w_{\perp,1}, \|\w_{\perp,-1}\|_2}\left[\erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right) \E_{\frac{\w_{\perp,-1}}{\|\w_{\perp,-1}\|_2},}\left[\chi \left\{\frac{w_{\perp,1}}{\|\w_{\perp,-1}\|_2} +\frac{\w_{\perp,-1}^\top}{\|\w_{\perp,-1}\|_2} \mathbf{1}_{k-r-1}>0 \right\} \right]\right] \nonumber \\
     &= 2\E_{w_{\perp,1}, \|\w_{\perp,-1}\|_2}\left[\erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right) \Pr_{\boldsymbol{\mu}\sim \text{Unif}(\mathcal{S}^{k-r-2})}\left[ \boldsymbol{\mu}^\top \mathbf{1}_{k-r-1}>-\frac{w_{\perp,1}}{\|\w_{\perp,-1}\|_2}  \right]\right] 
\end{align}
where $\boldsymbol{\mu} \in \mathbb{R}^{k-r-1}$ is drawn uniformly from the unit hypersphere in $ \mathbb{R}^{k-r-1}$. By the rotation symmetry of the unit hypersphere around the origin, we have
\begin{align}
     T_2  
     &= 2\E_{w_{\perp,1}, \|\w_{\perp,-1}\|_2}\left[\erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right) \Pr_{\boldsymbol{\mu}\sim \text{Unif}(\mathcal{S}^{k-r-2})}\left[ \mu_1 >-\frac{w_{\perp,1}}{(\sqrt{k-r-1})\|\w_{\perp,-1}\|_2}  \right]\right] 
\end{align}
We can compute $\Pr_{\boldsymbol{\mu}\sim \text{Unif}(\mathcal{S}^{k-r-2})}\left[ \mu_1 >-\frac{w_{\perp,1}}{(\sqrt{k-r-1})\|\w_{\perp,-1}\|_2}  \right]$ using the CDF of one coordinate of a vector sampled from the unit hypersphere:
\begin{align}
    \Pr_{\boldsymbol{\mu}\sim \text{Unif}(\mathcal{S}^{k-r-2})}\left[ \mu_1 < \beta  \right] &= \frac{1}{Z} \int_{-1}^\beta (1- \mu_1^2)^{\frac{k-r-2}{2}-1} d\mu_1\nonumber \\
    &=\frac{1}{2} + \frac{1}{Z} \beta \; _2 F_1\left(\frac{1}{2},-\frac{k-r-3}{2};\frac{3}{2};\beta^2\right)
\end{align}
for any $\beta\in [-1,1]$, where $Z:= \int_{-1}^1 (1- \mu_1^2)^{\frac{k-r-2}{2}-1} d\mu_1 = \frac{\sqrt{\pi}\Gamma\left(\frac{k-r-2}{2}\right)}{\Gamma\left(\frac{k-r-1}{2}\right)}$ and $_2 F_1(a,b;c;d)$ is the hypergeometric function. Using the Taylor  series expansion of the hypergeometric function around zero, we obtain
\begin{align}
   &\Pr_{\boldsymbol{\mu}\sim \text{Unif}(\mathcal{S}^{k-r-2})}\left[ \mu_1 >-\frac{w_{\perp,1}}{(\sqrt{k-r-1})\|\w_{\perp,-1}\|_2}  \right]\nonumber \\
   &= \frac{1}{2} + \frac{\Gamma\left(\frac{k-r-1}{2}\right)}{\sqrt{\pi}\Gamma\left(\frac{k-r-2}{2}\right)} \frac{w_{\perp,1}}{\sqrt{k-r-1}\|\w_{\perp,-1}\|_2}\left( 1 - \frac{k-r-4}{6(k-r-1)} \frac{w_{\perp,1}^2}{\|\w_{\perp,-1}\|_2^2} + O\left(\frac{w_{\perp,1}^4}{\|\w_{\perp,-1}\|_2^4}\right) \right)
\end{align}
Combining this with the Taylor expansion of the error function, we have
\begin{align}
    T_2  &= 2\sqrt{2}\frac{\Gamma\left(\frac{k-r-1}{2}\right)}{{\pi}\sqrt{k-r-1}\Gamma\left(\frac{k-r-2}{2}\right)} \E_{w_{\perp,1}, \|\w_{\perp,-1}\|_2}\Bigg[\left( \frac{w_{\perp,1}}{\|\w_{\perp,-1}\|_2} -  \frac{w_{\perp,1}^3}{6\|\w_{\perp,-1}\|_2^3} + O\left( \frac{|w_{\perp,1}|^5}{\|\w_{\perp,-1}\|_2^5} \right)\right) \nonumber\\
    &\quad  \quad \quad \quad\quad \quad \quad \quad\quad \quad \quad \quad\quad \quad \quad \quad \times \left( \frac{w_{\perp,1}}{\|\w_{\perp,-1}\|_2} - \frac{k-r-4}{6(k-r-1)} \frac{w_{\perp,1}^3}{\|\w_{\perp,-1}\|_2^3} + O\left(\frac{|w_{\perp,1}|^5}{\|\w_{\perp,-1}\|_2^5}\right) \right)  \Bigg] \nonumber \\
    &= 2\sqrt{2}\frac{\Gamma\left(\frac{k-r-1}{2}\right)}{{\pi}\sqrt{k-r-1}\Gamma\left(\frac{k-r-2}{2}\right)} \E_{w_{\perp,1}, \|\w_{\perp,-1}\|_2}\Bigg[\left( \frac{w_{\perp,1}^2}{\|\w_{\perp,-1}\|_2^2} -  \frac{w_{\perp,1}^4}{3\|\w_{\perp,-1}\|_2^4} + O\left( \frac{|w_{\perp,1}|^6}{\|\w_{\perp,-1}\|_2^6} \right)\right) 
 \Bigg] \nonumber \\
    &= 2\sqrt{2}\frac{\Gamma\left(\frac{k-r-1}{2}\right)}{{\pi}\sqrt{k-r-1}\Gamma\left(\frac{k-r-2}{2}\right)} \left( \frac{1}{k-r-3} -  \frac{1}{(k-r-3)(k-r-5)} + O\left( \frac{1}{k^3} \right)\right) 
 \nonumber \\
\end{align}


Combining the above expressions for $T_1,T_2$, and $T_3$ via \eqref{3t} yields
\begin{align}
    \E_{\w_{\perp}}[(a_1-b_1)^2] &=  \frac{1}{2\pi}\left( \frac{1}{k-r} + \frac{1}{(k-r)^2}\right) + O\left(\frac{1}{(k-r)^3}\right) \nonumber \\
    &\quad + \frac{1}{2 \pi}\left(   \frac{1}{k-r-3} - \frac{1}{(k-r-3)(k-r-5)} \right)  + O\left(\frac{1}{k^3}\right)  \nonumber \\
    &\quad - 2  \nonumber\\
    &= O((k-r)^{-3})
\end{align}
As in the proof for Step 2, we leverage the above variance bound and invoke Chebyshev's Inequality and a union bound to obtain:
\begin{align}
    \Pr
\end{align}

{\color{blue}
Now that we have bounded the first and second moments of $f_1(\w)$, we can use Chebyshev's Inequality to write
\begin{align}
    \Pr_{\w}\left[|f_1(w)|\geq \frac{2^{r/2}crk^{1/2}}{C k^{3/2}}\right] \leq \frac{1}{2^r c^2 k}
\end{align} for some constants $c,C$.
Since each coordinate of $\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa =  \E_{\vv} \left[(\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} )- \sigma'( \mathbf{w}_{\perp}^\top\mathbf{v} )) \vv \right]$ is identically distributed, 
\begin{align}
    \Pr_{\w}\left[|f_i(w)|\geq \frac{2^{r/2}crk^{1/2}}{Ck^{3/2}}\right] \leq \frac{1}{2^r c^2 k}
\end{align} 
for all $i \in [k-r]$, where $f_i(\w):= \E_{\vv} \left[(\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} )- \sigma'( \mathbf{w}_{\perp}^\top\mathbf{v} )) v_i \right]$.
Thus, by a union bound over all coordinates, we have 
\begin{align}
   \Pr_{\w}\left[\left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa\right\|_2^2 \geq \frac{2^r c^2 r^2}{C^2 k} \right]& \leq \Pr_{\w}\left[\cup_{i=1}^{k-r} |f_i(w)|\geq \frac{2^{r/2} c r}{C k}\right] \nonumber \\ %\frac{c'rk^{1/2}}{k^{3/2}}
   &\leq \sum_{i=1}^{k-r} \Pr_{\w}\left[|f_i(w)|\geq \frac{ 2^{r/2} c rk^{1/2}}{C k^{3/2}}\right]\nonumber \\
   &\leq \frac{1}{2^{r} c^2} 
\end{align}
Finally we union bound over all $\mathbf{u}\in \uH^r$:
\begin{align}
    \Pr_{\w}\left[ \cup_{\mathbf{u} \in \mathcal{H}^r} \left\|\E_{\vv} \left[\sigma'( \mathbf{w}_{\parallel}^\top \mathbf{u} + \mathbf{w}_{\perp}^\top\mathbf{v} ) \mathbf{v} \right] - \aaa\right\|_2^2 \geq \frac{2^r c^2 r^2}{C^2 k} \right] \leq \frac{1}{c^2} 
\end{align}
Choose $c=100$ to complete the proof of this step.

}



    \item \textbf{Step 4: $\left\|\mathbf{A}^{\circ,\tilde{\mathcal{N}}}_{\perp,\perp} - \mathbf{A}^{\circ,{\mathcal{N}}}_{\perp,\perp}\right\|_2 = O(k^{-1/2})$ with constant probability.}
Let $\mathbf{c}:=\E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top\z) \z]$, thus $ \mathbf{A}^{\circ,{\mathcal{N}}}_{\perp,\perp} = 2^{-r} \mathbf{cc}^\top$. Recall $\mathbf{A}^{\circ,\tilde{\mathcal{N}}}_{\perp,\perp} = 2^{-r}\bbb\bbb^\top $ where $b_i:= \E_{v_i \sim \text{Unif}(\{-1,1\}),\z_{-1}\sim \mathcal{N}(\mathbf{0}_{k-r-1},\mathbf{I}_{k-r-1})}[\sigma'(w_{\perp,i} v_i + \w_{\perp,-i}^\top\z_{-1}) v_i]$ for all $i \in [k-r]$. 

By the same analysis in \eqref{186} bounding the difference between two symmetric outer products, we have
\begin{align}
    \left\|\mathbf{A}^{\circ,\tilde{\mathcal{N}}}_{\perp,\perp} - \mathbf{A}^{\circ,{\mathcal{N}}}_{\perp,\perp}\right\|_2 %\nonumber \\
    % &= \left\|\mathbf{bb}^\top - \E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top\z) \z]\E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top\z) \z]^\top\right\|_2 \nonumber \\
    % &\leq \|\mathbf{b}+ \E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top\z) \z]\|_2 \|\mathbf{b} - \E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top\z) \z]\|_2
    &\leq 2^{-r}\|\mathbf{b}+ \mathbf{c}\|_2 \|\mathbf{b} -\mathbf{c}\|_2
\end{align}
 
We again proceed by bounding the first coordinate of the the difference between the two relevant vectors, here ${b}_1 - c_1$.

 % $\mathbf{c}= \E_{\z\sim \mathcal{N}(\mathbf{0}_{k-r},\mathbf{I}_{k-r})}[\sigma'(\w_\perp^\top \z)\z]$. 

Using  \eqref{odd} and the Taylor expansion of the error function around zero, we obtain
\begin{align}
    b_1 &=  \frac{1}{2} \erf\left( \frac{w_{\perp,1}}{\sqrt{2}\|\w_{\perp,-1}\|_2} \right)  \nonumber \\
    &=  \frac{1}{\sqrt{2\pi}} \left( \frac{w_{\perp,1}}{\|\w_{\perp,-1}\|_2}  - \frac{w_{\perp,1}^3}{6\|\w_{\perp,-1}\|_2^3} + O\left( \left( \frac{w_{\perp,1}}{\|\w_{\perp,-1}\|_2} \right)^5 \right)  \right)  \nonumber \\
\end{align}

Also, from \eqref{halfnormal}, we have
\begin{align}
   {c}_1 = \frac{1}{\sqrt{2\pi}}\frac{w_{\perp,1}}{\|\w_\perp\|_2} 
\end{align}

Next, we have
\begin{align}
    \E_{\w_{\perp}} [b_1] =   \E_{\w_{\perp}} [c_1] = 0
\end{align}
    by symmetry of the Gaussian distribution around zero. Further,
 \begin{align}
    \E_{\w_{\perp}} [(b_1 - c_1)^2] &= \frac{1}{4\pi}\Bigg( \E_{\w_{\perp}} \left[ \frac{w_{\perp,1}^2}{\|\w_{\perp,-1}\|_2^2} - \frac{w_{\perp,1}^4}{3\|\w_{\perp,-1}\|_2^4} + O\left( \left( \frac{w_{\perp,1}}{\|\w_{\perp,-1}\|_2} \right)^6 \right) \right] + \E_{\w_{\perp}} \left[\frac{w_{\perp,1}^2}{\|\w_{\perp}\|_2^2}  \right] \nonumber \\
    &\quad - 2 \E_{\w_{\perp}} \left[\frac{w_{\perp,1}^2}{\|\w_{\perp,-1}\|_2\|\w_{\perp}\|_2} - \frac{w_{\perp,1}^4}{6\|\w_{\perp,-1}\|_2^3\|\w_{\perp}\|_2} + O\left( \left( \frac{w_{\perp,1}}{\|\w_{\perp,-1}\|_2} \right)^5  \right) \frac{w_{\perp,1}}{\|\w_{\perp}\|_2} \right]   \Bigg)\nonumber \\
    &= \frac{1}{4\pi}\Bigg( \frac{1}{k-r-3}  - \frac{1}{(k-r-3)(k-r-5)} +  O\left(\frac{1}{(k-r)^3}\right) + \E_{\w_{\perp}} \left[\frac{w_{\perp,1}^2}{\|\w_{\perp}\|_2^2}  \right] \nonumber \\
    &\quad - 2 \E_{\w_{\perp}} \left[\frac{w_{\perp,1}^2}{\|\w_{\perp,-1}\|_2\|\w_{\perp}\|_2} - \frac{w_{\perp,1}^4}{6\|\w_{\perp,-1}\|_2^3\|\w_{\perp}\|_2} + O\left( \left( \frac{w_{\perp,1}}{\|\w_{\perp,-1}\|_2} \right)^5  \right) \frac{w_{\perp,1}}{\|\w_{\perp}\|_2} \right]   \Bigg)\label{197}
\end{align}   
Note that
\begin{align}
    \E_{\w_{\perp}} \left[\frac{w_{\perp,1}^2}{\|\w_{\perp}\|_2^2} \right] = \E_{\w_{\perp}} \left[\frac{w_{\perp,2}^2}{\|\w_{\perp}\|_2^2} \right] = \hdots = \E_{\w_{\perp}} \left[\frac{w_{\perp,k-r}^2}{\|\w_{\perp}\|_2^2} \right] 
\end{align}
and 
\begin{align}
   \sum_{i=1}^{k-r} \E_{\w_{\perp}} \left[\frac{w_{\perp,i}^2}{\|\w_{\perp}\|_2^2} \right] =  \E_{\w_{\perp}} \left[\frac{\|\w_{\perp}\|_2^2}{\|\w_{\perp}\|_2^2} \right] = 1,
\end{align}
therefore 
\begin{align}
    \E_{\w_{\perp}} \left[\frac{w_{\perp,1}^2}{\|\w_{\perp}\|_2^2} \right] = \frac{1}{k-r}.
\end{align}

We also have $ \E_{\w_{\perp}} [\frac{w_{\perp,1}^2}{\|\w_{\perp,-1}\|_2\|\w_{\perp}\|_2}] = \frac{1}{k-r-1.5} $ {\color{red}***empirically, not sure yet how to prove. Let $a= w_{\perp,1}/\|\w_{\perp,-1}\|_2$ and $a= w_{\perp,1}/\|\w_{\perp,-1}\|_2$ It is equivalent to  showing $ 2E[1/ab] =  E[1/a^2] + E[1/b^2] + O(1/k^3)$, i.e. $E[(1/a-1/b)^2] = O(1/k^3)$. Note that the other terms in  \eqref{197} cancel with each other. Note also that $E[(1/a-1/b)/w_{\perp,1}] = O(1/k^{1.5})$. Finally, note that $1/a-1/b > 0$.***}








    
\end{itemize}

This completes the proof.

==> tmp.tex <==
First note that there are ${r}\choose{0}$ subsets of $[r]$ of size 0, ${r}\choose{1}$ subsets of $[r]$ of size 1, and so on, thus there are ${r\choose 0} + {r\choose 1} + \dots +  {r \choose r} = 2^r$ sparse parity tasks in total. Let $d_H(\mathbf{v}, \mathbf{v}') = \sum_{i=1}^r \chi\{\mathbf{v}_i \neq \mathbf{v}_i'\}$ be the Hamming distance between two Boolean vectors of length $r$.  If $d_H(\mathbf{v},\mathbf{v}') = 0$, then clearly  ${g}_{i}(\mathbf{v}) = {g}_{i}(\mathbf{v}')$ for all ${g}_{i} \in \mathcal{T}$. 


    On the other hand, if $d_H(\mathbf{v},\mathbf{v}') = \gamma$ for any $\gamma \in \{1,\dots, r\}$, then $\mathbf{v}$ and $\mathbf{v}'$ share the same values for $r - \gamma$ coordinates, so must share the same label on all sparse parity tasks on subsets of these coordinates, of which there are $2^{r - \gamma} = 2^{r - \gamma} {\gamma \choose 0}$. Next, there are $2^{r - \gamma}\times {\gamma \choose 1}$ sparse parity tasks on one coordinate on which $\mathbf{v}$ and $\mathbf{v}'$ differ and other coordinates on which $\mathbf{v}$ and $\mathbf{v}'$ agree. Since these tasks are sparse parities on a set of coordinates on which $\mathbf{v}$ and $\mathbf{v}'$ differ on an odd number of coordinates, $g_i(\mathbf{v}) \neq g_i(\mathbf{v}')$ for each of these $2^{r - \gamma}\times {\gamma \choose 1}$ tasks. Similarly, there are $2^{r - \gamma}\times {\gamma \choose 2}$ tasks on two coordinates on which $\mathbf{v}$ and $\mathbf{v}'$ differ, and since two is even, $g_i(\mathbf{v}) = g_i(\mathbf{v}')$ for all such tasks. 
    Extrapolating this argument, if $\gamma$ is even, then there are $2^{r - \gamma}({\gamma\choose 0} + {\gamma \choose 2} + \dots +  {\gamma \choose \gamma}) = 2^{r - \gamma} 2^{\gamma-1} = 2^{r-1}$ tasks for which $g_i(\mathbf{v}) = g_i(\mathbf{v}')$, and 
$2^{r - \gamma}({\gamma\choose 1} + {\gamma \choose 3} + \dots +  {\gamma \choose \gamma-1}) = 2^{r - \gamma} 2^{\gamma-1} = 2^{r-1}$ tasks for which $g_i(\mathbf{v}) \neq  g_i(\mathbf{v}')$. Likewise,  if $\gamma$ is odd, there are $2^{r - \gamma}({\gamma\choose 0} + {\gamma \choose 2} + \dots +  {\gamma \choose \gamma - 1})  = 2^{r-1}$ tasks for which $g_i(\mathbf{v}) = g_i(\mathbf{v}')$, and 
$2^{r - \gamma}({\gamma\choose 1} + {\gamma \choose 3} + \dots +  {\gamma \choose \gamma-1}) = 2^{r-1}$ tasks for which $g_i(\mathbf{v}) \neq  g_i(\mathbf{v}')$. 
